MetFI: Model-driven Fault Simulation Framework

Safety-critical designs need to ensure reliable operations under hostile conditions with a certain degree of confidence. The continuously higher complexity of these designs makes them more susceptible to the risk of failure. ISO26262 recommends fault injection as the proper technique to verify and measure the dependability of safety-critical designs. To cope with the complexity, a lot of effort and stringent verification flow is needed. Moreover, many fault injection tools offer only a limited degree of controllability. We propose MetaFI, a model-driven simulator-independent fault simulation framework that provides multi-purpose fault injection strategies such as Statistical Fault Injection, Direct Fault Injection, Exhaustive Fault Injection, and at the same time reduces manual efforts. The framework enables injection of Stuck-at faults, Single-Event Transient faults, Single-Event Upset faults as well as Timing faults. The fault simulation is performed at the Register Transfer Level (RTL) of a design, in which parts of the design targeted for fault simulation are represented with Gate-level (GL) granularity. MetaFI is scalable with a full System-on-Chip (SoC) design and to demonstrate the applicability of the framework, fault simulation was applied to various components of two different SoCs. One SoC is running the Dhrystone application and the other one is running a Fingerprint calculation application. A minimal effort of 2 persondays was required to run 38 various fault injection campaigns on both the designs. The framework provided significant data regarding failure rates of the components. Results concluded that Prefetcher, a component of the SoC processor, is more susceptible to failures than the other targeted components on both the SoCs, regardless of the running application.

==> include/references.tex <==
%---------------------------------------------------------------------------------------------------------------------
%Papers/Books (including own) related to modeling (Metamodeling/mda) and generation (RTL, property/assertion) techniques
%---------------------------------------------------------------------------------------------------------------------

@incollection{Mellor.etal-2002,
	title		={{Model-driven architecture}},
	author		={Mellor, Stephen J and Scott, Kendall and Uhl, Axel and Weise, Dirk},
	booktitle	={{Advances in Object-Oriented Information Systems}},
	pages		={ 290-297},
	year		={2002},
	publisher	={Springer}
}

@INPROCEEDINGS{Hangal.etal-2005, 
	author		={Sudheendra Hangal and Sridhar Narayanan and Naveen Chandra and Sandeep Chakravorty}, 
	booktitle	={{Proceedings 42nd Design Automation Conference, 2005.}}, 
	title		={{IODINE: a tool to automatically infer dynamic invariants for hardware designs}}, 
	year		={2005},  
	pages		={ 775-778}, 
	doi			={10.1109/DAC.2005.193920}, 
	ISSN		={0738-100X}, 
	month		={June},}

@article{Truyen-2006,
	author 		= {F. Truyen},
	title 		= {{The fast Guide to Model Driven Architecture}},
	note 		= {\url{http://www.omg.org/mda/mda_files/Cephas_MDA_Fast_Guide.pdf}},
	urldate 	= {2016-02-08},
	publisher 	= {Cephas Consulting Corp},
	year 		= {2006}
}

@Misc{Ecker.etal-2007,
	Title        = {{XML-Based Assertion Generation}},
	Author       = {Wolfgang Ecker and Volken Essen and Michael Hull and Thomas Steininger and Michael Veltan},
	note		 = "\url{https://www.design-reuse.com/articles/15487/xml-based-assertion-generation.html}",
	note 		 = "[Online: Accessed on 25.July.2019]"
}

@inproceedings{Rogin.etal-2008,
   author       = {Rogin, Frank and Klotz, Thomas and Fey, G\"{o}rschwin and Drechsler, Rolf and R\"{u}lke, Steffen},
   title        = {{Automatic Generation of Complex Properties for Hardware Designs}},
   booktitle    = {{Proceedings of the Conference on Design, Automation and Test in Europe}},
   series       = {DATE '08},
   year         = {2008},
   isbn         = {978-3-9810801-3-1},
   location     = {Munich, Germany},
   pages        = { 545-548},
   numpages     = {4},
   url          = {http://doi.acm.org/10.1145/1403375.1403506},
   doi          = {10.1145/1403375.1403506},
   acmid        = {1403506},
   publisher    = {ACM},
   address      = {New York, NY, USA},
}   

@INPROCEEDINGS{Vasudevan.etal-2010, 
	author      ={S. Vasudevan and D. Sheridan and S. Patel and D. Tcheng and B. Tuohy and D. Johnson}, 
	booktitle   ={DATE 2010}, 
	title       ={{GoldMine: Automatic assertion generation using data mining and static analysis}}, 
	year        ={2010}, 
	pages       ={ 626-629}, 
	doi         ={10.1109/DATE.2010.5457129}, 
	ISSN        ={1530-1591}, 
	month       ={March},}


@INPROCEEDINGS{Zhang.etal-2017, 
		author={T. Zhang and D. Saab and J. A. Abraham}, 
		booktitle={{2017 IEEE Computer Society Annual Symposium on VLSI (ISVLSI)}}, 
		title={{Automatic Assertion Generation for Simulation, Formal Verification and Emulation}},
		pages={ 471-476}, 
		doi={10.1109/ISVLSI.2017.88}, }


@Article{Lecomtea.etal-2011,
	author =       "S. Lecomtea and S. Guillouard and C. Moyb and P. Leray and P. Soulard",
	title =        "{{A co-design methodology based on model driven architecture for real time embedded systems}}",
	journal =      "Mathematical and Computer Modeling",
	volume =       "53",
	number =       "3-4",
	pages =        "pp. 471-484",
	year =         "2011 ",
	DOI =          {{10.1016/j.mcm.2010.03.035}}
} 

@inproceedings{Ecker.etal-2012,
	author = {Ecker, W and Velten, M and Zafari, L and Goyal, A},
	booktitle = {{MeCoES - Metamodelling and Code Generation for Embedded Systems: Workshop with ESWEEK}},
	editor = {Mueller, Wolfgang and Ecker, Wolfgang},
	title = {{Metamodeling and Code Generation -The Infineon Approach}},
}

@book{Arnouldus.etal-2012,
	author = {J. {Arnouldus} and M.V.D. {Brand} and A. {Serebrenik} and J.J {Brunekreef}},
	title = {{Code Generation with Templates}},
	year = {2012},
	isbn = {978-94-91216-56-5},
	edition = {1st},
	publisher = {Springer Science and Business Media},
	address = {Secaucus, NJ, USA},
}

@INPROCEEDINGS{Findenig.etal-2012,
  author={R. {Findenig} and T. {Leitner} and W. {Ecker}},
  booktitle={{2012 IEEE International High Level Design Validation and Test Workshop (HLDVT)}}, 
  title={{Single-source hardware modeling of different abstraction levels with State Charts}}, 
  year={2012},
  pages={ 41-48},}

@INPROCEDINGS{Bachrach.etal-2012, 
		author={J. {Bachrach} and H. {Vo} and B. {Richards} and Y. {Lee} and A. {Waterman} and R. {Avi {\^z}ienis} and J. {Wawrzynek} and K. {Asanovi {\^c}}}, 
		booktitle={{DAC Design Automation Conference 2012}}, 
		title={{Chisel: Constructing hardware in a Scala embedded language}}, 
		year={2012},
		pages={ 1212-1221}, 
		doi={10.1145/2228360.2228584}, 
		ISSN={0738-100X}, 
		month={June},}

@inproceedings{Ecker.etal-2014,
	author = {Ecker, Wolfgang and Velten, Michael and Zafari, Leily and Goyal, Ajay},
	biburl = {http://www.bibsonomy.org/bibtex/2fca77ddc52ecd7db753a51e362324206/dblp},
	booktitle = {DATE},
	editor = {Fettweis, Gerhard and Nebel, Wolfgang},
	ee = {http://dl.acm.org/citation.cfm?id=2617055},
	isbn = {978-3-9815370-2-4},
	pages = { 1-2},
	publisher = {European Design and Automation Association},
	title = {{The metamodeling approach to system level synthesis.}},
	year = 2014
}

@INPROCEEDINGS{Sheridan.etal-2014, 
	author={D. Sheridan and L. Liu and H. Kim and S. Vasudevan}, 
	booktitle={2014 27th International Conference on VLSI Design and 2014 13th International Conference on Embedded Systems}, 
	title={{A Coverage Guided Mining Approach for Automatic Generation of Succinct Assertions}}, 
	year={2014},
	pages={ 68-73}, 
	doi={10.1109/VLSID.2014.19}, 
	ISSN={1063-9667}, 
	month={Jan},}

@INPROCEEDINGS{Kayed.etal-2014, 
		author={M. O. Kayed and M. Abdelsalam and R. Guindi}, 
		booktitle={{2014 15th International Microprocessor Test and Verification Workshop}}, 
		title={{A Novel Approach for SVA Generation of DDR Memory Protocols Based on TDML}}, 
		year={2014}, 
		pages={ 61-66}, 
		doi={10.1109/MTV.2014.15}, 
		ISSN={1550-4093}, 
		month={Dec},}

@INPROCEEDINGS{Ecker-Velten.etal-2014, 
	author={W. {Ecker} and M. {Velten} and L. {Zafari} and A. {Goyal}}, 
	booktitle={{2014 51st ACM/EDAC/IEEE Design Automation Conference}}, 
	title={{Metasynthesis for Designing Automotive SoCs}}, 
	year={2014}, 
	ISSN={0738-100X}, 
	month={June},}

@online{Siegel-2014,
	author =       "Jon M. Siegel",
	year =         "2014",
	title =        "Model Driven Architecture  \textsuperscript{\textregistered} (MDA): The MDA Guide Rev 2.0 ",
	note =          {\url{https://www.omg.org/mda/presentations.htm}},
	month =        {june},
	lastaccessed = "02.April.2019",
}

@INPROCEEDINGS{Danese.etal-2015, 
		author={A. Danese and T. Ghasempouri and G. Pravadelli}, 
		booktitle={2015 Design, Automation Test in Europe Conference Exhibition (DATE)}, 
		title={{Automatic extraction of assertions from execution traces of behavioural models}},
		pages={ 67-72}, 
		doi={10.7873/DATE.2015.0110}, 
		ISSN={1530-1591}, 
	}

@online{OMG-2016,
	author = {"OMG"},
	title = {{MDA - The Architecture of Choice for a Changing World}},
	year      = {2016},  
	note = {\url{http://www.omg.org/mda/}},
	urldate = {2016-02-08}}

@online{Liangora-2016,
	author 	= {Liangora Research Lab},
	title 	= {{What is MDA? Why considering BNPM}},
	note	= {\url{https://research.linagora.com/pages/viewpage.action?pageId=3639295}},
	urldate = {2016-04-25}
}

@inproceedings{Schreiner.etal-2016,
	author    = {J. Schreiner and	R. Findenig and	W. Ecker},
	title     = {{Design Centric Modeling of Digital Hardware}},
	booktitle = {{IEEE} International High Level Design Validation and Test Workshop, {HLDVT} 2016},
	pages     = { 46--52},
	year      = {2016}
}

@INPROCEEDINGS{Ecker.etal-2016, 
	author={W. Ecker and J. Schreiner}, 
	booktitle={{2016 IFIP/IEEE International Conference on Very Large Scale Integration (VLSI-SoC)}}, 
	title={Introducing Model-of-Things (MoT) and Model-of-Design (MoD) for simpler and more efficient hardware generators}, 
	year={2016}, 
	pages={ 1-6}, 
	doi={10.1109/VLSI-SoC.2016.7753576}, 
	month={Sept},
}

@inproceedings{Urdahl.etal-2016,
		author = {J. Urdahl and S. Udupi and T. Ludwig and D. Stoffel and W. Kunz},
		title = {{Properties First? A New Design Methodology for Hardware, and Its Perspectives in Safety Analysis}},
		booktitle = {Proceedings of the 35th International Conference on Computer-Aided Design},
		series = {ICCAD '16},
		year = {2016},
		isbn = {978-1-4503-4466-1},
		location = {Austin, Texas},
		pages = { 84:1--84:8},
		url = {http://doi.acm.org/10.1145/2966986.2980086},
		doi = {10.1145/2966986.2980086},
		acmid = {2980086},
		publisher = {ACM},
} 


@inproceedings{Schreiner.etal-2017,
	author = {J. Schreiner and F. Willgerodt and W. Ecker},
	title = {A New Approach for Generating View Generators},
	booktitle = {Design and Verification Conference - US},
	Year = {2017},
	Month = {Feb},
	note  ={\url{http://events.dvcon.org/2017/proceedings/papers/04P_18.pdf}},
} 

@incollection{Ecker.etal-2017,
	author      = "W. Ecker and J. Schreiner",
	title       = "Metamodeling",
	editor      = "Ha, Soonhoi and Teich, Jürgen ",
	booktitle   = "Handbook of Hardware/Software Codesign",
	publisher   = "Springer",
	year        = 2017,
	pages       = "266-290",
	chapter     = 10,
}

@INPROCEEDINGS{Devarajegowda-Ecker-2017,
	author		={K. {Devarajegowda} and W. {Ecker}},
	booktitle	={{2017 IEEE International High Level Design Validation and Test Workshop (HLDVT)}},
	title		={On generation of properties from specification},
	year		={2017},
	pages		={ 95-98},
	doi			={10.1109/HLDVT.2017.8167470},
	ISSN		={2471-7827},
	month		={Oct},}

@INPROCEEDINGS{Devarajegowda.etal-2017,
	author		={K. {Devarajegowda} and J. {Schreiner} and R. {Findenig} and W. {Ecker}},
	booktitle	={{2017 IEEE/ACM ICCAD}},
	title		={{Python Based Framework for HDSLs with an Underlying Formal Semantics}},
	year		={2017},
	pages		={ 1019-1025},
	doi			={10.1109/ICCAD.2017.8203893},
	ISSN		={1558-2434},
	month       ={Nov},
}

@INPROCEEDINGS{Devarajegowda-Schreiner.etal-2018,
	author	    = {K. {Devarajegowda}, and J. {Schreiner} and W. {Ecker}},
	title 	    = {Synthesis of Decoder Tables using Formal Verification Tools},
	booktitle   = {Design and Verification Conference - US (DVCon-US)},
	Year 	    = {2018},
	Month 	    = {February},
	Url         = {http://events.dvcon.org/2018/proceedings}
} 

@INPROCEEDINGS{Devarajegowda-Ecker-2018,
	author		={K. {Devarajegowda} and W. {Ecker}},
	booktitle	={{2018 IFIP/IEEE Intl. Conf. on Very Large Scale Integration (VLSI-SoC)}},
	title		={{Meta-model Based Automation of Properties for Pre-Silicon Verification}},
	year		={2018},
	pages		={ 231-236},
	doi			={10.1109/VLSI-SoC.2018.8644957},
	ISSN		={2324-8432},
	month		={Oct},}

@INPROCEEDINGS{Ecker-Devarajegowda.etal-2019,
	author		={W. {Ecker} and K. {Devarajegowda} and M. {Werner} and Z. {Han} and L. {Servadei}},
	booktitle	={2019 Design, Automation Test in Europe Conference Exhibition (DATE)},
	title		={Embedded Systems' Automation following OMG's Model Driven Architecture Vision},
	year		={2019},
	pages		={ 1301-1306},
	doi			={10.23919/DATE.2019.8715154},
	ISSN		={1530-1591},
	month		={March},
}

@INPROCEEDINGS{Devarajegowda.etal-2019,
	author		={K. {Devarajegowda} and W. {Ecker} and W. {Kunz}},
	booktitle	={MBMV 2019; 22nd Workshop - Methods and Description Languages for Modelling and Verification of Circuits and Systems},
	title		={How to Keep 4-Eyes Principle in a Design and Property Generation Flow},
	year		={2019},
	pages		={ 1-6},
	month		={April},
}	

@INPROCEEDINGS{Devarajegowda-Servadei.etal-2019,
	author		={K. {Devarajegowda} and L. {Servadei} and Z. {Han} and M. {Werner} and W. {Ecker}},
	booktitle	={2019 22nd Euromicro Conference on Digital System Design (DSD)},
	title		={Formal Verification Methodology in an Industrial Setup},
	year		={2019},
	pages		={ 610-614},
	doi			={10.1109/DSD.2019.00094},
	ISSN		={null},
	month		={Aug},
}


@INPROCEEDINGS{Han-Devarajegowda.etal-2019,
	author		={Z. {Han} and K. {Devarajegowda} and M. {Werner} and W. {Ecker}},
	booktitle	={{2019 IEEE Nordic Circuits and Systems Conference (NORCAS): NORCHIP and International Symposium of System-on-Chip (SoC)}},
	title		={Towards a Python-Based One Language Ecosystem for Embedded Systems Automation},
	year		={2019},
	pages		={ 1-7},
	keywords	={Domain-Specific Language Generation;Metamodeling;Design Automation},
	doi			={10.1109/NORCHIP.2019.8906949},
	ISSN		={null},
	month		={Oct},
}

@ARTICLE{Ludwig.etal-2019,
  author={T. {Ludwig} and J. {Urdahl} and D. {Stoffel} and W. {Kunz}},
  journal={{IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems}}, 
  title={Properties First - Correct-By-Construction RTL Design in System-Level Design Flows}, 
  year={2019},
 }

@INPROCEEDINGS{Zhao-Harris-2019,
  author={J. {Zhao} and I. G. {Harris}},
  booktitle={2019 Design, Automation   Test in Europe Conference   Exhibition (DATE)}, 
  title={Automatic Assertion Generation from Natural Language Specifications Using Subtree Analysis}, 
  year={2019},
  pages={ 598-601},}

@INPROCEEDINGS{Bavache.etal-2020,
	author={V. B. {Bavache} and H. {Zhao} and H. {Hartliehe} and E. 
				{Kaja} and K. {Devarajegowda} and W. {Ecker}},
	booktitle={2020 Baltic Electronics Conference)}, 
	title={Automated SoC Hardening with Model Transformation}, 
	year={2020},}


%---------------------------------------------------------------------------------------------------------------------
%Papers/Journals/Books  on (Formal) Verification
%---------------------------------------------------------------------------------------------------------------------

  @article{DPLL-1960,
	author = {Davis, Martin and Putnam, Hilary},
	title = {{A Computing Procedure for Quantification Theory}},
	year = {1960},
	issue_date = {July 1960},
	publisher = {Association for Computing Machinery},
	address = {New York, NY, USA},
	volume = {7},
	number = {3},
	issn = {0004-5411},
	url = {https://doi.org/10.1145/321033.321034},
	doi = {10.1145/321033.321034},
	journal = {J. ACM},
	month = jul,
	pages = { 201-215},}

@article{Kripke-1963, 
	title={{Semantical considerations for modal logics. Proceedings of a Colloquium on Modal and Many-valued Logics, Helsinki, 23-26 August, 1962, Acta Philosophica Fennica1963}}, 
	volume={34}, DOI={10.2307/2270922}, 
	number={3}, 
	journal={Journal of Symbolic Logic}, 
	publisher={Cambridge University Press}, 
	author={Saul A. Kripke},
	year={1969},}


@ARTICLE{Lawrence.etal-1988,
	author = {Lawrence C. Paulson},
	title = {{Isabelle: The next seven hundred theorem provers}},
	journal = {In Ewing L. Lusk and Ross A. Overbeek, editors, 9th International Conference on Automated Deduction, volume 310 of LNCS},
	year = {1988},
	volume = {23},
	pages = { 772-773}
}

@article{Jeroslow-Jinchang-1990,
	title={{Solving propositional satisfiability problems}},
	author={Robert G. Jeroslow and Jinchang Wang},
	journal={Annals of Mathematics and Artificial Intelligence},
	year={1990},
	volume={1},
	pages={167-187}
}

@inproceedings{Emerson-1990,
	title={{Temporal and Modal Logic}},
	author={E. Allen Emerson},
	booktitle={{Handbook of Theoretical Computer Science, Volume B: Formal Models and Sematics}},
	year={1990}
}

@inproceedings{Kinniment.etal-1992,
	author    = {D. J. Kinniment and Albert Koelmans},
	editor    = {Victoria Stavridou and Thomas F. Melham and Raymond T. Boute},
	title     = {{Modelling and Verification of Timing Conditions with the Boyer Moore
	Prover}},
	booktitle = {Theorem Provers in Circuit Design, Proceedings of the {IFIP} {TC10/WG}
	10.2 International Conference on Theorem Provers in Circuit Design:
	Theory, Practice and Experience, Nijmegen, The Netherlands, 22-24
	June 1992, Proceedings},
	series    = {{IFIP} Transactions},
	volume    = {{A-10}},
	pages     = {ßß. 111--127},
	publisher = {North-Holland},
	year      = {1992},
}
@inproceedings{Owre.etal-1992,
	AUTHOR = {{S.} Owre and {J.} {M.} Rushby and and {N.} Shankar},
	TITLE = {{PVS:} {A} Prototype Verification System},
	BOOKTITLE = {11th International Conference on Automated Deduction (CADE)},
	YEAR = {1992},
	EDITOR = {Deepak Kapur},
	SERIES = {Lecture Notes in Artificial Intelligence},
	VOLUME = {607},
	PAGES = {748--752},
	ADDRESS = {Saratoga, {NY}},
	MONTH = {jun},
	PUBLISHER = {Springer-Verlag},
	URL = {http://www.csl.sri.com/papers/cade92-pvs/}
}

@Book{McMillan-1993,
	Title                    = {Symbolic Model Checking},
	Author                   = {K. L. McMillan},
	Publisher                = {Kluwer Academic Publishers},
	Year                     = {1993},
	
	Address                  = {Boston}
}

@inprocedings{Burch.etal-1994,
		author = {Burch, Jerry R. and Dill, David L.},
		title = {Automatic Verification of Pipelined Microprocessor Control},
		booktitle = {Proceedings of the 6th International Conference on Computer Aided Verification},
		series = {CAV '94},
		year = {1994},
		isbn = {3-540-58179-0},
		pages = {68--80},
		numpages = {13},
		acmid = {735662},
		publisher = {Springer-Verlag},
		address = {London, UK, UK},
	}

@InProceedings{Pierre-1995,
	author="Pierre, Laurence",
	editor="Camurati, Paolo E.
	and Eveking, Hans",
	title="Describing and verifying synchronous circuits with the Boyer-Moore theorem prover",
	booktitle="Correct Hardware Design and Verification Methods",
	year="1995",
	publisher="Springer Berlin Heidelberg",
	address="Berlin, Heidelberg",
	pages="35--55",
	isbn="978-3-540-45516-5"
}

@inprocedings{Jones.etal-1995,
		author = {Jones, Robert B. and Dill, David L. and Burch, Jerry R.},
		title = {Efficient Validity Checking for Processor Verification},
		booktitle = {{Proceedings of the 1995 IEEE/ACM International Conference on Computer-aided Design}},
		series = {ICCAD '95},
		year = {1995},
		isbn = {0-8186-7213-7},
		location = {San Jose, California, USA},
		pages = {2--6},
		numpages = {5},
		acmid = {224849},
		address = {Washington, DC, USA},
		keywords = {decision procedure, formal verification, microprocessor architecture, uninterpreted functions, validation},
	}

@inproceedings{Barth-1995,
	title={A Davis-Putnam based enumeration algorithm for linear pseudo-Boolean optimization},
	author={Peter Barth},
	year={1995}
}

@ARTICLE{Smith-Sohli-1995,
	author={J. E. {Smith} and G. S. {Sohi}},
	journal={{Proceedings of the IEEE}}, 
	title={The microarchitecture of superscalar processors}, 
	year={1995},
	volume={83},
	number={12},
	pages={1609-1624},}

@INPROCEEDINGS{Swamy-1997, 
	author={G. Swamy}, 
	booktitle={VLSI Design, 1997. Proceedings., Tenth International Conference on}, 
	title={Formal verification of digital systems}, 
	year={1997}, 
	pages={213-217}, 
	keywords={digital systems;finite state machines;formal verification;logic design;automated decision;design;digital system;equivalence checking;finite state machine;formal verification;hardware;language containment;logical system;model checking;Art;Automata;Circuit simulation;Design methodology;Digital systems;Formal verification;Graphics;Hardware;Laboratories;Sequential circuits}, 
	doi={10.1109/ICVD.1997.568078}, 
	ISSN={1063-9667}, 
	month={Jan},}


@ARTICLE{Kaufmann.etal-1997,
	author = {Matt Kaufmann and J. Strother Moore and Of Boyer},
	title = {An Industrial Strength Theorem Prover for a Logic Based on Common Lisp},
	journal = {IEEE Transactions on Software Engineering},
	year = {1997},
	volume = {23},
	pages = {203--213}
}


@inprocedings{Damm.etal-1998,
		author = {Damm, Werner and Pnueli, Amir and Ruah, Sitvanit},
		title = {Herbrand Automata for Hardware Verification},
		booktitle = {Proceedings of the 9th International Conference on Concurrency Theory},
		series = {CONCUR '98},
		year = {1998},
		isbn = {3-540-64896-8},
		pages = {67--83},
		numpages = {17},
		acmid = {701323},
		publisher = {Springer-Verlag},
		address = {Berlin, Heidelberg},
	}

@inprocedings{Berezin.etal-1998,
		author = {Berezin, S. and Biere, A. and Clarke, E. M. and Zhu, Y.},
		title = {Combining Symbolic Model Checking with Uninterpreted Functions for Out-of-Order Processor Verification},
		booktitle = {Proceedings of the Second International Conference on Formal Methods in Computer-Aided Design},
		series = {FMCAD '98},
		isbn = {3-540-65191-8},
		pages = {369--386},
		numpages = {18},
		acmid = {683063},
		publisher = {Springer-Verlag},
		address = {London, UK},
	}

@InProceedings{Emerson.etal-1999,
	Title                    = {Parametric Quantitative Temporal Reasoning},
	Author                   = {Emerson, E.A. and Trefler, R.J.},
	Booktitle                = {Logic in Computer Science, 1999. Proceedings. 14th Symposium on},
	Year                     = {1999},
	Pages                    = {336 -343},
	
	Doi                      = {10.1109/LICS.1999.782628},
	File                     = {:./files/1999-EmersonTrefler.pdf:PDF},
}



@book{Kropf-1999,
	author = {T. {Kropf}},
	title = {{Introduction to Formal Hardware Verification: Methods and Tools for Designing Correct Circuits and Systems}},
	year = {1999},
	isbn = {3540654453},
	edition = {1st},
	publisher = {Springer-Verlag New York, Inc.},
	address = {Secaucus, NJ, USA},
}

@article{Clarke.etal-1999,
	author = {Clarke, Edmund M. and Grumberg, Orna and Long, David E.},
	title = {Model Checking and Abstraction},
	year = {1994},
	issue_date = {September 1994},
	publisher = {Association for Computing Machinery},
	address = {New York, NY, USA},
	volume = {16},
	number = {5},
	issn = {0164-0925},
	url = {https://doi.org/10.1145/186025.186051},
	doi = {10.1145/186025.186051},
	journal = {ACM Trans. Program. Lang. Syst.},
	month = sep,
	pages = {1512-1542},
	numpages = {31},
	keywords = {abstract interpretation, temporal logic, model checking, binary decision diagrams (BDDs)}
}


@InProceedings{Uribe-2000,
	author="Uribe, Tom{\'a}s E.",
	editor="Kirchner, H{\'e}l{\`e}ne
	and Ringeissen, Christophe",
	title="Combinations of Model Checking and Theorem Proving",
	booktitle="Frontiers of Combining Systems",
	year="2000",
	publisher="Springer Berlin Heidelberg",
	address="Berlin, Heidelberg",
	pages="151--170",
	isbn="978-3-540-46421-1"
}


@ARTICLE{Clarke.etal-2001,
	author={E. {Clarke} and A. {Biere} and R. {Raimi} and Y. {Zhu}},
	title={{Bounded Model Checking Using Satisfiability Solving}},
	journal={Formal Methods in System Design},
	year={2001},
	month={July},
	day={01},
	volume={19},
	number={1},
	issn={1572-8102},
	doi={10.1023/A:1011276507260},
	url={https://doi.org/10.1023/A:1011276507260},
}

@InProceedings{RufHoffmann.etal-2001,
	Title                    = {Simulation-Guided Property Checking Based on Multi-Valued AR-Automata},
	Author                   = {JuErgen Ruf and Dirk W. Hoffmann and Thomas Kropf and Wolfgang Rosenstiel},
	Booktitle                = {Proc. International Conference on Design, Automation and Test in Europe ({DATE})},
	Year                     = {2001},
	Pages                    = {742 -748},
	
	Doi                      = {10.1109/DATE.2001.915111},
	File                     = {:./files/2001-RufHoffmann.etal.pdf:PDF},
	Timestamp                = {2006.09.21}
}

@INPROCEEDINGS{Roy.etal-2002,
	author={S. K. {Roy} and S. {Ramesh}},
	booktitle={Proceedings of ASP-DAC/VLSI Design 2002. 7th Asia and South Pacific Design Automation Conference and 15h International Conference on VLSI Design}, 
	title={Functional verification of system on chips - practices, issues and challenges}, 
	year={2002},
	volume={},
	number={},
	pages={11-13},}

@INPROCEEDINGS{Wedler.etal-2004,
	author={M. {Wedler} and D. {Stoffel} and W. {Kunz}},
	booktitle={Proceedings Design, Automation and Test in Europe Conference and Exhibition},
	title={{Arithmetic Reasoning in DPLL-based SAT Solving}},
	year={2004},
	volume={1},
	number={},
	pages={30-35 Vol.1},
	doi={10.1109/DATE.2004.1268823},
	ISSN={},
	month={Feb},}

@Inbook{Iman.etal-2004,
	title="e Reuse Methodology",
	bookTitle="The e Hardware Verification Language",
	year="2004",
	author ={S. {Iman} and S. {Joshi}},
	publisher="Springer US",
	address="Boston, MA",
	pages="267--278",
	isbn="978-1-4020-8024-1",
	doi="10.1007/1-4020-8024-7_15",
	url="https://doi.org/10.1007/1-4020-8024-7_15"
}
@INPROCEEDINGS{Ecker.etal-2004,
		author    = {W. {Ecker} and V. {Esen} and T. {Steininger} and M. {Zambaldi}},
		title     = {Memory Models for the Formal Verification of Assembler Code Using Bounded Model Checking},
		booktitle = {{7th IEEE International Symposium on Object-Oriented Real-Time Distributed Computing (ISORC} 2004), 12-14 May 2004, Vienna, Austria}},
		pages     = {129--135},
		year      = {2004},
		biburl    = {http://dblp.org/rec/bib/conf/isorc/EckerESZ04},
		bibsource = {dblp computer science bibliography, http://dblp.org},
	}

@misc{Bormann-Busch-2005,
	author =       {J. {Bormann} and H. {Busch}},
	year =         "2005",
	month =        sep,
	title =        {Verfahren zur Bestimmung der G\"ute einer Menge von Eigenschaften (Method for determining the quality of a set of properties). European Patent Application, Publication Number EP1764715},
}

@article{Nieuwenhuis.etal-2006,
	title={Solving SAT and SAT Modulo Theories: From an abstract Davis--Putnam--Logemann--Loveland procedure to DPLL(T)},
	author={Robert Nieuwenhuis and Albert Oliveras and Cesare Tinelli},
	journal={J. ACM},
	year={2006},
	volume={53},
	pages={937-977}
}

@INPROCEEDINGS{Borman-Beyer.etal-2007, 
	author={J. {Bormann} and S. {Beyer} and A. {Maggiore} and M. {Siegel} and S. {Skalberg} and T. {Blackmore} and F. {Bruno}}, 
	title={{Complete Formal Verification of TriCore2 and other Processors}}, 
	booktitle = {Proceedings of DVCon-US},
	year = {2007},
}

@INPROCEEDINGS{Claessen-2007,
	author = {Koen Claessen},
	title = {A Coverage Analysis for Safety Property Lists},
	booktitle = {Proc. International Conference on Formal Methods in Computer-Aided
	Design ({FMCAD})},
	year = {2007},
	pages = {139-145},
	publisher = {{IEEE Computer Society}},
	file = {:./files/2007-Claessen.pdf:PDF},
	isbn = {0-7695-3023-0}
}

@ARTICLE{Wedler.etal-2007,
	author={M. {Wedler} and D. {Stoffel} and R. {Brinkmann} and W. {Kunz}},
	journal={{IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems}},
	title={A Normalization Method for Arithmetic Data-Path Verification}, 
	year={2007},
	volume={26},
	number={11},
	pages={1909-1922},}

@ARTICLE{Bhadra.etal-2007,
	author={J. {Bhadra} and M. S. {Abadir} and L. {Wang} and S. {Ray}},
	journal={{IEEE Design   Test of Computers}}, 
	title={A Survey of Hybrid Techniques for Functional Verification}, 
	year={2007},
	volume={24},
	pages={pp. 112-122},}

@ARTICLE{Nguyen.etal-2008,
	author={M. D. {Nguyen} and M. {Thalmaier} and M. {Wedler} and J. {Bormann} and D. {Stoffel} and W. {Kunz}},
	journal={{IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems}},
	title={{Unbounded Protocol Compliance Verification Using Interval Property Checking With Invariants}},
	year={2008},
	volume={27},
	pages={2068-2082},
	doi={10.1109/TCAD.2008.2006092},
}

@INPROCEEDINGS{Bofill.etal-2008,
	author={M. {Bofill} and R. {Nieuwenhuis} and A. {Oliveras} and E. {Rodriguez-Carbonell} and A. {Rubio}},
	booktitle={2008 Formal Methods in Computer-Aided Design}, 
	title={A Write-Based Solver for SAT Modulo the Theory of Arrays}, 
	year={2008},
	volume={},
	number={},
	pages={1-8},}

@book{Glasser-2009,
	author = {M. Glasser},
	title = {Open Verification Methodology Cookbook},
	year = {2009},
	publisher = {Springer Science \& Business Media},
	ISBN = {9781441909671},}

@INPROCEEDINGS{Urdahl.etal-2010,
	author={J. {Urdahl} and D. {Stoffel} and J. {Bormann} and M. {Wedler} and W. {Kunz}},
	booktitle={Formal Methods in Computer Aided Design},
	title={Path predicate abstraction by complete interval property checking},
	year={2010},
	pages={207-215},
	keywords={formal verification;path predicate abstraction;complete interval property checking;C-IPC;global system property;Concrete;System-on-a-chip;Safety;Input variables;Computational modeling;Integrated circuit modeling;Encoding},
	doi={},
	ISSN={null},
	month={Oct},}

  @inproceedings{Thalmaier.etal-2010,
	author = {Thalmaier, Max and Nguyen, Minh D. and Wedler, Markus and Stoffel, Dominik and Bormann, J\"{o}rg and Kunz, Wolfgang},
	title = {Analyzing K-Step Induction to Compute Invariants for SAT-Based Property Checking},
	year = {2010},
	isbn = {9781450300025},
	publisher = {Association for Computing Machinery},
	address = {New York, NY, USA},
	url = {https://doi.org/10.1145/1837274.1837319},
	doi = {10.1145/1837274.1837319},
	booktitle = {Proceedings of the 47th Design Automation Conference},
	pages = {176-181},
	numpages = {6},
	keywords = {invariants, k-step induction, IPC, symbolic traversal},
	location = {Anaheim, California},
	series = {DAC'10}
}

@INPROCEEDINGS{Een.etal-2011,
	author={N. {Een} and A. {Mishchenko} and R. {Brayton}},
	booktitle={2011 Formal Methods in Computer-Aided Design (FMCAD)}, 
	title={Efficient implementation of property directed reachability}, 
	year={2011},
	pages={125-134},}

@article{Kamkin.etal-2011,
	author = {Kamkin, A. S. and Chupilko, M. M.},
	title = {Survey of Modern Technologies of Simulation-Based Verification of Hardware},
	year = {2011},
	issue_date = {May 2011},
	publisher = {Plenum Press},
	address = {USA},
	volume = {37},
	number = {3},
	issn = {0361-7688},
	url = {https://doi.org/10.1134/S0361768811030017},
	doi = {10.1134/S0361768811030017},
	journal = {Program. Comput. Softw.},
	month = may,
	pages = {147-152},
	numpages = {6}
}

@INPROCEEDINGS{Lvov.etal-2012,
	author={A. {Lvov} and L. A. {Lastras-Montaño} and V. {Paruthi} and R. {Shadowen} and A. {El-Zein}},
	booktitle={2012 Formal Methods in Computer-Aided Design (FMCAD)},
	title={{Formal Verification of Error Correcting Circuits Using Computational Algebraic Geometry}},
	year={2012},
	pages={141-148},
	month={Oct},}

@INPROCEEDINGS{Marx.etal-2013,
	author={O. {Marx} and M. {Wedler} and D. {Stoffel} and W. {Kunz} and A. {Dreyer}},
	booktitle={{2013 IEEE/ACM International Conference on Computer-Aided Design (ICCAD)}}, 
	title={Proof logging for computer algebra based SMT solving}, 
	year={2013},
	pages={677-684},}

@INPROCEEDINGS{Hanna-2014,
	author={Z. {Hanna}},
	booktitle={2014 Formal Methods in Computer-Aided Design (FMCAD)}, 
	title={Challenging problems in industrial formal verification}, 
	year={2014},
	pages={1-1},}

@misc{Kunz-2015,
	author = {Wolfgang Kunz},
	title = {{Verification Of Digital Systems}},
	howpublished = {University lecture},
	organization = {EIT, TUKL, Kaiserslautern},
	location = {TU Kaiserslautern},
	month = {October 2014 - February 2015},
	note = "[Lecture notes - VDS, from Prof. Wolfgang Kunz at TU Kaiserslautern]"}

@book{Seligman.etal-2015,
	author = {Erik Seligman and Tom Schubert and M V Achutha Kiran kumar},
	title = {Formal Verification, An Essential Toolkit For Modern VLSI Design},
	year = {2015},
	publisher = {Morgan Kaufmann Publishers},
	isbn = {978-0-12-800727-3},}

@INPROCEEDINGS{Foster-2015,
	author={H. D. {Foster}},
	booktitle={{52nd ACM/EDAC/IEEE Design Automation Conf.}}, 
	title={{Trends in functional verification: A 2014 industry study}}, 
	year={2015},
	pages={1-6},}

@INPROCEDINGS{Urdahl.etal-2016, 
		author={J. {Urdahl} and S. {Udupi} and T. {Ludwig} and D. {Stoffel} and W. {Kunz}}, 
		booktitle={{2016 IEEE/ACM International Conference on Computer-Aided Design (ICCAD)}}, 
		title={Properties first? A new design methodology for hardware, and its perspectives in safety analysis}, 
		year={2016}, 
		pages={1-8}, 
		doi={10.1145/2966986.2980086}, 
		ISSN={1558-2434}, 
		month={Nov},}

@CONFERENCE{Baranowaski-Trunzer-2016,
	author = {R. {Baranowski} and M. {Trunzer}},
	title = {{Complete Formal Verification of a Family of Automotive DSPs}},
	booktitle = {Proceedings of {DVCon-EU}},
	year = {2016}}           


@ARTICLE{Chen.etal-2017,
	author={W. {Chen} and S. {Ray} and J. {Bhadra} and M. {Abadir} and L. {Wang}},
	journal={{IEEE Design   Test}},
	title={{Challenges and Trends in Modern SoC Design Verification}}, 
	year={2017},}

@INPROCEEDINGS{Ho.etal-2017,
	author={Y. {Ho} and A. {Mishchenko} and R. {Brayton}},
	booktitle={2017 Formal Methods in Computer Aided Design (FMCAD)}, 
	title={Property directed reachability with word-level abstraction}, 
	year={2017},
	volume={},
	number={},
	pages={132-139},}

@ARTICLE{UVM-ieee-standard-2017,
	author={},
	journal={IEEE Std 1800.2-2017}, 
	title={{IEEE Standard for Universal Verification Methodology Language Reference Manual}}, 
	year={2017},
	pages={1-472},}

@ARTICLE{Singh-Lin.etal-18, 
		author={E. {Singh} and D. {Lin} and C. {Barrett} and S. {Mitra}}, 
		journal={{IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems}}, 
		title={Logic Bug Detection and Localization Using Symbolic Quick Error Detection}, 
		year={2018}, 
		volume={}, 
		number={}, 
		ISSN={0278-0070}, 
		month={},}

@INPROCEDINGS{Fadiheh-Urdahl.etal-2018, 
		author={M. R. {Fadiheh} and J. {Urdahl} and S. S. {Nuthakki} and S. {Mitra} and C. {Barrett} and D. {Stoffel} and W. {Kunz}}, 
		booktitle={2018 Design, Automation Test in Europe Conference Exhibition (DATE)}, 
		title={Symbolic quick error detection using symbolic initial state for pre-silicon verification}, 
		year={2018}, 
		volume={}, 
		number={}, 
		pages={55-60}, 
		doi={10.23919/DATE.2018.8341979}, 
		ISSN={1558-1101}, 
		month={March},}

@Inbook{Holzmann-2018,
	author="Holzmann, Gerard J.",
	editor="Clarke, Edmund M.
	and Henzinger, Thomas A.
	and Veith, Helmut
	and Bloem, Roderick",
	title="Explicit-State Model Checking",
	bookTitle="Handbook of Model Checking",
	year="2018",
	publisher="Springer International Publishing",
	address="Cham",
	pages="153--171",
	isbn="978-3-319-10575-8",
	doi="10.1007/978-3-319-10575-8_5",
	url="https://doi.org/10.1007/978-3-319-10575-8_5"
}

@INPROCEEDINGS{Chiu.etal-2018,
	author		={P. {Chiu} and C. {Celio} and K. {Asanovi\'{c}} and D. {Patterson} and B. {Nikoli\'{c}}},
	booktitle	={{2018 IEEE Symposium on VLSI Circuits}}, 
	title		={An Out-of-Order RISC-V Processor with Resilient Low-Voltage Operation in 28NM CMOS}, 
	year		={2018},
	volume		={},
	number		={},
	pages		={61-62},}
	
@INPROCEDINGS{Fadiheh-Urdahl.etal-2018, 
		author={M. R. {Fadiheh} and J. {Urdahl} and S. S. {Nuthakki} and S. {Mitra} and C. {Barrett} and D. {Stoffel} and W. {Kunz}}, 
		booktitle={2018 Design, Automation Test in Europe Conference Exhibition (DATE)}, 
		title={Symbolic quick error detection using symbolic initial state for pre-silicon verification}, 
		year={2018}, 
		volume={}, 
		number={}, 
		pages={55-60}, 
		doi={10.23919/DATE.2018.8341979}, 
		ISSN={1558-1101}, 
		month={March},}

@INPROCEEDINGS{Singh-Devarajegowda.etal-2019,
	author		={E. {Singh} and K. {Devarajegowda} and S. {Simon} and R. {Schnieder} and K. {Ganesan} and M. {Fadiheh} and D. {Stoffel} and W. {Kunz} and C. {Barrett} and W. {Ecker} and S. {Mitra}},
	booktitle	={2019 Design, Automation Test in Europe Conference Exhibition (DATE)},
	title		={Symbolic QED Pre-silicon Verification for Automotive Microcontroller Cores: Industrial Case Study},
	year		={2019},
	pages		={1000-1005},
	doi			={10.23919/DATE.2019.8715271},
	ISSN		={1530-1591},
	month		={March},
}

@INPROCEEDINGS{Devarajegowda-Hiltl.etal-2020, 
	author		={K. {Devarajegowda} and V. {Hiltl} and T. {Rabenalt} and D. {Stoffel} and W. {Kunz} and W. {Ecker}}, 
	title		={Formal Verification by The Book: Error Detection and Correction Codes}, 
	booktitle 	= {Design and Verification Conference and Exhibition},
	series 		= {DVCon},
	year 		= {2020},
}

@INPROCEEDINGS{Devarajegowda-Fadiheh.etal-2020,
	author={K. {Devarajegowda} and M. R. {Fadiheh} and E. {Singh} and C. {Barrett} and S. {Mitra} and W. {Ecker} and D. {Stoffel} and W. {Kunz}},
	booktitle={2020 Design, Automation   Test in Europe Conference   Exhibition (DATE)}, 
	title={{Gap-free Processor Verification by S²QED and Property Generation}}, 
	year={2020},
	volume={},
	number={},
	pages={526-531},
	doi={10.23919/DATE48585.2020.9116515}}

%---------------------------------------------------------------------------------------------------------------------
% ISAs (RISC-V realted)
%---------------------------------------------------------------------------------------------------------------------

@INPROCEEDINGS{Hennessy-Jouppi.etal-1982,
	author		={J. {Hennessy} and N {Jouppi} and S {Przybylski} and C. {Rowen} and T. {Gross} and F. {Baskett} and J {Gill}},
	booktitle	={{15th Annual Workshop on Microprogramming, MICRO 15, Palo Alto, California, USA: IEEE Press}},
	title		={MIPS: A Microprocessor Architecture},
	year		={1982},
	pages		={17-22},
}

@online{SPARC-ISA-1994,
	author = {},
	title  = {{SPARC International Inc., The SPARC Architecture Manual, Version 8}},
	year   = {1994},
	url    = "http://sparc.org/technical-documents/#V9",
	lastaccessed = "March 28, 2020",
}


@online{Waterman-Asanovic-2017,
	author = {A. {Waterman} and K. {Asanovic}},
	title  = {{The RISC-V Instruction Set Manual, Volume I: User-Level ISA}},
	year   = {2017},
	month  = {May},
	note   = {\url{https://riscv.org/specifications}},
	lastaccessed = "March 28, 2019",
}

@online{ARM-A64-ISA,
	author = {ARM},
	title  = {{ARM\textregistered A64 Instruction Set Architecture}},
	year   = {2018},
	note   = {\url{https://static.docs.arm.com/ddi0596/a/DDI_0596_ARM_a64_instruction_set_architecture.pdf}},
	lastaccessed = "March 28, 2020",
}

@book{Shanley-2010,
	author = {Shanley, Tom},
	title = {X86 Instruction Set Architecture},
	year = {2010},
	isbn = {0977087859},
	publisher = {Mindshare Press}
}

@book{FI-techniques,
author = {Benso, Alfredo and Prinetto, Paolo},
year = {2003},
month = {01},
pages = {},
title = {Fault Injection Techniques and Tools for Embedded Systems Reliability Evaluation}
}

@INPROCEEDINGS{Blem.etal-2013,
	author={E. {Blem} and J. {Menon} and K. {Sankaralingam}},
	booktitle={{2013 IEEE 19th International Symposium on High Performance Computer Architecture (HPCA)}}, 
	title={Power struggles: Revisiting the RISC vs. CISC debate on contemporary ARM and x86 architectures}, 
	year={2013},
	volume={},
	number={},
	pages={1-12},}

@ARTICLE{F-collapsing,
  author={Lloy, A.},
  journal={IEEE Design   Test of Computers}, 
  title={Advanced fault collapsing (logic circuits testing)}, 
  year={1992},
  volume={9},
  number={1},
  pages={64-71},
  doi={10.1109/54.124518}}
	
	

@misc{grift,
	title                    = {{Griftl}},
	howpublished = "\url{https://github.com/riscv/ISA_Formal_Spec_Public_Review/blob/master/GRIFT.md}",
	note = "[Online: Accessed on 10.November.2020]",
}
@misc{forvis,
	title                    = {{Forvis}},
	howpublished = "\url{https://github.com/riscv/ISA_Formal_Spec_Public_Review/blob/master/Forvis.md}",
	note = "[Online: Accessed on 10.November.2020]",
}

@misc{sail,
	title                    = {{Sail}},
	howpublished = "\url{https://github.com/riscv/ISA_Formal_Spec_Public_Review/blob/master/Sail.md}",
	note = "[Online: Accessed on 10.November.2020]",
}

@misc{riscv-plv,
	title                    = {{Riscv-plv}},
	howpublished = "\url{https://github.com/riscv/ISA_Formal_Spec_Public_Review/blob/master/riscv-plv.md}",
	note = "[Online: Accessed on 10.November.2020]",
}

@misc{kami,
	title                    = {{Kami}},
	howpublished = "\url{https://github.com/riscv/ISA_Formal_Spec_Public_Review/blob/master/Kami.md}",
	note = "[Online: Accessed on 10.November.2020]",
}

@misc{sail_semantics,
	title                    = {{ISA Semantics for ARMv8-A, RISC-V, and CHERI-MIPS}},
	howpublished = "\url{https://www.cl.cam.ac.uk/~pes20/sail/sail-popl2019.pdf}",
	note = "[Online: Accessed on 11.November.2020]",
}
@misc{oss_riscv,
	title                    = {{Assuring the Integrity of RISC-V Cores and SoCs}},
	howpublished = "\url{https://www.onespin.com/resources/white-papers/}",
	note = "[Online: Accessed on 11.November.2020]",
}

@INPROCEEDINGS{8746054,
  author={M. {Chupilko} and A. {Kamkin} and A. {Kotsynyak} and A. {Protsenko} and S. {Smolov} and A. {Tatarnikov}},
  booktitle={2018 19th International Workshop on Microprocessor and SOC Test and Verification (MTV)}, 
  title={Test Program Generator MicroTESK for RISC-V}, 
  year={2018},
  volume={},
  number={},
  pages={6-11},
  doi={10.1109/MTV.2018.00011}}

@ARTICLE{8746055,
  author={M. {Freericks}},
  title={{The nML Machine Description Formalism}}, 
  journal={Technical Report TR SM-IMP/DIST/08, TU Berlin CS Department},
  year={1993},
  volume={},
  number={},
  pages={47}
  }
  
@INPROCEEDINGS{9116193,
  author={V. {Herdt} and D. {Große} and R. {Drechsler}},
  booktitle={2020 DATE}, 
  title={{Towards Specification and Testing of RISC-V ISA Compliance}}, 
  year={2020},
  volume={},
  number={},
  pages={995-998},
  doi={10.23919/DATE48585.2020.9116193}}
  
@INPROCEEDINGS{5457129,
  author={S. {Vasudevan} and D. {Sheridan} and S. {Patel} and D. {Tcheng} and B. {Tuohy} and D. {Johnson}},
  booktitle={2010 Design, Automation   Test in Europe Conference   Exhibition (DATE 2010)}, 
  title={GoldMine: Automatic assertion generation using data mining and static analysis}, 
  year={2010},
  volume={},
  number={},
  pages={626-629},
  doi={10.1109/DATE.2010.5457129}}
  
@INPROCEEDINGS{4484908,
  author={F. {Rogin} and T. {Klotz} and G. {Fey} and R. {Drechsler} and S. {Rulke}},
  booktitle={2008 Design, Automation and Test in Europe}, 
  title={Automatic Generation of Complex Properties for Hardware Designs}, 
  year={2008},
  volume={},
  number={},
  pages={545-548},
  doi={10.1109/DATE.2008.4484908}}
  
@misc{questa,
	title                    = {{Questa Property Generation}},
	howpublished = "\url{https://www.mentor.com/products/fv/questa-property-generation.}",
	note = "[Online: Accessed on 18.November.2020]",
}

@misc{jasper,
	title                    = {{Questa Property Generation}},
	howpublished = "\url{https://www.cadence.com/en_US/home/tools/system-design-and-verification/formal-and-static-verification/jasper-gold-verification-platform/formal-property-verification-app.html}",
	note = "[Online: Accessed on 18.November.2020]",
}



%---------------------------------------------------------------------------------------------------------------------
% Papers/Books/online-sources functional verification
%---------------------------------------------------------------------------------------------------------------------
@phdthesis{Bormann-phd-thesis-2009,
	author =       "J. {Bormann}",
	month =        {June},
	year =         {2009},
    advisor = "W. {Kunz}",
	school  =      {University of Kaiserslautern},
	title =        {Vollst{\"a}ndige Verifikation (Complete Functional Verification)},
	note =  {\url{https://kluedo.ub.uni-kl.de/frontdoor/deliver/index/docId/2108/file/diss_joerg_bormann.pdf}},
	lastaccessed = {April 2, 2019},
}

@InProceedings{Charleshyman-05,
	author={Hymans, Charles},
	editor={Cousot, Radhia},
	title={Verification of an Error Correcting Code by Abstract Interpretation},
	booktitle={Verification, Model Checking, and Abstract Interpretation},
	year={2005},
	publisher={Springer Berlin Heidelberg},
	address={Berlin, Heidelberg},
	pages={330--345},
	isbn={978-3-540-30579-8},
}

@book{Wille.etal-2005,
	author = {Bruce Wille and John C. Gross and Wolfgang Roesner},
	title = {Comprehensive Functional Verification},
	year = {2005},
	publisher = {Morgan Kaufmann Publishers},
	isbn = {0-12-751803-7},}


@ARTICLE{Lin-Hong.etal-2014, 
		author={D. {Lin} and T. {Hong} and Y. {Li} and E. {S} and S. {Kumar} and F. {Fallah} and N. {Hakim} and D. S. {Gardner} and S. {Mitra}}, 
		journal={{IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems}}, 
		title={Effective Post-Silicon Validation of System-on-Chips Using Quick Error Detection}, 
		year={2014}, 
		volume={33}, 
		number={10}, 
		pages={1573-1590}, 
		doi={10.1109/TCAD.2014.2334301}, 
		ISSN={0278-0070}, 
		month={Oct},}
	
	
@online{Urdahl-phd-thesis-2016,
		author =       "J. {Urdahl}",
		year =         "2016",
		school  =      "University of Kaiserslautern",
        advisor = "W. {Kunz}",
		title =        "Path Predicate Abstraction for Sound System-Level Modeling of Digital Circuits",
		note =  {\url{http://www.odbms.org/wp-content/uploads/2017/08/2015-Urdahl-1.pdf}},
		month =        {June},
		lastaccessed = "April 2, 2019",
	}

@ARTICLE{LRM-SV-2017,
	author={},
	journal={IEEE Std 1800-2017 (Revision of IEEE Std 1800-2012)}, 
	title={{IEEE Standard for SystemVerilog--Unified Hardware Design, Specification, and Verification Language}}, 
	year={2018},
	volume={},
	number={},
	pages={1-1315},}

@INPROCEEDINGS{Visalli-2017,
	author={G. {Visalli}},
	booktitle={2017 European Conference on Circuit Theory and Design (ECCTD)},
	title={{UVM-based verification of ECC module for flash memories}},
	year={2017},
	pages={1-4},
	doi={10.1109/ECCTD.2017.8093248},
	ISSN={},
	month={Sep.},}

%----------------------------------------------------------------------
% Tool vendors
%----------------------------------------------------------------------
@Misc{Onespin,
	author =   {{Onespin Solutions Gmbh}},
	title =    {{OneSpin 360MV}},
	note = {\url{https://www.onespin.com/}},
	note = "[Online: Accessed 01.May.2021]",}

@misc{Cadence,
	author = {{Cadence Design Systems, Inc.}},
	title = {{JasperGold Apps User Guide}},
	howpublished = "\url{https://www.cadence.com/}",
	note = "[Online: Accessed 05.December.2019]",}

@misc{Mentor,
	title                    = {{Questa Property Generation}},
	author                   = {{Mentor Graphics}},
	howpublished = "\url{https://www.mentor.com/}",
	note = "[Online: Accessed 05.December.2019]",}

@misc{Mentor-study-2020,
	title                    = {{The 2020 Wilson Research Group Functional Verification Study}},
	author                   = {{Mentor Graphics}},
	howpublished = "\url{https://blogs.sw.siemens.com/verificationhorizons/}",
	note = "[Online: Accessed 14.October.2020]",}

 @misc{Synopsys,
	title                    = {{VC Formal Apps}},
	author                   = {{Synopsys}},
	howpublished = "\url{https://www.synopsys.com/verification/static-and-formal-verification/vc-formal.html}",
	note = "[Online: Accessed on 05.December.2019]",}

@misc{HOL-4,
	title                    = {{The HOL-4 Proof Tool}},
	howpublished = "\url{http://hol.sf.net}",
	note = "[Online: Accessed on 05.December.2019]",}

@misc{ARM-ahbapb,
	title                    = {{AHB Example AMBA SYstem - Technical Reference Manual}},
	howpublished = "\url{https://static.docs.arm.com/ddi0170/a/DDI0170.pdf}",
	note = "[Online: Accessed on 15.August.2020]",}

@misc{AMBA-ahb,
	title                    = {{Arm AMBA 5 AHB Protocol Specification}},
	howpublished = "\url{https://developer.arm.com/documentation/ihi0033/latest/}",
	note = "[Online: Accessed on 04.May.2021]",}

@Misc{Xilinx,
	author =   {{Xilinx}},
	title =    {{Xilinx FPGA Platforms}},
	note = {\url{https://www.xilinx.com/}},
	note = "[Online: Accessed on 05.December.2019]",}

@Misc{Altera-Intel,
	author =   {{Altera}},
	title =    {{Hardware/Software Co-Verification Using FPGA Platforms}},
	note = {\url{https://www.intel.com/content/dam/www/programmable/us/en/pdfs/literature/wp/wp-01070-hardware-software-coverification-fpga.pdf}},
	note = "[Online: Accessed on 20.September.2020]",}

@Misc{Palladium-Cadence,
	author =   {{F. Schirrmeister}},
	title =    {{Improving Emulation Throughput for Multi-Project SoC Designs}},
	note = {\url{https://www.cadence.com/content/dam/cadence-www/global/en_US/documents/tools/system-design-verification/emulation-throughput-wp.pdf}},
	note = "[Online: Accessed on 20.September.2020]",}
	
	
@Misc{Verific,
	author =   {{Verific Design Automation}},
	title =    {{Verific}},
	note = {\url{https://www.verific.com/}},
	note = "[Online: Accessed 14.May.2021]",}

%----------------------------------------------------------------------
% Hardware design
%----------------------------------------------------------------------
@book{Patterson-Henessy-2011,
	author = {Patterson, David A. and Hennessy, John L.},
	title = {Computer Architecture: A Quantitative Approach},
	year = {2011},
	isbn = {1558800698},
	publisher = {Morgan Kaufmann Publishers Inc.},
	address = {San Francisco, CA, USA}
}

%----------------------------------------------------------------------
% Others
%----------------------------------------------------------------------
@book{Gonzalez-2008,
    author={D. L. {Gonzalez}},
    editor={Barbieri, Marcello and Hoffmeyer, Jesper},
    title={Error Detection and Correction Codes},
    bookTitle={The Codes of Life: The Rules of Macroevolution},
    year={2008},
    publisher={Springer Netherlands},
    address={Dordrecht},
    pages={379--394},
    isbn={978-1-4020-6340-4},
    doi={10.1007/978-1-4020-6340-4_17},
    url={https://doi.org/10.1007/978-1-4020-6340-4_17}}

@book{Nicolaidis-2010,
	author = {M. {Nicolaidis}},
	title = {{Soft Errors in Modern Electronic Systems}},
	year = {2010},
	isbn = {1441969926, 9781441969927},
	edition = {1st},
	publisher = {Springer Publishing Company, Incorporated},
}

@book{Kanekawa.etal-2010,
	author = {N {Kanekawa} and E. H. {Ibe} and T. {Suga} and Y {Uematsu}},
	title = {{Dependability in Electronic Systems: Mitigation of Hardware Failures, Soft Errors, and Electro-Magnetic Disturbances}},
	year = {2011},
	isbn = {978-1-4419-6714-5, 978-1-4899-8594-1},
	edition = {1st},
	publisher = {Springer-Verlag New York},
}

@article{Rossi.etal-2011,
	title={{Error Correcting Code Analysis for Cache Memory High Reliability and Performance}},
	author={D. {Rossi} and N. {Timoncini} and M. {Spica} and C. {Metra}},
	journal={2011 Design, Automation and Test in Europe},
	year={2011},
	pages={1-6},
}



% This file was created with JabRef 2.9.2.
% Encoding: UTF-8

@INPROCEEDINGS{1999-AziziAboulhamid.etal,
  author = {Mostafa Azizi and El Mostapha Aboulhamid and Sofiene Tahar},
  title = {Multithreading-based Coverification Technique of {HW}-{SW} Systems},
  booktitle = {Proc. International Conference Of Parallel Processing},
  year = {1999},
  pages = {1999-2005},
  bibsource = {DBLP, http://dblp.uni-trier.de},
  crossref = {DBLP:conf/pdpta/1999},
  file = {:./files/1999-AziziAboulhamid.etal.pdf:PDF},
  timestamp = {2006.09.27}
}

@INBOOK{2009-astiani.etal,
  chapter = {26},
  pages = {825--885},
  title = {Satisfiability Modulo Theories},
  publisher = {IOS Press},
  year = {2009},
  editor = {Biere, Armin and Heule, Marijn J. H. and van Maaren, Hans and Walsh,
	Toby},
  author = {Clark Barrett and Roberto Sebastiani and Sanjit Seshia and Cesare
	Tinelli},
  crossref = {HandbookOfSAT2009},
  file = {:./files/2009-BarrettSebastiani.etal.pdf:PDF},
  owner = {pavlenko},
  timestamp = {2010.02.25}
}

@INPROCEEDINGS{1994-BeckerDrechsler,
  author = {Bernd Becker and Rolf Drechsler},
  title = {{OFDD} Based Minimization of Fixed Polarity Reed-Muller Expressions
	Using Hybrid Genetic Algorithms},
  booktitle = {Computer Design: {VLSI} in Computers and Processors, 1994. {ICCD}
	'94. Proceedings., {IEEE} International Conference on},
  year = {1994},
  pages = {106 -110},
  month = {oct},
  bibsource = {DBLP, http://dblp.uni-trier.de},
  crossref = {DBLP:conf/iccd/1994},
  file = {:./files/1994-BeckerDrechsler.pdf:PDF},
  keywords = { FPRM minimization; HGAs; OFDD based minimization; fast heuristic
	methods; fixed polarity Reed-Muller expressions; genetic algorithms;
	hybrid GAs; hybrid genetic algorithms; ordered functional decision
	diagram; very large functions; decision theory; genetic algorithms;
	heuristic programming; logic CAD; minimisation of switching nets;},
  owner = {pavlenko},
  timestamp = {2011.06.03}
}

@INPROCEEDINGS{2010-BruttomessoPek.etal,
  author = {Roberto Bruttomesso and Edgar Pek and Natasha Sharygina and Aliaksei
	Tsitovich},
  title = {The {OpenSMT} Solver},
  booktitle = {TACAS},
  year = {2010},
  pages = {150-153},
  crossref = {DBLP:conf/tacas/2010},
  file = {:./files/2010-BruttomessoPek.etal.pdf:PDF},
  owner = {pavlenko},
  timestamp = {2010.07.26}
}

@INPROCEEDINGS{2007-KroeningSharygina,
  author = {Daniel Kroening and Natasha Sharygina},
  title = {Interactive presentation: Image computation and predicate refinement
	for {RTL} verilog using word level proofs},
  booktitle = {Proc. International Conference on Design, Automation and Test in
	Europe (DATE)},
  year = {2007},
  pages = {1325-1330},
  bibsource = {DBLP, http://dblp.uni-trier.de},
  crossref = {DBLP:conf/date/2007},
  file = {:./files/2007-KroeningSharygina.pdf:PDF},
  owner = {nguyen},
  timestamp = {2007.02.02}
}

@INPROCEEDINGS{1998-BasuMitra.etal,
  author = {A.Basu and R.S.Mitra and P.Marwedel},
  title = {Interface Synthesis For Embedded Application In Codesign Environment},
  booktitle = {{VLSI} Design, 1998. Proceedings., 1998 Eleventh International Conference
	on},
  year = {1998},
  pages = {85 -90},
  month = {jan},
  file = {:./files/1998-BasuMitra.etal.pdf:PDF},
  keywords = {MICKEY;addresses allocation;codesign environment;device drivers allocation;embedded
	applications;interface synthesis;programmable peripherals;programmable
	processor;high level synthesis;peripheral interfaces;real-time systems;storage
	allocation;},
  timestamp = {2006.10.04}
}

@ARTICLE{2006-HosangadiFallah.etal,
  author = {A.Hosangadi and F. Fallah and R. Kastner},
  title = {Optimizing Polynomial Expressions by Algebraic Factorization and
	Common Subexpression Elimination},
  journal = {{IEEE} Transactions on Computer-Aided Design},
  year = {2006},
  volume = {25},
  pages = {2012-2022},
  number = {10},
  month = {October},
  file = {:./files/2006-HosangadiFallah.etal.pdf:PDF},
  owner = {wedler},
  timestamp = {2006.12.18}
}

@INPROCEEDINGS{2004-Jerraya,
  author = {Ahmed A.Jerraya},
  title = {Long Term Trends For Embedded System Design},
  booktitle = {Proceedings of the Digital System Design, EUROMICRO Systems on (DSD)},
  year = {2004},
  pages = { 20 - 26},
  file = {:./files/2004-Jerraya.pdf:PDF},
  keywords = { CPU subsystem; electronic subsystem; embedded software; embedded
	system design; hardware platform; hardware subsystem; system-on-chip;
	embedded systems; hardware-software codesign; integrated circuit
	design; system-on-chip;},
  timestamp = {2006.10.04}
}

@INPROCEEDINGS{1998-MokkedemHosabetto.etal,
  author = {A.Mokkedem and R.Hosabetto and G.Gopalagrishnan},
  title = {Formalization And Proof Of A Solution To The {PCI} 2.1 Bus Transaction
	Ordering Problem},
  booktitle = {Proc. International Conference on Formal Methods in Computer-Aided
	Design ({FMCAD})},
  year = {1998},
  pages = {9--8},
  file = {:./files/1998-MokkedemHosabetto.etal.pdf:PDF},
  timestamp = {2006.09.19}
}

@INPROCEEDINGS{1999-VenerisAraman.etal,
  author = {A.Veneris and S.V.Araman and E.N.Hajj and W.K.Fuchs},
  title = {Multiple Design Error Diagnosis and Correction in {VLSI} Circuits},
  booktitle = {Proc. {IEEE} {VLSI} Test Symposium},
  year = {1999},
  pages = {58 -63},
  file = {:./files/1999-VenerisAraman.etal.pdf:PDF},
  keywords = {ISCAS'85 benchmark circuits;VLSI circuit design;digital VLSI circuits;error
	correction;error space;logic design errors;multiple design error
	diagnosis;test vector simulation;VLSI;digital integrated circuits;error
	correction;fault diagnosis;integrated circuit design;logic CAD;},
  timestamp = {2006.09.14}
}

@INPROCEEDINGS{2000-AagaardJones.etal,
  author = {Mark D. Aagaard and Robert B. Jones and Roope Kaivola and Katherine
	R. Kohatsu and Carl-Johan H. Seger},
  title = {Formal Verification Of Iterative Algorithms In Microprocessors},
  booktitle = {Design Automation Conference, 2000. Proceedings 2000. 37th},
  year = {2000},
  pages = {201 -206},
  file = {:./files/2000-AagaardJones.etal.pdf:PDF}
}

@ARTICLE{1995-AbadiLamport,
  author = {Abadi, Mart\'{\i}n and Lamport, Leslie},
  title = {Conjoining specifications},
  journal = {ACM Trans. Program. Lang. Syst.},
  year = {1995},
  volume = {17},
  pages = {507--535},
  number = {3},
  month = may,
  acmid = {201069},
  address = {New York, NY, USA},
  issn = {0164-0925},
  issue_date = {May 1995},
  keywords = {composition, concurrent programming, decomposition, liveness properties,
	modular specification, safety properties, temporal logic},
  numpages = {29},
  owner = {bao},
  publisher = {ACM},
  timestamp = {2012.11.22}
}

@ARTICLE{1991-AbadiLamport,
  author = {Martin Abadi and Leslie Lamport},
  title = {The Existence of Refinement Mappings},
  journal = {Theoretical Computer Science},
  year = {1991},
  volume = {82},
  pages = {253-284},
  number = {2},
  file = {:./files/1991-AbadiLamport.pdf:PDF},
  owner = {stoffel},
  timestamp = {2012.03.28}
}

@INPROCEEDINGS{1988-AbadiLamport,
  author = {Abadi, M. and Lamport, L.},
  title = {The existence of refinement mappings},
  booktitle = {Logic in Computer Science, 1988. {LICS} '88., Proceedings of the
	Third Annual Symposium on},
  year = {1988},
  pages = {165-175},
  file = {:./files/1988-AbadiLamport.pdf:PDF},
  keywords = {automata theory;existence;hierarchical specification method;liveness
	requirements;lower-level specification;refinement mappings;safety
	requirements;state machine;automata theory;},
  owner = {stoffel},
  timestamp = {2012.03.26}
}

@INPROCEEDINGS{2000-AbdullaBjesse.etal,
  author = {P. A. Abdulla and P. Bjesse and N. Een},
  title = {Symbolic Reachability Analysis Based on {SAT} Solver},
  booktitle = {Proc. International Conference on Tools and Algorithms for Construction
	and Analysis of Systems},
  year = {2000},
  file = {:./files/2000-AbdullaBjesse.etal.pdf:PDF}
}

@INPROCEEDINGS{1999-AboulhamidTahar,
  author = {Mostafa Azizi El Mostapha Aboulhamid and Sofine Tahar},
  title = {Properties Coverification for {HW}-{SW} Systems},
  booktitle = {Proc. Conference of Electronic Circuits and Systems ({ECS})},
  year = {1999},
  file = {:./files/1999-AboulhamidTahar.pdf:PDF}
}

@INPROCEEDINGS{2005-AbrahamBecker.etal,
  author = {Erika Abraham and Bernd Becker and Felix Klaedtke and Martin Steffen},
  title = {Optimizing bounded model checking for linear hybrid systems},
  booktitle = {LNCS},
  year = {2005},
  pages = {396--412},
  publisher = {Springer-Verlag},
  file = {:./files/2005-AbrahamBecker.etal.pdf:PDF}
}

@BOOK{1994-AbramoviciBreuer.etal,
  title = {Digital Systems Testing and Testable Design},
  publisher = {{IEEE} Press},
  year = {1994},
  editor = {repeated},
  author = {M. Abramovici and M. Breuer and A. Friedman},
  address = {Piscataway, New Jersey}
}

@MISC{web_absint,
  author = {{{AbsInt Angewandte Informatik GmbH.} Germany}},
  title = {Astr\'{e}e},
  howpublished = {http://www.absint.com},
  key = {Astree},
  owner = {villarraga},
  timestamp = {2014.04.15},
  url = {http://www.absint.com}
}

@MISC{AbtsLiljaBatainehEtAl1999a,
  author = {D. Abts and D. Lilja and A. Bataineh and S. Scott},
  title = {Dimensions of Verifying the HardwareSoftware Interface in a Shared-Memory
	Multiprocessor},
  year = {1999},
  owner = {stoffel},
  text = {Dennis Abts, David J. Lilja, Abdulla Bataineh, and Steve Scott, Dimensions
	of Verifying the HardwareSoftware Interface in a Shared-Memory Multiprocessor,
	Laboratory for Advanced Research in Computing Technology and Compilers
	Technical Report No. {ARCTiC} 99-04, May 1999, (http://wwwmount.
	ee.umn.edu/ lilja/papers.memory.html).},
  timestamp = {2016.05.10},
  url = {http://citeseer.ist.psu.edu/abts99dimensions.html}
}

@MISC{AccelleraOrganization2004a,
  author = {{Accellera Organization Inc.}},
  title = {Property Specification Language - Reference Manual, version 1.1},
  howpublished = {http://www.eda.org/vfv/docs/PSL-v1.1.pdf},
  month = {June},
  year = {2004},
  file = {:./files/2004-AccelleraOrganization.pdf:PDF},
  owner = {wedler},
  timestamp = {2007.03.28}
}

@TECHREPORT{2005-Achterberg,
  author = {T. Achterberg},
  title = {Conflict Analysis in Mixed Integer Programming},
  institution = {Zuse Institute Berlin},
  year = {2005},
  number = {05-19},
  file = {:./files/2005-Achterberg.pdf:PDF},
  url = {http://www.zib.de/Publications/abstracts/ZR-05-19/}
}

@TECHREPORT{2004-Achterberg,
  author = {T. Achterberg},
  title = {{SCIP} - a framework to integrate Constraint and Mixed Integer Programming},
  institution = {Zuse Institute Berlin},
  year = {2004},
  number = {04-19},
  file = {:./files/2004-Achterberg.pdf:PDF},
  url = {http://www.zib.de/Publications/abstracts/ZR-04-19/}
}

@TECHREPORT{2007-AchterbergBrinkmann.etal,
  author = {Tobias Achterberg and Raik Brinkmann and Markus Wedler},
  title = {Property Checking with Constraint Integer Programming},
  institution = {Zuse Institute Berlin},
  year = {2007},
  number = {07-37},
  file = {:./files/2007-AchterbergBrinkmann.etal.pdf:PDF},
  owner = {wedler},
  timestamp = {2008.06.27},
  url = {http://opus.kobv.de/zib/volltexte/2007/1065/}
}

@TECHREPORT{2005a-AchterbergKoch.etal,
  author = {T. Achterberg and Thorsten Koch and Alexander Martin},
  title = {{MIPLIB} 2003},
  institution = {Zuse Institute Berlin},
  year = {2005},
  number = {05-28},
  file = {:./files/2005a-AchterbergKoch.etal.pdf:PDF},
  language = {English},
  url = {http://www.zib.de/Publications/abstracts/ZR-05-28/}
}

@ARTICLE{2005-AchterbergKoch.etal,
  author = {T. Achterberg and Thorsten Koch and Alexander Martin},
  title = {Branching Rules Revisited},
  journal = {Operations Research Letters},
  year = {2005},
  volume = {33},
  pages = {42-54},
  file = {:./files/2005-AchterbergKoch.etal.pdf:PDF}
}

@TECHREPORT{2004-AchterbergKoch.etal,
  author = {T. Achterberg and Thorsten Koch and Alexander Martin},
  title = {Branching Rules Revisited},
  institution = {Zuse Institute Berlin},
  year = {2004},
  number = {04-13},
  file = {:./files/2004-AchterbergKoch.etal.pdf:PDF},
  url = {http://www.zib.de/Publications/abstracts/ZR-04-13/}
}

@MISC{2003-AchterbergKoch.etal,
  author = {T. Achterberg and Thorsten Koch and Alexander Martin},
  title = {The Mixed Integer Programming Library: {\sc Miplib 2003}},
  year = {2003},
  owner = {stoffel},
  timestamp = {2016.05.10},
  url = {http://miplib.zib.de}
}

@TECHREPORT{2002-AchterbergKoch.etal,
  author = {T. Achterberg and Thorsten Koch and Alexander Martin},
  title = {Branching on History Information},
  institution = {Zuse Institute Berlin},
  year = {2002},
  number = {02-32},
  file = {:./files/2002-AchterbergKoch.etal.pdf:PDF},
  url = {http://www.zib.de/Publications/abstracts/ZR-02-32/}
}

@INPROCEEDINGS{2007-AciicmezKoc.etal,
  author = {Acii{\c{c}}mez, Onur and Ko{\c{c}}, {\c{C}}etin Kaya and Seifert,
	Jean-Pierre},
  title = {On the power of simple branch prediction analysis},
  booktitle = {Proceedings of the 2nd ACM symposium on Information, computer and
	communications security},
  year = {2007},
  pages = {312--320},
  organization = {ACM}
}

@INPROCEEDINGS{2007-AciicmezSeifert,
  author = {Aciicmez, Onur and Seifert, Jean-Pierre},
  title = {Cheap hardware parallelism implies cheap security},
  booktitle = {Workshop on Fault Diagnosis and Tolerance in Cryptography (FDTC)},
  year = {2007},
  pages = {80--91},
  organization = {IEEE},
  owner = {fadiheh},
  timestamp = {2018.07.12}
}

@MISC{2003-Adamczyk,
  author = {Paul Adamczyk},
  title = {The Anthology of the Finite State Machine Design Patterns},
  howpublished = {10 th Conference of Pattern Languagees of Programms},
  year = {2003},
  file = {:./files/2003-Adamczyk.pdf:PDF},
  owner = {thalmaier},
  timestamp = {2006.08.28}
}

@BOOK{2003-AdamsLoustaunau,
  title = {An Introduction to {Gr\"obner} Bases},
  publisher = {(Graduate studies in mathematics) {AMS}},
  year = {2003},
  author = {William Adams and Philippe Loustaunau},
  owner = {wienand},
  timestamp = {2008.04.08}
}

@INPROCEEDINGS{2013-AgarwalArvind,
  author = {A. Agarwal and Arvind},
  title = {Leveraging rule-based designs for automatic power domain partitioning},
  booktitle = {2013 IEEE/ACM International Conference on Computer-Aided Design (ICCAD)},
  year = {2013},
  issn = {1092-3152},
  owner = {udupi},
  timestamp = {2015.05.05}
}

@INPROCEEDINGS{2005-AgarwalVemuri,
  author = {Anuradha Agarwal and Ranga Vemuri},
  title = {Hierarchical Performance Macromodels of Feasible Regions for Synthesis
	of Analog and {RF} Circuits},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2005},
  pages = { 430 - 436},
  file = {:./files/2005-AgarwalVemuri.pdf:PDF},
  timestamp = {2006.09.27}
}

@INPROCEEDINGS{2008-AgarwalDimopoulos,
  author = {N. Agarwal and N. Dimopoulos},
  title = {{FSMD} Partitioning for Low Power Using {ILP}},
  booktitle = {2008 IEEE Computer Society Annual Symposium on VLSI},
  year = {2008},
  pages = {63-68},
  month = {April},
  file = {:files/2008-AgarwalDimopoulos.pdf:PDF},
  issn = {2159-3469},
  owner = {stoffel},
  timestamp = {2016.04.25}
}

@MISC{2004-Aglietti,
  author = {Federico Aglietti},
  title = {{AHB} System Generator},
  year = {2004},
  owner = {nguyen},
  timestamp = {2009.01.08},
  url = {http://opencores.org/project,ahb_system_generator}
}

@INPROCEEDINGS{2015-AhnMalik.etal,
  author = {Sunha Ahn and Malik, S. and Gupta, A.},
  title = {Completeness bounds and sequentialization for model checking of interacting
	firmware and hardware},
  booktitle = {Hardware/Software Codesign and System Synthesis (CODES+ISSS), 2015
	International Conference on},
  year = {2015},
  pages = {202--211},
  file = {:files/2015-AhnMalik.etal.pdf:PDF},
  owner = {stoffel},
  timestamp = {2016.01.27}
}

@INPROCEEDINGS{2009-AhujaShukla,
  author = {Sumit Ahuja and Sandeep Shukla},
  title = {{MCBCG:} Model Checking Based Sequential Clock-Gating},
  booktitle = {{IEEE} Intl. High Level Design Validation and Test Workshop},
  year = {2009},
  pages = {20--25},
  month = {nov},
  owner = {udupi},
  timestamp = {Tue, 12 May 2015 17:11:46 +0200}
}

@MISC{2003-Aitch,
  author = {Thorn Aitch},
  title = {Aquarius: a pipelined {RISC} {CPU}},
  year = {2003},
  owner = {stoffel},
  timestamp = {2010.10.29},
  url = {http://opencores.org/project,aquarius}
}

@ARTICLE{1978-Akers,
  author = {S. B. Akers},
  title = {Binary Decision Diagrams},
  journal = {{IEEE} Transactions on Computers},
  year = {1978},
  volume = {C-27},
  pages = {509-516},
  number = {6},
  month = {June},
  file = {:./files/1978-Akers.pdf:PDF},
  owner = {wedler},
  timestamp = {2006.12.15}
}

@ARTICLE{1976-Akers,
  author = {Akers, S.B., Jr.},
  title = {A Logic System for Fault Test Generation},
  journal = {Computers, {IEEE} Transactions on},
  year = {1976},
  volume = {C-25},
  pages = {620 -630},
  number = {6},
  month = {june },
  file = {:./files/1976-Akers.pdf:PDF},
  issn = {0018-9340},
  keywords = {Fault diagnosis, fault test generation, logic networks, logic systems,
	stuck-at faults.;}
}

@ARTICLE{2015-AlamNasab.etal,
  author = {M. Riahi Alam and M. E. Salehi Nasab and S. M. Fakhraie},
  title = {Power-Efficient High-Level Synthesis by Centralized and Fine-Grained
	Clock Gating},
  journal = {IEEE Transactions on Computer-Aided Design of Integrated Circuits
	and Systems},
  year = {2015},
  volume = {34},
  pages = {1954-1963},
  number = {12},
  month = {Dec},
  issn = {0278-0070}
}

@BOOK{2009-Al-Bahadili,
  title = {On the use of discrete-event simulation in computer networks analysis
	and design},
  publisher = {New York, USA: Information Science Reference},
  year = {2009},
  editor = {Evon M. O. Abu-Taieh and Asim A. El-Sheikh},
  author = {Al-Bahadili, Hussein},
  pages = {418--442},
  journal = {Handbook of Research on Discrete-Event Simulation Environments: Technologies
	and Applications},
  owner = {schwarz},
  timestamp = {2017.01.13}
}

@INPROCEEDINGS{1997-AlevrasGroetschel.etal,
  author = {Dimitris Alevras and Martin Groetschel and Roland Wessaly},
  title = {Capacity and Survivability Models for Telecommunication Networks},
  booktitle = {Proceedings of the {EURO} {XV/INFORMS} {XXXIV} Meeting, Barcelona
	June 1997},
  year = {1997},
  editor = {Jaime Barcelo},
  address = {Barcelona, Spanien},
  organization = {Universitat Politecnica de Catalunya},
  file = {:./files/1997-AlevrasGroetschel.etal.pdf:PDF},
  language = {English}
}

@INPROCEEDINGS{2005-AliSafarpour.etal,
  author = {Moayad Fahim Ali and Sean Safarpour and Andreas Veneris and Magdy
	S. Abadir and Rolf Drechsler},
  title = {Post-Verification Debugging of Hierarchical Designs},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2005},
  pages = { 871 - 876},
  file = {:./files/2005-AliSafarpour.etal.pdf:PDF},
  keywords = { Quantified {Boolean} Formula Satisfiability; VLSI design; automated
	debugging method; benchmark design; hierarchical designs; industrial
	design; memory requirement; verification processes; VLSI; integrated
	circuit design;},
  timestamp = {2006.10.10}
}

@ARTICLE{1994-AldinaMonteiro.etal,
  author = {M. Alidina and J. Monteiro and S. Devadas and A. Ghosh and M. Papaefthymiou},
  title = {Precomputation-based sequential logic optimization for low power},
  journal = {IEEE Transactions on Very Large Scale Integration (VLSI) Systems},
  year = {1994},
  volume = {2},
  pages = {426-436},
  number = {4},
  month = {Dec},
  file = {:/import/var/jabref/files/1994-AldinaMonteiro.etal.pdf:PDF},
  owner = {udupi},
  timestamp = {2018.04.16}
}

@INPROCEEDINGS{2011-AlizadehFujita,
  author = {Alizadeh, B. and Fujita, M.},
  title = {Modular equivalence verification of polynomial datapaths with multiple
	word-length operands},
  booktitle = {High Level Design Validation and Test Workshop (HLDVT), 2011 IEEE
	International},
  year = {2011},
  pages = {9-16},
  file = {:files/2011-AlizadehFujita:PDF},
  issn = {1552-6674},
  keywords = {decision diagrams;digital arithmetic;algebraic techniques;arithmetic
	circuit synthesis;arithmetic circuit verification;canonical decision
	diagram;canonical polynomial representation;decision diagrams;modular
	Horner expansion diagram;modular equivalence verification;modular-HED;multiple-word-length
	operands;polynomial datapaths;polynomial function verification;Boolean
	functions;Computational modeling;Data structures;Hardware;Optimization;Polynomials;Vectors},
  owner = {marx},
  timestamp = {2013.04.04}
}

@ARTICLE{2010-AlizadehFujita,
  author = {Alizadeh, B. and Fujita, M.},
  title = {Modular Datapath Optimization and Verification Based on Modular-{HED}},
  journal = {Computer-Aided Design of Integrated Circuits and Systems, {IEEE}
	Transactions on},
  year = {2010},
  volume = {29},
  pages = {1422 -1435},
  number = {9},
  month = {sept. },
  file = {:./files/2010-AlizadehFujita.pdf:PDF},
  issn = {0278-0070},
  keywords = {Horner expansion diagram;datapath-dominated applications;equivalence
	checking;hidden monomials;high level synthesis;modular datapath optimization;modular
	datapath verification;modular-HED;multioutput polynomials;embedded
	systems;formal verification;high level synthesis;optimisation;polynomials;signal
	processing;}
}

@INPROCEEDINGS{2008-AlizadehFujita,
  author = {Bijan Alizadeh and Masahiro Fujita},
  title = {Modular-{HED}: A Canonical Decision Diagram for Modular Equivalence
	Verification of Polynomial Functions},
  booktitle = {Workshop on Constraints in Formal Verification, {CFV}},
  year = {2008},
  pages = {22-40},
  address = {Australia},
  month = {September},
  owner = {pavlenko},
  timestamp = {2010.07.29}
}

@INPROCEEDINGS{2007-AlizadehFujita,
  author = {Bijan Alizadeh and Masahiro Fujita},
  title = {M.: {LTED}: A Canonical and Compact Hybrid Word-{Boolean} Representation
	as a Formal Model for Hardware/Software Co-designs},
  booktitle = {The fourth Workshop on Constraints in Formal Verification ({CFV}
	2007)},
  year = {2007},
  pages = {15--29},
  file = {:./files/2007-AlizadehFujita.pdf:PDF},
  owner = {pavlenko},
  timestamp = {2010.07.29}
}

@MISC{2000-VSIAlliance,
  author = {VSI Alliance},
  title = {{VSI} Alliance Virtual Component Interface Standard},
  year = {2000},
  owner = {nguyen},
  timestamp = {2007.07.09},
  url = {http://www.vsi.org/documents/vsiadocuments.htm}
}

@INPROCEEDINGS{2016-AlmeidaBarosa.etal,
  author = {Almeida, Jos{\'e} Bacelar and Barbosa, Manuel and Barthe, Gilles
	and Dupressoir, Fran{\c{c}}ois and Emmi, Michael},
  title = {Verifying constant-time implementations},
  booktitle = {25th $\{$USENIX$\}$ Security Symposium ($\{$USENIX$\}$ Security 16)},
  year = {2016},
  pages = {53--70},
  owner = {jmueller},
  timestamp = {2019.08.16}
}

@INPROCEEDINGS{2002-AloulMarkov.etal,
  author = {Fadi A. Aloul and Igor L. Markov and Karem A. Sakallah},
  title = {Improve the Efficiency of Circuit-to-{BDD} Conversion by Gate and
	Input Ordering},
  booktitle = {Proc. International Conference on Computer Design({ICCD})},
  year = {2002},
  file = {:./files/2002-AloulMarkov.etal.pdf:PDF},
  timestamp = {2006.09.21}
}

@INPROCEEDINGS{2002-AloulRamani.etal,
  author = {F. A. Aloul and A. Ramani and I. L. Markov and K. A. Sakallah},
  title = {Generic {ILP} Versus Specialized 0-1 {ILP}: An Update},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2002},
  pages = { 450 - 457},
  file = {:./files/2002-AloulRamani.etal.pdf:PDF},
  keywords = { {Boolean} optimization problems; {Boolean} satisfiability problem;
	EDA SAT problems; FPGA routing; Max-Clique; Max-Cut; Max-ONEs optimization
	problem; Max-SAT optimization problem; Min Vertex Cover; SAT solvers;
	SAT-based routing; electronic design automation; generic ILP techniques;
	hardware verification; integer linear programming; optimized solvers;
	satisfied clauses; software verification; specialized 0-1 ILP techniques;
	{Boolean} functions; computability; electronic design automation;
	integer programming; linear programming; network routing;}
}

@INPROCEEDINGS{2000-AloulSakallah,
  author = {Fadi A. Aloul and Karem A. Sakallah},
  title = {Efficient Verification of the {PCI} Local Bus using {Boolean} Satisfiability},
  booktitle = {International Workshop on Logic Synthesis ({IWLS})},
  year = {2000},
  pages = {131--136},
  file = {:./files/2000-AloulSakallah.pdf:PDF},
  timestamp = {2006.09.19}
}

@INPROCEEDINGS{1993-AltMahlstedt,
  author = {J. Alt and U. Mahlstedt},
  title = {Simulation of non-classical faults on the gate level-fault modeling},
  booktitle = {VLSI Test Symposium, 1993. Digest of Papers., Eleventh Annual 1993
	IEEE},
  year = {1993},
  pages = {351 - 354},
  month = {April},
  file = {2013-AltMahlstedt.pdf:files/2013-AltMahlstedt.pdf:PDF},
  owner = {bartsch},
  timestamp = {2016.01.07}
}

@TECHREPORT{2002-AlthausBockmayr.etal,
  author = {Ernst Althaus and Alexander Bockmayr and Matthias Elf and Michael
	Juenger and Thomas Kasper and Kurt Mehlhorn},
  title = {{SCIL} - Symbolic Constraints in Integer Linear Programming},
  institution = {MPI Saarbruecken},
  year = {2002},
  number = {ALCOMFT-TR-02-133},
  month = {May},
  file = {:./files/2002-AlthausBockmayr.etal.pdf:PDF}
}

@INPROCEEDINGS{2004-AlthausKaramanis.etal,
  author = {Ernst Althaus and Nikiforos Karamanis and Alexander Koller},
  title = {Computing Locally Coherent Discourses},
  booktitle = {Proc. Annual Meeting of the Association for Computational Linguistics
	({ACL})},
  year = {2004},
  address = {Barcelona, Spain},
  file = {:./files/2004-AlthausKaramanis.etal.pdf:PDF}
}

@ARTICLE{2005-AlurBenedikt.etal,
  author = {Rajeev Alur and Michael Benedikt and Kousha Etessami and Patrice
	Godefroid and Thomas Reps and Mihalis Yannakakis},
  title = {Analysis of Recursive State Machines},
  journal = {{ACM} on Programing Language and Systems},
  year = {2005},
  volume = {Vol. 27},
  pages = {786-818},
  file = {:./files/2005-AlurBenedikt.etal.pdf:PDF},
  timestamp = {2006.09.27}
}

@CONFERENCE{2005-AlurEtessami.etal,
  author = {Rajeev Alur and Kousha Etessami and P. Madhusudan},
  title = {A Temporal Logic of Nested Calls and Returns},
  booktitle = {Proc. International Conference on Tools and Algorithms for the Construction
	and Analysis of Systems ({TACAS})},
  year = {2005},
  pages = {467--481},
  file = {:./files/2005-AlurEtessami.etal.pdf:PDF},
  owner = {nguyen},
  timestamp = {2007.02.02}
}

@ARTICLE{1999-AlurHenzinger,
  author = {Alur, Rajeev and Henzinger, Thomas A.},
  title = {Reactive Modules},
  journal = {Form. Methods Syst. Des.},
  year = {1999},
  volume = {15},
  pages = {7--48},
  number = {1},
  month = jul,
  acmid = {325890},
  address = {Hingham, MA, USA},
  issn = {0925-9856},
  issue_date = {July 1999},
  numpages = {42},
  owner = {bao},
  publisher = {Kluwer Academic Publishers},
  timestamp = {2012.11.22}
}

@INPROCEEDINGS{2000-AmalaEmerson.etal,
  author = {N. Amala and E. Emerson and P. Kurshan and S. Namjoshi},
  title = {Model Checking Synchronous Timing Diagrams},
  booktitle = {Proc. International Conference on Formal Methods in Computer-Aided
	Design ({FMCAD})},
  year = {2000},
  file = {:./files/2000-AmalaEmerson.etal.pdf:PDF},
  timestamp = {2006.09.19}
}

@ARTICLE{2003-AmaldiPfetsch.etal,
  author = {Edoardo Amaldi and Marc E. Pfetsch and Leslie E. Trotter, Jr.},
  title = {On the Maximum Feasible Subsystem Problem, {IIS}s, and {IIS}-Hypergraphs},
  journal = {Mathematical Programming},
  year = {2003},
  volume = {95},
  pages = {533-554},
  number = {3},
  file = {:./files/2003-AmaldiPfetsch.etal.pdf:PDF}
}

@ARTICLE{2002-AmmonsRastislav.etal,
  author = {Ammons, Glenn and Bod\'{\i}k, Rastislav and Larus, James R.},
  title = {Mining Specifications},
  journal = {SIGPLAN Not.},
  year = {2002},
  volume = {37},
  pages = {4--16},
  number = {1},
  month = jan,
  acmid = {503275},
  address = {New York, NY, USA},
  doi = {10.1145/565816.503275},
  issn = {0362-1340},
  issue_date = {Jan. 2002},
  numpages = {13},
  publisher = {ACM},
  url = {http://doi.acm.org/10.1145/565816.503275}
}

@INPROCEEDINGS{1997-AmonyBorrielloz.etal,
  author = {Tod Amony and Gaetano Borrielloz and Taokuan Huy and Jiwen Liuy},
  title = {Symbolic Timing Verification Of Timing Diagrams Using Presburger
	Formulas},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {1997},
  file = {:./files/1997-AmonyBorrielloz.etal.pdf:PDF},
  timestamp = {2006.09.21}
}

@INPROCEEDINGS{2002-AmyeenPomeranz.etal,
  author = {M. Enamul Amyeen and Irith Pomeranz and W. Kent Fuchs},
  title = {Theorems for Efficient Identification of Indistinguishable Fault
	Pairs in Synchronous Sequential Circuits},
  booktitle = {Proc. {IEEE} {VLSI} Test Symposium},
  year = {2002},
  file = {amyeen-VTS02.pdf:amyeen-VTS02.pdf:PDF},
  timestamp = {2006.09.14}
}

@INPROCEEDINGS{1999-AmyeenPomeranz.etal,
  author = {M. Enamul Amyeen and Irith Pomeranz and W. Kent Fuchs},
  title = {Implication and Evaluation Techniques for proving Fault Equivalence},
  booktitle = {Proc. {IEEE} {VLSI} Test Symposium},
  year = {1999},
  pages = {201 -207},
  file = {:./files/1999-AmyeenPomeranz.etal.pdf:PDF},
  timestamp = {2006.09.14}
}

@INPROCEEDINGS{2002-AnastasakisDamiano.etal,
  author = {Anastasakis, D. and Damiano, R. and Ma, H.-K.T. and Stanion, T.},
  title = {A Practical and Efficient Method for Compare-Point Matching},
  booktitle = {Design Automation Conference, 2002. Proceedings. 39th},
  year = {2002},
  pages = { 305 - 310},
  file = {:./files/2002-AnastasakisDamiano.etal.pdf:PDF},
  issn = {0738-100X },
  keywords = { ATPG; combinational block functionality; combinational equivalence
	checkers; compare-point matching; function-based matching methods;
	heuristic algorithm; industrial-sized circuits; latch mapping; nonfunction-based
	matching methods; sequential design verification; vector generation
	partitioning; automatic test pattern generation; combinational switching;
	formal verification; logic partitioning; logic testing; sequential
	circuits;}
}

@INPROCEEDINGS{2002-AndersonBjesse.etal,
  author = {Andersson, G. and Bjesse, P. and Cook, B. and Hanna, Z.},
  title = {A Proof Engine Approach to Solving Combinational Design Automation
	Problems},
  booktitle = {Design Automation Conference, 2002. Proceedings. 39th},
  year = {2002},
  pages = { 725 - 730},
  file = {:./files/2002-AndersonBjesse.etal.pdf:PDF},
  issn = {0738-100X },
  keywords = { combinational design automation problems; composite default strategies;
	proof engine approach; satisfiability solvers; strategies-functions;
	synergistic effects; variable instantiation; circuit {CAD}; combinational
	circuits; formal verification; logic {CAD};}
}

@UNPUBLISHED{2003-AndreelloCaprara.etal,
  author = {Giuseppe Andreello and Alberto Caprara and Matteo Fischetti},
  title = {Embedding Cuts in a Branch \& Cut Framework: a Computational Study
	with {0,1/2}-Cuts},
  note = {Preliminary Draft},
  month = {October},
  year = {2003},
  file = {:./files/2003-AndreelloCaprara.etal.pdf:PDF}
}

@BOOK{2002-Andrews,
  title = {Introduction to Mathematical Logic and Type Theory: To Truth through
	Proof},
  publisher = {Kluwer Academic Publishers},
  year = {2002},
  author = {Andrews, Peter B.},
  address = {Norwell, MA, USA},
  isbn = {1402007639},
  owner = {pavlenko},
  timestamp = {2010.07.23}
}

@INPROCEEDINGS{2004-AndrewsQadeer.etal,
  author = {Tony Andrews and Shaz Qadeer and Sriram Rajamani and Jakob Rehof
	and Yichen Xie},
  title = {{ZING} : A Model Checker for Concurrent Software},
  booktitle = {Proc. 6th International Conference on Computer Aided Design},
  year = {2004},
  pages = {484--487},
  file = {:./files/2004-AndrewsQadeer.etal.pdf:PDF},
  timestamp = {2006.09.22}
}

@MISC{2006-AnoepGanda.etal,
  author = {Shanny Anoep and El Drijver and Arvind Ganga and Martijn Kirsten},
  title = {Resolution proof for look-ahead {SAT} solvers},
  howpublished = {Master Report},
  year = {2006},
  file = {:./files/2006-AnoepGanda.etal.pdf:PDF},
  owner = {nguyen},
  timestamp = {2007.12.14}
}

@INPROCEEDINGS{2002-AntoniLeveugle.etal,
  author = {L. Antoni and R. Leveugle and M. Feher},
  title = {Using run-time reconfiguration for fault injection in hardware prototypes},
  booktitle = {17th IEEE International Symposium on Defect and Fault Tolerance in
	VLSI Systems},
  year = {2002},
  pages = {245-253},
  month = {November},
  file = {2002-AntoniLeveugle.etal.pdf:files/2002-AntoniLeveugle.etal.pdf:PDF},
  issn = {1550-5774},
  owner = {bartsch},
  timestamp = {2016.09.22}
}

@INPROCEEDINGS{2009-ArbelRokhlenko.etal,
  author = {E. Arbel and O. Rokhlenko and K. Yorav},
  title = {{SAT}-based synthesis of clock gating functions using 3-valued abstraction},
  booktitle = {Formal Methods in Computer-Aided Design, 2009. FMCAD 2009},
  year = {2009},
  pages = {198-204},
  month = {Nov},
  owner = {udupi},
  timestamp = {2016.07.21}
}

@INPROCEEDINGS{2017b-ArdeshirichamHu.etal,
  author = {Ardeshiricham, Armaiti and Hu, Wei and Kastner, Ryan},
  title = {Clepsydra: Modeling timing flows in hardware designs},
  booktitle = {IEEE/ACM International Conference on Computer-Aided Design (ICCAD)
	},
  year = {2017},
  pages = {147--154},
  organization = {IEEE},
  owner = {fadiheh},
  timestamp = {2018.07.13}
}

@INPROCEEDINGS{2017-ArdeshirichamHu.etal,
  author = {Ardeshiricham, Armaiti and Hu, Wei and Marxen, Joshua and Kastner,
	Ryan},
  title = {Register transfer level information flow tracking for provably secure
	hardware design},
  booktitle = {Design, Automation \& Test in Europe Conference (DATE)},
  year = {2017},
  pages = {1695--1700},
  organization = {IEEE},
  owner = {fadiheh},
  timestamp = {2018.07.12}
}

@ARTICLE{1990-ArlatAguera.etal,
  author = {J. Arlat and M. Aguera and L. Amat and Y. Crouzet and J.-C. Fabre
	and J.-C. Laprie and E. Martins and D. Powell},
  title = {Fault injection for dependability validation: a methodology and some
	applications},
  journal = {IEEE Transactions on Software Engineering},
  year = {1990},
  volume = {16},
  pages = {166 - 182},
  number = {2},
  month = {Feb},
  file = {1990-ArlatAguera.etal.pdf:files/1990-ArlatAguera.etal.pdf:PDF},
  issn = {0098-5589},
  owner = {bartsch},
  timestamp = {2015.09.10}
}

@MISC{1999-ARM,
  author = {{ARM Limited}},
  title = {{AMBA} Specification (Rev 2.0)},
  howpublished = {http://www.arm.com},
  year = {1999},
  file = {:./files/1999-ARM.pdf:PDF},
  owner = {thalmaier},
  publisher = {{ARM}},
  timestamp = {2006.11.24}
}

@INPROCEEDINGS{2005-ArmoniEgorov.etal,
  author = {Armoni, R. and Egorov, S. and Fraer, R. and Korchemny, D. and Vardi,
	M.Y.},
  title = {Efficient {LTL} Compilation for {SAT}-based Model Checking},
  booktitle = {Computer-Aided Design, 2005. {ICCAD}-2005. {IEEE/ACM} International
	Conference on},
  year = {2005},
  pages = { 877 - 884},
  month = {nov.},
  file = {:./files/2005-ArmoniEgorov.etal.pdf:PDF},
  issn = { },
  keywords = { BDD-based symbolic model checking; LTL compilation; LTL safety property;
	SAT-based model checking; automata construction; bounded model checking;
	deterministic automata; linear temporal logics; nondeterministic
	automata; formal logic; logic testing;}
}

@INPROCEEDINGS{2004-AronHooker.etal,
  author = {Ionut Aron and John N. Hooker and Tallys H. Yunes},
  title = {{SIMPL}: A System for Integrating Optimization Techniques},
  booktitle = {First International Conference on Integration of Artificial Intelligence
	({AI}) and Operations Research ({OR}) {CPAIOR}},
  year = {2004},
  editor = {Jean-Charles Regin and Michel Rueher},
  pages = {21-36},
  address = {Nice, France},
  month = {April},
  file = {:./files/2004-AronHooker.etal.pdf:PDF}
}

@INPROCEEDINGS{2005-AronsElster.etal,
  author = {Arons, Tamarah and Elster, Elad and Fix, Limor and Mador-Haim, Sela
	and Mishaeli, Michael and Shalev, Jonathan and Singerman, Eli and
	Tiemeyer, Andreas and Vardi, Moshe Y. and Zuck, Lenore D.},
  title = {Formal verification of backward compatibility of microcode},
  booktitle = {Proceedings of the 17th international conference on Computer Aided
	Verification},
  year = {2005},
  series = {CAV'05},
  pages = {185--198},
  address = {Berlin, Heidelberg},
  publisher = {Springer-Verlag},
  acmid = {2153256},
  file = {2005-AronsElster.etal.pdf:files/2005-AronsElster.etal.pdf:PDF},
  isbn = {3-540-27231-3, 978-3-540-27231-1},
  location = {Edinburgh, Scotland, UK},
  numpages = {14},
  owner = {villarraga},
  timestamp = {2012.12.03}
}

@INPROCEEDINGS{2008-AronsOzer.etal,
  author = {Arons, Tamarah and Elster, Elad and Ozer, Shlomit and Shalev, Jonathan
	and Singerman, Eli},
  title = {Efficient Symbolic Simulation of Low Level Software},
  booktitle = {Design, Automation and Test in Europe, 2008. DATE '08},
  year = {2008},
  pages = {825 -830},
  month = {march},
  file = {2008-AronsOzer.etal.pdf:files/2008-AronsOzer.etal.pdf:PDF},
  keywords = {formal hardware verification;low level software;microcode validation;symbolic
	execution;symbolic simulation;machine oriented languages;program
	verification;symbol manipulation;},
  owner = {villarraga},
  timestamp = {2012.07.18}
}

@ARTICLE{1993-AroraGouda,
  author = {Arora, A. and Gouda, M.},
  title = {Closure and Convergence :A foundation of Fault -Tolerant Computing},
  journal = {Software Engineering, IEEE Transactions on},
  year = {1993},
  volume = {19},
  pages = {1015 -1027},
  number = {11},
  month = {nov},
  file = {:./files/1993-AroraGouda.pdf:PDF},
  issn = {0098-5589},
  keywords = {closure;convergence;fault-tolerant computing;legal states;verification;fault
	tolerant computing;formal verification;}
}

@BOOK{2009-AroraBarak,
  title = {Computational Complexity: A Modern Approach},
  publisher = {Cambridge University Press},
  year = {2009},
  author = {Sanjeev Arora and Boaz Barak},
  owner = {villarraga},
  timestamp = {2015.10.05}
}

@ARTICLE{2016-AsanovicAvizienis.etal,
  author = {Asanovic, Krste and Avizienis, Rimas and Bachrach, Jonathan and Beamer,
	Scott and Biancolin, David and Celio, Christopher and Cook, Henry
	and Dabbelt, Daniel and Hauser, John and Izraelevitz, Adam and others},
  title = {The rocket chip generator},
  journal = {EECS Department, University of California, Berkeley, Tech. Rep. UCB/EECS-2016-17},
  year = {2016},
  owner = {fadiheh},
  timestamp = {2018.07.18}
}

@ARTICLE{2007-AscheidMeyr,
  author = {G. Ascheid and H. Meyr},
  title = {Opportunities for Application-Specific Processors: The Case of Wireless
	Communication},
  journal = {Customizable Embedded Processors},
  year = {2007},
  pages = {11--37},
  editor = {P. Ienne and R. Leupers},
  owner = {brehm},
  publisher = {Morgan Kaufmann Publishers},
  timestamp = {2007.03.28}
}

@ARTICLE{2001-AscheuerFischetti.etal,
  author = {Norbert Ascheuer and Matteo Fischetti and Martin Groetschel},
  title = {Solving the Asymmetric Travelling Salesman Problem with Time Windows
	by Branch-and-Cut},
  journal = {Mathematical Programming},
  year = {2001},
  volume = {90},
  pages = {475-506},
  number = {3},
  month = {May},
  file = {:./files/2001-AscheuerFischetti.etal.pdf:PDF},
  language = {English},
  publisher = {Springer}
}

@INPROCEEDINGS{1990-AsharDevadas.etal,
  author = {Ashar, P. and Devadas, S. and Newton, A.R.},
  title = {A unified approach to the decomposition and re-decomposition of sequential
	machines},
  booktitle = {Design Automation Conference, 1990. Proceedings., 27th {ACM/IEEE}},
  year = {1990},
  pages = {601 -606},
  month = {jun},
  file = {:./files/1990-AsharDevadas.etal.pdf:PDF},
  issn = {0738-100X},
  keywords = {CPU-time-efficient;FLAMES;cascade decompositions;cost function;decomposition
	topologies;distributed-style specifications;finite state machine
	decomposition;implicant covering;parallel decomposition;preserved
	partitions;re-decomposition algorithms;sequential logic synthesis
	system;sequential machines;state assignment;state transition graph;graph
	theory;logic CAD;sequential machines;state assignment;}
}

@ARTICLE{2001-AsharGupta.etal,
  author = {Pranav Ashar and Aarti Gupta and Sharad Malik},
  title = {Using Complete-1-Distinguishability for FSM Equivalence Checking},
  journal = {{ACM} Transactions on Design Automation of Electronic Systems},
  year = {2001},
  volume = {6},
  pages = {569 - 590},
  file = {:./files/2001-AsharGupta.etal.pdf:PDF},
  timestamp = {2006.09.13}
}

@BOOK{2001-Ashenden,
  title = {The Designer's Guide to VHDL},
  publisher = {Morgan Kaufmann Publishers Inc.},
  year = {2001},
  author = {Ashenden, Peter J.},
  address = {San Francisco, CA, USA},
  isbn = {1558606742},
  owner = {pavlenko},
  timestamp = {2010.10.07}
}

@INPROCEEDINGS{1959-Ashenhurst,
  author = {R. L. Ashenhurst},
  title = {The Decomposition of Switching Functions},
  booktitle = {Proc. International Symposium on the Theory of Switching},
  year = {1959},
  pages = {74-116}
}

@ARTICLE{2009-Ashton,
  author = {Ashton, Kevin},
  title = {{That 'Internet of Things' Thing}},
  journal = {RFID Journal},
  year = {2009},
  month = jun,
  citeulike-article-id = {13401010},
  file = {2009-Ashton.pdf:files/2009-Ashton.pdf:PDF},
  keywords = {directed, studies},
  owner = {schwarz},
  posted-at = {2014-10-19 14:34:30},
  priority = {2},
  timestamp = {2017.01.09}
}

@BOOK{2006-AstolaStankovic,
  title = {Fundamentals of Switching Theory and Logic Design},
  publisher = {Springer},
  year = {2006},
  author = {Jaakko T. Astola and Radomir S. Stankovic},
  file = {:./files/2006-AstolaStankovic.pdf:PDF},
  owner = {pavlenko},
  timestamp = {2010.07.07}
}

@ARTICLE{2000-AtamtuerkNemhauser.etal,
  author = {Alper Atamtuerk and George L. Nemhauser and Martin W.P. Savelsbergh},
  title = {Conflict Graphs in Integer Programming},
  journal = {European Journal of Operations Research},
  year = {2000},
  volume = {121},
  pages = {40-55},
  file = {:./files/2000-AtamtuerkNemhauser.etal.pdf:PDF}
}

@ARTICLE{2005-AtamtuerkSavelsbergh,
  author = {Alper Atamtuerk and Martin W.P. Savelsbergh},
  title = {Integer-Programming Software Systems},
  journal = {Annals of Operations Research},
  year = {2005},
  volume = {140},
  pages = {67-124},
  file = {:./files/2005-AtamtuerkSavelsbergh.pdf:PDF},
  url = {http://www.isye.gatech.edu/faculty/Martin_Savelsbergh/publications/ipsoftware-final.pdf}
}

@ARTICLE{2010-AtzoriIera.etal,
  author = {Luigi Atzori and Antonio Iera and Giacomo Morabito},
  title = {The Internet of Things: A survey },
  journal = {Computer Networks },
  year = {2010},
  volume = {54},
  pages = {2787 - 2805},
  number = {15},
  abstract = {This paper addresses the Internet of Things. Main enabling factor
	of this promising paradigm is the integration of several technologies
	and communications solutions. Identification and tracking technologies,
	wired and wireless sensor and actuator networks, enhanced communication
	protocols (shared with the Next Generation Internet), and distributed
	intelligence for smart objects are just the most relevant. As one
	can easily imagine, any serious contribution to the advance of the
	Internet of Things must necessarily be the result of synergetic activities
	conducted in different fields of knowledge, such as telecommunications,
	informatics, electronics and social science. In such a complex scenario,
	this survey is directed to those who want to approach this complex
	discipline and contribute to its development. Different visions of
	this Internet of Things paradigm are reported and enabling technologies
	reviewed. What emerges is that still major issues shall be faced
	by the research community. The most relevant among them are addressed
	in details. },
  issn = {1389-1286},
  keywords = {Internet of Things},
  owner = {schwarz},
  timestamp = {2017.01.09},
  url = {http://www.sciencedirect.com/science/article/pii/S1389128610001568}
}

@ARTICLE{1996-AuburyPage.etal,
  author = {Aubury, Matthew and Page, Ian and Randall, Geoff and Saul, Jonathan
	and Watts, Robin},
  title = {Handel-C language reference guide},
  journal = {Computing Laboratory. Oxford University, UK},
  year = {1996}
}

@INPROCEEDINGS{2002-AudemardBertoli.etal,
  author = {Gilles Audemard and Piergiorgio Bertoli and Alessandro Cimatti and
	Artur Kornilowicz and Roberto Sebastiani},
  title = {A {SAT}-based Approach for Solving Formulas over {Boolean} and Linear
	Mathematical Propositions},
  booktitle = {Proc. International Conference on Automated Deduction ({CAD})},
  year = {2002},
  pages = {195-210},
  file = {:./files/2002-AudemardBertoli.etal.pdf:PDF}
}

@MISC{0000-AustinErnst,
  author = {Todd Austin and Dan Ernst and Eric Larson and Chris Weaver},
  title = {SimpleScalar Tutorial},
  note = {Slides},
  file = {0000-AustinErnst.pdf:files/0000-AustinErnst.pdf:PDF},
  owner = {nguyen},
  timestamp = {2007.02.02}
}

@ARTICLE{2012-AzambujaPagliarini.etal,
  author = {J. R. Azambuja and S. Pagliarini and M. Altieri and F. L. Kastensmidt
	and M. Hubner and J. Becker and G. Foucard and R. Velazco},
  title = {A Fault Tolerant Approach to Detect Transient Faults in Microprocessors
	Based on a Non-Intrusive Reconfigurable Hardware},
  journal = {IEEE Transactions on Nuclear Science},
  year = {2012},
  volume = {59},
  pages = {1117-1124},
  number = {4},
  month = {August},
  file = {2012-AzambujaPagliarini.etal.pdf:files/2012-AzambujaPagliarini.etal.pdf:PDF},
  issn = {0018-9499},
  owner = {bartsch},
  timestamp = {2016.09.21}
}

@MISC{1997-Aziz,
  author = {Adnan Aziz},
  title = {Texas-97 benchmarks},
  year = {1997},
  note = {http://www-cad.EECS.Berkeley.EDU/ Respep/Research/Vis/texas-97},
  file = {texas97-benchmarks.tar.gz:texas97-benchmarks.tar.gz:TARGZ},
  owner = {stoffel},
  timestamp = {2016.05.11}
}

@TECHREPORT{1993-AzizSinghal.etal,
  author = {A. Aziz and V. Singhal and R. K. Brayton},
  title = {Verifying Interacting Finite State Machines: Complexity Issues},
  institution = {University of California at Berkeley},
  year = {1993},
  number = {UCB/ERL M93/52},
  month = {July},
  file = {:./files/1993-AzizSinghal.etal.pdf:PDF}
}

@MISC{2000-MarthiWhitney,
  author = {B.Marthi and M.Whitney},
  title = {Fault-Tolerant Quantum Computing},
  year = {2000},
  file = {:./files/2000-MarthiWhitney.pdf:PDF},
  owner = {stoffel},
  timestamp = {2006.09.14}
}

@INPROCEEDINGS{2008-BabicHutter,
  author = {Domagoj Babi\'c and Frank Hutter},
  title = {Spear Theorem Prover},
  booktitle = {Proc. of the {SAT} 2008 Race},
  year = {2008},
  file = {:./files/2008-BabicHutter.pdf:PDF}
}

@INPROCEEDINGS{2008-BabicHu,
  author = {Babic, Domagoj and Hu, Alan J.},
  title = {Calysto: scalable and precise extended static checking},
  booktitle = {Proceedings of the 30th {I}nternational {C}onference on {S}oftware
	{E}ngineering},
  year = {2008},
  series = {ICSE '08},
  pages = {211--220},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {1368118},
  file = {2008-BabicHu.pdf:files/2008-BabicHu.pdf:PDF},
  isbn = {978-1-60558-079-1},
  keywords = {formal verification, static analysis, static checking},
  location = {Leipzig, Germany},
  numpages = {10},
  owner = {villarraga},
  timestamp = {2012.08.27}
}

@ARTICLE{2006-BabighianBenini.etal,
  author = {Babighian, P. and Benini, L. and Macii, E.},
  title = {A Scalable Algorithm for {RTL} Insertion of Gated Clocks Based on
	{ODC}s Computation},
  journal = {IEEE Transactions on Computer-Aided Design of Integrated Circuits
	and Systems},
  year = {2006},
  volume = {24},
  pages = {29--42},
  number = {1},
  month = nov,
  acmid = {2301115},
  address = {Piscataway, NJ, USA},
  issue_date = {November 2006},
  keywords = {Low-power design, low-power dissipation},
  numpages = {14},
  owner = {udupi},
  publisher = {IEEE Press},
  timestamp = {2015.05.05}
}

@INPROCEEDINGS{2007-BabighianKamhi.etal,
  author = {P. Babighian and G. Kamhi and M. Vardi},
  title = {{PowerQuest}: Trace-Driven Data Mining for Power Optimization},
  booktitle = {2007 Design, Automation Test in Europe Conference Exhibition},
  year = {2007},
  pages = {1-6},
  month = {April},
  issn = {1530-1591}
}

@INCOLLECTION{1998-BachmannSchonemann,
  author = {Bachmann,O. and Sch\"onemann,H.},
  title = {Monomial Representations for {Gr\"obner} Bases Computations},
  booktitle = {Reports On Computer Algebra},
  publisher = {Centre for Computer Algebra,Technische Universit{\"a}t Kaiserslautern},
  year = {1998},
  number = {18},
  month = {January},
  file = {:./files/1998-BachmannSchonemann.pdf:PDF},
  owner = {wedler},
  timestamp = {2008.02.18}
}

@INPROCEEDINGS{1993-BaharFrohm.etal,
  author = {R. I. Bahar and E. A. Frohm and C. M. Gaona and G. Hachtel and E.
	Macii and A. Pardo and F. Somenzi},
  title = {Algebraic Decision Diagrams and their Application},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {1993},
  pages = {188 -191},
  file = {:./files/1993-BaharFrohm.etal.pdf:PDF}
}

@INPROCEEDINGS{2005-BalakrishnanReps.etal,
  author = {G. Balakrishnan and T. Reps and D.Melski and T. Teitelbaum},
  title = {{WYSINWYX}: What You See Is Not What You Execute},
  booktitle = {Working Conference on Verified Software},
  year = {2005},
  file = {:./files/2005-BalakrishnanReps.etal.pdf:PDF},
  timestamp = {2006.09.22}
}

@INPROCEEDINGS{2005a-BalakrishnanReps.etal,
  author = {G. Balakrishnan and T. Reps and N. Kidd and A. Lal and J. Lim and
	D. Melski and R. Gruian and S. Yong and C.-H. Chen and T. Teitelbaum},
  title = {Model Checking {X86} Executables With Code Surfer {X86} And {WPDS}},
  booktitle = {Computer Aided Verification ({CAV})},
  year = {2005},
  pages = {158-163},
  file = {:./files/2005a-BalakrishnanReps.etal.pdf:PDF},
  timestamp = {2006.09.22}
}

@INPROCEEDINGS{1998-BalakrishnanTahar,
  author = {Subhashini Balakrishnan and Sofiene Tahar},
  title = {Modeling and Formal Verification of a Commercial Microcontroller
	for Embedded System Applications},
  booktitle = {Proc. {IEEE} International Conference on Microelectronics ({ICM})},
  year = {1998},
  pages = {107 -110},
  file = {:./files/1998-BalakrishnanTahar.pdf:PDF},
  keywords = {PIC 16C71;RTL model;assembly language;embedded system;flowchart;formal
	verification;instruction set architecture;microcontroller;mouse controller;multiway
	decision graph;directed graphs;embedded systems;flowcharting;formal
	verification;instruction sets;microcontrollers;},
  timestamp = {2006.09.27}
}

@ARTICLE{2003-BalarinWatanabe.etal,
  author = {Felice Balarin and Yosinori Watanabe and Harry Hsieh and Luciano
	Lavagno and Claudio Passerone and Alberto Sangiovanni-Vincentelli},
  title = {Metropolis: An Integrated Electronic System Design Environment},
  journal = {Computer},
  year = {2003},
  volume = {36},
  pages = {45-52},
  number = {4},
  address = {Los Alamitos, CA, USA},
  file = {:./files/2003-BalarinWatanabe.etal.pdf:PDF},
  issn = {0018-9162},
  publisher = {IEEE Computer Society}
}

@ARTICLE{1975-Balas,
  author = {Egon Balas},
  title = {Facets of the knapsack Polytope},
  journal = {Mathematical Programming},
  year = {1975},
  volume = {8},
  pages = {146-164},
  file = {:./files/1975-Balas.pdf:PDF}
}

@ARTICLE{2001-BalasCeria.etal,
  author = {Egon Balas and Sebastian Ceria and Milind Dawande and Francois Margot
	and Gabor Pataki},
  title = {{OCTANE}: A New Heuristic for Pure 0-1 Programs},
  journal = {Operations Research},
  year = {2001},
  volume = {49},
  pages = {207-225},
  number = {2},
  file = {:./files/2001-BalasCeria.etal.pdf:PDF}
}

@ARTICLE{1980-BalasMartin,
  author = {Egon Balas and Clarence H. Martin},
  title = {Pivot-and-Complement: A Heuristic for 0-1 Programming},
  journal = {Management Science},
  year = {1980},
  volume = {26},
  pages = {86-96},
  number = {1},
  url = {http://mansci.journal.informs.org/content/26/1/86}
}

@ARTICLE{2004-BalasSchmieta.etal,
  author = {Egon Balas and Stefan Schmieta and Christopher Wallace},
  title = {Pivot and Shift - A Mixed Integer Programming Heuristic},
  journal = {Discrete Optimization},
  year = {2004},
  volume = {1},
  pages = {3 - 12},
  number = {1},
  file = {:./files/2004-BalasSchmieta.etal.pdf:PDF},
  issn = {1572-5286}
}

@INPROCEEDINGS{1995-BalivadaHoskote.etal,
  author = {Balivada, A. and Hoskote, Y. and Abraham, J.A.},
  title = {Verification of Transient Response of Linear Analog Circuits},
  booktitle = {{VLSI} Test Symposium, 1995. Proceedings., 13th {IEEE}},
  year = {1995},
  pages = {42 -47},
  month = {apr-3 may},
  file = {:./files/1995-BalivadaHoskote.etal.pdf:PDF},
  keywords = {Z-domain;circuit behavior;digital representation;extracted state equations;finite
	state machines;formal techniques;input waveforms;linear analog circuits;operational
	amplifier macro circuits;transfer function;transient response;active
	networks;analogue circuits;equivalent circuits;frequency-domain analysis;linear
	network analysis;operational amplifiers;state-space methods;transfer
	functions;transient analysis;transient response;}
}

@INPROCEEDINGS{2006-BallBounimova.etal,
  author = {Thomas Ball and Ella Bounimova and Byron Cook and Vladimir Levin
	and Jakob Lichtenberg and Con McGarvey and Bohus Ondrusek and Sriram
	K. Rajamani and Abdullah Ustuner},
  title = {Thorough Static Analysis of Device Drivers},
  booktitle = {Proceedings of the 2006 {EuroSys} conference},
  year = {2006},
  pages = {73--85},
  address = {New York, NY, USA},
  publisher = {ACM Press},
  file = {:./files/2006-BallBounimova.etal.pdf:PDF},
  isbn = {1-59593-322-0},
  location = {Leuven, Belgium},
  owner = {wedler},
  timestamp = {2007.04.13}
}

@INPROCEEDINGS{2004-BallCook.etal,
  author = {Thomas Ball and Byron Cook and Vladimir Levin and Sriram K. Rajamani},
  title = {{SLAM and static driver verifier: Technology transfer of formal methods
	inside Microsoft}},
  booktitle = {IFM},
  year = {2004},
  pages = {1--20},
  publisher = {Springer},
  owner = {stoffel},
  timestamp = {2016.05.10}
}

@INPROCEEDINGS{2001-BallMajumdar,
  author = {Thomas Ball and Rupak Majumdar},
  title = {Automatic Predicate Abstraction Of C Programs},
  booktitle = {Proceedings of the ACM SIGPLAN 2001 conference on Programming language
	design and implementation},
  year = {2001},
  series = {PLDI '01},
  pages = {203--213},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {378846},
  file = {:./files/2001-BallMajumdar.pdf:PDF},
  isbn = {1-58113-414-2},
  location = {Snowbird, Utah, United States},
  numpages = {11},
  timestamp = {2006.09.22}
}

@ARTICLE{2005-BallMillstein.etal,
  author = {Thomas Ball and Todd Millstein and Sriram K. Rajamani},
  title = {Polymorphic predicate abstraction},
  journal = {{ACM} Transactions on Programming Languages and Systems ({TOPLAS})},
  year = {2005},
  volume = {27},
  pages = {314--343},
  number = {2},
  address = {New York, NY, USA},
  file = {:./files/2005-BallMillstein.etal.pdf:PDF},
  issn = {0164-0925},
  owner = {wedler},
  publisher = {ACM Press},
  timestamp = {2007.04.13}
}

@INPROCEEDINGS{2001-BallPodelski.etal,
  author = {Ball, Thomas and Podelski, Andreas and Rajamani, Sriram K.},
  title = {{Boolean} and {Cartesian} Abstraction for Model Checking {C} Programs},
  booktitle = {Proceedings of the 7th International Conference on Tools and Algorithms
	for the Construction and Analysis of Systems},
  year = {2001},
  series = {TACAS 2001},
  pages = {268--283},
  address = {London, UK},
  publisher = {Springer-Verlag},
  acmid = {759192},
  file = {2001-BallPodelski.etal.pdf:files/2001-BallPodelski.etal.pdf:PDF},
  isbn = {3-540-41865-2},
  numpages = {16},
  owner = {villarraga},
  timestamp = {2012.08.27}
}

@INPROCEEDINGS{2002-BallRajamani,
  author = {T. Ball and S. K. Rajamani},
  title = {The {SLAM} Project: Debugging System Software via Static Analysis}
}

@TECHREPORT{2002a-BallRajamani,
  author = {Thomas Ball and Sriram K. Rajamani},
  title = {SLIC: A Specification Language for Interface Checking (of C)},
  institution = {Microsoft Research},
  year = {2002},
  number = {MSR-TR-2001-21},
  month = {January},
  owner = {villarraga},
  timestamp = {2014.04.15}
}

@INCOLLECTION{2013b-BaoBormann.etal.pdf,
  author = {Bao, Binghao and Bormann, J{\"o}rg and Wedler, Markus and Stoffel,
	Dominik and Kunz, Wolfgang},
  title = {Formal Plausibility Checks for Environment Constraints},
  booktitle = {Models, Methods, and Tools for Complex Chip Design},
  publisher = {Springer International Publishing},
  year = {2014},
  editor = {Haase, Jan},
  volume = {265},
  series = {Lecture Notes in Electrical Engineering},
  pages = {1-16},
  file = {:files/2013b-BaoBormann.etal.pdf:PDF},
  owner = {bao},
  timestamp = {2013.11.12}
}

@INPROCEEDINGS{2013a-BaoBormann.etal,
  author = {Binghao Bao and J{\"o}rg Bormann and Markus Wedler and Dominik Stoffel
	and Wolfgang Kunz},
  title = {Compositional Completeness over reactive Constraints},
  booktitle = {16. {GI/ITG/GMM} Workshop Methoden und Beschreibungssprachen zur
	Modellierung und Verifikation von Schaltungen und Systemen ({MBMV})},
  year = {2013},
  file = {:files/2013a-BaoBormann.etal.pdf:PDF},
  owner = {bao},
  timestamp = {2013.11.12}
}

@INPROCEEDINGS{2012-BaoBormann.etal,
  author = {Binghao Bao and J{\"o}rg Bormann and Markus Wedler and Dominik Stoffel
	and Wolfgang Kunz},
  title = {Formal Plausibility Checks for Environment Constraints},
  booktitle = {Proc. Forum on Specification \& Design Languages(FDL)},
  year = {2012},
  owner = {bao},
  timestamp = {2012.10.24}
}

@INCOLLECTION{2015-BaoVillarraga.etal,
  author = {Bao, Binghao and Villarraga, Carlos and Schmidt, Bernard and Stoffel,
	Dominik and Kunz, Wolfgang},
  title = {A New Property Language for the Specification of Hardware-Dependent
	Embedded System Software},
  booktitle = {Languages, Design Methods, and Tools for Electronic System Design},
  publisher = {Springer International Publishing},
  year = {2016},
  editor = {Oppenheimer, Frank and Medina Pasaje, Julio Luis},
  volume = {361},
  series = {Lecture Notes in Electrical Engineering},
  pages = {83-100},
  isbn = {978-3-319-24455-6},
  language = {English},
  owner = {stoffel},
  timestamp = {2016.05.10}
}

@INPROCEEDINGS{2014-BaoVillarraga.etal,
  author = {Bao, Binghao and Villarraga, Carlos and Schmidt, Bernard and Stoffel,
	Dominik and Kunz, Wolfgang},
  title = {A New Property Language for the Specification of Hardware-Dependent
	Embedded System Software},
  booktitle = {Proc. Forum on Specification And Design Languages (FDL)},
  year = {2014},
  address = {Munich, Germany},
  month = {Oct},
  note = {(accepted for publication)},
  owner = {stoffel},
  timestamp = {2014.07.01}
}

@ARTICLE{2015-BaranowskiKochte.etal,
  author = {Rafal Baranowski and Michael A. Kochte and Hans-Joachim Wunderlich},
  title = {Reconfigurable Scan Networks: Modeling, Verification, and Optimal
	Pattern Generation},
  journal = {ACM Trans. Des. Autom. Electron. Syst.},
  year = {2015},
  volume = {20},
  pages = {30:1-30:27},
  number = {2},
  month = {March},
  acmid = {2699863},
  articleno = {30},
  file = {2015-BaranowskiKochte.etal.pdf:files/2015-BaranowskiKochte.etal.pdf:PDF},
  issn = {1084-4309},
  issue_date = {February 2015},
  numpages = {27},
  owner = {bartsch},
  publisher = {ACM},
  timestamp = {2016.09.22}
}

@INPROCEEDINGS{2016-BaranowskiTrunzer,
  author = {Rafal Baranowski and Marco Trunzer},
  title = {Complete Formal Verification of a Family of Automotive {DSP}s},
  booktitle = {Proc. Design and Verification Conference Europe (DVCON-Europe)},
  year = {2016},
  file = {:files/2016-BaranowskiTrunzer.pdf:PDF},
  owner = {stoffel},
  timestamp = {2019.01.11}
}

@INPROCEEDINGS{2009-BarbaRincon.etal,
  author = {Jes{\'{u}}s Barba and Fernando Rinc{\'{o}}n and Francisco Moya and
	David Villa and Felix Jes{\'{u}}s Villanueva and Juan Carlos L{\'{o}}pez},
  title = {Automatic {HW/SW} Interface Generation for Seamless Integration from
	Object-Oriented Models},
  booktitle = {Proceedings of the 2009 International Conference on Embedded Systems
	{\&} Applications, {ESA} 2009, July 13-16, 2009, Las Vegas Nevada,
	{USA}},
  year = {2009},
  pages = {169--175},
  owner = {fehmel},
  timestamp = {2019.05.27}
}

@ARTICLE{1975-Barbacci,
  author = {Barbacci, Mario R.},
  title = {A Comparison of Register Transfer Languages for Describing Computers
	and Digital Systems},
  journal = {IEEE Trans. Comput.},
  year = {1975},
  volume = {24},
  pages = {137--150},
  number = {2},
  month = feb,
  address = {Washington, DC, USA},
  issn = {0018-9340},
  issue_date = {February 1975},
  numpages = {14},
  owner = {stoffel},
  publisher = {IEEE Computer Society},
  timestamp = {2016.05.10}
}

@ARTICLE{2005-BarnerGlazberg.etal,
  author = {Sharon Barner and Ziv Glazberg and Ishai Rabinovitz},
  title = {Wolf-Bug Hunter For Concurrent Software Using Formal Methods},
  journal = {Lecture notes in computer science},
  year = {2005},
  volume = {3576},
  pages = {153-157},
  file = {:./files/2005-BarnerGlazberg.etal.pdf:PDF},
  timestamp = {2006.09.22}
}

@INPROCEEDINGS{2003-BarnerRabinovitz,
  author = {Sharon Barner and Ishai Rabinovitz},
  title = {Efficient Symbolic Model Checking Of Software Using Partial Disjunctive
	Partitioning},
  booktitle = {Proc. Advanced Research Working Conference on Correct Hardware Design
	and Verification Methods},
  year = {2003},
  editor = {Geist, Daniel and Tronci, Enrico},
  volume = {2860},
  series = {Lecture Notes in Computer Science},
  pages = {35-50},
  publisher = {Springer Berlin / Heidelberg},
  note = {10.1007/978-3-540-39724-3_6},
  file = {:./files/2003-BarnerRabinovitz.pdf:PDF},
  isbn = {978-3-540-20363-6},
  keyword = {Computer Science},
  timestamp = {2006.09.22}
}

@INPROCEEDINGS{2010-BarrettStump.etal,
  author = {Clark Barrett and Aaron Stump and Cesare Tinelli},
  title = {The {SMT-LIB} Standard: Version 2.0},
  booktitle = {Proceedings of the 8th International Workshop on Satisfiability Modulo
	Theories (Edinburgh, England)},
  year = {2010},
  editor = {A. Gupta and D. Kroening},
  file = {:./files/2010-BarrettStump.etal.pdf:PDF},
  owner = {pavlenko},
  timestamp = {2010.06.09}
}

@INPROCEEDINGS{2007-BarrettTinelli,
  author = {Clark Barrett and Cesare Tinelli},
  title = {{CVC3}},
  booktitle = {Proceedings of the $19^{th}$ International Conference on Computer
	Aided Verification ({CAV} '07)},
  year = {2007},
  editor = {Werner Damm and Holger Hermanns},
  volume = {4590},
  series = {Lecture Notes in Computer Science},
  pages = {298--302},
  month = jul,
  publisher = {Springer-Verlag},
  note = {Berlin, Germany},
  file = {:./files/2007-BarrettTinelli.pdf:PDF},
  owner = {pavlenko},
  timestamp = {2010.07.26}
}

@INPROCEEDINGS{1998-BarrettDill.etal,
  author = {Clark. W. Barrett and David. L. Dill and Jeremy R. Levitt},
  title = {A Decision Procedure for Bit-Vector Arithmetic},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {1998},
  pages = {522 -527},
  file = {:./files/1998-BarrettDill.etal.pdf:PDF},
  keywords = {NP-hard;bit-vector arithmetic;decision procedure;hardware verification;digital
	arithmetic;formal verification;},
  owner = {wedler},
  timestamp = {2006.05.30}
}

@INPROCEEDINGS{2002-BarrettDill.etal,
  author = {Barrett, Clark W. and Dill, David L. and Stump, Aaron},
  title = {Checking Satisfiability of First-Order Formulas by Incremental Translation
	to {SAT}},
  booktitle = {CAV '02: Proceedings of the 14th International Conference on Computer
	Aided Verification},
  year = {2002},
  pages = {236--249},
  address = {London, UK},
  publisher = {Springer-Verlag},
  file = {:./files/2002-BarrettDill.etal.pdf:PDF},
  isbn = {3-540-43997-8},
  owner = {pavlenko},
  timestamp = {2010.07.26}
}

@MASTERSTHESIS{2013-ChristianBartsch,
  author = {Christian Bartsch},
  title = {Erweiterung eines formalen Werkzeugs für die Hardware-Software-Coverifikation
	mit Hilfe vom Simulationstechniken},
  school = {TU Kaiserslautern},
  year = {2013},
  type = {{Diplomarbeit}},
  file = {Diplomarbeit:files/2013-ChristianBartsch.pdf:PDF},
  owner = {bschmidt},
  timestamp = {2014.02.27}
}

@INPROCEEDINGS{2016-BartschRoedel.etal,
  author = {Christian Bartsch and Niko R{\"o}del and Carlos Villarraga and Dominik
	Stoffel Stoffel and Wolfgang Kunz},
  title = {A {HW}-dependent Software Model for Cross-Layer Fault Analysis in
	Embedded Systems},
  booktitle = {17th Latin-American Test Symposium (LATS)},
  year = {2016},
  pages = {153-158},
  month = {April},
  file = {2016-BartschRoedel.etal.pdf:files/2016-BartschRoedel.etal.pdf:PDF},
  owner = {bartsch},
  timestamp = {2016.07.19}
}

@INPROCEEDINGS{2015-BartschRoedel.etal,
  author = {C. Bartsch and N. Roedel and C. Villarraga and D. Stoffel and W.
	Kunz},
  title = {A {HW}-dependent Software Model for Cross-Layer Fault Analysis in
	Embedded Systems},
  booktitle = {International Workshop on Resiliency in Embedded Electronic Systems},
  year = {2015},
  month = {November},
  owner = {bartsch},
  timestamp = {2015.11.09}
}

@INPROCEEDINGS{2014-BartschVillarraga.etal,
  author = {Christian Bartsch and Carlos Villarraga and Bernard Schmidt and Dominik
	Stoffel and Wolfgang Kunz},
  title = {Efficient {SAT}/Simulation-based model generation for low-level embedded
	software},
  booktitle = {17. {GI/ITG/GMM} Workshop Methoden und Beschreibungssprachen zur
	Modellierung und Verifikation von Schaltungen und Systemen ({MBMV})},
  year = {2014},
  pages = {147-157},
  file = {:files/2014-BartschVillarraga.etal.pdf:PDF},
  owner = {bschmidt},
  timestamp = {2014.01.20}
}

@ARTICLE{2017-BartschVillarraga.etal,
  author = {Christian Bartsch and Carlos Villarraga and Dominik Stoffel Stoffel
	and Wolfgang Kunz},
  title = {A {HW/SW} Cross-Layer Approach for Determining Application-Redundant
	Hardware Faults in Embedded Systems},
  journal = {Journal of Electronic Testing},
  year = {2017},
  volume = {33},
  pages = {77--92},
  month = {Feb},
  file = {2017-BartschVillarraga.etal.pdf:files/2017-BartschVillarraga.etal.pdf:PDF},
  owner = {bartsch},
  timestamp = {2019.07.29}
}

@ARTICLE{1997-BartschSchubert,
  author = {E. Bartsch and M. Schubert},
  title = {Mixed Analog-Digital Circuit Modeling Using Event-Driven {VHDL}},
  journal = {{IEEE} International workshop on Behavioral Modeling and Simulation
	- BMAS 97},
  year = {1997},
  file = {:./files/1997-BartschSchubert.pdf:PDF}
}

@BOOK{1977-Barwise,
  title = {Handbook of mathematical logic},
  publisher = {North-Holland Publ.},
  year = {1977},
  author = {Barwise, Jon},
  address = {Amsterdam [u.a.]},
  file = {:./files/1977-Barwise.pdf:PDF},
  owner = {pavlenko},
  timestamp = {2010.07.23}
}

@ARTICLE{2006-BasuDas.etal,
  author = {P. Basu and S. Das and A.Banerjee and P. Dasgupta and P.P. Chakrabarti
	and C.R. Mohan and L. Fix and R. Armoni},
  title = {Design-Intent Coverage-A New Paradigm for Formal Property Verification},
  journal = {{IEEE} Transactions on Computer-Aided Design},
  year = {2006},
  volume = {25},
  pages = {1922-1934},
  number = {10},
  month = {October},
  file = {:./files/2006-BasuDas.etal.pdf:PDF},
  owner = {wedler},
  timestamp = {2006.12.15}
}

@ARTICLE{2011-BauerLeucker.etal,
  author = {Bauer, Andreas and Leucker, Martin and Schallhart, Christian},
  title = {Runtime Verification for LTL and TLTL},
  journal = {ACM Trans. Softw. Eng. Methodol.},
  year = {2011},
  volume = {20},
  pages = {14:1--14:64},
  number = {4},
  month = sep,
  acmid = {2000800},
  address = {New York, NY, USA},
  articleno = {14},
  file = {:files/2011-BauerLeucker.pdf:PDF},
  issn = {1049-331X},
  issue_date = {September 2011},
  keywords = {Assertion checkers, monitors, runtime verification},
  numpages = {64},
  owner = {udupi},
  publisher = {ACM},
  timestamp = {2015.04.29}
}

@INPROCEEDINGS{2002-BaumgartnerKuehlmann.etal,
  author = {Jason Baumgartner and Andreas Kuehlmann and Jacob A. Abraham},
  title = {Property Checking via Structural Analysis},
  booktitle = {Proc. International Conference Computer Aided Verification ({CAV})},
  year = {2002},
  pages = {151--165},
  address = {London, UK},
  publisher = {Springer-Verlag},
  file = {:./files/2002-BaumgartnerKuehlmann.etal.pdf:PDF},
  isbn = {3-540-43997-8},
  owner = {nguyen},
  timestamp = {2007.04.26}
}

@INPROCEEDINGS{2005-BayazitMalik,
  author = {Ali Alphan Bayazit and Sharad Malik},
  title = {Complementary Use of Runtime Validation and Model Checking},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2005},
  pages = { 1052 - 1059},
  file = {:./files/2005-BayazitMalik.pdf:PDF},
  keywords = { bugs detection; cache coherence system; clock cycles; hardware designs;
	model checking; on-chip hardware; runtime error detection; runtime
	validation; token sharing protocol; verification methodology; built-in
	self test; circuit testing; formal verification; modal analysis;},
  timestamp = {2006.09.27}
}

@BOOK{2002-Beck,
  title = {Test Driven Development: By Example},
  publisher = {Addison-Wesley},
  year = {2002},
  author = {Kent Beck},
  owner = {joakim},
  timestamp = {2016.03.18}
}

@INPROCEEDINGS{1995-BeckerDrechsler.etal,
  author = {Bernd Becker and Rolf Drechsler and Michael Theobald},
  title = {{OKFDD}s versus {OBDD}s and {OFDD}s},
  booktitle = {Proceedings of the 22nd International Colloquium on Automata, Languages
	and Programming},
  year = {1995},
  series = {ICALP '95},
  pages = {475--486},
  address = {London, UK, UK},
  publisher = {Springer-Verlag},
  acmid = {685358},
  file = {:./files/1995-BeckerDrechsler.etal.pdf:PDF},
  isbn = {3-540-60084-1},
  numpages = {12},
  timestamp = {2011.06.03}
}

@INPROCEEDINGS{1995-BeerBenDavid.etal,
  author = {Ilan Beer and Shoham Ben-David and Cindy Eisner and Yechiel Engel
	and Raanan Gewirtzman and Avner Landver},
  title = {Establishing {PCI} Compliance Using Formal Verification A Case Study},
  booktitle = {Proc. International Conference Proceedings Computers and Communications},
  year = {1995},
  pages = {373 -377},
  file = {:./files/1995-BeerBenDavid.etal.pdf:PDF},
  keywords = { PCI bus bridges; formal verification; symbolic model checking; computer
	interfaces; formal verification; logic testing;},
  timestamp = {2006.09.19}
}

@INPROCEEDINGS{2001-BeerBenDavid.etal,
  author = {Beer, Ilan and Ben-David, Shoham and Eisner, Cindy and Fisman, Dana
	and Gringauze, Anna and Rodeh, Yoav},
  title = {The Temporal Logic Sugar},
  booktitle = {Proceedings of the 13th International Conference on Computer Aided
	Verification},
  year = {2001},
  series = {CAV '01},
  pages = {363--367},
  address = {London, UK, UK},
  publisher = {Springer-Verlag},
  acmid = {734116},
  file = {:./files/2001-BeerBenDavid.etal.pdf:PDF},
  isbn = {3-540-42345-1},
  numpages = {5}
}

@ARTICLE{2008-Ben-DavidFisman,
  author = {Ben-David, Shoham and Fisman, Dana and Ruah, Sitvanit},
  title = {Embedding finite automata within regular expressions},
  journal = {Theor. Comput. Sci.},
  year = {2008},
  volume = {404},
  pages = {202--218},
  number = {3},
  month = sep,
  acmid = {1410846},
  address = {Essex, UK},
  file = {:./files/2008-Ben-DavidFisman.pdf:PDF},
  issn = {0304-3975},
  issue_date = {September, 2008},
  keywords = {Embedding, Finite automata, Linear translation, Model checking, On-the-fly,
	PSL, Regular expression},
  numpages = {17},
  publisher = {Elsevier Science Publishers Ltd.}
}

@MISC{2004-BenDavidFisman.etal,
  author = {Shoham Ben-David and Dana Fisman and Sitvanit Ruah},
  title = {Automata Construction For Regular Expressions In Model Checking},
  year = {2004},
  file = {:./files/2004-BenDavidFisman.etal.pdf:PDF},
  owner = {stoffel},
  timestamp = {2006.09.21}
}

@MISC{2016-Beniamini,
  author = {Beniamini, G},
  title = {Extracting qualcomm’s keymaster keys—breaking android full disk encryption},
  year = {2016},
  owner = {fadiheh},
  timestamp = {2018.07.18},
  url = {http://bits-please.blogspot.com/2016/06/extracting-qualcomms-keymaster-keys.html}
}

@INPROCEEDINGS{1997-BeniniDeMicheli.etal,
  author = {L. Benini and G. De Micheli and E. Macii and M. Poncino and R. Scarsi},
  title = {Symbolic synthesis of clock-gating logic for power optimization of
	control-oriented synchronous networks},
  booktitle = {European Design and Test Conference, 1997. ED TC 97. Proceedings},
  year = {1997},
  pages = {514-520},
  month = {Mar},
  owner = {udupi},
  timestamp = {2016.07.21}
}

@INPROCEEDINGS{1994-BeniniSiegel.etal,
  author = {L. Benini and P. Siegel and G. De Micheli},
  title = {Automatic Synthesis of Gated Clocks for Power Reduction in Sequential
	Circuits},
  booktitle = {IEEE Design and Test of Computers},
  year = {1994},
  pages = {32--40},
  owner = {udupi},
  timestamp = {2019.03.26}
}

@PHDTHESIS{1977-Benthem,
  author = {van Benthem, Johan},
  title = {Modal Correspondence Theory},
  school = {Universiteit van Amsterdam},
  year = {1977},
  owner = {joakim},
  timestamp = {2014.08.05}
}

@INPROCEEDINGS{1998-BerezinBiere.etal,
  author = {Berezin, S. and Biere, A. and Clarke, E. M. and Zhu, Y.},
  title = {Combining Symbolic Model Checking with Uninterpreted Functions for
	Out-of-Order Processor Verification},
  booktitle = {Proc. of Intl. Conference on Formal Methods
	in Computer-Aided Design (FMCAD)},
  year = {1998},
	pages = {369--386},
  acmid = {683063},
  isbn = {3-540-65191-8},
  numpages = {18},
  owner = {fadiheh},
  timestamp = {2019.09.03}
}

@INPROCEEDINGS{1997-BerezinCampos.etal,
  author = {Sergey Berezin and Sergio Campos and Edmund M. Clarke},
  title = {Compositional Reasoning in Model Checking},
  booktitle = {Revised Lectures from the International Symposium on Compositionality:
	The Significant Difference},
  year = {1998},
  series = {COMPOS'97},
  pages = {81--102},
  address = {London, UK, UK},
  publisher = {Springer-Verlag},
  acmid = {701964},
  file = {:./files/1997-BerezinCampos.etal.pdf:PDF},
  isbn = {3-540-65493-3},
  numpages = {22},
  timestamp = {2006.09.13}
}

@ARTICLE{2002-BerezinClarke.etal,
  author = {S. Berezin and E. M. Clarke and A. Biere and Y. Zhu},
  title = {Verification of Out-Of-Order Processor Designs Using Model Checking
	and a Light-Weight Completion Function.},
  journal = {Formal Methods in System Design},
  year = {2002},
  volume = {20},
  pages = {159-186},
  number = {2},
  bibsource = {DBLP, http://dblp.uni-trier.de},
  file = {:./files/2002-BerezinClarke.etal.pdf:PDF},
  owner = {wedler},
  timestamp = {2006.08.29}
}

@TECHREPORT{2002-BergKroening.etal,
  author = {Christoph Berg and Daniel Kroening and Dirk Leinenbach},
  title = {Formal verification of the {VAMP} microprocessor (project status)},
  institution = {In Witold Charatonik and Harald Ganzinger, editors, Symposium on
	the Effectiveness of Logic in Computer Science (ELICS02},
  year = {2002},
  file = {:./files/2002-BergKroening.etal.pdf:PDF}
}

@MISC{2004-Bermingham,
  author = {Bermingham},
  title = {{UCE} Final Usability Report},
  year = {2004},
  file = {:./files/2004-Bermingham.pdf:PDF},
  owner = {stoffel},
  timestamp = {2006.09.21}
}

@ARTICLE{2000-BernardeschiFanteschi.etal,
  author = {C. Bernardeschi and A.Fanteschi and L. Simonsini},
  title = {Formally Verifying Fault Tolerant System Design},
  journal = {The Computer Journal},
  year = {2000},
  volume = {43, no.3},
  pages = {191-205},
  file = {:./files/2000-BernardeschiFanteschi.etal.pdf:PDF},
  timestamp = {2006.09.14}
}

@ARTICLE{2002-BernardeschiFantechi.etal,
  author = {Cinzia Bernardeschi and Alessandro Fantechi and Stefania Gnesi},
  title = {Model checking fault tolerant systems},
  journal = {Software Testing, Verification and Reliability},
  year = {2002},
  volume = {12},
  pages = {251 - 275},
  number = {4},
  file = {2002-BernardeschiFantechi.etal.pdf:files/2002-BernardeschiFantechi.etal.pdf:PDF},
  owner = {bartsch},
  publisher = {John Wiley \& Sons, Ltd.},
  timestamp = {2015.09.09}
}

@INCOLLECTION{1999-BernardeschiFantechi.etal,
  author = {Cinzia Bernardeschi and Alessandro Fantechi and Stefania Gnesi},
  title = {Formal Validation of the GUARDS Inter-consistency Mechanism},
  booktitle = {Computer Safety, Reliability and Security},
  publisher = {Springer Berlin Heidelberg},
  year = {1999},
  volume = {1698},
  series = {Lecture Notes in Computer Science},
  pages = {420-430},
  file = {1999-BernardeschiFantechi.etal.pdf:files/1999-BernardeschiFantechi.etal.pdf:PDF},
  isbn = {978-3-540-66488-8},
  owner = {bartsch},
  timestamp = {2015.08.03}
}

@ARTICLE{2014-BernardiCiganda.etal,
  author = {P. Bernardi and L. M. Ciganda and E. Sanchez and M. S. Reorda},
  title = {MIHST: A Hardware Technique for Embedded Microprocessor Functional
	On-Line Self-Test},
  journal = {IEEE Transactions on Computers},
  year = {2014},
  volume = {63},
  pages = {2760-2771},
  number = {11},
  month = {November},
  file = {2014-BernardiCiganda.etal.pdf:files/2014-BernardiCiganda.etal.pdf:PDF},
  issn = {0018-9340},
  owner = {bartsch},
  timestamp = {2016.09.21}
}

@INPROCEEDINGS{2005-BernardinisVincentelli,
  author = {F. De Bernardinis and A. Sangiovanni Vincentelli},
  title = {Efficient Analog Platform Characterization through Analog Constraint
	Graphs},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2005},
  pages = { 415 - 421},
  file = {:./files/2005-BernardinisVincentelli.pdf:PDF},
  keywords = { ADC design; analog circuits; analog constraint graphs; analog platform
	characterization; bipartite graph representation; circuit parameters;
	design parameters; power consumption; random configuration generator;
	system-level models; analogue integrated circuits; graph theory;
	integrated circuit design; integrated circuit modelling;},
  timestamp = {2006.09.27}
}

@INPROCEEDINGS{2002-BerrojoGonzalez.etal,
  author = {L. Berrojo and I. Gonzalez and F. Corno and M. Sonza Reorda and G.
	Squillero and L. Entrena and C. Lopez},
  title = {New Techniques for Speeding-up Fault-injection Campaigns},
  booktitle = {Proc. International Conference on Design, Automation and Test in
	Europe ({DATE})},
  year = {2002},
  pages = {847 -852},
  file = {:./files/2002-BerrojoGonzalez.etal.pdf:PDF},
  keywords = {ASIC;CAD tools;FPGA;RT-level VHDL descriptions;VHDL parsing;VHDL simulation;automatic
	insertion;automatic validation;fault-injection campaigns;fault-injection
	platform;fault-tolerant circuits;fault-tolerant mechanisms;industrial
	environment applications;application specific integrated circuits;circuit
	CAD;fault simulation;fault tolerance;field programmable gate arrays;hardware
	description languages;technology CAD (electronics);},
  timestamp = {2006.09.14}
}

@ARTICLE{1996-BerrouGlavieux,
  author = {Berrou, C. and Glavieux, A.},
  title = {Near optimum error correcting coding and decoding: turbo-codes},
  journal = {Communications, IEEE Transactions on},
  year = {1996},
  volume = {44},
  pages = {1261 -1271},
  number = {10},
  month = {oct},
  file = {:./files/1996-BerrouGlavieux.pdf:PDF},
  issn = {0090-6778},
  keywords = {concatenation;convolutional codes;correcting performance;extrinsic
	information;iterative processing;near optimum error correcting coding;near
	optimum error correcting decoding;nonuniform interleaving;recursive
	systematic codes;turbo-codes;codecs;convolutional codes;decoding;error
	correction codes;interleaved codes;iterative methods;}
}

@INPROCEEDINGS{2003-BerryKishinevsky.etal,
  author = {Gerard Berry and Michael Kishinevsky and Satnam Singh},
  title = {System Level Design and Verification Using a Synchronous Language},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2003},
  pages = { 433 - 439},
  month = {nov.},
  file = {:./files/2003-BerryKishinevsky.etal.pdf:PDF},
  keywords = { Esterel models; HDL; IP blocks; RTL; VHDL; VHSIC HDL; bus protocol;
	correct-by-construction compilation technique; correct-by-construction
	verification technique; design space exploration; event based simulation;
	formal semantics; formal verification; hardware description language;
	resistor-transistor logic; synchronous language; system Verilog;
	system level design; system level languages; system level tools;
	system level verification; systemC language; very high speed integrated
	circuit; formal specification; formal verification; hardware-software
	codesign; programming language semantics;},
  timestamp = {2006.09.22}
}

@ARTICLE{1992-BerryGonthier,
  author = {Berry, G{\'e}rard and Gonthier, Georges},
  title = {{The ESTEREL Synchronous Programming Language: Design, Semantics,
	Implementation}},
  journal = {Sci. Comput. Program.},
  year = {1992},
  volume = {19},
  pages = {87--152},
  number = {2},
  month = nov,
  acmid = {147279},
  address = {Amsterdam, The Netherlands, The Netherlands},
  issn = {0167-6423},
  issue_date = {Nov. 1992},
  numpages = {66},
  owner = {joakim},
  publisher = {Elsevier North-Holland, Inc.},
  timestamp = {2015.04.24}
}

@BOOK{2013-BertotCasteran,
  title = {Interactive theorem proving and program development: Coq’Art: the
	calculus of inductive constructions},
  publisher = {Springer Science \& Business Media},
  year = {2013},
  author = {Bertot, Yves and Cast{\'e}ran, Pierre},
  owner = {fadiheh},
  timestamp = {2018.07.17}
}

@MISC{2001-Besemer,
  author = {Thomas E. Besemer},
  title = {Managing Embedded Software Development},
  year = {2001},
  file = {:./files/2001-Besemer.pdf:PDF},
  owner = {stoffel},
  timestamp = {2006.10.04}
}

@BOOK{1985-BestRitter,
  title = {Linear Programming},
  publisher = {Prentice Hall},
  year = {1985},
  author = {M. J. Best and K. Ritter}
}

@TECHREPORT{1990a-BevierYoung,
  author = {William R. Bevier and William D. Young},
  title = {Machine Checked Proofs of the Design and Implementation of a Fault-Tolerant
	Circuit},
  institution = {NASA Contractor Report 182099},
  year = {1990},
  file = {:./files/1990a-BevierYoung.pdf:PDF},
  timestamp = {2006.09.14}
}

@TECHREPORT{1990-BevierYoung,
  author = {William R. Bevier and William D. Young},
  title = {The Proof of Correctness of a Fault-Tolerant Circuit Design},
  institution = {Computational Logic Inc.},
  year = {1990},
  file = {:./files/1990-BevierYoung.pdf:PDF},
  timestamp = {2006.09.14}
}

@INCOLLECTION{2004-BeyerDirk.etal,
  author = {Beyer, Dirk and Chlipala, AdamJ. and Henzinger, ThomasA. and Jhala,
	Ranjit and Majumdar, Rupak},
  title = {The Blast Query Language for Software Verification},
  booktitle = {Static Analysis},
  publisher = {Springer Berlin Heidelberg},
  year = {2004},
  editor = {Giacobazzi, Roberto},
  volume = {3148},
  series = {Lecture Notes in Computer Science},
  pages = {2-18},
  file = {2004-BeyerDirk.etal.pdf:files/2004-BeyerDirk.etal.pdf:PDF},
  isbn = {978-3-540-22791-5},
  owner = {villarraga},
  timestamp = {2014.04.15}
}

@ARTICLE{2007-BeyerHenzinger.etal,
  author = {Beyer, Dirk and Henzinger, Thomas A. and Jhala, Ranjit and Majumdar,
	Rupak},
  title = {The software model checker {B}last: {A}pplications to {S}oftware
	{E}ngineering},
  journal = {Int. J. Softw. Tools Technol. Transf.},
  year = {2007},
  volume = {9},
  pages = {505--525},
  month = {October},
  acmid = {1296695},
  address = {Berlin, Heidelberg},
  file = {2007-BeyerHenzinger.etal.pdf:files/2007-BeyerHenzinger.etal.pdf:PDF},
  issn = {1433-2779},
  issue = {5},
  keywords = {Memory safety, Model checking, Software specification, Software verification,
	Test-case generation},
  numpages = {21},
  owner = {villarraga},
  publisher = {Springer-Verlag},
  timestamp = {2012.08.27}
}

@INPROCEEDINGS{2005-BhardwajVrudhula,
  author = {Sarvesh Bhardwaj and Sarma Vrudhula},
  title = {Formalizing Designers Preferences for Multiattribute Optimization
	with Application to Leakage-Delay Tradeoffs},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2005},
  pages = { 713 - 718},
  file = {:./files/2005-BhardwajVrudhula.pdf:PDF},
  keywords = { constained optimization; convex gate sizing; energy-delay product;
	geometric programming; leakage-delay tradeoff; multiattribute optimization;
	objective function minimization; utility function; circuit optimisation;
	delay estimation; digital circuits; geometric programming;},
  timestamp = {2006.09.27}
}

@BOOK{1999-Bhasker,
  title = {A Verilog {HDL} Primer, Second Edition},
  publisher = {Star Galaxy Publishing},
  year = {1999},
  author = {Bhasker, J.},
  isbn = {096503917X},
  owner = {pavlenko},
  timestamp = {2010.10.07}
}

@INPROCEEDINGS{2005-BhuniaBanerjee.etal,
  author = {S. Bhunia and N. Banerjee and Q. Chen and H. Mahmoodi and K. Roy},
  title = {A novel synthesis approach for active leakage power reduction using
	dynamic supply gating},
  booktitle = {Proceedings. 42nd Design Automation Conference, 2005.},
  year = {2005},
  file = {:/import/var/jabref/files/2005-BhuniaBanerjee.pdf:PDF},
  issn = {0738-100X},
  owner = {udupi},
  timestamp = {2017.03.28}
}

@INPROCEEDINGS{2015-BidmeshkiMarkis,
  author = {Bidmeshki, Mohammad-Mahdi and Makris, Yiorgos},
  title = {Toward automatic proof generation for information flow policies in
	third-party hardware IP},
  booktitle = {Hardware Oriented Security and Trust (HOST), 2015 IEEE International
	Symposium on},
  year = {2015},
  pages = {163--168},
  organization = {IEEE},
  owner = {fadiheh},
  timestamp = {2018.07.13}
}

@ARTICLE{2008-Biere,
  author = {Armin Biere},
  title = {PicoSAT Essentials},
  journal = {JSAT},
  year = {2008},
  volume = {4},
  pages = {75-97},
  number = {2-4},
  owner = {marx},
  timestamp = {2012.11.09}
}

@MISC{2004-Biere,
  author = {Armin Biere},
  title = {No Need For Liveness Model Checking Algorithms},
  year = {2004},
  file = {:./files/2004-Biere.pdf:PDF},
  owner = {stoffel},
  timestamp = {2006.09.19}
}

@INPROCEEDINGS{2015-BiereForehlich,
  author = {Biere, Armin and Fr{\"o}hlich Andreas},
  title = {Evaluating {CDCL} Restart Schemes},
  booktitle = {Pragmatics of SAT 2015},
  year = {2015},
  owner = {villarraga},
  timestamp = {2016.07.27}
}

@INPROCEEDINGS{2002-BiereArtho.etal,
  author = {A. Biere and C. Artho and V. Schuppan},
  title = {Liveness Checking as Safety Checking},
  booktitle = {Proc. of 7. International Workshop on Formal Methods for Industrial
	Critical Systems (FMICS)},
  year = {2002},
  volume = {66},
  month = {July},
  file = {:./files/2002-BiereArtho.etal.pdf:PDF}
}

@BOOK{2003-BiereCimatti.etal,
  title = {Bounded Model Checking, Advances In Computers Volume 58},
  publisher = {Academic Press},
  year = {2003},
  author = {A. Biere and A. Cimatti and E. Clarke and O. Strichman and Y. Zhu},
  file = {:./files/2003-BiereCimatti.etal.pdf:PDF}
}

@INPROCEEDINGS{1999-BiereCimatti.etal,
  author = {A. Biere and A. Cimatti and E. Clarke and Y. Zhu},
  title = {Symbolic Model Checking Without {BDD}s},
  booktitle = {Proceedings of the 5th International Conference on Tools and Algorithms
	for Construction and Analysis of Systems},
  year = {1999},
  series = {TACAS '99},
  pages = {193--207},
  address = {London, UK, UK},
  publisher = {Springer-Verlag},
  acmid = {691738},
  file = {:./files/1999-BiereCimatti.etal.pdf:PDF},
  isbn = {3-540-65703-7},
  numpages = {15},
  owner = {thalmaier},
  timestamp = {2006.10.25}
}

@INPROCEEDINGS{1999a-BiereCimatti.etal,
  author = {A. Biere and A. Cimatti and E. M. Clarke and M. Fujita and Y. Zhu},
  title = {Symbolic Model Checking Using {SAT} Procedures Instead of {BDD}s},
  booktitle = {Proc. Design Automation Conference ({DAC})},
  year = {1999},
  pages = {317-320},
  month = {June},
  file = {:./files/1999a-BiereCimatti.etal.pdf:PDF}
}

@INPROCEEDINGS{1999-BiereClarke.etal,
  author = {A. Biere and E. Clarke and R. Raimi and Y. Zhu},
  title = {Verifying Safety Properties Of A Power {PC}-{TM} Microprocessor Using
	Symbolic Model Checking Without {BDD}s},
  booktitle = {Proc. International Conference on Computer Aided Verification ({CAV})},
  year = {1999},
  pages = {60--71},
  file = {:./files/1999-BiereClarke.etal.pdf:PDF},
  timestamp = {2006.10.04}
}

@INPROCEEDINGS{2002-BiereKunz,
  author = {Armin Biere and W. Kunz},
  title = {{SAT} and {ATPG}: {Boolean} Engines for Formal Hardware Verification},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2002},
  pages = { 782 - 785},
  address = {San Jose},
  month = {November},
  file = {:./files/2002-BiereKunz.pdf:PDF},
  keywords = { ATPG; {Boolean} engines; SAT; combinational equivalence checking;
	conjunctive normal form; formal hardware verification; property checking;
	satisfiability; {Boolean} functions; automatic test pattern generation;
	circuit analysis computing; computability; formal verification;}
}

@MISC{2006-BiereStrichman,
  author = {Armin Biere and Ofer Strichman},
  title = {{BMC}-Preproceedings},
  year = {2006},
  file = {:./files/2006-BiereStrichman.pdf:PDF},
  owner = {stoffel},
  timestamp = {2006.09.21}
}

@INPROCEEDINGS{1994-BitnerJain.etal,
  author = {James R. Bitner and Jawahar Jain and Magdy S. Abadir and Jacob A.
	Abraham and Donald S. Fussell},
  title = {Efficient Algorithmic Circuit Verification Using Indexed {BDD}s},
  booktitle = {Proc. Fault Tolerant Computing Symposium ({FTCS})},
  year = {1994},
  pages = {266-275},
  file = {:./files/1994-BitnerJain.etal.pdf:PDF}
}

@INCOLLECTION{2000-BixbyFenelon.etal,
  author = {Robert E. Bixby and M. Fenelon and Zonghao Gu and Ed Rothberg and
	Roland Wunderling},
  title = {{MIP}: Theory and Practice - Closing the Gap},
  booktitle = {Systems Modelling and Optimization: Methods, Theory, and Applications},
  publisher = {Kluwer},
  year = {2000},
  editor = {M.J.D. Powell and S. Scholtes},
  pages = {19-49},
  file = {:./files/2000-BixbyFenelon.etal.pdf:PDF}
}

@INPROCEEDINGS{2000-BjesseClaessen,
  author = {P. Bjesse and K. Claessen},
  title = {{SAT}-Based Verification without State Space Traversal},
  booktitle = {Proc. International Conference on Formal Methods in Computer-Aided
	Design ({FMCAD})},
  year = {2000},
  series = {FMCAD '00},
  pages = {372-389},
  address = {London, UK, UK},
  publisher = {Springer-Verlag},
  acmid = {683097},
  file = {:./files/2000-BjesseClaessen.pdf:PDF},
  isbn = {3-540-41219-0},
  numpages = {18},
  timestamp = {2006.09.19},
  url = {citeseer.nj.nec.com/328468.html}
}

@MISC{2005-BjesseHu,
  author = {Per Bjesse and Alan Hu},
  title = {Bounded Model Checking Preliminary Proceedings},
  year = {2005},
  file = {:./files/2005-BjesseHu.pdf:PDF},
  owner = {stoffel},
  timestamp = {2006.09.19}
}

@INPROCEEDINGS{2005-BjesseKukula,
  author = {Per Bjesse and James Kukula},
  title = {Automatic Generalized Phase Abstraction for Formal Verification},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2005},
  pages = { 1076 - 1082},
  file = {:./files/2005-BjesseKukula.pdf:PDF},
  keywords = { HDL code analysis; N-phase design style; clocks; combinational logic;
	formal verification; model checking; phase abstraction algorithm;
	syntactic analysis; circuit complexity; clocks; combinational circuits;
	formal verification;},
  timestamp = {2006.09.27}
}

@INPROCEEDINGS{1996-BlackHall.etal,
  author = {P. E. {Black} and K. M. {Hall} and M. D. {Jones} and T. N. {Larson}
	and P. J. {Windley}},
  title = {A brief introduction to formal methods},
  booktitle = {Proceedings of Custom Integrated Circuits Conference},
  year = {1996},
  pages = {377-380},
  month = {May},
  doi = {10.1109/CICC.1996.510579},
  file = {:files/1996-BlackHall.etal.pdf:PDF},
  keywords = {formal specification;logic CAD;circuit CAD;formal verification;logic
	design;formal methods;hardware design;logic systems;inference;specifications;implementation
	models;Mathematical model;Design methodology;Hardware;Laboratories;Logic
	design;Testing;Software design;Computer errors;Contracts;Software
	systems},
  owner = {udupi},
  timestamp = {2019.03.09}
}

@INPROCEEDINGS{2014-BleikertzVogel.etal,
  author = {Bleikertz, S{\"o}ren and Vogel, Carsten and Gro{\ss}, Thomas},
  title = {Cloud radar: near real-time detection of security failures in dynamic
	virtualized infrastructures},
  booktitle = {Proceedings of the 30th annual computer security applications conference},
  year = {2014},
  pages = {26--35},
  organization = {ACM},
  owner = {fadiheh},
  timestamp = {2018.07.12}
}

@TECHREPORT{2002-BleyKoch,
  author = {Andreas Bley and Thorsten Koch},
  title = {Integer Programming Approaches to Access and Backbone {IP}-Network
	Planning},
  institution = {Zuse Institute Berlin},
  year = {2002},
  number = {02-41},
  file = {:./files/2002-BleyKoch.pdf:PDF},
  language = {English}
}

@ARTICLE{2007-BloemGaller.etal,
  author = {Roderick Bloem and Stefan Galler and Barbara Jobstmann and Nir Piterman
	and Amir Pnueli and Martin Weiglhofer},
  title = {Specify, Compile, Run: Hardware from {PSL}},
  journal = {Electronic Notes in Theoretical Computer Science},
  year = {2007},
  volume = {190},
  pages = {3--16},
  number = {4},
  address = {Amsterdam, The Netherlands, The Netherlands},
  file = {:./files/2007-BloemGaller.etal.pdf:PDF},
  issn = {1571-0661},
  publisher = {Elsevier Science Publishers B. V.}
}

@MISC{Project-Verisoft,
  author = {{BMBF}},
  title = {{Verisoft XT}},
  howpublished = {http://www.verisoftxt.de},
  owner = {stoffel},
  timestamp = {2016.05.10}
}

@INPROCEEDINGS{1994-BochmannPetrenko,
  author = {Gregor v. Bochmann and Alexandre Petrenko},
  title = {Protocol Testing: Review of Methods and Relevance for Software Testing},
  booktitle = {Proceedings of the 1994 {ACM} {SIGSOFT} international symposium on
	Software testing and analysis},
  year = {1994},
  series = {ISSTA '94},
  pages = {109--124},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {187153},
  file = {:./files/1994-BochmannPetrenko.pdf:PDF},
  isbn = {0-89791-683-2},
  location = {Seattle, Washington, United States},
  numpages = {16},
  timestamp = {2006.09.21}
}

@ARTICLE{1998-BockmayrKasper,
  author = {Alexander Bockmayr and Thomas Kasper},
  title = {Branch-and-Infer: A Unifying Framework for Integer and Finite Domain
	Constraint Programming},
  journal = {{INFORMS} Journal on Computing},
  year = {1998},
  volume = {10},
  pages = {287-300},
  number = {3},
  file = {:./files/1998-BockmayrKasper.pdf:PDF}
}

@ARTICLE{2001-BockmayrPisaruk,
  author = {Alexander Bockmayr and Nicolai Pisaruk},
  title = {Solving Assembly Line Balancing Problems by Combining {IP} and {CP}},
  journal = {Computer Research Repository CoRR},
  year = {2001},
  volume = {cs.DM/0106002},
  bibsource = {DBLP, http://dblp.uni-trier.de},
  ee = {http://arxiv.org/abs/cs.DM/0106002},
  file = {:./files/2001-BockmayrPisaruk.pdf:PDF}
}

@INPROCEEDINGS{1995a-BoglioloDamiani,
  author = {Alessandro Bogliolo and Maurizio Damiani},
  title = {Synthesis of Combinational Circuits with Special Fault-Handling Capabilities},
  booktitle = {Proc. {IEEE} {VLSI} Test Symposium ({VTS})},
  year = {1995},
  pages = {454 -459},
  file = {:./files/1995a-BoglioloDamiani.pdf:PDF},
  keywords = {combinational circuit synthesis;fault-handling capabilities;fault-tolerant
	circuits;internal faults;multilevel logic optimization process;redundancy;self-checking
	circuits;circuit optimisation;circuit reliability;combinational circuits;design
	for testability;logic CAD;logic design;logic testing;multivalued
	logic;redundancy;},
  timestamp = {2006.09.14}
}

@INPROCEEDINGS{1995-BoglioloDamiani,
  author = {Alessandro Bogliolo and Maurizio Damiani},
  title = {Synthesis of Multilevel Fault-Tolerant Combinational Circuits},
  booktitle = {Proc. European Confernece on Design and Test},
  year = {1995},
  pages = {80 -85},
  file = {:./files/1995-BoglioloDamiani.pdf:PDF},
  keywords = { benchmark circuits; combinational circuits; fault-masking redundancy;
	fault-tolerant circuits; internal don't care conditions; logic optimization;
	multilevel circuits; circuit CAD; circuit optimisation; combinational
	circuits; logic CAD; multivalued logic circuits; redundancy;},
  timestamp = {2006.09.14}
}

@INPROCEEDINGS{1995-BoglioloDamiani.etal,
  author = {Alessandro Bogliolo and Maurizio Damiani and Piero Olivo and Bruno
	Ricco},
  title = {Reliability Evaluation of Combinational Logic Circuits by Symbolic
	Simulation},
  booktitle = {Proc. {IEEE} {VLSI} Test Symposium ({VTS})},
  year = {1995},
  pages = {235 -242},
  file = {:./files/1995-BoglioloDamiani.etal.pdf:PDF},
  keywords = {BDD-based symbolic simulation;VLSI;circuit functionality;control variables;fault
	indicators;fault-tolerant combinational logic circuits;mcnc benchmark
	circuits;reliability evaluation;undetectable multiple faults;VLSI;circuit
	analysis computing;combinational circuits;digital simulation;integrated
	circuit reliability;logic CAD;},
  timestamp = {2006.09.14}
}

@INPROCEEDINGS{2009-BolzaniCalimera.etal,
  author = {L. Bolzani and A. Calimera and A. Macii and E. Macii and M. Poncino},
  title = {Enabling concurrent clock and power gating in an industrial design
	flow},
  booktitle = {2009 Design, Automation Test in Europe Conference Exhibition},
  year = {2009},
  month = {April},
  file = {:files/2009-BolzianiCalimera.pdf:PDF},
  owner = {udupi},
  timestamp = {2018.06.04}
}

@ARTICLE{2007-BombieriFummi.etal,
  author = {Bombieri, N. and Fummi, F. and Pravadelli, G. and Fedeli, A.},
  title = {Hybrid, Incremental Assertion-Based Verification for {TLM} Design
	Flows},
  journal = {Design Test of Computers, {IEEE}},
  year = {2007},
  volume = {24},
  pages = {140 -152},
  number = {2},
  month = {march-april },
  file = {:./files/2007-BombieriFummi.etal.pdf:PDF},
  issn = {0740-7475},
  keywords = {RTL refinement;TLM design flows;hybrid incremental assertion-based
	verification methodology;industry design;transaction-level modeling;formal
	verification;transaction processing;}
}

@INPROCEEDINGS{2004-BoneIndri.etal,
  author = {Basilio Bona and Marina Indri and Nicola Smaldone},
  title = {Architectures for Rapid Prototyping of Model based Robot Controllers},
  booktitle = {Advances in Control of Articulated and Mobile Robots},
  year = {2004},
  editor = {Siciliano, Bruno and Melchiorri, Claudio and De Luca, Alessandro
	and Casalino, Giuseppe},
  volume = {10},
  series = {Springer Tracts in Advanced Robotics},
  pages = {144-144},
  publisher = {Springer Berlin / Heidelberg},
  note = {10.1007/978-3-540-44410-7_5},
  file = {:./files/2004-BoneIndri.etal.pdf:PDF},
  isbn = {978-3-540-20783-2},
  keyword = {Engineering},
  timestamp = {2006.09.21}
}

@INPROCEEDINGS{2005-BondDaniel,
  author = {Brad Bond and Luca Daniel},
  title = {Parameterized Model Order Reduction of Nonlinear Dynamical Systems},
  booktitle = {Proc. International Conference on Computer-Aided Design (ICCAD)},
  year = {2005},
  pages = { 487 - 494},
  file = {:./files/2005-BondDaniel.pdf:PDF},
  keywords = { MEM switch; analog nonlinear circuit; moment matching; nonlinear
	dynamical system; nonparameterized trajectory piecewise linear method;
	parameterized model order reduction; nonlinear dynamical systems;
	piecewise linear techniques;},
  timestamp = {2006.09.27}
}

@BOOK{1854-Boole,
  title = {An Investigation of the Laws of Thought},
  publisher = {Walton},
  year = {1854},
  author = {George Boole},
  address = {London},
  note = {Reprinted by Dover Books, New York, 1954},
  file = {:./files/1854-Boole.pdf:PDF}
}

@MISC{web_boolector,
  author = {boolector},
  owner = {stoffel},
  timestamp = {2008.10.23},
  url = {http://fmv.jku.at/boolector}
}

@ARTICLE{1951-Booth,
  author = {Andrew D. Booth},
  title = {A Signed Binary Multiplication Technique},
  journal = {Journal of Mechanics and Applied Mathematics},
  year = {1951},
  volume = {IV-2},
  pages = {236-240},
  file = {:./files/1951-Booth.pdf:PDF}
}

@ARTICLE{2011-BorkarShekhar.etal,
  author = {Borkar, Shekhar and Chien, Andrew A.},
  title = {The Future of Microprocessors},
  journal = {Commun. ACM},
  year = {2011},
  volume = {54},
  pages = {67--77},
  number = {5},
  month = may,
  acmid = {1941507},
  address = {New York, NY, USA},
  file = {2011-BorkarShekhar.etal.pdf:files/2011-BorkarShekhar.etal.pdf:PDF},
  issn = {0001-0782},
  issue_date = {May 2011},
  numpages = {11},
  owner = {villarraga},
  publisher = {ACM},
  timestamp = {2016.06.17}
}

@PHDTHESIS{2009-Bormann,
  author = {J{\"o}rg Bormann},
  title = {{Vollst\"andige Verifikation}},
  school = {Technische Universit\"at Kaiserslautern},
  year = {2009},
  type = {Dissertation},
  file = {:./files/2009-Bormann.pdf:PDF}
}

@CONFERENCE{2007-BormannBeyer.etal,
  author = {J. {Bormann} and S. {Beyer} and A. {Maggiore} and M. {Siegel} and S. {Skalberg} and T. {Blackmore} and F. {Bruno}},
  title = {Complete Formal Verification of {TriCore2} and Other Processors},
  booktitle = {Proceedings of {DVCon-US}},
  year = {2007},
  timestamp = {2010.07.05}
}

@MISC{2005-BormannBusch,
  author = {J. {Bormann} and H. {Busch}},
  title = {{Verfahren zur Bestimmung der G\"ute einer Menge von Eigenschaften
	(Method for determining the quality of a set of properties)}},
  howpublished = {European Patent Application, EP1764715},
  month = {09},
  year = {2005},
  owner = {nguyen},
  timestamp = {2008.07.16}
}

@INPROCEEDINGS{1999-BorndoerferGroetschel.etal,
  author = {Ralf Borndorfer and Martin Groetschel and Fridolin Klostermeier and
	Christian Kuettner},
  title = {Telebus Berlin: Vehicle Scheduling in a Dial-a-Ride System},
  booktitle = {Proceedings of the 7th International Workshop on Computer-Aided Transit
	Scheduling},
  year = {1999},
  editor = {Nigel H. M. Wilson},
  pages = {391?422},
  publisher = {Springer},
  classmath = {*90B90 90B06 90C57},
  file = {:./files/1999-BorndoerferGroetschel.etal.pdf:PDF},
  language = {English}
}

@ARTICLE{1997-BosmaCannon.etal,
  author = {Wieb Bosma and John Cannon and Catherine Playoust},
  title = {The {MAGMA} algebra system {I}: the user language},
  journal = {Journal of Symbolic Computation},
  year = {1997},
  volume = {24},
  pages = {235--265},
  number = {3-4},
  address = {Duluth, MN, USA},
  file = {:./files/1997-BosmaCannon.etal.pdf:PDF},
  issn = {0747-7171},
  owner = {wedler},
  publisher = {Academic Press, Inc.},
  timestamp = {2008.01.25}
}

@INPROCEEDINGS{1998-BouePetillon.etal,
  author = {J. Boue and P. Petillon and Y. Crouzet},
  title = {{MEFISTO-L}: a {VHDL}-based fault injection tool for the experimental
	assessment of fault tolerance},
  booktitle = {Digest of Papers. Twenty-Eighth Annual International Symposium on
	Fault-Tolerant Computing},
  year = {1998},
  pages = {168-173},
  month = {June},
  file = {1998-BouePetillon.etal.pdf:files/1998-BouePetillon.etal.pdf:PDF},
  issn = {0731-3071},
  owner = {bartsch},
  timestamp = {2016.11.28}
}

@BOOK{2008-BoulZilic,
  title = {Generating Hardware Assertion Checkers: For Hardware Verification,
	Emulation, Post-Fabrication Debugging and On-Line Monitoring},
  publisher = {Springer Publishing Company, Incorporated},
  year = {2008},
  author = {Boul, Marc and Zilic, Zeljko},
  edition = {1},
  isbn = {1402085850, 9781402085857},
  owner = {joakim},
  timestamp = {2016.07.21}
}

@ARTICLE{2005-BozzanoBruttomesso.etal,
  author = {Marco Bozzano and Roberto Bruttomesso and Alessandro Cimatti and
	Tommi Junttila and Peter van Rossum and Stephan Schulz and Roberto
	Sebastiani},
  title = {{MathSAT}: Tight Integration of {SAT} and Mathematical Decision Procedures},
  journal = {Journal of Automated Reasoning},
  year = {2005},
  volume = {35},
  pages = {265--293},
  number = {1--3},
  month = {oct},
  owner = {wedler},
  timestamp = {2008.02.07}
}

@INPROCEEDINGS{1990-BraceRudell.etal,
  author = {Karl. S. Brace and Richard. L. Rudell and Randal. E. Bryant},
  title = {Efficient Implementation of a {BDD} Package},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {1990},
  pages = {40-45},
  address = {Orlando, FL},
  month = {June},
  file = {:./files/1990-BraceRudell.etal.pdf:PDF}
}

@INPROCEEDINGS{2011-Bradley,
  author = {Bradley, Aaron R.},
  title = {SAT-based model checking without unrolling},
  booktitle = {Proceedings of the 12th international conference on Verification,
	model checking, and abstract interpretation},
  year = {2011},
  series = {VMCAI'11},
  pages = {70--87},
  address = {Berlin, Heidelberg},
  publisher = {Springer-Verlag},
  acmid = {1946291},
  file = {2011-Bradley.pdf:files/2011-Bradley.pdf:PDF},
  isbn = {978-3-642-18274-7},
  location = {Austin, TX, USA},
  numpages = {18},
  owner = {villarraga},
  timestamp = {2012.08.27}
}

@INBOOK{1977-BradleyHax.etal,
  chapter = {IntegerProgramming},
  pages = {272 - 319},
  title = {Applied Mathematical Programming},
  publisher = {Addison-Wesley},
  year = {1977},
  author = {S. Bradley and A. Hax, T. and Magnanti},
  file = {1977-BradleyHax.etal.pdf:files/1977-BradleyHax.etal.pdf:PDF},
  owner = {schwarz},
  timestamp = {2017.01.17}
}

@INPROCEEDINGS{1993a-Brand,
  author = {Daniel Brand},
  title = {Verification of Large Synthesized Designs},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {1993},
  pages = {534-537},
  file = {:./files/1993a-Brand.pdf:PDF}
}

@INPROCEEDINGS{2010-BrandtSchneider.etal,
  author = {Jens Brandt and Klaus Schneider and Sumit Ahuja and Sandeep K. Shukla},
  title = {The Model Checking View to Clock Gating and Operand Isolation},
  booktitle = {Proc. Intl. Conf. on Application of Concurrency to System Design},
  year = {2010},
  pages = {181--190},
  publisher = {IEEE Computer Society},
  acmid = {1844891},
  file = {:files/2010-BrandtSchneider.pdf:PDF},
  numpages = {10},
  owner = {udupi},
  timestamp = {2015.05.05}
}

@MISC{2007-BraunEveking.etal,
  author = {M. Braun and H. Eveking and V. Nimbler and M. Schickel},
  title = {Zuverl\"{a}ssigkeitserh\"{o}hung mit funktionalen Monitoren},
  year = {2007},
  file = {zud06-26.pdf:./2007-02-02-minh/zud06-26.pdf:PDF},
  owner = {nguyen},
  timestamp = {2007.02.02}
}

@INPROCEEDINGS{2007-BraunsteinEncrenaz,
  author = {Cecile Braunstein and Emmanuelle Encrenaz},
  title = {Using {CTL} formulae as component abstraction in a design and verification
	flow},
  booktitle = {International Conference on Application of Concurrency to System
	Design ({ACSD})},
  year = {2007},
  pages = {80-89},
  publisher = {IEEE Computer Society},
  file = {:./files/2007-BraunsteinEncrenaz.pdf:PDF},
  owner = {stoffel},
  timestamp = {2010.10.28}
}

@BOOK{1984-BraytonHachtel.etal,
  title = {Logic Minimization Algorithms for {VLSI} Synthesis},
  publisher = {Kluwer Academic Publishers},
  year = {1984},
  author = {R. K. Brayton and G. D. Hachtel and C. T. McMullen and A. L. Sangiovanni-Vincentelli}
}

@INPROCEEDINGS{1996-BraytonHachtel.etal,
  author = {R. K. Brayton and G. D. Hachtel and A. Sangiovanni-Vincentelli and
	F. Somenzi and A. Aziz and S.-T. Cheng and S. Edwards and S. Khatri
	and Y. Kukimoto and A. Pardo and S. Qadeer and R. K. Ranjan and S.
	Sarwary and T. R. Shiple and G. Swamy and T. Villa},
  title = {{VIS}: A system for Verification and Synthesis},
  booktitle = {Proc. International Conference on Computer-Aided Verification ({CAV})},
  year = {1996},
  editor = {R. Alur and T. Henzinger},
  volume = {1102},
  pages = {428-432},
  address = {New Brunswick, NJ},
  month = {July},
  file = {:./files/1996-BraytonHachtel.etal.pdf:PDF}
}

@ARTICLE{1987-BraytonRudell.etal,
  author = {R. K. Brayton and R. Rudell and A. L. Sangiovanni-Vincentelli and
	A. R. Wang},
  title = {{MIS}: Multi-Level Interactive Logic Optimization System},
  journal = {{IEEE} Transactions on Computer-Aided Design},
  year = {1987},
  volume = {6},
  pages = {1062-1081},
  number = {6},
  month = {November},
  file = {:./files/1987-BraytonRudell.etal.pdf:PDF},
  keywords = { Multiple-level logic; decomposition; don't cares; extraction; factorization;
	global phase assignment; kernels; logic minimization; resubstitution;
	simplification;}
}

@TECHREPORT{1999-BreitlingPhillips,
  author = {Max Breitling and Jan Phillips},
  title = {Black Box Views of State Machines},
  institution = {Technische Universtitaet Muenchen},
  year = {1999},
  file = {:./files/1999-BreitlingPhillips.pdf:PDF},
  timestamp = {2006.09.13}
}

@ARTICLE{2005-BrglezLi.etal,
  author = {Franc Brglez and Xiao Yu Li and Matthias F. Stallmann},
  title = {On {SAT} Instance Classes and a Methode for Reliable Performance
	Experiments with {SAT} Solvers},
  journal = {Annals of Mathematics and Artificial Intelligence},
  year = {2005},
  volume = {43},
  pages = {1--34},
  number = {1-4},
  month = jan,
  acmid = {1036204},
  address = {Hingham, MA, USA},
  file = {:./files/2005-BrglezLi.etal.pdf:PDF},
  issn = {1012-2443},
  issue_date = {January 2005},
  keywords = {conjunctive normal form, equivalence classes, experimental design,
	exponential and heavy-tail distributions, reliability function, satisfiability},
  numpages = {34},
  publisher = {Kluwer Academic Publishers},
  timestamp = {2006.09.21}
}

@PHDTHESIS{2010-Brickenstein,
  author = {Michael Brickenstein},
  title = {{Boolean} {Gr\"obner} Bases -- Theory, Algorithms and Applications},
  school = {Technische Universit{\"a}t Kaiserslautern, Germany},
  year = {2010},
  note = {to appear},
  optannote = {to appear},
  owner = {wedler},
  timestamp = {2010.02.15}
}

@INPROCEEDINGS{2008-BrickensteinDreyer,
  author = {Michael Brickenstein and Alexander Dreyer},
  title = {Gr\"obner} # -free # Normal # Forms # for # {Boolean} # Polynomials
}

@ARTICLE{2009-BrickensteinDreyer,
  author = {Michael Brickenstein and Alexander Dreyer},
  title = {{PolyBoRi}: A Framework for {Gr\"obner} Basis Computations with {Boolean}
	Polynomials},
  journal = {Journal of Symbolic Computation},
  year = {2009},
  volume = {44},
  pages = {1326--1345},
  number = {9},
  note = {{Effective Methods in Algebraic Geometry}},
  file = {:./files/2009-BrickensteinDreyer.pdf:PDF},
  issn = {0747-7171},
  keywords = {{Boolean} {Gr\"obner} basis},
  owner = {wedler},
  timestamp = {2010.02.15}
}

@ARTICLE{2009-BrickensteinDreyer.etal,
  author = {Michael Brickenstein and Alexander Dreyer and Gert-Martin Greuel
	and Markus Wedler and Oliver Wienand},
  title = {New developments in the theory of {Gr\"obner} bases and applications
	to formal verification},
  journal = {Journal of Pure and Applied Algebra},
  year = {2009},
  volume = {213},
  pages = {1612-1635},
  file = {:./files/2009-BrickensteinDreyer.etal.pdf:PDF},
  owner = {wedler},
  timestamp = {2008.01.21}
}

@INPROCEEDINGS{2015-BringmannEcker.etal,
  author = {Bringmann, Oliver and Ecker, Wolfgang and Gerstlauer, Andreas and
	Goyal, Ajay and Mueller-Gritschneder, Daniel and Sasidharan, Prasanth
	and Singh, Simranjit},
  title = {The Next Generation of Virtual Prototyping: Ultra-fast Yet Accurate
	Simulation of HW/SW Systems},
  booktitle = {Proceedings of the 2015 Design, Automation \& Test in Europe Conference
	\& Exhibition},
  year = {2015},
  series = {DATE '15},
  pages = {1698--1707},
  address = {San Jose, CA, USA},
  publisher = {EDA Consortium},
  acmid = {2757206},
  file = {2015-BringmannEcker.etal.pdf:files/2015-BringmannEcker.etal.pdf:PDF},
  isbn = {978-3-9815370-4-8},
  location = {Grenoble, France},
  numpages = {10},
  owner = {schwarz},
  timestamp = {2017.01.20}
}

@PHDTHESIS{2003-Brinkmann,
  author = {R. Brinkmann},
  title = {Preprocessing for Property Checking of Sequential Circuit on the
	Register Transfer Level},
  school = {Technische Universit\"at Kaiserslautern},
  year = {2003},
  type = {Dissertation},
  file = {:./files/2003-Brinkmann.pdf:PDF}
}

@UNPUBLISHED{2004-BrinkmannAchterberg,
  author = {Raik Brinkmann and T. Achterberg},
  title = {{Lose Kopplung von {CP}- und {MIP}-Beweisern}},
  note = {Internal Report IFX-1.2-3/4 of {BMBF} project {\scshape Valse-XT}},
  month = {July},
  year = {2004}
}

@INPROCEEDINGS{2002-BrinkmannDrechsler,
  author = {R. Brinkmann and R. Drechsler},
  title = {{RTL}-Datapath Verification using Integer Linear Programming},
  booktitle = {Design Automation Conference, 2002. Proceedings of {ASP}-{DAC} 2002.
	7th Asia and South Pacific and the 15th International Conference
	on {VLSI} Design. Proceedings.},
  year = {2002},
  pages = {741 -746},
  address = {Bangalore, India},
  file = {:./files/2002-BrinkmannDrechsler.pdf:PDF}
}

@INBOOK{2004-BrinkmannJohannsen.etal,
  chapter = {Application of Property Checking and Underlying Techniques},
  pages = {125-166},
  title = {Advanced Formal Verification},
  publisher = {Springer US},
  year = {2004},
  author = {R. Brinkmann and P. Johannsen and K. Winkelmann},
  address = {Boston, MA, USA},
  isbn = {978-1-4020-2530-3},
  keyword = {Computer Science},
  owner = {villarraga},
  timestamp = {2016.07.29}
}

@MISC{1998-BrookeKendrick.etal,
  author = {Antony Brooke and David Kendrick and Alexander Meeraus and Ramesh
	Raman and Richard E. Rosenthal},
  title = {{GAMS} - A User's Guide},
  month = {December},
  year = {1998},
  file = {:./files/1998-BrookeKendrick.etal.pdf:PDF},
  organization = {GAMS Developement Corporation},
  owner = {stoffel},
  timestamp = {2016.05.11},
  url = {http://www.gams.com}
}

@BOOK{1990-Brown,
  title = {{Boolean} Reasoning (The Logic of {Boolean} Equations)},
  publisher = {Kluwer Academic Publishers},
  year = {1990},
  author = {F. M. Brown}
}

@ARTICLE{1996-BrownRose,
  author = {Stephen Brown and Jonathan Rose},
  title = {{FPGA} and {CPLD} Architectures: A Tutorial},
  journal = {{IEEE} Design and Test of Computers},
  year = {1996},
  volume = {13},
  pages = {42--57},
  number = {2},
  file = {:./files/1996-BrownRose.pdf:PDF},
  timestamp = {2011.01.06}
}

@ARTICLE{1988-BrowneClarke.etal,
  author = {Browne, M. C. and Clarke, E. M. and Gr\"{u}mberg, O.},
  title = {Characterizing Finite Kripke Structures in Propositional Temporal
	Logic},
  journal = {Theor. Comput. Sci.},
  year = {1988},
  volume = {59},
  pages = {115--131},
  number = {1-2},
  month = jul,
  acmid = {55083},
  address = {Essex, UK},
  issn = {0304-3975},
  issue_date = {July 1988},
  numpages = {17},
  owner = {stoffel},
  publisher = {Elsevier Science Publishers Ltd.},
  timestamp = {2016.05.10}
}

@ARTICLE{1991-BruckertAlonso.etal,
  author = {William F. Bruckert and Carlos Alonso and James M. Melvin},
  title = {Verification of the First Fault-tolerant {VAX} System},
  journal = {Digital Technical Journal},
  year = {1991},
  volume = {3},
  pages = {0-},
  number = {1},
  file = {:./files/1991-BruckertAlonso.etal.pdf:PDF},
  timestamp = {2006.09.14}
}

@INPROCEEDINGS{2009-BrummayerBiere,
  author = {R. Brummayer and A. Biere},
  title = {Boolector: An Efficient {SMT} Solver for Bit-Vectors and Arrays},
  booktitle = {Proceedings of the 15th International Conference on Tools and Algorithms
	for the Construction and Analysis of Systems: Held as Part of the
	Joint European Conferences on Theory and Practice of Software, {ETAPS}
	2009,},
  year = {2009},
  series = {TACAS '09},
  pages = {174--177},
  address = {Berlin, Heidelberg},
  publisher = {Springer-Verlag},
  acmid = {1532912},
  file = {:./files/2009-BrummayerBiere.pdf:PDF},
  isbn = {978-3-642-00767-5},
  location = {York, UK},
  numpages = {4},
  owner = {thalmaier},
  timestamp = {2006.10.25}
}

@ARTICLE{2005-BruschiFerrandi.etal,
  author = {Francesco Bruschi and Fabrizio Ferrandi and Donatella Sciuto},
  title = {A Framework for the Functional Verification of {SystemC} Models},
  journal = {International Journal of Parallel Programming,},
  year = {2005},
  volume = {33},
  pages = {667-695},
  file = {:./files/2005-BruschiFerrandi.etal.pdf:PDF},
  timestamp = {2006.10.04}
}

@INPROCEEDINGS{2007-BruttomessoCimatti.etal,
  author = {Roberto Bruttomesso and Alessandro Cimatti and Anders Franz{\'e}n
	and Alberto Griggio and Ziyad Hanna and Alexander Nadel and Amit
	Palti and Roberto Sebastiani},
  title = {A Lazy and Layered {SMT}({BV}) Solver for Hard Industrial Verification
	Problems},
  booktitle = {Proceedings of the 19th international conference on Computer aided
	verification},
  year = {2007},
  series = {CAV'07},
  pages = {547--560},
  address = {Berlin, Heidelberg},
  publisher = {Springer-Verlag},
  acmid = {1770423},
  file = {:./files/2007-BruttomessoCimatti.etal.pdf:PDF},
  isbn = {978-3-540-73367-6},
  location = {Berlin, Germany},
  numpages = {14}
}

@INPROCEEDINGS{2007-BryantKroening.etal,
  author = {Al E. Bryant and Daniel Kroening and Jo�l Ouaknine and Sanjit A.
	Seshia and Ofer Strichman and Bryan Brady and Eth Z�rich},
  title = {Deciding bit-vector arithmetic with abstraction},
  booktitle = {Proceedings of the 13th international conference on Tools and algorithms
	for the construction and analysis of systems},
  year = {2007},
  series = {TACAS'07},
  pages = {358--372},
  address = {Berlin, Heidelberg},
  publisher = {Springer-Verlag},
  acmid = {1763544},
  file = {:./files/2007-BryantKroening.etal.pdf:PDF},
  isbn = {978-3-540-71208-4},
  location = {Braga, Portugal},
  numpages = {15},
  owner = {pavlenko},
  timestamp = {2010.07.26}
}

@ARTICLE{1986-Bryant,
  author = {Randal E. Bryant},
  title = {Graph-based Algorithms for {Boolean} Function Manipulation},
  journal = {{IEEE} Transactions on Computers},
  year = {1986},
  volume = {35},
  pages = {677-691},
  number = {8},
  month = {August},
  file = {:./files/1986-Bryant.pdf:PDF}
}

@INPROCEEDINGS{2000-BryantChauhan.etal,
  author = {Randal E. Bryant and P. Chauhan and Edmund M. Clarke and A. Coel},
  title = {A Theory of Consistency for Modular Synchronous Systems},
  booktitle = {Proceedings of the Third International Conference on Formal Methods
	in Computer-Aided Design},
  year = {2000},
  series = {FMCAD '00},
  pages = {486--504},
  address = {London, UK, UK},
  publisher = {Springer-Verlag},
  acmid = {758717},
  file = {:./files/2000-BryantChauhan.etal.pdf:PDF},
  isbn = {3-540-41219-0},
  numpages = {19},
  timestamp = {2006.09.19}
}

@INPROCEEDINGS{1995-BryantChen,
  author = {R. E. Bryant and Y.-A. Chen},
  title = {Verification of arithmetic circuits with binary moment diagrams},
  booktitle = {DAC '95: Proceedings of the 32nd ACM/IEEE conference on Design automation},
  year = {1995},
  pages = {535--541},
  address = {New York, NY, USA},
  publisher = {ACM},
  file = {:./files/1995-BryantChen.pdf:PDF},
  isbn = {0-89791-725-1},
  location = {San Francisco, California, United States}
}

@INPROCEEDINGS{1990-BryantSeger,
  author = {Randal E. Bryant and Carl-Johan H.Seger},
  title = {Formal Verification Of Digital Circuit Using Symbolic Ternary System
	Model},
  booktitle = {Proceedings of the 2nd International Workshop on Computer Aided Verification},
  year = {1990},
  series = {CAV '90},
  pages = {33--43},
  address = {London, UK, UK},
  publisher = {Springer-Verlag},
  acmid = {735043},
  file = {:./files/1990-BryantSeger.pdf:PDF},
  isbn = {3-540-54477-1},
  numpages = {11},
  timestamp = {2006.09.21}
}

@ARTICLE{2004-BrylowPalsbergy,
  author = {Dennis Brylow and Jens Palsbergy},
  title = {Deadline Analysis of Interrupt-Driven Software},
  journal = {IEEE Transactions on Software Engineering},
  year = {2004},
  volume = {30},
  pages = { 634 - 655},
  number = {10},
  month = {oct.},
  file = {:./files/2004-BrylowPalsbergy.pdf:PDF},
  keywords = { Z86-based microcontroller; Zilog architecture resource bounding infrastructure;
	deadline analysis; embedded systems; interrupt handling; interrupt-driven
	Z86-based software; multiresolution static analysis; software verification;
	testing oracles; worst-case execution time; embedded systems; formal
	verification; interrupts; microcontrollers; program compilers; program
	diagnostics; program testing;},
  timestamp = {2006.09.22}
}

@ARTICLE{1976-Buchberger,
  author = {Buchberger, B.},
  title = {Some properties of {Gr\"obner} bases for polynomial ideals},
  journal = {SIGSAM Bull.},
  year = {1976},
  volume = {10},
  pages = {19--24},
  number = {4},
  address = {New York, NY, USA},
  file = {:./files/1976-Buchberger.pdf:PDF},
  issn = {0163-5824},
  owner = {pavlenko},
  publisher = {ACM},
  timestamp = {2010.10.26}
}

@PHDTHESIS{1965-Buchberger,
  author = {B. Buchberger},
  title = {Ein Algorithmus zum Auffinden der Basiselemente des Restklassenringes
	nach einem nulldimensionalen Polynomideal},
  school = {University of Innsbruck, Austria},
  year = {1965},
  type = {Dissertation},
  file = {:./files/1965-Buchberger.pdf:PDF}
}

@ARTICLE{2000-BunkerGopalakrishnan.etal,
  author = {Annette Bunker and Ganesh Gopalakrishnan and Sally A.Mckey},
  title = {Formal Hardware Specification Languages for Protocol Compliance Verification},
  journal = {{ACM} Transactions on Design Automation of Electronic Systems},
  year = {2000},
  volume = {V},
  pages = {1-29},
  file = {:./files/2000-BunkerGopalakrishnan.etal.pdf:PDF},
  timestamp = {2006.09.19}
}

@INPROCEEDINGS{1991-BurchClarke.etal,
  author = {J. R. Burch and E. M. Clarke and D. E. Long},
  title = {Representing Circuits more Efficiently in Symbolic Model Checking},
  booktitle = {Proc. {ACM}/{IEEE} International Design Automation Conference ({DAC})},
  year = {1991},
  pages = {403--407},
  publisher = {ACM Press},
  file = {:./files/1991-BurchClarke.etal.pdf:PDF},
  isbn = {0-89791-395-7},
  location = {San Francisco, California, United States}
}

@ARTICLE{1994-BurchClarke.etal,
  author = {J. R. Burch and E. M. Clarke and D. E. Long and K. L. McMillan and
	D. L. Dill},
  title = {Symbolic Model Checking for Sequential Circuit Verification},
  journal = {{IEEE} Transactions on Computer-Aided Design},
  year = {1994},
  volume = {13},
  pages = {401-424},
  number = {4},
  month = {April},
  file = {:./files/1994-BurchClarke.etal.pdf:PDF}
}

@INPROCEEDINGS{1990-BurchClarke.etal,
  author = {J. R. Burch and E. M. Clarke and K. L. McMillan and D. L. Dill},
  title = {Sequential Circuit Verification using Symbolic Model Checking},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {1990},
  pages = {46-51},
  month = {June},
  file = {:./files/1990-BurchClarke.etal.pdf:PDF}
}

@INPROCEEDINGS{1994-BurchDill,
  author = {J. R. Burch and D. L. Dill},
  title = {Automatic Verification of Pipelined Microprocessors Control},
  booktitle = {Proc. Intl. Conference Computer Aided Verification ({CAV})},
  year = {1994},
  volume = {818},
  pages = {68--80},
  file = {:./files/1994-BurchDill.pdf:PDF},
  owner = {wedler},
  timestamp = {2006.08.29}
}

@INPROCEEDINGS{1998-BurchSinghal,
  author = {J. R. Burch and V. Singhal},
  title = {Robust Latch Mapping for Combinational Equivalence Checking},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {1998},
  pages = { 563 - 569},
  file = {:./files/1998-BurchSinghal.pdf:PDF}
}

@ARTICLE{2000-BushPincus.etal,
  author = {Bush, William R. and Pincus, Jonathan D. and Sielaff, David J.},
  title = {A Static Analyzer for Finding Dynamic Programming Errors},
  journal = {Softw. Pract. Exper.},
  year = {2000},
  volume = {30},
  pages = {775--802},
  number = {7},
  month = jun,
  acmid = {348428},
  address = {New York, NY, USA},
  issn = {0038-0644},
  issue_date = {June 2000},
  keywords = {program analysis, program error checking},
  numpages = {28},
  owner = {villarraga},
  publisher = {John Wiley \& Sons, Inc.},
  timestamp = {2016.08.01}
}

@INPROCEEDINGS{1995-HealyWhalley.etal,
  author = {C.A.Healy and D.B.Whalley and M.G.Harmon},
  title = {Integrating The Timing Analysis Of Pipelining and Instruction Caching},
  booktitle = {Proc. {IEEE} on Real-Time Systems Symposium},
  year = {1995},
  pages = {288 -297},
  file = {:./files/1995-HealyWhalley.etal.pdf:PDF},
  keywords = {code segments;data memory references;delays;execution time;graphical
	user interface;instruction caching;memory references;multicycle delays;pipeline
	path analysis;pipelining;real-time systems;timing analysis;timing
	analyzer;worst-case performance;buffer storage;delays;graphical user
	interfaces;pipeline processing;real-time systems;timing;},
  timestamp = {2006.09.21}
}

@INPROCEEDINGS{1999-FerdinandHechmann.etal,
  author = {C.Ferdinand and R.Hechmann and H.Theiling and S.Theiling and R.Welhelm
	and M.Schmidt},
  title = {Reliable and Precise WCETD Determination FOR Real Life Processor},
  booktitle = {Proceedings of the First International Workshop on Embedded Software},
  year = {2001},
  series = {EMSOFT '01},
  pages = {469--485},
  address = {London, UK, UK},
  publisher = {Springer-Verlag},
  acmid = {703893},
  file = {:./files/1999-FerdinandHechmann.etal.pdf:PDF},
  isbn = {3-540-42673-6},
  numpages = {17},
  timestamp = {2006.09.22}
}

@INPROCEEDINGS{2016a-CabodiCamurati.etal,
  author = {Cabodi, G and Camurati, P and Finocchiaro, SF and Loiacono, C and
	Savarese, F and Vendraminetto, D},
  title = {Secure embedded architectures: Taint properties verification},
  booktitle = {International Conference on Development and Application Systems (DAS)},
  year = {2016},
  pages = {150--157},
  organization = {IEEE},
  owner = {fadiheh},
  timestamp = {2018.07.12}
}

@INPROCEEDINGS{2016b-CabodiCamurati.etal,
  author = {G. Cabodi and P. Camurati and S. F. Finocchiaro and C. Loiacono and
	F. Savarese and D. Vendraminetto},
  title = {Secure Path Verification},
  booktitle = {2016 1st IEEE International Verification and Security Workshop (IVSW)},
  year = {2016},
  pages = {1-6},
  owner = {fadiheh},
  timestamp = {2018.07.12}
}

@ARTICLE{2017-CabodiCamurati.etal,
  author = {Cabodi, Gianpiero and Camurati, Paolo and Finocchiaro, Sebastiano
	F and Savarese, Francesco and Vendraminetto, Danilo},
  title = {Embedded Systems Secure Path Verification at the {HW/SW} Interface},
  journal = {IEEE Design \& Test},
  year = {2017},
  volume = {34},
  pages = {38--46},
  number = {5},
  owner = {fadiheh},
  publisher = {IEEE},
  timestamp = {2018.07.12}
}

@INPROCEEDINGS{1996a-CabodiCamurati.etal,
  author = {G. Cabodi and P. Camurati and L. Lavagno and E. Macii and M. Poncino
	and S. Quer and E. Sentovich},
  title = {Enhancing {FSM} Traversal by Temporary Re-Encoding},
  booktitle = {Proc. International Conference on Computer Design ({ICCD})},
  year = {1996},
  pages = {6 -11},
  file = {:./files/1996a-CabodiCamurati.etal.pdf:PDF},
  keywords = {FSM traversal enhancement;finite-state machines synthesis;optimization;symbolic-state
	manipulation techniques;temporary re-encoding;finite state machines;minimisation
	of switching nets;}
}

@INPROCEEDINGS{1997-CabodiCamurati.etal,
  author = {Gianpiero Cabodi and Paolo Camurati and Luciano Lavagno and Stefano
	Quer},
  title = {Disjunctive Partitioning and Partial Iterative Squaring: an Effective
	Approach for Symbolic Traversal of Large Circuits},
  booktitle = {Proc. Annual Conference on Design Automation},
  year = {1997},
  pages = {728--733},
  file = {:./files/1997-CabodiCamurati.etal.pdf:PDF},
  isbn = {0-89791-920-3},
  location = {Anaheim, California, United States}
}

@ARTICLE{2015-CabodiCamurati.etal,
  author = {Cabodi, G and Camurati, P and Loiacono, C and Pipitone, G and Savarese,
	F and Vendraminetto, D},
  title = {Formal verification of embedded systems for remote attestation},
  journal = {WSEAS Transactions on Computers},
  year = {2015},
  volume = {14},
  pages = {760--769},
  owner = {fadiheh},
  timestamp = {2018.07.12}
}

@INPROCEEDINGS{1996-CabodiCamurati.etal,
  author = {Gianpiero Cabodi and Paolo Camurati and Stefano Quer},
  title = {Improved Reachability Analysis of Large Finite State Machines},
  booktitle = {Proc. international conference on Computer-aided design ({ICCAD})},
  year = {1996},
  pages = {354 -360},
  file = {:./files/1996-CabodiCamurati.etal.pdf:PDF},
  keywords = {binary decision diagrams;divide-and-conquer;image computation;large
	finite state machines;logic design;optimized traversal technique;page
	faults;reachability analysis;secondary memory;state set decomposition;symbolic
	traversals;circuit diagrams;circuit optimisation;circuit testing;divide
	and conquer methods;finite state machines;logic CAD;logic testing;},
  timestamp = {2006.09.13}
}

@ARTICLE{2010-CabodiLavagno.etal,
  author = {Cabodi, Gianpiero and Lavagno, Luciano and Murciano, Marco and Kondratyev,
	Alex and Watanabe, Yosinori},
  title = {Speeding-up Heuristic Allocation, Scheduling and Binding with {SAT-based}
	Abstraction/Refinement Techniques},
  journal = {ACM Trans. Des. Autom. Electron. Syst.},
  year = {2010},
  volume = {15},
  pages = {12:1--12:34},
  number = {2},
  month = mar,
  acmid = {1698762},
  address = {New York, NY, USA},
  articleno = {12},
  issn = {1084-4309},
  issue_date = {February 2010},
  keywords = {High level synthesis, allocation, binding, resource estimation, satisfiability,
	scheduling},
  numpages = {34},
  owner = {villarraga},
  publisher = {ACM},
  timestamp = {2016.07.27}
}

@ARTICLE{2004-CabodiNocco.etal,
  author = {Gianpiero Cabodi and Sergio Nocco and Stefano Quer},
  title = {Improving {SAT}-based Bounded Model Checking by Means of {BDD}-based
	Approximate Traversals},
  journal = {Journal of Universal Computer Science},
  year = {2004},
  volume = {10},
  pages = {1693-1730},
  file = {:./files/2004-CabodiNocco.etal.pdf:PDF},
  owner = {nguyen},
  timestamp = {2007.02.02}
}

@INPROCEEDINGS{2008-CadarDunbar.etal,
  author = {Cadar, Cristian and Dunbar, Daniel and Engler, Dawson},
  title = {KLEE: Unassisted and Automatic Generation of High-coverage Tests
	for Complex Systems Programs},
  booktitle = {Proceedings of the 8th USENIX Conference on Operating Systems Design
	and Implementation},
  year = {2008},
  series = {OSDI'08},
  pages = {209--224},
  address = {Berkeley, CA, USA},
  publisher = {USENIX Association},
  acmid = {1855756},
  location = {San Diego, California},
  numpages = {16},
  owner = {villarraga},
  timestamp = {2016.08.01}
}

@INPROCEEDINGS{2006-CadarGanesh.etal,
  author = {C. {Cadar} and V. {Ganesh} and P. M. {Pawlowski} and D. L. {Dill} and D. R. {Engler}},
  title = {{EXE}: Automatically Generating Inputs of Death},
  booktitle = {Proceedings of the 13th ACM Conference on Computer and Communications
	Security},
  year = {2006},
  series = {CCS '06},
  pages = {322--335},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {1180445},
  isbn = {1-59593-518-5},
  keywords = {attack generation, bug finding, constraint solving, dynamic analysis,
	symbolic execution, test case generation},
  location = {Alexandria, Virginia, USA},
  numpages = {14},
  owner = {villarraga},
  timestamp = {2016.07.19}
}

@ARTICLE{2013-CadarSen,
  author = {Cadar, Cristian and Sen, Koushik},
  title = {Symbolic Execution for Software Testing: Three Decades Later},
  journal = {Commun. ACM},
  year = {2013},
  volume = {56},
  pages = {82--90},
  number = {2},
  month = feb,
  acmid = {2408795},
  address = {New York, NY, USA},
  file = {2013-CadarSen.pdf:files/2013-CadarSen.pdf:PDF},
  issn = {0001-0782},
  issue_date = {February 2013},
  numpages = {9},
  owner = {villarraga},
  publisher = {ACM},
  timestamp = {2014.04.24}
}

@INPROCEEDINGS{2003-CaiGajski,
  author = {L. {Cai} and D. {Gajski}},
  title = {Transaction level modeling: an overview},
  booktitle = {First IEEE/ACM/IFIP International Conference on Hardware/ Software
	Codesign and Systems Synthesis (IEEE Cat. No.03TH8721)},
  year = {2003},
  pages = {19-24},
  file = {2003-CaiGajski.pdf:files/2003-CaiGajski.pdf:PDF}
}

@PHDTHESIS{1996-Campos,
  author = {Campos, Sergio Vale Aguiar},
  title = {A quantitative approach to the formal verification of real-time systems},
  school = {Carnegie Mellon University},
  year = {1996},
  address = {Pittsburgh, PA, USA},
  note = {AAI9813817},
  file = {:./files/1996-Campos.pdf:PDF},
  isbn = {0-591-64746-X},
  publisher = {Carnegie Mellon University}
}

@ARTICLE{2018-CanellaVanbulck.etal,
  author = {Canella, Claudio and Van Bulck, Jo and Schwarz, Michael and Lipp,
	Moritz and von Berg, Benjamin and Ortner, Philipp and Piessens, Frank
	and Evtyushkin, Dmitry and Gruss, Daniel},
  title = {A systematic evaluation of transient execution attacks and defenses},
  journal = {arXiv preprint arXiv:1811.05441},
  year = {2018}
}

@INCOLLECTION{2018-CasselHowar.etal,
  author = {Cassel, Sofia and Howar, Falk and Jonsson, Bengt and Steffen, Bernhard},
  title = {Extending automata learning to extended finite state machines},
  booktitle = {Machine Learning for Dynamic Software Analysis: Potentials and Limits},
  publisher = {Springer},
  year = {2018},
  pages = {149--177}
}

@BOOK{2015-CastanoSchagaev,
  title = {Resilient Computer System Design},
  publisher = {Springer},
  year = {2015},
  author = {Victor Castano and Igor Schagaev},
  owner = {bartsch},
  timestamp = {2016.09.21}
}

@ARTICLE{1997-CauZedan,
  author = {Antonio Cau and Huusein Zedan},
  title = {Refining Interval Temporal Logic Specifications},
  journal = {Lecture Notes In Computer Science},
  year = {1997},
  volume = {1231},
  pages = {79 - 94},
  file = {:./files/1997-CauZedan.pdf:PDF},
  timestamp = {2006.09.13}
}

@INPROCEEDINGS{2002-CesarioBaghdadi.etal,
  author = {W. Cesario and A. Baghdadi and L. Gauthier and D. Lyonnard and M.
	Diaz-Nava and G. Nicolescu and Y. Paviot and S. Yoo and A.A. Jerraya},
  title = {Component-Based Design Approach for Multicore {SoCs1}},
  booktitle = {Proceedings of the 39th annual Design Automation Conference},
  year = {2002},
  series = {DAC '02},
  pages = {789--794},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {514115},
  isbn = {1-58113-461-4},
  keywords = {HW/SW interfaces abstraction, component-based design, multicore System-on-Chip},
  location = {New Orleans, Louisiana, USA},
  numpages = {6}
}

@INPROCEEDINGS{1993-ChaRudnick.etal,
  author = {Hungse Cha and Elithabeth M.Rudnick and Gwan S.Choi and Janak H.Patel
	and Ravishankar K.Iyer},
  title = {A Fast and Accurate gate -Level Transient Fault Simulation Environment},
  booktitle = {Fault-Tolerant Computing, 1993. {FTCS}-23. Digest of Papers., The
	Twenty-Third International Symposium on},
  year = {1993},
  pages = {310 -319},
  file = {:./files/1993-ChaRudnick.etal.pdf:PDF},
  keywords = {ISCAS-89 sequential benchmark circuits;fault models;gate-level transient
	fault simulation environment;high level models;latch operation;latch
	outputs;timing fault simulator;zero-delay parallel fault simulator;sequential
	circuits;},
  timestamp = {2006.09.14}
}

@ARTICLE{2005-ChaiKuehlmann,
  author = {Donald Chai and Andreas Kuehlmann},
  title = {A Fast Pseudo-{Boolean} Constraint Solver},
  journal = {{IEEE} Transactions on Computer-Aided Design},
  year = {2005},
  volume = {24},
  pages = {305-317},
  number = {3},
  month = {March},
  file = {:./files/2005-ChaiKuehlmann.pdf:PDF}
}

@INPROCEEDINGS{2003-ChaiKuehlmann,
  author = {Donald Chai and Andreas Kuehlmann},
  title = {A Fast Pseudo-{Boolean} Constraint Solver},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {2003},
  pages = {830-835},
  file = {:./files/2003-ChaiKuehlmann.pdf:PDF}
}

@ARTICLE{2004-ChakiClarke.etal,
  author = {Sagar Chaki and Edmund Clarke and Alex Groce and Somesh Jha and Helmut
	Veith},
  title = {Modular Verification of Software Components in {C}},
  journal = {{IEEE} Transactions on Software Engineering},
  year = {2004},
  volume = {30},
  pages = { 388 - 402},
  number = {6},
  month = {june},
  file = {:./files/2004-ChakiClarke.etal.pdf:PDF},
  keywords = { {Boolean} satisfiability; C program; Linux kernel; counterexample
	guided abstraction refinement; finite state machine specification;
	formal method; modular verification; predicate abstraction; software
	component; software design; software engineering; theorem proving;
	{Boolean} algebra; C language; computability; finite state machines;
	formal specification; program verification; theorem proving;},
  timestamp = {2006.09.22}
}

@INPROCEEDINGS{2005-ChakiIvers.etal,
  author = {Sagar Chaki and James Ivers and Natasha Sharygina and Kurt Wallnau},
  title = {The {ComFoRT} Reasoning Framework},
  booktitle = {Proceedings of the 17th international conference on Computer Aided
	Verification},
  year = {2005},
  series = {CAV'05},
  pages = {164--169},
  address = {Berlin, Heidelberg},
  publisher = {Springer-Verlag},
  acmid = {2153253},
  file = {:./files/2005-ChakiIvers.etal.pdf:PDF},
  isbn = {3-540-27231-3, 978-3-540-27231-1},
  location = {Edinburgh, Scotland, UK},
  numpages = {6},
  timestamp = {2006.09.22}
}

@PHDTHESIS{2005-Chaki,
  author = {Sagar J. Chaki},
  title = {A Counterexample Guided Abstraction},
  school = {School of Computer Science Carnegie Mellon University Pittsburgh},
  year = {2005},
  file = {:./files/2005-Chaki.pdf:PDF},
  timestamp = {2006.09.21}
}

@PHDTHESIS{1996-Chamillard,
  author = {A.T. Chamillard},
  title = {An Empirical Comparison Of Static Concurrency Analysis Techniques},
  school = {University of Massachusetts Amherst},
  year = {1996},
  file = {:./files/1996-Chamillard.pdf:PDF},
  timestamp = {2006.09.21}
}

@TECHREPORT{1996-ChamillardClarke.etal,
  author = {Chamillard, A. T. and Clarke, L. A. and Avrunin, G. S.},
  title = {Experimental Design for Comparing Static Concurrency Analysis},
  institution = {University of Massachusetts},
  year = {1996},
  address = {Amherst, MA, USA},
  file = {experimental design for comparing static concurrency analysis techniques.pdf:experimental design for comparing static concurrency analysis techniques.pdf:PDF},
  publisher = {University of Massachusetts}
}

@INPROCEEDINGS{2005-ChangBertacco.etal,
  author = {Kai-hui Chang and Valeria Bertacco and Igor L. Markov},
  title = {Simulation-based Bug Trace Minimization with {BMC}-based Refinement},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2005},
  pages = { 1045 - 1051},
  file = {:./files/2005-ChangBertacco.etal.pdf:PDF},
  keywords = { BMC-based refinement; Butramin; bug trace minimizer; equivalent trace;
	picoJava microprocessor; random simulator; semi-formal verification
	software; simulation-based bug trace minimization; circuit CAD; circuit
	simulation; equivalent circuits; formal verification; integrated
	circuit design;},
  timestamp = {2006.09.27}
}

@MISC{2009-ChapmanJones,
  author = {Ken Chapman and Les Jones},
  title = {{SEU Strategies for Virtex-5 Devices}},
  year = {2009},
  file = {2009-ChapmanJones.pdf:files/2009-ChapmanJones.pdf:PDF},
  owner = {villarraga},
  timestamp = {2016.06.07},
  url = {http://www.xilinx.com/}
}

@INPROCEEDINGS{1999-CharpentierChandy,
  author = {Michel Charpentier and K.Mani Chandy},
  title = {Towards Compositional Apprach to the Design and Verification of Distributed
	System},
  booktitle = {Proceedings of the Wold Congress on Formal Methods in the Development
	of Computing Systems-Volume I - Volume I},
  year = {1999},
  series = {FM '99},
  pages = {570--589},
  address = {London, UK, UK},
  publisher = {Springer-Verlag},
  acmid = {730466},
  file = {:./files/1999-CharpentierChandy.pdf:PDF},
  isbn = {3-540-66587-0},
  numpages = {20},
  timestamp = {2006.09.13}
}

@INPROCEEDINGS{2003-ChatterjeeMa.etal,
  author = {Krishnendu Chatterjee and Di Ma and Rupak Majumdar and Tian Zhao
	and Thomas A. Henzinger and Jens Palsberg},
  title = {Stack Size Analysis for Interrupt-Driven Programs},
  booktitle = {Proc. International Static Analysis Symposium ({SAS})},
  year = {2003},
  volume = {2694},
  series = {LNCS},
  pages = {109-126},
  file = {:./files/2003-ChatterjeeMa.etal.pdf:PDF},
  owner = {nguyen},
  timestamp = {2007.02.02}
}

@INPROCEEDINGS{2005-ChatterjeeMishchenko.etal,
  author = {S. Chatterjee and A. Mishchenko and R. Brayton and X. Wang and T.
	Kam},
  title = {Reducing Structural Bias in Technology Mapping},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2005},
  pages = { 519 - 526},
  file = {:./files/2005-ChatterjeeMishchenko.etal.pdf:PDF},
  keywords = { combinational equivalence; cut-based {Boolean} matching; cut-based
	mapping; library gates; lossless synthesis; structural bias reduction;
	technology mapping; {Boolean} functions; logic design; logic gates;
	logic simulation;},
  timestamp = {2006.09.27}
}

@INPROCEEDINGS{2006-ChattopadhyaySinha.etal,
  author = {Anupam Chattopadhyay and Arnab Sinha and Diandian Zhang and Rainer
	Leupers and Gerd Ascheid and Heinrich Meyr},
  title = {Integrated Verification Approach during {ADL}-Driven Processor Design},
  booktitle = {{RSP} '06: Proceedings of the Seventeenth {IEEE} International Workshop
	on Rapid System Prototyping},
  year = {2006},
  pages = {110--118},
  address = {Washington, DC, USA},
  publisher = {IEEE Computer Society},
  file = {:./files/2006-ChattopadhyaySinha.etal.pdf:PDF},
  isbn = {0-7695-2580-6}
}

@INPROCEEDINGS{2013-ChaudhariPark.etal,
  author = {A. Chaudhari and J. Park and J. Abraham},
  title = {A framework for low overhead hardware based runtime control flow
	error detection and recovery},
  booktitle = {31st VLSI Test Symposium (VTS)},
  year = {2013},
  pages = {1-6},
  month = {April},
  file = {2013-ChaudhariPark.etal.pdf:files/2013-ChaudhariPark.etal.pdf:PDF},
  issn = {1093-0167},
  owner = {bartsch},
  timestamp = {2016.09.21}
}

@INPROCEEDINGS{1994-ChaudhuriWalker,
  author = {S. Chaudhuri and R. A. Walker},
  title = {ILP-based scheduling with time and resource constraints in high level
	synthesis},
  booktitle = {Proceedings of 7th International Conference on VLSI Design},
  year = {1994},
  pages = {17-20},
  month = {Jan},
  file = {1994-ChaudhuriWalker.pdf:files/1994-ChaudhuriWalker.pdf:PDF},
  issn = {1063-9667},
  keywords = {VLSI;duality (mathematics);integer programming;logic CAD;resource
	allocation;scheduling;ILP-based scheduling;duality theory;formal
	analysis;high level synthesis;integer linear program;polyhedral theory;resource
	constraints;resource requirement;scheduling polytope;time constraints;Algorithm
	design and analysis;Constraint optimization;Flow graphs;High level
	synthesis;Mathematical analysis;Polynomials;Robustness;Scheduling
	algorithm;Silicon carbide;Time factors},
  owner = {schwarz},
  timestamp = {2017.01.09}
}

@INPROCEEDINGS{2003-ChaudhuriKlein,
  author = {Siddhartha Ray Chaudhuri and Russel Klein},
  title = {Hardware/Software Co-Verification of {CDMA} {ASIC} Designs},
  booktitle = {Proc. International {HDL} Conference},
  year = {2003},
  file = {:./files/2003-ChaudhuriKlein.pdf:PDF},
  timestamp = {2006.09.27}
}

@INPROCEEDINGS{2002-ChauhanClarke.etal,
  author = {P. Chauhan and E. Clarke and J. Kukula and S. Sapra and H. Veith
	and D. Wang},
  title = {Automated Abstraction Refinement for Model Checking Large State Spaces
	using {SAT} based Conflict Analysis},
  booktitle = {Proceedings of the 4th International Conference on Formal Methods
	in Computer-Aided Design},
  year = {2002},
  series = {FMCAD '02},
  pages = {33--51},
  address = {London, UK, UK},
  publisher = {Springer-Verlag},
  acmid = {683250},
  file = {:./files/2002-ChauhanClarke.etal.pdf:PDF},
  isbn = {3-540-00116-6},
  numpages = {19},
  timestamp = {2006.09.12}
}

@INPROCEEDINGS{1999-ChauhanClarke.etal,
  author = {Pankaj Chauhan and Edmund M. Clarke and Yuan Lu and Dong Wang},
  title = {Verifying {IP-Core} based {System-On-Chip} Designs},
  booktitle = {{ASIC}/{SOC} Conference, 1999. Proceedings. Twelfth Annual {IEEE}
	International},
  year = {1999},
  pages = {27 -31},
  file = {:./files/1999-ChauhanClarke.etal.pdf:PDF},
  keywords = {ASIC;IP-core based system-on-chip designs;PCI local bus;SMV;bus protocol;glue
	logic;protocol specification;standard bus interconnect;symbolic model
	checker;verification techniques;verified bus protocols;VLSI;application
	specific integrated circuits;circuit CAD;industrial property;integrated
	circuit design;logic CAD;protocols;symbol manipulation;},
  timestamp = {2007.04.12}
}

@INPROCEEDINGS{2009-ChauhanGoyal.etal,
  author = {P. Chauhan and D. Goyal and G. Hasteer and A. Mathur and N. Sharma},
  title = {Non-cycle-accurate sequential equivalence checking},
  booktitle = {Proc. Design Automation Conference ({DAC})},
  year = {2009},
  pages = {460--465},
  file = {:./files/2009-ChauhanGoyal.etal.pdf:PDF}
}

@INPROCEEDINGS{2005-ChenKandemir,
  author = {Guilin Chen and Mahmut Kandemir},
  title = {Runtime Integrity Checking for Inter-Object Connections},
  booktitle = {Proc. International Conference on Computer-Aided Design (ICCAD)},
  year = {2005},
  pages = { 303 - 306},
  file = {:./files/2005-ChenKandemir.pdf:PDF},
  keywords = { Java virtual machine; Java-based embedded systems; application programmer;
	connectivity rules; heap memory; inter-object connections; inter-object
	link; rule based approach; rule language; runtime integrity checking;
	Java; electronic engineering computing; embedded systems; knowledge
	based systems; virtual machines;},
  timestamp = {2006.09.27}
}

@INPROCEEDINGS{2014-ChenVenkataramani,
  author = {Chen, Jie and Venkataramani, Guru},
  title = {{CC-Hunter}: Uncovering Covert Timing Channels on Shared Processor
	Hardware},
  booktitle = {Annual IEEE/ACM Intl. Symp. on Microarchitecture},
  year = {2014},
  pages = {216-228},
  organization = {IEEE},
  owner = {fadiheh},
  timestamp = {2018.12.05}
}

@INPROCEEDINGS{2001-ChenChen,
  author = {Jiunn-Chern. Chen and Yirng-An Chen},
  title = {Equivalence Checking of Integer Multipliers},
  booktitle = {Proc. Asia and South Pacific Design Automation Conference ({ASPDAC})},
  year = {2001},
  pages = {169 -174},
  address = {Yokohama, Japan},
  file = {:./files/2001-ChenChen.pdf:PDF},
  keywords = {Wallace tree multiplier;array multiplier;backward substitution method;complexity
	bound;equivalence checking;integer multipliers;layered-backward substitution
	algorithm;multiplicative power hybrid decision diagrams;word-level
	representation;binary decision diagrams;circuit analysis computing;computational
	complexity;digital arithmetic;integrated logic circuits;multiplying
	circuits;}
}

@ARTICLE{2001-ChenDey,
  author = {Li Chen and S. Dey},
  title = {Software-based self-testing methodology for processor cores},
  journal = {IEEE Transactions on Computer-Aided Design of Integrated Circuits
	and Systems},
  year = {2001},
  volume = {20},
  pages = {369-380},
  number = {3},
  month = {March},
  file = {2001-ChenDey.pdf:files/2001-ChenDey.pdf:PDF},
  issn = {0278-0070},
  owner = {bartsch},
  timestamp = {2016.09.21}
}

@ARTICLE{2015-ChenEbrahimi.etal,
  author = {Chen, Liang and Ebrahimi, Mojtaba and Tahoori, Mehdi B.},
  title = {Formal Quantification of the Register Vulnerabilities to Soft Error
	in {RTL} Control Paths},
  journal = {Journal of Electronic Testing},
  year = {2015},
  volume = {31},
  pages = {193--206},
  abstract = {Radiation-induced soft error is a significant reliability issue in
	nanoscale technology nodes. As the sequential registers are major
	contributors to the system soft error rate, accurate analysis of
	their vulnerabilities at early design phases is essential for cost-efficient
	error mitigation. In this paper, a novel approach is proposed to
	quantify the soft error vulnerabilities of the registers in control
	paths at Register-Transfer Level (RTL). By modeling the control path
	as a state transition system, formal probabilistic model checking
	is adopted to compute the register vulnerabilities by taking the
	workload dependency into consideration. Efficient RTL abstraction
	and model simplification techniques are proposed to achieve an exponential
	reduction of the state space, enabling our methodology to analyze
	large control modules in a typical embedded processor. The experimental
	results show the effectiveness of the proposed techniques, which
	can successfully quantify the non-uniform register vulnerabilities
	in RTL designs.},
  day = {01},
  doi = {10.1007/s10836-015-5519-3},
  issn = {1573-0727},
  owner = {udupi},
  timestamp = {2018.07.23},
  url = {https://doi.org/10.1007/s10836-015-5519-3}
}

@ARTICLE{0000-ChenFarkash.etal,
  author = {Chen, Wen and Farkash, Monica and Huang, Jing and Bhadra, Jayanta},
  title = {Addressing Information Flow Properties for {HW} Security Verification},
  owner = {fadiheh},
  timestamp = {2018.07.14}
}

@BOOK{1996-ChenBushnell,
  title = {Efficient Branch and Bound Search with Application to Computer-Aided
	Design},
  publisher = {Kluwer Academic Publishers},
  year = {1996},
  author = {X. Chen and M. Bushnell},
  address = {Boston, MA}
}

@INPROCEEDINGS{1999-ChengHuang.etal,
  author = {K.-T. Cheng and S.-Y. Huang and W.-J. Dai},
  title = {Fault Emulation: A New Methodology for Fault Grading},
  booktitle = {IEEE Transaction on Computer-Aided Design of Integrated Circuits
	and Systems},
  year = {1999},
  pages = {1487 - 1495},
  month = {October},
  file = {:files/1999-ChengHuang.etal.pdf:PDF},
  owner = {bartsch},
  timestamp = {2014.07.30}
}

@INPROCEEDINGS{2017-CherupalliDuwe.etal,
  author = {H. Cherupalli and H. Duwe and W. Ye and R. Kumar and J. Sartori},
  title = {Enabling Effective Module-Oblivious Power Gating for Embedded Processors},
  booktitle = {2017 IEEE International Symposium on High Performance Computer Architecture
	(HPCA)},
  year = {2017},
  pages = {157-168},
  month = {Feb},
  file = {:/import/var/jabref/files/2017-CherupalliDuwe.etal.pdf:PDF},
  owner = {udupi},
  timestamp = {2018.04.16}
}

@ARTICLE{2016-ChiappettaSavas.etal,
  author = {Chiappetta, Marco and Savas, Erkay and Yilmaz, Cemal},
  title = {Real time detection of cache-based side-channel attacks using hardware
	performance counters},
  journal = {Applied Soft Computing},
  year = {2016},
  volume = {49},
  pages = {1162--1174},
  owner = {fadiheh},
  publisher = {Elsevier},
  timestamp = {2018.07.12}
}

@INPROCEEDINGS{1990-ChoHachtel.etal,
  author = {Hyunwoo Cho and Gary Hachtel and Seh-Woong Jeong and Bernard Plessier
	and Eric Schwarz and Fabio Somenzi},
  title = {{ATPG} Aspects of {FSM} Verification},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {1990},
  pages = {134 -137},
  file = {:./files/1990-ChoHachtel.etal.pdf:PDF},
  keywords = {PODEM feature;automatic test pattern generation;finite state machine
	verification;free-variable recognition feature;identical subtree
	recombination;image computation;iterative networks;primary input
	splitting;serial multipliers;tautological subspaces;unbalanced bipartitioning
	trees;finite automata;logic CAD;logic testing;sequential circuits;}
}

@ARTICLE{1996a-ChoHachtel.etal,
  author = {Hyunwoo Cho and G. D. Hachtel and E. Macii and B. Plessier and F.
	Somenzi:},
  title = {Algorithms for Approximate {FSM} Traversal Based on State Space Decomposition},
  journal = {{IEEE} Transactions on Computer-Aided Design},
  year = {1996},
  volume = {15},
  pages = {1465-1478},
  number = {12},
  month = {December},
  file = {:./files/1996a-ChoHachtel.etal.pdf:PDF}
}

@ARTICLE{1996-ChoHachtel.etal,
  author = {Hyunwoo Cho and G. D. Hachtel and E. Macii and M. Poncino and F.
	Somenzi},
  title = {Automatic State Space Decomposition for Approximate {FSM} Traversal
	Based on Circuit Analysis},
  journal = {{IEEE} Transactions on Computer-Aided Design},
  year = {1996},
  volume = {15},
  pages = {1451-1464},
  number = {12},
  month = {December},
  file = {:./files/1996-ChoHachtel.etal.pdf:PDF},
  keywords = {ISCAS'89 sequential benchmarks;affinity;approximate FSM traversal;automatic
	state space decomposition;circuit analysis;gate-level description;good
	partitions;graph partitioning problem;latch connectivity;latch correlation;latches;logic
	optimization;sequential circuit;structural analysis;circuit CAD;circuit
	optimisation;finite state machines;flip-flops;logic CAD;logic partitioning;sequential
	circuits;state-space methods;}
}

@INPROCEEDINGS{1994-ChoHachtel.etal,
  author = {H. Cho and G. D. Hachtel and E. Macii and Massimo Poncino and F.
	Somenzi},
  title = {A Structural Approach for State Space Decomposition for Approximate
	Reachability Analysis},
  booktitle = {Computer Design: {VLSI} in Computers and Processors, 1994. {ICCD}
	'94. Proceedings., IEEE International Conference on},
  year = {1994},
  pages = {236 -239},
  file = {:./files/1994-ChoHachtel.etal.pdf:PDF},
  keywords = { FSM traversal; approximate reachability analysis; benchmarks; circuit
	structure; directed graph; finite state machines; gate-level description;
	graph partitioning problem; latch connectivity; latch correlation;
	sequential circuit; state space decomposition; state space decomposition
	problem; structural approach; directed graphs; finite automata; finite
	state machines; flip-flops; graph theory; performance evaluation;
	sequential circuits;}
}

@INPROCEEDINGS{2013-ChoMirkhani.etal,
  author = {H. Cho and S. Mirkhani and C. Y. Cher and J. A. Abraham and S. Mitra},
  title = {Quantitative evaluation of soft error injection techniques for robust
	system design},
  booktitle = {2013 50th ACM/EDAC/IEEE Design Automation Conference (DAC)},
  year = {2013},
  issn = {0738-100X},
  owner = {udupi},
  timestamp = {2018.07.24}
}

@ARTICLE{2003-ChocklerKupferman.etal,
  author = {Hana Chockler and Orna Kupferman and Moshe Vardi},
  title = {Coverage metrics for formal verification},
  journal = {International Journal on Software Tools for Technology Transfer},
  year = {2006},
  volume = {8},
  pages = {373--386},
  number = {4},
  address = {Berlin, Heidelberg},
  file = {:./files/2003-ChocklerKupferman.etal.pdf:PDF},
  issn = {1433-2779},
  publisher = {Springer-Verlag}
}

@TECHREPORT{1999-ChoiYe,
  author = {C. C. Choi and Y. Ye},
  title = {Application of Semidefinite Programming to Circuit Partitioning},
  institution = {Department of Management Sciences, The University of Iowa},
  year = {1999},
  address = {Iowa City, Iowa 52242},
  file = {:./files/1999-ChoiYe.pdf:PDF},
  url = {citeseer.ist.psu.edu/choi99application.html}
}

@INPROCEEDINGS{2001-ChoiYun.etal,
  author = {Hoon Choi and Byeongwhee Yun and Yuntae Lee and Hyunglae Roh},
  title = {Model Checking of {S3C2400X} Industrial Embedded {SOC} Product},
  booktitle = {Proc. International Design automation Conference ({DAC})},
  year = {2001},
  pages = { 611 - 616},
  file = {:./files/2001-ChoiYun.etal.pdf:PDF},
  keywords = { RTL implementation; S3C2400X SOC product; environment modeling; gated
	clocks; industrial embedded SOC; model checking; multiple clock;
	synchronization logic; system on chip; unsynchronized clocks; verification;
	clocks; embedded systems; hardware description languages; integrated
	circuit design; logic CAD;},
  timestamp = {2006.09.27}
}

@INPROCEEDINGS{1992-ChouOrtega.etal,
  author = {Pai Chou and Ross Ortega and Gaetano Borriello},
  title = {Synthesis of the Hardware/Software Interface in Microcontroller-Based
	Systems},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {1992},
  pages = {488 -495},
  file = {:./files/1992-ChouOrtega.etal.pdf:PDF},
  keywords = {code size;data structures;device driver routines;hardware/software
	interface;microcontroller-based systems;port allocation algorithm;data
	structures;logic CAD;microcontrollers;},
  timestamp = {2006.10.04}
}

@ARTICLE{1996-ChowHo.etal,
  author = {Sue-Hong Chow and Yi-Cheng Ho and Tingting Hwang and C.L. Liu},
  title = {Low Power Realization of Finite State Machines -- A Decomposition
	Approach},
  journal = {Transaction an Design Atomation of Electronic Systems},
  year = {1996},
  volume = {1, No.3},
  pages = {315 - 340},
  file = {:./files/1996-ChowHo.etal.pdf:PDF},
  owner = {thalmaier},
  timestamp = {2006.08.28}
}

@INPROCEEDINGS{2012-ChristHoenicke.etal,
  author = {J{\"u}rgen Christ and Jochen Hoenicke and Alexander Nutz},
  title = {SMTInterpol: An Interpolating SMT Solver},
  booktitle = {SPIN},
  year = {2012},
  pages = {248-254},
  owner = {marx},
  timestamp = {2013.04.08}
}

@INPROCEEDINGS{2002-CiesielkiZeng.etal,
  author = {M. Ciesielski and Z. Zeng and P. Kalla and B. Rouzeyre},
  title = {Taylor Expansion Diagrams: A Compact, Canonical Representation with
	Applications to Symbolic Verification},
  booktitle = {Proc. International Conference on Design, Automation and Test in
	Europe ({DATE})},
  year = {2002},
  pages = {285-291},
  file = {:./files/2002-CiesielkiZeng.etal.pdf:PDF}
}

@INPROCEEDINGS{1999-CimattiClarke.etal,
  author = {A. Cimatti and E. M. Clarke and F. Giunchiglia and M. Roveri},
  title = {{NuSMV}: a New Symbolic Model Verifier},
  booktitle = {Proc. International Conference on Computer Aided Verification ({CAV})},
  year = {1999},
  editor = {{N. H}albwachs and {D. P}eled},
  number = {1633},
  series = {{L}ecture {N}otes in {C}omputer {S}cience},
  pages = {495-499},
  address = {{T}rento, {I}taly},
  month = {July},
  publisher = {{S}pringer},
  file = {:./files/1999-CimattiClarke.etal.pdf:PDF}
}

@INPROCEEDINGS{2011-CimattiGriggio.etal,
  author = {Cimatti, Alessandro and Griggio, Alberto and Micheli, Andrea and
	Narasamdya, Iman and Roveri, Marco},
  title = {{KRATOS}: a software model checker for {SystemC}},
  booktitle = {Intl. Conf. on Computer-Aided Verification (CAV)},
  year = {2011},
  series = {CAV'11},
  pages = {310--316},
  publisher = {Springer},
  file = {:files/2011-CimattiGriggio.etal.pdf:PDF},
  isbn = {978-3-642-22109-5},
  location = {Snowbird, UT},
  numpages = {7},
  owner = {joakim},
  timestamp = {2012.12.17}
}

@INPROCEEDINGS{2010-CimattiMicheli.etal,
  author = {Cimatti, Alessandro and Micheli, Andrea and Narasamdya, Iman and
	Roveri, Marco},
  title = {Verifying {SystemC}: a software model checking approach},
  booktitle = {Formal Methods in Computer-Aided Design (FMCAD)},
  year = {2010},
  pages = {51--60},
  address = {Austin, TX},
  file = {:files/2010-CimattiMicheli.etal.pdf:PDF},
  numpages = {10},
  owner = {joakim},
  timestamp = {2012.12.17}
}

@INPROCEEDINGS{2001a-CiveraMacchiarulo.etal,
  author = {P. Civera and L. Macchiarulo and M. Rebadengo and M. S. Reorda and
	M. Violante},
  title = {FPGA-based Fault Injection for Microprocessor Systems},
  booktitle = {Proc. 10th Asian Test Symposium},
  year = {2001},
  pages = {304 - 309},
  month = {November},
  file = {:files/2001-CiveraMacchiarulo.etal.pdf:PDF},
  owner = {bartsch},
  timestamp = {2014.07.30}
}

@INPROCEEDINGS{2001b-CiveraMacchiarulo.etal,
  author = {P. Civera and L. Macchiarulo and M. Rebaudengo and M. Sonza Reorda
	and M. Violante},
  title = {{FPGA}-based Fault Injection Techniques for Fast Evaluation of Fault
	Tolerance in {VLSI} Circuits},
  booktitle = {Proc. International Conference on Field-Programmable Logic and Applications},
  year = {2001},
  pages = {493--502},
  address = {London, UK, UK},
  publisher = {Springer-Verlag},
  acmid = {739881},
  file = {:./files/2001-CiveraMacchiarulo.etal.pdf:PDF},
  isbn = {3-540-42499-7},
  numpages = {10},
  timestamp = {2006.09.14}
}

@INPROCEEDINGS{2007-Claessen,
  author = {Koen Claessen},
  title = {A Coverage Analysis for Safety Property Lists},
  booktitle = {Proc. International Conference on Formal Methods in Computer-Aided
	Design ({FMCAD})},
  year = {2007},
  pages = {139-145},
  publisher = {IEEE Computer Society},
  file = {:./files/2007-Claessen.pdf:PDF},
  isbn = {0-7695-3023-0}
}

@ARTICLE{2000-ClaessenHughes,
  author = {Claessen, Koen and Hughes, John},
  title = {QuickCheck: A Lightweight Tool for Random Testing of Haskell Programs},
  journal = {SIGPLAN Not.},
  year = {2000},
  volume = {35},
  pages = {268--279},
  number = {9},
  month = sep,
  acmid = {351266},
  address = {New York, NY, USA},
  issn = {0362-1340},
  issue_date = {Sept. 2000},
  numpages = {12},
  owner = {villarraga},
  publisher = {ACM},
  timestamp = {2016.08.01}
}

@INBOOK{1985-Clark,
  chapter = {5},
  pages = {94-146},
  title = {Analysis of Reduced Memory {TMR} Systems},
  year = {1985},
  author = {Clark},
  file = {:./files/1985-Clark.pdf:PDF},
  timestamp = {2006.09.14}
}

@ARTICLE{1995-ClarkPradhan,
  author = {J. A. Clark and D. K. Pradhan},
  title = {Fault injection: a method for validating computer-system dependability},
  journal = {Computer},
  year = {1995},
  volume = {28},
  pages = {47-56},
  number = {6},
  month = {Jun},
  file = {1995-ClarkPradhan.pdf:files/1995-ClarkPradhan.pdf:PDF},
  issn = {0018-9162},
  owner = {bartsch},
  timestamp = {2016.11.28}
}

@ARTICLE{2001-ClarkeBiere.etal,
  author = {Clarke, Edmund and Biere, Armin and Raimi, Richard and Zhu, Yunshan},
  title = {Bounded Model Checking Using Satisfiability Solving},
  journal = {Form. Methods Syst. Des.},
  year = {2001},
  volume = {19},
  pages = {7--34},
  number = {1},
  month = jul,
  acmid = {510987},
  address = {Hingham, MA, USA},
  issn = {0925-9856},
  issue_date = {July 2001},
  keywords = {bounded model checking, cone of influence reduction, model checking,
	processor verification, satisfiability},
  numpages = {28},
  owner = {stoffel},
  publisher = {Kluwer Academic Publishers},
  timestamp = {2016.05.10}
}

@INPROCEEDINGS{2000-ClarkeGerman.etal,
  author = {E. Clarke and S. German and Y. Lu and H. Veit and D. Wang},
  title = {Executable Protocol Specification in {ESL}},
  booktitle = {Proceedings of the Third International Conference on Formal Methods
	in Computer-Aided Design},
  year = {2000},
  series = {FMCAD '00},
  pages = {197--216},
  address = {London, UK, UK},
  publisher = {Springer-Verlag},
  acmid = {683228},
  file = {:./files/2000-ClarkeGerman.etal.pdf:PDF},
  isbn = {3-540-41219-0},
  numpages = {20},
  timestamp = {2006.09.19}
}

@ARTICLE{2003-ClarkeGrumberg.etal,
  author = {Edmund Clarke and Orna Grumberg and Somesh Jha and Yuan Lu and Helmut
	Veith},
  title = {Counterexample-guided abstraction refinement for symbolic model checking},
  journal = {Journal of the {ACM}},
  year = {2003},
  volume = {50},
  pages = {752--794},
  number = {5},
  address = {New York, NY, USA},
  file = {:./files/2003-ClarkeGrumberg.etal.pdf:PDF},
  issn = {0004-5411},
  owner = {wedler},
  publisher = {ACM Press},
  timestamp = {2007.03.23}
}

@INPROCEEDINGS{2003a-ClarkeGrumberg.etal,
  author = {Edmund Clarke and Orna Grumberg and Muralidhar Talupur and Dong Wang},
  title = {High Level Verification of Control Intensive Systems Using Predicate
	Abstraction},
  booktitle = {Proc. {ACM} and {IEEE} International Conference on Formal Methods
	and Models for Co-Design ({MEMOCODE})},
  year = {2003},
  pages = {55 -64},
  file = {:./files/2003a-ClarkeGrumberg.etal.pdf:PDF},
  timestamp = {2006.09.12}
}

@INCOLLECTION{2008-ClarkeGupta.etal,
  author = {Clarke, Edmund and Gupta, Anubhav and Jain, Himanshu and Veith, Helmut},
  title = {Model Checking: Back and Forth between Hardware and Software},
  booktitle = {Verified Software: Theories, Tools, Experiments},
  publisher = {Springer-Verlag},
  year = {2008},
  editor = {Meyer, Bertrand and Woodcock, Jim},
  pages = {251--255},
  address = {Berlin, Heidelberg},
  acmid = {1417105},
  file = {:./files/2008-ClarkeGupta.etal.pdf:PDF},
  isbn = {978-3-540-69147-1},
  numpages = {5}
}

@MISC{2002a-ClarkeGupta.etal,
  author = {Edmund Clarke and Anubhav Gupta and James Kukula and Ofer Strichman},
  title = {{SAT}-based Abstraction-Refinement using {ILP} and Machine Learning
	Techniques},
  note = {slides},
  file = {:./files/2002a-ClarkeGupta.etal.pdf:PDF},
  owner = {stoffel},
  timestamp = {2006.09.12}
}

@INPROCEEDINGS{2002-ClarkeGupta.etal,
  author = {Edmund Clarke and Anubhav Gupta and James Kukula and Ofer Strichman},
  title = {{SAT}-based Abstraction-Refinement using {ILP} and Machine Learning
	Techniques},
  booktitle = {Proceedings of the 14th International Conference on Computer Aided
	Verification},
  year = {2002},
  series = {CAV '02},
  pages = {265--279},
  address = {London, UK, UK},
  publisher = {Springer-Verlag},
  acmid = {734428},
  file = {:./files/2002-ClarkeGupta.etal.pdf:PDF},
  isbn = {3-540-43997-8},
  numpages = {15},
  timestamp = {2006.09.12}
}

@TECHREPORT{2004-ClarkeJain.etal,
  author = {Edmund Clarke and Himanshu Jain and Daniel Kroening},
  title = {Predicate Abstraction and Refinement Techniques for Verifying Verilog},
  institution = {School of Computer Science, Carnegie Mellon University},
  year = {2004},
  address = {Pittsburgh, PA 15213},
  file = {:./files/2004-ClarkeJain.etal.pdf:PDF},
  owner = {wedler},
  timestamp = {2007.12.17}
}

@INPROCEEDINGS{2004-ClarkeKroening.etal,
  author = {Edmund Clarke and Daniel Kroening and Flavio Lerda},
  title = {A Tool For Checking ANSI C Programs},
  booktitle = {In Tools and Algorithms for the Construction and Analysis of Systems},
  year = {2004},
  pages = {168--176},
  publisher = {Springer},
  file = {:./files/2004-ClarkeKroening.etal.pdf:PDF},
  timestamp = {2006.09.22}
}

@INPROCEEDINGS{2003-ClarkeKroening.etal,
  author = {Clarke, Edmund and Kroening, Daniel and Yorav, Karen},
  title = {Behavioral consistency of {C} and {V}erilog programs using {B}ounded
	{M}odel {C}hecking},
  booktitle = {Proceedings of the 40th annual {D}esign {A}utomation {C}onference},
  year = {2003},
  series = {DAC '03},
  pages = {368--371},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {775928},
  date-added = {2012-02-26 22:40:17 +0100},
  date-modified = {2012-02-26 22:53:39 +0100},
  file = {2003-ClarkeKroening.etal.pdf:files/2003-ClarkeKroening.etal.pdf:PDF},
  isbn = {1-58113-688-9},
  keywords = {ANSI-C, equivalence checking, verilog},
  location = {Anaheim, CA, USA},
  numpages = {4},
  owner = {villarraga},
  timestamp = {2012.08.27}
}

@INPROCEEDINGS{1989-ClarkeLong.etal,
  author = {Clarke, E. and Long, D. and McMillan, K.},
  title = {Compositional Model Checking},
  booktitle = {Proceedings of the Fourth Annual Symposium on Logic in Computer Science
	(LICS)},
  year = {1989},
  pages = {353--362},
  address = {Piscataway, NJ, USA},
  publisher = {MIT Press},
  acmid = {77387},
  isbn = {0-8186-1954-6},
  location = {Pacific Grove, California, United States},
  numpages = {10},
  owner = {bao},
  timestamp = {2012.11.22}
}

@INPROCEEDINGS{2000-ClarkeLuz.etal,
  author = {Edmund Clarke and Yuan Luz and Helmut Veithy and Dong Wang},
  title = {{EPSL} Executable Protocol Specification Language},
  booktitle = {Proc. International Conference Formal Methods in Computer-Aided Design
	({FMCAD})},
  year = {2000},
  file = {:./files/2000-ClarkeLuz.etal.pdf:PDF},
  timestamp = {2006.09.19}
}

@MISC{2006-Clarke,
  author = {Edmund M. Clarke},
  title = {Grand Challenge Problem:Model Check Concurrent Software},
  note = {Presentation slides.},
  file = {:./files/2006-Clarke.ppt:PPT},
  owner = {nguyen},
  timestamp = {2007.02.02}
}

@ARTICLE{1981-ClarkeEmerson,
  author = {E. M. Clarke and E.A. Emerson},
  title = {Synthesis of Synchronization Skeletons for Branching Time Temporal
	Logic},
  journal = {Lecture Notes in Computer Science},
  year = {1981},
  volume = {131},
  editor = {Dexter Kozen},
  file = {:./files/1981-ClarkeEmerson.pdf:PDF},
  publisher = {Springer-Verlag}
}

@ARTICLE{1986-ClarkeEmerson.etal,
  author = {Clarke, E. M. and Emerson, E. A. and Sistla, A. P.},
  title = {Automatic Verification of Finite-state Concurrent Systems Using Temporal
	Logic Specifications},
  journal = {ACM Trans. Program. Lang. Syst.},
  year = {1986},
  volume = {8},
  pages = {244--263},
  number = {2},
  month = apr,
  address = {New York, NY, USA},
  issn = {0164-0925},
  issue_date = {April 1986},
  numpages = {20},
  owner = {joakim},
  publisher = {ACM},
  timestamp = {2014.05.22}
}

@INPROCEEDINGS{2001-ClarkeGrumberg.etal,
  author = {Clarke, Edmund M. and Grumberg, Orna and Jha, Somesh and Lu, Yuan
	and Veith, Helmut},
  title = {Progress on the State Explosion Problem in Model Checking},
  booktitle = {Informatics - 10 Years Back. 10 Years Ahead.},
  year = {2001},
  pages = {176--194},
  address = {London, UK, UK},
  publisher = {Springer-Verlag},
  acmid = {724453},
  file = {:./files/2001-ClarkeGrumberg.etal.pdf:PDF},
  isbn = {3-540-41635-8},
  numpages = {19}
}

@INPROCEEDINGS{2000-ClarkeGrumberg.etal,
  author = {Edmund M. Clarke and Orna Grumberg and Somesh Jha and Yuan Lu and
	Helmut Veith},
  title = {Counterexample-Guided Abstraction Refinement},
  booktitle = {Proc. International Conference on Computer Aided Verification ({CAV})},
  year = {2000},
  pages = {154-169},
  file = {:./files/2000-ClarkeGrumberg.etal.pdf:PDF}
}

@ARTICLE{1994-ClarkeGrumberg.etal,
  author = {Edmund M. Clarke and Orna Grumberg and David E. Long},
  title = {Model Checking and Abstraction},
  journal = {{ACM} Transactions on Programming Languages and Systems},
  year = {1994},
  volume = {16},
  pages = {1512--1542},
  number = {5},
  month = {September},
  file = {:./files/1994-ClarkeGrumberg.etal.pdf:PDF},
  publisher = {ACM Press},
  url = {citeseer.ist.psu.edu/clarke92model.html}
}

@INPROCEEDINGS{1999a-ClarkeGrumberg.etal,
  author = {E. M. Clarke and O. Grumberg and M. Minea and D. Peled},
  title = {State Space Reduction Using Partial Order Techniques},
  booktitle = {SOFTWARE TOOLS FOR TECHNOLOGY TRANSFER},
  year = {1999},
  pages = {279--287},
  publisher = {Springer-Verlag},
  file = {:./files/1999a-ClarkeGrumberg.etal.pdf:PDF}
}

@BOOK{1999-ClarkeGrumberg.etal,
  title = {Model Checking},
  publisher = {MIT Press},
  year = {1999},
  author = {E. M. Clarke and O. Grumberg and D. A. Peled},
  address = {London, England},
  file = {:./files/1999-ClarkeGrumberg.etal.pdf:PDF}
}

@INPROCEEDINGS{2014-ClarksonFinkbeiner.etal,
  author = {Clarkson, Michael R and Finkbeiner, Bernd and Koleini, Masoud and
	Micinski, Kristopher K and Rabe, Markus N and S{\'a}nchez, C{\'e}sar},
  title = {Temporal logics for hyperproperties},
  booktitle = {International Conference on Principles of Security and Trust},
  year = {2014},
  pages = {265--284},
  organization = {Springer},
  owner = {fadiheh},
  timestamp = {2018.11.28}
}

@ARTICLE{2010-ClarksonSchneider,
  author = {Clarkson, Michael R and Schneider, Fred B},
  title = {Hyperproperties},
  journal = {Journal of Computer Security},
  year = {2010},
  volume = {18},
  pages = {1157--1210},
  number = {6},
  owner = {fadiheh},
  publisher = {IOS Press},
  timestamp = {2018.11.28}
}

@INPROCEEDINGS{1994-CmelikKeppel,
  author = {Cmelik, Bob and Keppel, David},
  title = {Shade: A Fast Instruction-Set Simulator for Execution Profiling},
  booktitle = {Proceedings of the 1994 ACM SIGMETRICS conference on Measurement
	and modeling of computer systems},
  year = {1994},
  series = {SIGMETRICS '94},
  pages = {128--137},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {183032},
  file = {:./files/1994-CmelikKeppel.pdf:PDF},
  isbn = {0-89791-659-X},
  location = {Nashville, Tennessee, United States},
  numpages = {10}
}

@INPROCEEDINGS{2013-CohenPaul.etal,
  author = {Cohen, Ernie and Paul, Wolfgang and Schmaltz, Sabine},
  title = {Theory of Multi-Core Hypervisor Verification},
  booktitle = {SOFSEM 2013: Theory and Practice of Computer Science},
  year = {2013},
  editor = {Peter van Emde Boas and Frans C. A. Groen and Giuseppe F. Italiano
	and Jerzy Nawrocki and Harald Sack},
  volume = {7741},
  series = {Lecture Notes in Computer Science},
  pages = {1-27},
  publisher = {Springer},
  owner = {joakim},
  timestamp = {2016.03.18}
}

@MISC{2004-COIN,
  author = {{COIN-OR}},
  title = {Computational Infrastructure for Operations Research},
  owner = {stoffel},
  timestamp = {2016.05.10},
  url = {http://www.coin-or.org}
}

@INPROCEEDINGS{1990-Colmerauer,
  author = {Alain Colmerauer},
  title = {An introduction to Prolog {III}},
  booktitle = {Communications of the {ACM}},
  year = {1990},
  volume = {33},
  pages = {69-90},
  month = {July},
  comment = {Conference or Journal},
  file = {:./files/1990-Colmerauer.pdf:PDF}
}

@INPROCEEDINGS{2007-CondratKalla,
  author = {Condrat, Christopher and Kalla, Priyank},
  title = {A {Gr\"obner} basis approach to {CNF} formulae preprocessing},
  booktitle = {Proceedings of the 13th international conference on Tools and algorithms
	for the construction and analysis of systems},
  year = {2007},
  series = {TACAS'07},
  pages = {618--631},
  address = {Berlin, Heidelberg},
  publisher = {Springer-Verlag},
  location = {Braga, Portugal},
  numpages = {14}
}

@INPROCEEDINGS{2004-CongFan.etal,
  author = {Jason Cong and Yiping Fan and Guoling Han and Zhiru Zhang},
  title = {Application-Specific Instruction Generation for Configurable Processor
	Architectures},
  booktitle = {Proc. 2004 {ACM}/{SIGDA} 12th international symposium on Field programmable
	gate arrays},
  year = {2004},
  pages = {183-189},
  publisher = {ACM},
  file = {:./files/2004-CongFan.etal.pdf:PDF},
  isbn = {1-58113-829-6},
  owner = {loitz},
  review = {Good paper on Instruction Generation},
  timestamp = {2007.01.08},
  url = {http://dblp.uni-trier.de/db/conf/fpga/fpga2004.html#CongFHZ04}
}

@ARTICLE{2010-CongLiu.etal,
  author = {Jason Cong and Bin Liu and Rupak Majumdar and Zhiru Zhang},
  title = {Behavior-Level Observability Analysis for Operation Gating in Low-Power
	Behavioral Synthesis},
  journal = {{ACM} Transactions on Design Automation of Electronic Systems},
  year = {2010},
  volume = {16},
  pages = {1--29},
  number = {1},
  month = {nov},
  owner = {udupi},
  timestamp = {2015.08.03}
}

@INPROCEEDINGS{2002-Constantinescu,
  author = {Cristian Constantinescu},
  title = {Impact of Deep Submicron Technology on Dependability of {VLSI} Circuits},
  booktitle = {Proc. International Conference on Dependable Systems and Networks},
  year = {2002},
  pages = { 205 - 209},
  file = {:./files/2002-Constantinescu.pdf:PDF},
  keywords = { COTS; VLSI circuit dependability; VLSI circuit design; case studies;
	commercial-off-the-shelf systems; data integrity; deep submicron
	technology; interconnect dimensions; intermittent faults; manufacturing
	residuals; microprocessors; permanent faults; power voltages; semiconductor
	industry; semiconductor technology; timing violations; transient
	faults; transistor; VLSI; data integrity; fault tolerant computing;
	integrated circuit design; integrated circuit manufacture; integrated
	circuit reliability; microprocessor chips; timing;},
  timestamp = {2006.09.14}
}

@ARTICLE{2009-ConstantinidesMutlu.etal,
  author = {K. Constantinides and O. Mutlu and T. Austin and V. Bertacco},
  title = {A Flexible Software-Based Framework for Online Detection of Hardware
	Defects},
  journal = {IEEE Transactions on Computers},
  year = {2009},
  volume = {58},
  pages = {1063-1079},
  number = {8},
  month = {August},
  file = {2009-ConstantinidesMutlu.etal.pdf:files/2009-ConstantinidesMutlu.etal.pdf:PDF},
  issn = {0018-9340},
  owner = {bartsch},
  timestamp = {2016.09.21}
}

@INPROCEEDINGS{2005-CookKroening.etal,
  author = {Byron Cook and Daniel Kroening and Natasha Sharygina},
  title = {Symbolic Model Checking For Asynchronous {Boolean} Programs},
  booktitle = {Proceedings of the 12th international conference on Model Checking
	Software},
  year = {2005},
  series = {SPIN'05},
  pages = {75--90},
  address = {Berlin, Heidelberg},
  publisher = {Springer-Verlag},
  acmid = {2156355},
  file = {:./files/2005-CookKroening.etal.pdf:PDF},
  isbn = {3-540-28195-9, 978-3-540-28195-5},
  location = {San Francisco, CA},
  numpages = {16},
  timestamp = {2006.09.22}
}

@INPROCEEDINGS{1971-Cook,
  author = {Stephen A. Cook},
  title = {The Complexity of Theorem Proving Procedures},
  booktitle = {Proc. Annual {ACM} Symposium on the Theory of Computing},
  year = {1971},
  pages = {151-158},
  file = {:./files/1971-Cook.pdf:PDF}
}

@MISC{2002-CooperHarvey.etal,
  author = {Keith D. Cooper and Timothy J. Harvey and Todd Waterman},
  title = {Building a Control-flow Graph from Scheduled Assembly Code},
  year = {2002},
  file = {:./files/2002-CooperHarvey.etal.pdf:PDF},
  owner = {stoffel},
  text = {Keith D. Cooper, Timothy J. Harvey, and Todd Waterman. Building a
	Control-flow Graph from Scheduled Assembly Code. Technical Report
	TR02-399, Rice University, June 2002.},
  timestamp = {2016.05.10},
  url = {citeseer.ist.psu.edu/article/cooper02building.html}
}

@INPROCEEDINGS{2000-CorbettDwyer.etal,
  author = {Corbett, James C and Dwyer, Matthew B and Hatcliff, John and Laubach,
	Shawn and Pasareanu, Corina S and Zheng, Hongjun and others},
  title = {Bandera: Extracting finite-state models from Java source code},
  booktitle = {Software Engineering, 2000. Proceedings of the 2000 International
	Conference on},
  year = {2000},
  pages = {439--448},
  organization = {IEEE}
}

@INPROCEEDINGS{2009-CordeiroFischer.etal,
  author = {Lucas Cordeiro and Bernd Fischer and Huan Chen and Joao Marques-Silva},
  title = {Semiformal Verification of Embedded Software in Medical Devices Considering
	Stringent Hardware Constraints},
  booktitle = {Proc. International Conference on Embedded Software and Systems ({ICESS})},
  year = {2009},
  pages = {396 -403},
  file = {:./files/2009-CordeiroFischer.etal.pdf:PDF},
  owner = {stoffel},
  timestamp = {2010.10.29}
}

@BOOK{1994-CormenLeiserson.etal,
  title = {Introduction to Algorithms},
  publisher = {McGraw-Hill Book Company},
  year = {1994},
  author = {Thomas H. Cormen and Charles E. Leiserson and Ronald L. Rivest},
  file = {:./files/1994-CormenLeiserson.etal.pdf:PDF},
  owner = {nguyen},
  timestamp = {2008.05.06}
}

@INPROCEEDINGS{1998-CornoPatel.etal,
  author = {Fulvio Corno And Janak H. Patel And Elizabeth M. Rudnick And Matteo
	Sonza Reorda and Roberto Vietti and Politecnico Di Torino},
  title = {Enhancing Topological {ATPG} with High-Level Information and Symbolic
	Technique},
  booktitle = {Computer Design: {VLSI} in Computers and Processors, 1998. {ICCD}
	'98. Proceedings. International Conference on},
  year = {1998},
  pages = {504 -509},
  month = {oct},
  file = {:./files/1998-CornoPatel.etal.pdf:PDF},
  keywords = {ATPG algorithms;Fault Coverage;Fault Efficiency;state graphs;symbolic
	techniques;topological ATPG;automatic testing;logic testing;network
	topology;},
  timestamp = {2006.09.13}
}

@INPROCEEDINGS{1999a-CornoReorda.etal,
  author = {Fulvio Corno and Matteo Sonza Reorda and Giovanni Squillero},
  title = {Approximate Equivalence Verification for Protocol Interface Implementation
	via Genetic Algorithms},
  booktitle = {Proceedings of the First European Workshops on Evolutionary Image
	Analysis, Signal Processing and Telecommunications},
  year = {1999},
  pages = {182--192},
  address = {London, UK, UK},
  publisher = {Springer-Verlag},
  acmid = {651855},
  file = {:./files/1999a-CornoReorda.etal.pdf:PDF},
  isbn = {3-540-65837-8},
  numpages = {11},
  timestamp = {2006.09.13}
}

@INPROCEEDINGS{1999b-CornoReorda.etal,
  author = {F. Corno and M. Sonza Reorda and G. Squillero},
  title = {Approximate Equivalence Verification of Sequential Circuits via Genetic
	Algorithms},
  booktitle = {Proc. International Conference on Design, Automation and Test in
	Europe (DATE)},
  year = {1999},
  pages = {754 -755},
  file = {:./files/1999b-CornoReorda.etal.pdf:PDF},
  keywords = {CPU time;VEGA2;approximate equivalence verification;genetic algorithm-based
	approach;optimization process;prototypical tool;sequential circuits;verification
	tool;circuit analysis computing;formal verification;genetic algorithms;integrated
	logic circuits;logic CAD;sequential circuits;},
  timestamp = {2006.09.13}
}

@INPROCEEDINGS{1999-CornoReorda.etal,
  author = {Fulvio Corno and Matteo Sonza Reorda and Giovanni Squillero},
  title = {Simulation-Based Sequential Equivalence Checking of {RTL} {VHDL}},
  booktitle = {Proceedings of Electronics, Circuits and Systems},
  year = {1999},
  volume = {1},
  pages = {351-354},
  file = {:./files/1999-CornoReorda.etal.pdf:PDF},
  keywords = {RAVE;RT-level descriptions;RTL VHDL;commercial VHDL tools;equivalence
	verification;sequential equivalence checking;simulation-based equivalence
	checking;circuit simulation;formal verification;hardware description
	languages;high level synthesis;},
  timestamp = {2006.09.13}
}

@INPROCEEDINGS{1995-Correale,
  author = {Correale,Jr., Anthony},
  title = {Overview of the Power Minimization Techniques Employed in the IBM
	PowerPC 4Xx Embedded Controllers},
  booktitle = {Proceedings of the 1995 International Symposium on Low Power Design},
  year = {1995},
  series = {ISLPED '95},
  pages = {75--80},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {224095},
  file = {:files/1995-Correale.pdf:PDF},
  isbn = {0-89791-744-8},
  location = {Dana Point, California, USA},
  numpages = {6},
  owner = {udupi},
  timestamp = {2015.06.01}
}

@INPROCEEDINGS{0000-Corretjer,
  author = {Ivan Corretjer},
  title = {Peripheral Devices in Embedded Systems},
  file = {0000-Corretjer.pdf:files/0000-Corretjer.pdf:PDF},
  timestamp = {2006.10.04}
}

@MISC{2004-Corretjer,
  author = {Ivan M. Corretjer},
  title = {Peripheral Device Modeling for Embedded System Simulators},
  year = {2004},
  file = {:./files/2004-Corretjer.pdf:PDF},
  owner = {stoffel},
  timestamp = {2006.10.04}
}

@MASTERSTHESIS{2013-Cortes,
  author = {Carlos Francisco Calvillo Cortes},
  title = {High Level Synthesis of Control Flow Units: Synthesizable Model of
	a Pipelined Data Cache for the Cadence {C}-to-Silicon Compiler},
  school = {Technische Universit\"at Kaiserslautern},
  year = {2013},
  owner = {joakim},
  timestamp = {2015.07.29}
}

@MISC{2000a-CortesEles.etal,
  author = {Luis Alejandro Cortes and Petru Eles and Zebo Peng},
  title = {Verification Methodology for Heterogeneous HardwareSoftware Systems},
  year = {2000},
  file = {:./files/2000a-CortesEles.etal.pdf:PDF},
  owner = {stoffel},
  timestamp = {2006.09.27}
}

@INPROCEEDINGS{2000-CortesEles.etal,
  author = {L. A. Cortes and P. Eles and Z. Peng},
  title = {Formal Coverification of Embedded Systems using Model Checking},
  booktitle = {Proc. Euromicro Conference},
  year = {2000},
  volume = {1},
  pages = {106-113},
  file = {:./files/2000-CortesEles.etal.pdf:PDF},
  keywords = {CTL;PRES;Petri nets;computational model;correctness proving;coverification
	method;embedded system;embedded systems;formal coverification;formal
	reasoning;hardware/software systems;medical monitoring system;model
	checking;symbolic model checking;timing requirements;verification
	techniques;Petri nets;circuit analysis computing;embedded systems;formal
	verification;hardware-software codesign;},
  timestamp = {2006.09.27}
}

@ARTICLE{2013-CotroneoNatella,
  author = {D. Cotroneo and R. Natella},
  title = {Fault Injection for Software Certification},
  journal = {IEEE Security and Privacy},
  year = {2013},
  volume = {11},
  pages = {38-45},
  number = {4},
  month = {July},
  file = {2013-CotroneoNatella.pdf:files/2013-CotroneoNatella.pdf:PDF},
  issn = {1540-7993},
  owner = {bartsch},
  timestamp = {2016.11.28}
}

@INPROCEEDINGS{1989-CoudertBerthet.etal,
  author = {O. Coudert and C. Berthet and J.C. Madre},
  title = {Verification of Sequential Machines Using {Boolean} Functional Vectors},
  booktitle = {Proceedings of the {IFIP} International Workshop Applied Formal Methods
	for Correct {VLSI} Design},
  year = {1989},
  pages = {111-128},
  month = {June},
  standort = {not available},
  sw = {Symbolic automata traversal}
}

@ARTICLE{1989a-CoudertBerthet.etal,
  author = {Oliver Coudert and C. Berthet and Jean-Christophe Madre},
  title = {Verification of Synchronous Sequential Machines Based on Symbolic
	Execution},
  journal = {Lecture Notes on Computer Science},
  year = {1989},
  volume = {407},
  pages = {365-373},
  month = {June},
  editor = {J. Sifakis},
  file = {:./files/1989a-CoudertBerthet.etal.pdf:PDF},
  publisher = {Springer-Verlag}
}

@INPROCEEDINGS{1992-CoudertMadre,
  author = {O. Coudert and J. Madre},
  title = {Implicit and Incremental Computation of Primes and Essential Primes
	of {Boolean} Functions},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {1992},
  pages = {36-39},
  file = {:./files/1992-CoudertMadre.pdf:PDF}
}

@INPROCEEDINGS{1993-CoudertMadre.etal,
  author = {O. Coudert and J. Madre and H. Fraisse},
  title = {A New Viewpoint on Two-Level Logic Minimization},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {1993},
  pages = {625-630},
  file = {:./files/1993-CoudertMadre.etal.pdf:PDF}
}

@INPROCEEDINGS{1990-CoudertMadre,
  author = {Olivier Coudert and Jean Christophe Madre},
  title = {A Unified Framework for the Formal Verification of Sequential Circuits},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {1990},
  pages = {126 -129},
  file = {:./files/1990-CoudertMadre.pdf:PDF},
  keywords = {{Boolean} functions;characteristic functions;formal verification;sequential
	circuits;sets of transitions;simulation;typed decision graphs;unified
	framework;{Boolean} functions;circuit analysis computing;logic CAD;sequential
	circuits;},
  timestamp = {2006.09.13}
}

@MISC{2005-Cousot,
  author = {Patrick Cousot},
  title = {Tutorial in : Abstract Interpretation},
  year = {2005},
  file = {:./files/2005-Cousot.pdf:PDF},
  owner = {stoffel},
  timestamp = {2006.09.22}
}

@ARTICLE{1997-Cousot,
  author = {Patrick Cousot},
  title = {Program Analysis : The Abstract Interpretation Perspective},
  journal = {{ACM} {SIGPLAN} Notices},
  year = {1997},
  volume = {32},
  pages = {73 - 76},
  file = {:./files/1997-Cousot.pdf:PDF},
  timestamp = {2006.09.21}
}

@ARTICLE{1996-Cousot,
  author = {Patrick Cousot},
  title = {Abstract Interpretation},
  journal = {ACM computing surveys},
  year = {1996},
  volume = {28},
  pages = {324--328},
  number = {2},
  month = {jun},
  acmid = {234740},
  address = {New York, NY, USA},
  file = {:./files/1996-Cousot.pdf:PDF},
  issn = {0360-0300},
  numpages = {5},
  publisher = {ACM},
  timestamp = {2006.09.12}
}

@INPROCEEDINGS{2001-CousotCousot,
  author = {Cousot, Patrick and Cousot, Radhia},
  title = {Verification of Embedded Software: Problems and Perspectives},
  booktitle = {Proceedings of the First International Workshop on Embedded Software},
  year = {2001},
  series = {EMSOFT '01},
  pages = {97--113},
  address = {London, UK, UK},
  publisher = {Springer-Verlag},
  acmid = {706258},
  file = {:./files/2001-CousotCousot.pdf:PDF},
  isbn = {3-540-42673-6},
  numpages = {17}
}

@MISC{web_coverty,
  author = {{{Coverty, Inc.} {USA}}},
  title = {{Coverty Code Advisor}},
  howpublished = {http://www.coverity.com/},
  key = {Coverty},
  owner = {villarraga},
  timestamp = {2014.04.15},
  url = {http://www.coverity.com/products/code-advisor/}
}

@MISC{2003-Cowlishaw,
  author = {Mike Cowlishaw},
  title = {Decimal Arithmetic Encoding Strawman},
  year = {2003},
  file = {:./files/2003-Cowlishaw.pdf:PDF},
  owner = {stoffel},
  timestamp = {2006.10.04}
}

@INPROCEEDINGS{2003a-Cowlishaw,
  author = {Michael F. Cowlishaw},
  title = {Decimal Floating-Point: Algorism for Computers},
  booktitle = {Proc. {IEEE} Symposium on Computer Arithmetic ({ARITH})},
  year = {2003},
  pages = { 104 - 111},
  file = {:./files/2003a-Cowlishaw.pdf:PDF},
  keywords = { IEEE 854 standard; decimal floating point arithmetic; decimal hardware;
	decimal processing; human centric application; software decimal arithmetic;
	IEEE standards; floating point arithmetic; hardware-software codesign;
	mathematics computing; process algebra;},
  timestamp = {2006.10.04}
}

@BOOK{2007-CoxLittle.etal,
  title = {Ideals, Varieties, and Algorithms: An Introduction to Computational
	Algebraic Geometry and Commutative Algebra, 3/e (Undergraduate Texts
	in Mathematics)},
  publisher = {Springer-Verlag New York, Inc.},
  year = {2007},
  author = {Cox, David A. and Little, John and O'Shea, Donal},
  address = {Secaucus, NJ, USA},
  isbn = {0387356509},
  owner = {pavlenko},
  timestamp = {2010.10.21}
}

@INPROCEEDINGS{2005-CsallnerSmaragdakis,
  author = {Csallner, Christoph and Smaragdakis, Yannis},
  title = {{Check 'N' Crash}: Combining Static Checking and Testing},
  booktitle = {Proceedings of the 27th International Conference on Software Engineering},
  year = {2005},
  series = {ICSE '05},
  pages = {422--431},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {1062533},
  isbn = {1-58113-963-2},
  keywords = {automatic testing, dynamic analysis, extended static checking, static
	analysis, test case generation, usability},
  location = {St. Louis, MO, USA},
  numpages = {10},
  owner = {villarraga},
  timestamp = {2016.08.01}
}

@ARTICLE{2004-CsallnerSmaragdakis,
  author = {Csallner, Christoph and Smaragdakis, Yannis},
  title = {JCrasher: An Automatic Robustness Tester for Java},
  journal = {Softw. Pract. Exper.},
  year = {2004},
  volume = {34},
  pages = {1025--1050},
  number = {11},
  month = sep,
  acmid = {1044434},
  address = {New York, NY, USA},
  issn = {0038-0644},
  issue_date = {September 2004},
  keywords = {java, random testing, software testing, state re-initialization, test
	case generation},
  numpages = {26},
  owner = {villarraga},
  publisher = {John Wiley \& Sons, Inc.},
  timestamp = {2016.08.01}
}

@ARTICLE{2006-CurrieFeng.etal,
  author = {Currie, David and Feng, Xiushan and Fujita, Masahiro and Hu, Alan
	J. and Kwan, Mark and Rajan, Sreeranga},
  title = {Embedded software verification using symbolic execution and uninterpreted
	functions},
  journal = {Int. J. Parallel Program.},
  year = {2006},
  volume = {34},
  pages = {61--91},
  number = {1},
  month = {Feb},
  acmid = {1182765},
  address = {Norwell, MA, USA},
  file = {2006-CurrieFeng.etal.pdf:files/2006-CurrieFeng.etal.pdf:PDF},
  issn = {0885-7458},
  issue_date = {Febraury 2006},
  keywords = {DSP, VLIW, embedded software, formal verification},
  numpages = {31},
  owner = {villarraga},
  publisher = {Kluwer Academic Publishers},
  timestamp = {2012.12.03}
}

@INPROCEEDINGS{2000-CurrieHu.etal,
  author = {Currie, David W. and Hu, Alan J. and Rajan, Sreeranga},
  title = {Automatic formal verification of {DSP} software},
  booktitle = {Proceedings of the 37th {A}nnual {D}esign {A}utomation {C}onference},
  year = {2000},
  series = {DAC '00},
  pages = {130--135},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {337339},
  date-added = {2012-02-26 22:38:32 +0100},
  date-modified = {2012-02-26 22:56:31 +0100},
  file = {2000-CurrieHu.etal.pdf:files/2000-CurrieHu.etal.pdf:PDF},
  isbn = {1-58113-187-9},
  location = {Los Angeles, California, United States},
  numpages = {6},
  owner = {villarraga},
  timestamp = {2012.08.27}
}

@ARTICLE{1961-Curtis,
  author = {H. Allen Curtis},
  title = {A Generalized Tree Circuit},
  journal = {Journal of the Association of Computing Machinery},
  year = {1961},
  volume = {8},
  pages = {484--496},
  number = {4},
  month = oct,
  acmid = {321091},
  address = {New York, NY, USA},
  file = {:./files/1961-Curtis.pdf:PDF},
  issn = {0004-5411},
  numpages = {13},
  publisher = {ACM}
}

@MISC{2001-CyrBois.etal,
  author = {Genevieve Cyr and Guy Bois and Mustapha Aboulhamid},
  title = {Synthesis of Communication Interface for {SoC} using {VSIA} Recommendations},
  year = {2001},
  file = {:./files/2001-CyrBois.etal.pdf:PDF},
  owner = {stoffel},
  timestamp = {2006.09.19}
}

@ARTICLE{2008-SilvaKroening.etal,
  author = {D'Silva, Vijay and Kroening, Daniel and Weissenbacher, Georg},
  title = {A {S}urvey of automated techniques for formal software verification},
  journal = {IEEE Transactions on Computer-Aided Design of Integrated Circuits
	and Systems (TCAD)},
  year = {2008},
  volume = {27},
  pages = {1165--1178},
  number = {7},
  month = {July},
  date-added = {2012-02-26 22:34:27 +0100},
  date-modified = {2012-02-26 22:34:27 +0100},
  file = {2008-SilvaKroening.etal.pdf:files/2008-SilvaKroening.etal.pdf:PDF},
  owner = {villarraga},
  publisher = {IEEE},
  timestamp = {2012.08.27}
}

@ARTICLE{1986-DagenaisAgarwal.etal,
  author = {Dagenais, M.R. and Agarwal, V.K. and Rumin, N.C.},
  title = {{McBOOLE}: A New Procedure for Exact Logic Minimization},
  journal = {Computer-Aided Design of Integrated Circuits and Systems, IEEE Transactions
	on},
  year = {1986},
  volume = {5},
  pages = { 229 - 238},
  number = {1},
  month = {january},
  file = {:./files/1986-DagenaisAgarwal.etal.pdf:PDF},
  issn = {0278-0070}
}

@ARTICLE{2018-DaiBrayton,
  author = {Y. Y. Dai and R. K. Brayton},
  title = {Verification and Synthesis of Clock-Gated Circuits},
  journal = {IEEE Transactions on Computer-Aided Design of Integrated Circuits
	and Systems},
  year = {2018},
  file = {:/import/var/jabref/files/2018-DaiBrayton.pdf:PDF},
  owner = {udupi},
  timestamp = {2018.05.14}
}

@INPROCEEDINGS{1998-DammPnueli.etal,
  author = {Damm, Werner and Pnueli, Amir and Ruah, Sitvanit},
  title = {Herbrand Automata for Hardware Verification},
  booktitle = {Proc. of Intl. Conference on Concurrency Theory},
  year = {1998},
  pages = {67--83},
  acmid = {701323},
  isbn = {3-540-64896-8},
  numpages = {17},
  owner = {fadiheh},
  timestamp = {2019.09.03}
}

@ARTICLE{2005-DannaRothberg.etal,
  author = {Emilie Danna and Edward Rothberg and Claude Le Pape},
  title = {Exploring Relaxation Induced Neighborhoods to Improve {MIP} Solutions},
  journal = {Mathematical Programming},
  year = {2005},
  volume = {102},
  pages = {71--90},
  number = {1},
  month = {jan},
  acmid = {1041527},
  address = {Secaucus, NJ, USA},
  file = {:./files/2005-DannaRothberg.etal.pdf:PDF},
  issn = {0025-5610},
  keywords = {Heuristics, Hybrid algorithms, Local search, Mixed integer programming},
  numpages = {20},
  publisher = {Springer-Verlag New York, Inc.}
}

@INCOLLECTION{1951-Dantzig,
  author = {George B. Dantzig},
  title = {Maximization of a Linear Function of Variables Subject to Linear
	Inequalities},
  booktitle = {Activity Analysis of Production and Allocation},
  publisher = {John Wiley \& Sons},
  year = {1951},
  editor = {T.C. Koopmans},
  pages = {330-335},
  address = {New York}
}

@INPROCEEDINGS{2008-DarbariHashimi.etal,
  author = {A. Darbari and B. A. Hashimi and P. Harrod and D. Bradley},
  title = {A New Approach for Transient Fault Injection Using Symbolic Simulation},
  booktitle = {14th IEEE International On-Line Testing Symposium},
  year = {2008},
  pages = {93-98},
  month = {July},
  issn = {1942-9398},
  owner = {bartsch},
  timestamp = {2016.12.01}
}

@INPROCEEDINGS{2005-TathagatoChakrabarti,
  author = {Tathagato Rai Dastidar and Chakrabarti, P.P.},
  title = {A verification system for transient response of analog circuits using
	model checking},
  booktitle = {VLSI Design, 2005. 18th International Conference on},
  year = {2005},
  pages = { 195 - 200},
  month = {jan.},
  file = {:./files/2005-TathagatoChakrabarti.pdf:PDF},
  issn = {1063-9667}
}

@INPROCEEDINGS{2009-DaveauBlampey.etal,
  author = {J. M. Daveau and A. Blampey and G. Gasiot and J. Bulone and P. Roche},
  title = {An industrial fault injection platform for soft-error dependability
	analysis and hardening of complex system-on-a-chip},
  booktitle = {IEEE International Reliability Physics Symposium},
  year = {2009},
  pages = {212-220},
  month = {April},
  issn = {1541-7026},
  owner = {bartsch},
  timestamp = {2016.12.01}
}

@ARTICLE{1969-Davidson,
  author = {E. Davidson},
  title = {An Algorithm for {NAND} Decomposition under Network Constraints},
  journal = {IEEE Transactions on Computers},
  year = {1969},
  volume = {Vol. C-18},
  pages = {1098-1109},
  number = {12},
  month = {December},
  file = {:./files/1969-Davidson.pdf:PDF}
}

@ARTICLE{1962-DavisLogemann.etal,
  author = {Martin Davis and George Logemann and Donald Loveland},
  title = {A Machine Program for Theorem Proving},
  journal = {Communications of the {ACM}},
  year = {1962},
  volume = {5},
  pages = {394-397},
  file = {:./files/1962-DavisLogemann.etal.pdf:PDF}
}

@ARTICLE{1960-DavisPutnam,
  author = {Martin Davis and Hilary Putnam},
  title = {A Computing Procedure for Quantification Theory},
  journal = {Journal of the Association for Computing Machinery},
  year = {1960},
  volume = {7},
  pages = {201-215},
  file = {:./files/1960-DavisPutnam.pdf:PDF}
}

@MISC{2003-Deadman,
  author = {Bernard Deadman},
  title = {{PSL/Sugar}-Tutorial: Protocol Modeling},
  howpublished = {Design and Verification Conference ({DVCon})},
  year = {2003},
  booktitle = {PSL/Sugar Tutorial},
  file = {:./files/2003-Deadman.pdf:PDF},
  owner = {stoffel},
  timestamp = {2006.09.19}
}

@ARTICLE{2012-DeckerGreuel.etal,
  author = {Decker, W. and Greuel, G.-M. and Pfister, G. and Sch{\"o}nemann,
	H.},
  title = {{\sc Singular} {3-1-4} --- {A} computer algebra system for polynomial
	computations},
  year = {2012},
  note = {http://www.singular.uni-kl.de},
  owner = {marx},
  timestamp = {2012.11.13}
}

@BOOK{1820-Defoe,
  title = {The Life and Adventures of Robinson Crusoe},
  publisher = {Cadell, Davies, Strand and Blackwood},
  year = {1820},
  author = {Daniel Defoe},
  address = {Edinburgh}
}

@INPROCEEDINGS{1998-DeharbeShankar.etal,
  author = {Deharbe, D. and Shankar, S. and Clarke, E.M.},
  title = {Formal Verification of {VHDL} The Model Checker {CV}},
  booktitle = {Integrated Circuit Design, 1998. Proceedings. {XI} Brazilian Symposium
	on},
  year = {1998},
  pages = {95 -98},
  month = {sep-3 oct},
  file = {:./files/1998-DeharbeShankar.etal.pdf:PDF}
}

@MISC{2005-Dellacherie,
  author = {S. Dellacherie},
  title = {Automatic Protocol Compliance Check for {OCP}-Based Designs},
  year = {2005},
  note = {slides},
  file = {:./files/2005-Dellacherie.pdf:PDF},
  owner = {stoffel},
  timestamp = {2006.09.21}
}

@INPROCEEDINGS{2012-DemmeMartin.etal,
  author = {Demme, John and Martin, Robert and Waksman, Adam and Sethumadhavan,
	Simha},
  title = {Side-channel vulnerability factor: A metric for measuring information
	leakage},
  booktitle = {Annual International Symposium on Computer Architecture (ISCA)},
  year = {2012},
  pages = {106--117},
  organization = {IEEE},
  owner = {fadiheh},
  timestamp = {2018.11.28}
}

@INPROCEEDINGS{2014-DemmeSethumadhavan,
  author = {Demme, John and Sethumadhavan, Simha},
  title = {Side-channel vulnerability metrics: {SVF} vs. {CSV}},
  booktitle = {Proc. of 11th Annual Workshop on Duplicating, Deconstructing and
	Debunking (WDDD)},
  year = {2014},
  owner = {fadiheh},
  timestamp = {2018.11.28}
}

@INPROCEEDINGS{1990-DeNicolaVaandrager,
  author = {De Nicola, Rocco and Vaandrager, Frits},
  title = {Action Versus State Based Logics for Transition Systems},
  booktitle = {Proceedings of the LITP Spring School on Theoretical Computer Science
	on Semantics of Systems of Concurrent Processes},
  year = {1990},
  pages = {407--419},
  address = {New York, NY, USA},
  publisher = {Springer-Verlag New York, Inc.},
  isbn = {0-387-53479-2},
  location = {La Roche Posay, France},
  numpages = {13},
  owner = {stoffel},
  timestamp = {2016.05.10}
}

@MISC{web-Dershowitz,
  author = {Nachum Dershowitz},
  title = {Software Horror Stories},
  owner = {bschmidt},
  timestamp = {2014.06.27},
  url = {http://www.cs.tau.ac.il/~nachumd/horror.html}
}

@INPROCEEDINGS{1989-Devadas,
  author = {Srinivas Devadas},
  title = {General Decomposition of Sequential Machines: Relationship to State
	Assignment},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {1989},
  pages = { 314 - 320},
  file = {:./files/1989-Devadas.pdf:PDF},
  owner = {thalmaier},
  timestamp = {2006.08.28}
}

@ARTICLE{2000-DevillersGriffioen.etal,
  author = {Devillers, Marco and Griffioen, David and Romijn, Judi and Vaandrager,
	Frits},
  title = {Verification of a Leader Election Protocol: Formal Methods Applied
	to {IEEE} 1394},
  journal = {Form. Methods Syst. Des.},
  year = {2000},
  volume = {16},
  pages = {307--320},
  number = {3},
  month = {jun},
  acmid = {349278},
  address = {Hingham, MA, USA},
  file = {:./files/2000-DevillersGriffioen.etal.pdf:PDF},
  issn = {0925-9856},
  issue_date = {June 2000},
  keywords = {I/O automata, IEEE 1394, PVS, concurrency theory, formal methods,
	leader election algorithm, protocols, theorem provers, tree identify
	phase},
  numpages = {14},
  publisher = {Kluwer Academic Publishers}
}

@INPROCEEDINGS{2000-DiazCodognet,
  author = {D. Diaz and P. Codognet},
  title = {The {GNU} Prolog System and its Implementation},
  booktitle = {Proc. {ACM} symposium on Applied computing},
  year = {2000},
  pages = {728-732},
  file = {:./files/2000-DiazCodognet.pdf:PDF},
  url = {citeseer.ist.psu.edu/diaz00gnu.html}
}

@INPROCEEDINGS{2012-DiepenbeckSoeken.etal,
  author = {M. Diepenbeck and M. Soeken and D. Gro{\ss}e and R. Drechsler},
  title = {Behavior-Driven Development for Circuit Design and Verification},
  booktitle = {IEEE Intl. High-Level Design Validation and Test Workshop (HLDVT)},
  year = {2012},
  file = {:files/2012-DiepenbeckSoeken.etal.pdf:PDF}
}

@BOOK{2000-Diestel,
  title = {Graph Theory},
  publisher = {Springer-Verlag Berlin Heidelberg},
  year = {2000},
  author = {Reinhard Diestel},
  file = {2000-Diestel.pdf:files/2000-Diestel.pdf:PDF},
  owner = {schwarz},
  timestamp = {2017.01.17}
}

@INPROCEEDINGS{1996-Dill,
  author = {Dill, David L.},
  title = {The {M}urphi {V}erification {S}ystem},
  booktitle = {Proceedings of the 8th {I}nternational {C}onference on {C}omputer
	{A}ided {V}erification},
  year = {1996},
  series = {CAV '96},
  pages = {390--393},
  address = {London, UK},
  publisher = {Springer-Verlag},
  acmid = {735832},
  isbn = {3-540-61474-5},
  numpages = {4},
  owner = {villarraga},
  timestamp = {2012.08.27}
}

@INPROCEEDINGS{1992-DillDrexler.etal,
  author = {D. L. Dill and A. J. Drexler and A. J. Hu and C. Han Yang},
  title = {Protocol Verification as a Hardware Design Aid},
  booktitle = {Proc. {IEEE} International Conference on Computer Design ({ICCD})},
  year = {1992},
  pages = {522 -525},
  month = {oct},
  file = {:./files/1992-DillDrexler.etal.pdf:PDF},
  keywords = { Mur phi ; automatic formal protocol verification; computation; hardware
	design aid; protocol description language; formal verification; protocols;}
}

@INPROCEEDINGS{1999-Dimitrov,
  author = {Jordan Dimitrov},
  title = {Compositional Reasoning about Events in Interval Temporal Logic},
  booktitle = {Proc. International Conference On Computer Aided Verifcation({CAV})},
  year = {1999},
  file = {:./files/1999-Dimitrov.pdf:PDF},
  timestamp = {2006.09.13}
}

@INPROCEEDINGS{1988-DincbasHentenryck.etal,
  author = {Mehmet Dincbas and Pascal {van Hentenryck} and Helmut Simonis and
	Abderrahmane Aggoun and Thomas Graf and Fran\c{c}oise Berthier},
  title = {The Constraint Logic Programming Language {CHiP}},
  booktitle = {Proc. International Conference on Fifth Generation Computer Systems},
  year = {1988},
  pages = {693-702},
  address = {Tokyo}
}

@INPROCEEDINGS{2017-DiPompeoIncerto.etal,
  author = {Di Pompeo, Daniele and Incerto, Emilio and Muttillo, Vittoriano and
	Pomante, Luigi and Valenete, Giacomo},
  title = {An Efficient Performance-Driven Approach for HW/SW Co-Design},
  booktitle = {Proceedings of the 8th ACM/SPEC on International Conference on Performance
	Engineering},
  year = {2017},
  pages = {323--326},
  owner = {fehmel},
  timestamp = {2019.05.27}
}

@INPROCEEDINGS{2010-DomnitserAbughazel.etal,
  author = {Domnitser, Leonid and Abu-Ghazaleh, Nael and Ponomarev, Dmitry},
  title = {A predictive model for cache-based side channels in multicore and
	multithreaded microprocessors},
  booktitle = {International Conference on Mathematical Methods, Models, and Architectures
	for Computer Network Security},
  year = {2010},
  pages = {70--85},
  organization = {Springer},
  owner = {fadiheh},
  timestamp = {2018.11.22}
}

@INPROCEEDINGS{2002-DoniniLiberatore.etal,
  author = {F. M. Donini and P. Liberatore and F. Massacci and M.Schaerf},
  title = {Solving {QBF} with {SMV}},
  booktitle = {Proc. International Conference on Principles of Knowledge Representation
	and Reasoning (KR 2002)},
  year = {2002},
  pages = {578-589},
  file = {:./files/2002-DoniniLiberatore.etal.pdf:PDF}
}

@ARTICLE{2015-DoychevKoepf.etal,
  author = {Doychev, Goran and K{\"o}pf, Boris and Mauborgne, Laurent and Reineke,
	Jan},
  title = {Cacheaudit: A tool for the static analysis of cache side channels},
  journal = {ACM Transactions on Information and System Security (TISSEC)},
  year = {2015},
  volume = {18},
  pages = {4},
  number = {1},
  owner = {jmueller},
  publisher = {ACM},
  timestamp = {2019.08.16}
}

@ARTICLE{1998a-DrechslerBecker,
  author = {Drechsler, R. and Becker, B.},
  title = {Ordered Kronecker functional decision diagrams-a data structure for
	representation and manipulation of {Boolean} functions},
  journal = {Computer-Aided Design of Integrated Circuits and Systems, IEEE Transactions
	on},
  year = {1998},
  volume = {17},
  pages = {965 -973},
  number = {10},
  month = {oct},
  file = {:./files/1998a-DrechslerBecker.pdf:PDF},
  issn = {0278-0070},
  keywords = {{Boolean} functions;OKFDDs;PUMA;data structure;decomposition-type
	choice;dynamic variable ordering;elementary manipulation algorithms;interleaving;manipulation;ordered
	Kronecker functional decision diagrams;reordering-based method;representation;sifting;Boolean
	functions;binary decision diagrams;data structures;logic CAD;minimisation
	of switching nets;multivalued logic circuits;}
}

@BOOK{1998-DrechslerBecker,
  title = {Graphenbasierte Funktionsdarstellung - Boolesche und Pseudo-Boolesche
	Funktionen},
  publisher = {Teubner},
  year = {1998},
  author = {Rolf Drechsler and Bernd Becker},
  pages = {1-200},
  series = {Leitf{\"a}den der Informatik},
  bibsource = {DBLP, http://dblp.uni-trier.de},
  isbn = {978-3-519-02149-0}
}

@ARTICLE{1998-DrechslerBecker.etal,
  author = {Drechsler, R. and Becker, B. and Jahnke, A.},
  title = {On Variable Ordering and Decomposition Type Choice in {OKFDD}s},
  journal = {Computers, {IEEE} Transactions on},
  year = {1998},
  volume = {47},
  pages = {1398 -1403},
  number = {12},
  month = {dec},
  file = {:./files/1998-DrechslerBecker.etal.pdf:PDF},
  issn = {0018-9340},
  keywords = {OKFDDs;binary decision diagrams;decomposition type choice;ecision
	diagrams;multilevel circuits;ordered Kronecker Functional Decision
	Diagrams;tree-like circuit;upper bound;variable ordering;Boolean
	functions;binary decision diagrams;circuit complexity;}
}

@ARTICLE{1997-DrechslerBecker.etal,
  author = {Rolf Drechsler and Bernd Becker and Stefan Ruppertz},
  title = {The {K*BMD}: A Verification Data Structure},
  journal = {IEEE Design and Test of Computers},
  year = {1997},
  volume = {14},
  pages = {51-59},
  number = {2},
  address = {Los Alamitos,CA,USA},
  file = {:./files/1997-DrechslerBecker.etal.pdf:PDF},
  owner = {wedler},
  publisher = {IEEE Computer Society},
  timestamp = {2008.02.18}
}

@INPROCEEDINGS{1996-DrechslerBecker.etal,
  author = {R. Drechsler and B. Becker and S. Ruppertz},
  title = {{K*BMDs}: A New Data Structure for Verification},
  booktitle = {Proc. European Design and Test Conference ({EDTC})},
  year = {1996},
  pages = {2-8},
  file = {:./files/1996-DrechslerBecker.etal.pdf:PDF}
}

@INPROCEEDINGS{1994-DrechslerBecker.etal,
  author = {Rolf Drechsler and Bernd Becker and A. Sarabi and M. Theobald and
	M. Perkowski},
  title = {Efficient Representation and Manipulation of Switching Functions
	Based on Ordered {Kronecker} Functional Decision Diagrams},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {1994},
  pages = {415-419},
  file = {:./files/1994-DrechslerBecker.etal.pdf:PDF}
}

@INPROCEEDINGS{2012-DrechslerDiepenbeck.etal,
  author = {Drechsler, Rolf and Diepenbeck, Melanie and Gro{\ss}e, Daniel and
	K{\"u}hne, Ulrich and Le, Hoang M. and Seiter, Julia and Soeken,
	Mathias and Wille, Robert},
  title = {Completeness-Driven Development},
  booktitle = {Graph Transformations},
  year = {2012},
  pages = {38--50},
  publisher = {Springer},
  file = {:files/2012-DrechslerDiepenbeck.etal.pdf:PDF}
}

@CONFERENCE{2011-DreyerMarx.etal,
  author = {Alexander Dreyer and Oliver Marx and Evgeny Pavlenko and Markus Wedler
	and Dominik Stoffel and Wolfgang Kunz and Gert-Martin Greuel},
  title = {Preprocessing polynomials for arithmetic reasoning within the {SMT-Solver
	STABLE}},
  booktitle = {Seventh International Workshop on Constraints in Formal Verification
	(CFV'11)},
  year = {2011},
  address = {San Jose, USA},
  file = {:./files/2011-DreyerMarx.etal.pdf:PDF},
  owner = {pavlenko},
  timestamp = {2011.11.16}
}

@INPROCEEDINGS{2006-DutertreMoura,
  author = {Bruno Dutertre and Leonardo de Moura},
  title = {A Fast Linear-Arithmetic Solver for {DPLL(T)}},
  booktitle = {Proc. International Conference Computer Aided Verification ({CAV})},
  year = {2006},
  volume = {4144},
  series = {LNCS},
  pages = {81--94},
  publisher = {Springer-Verlag},
  editors = {T. Ball and R. B. Jones},
  file = {:./files/2006-DutertreMoura.pdf:PDF},
  owner = {wedler},
  timestamp = {2008.02.08}
}

@TECHREPORT{2006a-DutertreMoura,
  author = {Bruno Dutertre and Leonardo De Moura},
  title = {The yices {SMT} solver},
  institution = {Computer Science Laboratory, SRI International},
  year = {2006},
  file = {:./files/2006a-DutertreMoura.pdf:PDF},
  owner = {pavlenko},
  timestamp = {2011.03.08}
}

@INPROCEEDINGS{2005-DwyerHatcliff.etal,
  author = {Matthew B. Dwyer and John Hatcliff and Matthew Hoosier and Robby},
  title = {Building Your Own Software Model Checker Using the Bogor Extensible
	Model Checking Framework},
  booktitle = {Proc. International Conference on Computer Aided Verification ({CAV})},
  year = {2005},
  pages = {148--152},
  address = {Berlin, Heidelberg},
  publisher = {Springer-Verlag},
  acmid = {2153250},
  file = {:./files/2005-DwyerHatcliff.etal.pdf:PDF},
  isbn = {3-540-27231-3, 978-3-540-27231-1},
  location = {Edinburgh, Scotland, UK},
  numpages = {5},
  timestamp = {2006.09.22}
}

@INPROCEEDINGS{2002-BryantLahiri.etal,
  author = {E.Bryant and K.Lahiri and A.Seshia},
  title = {Modeling and Verifying Systems using a Logic of Counter Arithmetic
	with Lambda Expressions and Uninterpreted Functions},
  booktitle = {Proceedings of the 14th International Conference on Computer Aided
	Verification},
  year = {2002},
  series = {CAV '02},
  pages = {78--92},
  address = {London, UK, UK},
  publisher = {Springer-Verlag},
  acmid = {734437},
  file = {:./files/2002-BryantLahiri.etal.pdf:PDF},
  isbn = {3-540-43997-8},
  numpages = {15},
  timestamp = {2006.09.21}
}

@INPROCEEDINGS{2003-ClarkeKroening,
  author = {E.Clarke and D.Kroening},
  title = {Hardware Verification Using {ANSI-C} Programs As a Reference},
  booktitle = {Design Automation Conference, 2003. Proceedings of the {ASP}-{DAC}
	2003. Asia and South Pacific},
  year = {2003},
  pages = { 308 - 311},
  month = {jan},
  file = {:./files/2003-ClarkeKroening.pdf:PDF},
  keywords = { ANSI-C programs; SAT based bounded model checking; Verilog; bit vector
	logic decision problem; data encryption standard; equivalence problem;
	hardware verification; C language; computability; cryptography; formal
	verification; hardware description languages;},
  timestamp = {2006.09.27}
}

@INPROCEEDINGS{2003b-EenSoerensson,
  author = {Niklas E{\'e}n and Niklas S{\"o}rensson},
  title = {An Extensible {SAT} Solver},
  booktitle = {SAT},
  year = {2003},
  pages = {502-518},
  bibsource = {DBLP, http://dblp.uni-trier.de},
  owner = {villarraga},
  timestamp = {2012.12.03}
}

@MISC{web_ebddres,
  author = {{EBDDRES}},
  owner = {pavlenko},
  timestamp = {2011.03.04},
  url = {http://fmv.jku.at/ebddres}
}

@ARTICLE{2009-EbertJones,
  author = {Christof Ebert and Capers Jones},
  title = {Embedded Software: Facts, Figures, and Future},
  journal = {Computer},
  year = {2009},
  volume = {42},
  pages = {42-52},
  number = {4},
  address = {Los Alamitos, CA, USA},
  file = {2009-EbertJones.pdf:files/2009-EbertJones.pdf:PDF},
  issn = {0018-9162},
  owner = {villarraga},
  publisher = {IEEE Computer Society},
  timestamp = {2016.06.29}
}

@INPROCEEDINGS{2013-EbrahimiChen.etal,
  author = {M. Ebrahimi and L. Chen and H. Asadi and M. B. Tahoori},
  title = {{CLASS}: Combined logic and architectural soft error sensitivity
	analysis},
  booktitle = {Design Automation Conference {(ASP-DAC)}, 2013 18th Asia and South
	Pacific},
  year = {2013},
  pages = {601-607},
  month = {Jan},
  file = {2013-EbrahimiChen.etal.pdf:files/2013-EbrahimiChen.etal.pdf:PDF},
  issn = {2153-6961},
  owner = {villarraga},
  timestamp = {2016.08.19}
}

@INPROCEEDINGS{2015-EbrahimiSayed.etal,
  author = {M. Ebrahimi and N. Sayed and M. Rashvand and M. B. Tahoori},
  title = {Fault injection acceleration by architectural importance sampling},
  booktitle = {2015 International Conference on Hardware/Software Codesign and System
	Synthesis (CODES+ISSS)},
  year = {2015},
  owner = {udupi},
  timestamp = {2018.07.24}
}

@INPROCEEDINGS{2004-EckerEsen.etal,
  author = {Dr. Wolfgang Ecker and Volkan Esen and Thomas Steininger},
  title = {Memory Models for the Formal Verification of Assembler Code Using
	Bounded Model Checking},
  booktitle = {Proc. IEEE International Symposium on Object-Oriented Real-Time Distributed
	Computing.},
  year = {2004},
  pages = {129 -135},
  file = {:./files/2004-EckerEsen.etal.pdf:PDF},
  keywords = {assembler code;bounded model checking;formal proof complexity;formal
	verification;in-house BMC-Tool;instruction-set;memory models;optimization;processor-unit;assembly
	language;formal verification;hardware description languages;instruction
	sets;storage allocation;synchronisation;},
  timestamp = {2006.09.22}
}

@INPROCEEDINGS{2012-EckerVelten.etal,
  author = {Wolfgang Ecker and Michael Velten and Leily Zafari and Ajay Goyal},
  title = {Metamodeling and Code Generation - The Infineon Approach},
  booktitle = {Metamodelling and Code Generation for Embedded Systems},
  year = {2012},
  pages = {1--4},
  timestamp = {2014.02.07}
}

@CONFERENCE{2003-ClarkeTalupur.etal,
  author = {Edmund Clarke, Muralidhar Talupur, Helmut Veith and Dong Wang},
  title = {{SAT} Based Predicate Abstraction for Hardware Verification},
  booktitle = {Conference on Theory and Applications of Satisfiability Testing},
  year = {2003},
  editor = {Giunchiglia Enrico and Tacchella Armando},
  volume = {2919},
  series = {{LNCS}},
  pages = {78-92},
  month = {5},
  publisher = {Springer Berlin / Heidelberg},
  chapter = {SAT Based Predicate Abstraction for Hardware Verification},
  file = {:./files/2003-ClarkeTalupur.etal.pdf:PDF},
  owner = {nguyen},
  timestamp = {2008.06.03},
  url = {http://www.springerlink.com/content/qhbbw31mecb9033r/}
}

@INPROCEEDINGS{2001-EdwardsMa.etal,
  author = {Stephen A. Edwards and Tony Ma and Robert Damiano},
  title = {Using a Hardware Model Checker to Verify Software},
  booktitle = {Proc. International Conference on {ASIC} ({ASICON})},
  year = {2001},
  pages = {85 -90},
  file = {:./files/2001-EdwardsMa.etal.pdf:PDF},
  keywords = {C programs;C subset netlist translation procedure;embedded software
	verification;finite-state model checking;hardware circuits;hardware
	model checker;industrial-sized netlists;integer manipulation;memory
	allocation;model checking;nonrecursive programs;software verification;synthesis
	procedure;unstructured control flow;C language;electronic design
	automation;embedded systems;program verification;},
  timestamp = {2006.09.27}
}

@INPROCEEDINGS{2001-Een,
  author = {Nicklas Een},
  title = {P=NP What Does It Mean},
  booktitle = {Theory of Science and Resarch Ethics},
  year = {2001},
  file = {:./files/2001-Een.pdf:PDF},
  timestamp = {2006.09.21}
}

@ARTICLE{2003a-EenSoerensson,
  author = {Niklas Een and Niklas Soerensson},
  title = {Temporal Induction by Incremental {SAT} Solving},
  journal = {Electronic Notes in Theoretical Computer Science},
  year = {2003},
  volume = {89},
  pages = {543 - 560},
  number = {4},
  file = {:./files/2003a-EenSoerensson.pdf:PDF},
  issn = {1571-0661}
}

@ARTICLE{2000-vanEijk,
  author = {C. A. J. van Eijk},
  title = {Sequential equivalence checking based on structural similarities},
  journal = {IEEE Transactions on Computer-Aided Design of Integrated Circuits
	and Systems},
  year = {2000},
  volume = {19},
  pages = {814-819},
  number = {7},
  month = {Jul},
  issn = {0278-0070},
  keywords = {circuit optimisation;finite state machines;formal verification;logic
	CAD;sequential circuits;timing;ISCAS'89 benchmarks;circuit optimization;functional
	equivalence;retiming;sequential circuits;sequential equivalence checking;structural
	similarities;Boolean functions;Circuit synthesis;Combinational circuits;Data
	structures;Formal verification;Integrated circuit synthesis;Logic;Optimization
	methods;Process design;Sequential circuits},
  owner = {villarraga},
  timestamp = {2016.07.18}
}

@INPROCEEDINGS{1998-Eijk,
  author = {C. A. J. van Eijk},
  title = {Sequential Equivalence Checking without State Space Traversal},
  booktitle = {Proc. International Conference on Design, Automation and Test in
	Europe ({DATE})},
  year = {1998},
  pages = {618-623},
  address = {Paris, France},
  month = {March},
  file = {:./files/1998-Eijk.pdf:PDF}
}

@PHDTHESIS{1997-Eijk,
  author = {C. A. J. van Eijk},
  title = {Formal Methods for the Verification of Digital Circuits},
  school = {Eindhoven University of Technology},
  year = {1997},
  type = {Dissertation},
  file = {:./files/1997-Eijk.pdf:PDF}
}

@INPROCEEDINGS{1996-EijkJess,
  author = {C.A.J. van Eijk and J.A.G. Jess},
  title = {Exploiting Functional Dependencies in Finite State Machine Verification},
  booktitle = {Proc. European Design and Test Conference (EDTC)},
  year = {1996},
  pages = {9 -14},
  file = {:./files/1996-EijkJess.pdf:PDF},
  keywords = { FSM verification; finite state machine; functional dependencies;
	functionally dependent state variables; state encodings; encoding;
	finite state machines; formal verification; logic CAD; logic design;},
  timestamp = {2006.09.21}
}

@INPROCEEDINGS{1995-EijkJess,
  author = {C.A.J. van Eijk and J. A. G. Jess},
  title = {Detection of Equivalent State Variables in Finite State Machine Verification},
  booktitle = {In Proc of the International Workshop on Logic Synthesis},
  year = {1995},
  pages = {3--35},
  owner = {villarraga},
  timestamp = {2016.07.18}
}

@ARTICLE{2000-Eiriksson,
  author = {Asgeir Por EirIksson},
  title = {The Formal Design of {1M}-gate {ASIC}s},
  journal = {Formal Methods in System Design},
  year = {2000},
  volume = {16},
  pages = {7-22},
  file = {:./files/2000-Eiriksson.pdf:PDF},
  timestamp = {2006.10.12}
}

@INPROCEEDINGS{1998-Eiriksson,
  author = {Asgeir Por EirIksson},
  title = {The Formal Design of {1-M} gate {ASIC}s},
  booktitle = {Proc. International Conference on Formal Methods in Computer-Aided
	Design ({FMCAD})},
  year = {1998},
  pages = {49--63},
  address = {London, UK, UK},
  publisher = {Springer-Verlag},
  acmid = {683089},
  file = {:./files/1998-Eiriksson.pdf:PDF},
  isbn = {3-540-65191-8},
  numpages = {15},
  timestamp = {2006.09.21}
}

@ARTICLE{2005-EisenbarthKoschke.etal,
  author = {Eisenbarth, Thomas and Koschke, Rainer and Vogel, Gunther},
  title = {Static object trace extraction for programs with pointers},
  journal = {Journal of Systems and Software},
  year = {2005},
  volume = {77},
  pages = {263--284},
  number = {3},
  publisher = {Elsevier}
}

@INPROCEEDINGS{2003-EisenblaetterFuegenschuh.etal,
  author = {Andreas Eisenblaetter and Armin Fuegenschuh and Hans-Florian Geerdes
	and Daniel Junglas and Thorsten Koch and Alexander Martin},
  title = {Optimization Methods for {UMTS} Radio Network Planning},
  booktitle = {Proc. International Conference on Operation Research},
  year = {2003},
  pages = {31-38},
  publisher = {Springer},
  note = {ZIB-Report 03-41},
  editors = {D. Ahr and R. Fahrion and M. Oswald and Gerd Reinelt},
  file = {:./files/2003-EisenblaetterFuegenschuh.etal.pdf:PDF},
  isbn = {3-540-21445-3},
  language = {English}
}

@ARTICLE{2002-EisenblaetterKoch.etal,
  author = {Andreas Eisenblaetter and Thorsten Koch and Alexander Martin and
	T. Achterberg and Armin Fuegenschuh and Arie Koster and Oliver Wegel
	and Roland Wessaely},
  title = {Modelling Feasible Network Configurations for {UMTS}},
  journal = {Telecommunications Network Design and Management},
  year = {2002},
  volume = {23},
  pages = {1-24},
  address = {Boston/Dordrecht/London},
  editor = {G. Anandalingam and S. Raghavan},
  file = {:./files/2002-EisenblaetterKoch.etal.pdf:PDF},
  publisher = {Kluwer Academic Publishers},
  seealso = {EiFuKoKoMaPfWeWe02},
  series = {Operations Research/Computer Science Interfaces},
  url = {http://www.wkap.nl/prod/b/1-4020-7318-6}
}

@ARTICLE{1982-EmersonClarke,
  author = {Emerson, E Allen and Clarke, Edmund M},
  title = {Using branching time temporal logic to synthesize synchronization
	skeletons},
  journal = {Science of Computer programming},
  year = {1982},
  volume = {2},
  pages = {241--266},
  number = {3},
  owner = {fadiheh},
  publisher = {Elsevier},
  timestamp = {2018.07.27}
}

@ARTICLE{1986-EmersonHalpern,
  author = {Emerson, E. Allen and Halpern, Joseph Y.},
  title = {``Sometimes'' and ``Not Never'' Revisited: On Branching Versus Linear
	Time Temporal Logic},
  journal = {J. ACM},
  year = {1986},
  volume = {33},
  pages = {151--178},
  number = {1},
  month = jan,
  acmid = {4999},
  address = {New York, NY, USA},
  issn = {0004-5411},
  issue_date = {Jan. 1986},
  numpages = {28},
  owner = {stoffel},
  publisher = {ACM},
  timestamp = {2016.05.10}
}

@INPROCEEDINGS{1999-EmersonTrefler,
  author = {Emerson, E.A. and Trefler, R.J.},
  title = {Parametric Quantitative Temporal Reasoning},
  booktitle = {Logic in Computer Science, 1999. Proceedings. 14th Symposium on},
  year = {1999},
  pages = {336 -343},
  file = {:./files/1999-EmersonTrefler.pdf:PDF},
  keywords = {atomic events;model checking algorithm;parameterized real-time computation
	tree logic;parametric quantitative temporal reasoning;polynomial;quantitative
	reasoning;quantitative temporal specifications;temporal ordering;formal
	specification;polynomials;temporal logic;temporal reasoning;timing;}
}

@INPROCEEDINGS{1999-EngblomErmedahl,
  author = {Jakob Engblom and Andreas Ermedahl},
  title = {Pipeline Timing Analysis Using Trace Driven Simulator},
  booktitle = {Proc. International Conference on Real-Time Computing Systems and
	Applications},
  year = {1999},
  pages = {88 -95},
  file = {:./files/1999-EngblomErmedahl.pdf:PDF},
  keywords = {CPU;cache analysis;embedded real-time systems;execution time predictions;high-level
	program flow analysis;instructions;pipeline timing analysis;pipelined
	processors;trace-driven simulator;worst-case execution time;data
	flow analysis;embedded systems;pipeline processing;virtual machines;},
  timestamp = {2006.09.22}
}

@MISC{0000-EngblomErmedahl.etal,
  author = {J. Engblom and A. Ermedahl and G. Kostafsson and H. Hansson and M.
	Sjoedin},
  title = {WCET Analysis for Embedded Real Time Systems},
  file = {0000-EngblomErmedahl.etal.pdf:files/0000-EngblomErmedahl.etal.pdf:PDF},
  owner = {stoffel},
  timestamp = {2006.09.22}
}

@INPROCEEDINGS{2001-EngblomErmedahl.etal,
  author = {Jakob Engblom and Andreas Ermedahl and Friedhelm Stappert},
  title = {A Worst-Case Execution-Time Analysis Tool Prototype for Embedded
	Real-Time Systems},
  booktitle = {The first Workshop on Real-Time Tools ({RT-TOOLS} 2001) held in conjunction
	with {CONCUR} 2001, Aalborg},
  year = {2001},
  editor = {Paul Pettersson},
  month = {August},
  file = {:./files/2001-EngblomErmedahl.etal.pdf:PDF},
  url = {http://www.mrtc.mdh.se/index.php?choice=publications&id=0992}
}

@INPROCEEDINGS{2000-EnglerChelf.etal,
  author = {Engler, Dawson and Chelf, Benjamin and Chou, Andy and Hallem, Seth},
  title = {Checking system rules using system-specific, programmer-written compiler
	extensions},
  booktitle = {Proceedings of the 4th conference on Symposium on Operating System
	Design \& Implementation - Volume 4},
  year = {2000},
  series = {OSDI'00},
  pages = {1--1},
  address = {Berkeley, CA, USA},
  publisher = {USENIX Association},
  acmid = {1251230},
  file = {:./files/2000-EnglerChelf.etal.pdf:PDF},
  location = {San Diego, California},
  numpages = {1}
}

@INPROCEEDINGS{1993-EntrenaCheng,
  author = {L. A. Entrena and K. T. Cheng},
  title = {Sequential Logic Optimization by Redundancy Addition and Removal},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {1993},
  pages = {310-315},
  month = {November},
  file = {:./files/1993-EntrenaCheng.pdf:PDF}
}

@ARTICLE{2012-EntrenaGarcia-Valderas.etal,
  author = {L. Entrena and M. Garcia-Valderas and R. Fernandez-Cardenal and A.
	Lindoso and M. Portela and C. Lopez-Ongil},
  title = {Soft Error Sensitivity Evaluation of Microprocessors by Multilevel
	Emulation-Based Fault Injection},
  journal = {IEEE Transactions on Computers},
  year = {2012},
  volume = {61},
  pages = {313-322},
  number = {3},
  month = {March},
  file = {2012-EntrenaGarcia-Valderas.etal.pdf:files/2012-EntrenaGarcia-Valderas.etal.pdf:PDF},
  issn = {0018-9340},
  owner = {bartsch},
  timestamp = {2016.11.30}
}

@INPROCEEDINGS{2001-EntrenaLopez.etal,
  author = {Luis Entrena and Celia Lopez and Emilio Olias},
  title = {Automatic Generation of Fault Tolerant {VHDL} Designs in {RTL}},
  booktitle = {Proc. International Forum on Design Languages},
  year = {2001},
  file = {:./files/2001-EntrenaLopez.etal.pdf:PDF},
  journal = {Forum on Design Languages},
  timestamp = {2006.09.14}
}

@INPROCEEDINGS{2005-ErleSchwarz.etal,
  author = {Mark A. Erle and Eric M. Schwarz and Michael J. Schulte},
  title = {Decimal Multiplication With Efficient Partial Product Generation},
  booktitle = {Proc. IEEE Symposium on Computer Arithmetic},
  year = {2005},
  pages = { 21 - 28},
  file = {:./files/2005-ErleSchwarz.etal.pdf:PDF},
  keywords = { accounting; banking; combinational circuit; currency conversion;
	digit-by-digit multiplier; financial analysis; fixed-point decimal
	multiplication; insurance; recoding scheme; signed-digit adder; signed-digit
	partial products; signed-magnitude representations; tax calculation;
	adders; combinational circuits; fixed point arithmetic; floating
	point arithmetic; multiplying circuits;},
  timestamp = {2006.10.04}
}

@INPROCEEDINGS{2005-ErmedahlGustafsson.etal,
  author = {Andreas Ermedahl and Jan Gustafsson and Bj{\"o}rn Lisper},
  title = {Experiences from Industrial WCET Analysis Case Studies},
  booktitle = {Proc. Fifth International Workshop on Worst-Case Execution Time (WCET)
	Analysis},
  year = {2005},
  editor = {Reinhard Wilhelm},
  month = {July},
  file = {:./files/2005-ErmedahlGustafsson.etal.pdf:PDF},
  timestamp = {2006.09.22},
  url = {http://www.mrtc.mdh.se/index.php?choice=publications&id=0932}
}

@INPROCEEDINGS{2005-EvangelistaFrancois.etal,
  author = {Sami Evangelista and Jean-Francois and Pradat-Peyre},
  title = {Memory Efficient State Space Storage in Explicit Software Model Checking},
  booktitle = {Model Checking Software},
  year = {2005},
  volume = {Volume 3639/2005},
  series = {Lecture Notes in Computer Science},
  pages = {43-57},
  publisher = {Springer Berlin / Heidelberg},
  abstract = {The limited amount of memory is the major bottleneck in model checking
	tools based on an explicit states enumeration. In this context, techniques
	allowing an efficient representation of the states are precious.
	We present in this paper a novel approach which enables to store
	the state space in a compact way. Though it belongs to the family
	of explicit storage methods, we qualify it as semi-explicit since
	all states are not explicitly represented in the state space. Our
	experiments report a memory reduction ratio up to 95% with only a
	tripling of the computing time in the worst case.},
  file = {:./files/2005-EvangelistaFrancois.etal.pdf:PDF},
  keywords = {State Exploring Assembly Model Checker},
  owner = {nguyen},
  timestamp = {2006.08.29},
  url = {http://www.springerlink.com/content/0yyma7pck569akby/fulltext.pdf}
}

@INPROCEEDINGS{2011-EvekingDornes.etal,
  author = {Hans Eveking and Tobias Dornes and Martin Schweikert},
  title = {Using {SystemVerilog Assertions} to Relate Non-cycle-accurate to
	Cycle-accurate Designs},
  booktitle = {Proc. of 16th {IEEE} International High Level Design Validation and
	Test Workshop ({HLDVT})},
  year = {2011},
  pages = {17--24},
  file = {:./files/2011-EvekingDornes.etal.pdf:PDF}
}

@INPROCEEDINGS{1996-BalarinHsieh.etal,
  author = {F.Balarin and H.Hsieh and A.Jurecska and M.Marelli and L.Lavagno},
  title = {Formal Verification Of Embedded System Based On {CFSM}},
  booktitle = {Proc. Annual Conference on Design Automation},
  year = {1996},
  pages = {568 -571},
  file = {:./files/1996-BalarinHsieh.etal.pdf:PDF},
  keywords = {CFSM networks;POLIS;abstractions;automata-theoretic techniques;bread-boarding;codesign
	finite state machines;embedded systems;formal model;formal proof;formal
	verification;functional properties;functionality;industrial embedded
	system;safety requirements;simulation;timing;digital simulation;finite
	state machines;formal specification;formal verification;logic design;real-time
	systems;},
  timestamp = {2006.09.27}
}

@INPROCEEDINGS{1998-VaragsBezzera.etal,
  author = {F.Varags and E.Bezzera and A.Terroso and D. Barros},
  title = {Realiability Verification of Fault-Tolerant Systems Design Based
	on Mutation Analysis},
  year = {1998},
  pages = {55 -58},
  file = {:./files/1998-VaragsBezzera.etal.pdf:PDF},
  keywords = { CAD tools; fault injection; fault-tolerant systems design; mutation
	analysis; reliability verification; simulation data analysis; digital
	systems; embedded systems; fault tolerant computing; hardware description
	languages; hardware-software codesign; program testing;},
  timestamp = {2006.09.14}
}

@BOOK{1992-Fabricius,
  title = {Modern Digital Design and Switching Theory},
  publisher = {CRC Press},
  year = {1992},
  author = {E. Fabricius}
}

@INPROCEEDINGS{2019-FadihehStoffel.etal,
  author = {Fadiheh, Mohammad Rahmani and Stoffel, Dominik and Barrett, Clark
	and Mitra, Subhasish and Kunz, Wolfgang},
  title = {Processor Hardware Security Vulnerabilities and their Detection by
	Unique Program Execution Checking},
  booktitle = {Design, Automation \& Test in Europe Conference (DATE)},
  year = {2019},
  owner = {fadiheh},
  timestamp = {2019.01.23}
}

@ARTICLE{2018-FadihehStoffel.etal,
  author = {Fadiheh, Mohammad Rahmani and Stoffel, Dominik and Barrett, Clark
	and Mitra, Subhasish and Kunz, Wolfgang},
  title = {Processor Hardware Security Vulnerabilities and their Detection by
	Unique Program Execution Checking},
  journal = {arXiv preprint arXiv:1812.04975},
  year = {2018},
  owner = {fadiheh},
  timestamp = {2018.12.03}
}

@INPROCEEDINGS{2018-FadihehUrdahl.etal,
  author = {Fadiheh, Mohammad Rahmani and Urdahl, Joakim and Nuthakki, Srinivas
	Shashank and Mitra, Subhasish and Barrett, Clark and Stoffel, Dominik
	and Kunz, Wolfgang},
  title = {Symbolic quick error detection using symbolic initial state for pre-silicon
	verification},
  booktitle = {Design, Automation \& Test in Europe Conference (DATE)},
  year = {2018},
  pages = {55--60},
  organization = {IEEE},
  owner = {fadiheh},
  timestamp = {2018.07.12}
}

@ARTICLE{2001-FallahDevadas.etal,
  author = {F. Fallah and S. Devadas and K. Keutzer},
  title = {Functional Vector Generation for {HDL} Models Using Linear Programming
	and {Boolean} Satisfiability},
  journal = {IEEE Transactions on Computer-Aided Design},
  year = {2001},
  volume = {20},
  pages = {994-1002},
  number = {8},
  month = {August},
  file = {:./files/2001-FallahDevadas.etal.pdf:PDF}
}

@MASTERSTHESIS{2012-ThomasFehmel,
  author = {Thomas Fehmel},
  title = {Modellgenerierung von Interrupt basierten HW/SW-Systemen f\"ur die
	formale Verifikation},
  school = {TU Kaiserslautern},
  year = {2012},
  type = {{Diplomarbeit}},
  file = {:files/2012-ThomasFehmel.pdf:PDF},
  owner = {bschmidt},
  timestamp = {2013.12.20}
}

@MASTERSTHESIS{2011-ThomasFehmel,
  author = {Thomas Fehmel},
  title = {Extraktion des Kontrollflussgrafen (CFG) aus Maschienencode f\"ur
	die Software-Verifikation},
  school = {TU Kaiserslautern},
  year = {2011},
  type = {{Studienarbeit}},
  file = {:files/2011-ThomasFehmel.pdf:PDF},
  owner = {bschmidt},
  timestamp = {2013.12.20}
}

@ARTICLE{2018-Fehmel,
  author = {T. Fehmel and D. Stoffel and W. Kunz},
  title = {Generation of Abstract Driver Models for IP Integration Verification},
  journal = {IEEE Transactions on Emerging Topics in Computing},
  year = {2018},
  owner = {fehmel},
  timestamp = {2019.05.27}
}

@INPROCEEDINGS{2005-FengHu.etal,
  author = {Xiushan Feng and Alan J. Hu and Jin Yang},
  title = {Partitioned Model Checking from Software Specifications},
  booktitle = {Proc. Asia South Pacific Design Automation Conference},
  year = {2005},
  pages = {583--587},
  publisher = {IEEE Press},
  file = {:./files/2005-FengHu.etal.pdf:PDF}
}

@INPROCEEDINGS{2017-FerraiuoloXu.etal,
  author = {Ferraiuolo, Andrew and Xu, Rui and Zhang, Danfeng and Myers, Andrew
	C and Suh, G Edward},
  title = {Verification of a practical hardware security architecture through
	static information flow analysis},
  booktitle = {ACM SIGARCH Computer Architecture News},
  year = {2017},
  volume = {45},
  number = {1},
  pages = {555--568},
  organization = {ACM},
  owner = {fadiheh},
  timestamp = {2018.07.13}
}

@INPROCEEDINGS{2018-FerraiuoloZhao.etal,
  author = {Ferraiuolo, Andrew and Zhao, Mark and Myers, Andrew C and Suh, G
	Edward},
  title = {HyperFlow: A processor architecture for nonmalleable, timing-safe
	information flow security},
  booktitle = {Proceedings of the 2018 ACM SIGSAC Conference on Computer and Communications
	Security},
  year = {2018},
  pages = {1583--1600},
  organization = {ACM}
}

@INPROCEEDINGS{2004-FeyGrosse.etal,
  author = {G{\"o}rschwin Fey and Daniel Gro{\ss}e and Tim Cassens and Christian
	Genz and Tim Warode and Rolf Drechsler},
  title = {{ParSyC}: An Efficient {SystemC}Ma Parser},
  booktitle = {Workshop on Synthesis And System Integration of Mixed Information
	technologies (SASIMI)},
  year = {2004},
  pages = {148--154},
  address = {Kanazawa, Japan},
  month = {Oct.},
  file = {:files/2004-FeyGross.etal.pdf:PDF}
}

@INPROCEEDINGS{2005-FidgeCook,
  author = {Colin Fidge and Phil Cook},
  title = {Model Checking Interrupt Dependent Software},
  booktitle = {Software Engineering Conference, 2005. {APSEC} '05. 12th Asia-Pacific},
  year = {2005},
  pages = {51-58},
  file = {:./files/2005-FidgeCook.pdf:PDF},
  timestamp = {2006.09.22}
}

@PHDTHESIS{1992-Filkorn,
  author = {Thomas Filkorn},
  title = {Symbolische Methoden fuer die Verifikation endlicher Zustandssysteme},
  school = {Institut fuer Informatik der Technischen Universitaet Muenchen},
  year = {1992},
  type = {Dissertation}
}

@TECHREPORT{2005-FischettiBertacco.etal,
  author = {Matteo Fischetti and Livio Bertacco and Andrea Lodi},
  title = {A Feasibility Pump Heuristic for General Mixed-Integer Problems},
  institution = {Universitaet di Bologna - D.E.I.S. - Operations Research},
  year = {2005},
  file = {:./files/2005-FischettiBertacco.etal.pdf:PDF}
}

@ARTICLE{2005-FischettiGlover.etal,
  author = {Matteo Fischetti and Fred Glover and Andrea Lodi},
  title = {The Feasibility Pump},
  journal = {Mathematical Programming},
  year = {2005},
  volume = {104},
  pages = {91-104},
  number = {1},
  file = {:./files/2005-FischettiGlover.etal.pdf:PDF}
}

@TECHREPORT{2004-FischettiGlover.etal,
  author = {Matteo Fischetti and Fred Glover and Andrea Lodi},
  title = {The Feasibility Pump},
  institution = {Universit{\`a} di Bologna - D.E.I.S. - Operations Research},
  year = {2004},
  number = {OR-04-4},
  file = {:./files/2004-FischettiGlover.etal.pdf:PDF}
}

@ARTICLE{2003-FischettiLodi,
  author = {Matteo Fischetti and Andrea Lodi},
  title = {Local Branching},
  journal = {Mathematical Programming},
  year = {2003},
  volume = {98},
  pages = {23-47},
  number = {1-3},
  file = {:./files/2003-FischettiLodi.pdf:PDF}
}

@ARTICLE{1999-Fisler,
  author = {Kathi Fisler},
  title = {Timing Diagrams Formalization and Algorithmic Verification},
  journal = {Journal of Logic, Language and Information},
  year = {1999},
  volume = {8},
  pages = {323-361},
  number = {3},
  file = {:./files/1999-Fisler.pdf:PDF},
  timestamp = {2006.09.19}
}

@INPROCEEDINGS{2005-FlanaganGodefroid,
  author = {Flanagan, Cormac and Godefroid, Patrice},
  title = {Dynamic Partial-Order Reduction for Model Checking Software},
  booktitle = {Proceedings of the 32nd {ACM} {SIGPLAN}-{SIGACT} symposium on Principles
	of programming languages},
  year = {2005},
  series = {POPL '05},
  pages = {110--121},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {1040315},
  file = {:./files/2005-FlanaganGodefroid.pdf:PDF},
  isbn = {1-58113-830-X},
  keywords = {partial-order reduction, software model checking},
  location = {Long Beach, California, USA},
  numpages = {12}
}

@INPROCEEDINGS{2005-FloresMonteiro.etal,
  author = {Paulo Flores and Jose Monteiro and Eduardo Costa},
  title = {An Exact Algorithm for the Maximal Sharing of Partial Terms in Multiple
	Constant Multiplications},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2005},
  pages = { 13 - 16},
  file = {:./files/2005-FloresMonteiro.etal.pdf:PDF},
  keywords = { AND gates; {Boolean} network; CSD representation; MSD representation;
	{SAT}-based solver; adders; binary representation; exact algorithm;
	integer linear programming; maximal partial term sharing; multiple
	constant multiplication; set of coefficient; subtracters; Boolean
	functions; FIR filters; adders; digital arithmetic; integer programming;
	linear programming; logic design; logic gates;},
  timestamp = {2006.09.27}
}

@MISC{0000-Folkesson,
  author = {Peter Folkesson},
  title = {Fault-Tolerant Computing Fault Injection for Dependability Validation},
  note = {slides},
  file = {0000-Folkesson.pdf:files/0000-Folkesson.pdf:PDF},
  owner = {stoffel},
  timestamp = {2006.09.14}
}

@TECHREPORT{1996-Folkesson,
  author = {Peter Folkesson},
  title = {Experimental Validation of a Fault-Tolerant System Using Physical
	Fault Injection},
  institution = {Technische Universit{\"a}t Wien, Institut f{\"u}r Technische Informatik},
  year = {1996},
  file = {:./files/1996-Folkesson.pdf:PDF},
  timestamp = {2006.09.14}
}

@MISC{2004-ForrestNuez.etal,
  author = {John Forrest and David de la Nuez and Robin Lougee-Heimer},
  title = {{CLP} User Guide},
  month = {August},
  year = {2004},
  organization = {COIN-OR},
  owner = {stoffel},
  timestamp = {2016.05.11},
  url = {http://www.coin-or.org/Clp/userguide}
}

@MISC{web_kascpar,
  author = {{FZI} {Forschungszentrum f{\"u}r Informatik}},
  title = {{KaSCPar}},
  howpublished = {ftp.fzi.de/downloads/sim/archives/kascpar-documentation.pdf},
  key = {web_kascpar},
  owner = {stoffel},
  timestamp = {2016.05.11},
  url = {ftp.fzi.de/downloads/sim/archives/kascpar-documentation.pdf}
}

@MISC{2014-Foster,
  author = {Harry Foster},
  title = {The Wilson Research Group Functional Verification Study},
  howpublished = {Mentor Graphics},
  year = {2014},
  owner = {joakim},
  timestamp = {2016.03.18}
}

@MISC{web_clang,
  author = {{LLVM} Foundation},
  title = {{Clang}},
  howpublished = {http://clang.llvm.org},
  key = {web_clang},
  owner = {stoffel},
  timestamp = {2016.05.11},
  url = {http://clang.llvm.org}
}

@MISC{web_llvm,
  author = {{LLVM} Foundation},
  title = {{LLVM}},
  howpublished = {http://llvm.org},
  key = {web_llvm},
  owner = {stoffel},
  timestamp = {2016.05.11},
  url = {http://llvm.org}
}

@BOOK{2002-FourerGay.etal,
  title = {{AMPL}: A Modelling Language for Mathematical Programming},
  publisher = {Duxbury Press, Brooks/Cole Publishing Company},
  year = {2002},
  author = {Robert Fourer and David M. Gay and Brian W. Kernighan},
  edition = {2nd},
  month = {November},
  file = {:./files/2002-FourerGay.etal.pdf:PDF}
}

@INPROCEEDINGS{2002-Fox,
  author = {Anthony C. J. Fox},
  title = {Formal Specification and Verification of {ARM6}},
  booktitle = {Proc. International Conference on on Theorem Proving in Higher Order
	Logics ({TPHOLs})},
  year = {2003},
  pages = {25-40},
  bibsource = {DBLP, http://dblp.uni-trier.de},
  ee = {http://springerlink.metapress.com/openurl.asp?genre=article{\&}issn=0302-9743{\&}volume=2758{\&}spage=25},
  file = {foxarm6.pdf:foxarm6.pdf:PDF},
  owner = {wedler},
  timestamp = {2008.12.18}
}

@INPROCEEDINGS{2008-FraerKamhi.etal,
  author = {R. Fraer and G. Kamhi and M. K. Mhameed},
  title = {A new paradigm for synthesis and propagation of clock gating conditions},
  booktitle = {Design Automation Conference, 2008. DAC 2008. 45th ACM/IEEE},
  year = {2008},
  pages = {658-663},
  month = {June},
  abstract = {Clock gating has become a standard practice for saving dynamic power
	in the clock network. Due to design reuse, it is common to find designs
	that have already some partial clock gating. We propose to exploit
	the existing clock gating in order to extract stronger gating conditions
	for blocks that are poorly gated or not gated at all. A second contribution
	of our paper is a robust and scalable approach to extract stability
	conditions for clock gating. Finally, we present a uniform treatment
	of unobservability and stability as dual approaches for propagating
	gating conditions forward and backward. Experimental results demonstrate
	significant power reduction (in the range of 14% - 55% of the clock
	power) on Intel micro-processor designs.},
  issn = {0738-100X},
  keywords = {clocks;logic design;logic gates;low-power electronics;microprocessor
	chips;Intel microprocessor designs;clock gating condition;logic synthesis;power
	reduction;Clocks;Design optimization;Energy consumption;Floating-point
	arithmetic;Logic design;Network synthesis;Pipelines;Power dissipation;Robust
	stability;Synchronization;Low-power design;clock gating}
}

@ARTICLE{2006-FreibotheSchoenherr.etal,
  author = {M. Freibothe and J. Schoenherr and B. Straube},
  title = {Formal Verification of the Quasi-Static Behavior of Mixed-Signal
	Circuits by Property Checking},
  journal = {Electronic Notes in Theoretical Computer Science},
  year = {2006},
  volume = {153},
  pages = {23 - 35},
  number = {3},
  file = {:./files/2006-FreibotheSchoenherr.etal.pdf:PDF},
  issn = {1571-0661}
}

@BOOK{1997-FroehwirthAbdennadher,
  title = {Constraint-Programmierung Grundlagen und Anwendungen},
  publisher = {Springer},
  year = {1997},
  author = {T. Froehwirth and S. Abdennadher}
}

@MISC{1995-FroesslGerlach.etal,
  author = {Juergen Froessl and Joachim Gerlach and Thomas Kropf},
  title = {Symbolic Model-Checking for Real-Time Circuits and Specifications},
  year = {1995},
  file = {:./files/1995-FroesslGerlach.etal.pdf:PDF},
  owner = {stoffel},
  timestamp = {2016.05.11}
}

@INPROCEEDINGS{1988-FujitaFujisawa.etal,
  author = {M. Fujita and H. Fujisawa and N. Kawato},
  title = {Evaluation and improvements of {Boolean} Comparison Method Based
	on Binary Decision Diagrams},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {1988},
  pages = {2-5},
  address = {Santa Clara, CA},
  month = {November},
  file = {:./files/1988-FujitaFujisawa.etal.pdf:PDF}
}

@INPROCEEDINGS{1991-FujitaMatsunaga.etal,
  author = {M. Fujita and Y. Matsunaga and T. Kakuda},
  title = {On Variable Ordering of Binary Decision Diagrams for the Application
	of Multi-Level Logic Synthesis},
  booktitle = {Proc. European Design Automation Conference ({EDAC})},
  year = {1991},
  pages = {50-54},
  month = {March},
  file = {:./files/1991-FujitaMatsunaga.etal.pdf:PDF}
}

@ARTICLE{1997-FujitaMcGeer.etal,
  author = {M. Fujita and P. McGeer and J. Yang},
  title = {Multi-Terminal Binary Decision Diagrams: an Efficient Data Structure
	for Matrix Representation},
  journal = {Formal Methods in System Design},
  year = {1997},
  volume = {10},
  pages = {149-169},
  file = {:./files/1997-FujitaMcGeer.etal.pdf:PDF}
}

@BOOK{1985-Fujiwara,
  title = {Logic Testing and Design for Testability},
  publisher = {{MIT}-Press Series in Computer Systems},
  year = {1985},
  editor = {Herb Schwetman},
  author = {H. Fujiwara}
}

@INPROCEEDINGS{1985-FujiwaraShimono,
  author = {H. Fujiwara and T. Shimono},
  title = {{FAN}: A Fanout-Oriented Test Pattern Generation Algorithm},
  booktitle = {Proc. {IEEE} International Symposium on Circuits and Systems},
  year = {1985},
  pages = {671-674},
  month = {June}
}

@INPROCEEDINGS{2000-CornoReorda.etal,
  author = {Fulvio Corno, Matteo Sonza Reorda, Giovanni Squillero},
  title = {Evolving Cellular Automata for Self-Testing Hardware},
  booktitle = {Conference on Evolvable Systems: From Biology to Hardware},
  year = {2000},
  pages = {31--40},
  address = {London, UK, UK},
  publisher = {Springer-Verlag},
  acmid = {656899},
  file = {:./files/2000-CornoReorda.etal.pdf:PDF},
  isbn = {3-540-67338-5},
  numpages = {10},
  timestamp = {2006.09.14}
}

@MISC{1999-AignerDiwan.etal,
  author = {G.Aigner and A.Diwan and D.Heine and M.Lam and D.Moore and B.Murphy
	and C.Sapuntazakis},
  title = {An Overview Of The Suif-2 Compiler Infrastructre},
  year = {1999},
  file = {:./files/1999-AignerDiwan.etal.pdf:PDF},
  owner = {stoffel},
  timestamp = {2006.09.21}
}

@ARTICLE{2000-EvenPaul,
  author = {G.Even and W.J.Paul},
  title = {On The Chip Of Ieee Complaint Folting Point Units},
  journal = {IEEE Transaction On Computers},
  year = {2000},
  volume = {49},
  pages = {398-413},
  file = {:./files/2000-EvenPaul.pdf:PDF},
  timestamp = {2006.10.04}
}

@INPROCEEDINGS{2005-GadkariRamesh,
  author = {Ambar A. Gadkari and S. Ramesh},
  title = {Automated Synthesis Of Assertion Monitors Using Visual Specifications},
  booktitle = {Proc. International Conference on Design, Automation and Test in
	Europe ({DATE})},
  year = {2005},
  volume = {1},
  pages = { 390 - 395},
  file = {:./files/2005-GadkariRamesh.pdf:PDF},
  keywords = { CESC language; Clocked Event Sequence Chart; assertion-based verification;
	automated assertion monitor synthesis; bus protocols; clock domains;
	formal semantics; graphical syntax; synchronous language paradigm;
	system design; system level design; system level interactions; textual
	syntax; visual language; visual specifications; formal verification;
	monitoring; programming language semantics; systems analysis; visual
	languages;},
  timestamp = {2006.09.19}
}

@MISC{2001-Gaertner,
  author = {Felix Gaertner},
  title = {Formalization and Verifcation of Fault Tolerance and Security},
  year = {2001},
  file = {:./files/2001-Gaertner.pdf:PDF},
  owner = {stoffel},
  timestamp = {2006.09.14}
}

@BOOK{2000-GajskiZhu.etal,
  title = {SPECC: Specification Language and Methodology},
  year = {2000},
  author = {Gajski, Daniel and Zhu, Jianwen and D. Omer, R and Gerstlauer, Andreas
	and Zhao, Shuqing},
  month = {01}
}

@ARTICLE{1993-GalloLongo.etal,
  author = {Giorgio Gallo and Giustino Longo and Stefano Pallottino and Sang
	Nguyen},
  title = {Directed hypergraphs and applications },
  journal = {Discrete Applied Mathematics },
  year = {1993},
  volume = {42},
  pages = {177 - 201},
  number = {2–3},
  file = {1993-GalloLongo.etal.pdf:files/1993-GalloLongo.etal.pdf:PDF},
  issn = {0166-218X},
  owner = {schwarz},
  timestamp = {2017.01.17},
  url = {http://www.sciencedirect.com/science/article/pii/0166218X9390045P}
}

@INPROCEEDINGS{2006-GaluzziPanainte.etal,
  author = {Carlo Galuzzi and Elena Moscu Panainte and Yana Yankova and Koen
	Bertels and Stamatis Vassiliadis},
  title = {Automatic Selection of Application-Specific Instruction-Set Extensions},
  booktitle = {Proc. international conference on Hardware/software codesign and
	system synthesis},
  year = {2006},
  pages = {160 -165},
  file = {:./files/2006-GaluzziPanainte.etal.pdf:PDF},
  keywords = {application-specific instruction-set extensions;automatic selection;hardware
	resources constraints;hardware-software codesign;instruction sets;},
  owner = {loitz},
  review = {I have some doubts about the use of MAXMISOs. How are they handled
	if a complete MAXMISO is not fitting in the architecture?},
  timestamp = {2007.01.08}
}

@ARTICLE{2001-GanaiYalagandula.etal,
  author = {Ganai, Malay and Yalagandula, Praveen and Aziz, Adnan and Kuehlmann,
	Andreas and Singhal, Vigyan},
  title = {SIVA: A System for Coverage-Directed State Space Search},
  journal = {J. Electron. Test.},
  year = {2001},
  volume = {17},
  pages = {11--27},
  number = {1},
  month = feb,
  acmid = {570006},
  address = {Norwell, MA, USA},
  file = {:./files/2001-GanaiYalagandula.etal.pdf:PDF},
  issn = {0923-8174},
  issue_date = {February 2001},
  keywords = {coverage, formal methods, functional verification, guided search},
  numpages = {17},
  publisher = {Kluwer Academic Publishers}
}

@INPROCEEDINGS{2005a-GanaiGupta.etal,
  author = {Malay K. Ganai and Aarti Gupta and Pranav Ashar},
  title = {Verification of Embedded Memory Systems using Efficient Memory Modeling.},
  booktitle = {Proc. International Conference on Design, Automation and Test in
	Europe ({DATE})},
  year = {2005},
  pages = {1096-1101},
  abstract = {We describe verification techniques for embedded memory systems using
	efficient memory modeling (EMM), without explicitly modeling each
	memory bit. We extend our previously proposed approach of EMM in
	Bounded Model Checking (BMC) for a single read/write port single
	memory system, to more commonly occurring systems with multiple memories,
	having multiple read and write ports. More importantly, we augment
	such EMM to providing correctness proofs, in addition to finding
	real bugs as before. The novelties of our verification approach are
	in a) combining EMM with proof-based abstraction that preserves the
	correctness of a property up to a certain analysis depth of {SAT}-based
	BMC, and b) modeling arbitrary initial memory state precisely and
	thereby, providing inductive proofs using {SAT}-based BMC for embedded
	memory systems. Similar to the previous approach, we construct a
	verification model by eliminating memory arrays, but retaining the
	memory interface signals with their control logic and adding constraints
	on those signals at every analysis depth to preserve the data forwarding
	semantics. The size of these EMM constraints depends quadratically
	on the number of memory accesses and the number of read and write
	ports; and linearly on the address and data widths and the number
	of memories. We show the effectiveness of our approach on several
	industry designs and software programs.},
  file = {:./files/2005a-GanaiGupta.etal.pdf:PDF},
  owner = {nguyen},
  timestamp = {2006.09.08}
}

@INPROCEEDINGS{2004a-GanaiGupta.etal,
  author = {Malay K. Ganai and Aarti Gupta and Pranav Ashar},
  title = {Efficient Modeling of Embedded Memories in Bounded Model Checking.},
  booktitle = {Proc. International Conference on Computer Aided Verification (CAV)},
  year = {2004},
  volume = {3114},
  number = {3-540-22342-8},
  series = {Lecture Notes in Computer Science},
  pages = {440-452},
  publisher = {Springer},
  abstract = {Abstract. We describe a viable approach for memory abstraction that
	preserves memory semantics, thereby augmenting the capability of
	{SAT}-based {BMC} to handle designs with large embedded memory without
	explicitly modeling each memory bit. Our method does not require
	examining the design or changing the {SAT} solver and is guaranteed
	not to generate false negatives. The proposed method is similar,
	but with key enhancements, to the previous abstract interpretation
	of memory that captures its forwarding semantics, i.e., a data read
	from a memory location is same as the most recent data written at
	the same location. In our method, we construct an abstract model
	for BMC by eliminating memory arrays, but retaining the memory interface
	signals and adding constraints on those signals at every analysis
	depth to preserve the memory semantics. The size of these memory-modeling
	constraints depends quadratically on the number of memory accesses
	and linearly on the bus widths of memory interface signals. Since
	the analysis depth of BMC bounds the number of memory accesses, these
	constraints are significantly smaller than the explicit memory model.
	The novelty of our memory-modeling constraints is that they capture
	the exclusivity of a read and write pair explicitly, i.e., when a
	{SAT} solver decides on a valid read and write pair, other pairs
	are implied invalid immediately, thereby reducing the solve time.
	We have implemented these techniques in our {SAT}-based BMC framework
	where we demonstrate the effectiveness of such an abstraction on
	a number of hardware and software designs with large embedded memories.
	We show at least an order of magnitude improvement (both in time
	and space) using our method over explicit modeling of each memory
	bit. We also show that our method of adding constraints boosts the
	performance of the SAT solver (in BMC) significantly as opposed to
	the conventional way of modeling these constraints as nested if-then-else
	expressions.},
  ee = {http://springerlink.metapress.com/openurl.asp?genre=article{\&}issn=0302-9743{\&}volume=3114{\&}spage=440},
  file = {:./files/2004a-GanaiGupta.etal.pdf:PDF},
  keywords = {BMC, Modeling, Embedded, Memory},
  owner = {nguyen},
  timestamp = {2006.09.08},
  url = {http://springerlink.metapress.com/openurl.asp?genre=article{\&}issn=0302-9743{\&}volume=3114{\&}spage=440}
}

@INPROCEEDINGS{2004-GanaiGupta.etal,
  author = {M. K. Ganai and A. Gupta and P. Ashar},
  title = {Efficient {SAT}-based unbounded symbolic model checking using circuit
	cofactoring},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2004},
  pages = {510--517},
  address = {Washington, DC, USA},
  publisher = {IEEE Computer Society},
  file = {:./files/2004-GanaiGupta.etal.pdf:PDF},
  isbn = {0-7803-8702-3},
  owner = {wedler},
  timestamp = {2008.04.21}
}

@INPROCEEDINGS{2002-GaneshBerezin.etal,
  author = {Vijay Ganesh and Sergey Berezin and David L. Dill},
  title = {Deciding Presburger Arithmetic by Model Checking and Comparisons
	with Other Methods},
  booktitle = {Proc. International Conference on Formal Methods in Computer-Aided
	Design ({FMCAD})},
  year = {2002},
  pages = {171--186},
  address = {London, UK, UK},
  publisher = {Springer-Verlag},
  acmid = {683249},
  file = {:./files/2002-GaneshBerezin.etal.pdf:PDF},
  isbn = {3-540-00116-6},
  numpages = {16},
  timestamp = {2006.09.21}
}

@INPROCEEDINGS{2007-GaneshDill,
  author = {Vijay Ganesh and David L. Dill},
  title = {A decision procedure for bit-vectors and arrays},
  booktitle = {Proceedings of the Computer Aided Verification Conference},
  year = {2007},
  pages = {524--536},
  publisher = {Springer},
  file = {:./files/2007-GaneshDill.pdf:PDF},
  owner = {pavlenko},
  timestamp = {2010.07.26}
}

@INPROCEEDINGS{2004-GanzingerHagen.etal,
  author = {H. Ganzinger and G. Hagen and R. Nieuwenhuis and A. Oliveras and
	C. Tinelli},
  title = {{DPLL(T)}: Fast Decision Procedures},
  booktitle = {Proc. International Conference on Computer Aided Verification ({CAV})},
  year = {2004},
  pages = {26-37},
  month = {July},
  file = {:./files/2004-GanzingerHagen.etal.pdf:PDF}
}

@BOOK{1979-GareyJohnson,
  title = {Computers and Intractability: A Guide to the Theory of {NP}-Completeness},
  publisher = {W.H. Freeman and Company},
  year = {1979},
  author = {Michael R. Garey and David S. Johnson},
  address = {New York}
}

@INPROCEEDINGS{2005-Gascard,
  author = {Gascard, E.},
  title = {From Sequential Extended Regular Expressions to Determinstic Finite
	Automata},
  booktitle = {Information and Communications Technology, 2005. Enabling Technologies
	for the New Knowledge Society: {ITI} 3rd International Conference
	on},
  year = {2005},
  pages = {145 -157},
  month = {dec.},
  file = {:./files/2005-Gascard.pdf:PDF},
  keywords = {PSL SERE assertion;VHDL description;deterministic finite automata;property
	specification language;sequential extended regular expressions assertions;deterministic
	automata;finite automata;formal specification;formal verification;hardware
	description languages;},
  timestamp = {2006.09.21}
}

@ARTICLE{2016-GeYarom.etal,
  author = {Ge, Qian and Yarom, Yuval and Cock, David and Heiser, Gernot},
  title = {A survey of microarchitectural timing attacks and countermeasures
	on contemporary hardware},
  journal = {Journal of Cryptographic Engineering},
  year = {2016},
  volume = {8},
  pages = {1-27},
  month = {10},
  publisher = {Springer}
}

@INPROCEEDINGS{1994-GeistBeer,
  author = {Daniel Geist and Ilan Beer},
  title = {Efficient Model Checking by Automated Ordering of Transition Relation
	Partitions},
  booktitle = {Proc. International Conference on Computer Aided Verification ({CAV})},
  year = {1994},
  pages = {299--310},
  publisher = {Springer-Verlag},
  file = {:./files/1994-GeistBeer.pdf:PDF},
  isbn = {3-540-58179-0}
}

@TECHREPORT{1996-GeistLandver.etal,
  author = {Daniel Geist and Avner Landver and Bruce W. Singer},
  title = {Formal Verification of a Processor's Bus Interface Unit},
  institution = {{IBM} Research},
  year = {1996},
  note = {Case studies},
  file = {:./files/1996-GeistLandver.etal.pdf:PDF},
  owner = {nguyen},
  timestamp = {2007.02.02}
}

@INPROCEEDINGS{2008-Gelder,
  author = {Allen Van Gelder},
  title = {Verifying RUP Proofs of Propositional Unsatisfiability},
  booktitle = {ISAIM},
  year = {2008},
  file = {:./files/2008-Gelder.pdf:PDF},
  owner = {marx},
  timestamp = {2012.11.09}
}

@INPROCEEDINGS{2017-Genius,
  author = {Genius, Daniela and Li, Letitia and Apvrille, Ludovic},
  title = {Model-driven Performance Evaluation and Formal Verification for Multi-level
	Embedded System Design},
  booktitle = {5th International Conference on Model-Driven Engineering and Software
	Development (MODELSWARD 2017)},
  year = {2017},
  owner = {fehmel},
  timestamp = {2019.07.04}
}

@ARTICLE{2003-GentiliniPiazza.etal,
  author = {Raffaella Gentilini and Carla Piazza and Alberto Policriti},
  title = {From Bisimulation to Simulation: Coarsest Partition Problems},
  journal = {J. Autom. Reasoning},
  year = {2003},
  volume = {31},
  pages = {73-103},
  number = {1},
  owner = {stoffel},
  timestamp = {2016.05.10}
}

@ARTICLE{1999-GiraultLee.etal,
  author = {Alain Girault and Bilung Lee and Edward a. Lee},
  title = {Hierarchical Finite State Machines with Multiple Concurrency Models},
  journal = {{IEEE} Transaction on Computer-Aided Design},
  year = {1999},
  volume = {18, No 6},
  pages = {742 - 760},
  file = {:./files/1999-GiraultLee.etal.pdf:PDF},
  owner = {thalmaier},
  timestamp = {2006.08.28}
}

@BOOK{2004-GloeklerMeyr,
  title = {Design of Energy-Efficient Application-Specific Instruction Set Processors
	({ASIP}s)},
  publisher = {Kluwer Academic Publishers},
  year = {2004},
  author = {Tilman Gl\"{o}kler and Heinrich Meyr},
  owner = {loitz},
  timestamp = {2007.01.08}
}

@ARTICLE{1997a-GloverLaguna,
  author = {Fred Glover and Manuel Laguna},
  title = {General Purpose Heuristics for Integer Programming - Part {I}},
  journal = {Journal of Heuristics},
  year = {1997},
  volume = {2},
  pages = {343-358},
  number = {2},
  month = dec,
  acmid = {594966},
  address = {Hingham, MA, USA},
  file = {:./files/1997a-GloverLaguna.pdf:PDF},
  issn = {1381-1231},
  issue = {4},
  keywords = {integer programming; branch and cut; cut search; ray probing},
  language = {English},
  numpages = {19},
  publisher = {Kluwer Academic Publishers}
}

@BOOK{1997-GloverLaguna,
  title = {Tabu Search},
  publisher = {Kluwer Academic Publisher},
  year = {1997},
  author = {Fred Glover and Manuel Laguna},
  address = {Boston, Dordrecht, London}
}

@INCOLLECTION{2000-GloverLokketangen.etal,
  author = {Fred Glover and Arne Loekketangen and David L. Woodruff},
  title = {Scatter Search to Generate Diverse {MIP} Solutions},
  booktitle = {Computing Tools for Modeling, Optimization and Simulation: Interfaces
	in Computer Science and Operations Research},
  publisher = {Kluwer Academic Publishers},
  year = {2000},
  editor = {M. Laguna and J. L. Gonz{\'a}lez-Velarde},
  pages = {299-317},
  file = {:./files/2000-GloverLokketangen.etal.pdf:PDF}
}

@ARTICLE{2017-GluzerWimer,
  author = {D. Gluzer and S. Wimer},
  title = {Probability-Driven Multibit Flip-Flop Integration With Clock Gating},
  journal = {IEEE Transactions on Very Large Scale Integration (VLSI) Systems},
  year = {2017},
  volume = {25},
  pages = {1173-1177},
  file = {:files/2017-GluzerWimer.pdf:PDF},
  issn = {1063-8210}
}

@INCOLLECTION{1997-Godefroid,
  author = {Godefroid, Patrice},
  title = {VeriSoft: A tool for the automatic analysis of concurrent reactive
	software},
  booktitle = {Computer Aided Verification},
  publisher = {Springer Berlin / Heidelberg},
  year = {1997},
  editor = {Grumberg, Orna},
  volume = {1254},
  series = {Lecture Notes in Computer Science},
  pages = {476-479},
  affiliation = {Lucent Technologies Bell Laboratories 1000 E. Warrenville Road 60566
	Naperville IL USA 1000 E. Warrenville Road 60566 Naperville IL USA},
  file = {:./files/1997-Godefroid.pdf:PDF},
  isbn = {978-3-540-63166-8},
  keyword = {Computer Science}
}

@ARTICLE{2005-Godefroid,
  author = {Patrice Godefroid},
  title = {Software Model Checking The Verisoft Approach},
  journal = {Formal Methods in System Design, 2005},
  year = {2005},
  volume = {26},
  pages = {77 - 101},
  file = {:./files/2005-Godefroid.pdf:PDF},
  timestamp = {2006.09.22}
}

@INPROCEEDINGS{1997a-Godefroid,
  author = {Godefroid, Patrice},
  title = {Model Checking for Programming Languages Using {VeriSoft}},
  booktitle = {Proceedings of the 24th ACM SIGPLAN-SIGACT Symposium on Principles
	of Programming Languages},
  year = {1997},
  series = {POPL-97},
  pages = {174--186},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {263717},
  file = {:import/var/jabref/files/1997a-Godefroid.pdf:PDF},
  isbn = {0-89791-853-3},
  location = {Paris, France},
  numpages = {13}
}

@INCOLLECTION{2005-GodefroidKlarlund,
  author = {Godefroid, Patrice and Klarlund, Nils},
  title = {Software Model Checking: Searching for Computations in the Abstract
	or the Concrete},
  booktitle = {Integrated Formal Methods},
  publisher = {Springer Berlin / Heidelberg},
  year = {2005},
  editor = {Romijn, Judi and Smith, Graeme and van de Pol, Jaco},
  volume = {3771},
  series = {Lecture Notes in Computer Science},
  pages = {20-32},
  note = {10.1007/11589976_3},
  affiliation = {Bell Laboratories, Lucent Technologies},
  file = {:./files/2005-GodefroidKlarlund.pdf:PDF},
  isbn = {978-3-540-30492-0},
  keyword = {Computer Science}
}

@ARTICLE{2005-GodefroidKarlund.etal,
  author = {Godefroid, Patrice and Klarlund, Nils and Sen, Koushik},
  title = {{DART: Directed Automated Random Testing}},
  journal = {SIGPLAN Not.},
  year = {2005},
  volume = {40},
  pages = {213--223},
  number = {6},
  month = jun,
  acmid = {1065036},
  address = {New York, NY, USA},
  issn = {0362-1340},
  issue_date = {June 2005},
  keywords = {automated test generation, interfaces, program verification, random
	testing, software testing},
  numpages = {11},
  owner = {villarraga},
  publisher = {ACM},
  timestamp = {2016.07.19}
}

@INBOOK{2003-Goldberg,
  chapter = {Computer Arithmetic},
  pages = {H-1-H-74},
  title = {Computer Architecture A Quantitative Approach},
  publisher = {Morgan Kaufmann},
  year = {2003},
  editor = {3rd},
  author = {David Goldberg},
  file = {:./files/2003-Goldberg.pdf:PDF},
  owner = {loitz},
  timestamp = {2007.01.08}
}

@ARTICLE{1991-Goldberg,
  author = {David Goldberg},
  title = {What Every Computer Scientist Should Know About Floating-Point Arithmetic},
  journal = {{ACM} Computing Surveys},
  year = {1991},
  volume = {23},
  pages = {5--48},
  file = {:./files/1991-Goldberg.pdf:PDF},
  owner = {loitz},
  timestamp = {2007.01.08}
}

@INPROCEEDINGS{2002-GoldbergNovikov,
  author = {E. Goldberg and Y. Novikov},
  title = {BerkMin: A Fast and Robust {SAT} Solver},
  booktitle = {Proc. International Conference on Design, Automation and Test in
	Europe ({DATE})},
  year = {2002},
  pages = {142-149},
  file = {:./files/2002-GoldbergNovikov.pdf:PDF},
  url = {citeseer.ist.psu.edu/goldberg02berkmin.html}
}

@INPROCEEDINGS{2003-GoloubevaRebaudengo.etal,
  author = {O. Goloubeva and M. Rebaudengo and M. Sonza Reorda and M. Violante},
  title = {Soft-error detection using control flow assertions},
  booktitle = {18th IEEE International Symposium on Defect and Fault Tolerance in
	VLSI Systems},
  year = {2003},
  pages = {581-588},
  month = {November},
  file = {2003-GoloubevaRebaudengo.etal.pdf:files/2003-GoloubevaRebaudengo.etal.pdf:PDF},
  issn = {1550-5774},
  owner = {bartsch},
  timestamp = {2016.09.21}
}

@INPROCEEDINGS{1963-Gomory,
  author = {Ralph E. Gomory},
  title = {An Algorithm for Integer Solutions to Linear Programming},
  booktitle = {Recent Advances in Mathematical Programming},
  year = {1963},
  editor = {R.L. Graves and P. Wolfe},
  pages = {269-302},
  address = {New York},
  publisher = {McGraw-Hill},
  file = {:./files/1963-Gomory.pdf:PDF}
}

@INPROCEEDINGS{2007-Gonthier,
  author = {Georges Gonthier},
  title = {{The Four Colour Theorem: Engineering of a Formal Proof}},
  booktitle = {Computer Mathematics, 8th Asian Symposium, {ASCM}, Singapore, December
	15-17, 2007. Revised and Invited Papers},
  year = {2007},
  owner = {stoffel},
  timestamp = {2016.05.10}
}

@ARTICLE{2000-Gonzalez,
  author = {Ricardo E. Gonzalez},
  title = {{Xtensa} --- {A} Configurable and Extensible Processor},
  journal = {{IEEE} Micro},
  year = {2000},
  volume = {20},
  pages = {60--70},
  number = {2},
  file = {:./files/2000-Gonzalez.pdf:PDF},
  owner = {loitz},
  timestamp = {2007.01.08}
}

@PROCEEDINGS{2006-GopalakrishnanOLeary,
  title = {Multithreading in Hardware and Software: Formal Approaches to Design
	and Verification},
  year = {2006},
  author = {Ganesh Gopalakrishnan and John O'Leary},
  file = {:./files/2006-GopalakrishnanOLeary.pdf:PDF},
  timestamp = {2006.09.21}
}

@INPROCEEDINGS{1999-GovindarajuDill.etal,
  author = {Shankar G. Govindaraju and David L. Dill and Jules P. Bergmann},
  title = {Improved Approximate Reachability Using Auxiliary State Variables},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {1999},
  pages = {312-316},
  file = {:./files/1999-GovindarajuDill.etal.pdf:PDF},
  url = {citeseer.ist.psu.edu/govindaraju99improved.html}
}

@INPROCEEDINGS{1998-GovindarajuDill.etal,
  author = {Shankar G. Govindaraju and David L. Dill and Alan J. Hu and Mark
	A. Horowitz},
  title = {Approximate Reachability with {BDDs} Using Overlapping Projections},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {1998},
  pages = {451-456},
  file = {:./files/1998-GovindarajuDill.etal.pdf:PDF}
}

@ARTICLE{2014-Gracia-MoranBaraza-Calvo.etal,
  author = {J. Gracia-Moran and J.C. Baraza-Calvo and D. Gil-Tomas and L.J. Saiz-Adalid
	and P.J. Gil-Vicente},
  title = {Effects of Intermittent Faults on the Reliability of a Reduced Instruction
	Set Computing ({RISC}) Microprocessor},
  journal = {IEEE Transactions on Reliability},
  year = {2014},
  volume = {63},
  pages = {144-153},
  number = {1},
  month = {March},
  file = {2014-Gracia-MoranBaraza-Calvo.etal.pdf:files/2014-Gracia-MoranBaraza-Calvo.etal.pdf:PDF},
  issn = {0018-9529},
  owner = {bartsch},
  timestamp = {2015.08.03}
}

@INPROCEEDINGS{1997-GrafSaidi,
  author = {Susanne Graf and Hassen Sa\"{\i}di},
  title = {Construction of Abstract State Graphs with {PVS}},
  booktitle = {Proc. International Conference Computer Aided Verification ({CAV})},
  year = {1997},
  volume = {1254},
  series = {LNCS},
  pages = {72--83},
  address = {London, UK},
  publisher = {Springer-Verlag},
  file = {:./files/1997-GrafSaidi.pdf:PDF},
  isbn = {3-540-63166-6},
  owner = {nguyen},
  timestamp = {2008.06.03},
  url = {http://portal.acm.org/citation.cfm?id=647766.733618\&coll=GUIDE\&dl=GUIDE}
}

@BOOK{1994-GrahamKnuth.etal,
  title = {Concrete Mathematics, Second Edition},
  publisher = {Addison-Wesley},
  year = {1994},
  author = {R. L. Graham and D. E. Knuth and O. Patashni},
  file = {:./files/1994-GrahamKnuth.etal.pdf:PDF}
}

@MISC{web-graphviz,
  author = {{Graphviz}},
  title = {Graph Visualization Softwarediepen},
  howpublished = {https://www.graphviz.org/},
  key = {graphviz},
  owner = {ludwig},
  timestamp = {2018.01.11}
}

@BOOK{1996-GrassmannTremblay,
  title = {Logic and Discrete Mathematics},
  publisher = {Prentice Hall},
  year = {1996},
  author = {W. K. Grassmann and J.-P. Tremblay}
}

@BOOK{2007-GreuelPfister,
  title = {A {SINGULAR} Introduction to Commutative Algebra},
  publisher = {Springer Verlag},
  year = {2007},
  author = {G.-M. Greuel and G. Pfister},
  address = {Berlin, Heidelberg, New York},
  edition = {2nd},
  note = {705 pages},
  file = {:./files/2007-GreuelPfister.pdf:PDF},
  owner = {wedler},
  timestamp = {2008.01.21}
}

@MISC{1990-GreuelPfister.etal,
  author = {G.-M. Greuel and G. Pfister and H. Sch\"{o}nemann},
  title = {{SINGULAR} - A Computer Algebra System for Polynomial Computations},
  year = {1990},
  note = {Free software under the GNU General Public License (1990 - to date)},
  owner = {stoffel},
  timestamp = {2016.05.11},
  url = {http://www.singular.uni-kl.de/}
}

@ARTICLE{2007-GreuelSeelisch.etal,
  author = {G.~-M. Greuel and F. Seelisch and O. Wienand},
  title = {The {Gr\"obner} basis of the ideal of vanishing polynomials},
  journal = {Journal of Symbolic Computation},
  year = {2007},
  pages = {14},
  file = {:./files/2007-GreuelSeelisch.etal.pdf:PDF},
  owner = {wedler},
  timestamp = {2008.01.21},
  url = {http://www.citebase.org/abstract?id=oai:arXiv.org:0709.2978}
}

@INPROCEEDINGS{2002-GrieskampGurevich.etal,
  author = {Grieskamp, Wolfgang and Gurevich, Yuri and Schulte, Wolfram and Veanes,
	Margus},
  title = {Generating Finite State Machines from Abstract State Machines},
  booktitle = {Proceedings of the 2002 ACM SIGSOFT International Symposium on Software
	Testing and Analysis},
  year = {2002},
  owner = {fehmel},
  timestamp = {2019.05.27}
}

@INPROCEEDINGS{2005-Grimm,
  author = {Klaus Grimm},
  title = {Anforderungen an das Software-Engineering aus der Sicht der Automobilindustrie},
  booktitle = {ASIM-STS-Fachgruppentreffen 2005, Simulations- und Testmethoden f�r
	Software in Fahrzeugsystemen},
  year = {2005},
  file = {:import/var/jabref/files/2005-Grimm.pdf:PDF},
  owner = {bschmidt},
  timestamp = {2014.06.27}
}

@INPROCEEDINGS{2012-GrinschglKrieg.etal,
  author = {J. Grinschgl and A. Krieg and C. Steger and R. Weiss and H. Bock
	and J. Haid},
  title = {Efficient fault emulation based on post-injection fault effect analysis
	(PIFEA)},
  booktitle = {IEEE 55th International Midwest Symposium on Circuits and Systems
	(MWSCAS)},
  year = {2012},
  pages = {526-529},
  month = {Aug},
  file = {2012-GrinschglKrieg.etal.pdf:files/2012-GrinschglKrieg.etal.pdf:PDF},
  issn = {1548-3746},
  owner = {bartsch},
  timestamp = {2016.11.30}
}

@INPROCEEDINGS{2006-GrosseKuehne.etal,
  author = {Gro{\ss}e, Daniel and K\"{u}hne, Ulrich and Drechsler, Rolf},
  title = {{HW/SW} co-verification of embedded systems using bounded model checking},
  booktitle = {{GLSVLSI} '06: Proceedings of the 16th {ACM} Great Lakes symposium
	on {VLSI}},
  year = {2006},
  pages = {43--48},
  file = {:./files/2006-GrosseKuehne.etal.pdf:PDF},
  owner = {stoffel},
  timestamp = {2010.10.29}
}

@INPROCEEDINGS{2010-GrosseLe.etal,
  author = {Daniel Gro{\ss}e and Hoang M. Le and Rolf Drechsler},
  title = {Proving transaction and system-level properties of untimed {SystemC}
	{TLM} designs},
  booktitle = {Proc. {ACM}/{IEEE} International Conference on Formal Methods and
	Models for Codesign ({MEMOCODE})},
  year = {2010},
  pages = {113-122},
  file = {:./files/2010-GrosseLe.etal.pdf:PDF}
}

@ARTICLE{1989-GroetschelJuenger.etal,
  author = {Martin Groetschel and Michael Juenger and Gerd Reinelt},
  title = {Via Minimization with Pin Preassignments and Layer Preference},
  journal = {{ZAMM} - Zeitschrift fuer Angewandte Mathematik und Mechanik},
  year = {1989},
  volume = {69},
  pages = {393-399},
  number = {11},
  classmath = {*05C35 05C10 90C35 94C15 05C85},
  file = {:./files/1989-GroetschelJuenger.etal.pdf:PDF},
  language = {English}
}

@ARTICLE{1997-GroetschelMartin.etal,
  author = {Martin Groetschel and Alexander Martin and Robert Weismantel},
  title = {The Steiner Tree Packing Problem in {VLSI} Design},
  journal = {Mathematical Programming},
  year = {1997},
  volume = {78},
  pages = {265-281},
  number = {2},
  classmath = {*90C35 05C70},
  file = {:./files/1997-GroetschelMartin.etal.pdf:PDF},
  language = {English}
}

@ARTICLE{1979a-GroetschelPadberg,
  author = {Martin Groetschel and Manfred W. Padberg},
  title = {On the Symmetric Traveling Salesman Problem {I}: Inequalities},
  journal = {Mathematical Programming},
  year = {1979},
  volume = {16},
  pages = {265-280},
  file = {:./files/1979a-GroetschelPadberg.pdf:PDF}
}

@INPROCEEDINGS{2007-GrosseKuehne.etal,
  author = {Grosse, Daniel and K\"{u}hne, Ulrich and Drechsler, Rolf},
  title = {Estimating functional coverage in bounded model checking},
  booktitle = {Proc. International Conference on Design, Automation and Test in
	Europe ({DATE})},
  year = {2007},
  pages = {1176--1181},
  file = {:./files/2007-GrosseKuehne.etal.pdf:PDF},
  isbn = {978-3-9810801-2-4},
  location = {Nice, France},
  owner = {wedler},
  timestamp = {2010.01.11}
}

@ARTICLE{1996-GroetschelMartin.etal,
  author = {Martin Grotschel and Alexander Martin and Robert Weismantel},
  title = {Packing Steiner Trees: a Cutting Plane Algorithm and Computational
	Results},
  journal = {Mathematical Programming},
  year = {1996},
  volume = {72},
  pages = {125-145},
  number = {2},
  classmath = {*90C35 52B12},
  file = {:./files/1996-GroetschelMartin.etal.pdf:PDF},
  language = {English}
}

@ARTICLE{1995-GroetschelMartin,
  author = {Martin Grotschel and Alexander Martin and Robert Weismantel},
  title = {Routing in Grid Graphs by Cutting Planes},
  journal = {ZOR - Mathematical Methods of Operations Research},
  year = {1995},
  volume = {41},
  pages = {255-275},
  number = {3},
  classmath = {*90C35},
  file = {:./files/1995-GroetschelMartin.pdf:PDF},
  language = {English}
}

@INBOOK{2004-GrumbergSchuster.etal,
  chapter = {Memory Efficient All-Solutions SAT Solver and Its Application for
	Reachability Analysis},
  pages = {275--289},
  title = {Formal Methods in Computer-Aided Design: 5th International Conference,
	FMCAD 2004, Austin, Texas, USA, November 15-17, 2004. Proceedings},
  publisher = {Springer Berlin Heidelberg},
  year = {2004},
  author = {Grumberg, Orna and Schuster, Assaf and Yadgar, Avi},
  address = {Berlin, Heidelberg},
  booktitle = {Formal Methods in Computer-Aided Design: 5th International Conference,
	FMCAD 2004, Austin, Texas, USA, November 15-17, 2004. Proceedings},
  isbn = {978-3-540-30494-4},
  owner = {villarraga},
  timestamp = {2016.07.28}
}

@INPROCEEDINGS{2013-Grundy,
  author = {Jim Grundy},
  title = {Firmware validation: challenges and opportunities},
  booktitle = {Formal Methods in Computer-Aided Design, {FMCAD} 2013, Portland,
	OR, USA, October 20-23, 2013},
  year = {2013},
  pages = {11},
  bibsource = {dblp computer science bibliography, http://dblp.org},
  biburl = {http://dblp.uni-trier.de/rec/bib/conf/fmcad/Grundy13},
  file = {2013-Grundy.pdf:files/2013-Grundy.pdf:PDF},
  owner = {villarraga},
  timestamp = {Wed, 25 Feb 2015 15:27:31 +0100}
}

@BOOK{2002-GroetkerLiao.etal,
  title = {System design with SystemC},
  publisher = {Kluwer Academic Publishers},
  year = {2002},
  author = {T. Gr�tker and S. Liao and G. Martin and S. Swan},
  owner = {W},
  timestamp = {2010.09.21}
}

@ARTICLE{2013-GubbiBuyya.etal,
  author = {Jayavardhana Gubbi and Rajkumar Buyya and Slaven Marusic and Marimuthu
	Palaniswami},
  title = {Internet of Things (IoT): A vision, architectural elements, and future
	directions },
  journal = {Future Generation Computer Systems },
  year = {2013},
  volume = {29},
  pages = {1645 - 1660},
  number = {7},
  note = {Including Special sections: Cyber-enabled Distributed Computing for
	Ubiquitous Cloud and Network Services \&amp; Cloud Computing and
	Scientific Applications — Big Data, Scalable Analytics, and Beyond
	},
  abstract = {Abstract Ubiquitous sensing enabled by Wireless Sensor Network (WSN)
	technologies cuts across many areas of modern day living. This offers
	the ability to measure, infer and understand environmental indicators,
	from delicate ecologies and natural resources to urban environments.
	The proliferation of these devices in a communicating–actuating network
	creates the Internet of Things (IoT), wherein sensors and actuators
	blend seamlessly with the environment around us, and the information
	is shared across platforms in order to develop a common operating
	picture (COP). Fueled by the recent adaptation of a variety of enabling
	wireless technologies such as \{RFID\} tags and embedded sensor and
	actuator nodes, the IoT has stepped out of its infancy and is the
	next revolutionary technology in transforming the Internet into a
	fully integrated Future Internet. As we move from www (static pages
	web) to web2 (social networking web) to web3 (ubiquitous computing
	web), the need for data-on-demand using sophisticated intuitive queries
	increases significantly. This paper presents a Cloud centric vision
	for worldwide implementation of Internet of Things. The key enabling
	technologies and application domains that are likely to drive IoT
	research in the near future are discussed. A Cloud implementation
	using Aneka, which is based on interaction of private and public
	Clouds is presented. We conclude our IoT vision by expanding on the
	need for convergence of WSN, the Internet and distributed computing
	directed at technological research community. },
  file = {2013-GubbiBuyya.etal.pdf:files/2013-GubbiBuyya.etal.pdf:PDF},
  issn = {0167-739X},
  keywords = {Internet of Things},
  owner = {schwarz},
  timestamp = {2017.01.09},
  url = {http://www.sciencedirect.com/science/article/pii/S0167739X13000241}
}

@INPROCEEDINGS{2011-GullaschBangerter.etal,
  author = {Gullasch, David and Bangerter, Endre and Krenn, Stephan},
  title = {Cache games--Bringing access-based cache attacks on {AES} to practice},
  booktitle = {IEEE Symposium on Security and Privacy (SP) },
  year = {2011},
  pages = {490--505},
  organization = {IEEE},
  owner = {fadiheh},
  timestamp = {2018.07.12}
}

@INPROCEEDINGS{2003a-GuptaGanai.etal,
  author = {Aarti Gupta and Malay Ganai and Chao Wang and Zijiang Yang and Pranav
	Ashar},
  title = {Abstraction and {BDD}s Complement {SAT}-based {BMC} in {DiVer}},
  booktitle = {Proc. of the 15th Conf. on Computer-Aided Verification},
  year = {2003},
  pages = {206--209},
  publisher = {Springer},
  file = {:./files/2003a-GuptaGanai.etal.pdf:PDF},
  timestamp = {2006.09.19}
}

@INPROCEEDINGS{2003-GuptaGanai.etal,
  author = {Aarti Gupta and Malay Ganai and Zijiang Yang and Pranav Ashar},
  title = {Iterative Abstraction using {SAT}-based {BMC} with Proof Analysis},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2003},
  pages = {416},
  address = {Washington, DC, USA},
  publisher = {IEEE Computer Society},
  file = {:./files/2003-GuptaGanai.etal.pdf:PDF},
  isbn = {1-58113-762-1},
  owner = {nguyen},
  timestamp = {2007.04.12}
}

@INPROCEEDINGS{2005-GuptaSelvidge,
  author = {Amit Gupta and Charley Selvidge},
  title = {Acyclic Modeling of Combinational Loops},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2005},
  pages = { 343 - 347},
  file = {:./files/2005-GuptaSelvidge.pdf:PDF},
  keywords = { acyclic circuit; acyclic combinational logic; acyclic model; automated
	synthesis-compiler; equivalent circuit; feedback logic; feedback
	path; gate-level combinational loop; gate-level designs; latch behavior;
	level sensitive latch; loop conversion; nonoscillatory loops; replacement
	circuit; circuit feedback; combinational circuits; equivalent circuits;
	flip-flops; integrated circuit design; integrated circuit modelling;
	logic design;},
  timestamp = {2006.09.27}
}

@INPROCEEDINGS{2001-GuptaYang.etal,
  author = {Aarti Gupta and Zijiang Yang and Pranav Ashar and Lintao Zhang and
	Sharad Malik},
  title = {Partition-Based Decision Heuristics for Image Computation using {BDD}
	and {SAT}},
  booktitle = {Proc. International Conference on Computer-Aided Design (ICCAD)},
  year = {2001},
  pages = {286 -292},
  file = {:./files/2001-GuptaYang.etal.pdf:PDF},
  keywords = {BDDs;{Boolean} satisfiability;CNF graph;SAT;benchmark sequential circuits;clause
	partitions;clause-variable dependency matrix;conjunctive normal form;decision
	heuristics;disjoint variable supports;hypergraph partitioning techniques;image
	computation;partition-based decision heuristics;partitioning information;reachability
	analysis;separator-set induced partitioning;{Boolean} functions;binary
	decision diagrams;computability;formal verification;graph theory;logic
	CAD;logic partitioning;reachability analysis;sequential circuits;},
  timestamp = {2006.09.13}
}

@INPROCEEDINGS{2001-GuentherHett.etal,
  author = {Wolfgang G�nther and Andreas Hett and Bernd Becker},
  title = {Application of Linearly Transformed {BDDs} in Sequential Verification},
  booktitle = {Proc. Asia and South Pacific Design Automation Conference, 2001},
  year = {2001},
  pages = {91 -96},
  file = {:./files/2001-GuentherHett.etal.pdf:PDF},
  keywords = {binary decision diagrams;computational power;dynamic reordering;linearly
	transformed BDDs;reachable states;relational product;sequential verification;sequential
	verification domain;binary decision diagrams;finite state machines;formal
	verification;logic CAD;reachability analysis;sequential circuits;},
  owner = {pavlenko},
  timestamp = {2011.06.03}
}

@INPROCEEDINGS{1994-ChaPatel,
  author = {H.Cha and H.Patel},
  title = {Latch Design for Transient Pulse Tolerance},
  booktitle = {Proc. {IEEE} International Conference on Computer Design: {VLSI}
	in Computer \& Processors},
  year = {1994},
  pages = {385 -388},
  file = {:./files/1994-ChaPatel.pdf:PDF},
  keywords = { ISCAS-89 benchmark circuits; VLSI circuits; direct hits; fault injection;
	high energy particles; latch design; memory elements; radiation hardening;
	transient pulse tolerance; transient pulses; VLSI; flip-flops; logic
	design; radiation hardening (electronics); transients;},
  timestamp = {2006.09.14}
}

@INPROCEEDINGS{2000-HsiehBalarin.etal,
  author = {H.Hsieh and F.Balarin and L.Lavagno},
  title = {Efficient Method For Embedded System Design Space Exploration},
  booktitle = {Proc. International Design Automation Conference (DAC)},
  year = {2000},
  pages = {607 -612},
  file = {:./files/2000-HsiehBalarin.etal.pdf:PDF},
  timestamp = {2006.09.27}
}

@ARTICLE{1999-SegerBryant,
  author = {Carl-Johan H.Seger and Randal E.Bryant},
  title = {Formal Verification By Symbolic Evaluation And Partially-Orderd Trajectories},
  journal = {Formal Methods in System Design},
  year = {1999},
  volume = {6},
  pages = {147 - 189},
  file = {:./files/1999-SegerBryant.pdf:PDF},
  timestamp = {2006.09.21}
}

@ARTICLE{2000-TheilingFedinand.etal,
  author = {H.Theiling and C.Fedinand and R.Welhelm},
  title = {Fast Precise {WCET} Prediction By Separate Cache Path Analyses},
  journal = {Real-Time Systems},
  year = {2000},
  volume = {18},
  pages = {157 - 179},
  file = {:./files/2000-TheilingFedinand.etal.pdf:PDF},
  timestamp = {2006.09.22}
}

@BOOK{2011-HaberleinTobias,
  title = {Technische Informatik - Ein Tutorium der Maschinenprogrammierung
	und Rechnertechnik},
  publisher = {Vieweg+Teubner},
  year = {2011},
  author = {Tobias H{\"a}berlein},
  owner = {bschmidt},
  timestamp = {2014.05.20}
}

@ARTICLE{1996-HachtelMacii.etal,
  author = {Gary D. Hachtel and Enrico Macii and Abelardo Pardo and Fabio Somenzi},
  title = {Markovian Analysis of Large Finite State Machines},
  journal = {{IEEE} Transactions on Computer-Aided Design},
  year = {1996},
  volume = {15},
  pages = {1479-1493},
  number = {12},
  month = {December},
  file = {:./files/1996-HachtelMacii.etal.pdf:PDF}
}

@INPROCEEDINGS{1994-HachtelMacii.etal,
  author = {Gary D. Hachtel and Enrico Macii and Abelardo Pardo and Fabio Somenzi},
  title = {Probabilistic Analysis of Large Finite State Machines},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {1994},
  pages = {270-275},
  file = {:./files/1994-HachtelMacii.etal.pdf:PDF}
}

@BOOK{1996-HachtelSomenzi,
  title = {Logic Synthesis and Verification Algorithms},
  publisher = {Kluwer Academic Publishers},
  year = {1996},
  author = {Gary D. Hachtel and Fabio Somenzi},
  address = {Boston}
}

@INPROCEEDINGS{2012-HaedickeGrosse.etal,
  author = {Finn Haedicke and Daniel Gro{\ss}e and Rolf Drechsler},
  title = {A guiding coverage metric for formal verification},
  booktitle = {DATE},
  year = {2012},
  pages = {617-622},
  owner = {bao},
  timestamp = {2012.11.08}
}

@PROCEEDINGS{2014-HajisheykhiEbnenasir.etal,
  title = {Evaluating the Effect of Faults in SystemC TLM Models Using UPPAAL},
  year = {2014},
  author = {Hajisheykhi, Reza and Ebnenasir, Ali and Kulkarni, Sandeep S.},
  booktitle = {Software Engineering and Formal Methods},
  isbn = {978-3-319-10431-7},
  owner = {udupi},
  pages = {175--189},
  timestamp = {2018.09.04}
}

@BOOK{1993-Halbwachs,
  title = {Synchronous Programming of Reactive Systems},
  publisher = {Kluwer Academic Publishers},
  year = {1993},
  author = {Nicolas Halbwachs},
  owner = {bartsch},
  timestamp = {2016.09.22}
}

@INPROCEEDINGS{1995-HamaguchiMorita.etal,
  author = {Kiyoharu Hamaguchi and Akihito Morita and Shuzo Yajima},
  title = {Efficient Construction of Binary Moment Diagrams for Verifying Arithmetic
	Circuits},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {1995},
  pages = {78-82},
  month = {November},
  file = {:./files/1995-HamaguchiMorita.etal.pdf:PDF}
}

@ARTICLE{2014-HanShin,
  author = {I. Han and Y. Shin},
  title = {Simplifying Clock Gating Logic by Matching Factored Forms},
  journal = {IEEE Transactions on Very Large Scale Integration (VLSI) Systems},
  year = {2014},
  volume = {22},
  pages = {1338-1349},
  number = {6},
  month = {June},
  file = {:files/2014-HanShin.pdf:PDF},
  issn = {1063-8210}
}

@INPROCEEDINGS{1995-HankataramanHartanto.etal,
  author = {S. Hankataraman and I. Hartanto and W. Kent Fuchs and E.M.Rudnick
	and S.Chakravarty and J.H.Patal},
  title = {Rapid Diagnostic Fault Simaulation of Stuck-at Faults in Sequential
	Circuits Using Compact Lists},
  year = {1995},
  pages = {133 -138},
  file = {:./files/1995-HankataramanHartanto.etal.pdf:PDF},
  timestamp = {2006.09.14}
}

@INPROCEEDINGS{2012-HaoRay.etal,
  author = {Hao, Kecheng and Ray, Sandip and Xie, Fei},
  title = {Equivalence checking for behaviorally synthesized pipelines},
  booktitle = {Proc. Design Automation Conference ({DAC})},
  year = {2012},
  pages = {344--349},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {2228423},
  file = {:files/2012-HaoRay.etal.pdf:PDF},
  keywords = {behavioral synthesis, equivalence checking, pipeline},
  location = {San Francisco, California},
  numpages = {6},
  owner = {joakim},
  timestamp = {2013.05.07}
}

@INPROCEEDINGS{2010-HaoXie.etal,
  author = {Hao, Kecheng and Xie, Fei and Ray, Sandip and Yang, Jin},
  title = {Optimizing equivalence checking for behavioral synthesis},
  booktitle = {Proc. Design, Automation and Test in Europe (DATE)},
  year = {2010},
  pages = {1500--1505},
  address = {Leuven, Belgium},
  acmid = {1871290},
  file = {:files/2010-HaoXie.etal.pdf:PDF},
  location = {Dresden, Germany},
  numpages = {6},
  owner = {joakim},
  timestamp = {2013.05.07}
}

@ARTICLE{1987-Harel,
  author = {David Harel},
  title = {Statecharts: A visual Formalism for Complex Systems},
  journal = {Science of Computer Programming},
  year = {1987},
  volume = {8},
  pages = {231--274},
  number = {3},
  month = {jun},
  acmid = {34886},
  address = {Amsterdam, The Netherlands, The Netherlands},
  file = {:./files/1987-Harel.pdf:PDF},
  issn = {0167-6423},
  numpages = {44},
  owner = {thalmaier},
  publisher = {Elsevier North-Holland, Inc.},
  timestamp = {2006.08.28}
}

@ARTICLE{2013-SastryAdve.etal,
  author = {S. K. Sastry Hari and S. V. Adve and H. Naeimi and P. Ramachandran},
  title = {Relyzer: Application Resiliency Analyzer for Transient Faults},
  journal = {IEEE Micro},
  year = {2013},
  volume = {33},
  pages = {58-66},
  number = {3},
  month = {May},
  file = {2013-SastryAdve.etal.pdf:files/2013-SastryAdve.etal.pdf:PDF},
  issn = {0272-1732},
  owner = {bartsch},
  timestamp = {2016.11.28}
}

@INPROCEEDINGS{2014-HariVenkatagiri.etal,
  author = {S. K. S. Hari and R. Venkatagiri and S. V. Adve and H. Naeimi},
  title = {{GangES}: Gang error simulation for hardware resiliency evaluation},
  booktitle = {ACM/IEEE 41st International Symposium on Computer Architecture (ISCA)},
  year = {2014},
  pages = {61-72},
  month = {June},
  file = {2014-HariVenkatagiri.etal.pdf:files/2014-HariVenkatagiri.etal.pdf:PDF},
  issn = {1063-6897},
  owner = {bartsch},
  timestamp = {2016.11.29}
}

@INPROCEEDINGS{2000-HarrisStokes.etal,
  author = {David Harris and Deverl Stokes and Russell Klein},
  title = {Executing an {RTOS} On Simulated Hardware Using Co-Verification},
  booktitle = {Embedded Systems Conference},
  year = {2000},
  file = {:./files/2000-HarrisStokes.etal.pdf:PDF},
  institution = {Mentor Graphics Embedded Systems Conference},
  timestamp = {2006.09.27}
}

@MISC{0000-Harris,
  author = {Laune Harris},
  title = {Analysis Of Stripped Binary Code},
  note = {Slides},
  file = {0000-Harris.ppt:files/0000-Harris.ppt:PowerPoint},
  owner = {nguyen},
  timestamp = {2007.02.02}
}

@BOOK{2009-Harrison,
  title = {Handbook of Practical Logic and Automated Reasoning},
  publisher = {Cambridge University Press},
  year = {2009},
  author = {Harrison, John},
  address = {New York, NY, USA},
  edition = {1st},
  isbn = {0521899575, 9780521899574},
  owner = {villarraga},
  timestamp = {2016.07.18}
}

@INPROCEEDINGS{2002a-HartongHedrich.etal,
  author = {Hartong, W. and Hedrich, L. and Barke, E.},
  title = {An Approach to Model Checking for Nonlinear Analog Systems},
  booktitle = {Design, Automation and Test in Europe Conference and Exhibition,
	2002. Proceedings},
  year = {2002},
  pages = {1080},
  file = {:./files/2002a-HartongHedrich.etal.pdf:PDF},
  keywords = {Schmitt trigger circuit;analog verification;digital CTL model checking;discrete
	model generation;hybrid model checking;model checking;nonlinear analog
	systems;nonlinear opamp model;second order lowpass filter;state space
	regions;tunnel diode oscillator circuit;analogue circuits;circuit
	testing;nonlinear network analysis;state-space methods;}
}

@INPROCEEDINGS{2002-HartongHedrich.etal,
  author = {W. Hartong and L. Hedrich and E. Barke},
  title = {On Discret Modeling and Model Checking for Nonlinear Analog Systems},
  booktitle = {Proc. International Conference on Computer Aided Verification ({CAV})},
  year = {2002},
  pages = {401--413},
  address = {London, UK, UK},
  publisher = {Springer-Verlag},
  acmid = {734409},
  file = {:./files/2002-HartongHedrich.etal.pdf:PDF},
  isbn = {3-540-43997-8},
  journal = {Conference on Computer-Aided Verification - CAV 2002},
  numpages = {13}
}

@ARTICLE{1995-HasanCiesielski,
  author = {Zafar Hasan and Maciej J. Ciesielski},
  title = {Decomposition \& Functional Verification of {FSM}s},
  journal = {{VLSI} Design: An International Journal of Custom-Chip Design, Simulation
	and Testing},
  year = {1995},
  citeseerurl = {53826.html},
  file = {:./files/1995-HasanCiesielski.pdf:PDF},
  howpublished = {VLSI Design: An International Journal of Custom-Chip Design, Simulation
	and Testing},
  owner = {thalmaier},
  timestamp = {2006.08.28}
}

@ARTICLE{1993-HaselhurstSeger,
  author = {Scott Haselhurst and Carl-John H.Seger},
  title = {A Simple Theorem Prover Based on Symbolic Trajectory Evaluation and
	{BDD}s},
  journal = {Computer-Aided Design of Integrated Circuits and Systems, IEEE Transactions
	on},
  year = {1993},
  volume = {14},
  pages = {413 -422},
  number = {4},
  month = {apr},
  file = {:./files/1993-HaselhurstSeger.pdf:PDF},
  keywords = {BDD;VLSI design;binary decision diagram;coherent system;data representation;design
	automation;formal hardware verification;partial verification results;symbolic
	trajectory evaluation;theorem prover;VLSI;circuit CAD;data structures;formal
	verification;inference mechanisms;integrated circuit design;theorem
	proving;},
  timestamp = {2006.09.21}
}

@PHDTHESIS{1998-Hasteer,
  author = {Gagan Hasteer},
  title = {Efficient Equivalence Checking In a Modular Design Environment},
  school = {University of Illinois at Urbana-Champaign},
  year = {1998},
  file = {:./files/1998-Hasteer.pdf:PDF},
  timestamp = {2006.09.13}
}

@ARTICLE{1998-HasteerMathur.etal,
  author = {Gagan Hasteer and Anmol Mathur and Prithviraj Banerjee},
  title = {Efficient Equivalence Checking of Multi-Phase Designs Using Phase
	Abstraction and Retiming},
  journal = {ACM Transactions on Design Automation of Electronic Systems ({TODAES})},
  year = {1998},
  volume = {3},
  pages = {600--625},
  number = {4},
  month = {oct},
  acmid = {296348},
  address = {New York, NY, USA},
  file = {Efficient equivalence checking of multi-phase designs using phase abstraction and retiming.pdf:Efficient equivalence checking of multi-phase designs using phase abstraction and retiming.pdf:PDF},
  issn = {1084-4309},
  keywords = {binary decision, diagram, encoding density, multi-phase FSM, product
	machine, sequential hardware equivalence, steady states},
  numpages = {26},
  publisher = {ACM},
  timestamp = {2006.09.13}
}

@BOOK{2010-HaubeltTeich,
  title = {{Digitale} Hardware/Software-{Systeme} Spezifikation und Verifikation},
  publisher = {Springer-Verlag Berlin Heidelberg},
  year = {2010},
  author = {Christian Haubelt and Juergen Teich},
  file = {Buch_als_PDF:files/2010-HaubeltTeich.pdf:PDF},
  owner = {bschmidt},
  timestamp = {2014.04.02}
}

@ARTICLE{2000-HavelPressburger,
  author = {Havelund, Klaus and Thomas Pressburger},
  title = {Model {C}hecking {J}ava {P}rograms {U}sing {J}ava {P}ath{F}inder},
  journal = {International Journal on Software Tools for Technology Transfer STTT},
  year = {2000},
  volume = {2},
  pages = {366-381},
  number = {4},
  file = {2000-HavelPressburger.pdf:files/2000-HavelPressburger.pdf:PDF},
  owner = {villarraga},
  timestamp = {2012.08.27}
}

@MISC{2002-HaverinenLeclercq.etal,
  author = {Anssi Haverinen and Maxime Leclercq and Drew Wingard and Norman Weyrich},
  title = {White Paper for SoC Communication Modeling},
  year = {2002},
  file = {:./files/2002-HaverinenLeclercq.etal.pdf:PDF},
  owner = {stoffel},
  timestamp = {2006.09.19}
}

@ARTICLE{2013-HazraMukher.etal,
  author = {Hazra, A. and Mukherjee, R. and Dasgupta, P. and Pal, A. and Harer,
	K.M. and Banerjee, A. and Mukherjee, S.},
  title = {POWER-TRUCTOR: An Integrated Tool Flow for Formal Verification and
	Coverage of Architectural Power Intent},
  journal = {Computer-Aided Design of Integrated Circuits and Systems, IEEE Transactions
	on},
  year = {2013},
  volume = {32},
  pages = {1801-1813},
  number = {11},
  month = {Nov},
  file = {2013-HazraMukher.etal.pdf:files/2013-HazraMukher.etal.pdf:PDF},
  issn = {0278-0070},
  keywords = {formal verification;hardware-software codesign;power system management;system-on-chip;POWER-TRUCTOR;coverage
	analysis;end-to-end automated framework;generic power management
	logics;global power management policies;local power controllers;on-chip
	architectural power management decisions;power intent verification;power
	requirements;system-on-chip designs;verification coverage;Computational
	modeling;Hardware;Hardware design languages;Integrated circuit modeling;Power
	control;Software;Timing;Assertion;coverage;formal verification;hardware/software
	co-verification;power intent verification},
  owner = {villarraga},
  timestamp = {2014.07.02}
}

@ARTICLE{1999-HeTurner,
  author = {Ji He and Kenneth J. Turner},
  title = {Protocol Inspired Hardware Testing},
  journal = {Communicating Systems XII},
  year = {1999},
  volume = {12},
  pages = {131-147},
  file = {:./files/1999-HeTurner.pdf:PDF},
  timestamp = {2006.09.19}
}

@INPROCEEDINGS{1996-HeinkelGlauert,
  author = {Ulrich Heinkel and Wolfram H. Glauert},
  title = {Method Towards Design Validation Using Extended Timing Diagrams},
  booktitle = {Proc. International Conference on Computer-Aided Design},
  year = {1996},
  file = {:./files/1996-HeinkelGlauert.pdf:PDF},
  timestamp = {2006.09.21}
}

@BOOK{2007-HennessyPatterson,
  title = {Computer architecture: a quantitative approach},
  publisher = {Morgan Kaufmann Publishers Inc.},
  year = {2007},
  author = {Hennessy, John L. and Patterson, David A.},
  address = {San Francisco, CA, USA},
  edition = {Fourth Edition},
  file = {:./files/2002-HennessyPatterson.pdf:PDF},
  isbn = {1-55860-596-7},
  owner = {pavlenko},
  timestamp = {2010.07.29}
}

@INPROCEEDINGS{2002-HenzingerJhala.etal,
  author = {Thomas A. Henzinger and Ranjit Jhala and Rupak Majumdar},
  title = {Lazy Abstraction},
  booktitle = {Proc. ACM SIGPLAN-SIGACT Symposium on Principles of Programming Languages
	(POPL)},
  year = {2002},
  pages = {58--70},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {503279},
  file = {:./files/2002-HenzingerJhala.etal.pdf:PDF},
  isbn = {1-58113-450-9},
  location = {Portland, Oregon},
  numpages = {13},
  timestamp = {2006.09.22}
}

@INPROCEEDINGS{2000-HenzingerQadeer.etal,
  author = {Thomas A. Henzinger and Shaz Qadeer and Sriram K. Rajamani},
  title = {Decomposing refinement proofs using assume-guarantee reasoning},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2000},
  pages = {245--253},
  address = {Piscataway, NJ, USA},
  publisher = {IEEE Press},
  file = {:./files/2000-HenzingerQadeer.etal.pdf:PDF},
  isbn = {0-7803-6448-1},
  location = {San Jose, California},
  owner = {wedler},
  timestamp = {2007.08.27}
}

@INPROCEEDINGS{2003-HenzingerJhala.etal,
  author = {T. Henzinger and R. Jhala and R. Majumdar and M. Sanvido},
  title = {Extreme model checking},
  booktitle = {Proc. International Symposium on Verification (Theory and Practice)},
  year = {2003},
  series = {LNCS},
  pages = {180-181},
  file = {:./files/2003-HenzingerJhala.etal.pdf:PDF},
  owner = {nguyen},
  timestamp = {2007.02.02},
  url = {http://citeseer.ist.psu.edu/henzinger03extreme.html}
}

@INPROCEEDINGS{2019-HerdtGrosse.etal,
  author = {Herdt, Vladimir. and Gro{\ss}e, Daniel and Drechsler, Rolf and Gerum,
	Christoph and Jung Alexander and Benz, Joscha-Joel and Bringmann,
	Oliver and Schwarz, Michael and Stoffel, Dominik and Kunz, Wolfgang},
  title = {Systematic RISC-V based Firmware Design},
  booktitle = {Proceedings of "Forum Design Languages" (FDL)},
  year = {2019},
  month = {September},
  note = {(accepted)},
  owner = {schwarz},
  timestamp = {2019.08.06}
}

@INPROCEEDINGS{2015-HeuleSchaub,
  author = {Heule, Marijn J. H. and Schaub, Torsten},
  title = {What's Hot in the SAT and ASP Competitions},
  booktitle = {Proceedings of the Twenty-Ninth AAAI Conference on Artificial Intelligence},
  year = {2015},
  series = {AAAI'15},
  pages = {4322--4323},
  publisher = {AAAI Press},
  acmid = {2888386},
  file = {2015-HeuleSchaub.pdf:files/2015-HeuleSchaub.pdf:PDF},
  isbn = {0-262-51129-0},
  location = {Austin, Texas},
  numpages = {2},
  owner = {villarraga},
  timestamp = {2016.07.14}
}

@ARTICLE{2009-HieronsBogdanov.etal,
  author = {Hierons, Robert and Bogdanov, Kirill and Bowen, Jonathan and Cleaveland,
	Rance and Derrick, John and Dick, Jeremy and Gheorghe, Marian and
	Harman, Mark and Kapoor, Kalpesh and Krause, Paul and Lüttgen, Gerald
	and J. H. Simons, Anthony and Vilkomir, Sergiy and R. Woodward, Martin
	and Zedan, Hussein},
  title = {Using Formal Specifications to Support Testing},
  journal = {{ACM} Computing Surveys},
  year = {2009},
  volume = {41},
  pages = {1-76},
  owner = {fehmel},
  timestamp = {2019.05.27}
}

@ARTICLE{1969-Hillier,
  author = {Frederick S. Hillier},
  title = {Efficient Heuristic Procedures for Integer Linear Programming with
	an Interior},
  journal = {Operations Research},
  year = {1969},
  volume = {17},
  pages = {600-637}
}

@MISC{0000-Ho,
  author = {Pei-Hsin Ho},
  title = {State of the Art Formal Property Verification Technology for Ic Designs},
  file = {0000-Ho.pdf:files/0000-Ho.pdf:PDF},
  owner = {stoffel},
  timestamp = {2006.09.21}
}

@INPROCEEDINGS{1999-HoerethDrechsler,
  author = {S. Hoereth and R. Drechsler},
  title = {Formal Verification of Word-Level Specifications},
  booktitle = {Proc. International Conference on Design, Automation and Test in
	Europe ({DATE})},
  year = {1999},
  pages = {52-58},
  file = {:./files/1999-HoerethDrechsler.pdf:PDF}
}

@INPROCEEDINGS{2001-HoffmannKogel.etal,
  author = {Andreas Hoffmann and Tim Kogel and Heinrich Meyr},
  title = {A Framework for Fast Hardware-Software Co-Simulation},
  booktitle = {Proc. International Conference on Design Automation and Test in Europe
	(DATE)},
  year = {2001},
  pages = {760 -764},
  file = {:./files/2001-HoffmannKogel.etal.pdf:PDF},
  keywords = {LISA machine description language;SystemC simulation class library;abstract
	macrocycle based C++ processes;bit-true models;co-simulation framework;co-simulation
	interface;complete tool-suite;fast compiled processor simulator assembler;fast
	hardware-software co-simulation;fast prototyping;hardware modeling
	efficiency;hardware modeling strategy;instruction-set;linker HLL-compiler;phase
	accuracy;programmable architectures;simulation speed;system-on-chip
	designs;virtual prototype;C++ language;digital signal processing
	chips;embedded systems;hardware-software codesign;instruction sets;integrated
	circuit design;microcontrollers;program compilers;simulation languages;software
	prototyping;},
  timestamp = {2006.09.27}
}

@INPROCEEDINGS{1996-HojatiKrishnan.etal,
  author = {Ramin Hojati and Sriram C. Krishnan and Robert K. Brayton},
  title = {Early Quantification and Partitioned Transition Relations},
  booktitle = {Proc. International Conference on Computer Design, {VLSI} in Computers
	and Processors},
  year = {1996},
  pages = {12--19},
  publisher = {IEEE Computer Society},
  file = {:./files/1996-HojatiKrishnan.etal.pdf:PDF},
  isbn = {0-8186-7554-3}
}

@INPROCEEDINGS{2009-HolcombLi.etal,
  author = {D. Holcomb and Wenchao Li and S. A. Seshia},
  title = {Design as you see {FIT}: System-level soft error analysis of sequential
	circuits},
  booktitle = {2009 Design, Automation Test in Europe Conference Exhibition},
  year = {2009},
  issn = {1530-1591},
  owner = {udupi},
  timestamp = {2018.07.24}
}

@ARTICLE{2002-HolzmannSmith,
  author = {G.J. Holzmann and M.H. Smith},
  title = {An Automated Verification Method for Distributed Systems Software
	based on Model Extraction},
  journal = {{IEEE} Transactions on Software Engineering},
  year = {2002},
  volume = {28},
  pages = {364 -377},
  number = {4},
  month = {apr},
  file = {:./files/2002-HolzmannSmith.pdf:PDF},
  keywords = {Lucent Technologies;automated verification method;call processing
	software;case studies;distributed systems software;formal methods;formal
	model;industrial software development;model extraction;reactive systems;software
	testing;software verification methods;source code;telephone switch;distributed
	processing;program testing;program verification;telecommunication
	computing;},
  timestamp = {2006.09.22}
}

@ARTICLE{1997-Holzmann,
  author = {Gerard J. Holzmann},
  title = {The {SPIN} Model Checker},
  journal = {{IEEE} Transactions on Software Engineering},
  year = {1997},
  volume = {23},
  pages = {279--295},
  file = {:./files/1997-Holzmann.pdf:PDF}
}

@INPROCEEDINGS{1995-HolzmannPeled,
  author = {Gerard J. Holzmann and Doron Peled},
  title = {An improvement in formal verification},
  booktitle = {Proc. International Conference on Formal Description Techniques},
  year = {1995},
  pages = {197--211},
  address = {London, UK, UK},
  publisher = {Chapman \& Hall, Ltd.},
  file = {:./files/1995-HolzmannPeled.pdf:PDF},
  isbn = {0-412-64450-9},
  owner = {nguyen},
  timestamp = {2008.05.20}
}

@INPROCEEDINGS{1997-HongBeerel.etal,
  author = {Youpyo Hong and Peter A. Beerel and Jerry R. Burch and Kenneth L.
	McMillan},
  title = {Safe {BDD} minimization using don't cares},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {1997},
  pages = {208--213},
  address = {New York, NY, USA},
  publisher = {ACM},
  file = {:./files/1997-HongBeerel.etal.pdf:PDF},
  isbn = {0-89791-920-3},
  location = {Anaheim, California, United States}
}

@ARTICLE{1993-Hooker,
  author = {J.N. Hooker},
  title = {Solving the incremental satisfiability problem},
  journal = {The Journal of Logic Programming},
  year = {1993},
  volume = {15},
  pages = {177 - 186},
  number = {1},
  issn = {0743-1066},
  owner = {villarraga},
  timestamp = {2016.07.27}
}

@INPROCEEDINGS{1997-Hooker,
  author = {John N. Hooker},
  title = {Constraint Satisfaction Methods for Generating Valid Cuts},
  booktitle = {Advances in Computational and Stochastic Optimization, Logic Programming
	and Heuristic Search},
  year = {1997},
  editor = {D.L. Woodruff},
  pages = {1-30},
  address = {Dordrecht},
  file = {:./files/1997-Hooker.pdf:PDF}
}

@BOOK{1979-Harrison,
  title = {Introduction to Automata Theory, Languages and Computation},
  publisher = {Addison-Wesley Publishing Company},
  year = {1979},
  editor = {Michael A. Harrison},
  author = {John E. Hopcroft and Jeffrey D. Ullman},
  owner = {nguyen},
  timestamp = {2007.04.19}
}

@INPROCEEDINGS{2013-HornTautschnig.etal,
  author = {Horn, Alex and Tautschnig, Michael and Val, Celina and Liang, Lihao
	and Melham, Tom and Grundy, Jim and Kroening, Daniel},
  title = {Formal Co-Validation of Low-Level Hardware/Software Interfaces},
  booktitle = {Formal Methods in Computer-Aided Design (FMCAD), 2013},
  year = {2013},
  pages = {121-128},
  month = {Oct},
  file = {2013-HornTautschnig.etal.pdf:files/2013-HornTautschnig.etal.pdf:PDF},
  keywords = {formal verification;hardware-software codesign;user interfaces;Ethernet
	MAC;I2C bus;bug-finding technique;executable hardware model;formal
	co-validation;hardware-specific protocol rules;low-level hardware-software
	interfaces;microelectronics industry;real-time clock;software I/O;symbolic
	co-execution;temperature sensor;verifiable codesign},
  owner = {villarraga},
  timestamp = {2014.04.15}
}

@INPROCEEDINGS{2013-HornSauppe.etal,
  author = {Thomas Horn and Matthias Sauppe and Erik Markert and Ulrich Heinkel
	and Wolfgang R{\"o}ssel and Hans-Werner Sahm},
  title = {Einsatz formaler {Methoden} zur {Energieeinsparung}},
  booktitle = {MBMV},
  year = {2013},
  pages = {141-146},
  owner = {joakim},
  timestamp = {2013.07.25}
}

@INPROCEEDINGS{1999-HoskoteKam.etal,
  author = {Hoskote, Yatin and Kam, Timothy and Ho, Pei-Hsin and Zhao, Xudong},
  title = {Coverage estimation for symbolic model checking},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {1999},
  pages = {300--305},
  address = {New York, NY, USA},
  publisher = {ACM},
  file = {:./files/1999-HoskoteKam.etal:PDF},
  isbn = {1-58133-109-7},
  location = {New Orleans, Louisiana, United States},
  owner = {wedler},
  timestamp = {2010.01.11}
}

@INPROCEEDINGS{2004-Howison,
  author = {James Howison and Abby Goodrum},
  title = {Why can?t {I} manage academic papers like {MP3s}? The evolution and
	intent of metadata standards},
  booktitle = {Proceedings of the 2004 Colleges, Code and Intellectual Property
	Conference},
  year = {2004},
  number = {57},
  series = {ACRL Publications in Librarianship},
  address = {College Park, MD},
  file = {:./files/2004-Howison.pdf:PDF},
  researchr = {http://researchr.org/publication/HowisonG%3A2004},
  tags = {digital libraries, information retrieval, p2p}
}

@INPROCEEDINGS{1998-HsiehLevitan,
  author = {Yee-Wing Hsieh and Steven P. Levitan},
  title = {Model Abstraction for Formal Verification},
  booktitle = {Proc. International Conference on Design, Automation and Test in
	Europe ({DATE})},
  year = {1998},
  pages = {140 -147},
  file = {:./files/1998-HsiehLevitan.pdf:PDF},
  keywords = {VHDL;circuit design;formal verification;model abstraction;semantic
	extraction;circuit CAD;formal verification;hardware description languages;},
  timestamp = {2006.09.12}
}

@INPROCEEDINGS{1999-Hsiung,
  author = {Pao-Ann Hsiung},
  title = {Hardware-Software Coverification of Concurrent Embedded Real-Time
	Systems},
  booktitle = {Proc. International Conference on Hardware Software Codesign},
  year = {1999},
  pages = {216 -223},
  file = {:./files/1999-Hsiung.pdf:PDF},
  keywords = {concurrent embedded real-time systems;cosimulation;hardware-software
	codesign;hardware-software coverification;high-assurance systems;linear
	hybrid automata;state-space explosion;system specifications;verification
	scalability;embedded systems;formal verification;hardware-software
	codesign;protocols;},
  timestamp = {2006.09.27}
}

@ARTICLE{1997-HsuehTsai.etal,
  author = {Mei-Chen Hsueh and T.K. Tsai and R.K. Iyer},
  title = {Fault injection techniques and tools},
  journal = {Computer},
  year = {1997},
  volume = {30},
  pages = {75 -- 82},
  number = {4},
  month = {Apr},
  file = {1997-HsuehTsai.etal.pdf:files/1997-HsuehTsai.etal.pdf:PDF},
  issn = {0018-9162},
  owner = {bartsch},
  timestamp = {2015.09.10}
}

@INPROCEEDINGS{1997-Hu,
  author = {Alan J. Hu},
  title = {Formal Hardware Verification with {BDD}s: An Introduction},
  booktitle = {{IEEE} Pacific Rim Conference on Communications, Computers, and Signal
	Processing ({PACRIM})},
  year = {1997},
  volume = {2},
  pages = {677 -682},
  month = {aug},
  file = {:./files/1997-Hu.pdf:PDF},
  keywords = {BDD;binary decision diagrams;combinational equivalence checking;formal
	hardware verification;logic design;model checking;research;sequential
	equivalence checking;symbolic simulation;symbolic trajectory evaluation;Boolean
	functions;combinational circuits;diagrams;formal verification;logic
	design;symbol manipulation;},
  owner = {pavlenko},
  timestamp = {2011.01.17}
}

@INPROCEEDINGS{2003a-HuCasas.etal,
  author = {Alan J. Hu and Jeremy Casas and Jin Yang},
  title = {Efficient Generation of Monitor Circuits for {GSTE} Assertion Graphs},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2003},
  pages = {154-159},
  file = {:./files/2003a-HuCasas.etal.pdf:PDF},
  isbn = {1-58113-762-1},
  owner = {nguyen},
  timestamp = {2007.12.13}
}

@INPROCEEDINGS{2003-HuCasas.etal,
  author = {Alan J. Hu and Jeremy Casas and Jin Yangpa},
  title = {Reasoning about {GSTE} Assertion Graphs},
  booktitle = {Proc. Advanced Research Working Conference on Correct Hardware Design
	and Verification Methods ({CHARME})},
  year = {2003},
  pages = {170--184},
  publisher = {Springer},
  note = {Lecture Notes in Computer Science Vol.~2860},
  file = {:./files/2003-HuCasas.etal.pdf:PDF}
}

@INPROCEEDINGS{1992-HuDill,
  author = {Alan J. Hu and David L. Dill},
  title = {Reducing {BDD} Size by Exploiting Functional Dependencies},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {1992},
  pages = {522-525},
  file = {:./files/1992-HuDill.pdf:PDF}
}

@INPROCEEDINGS{1994-HuYork.etal,
  author = {Alan J. Hu and Gary York and David L. Dill},
  title = {New Techniques for Efficient Verification with Implicitly Conjoined
	{BDD}s},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {1994},
  pages = {276-282},
  file = {:./files/1994-HuYork.etal.pdf:PDF}
}

@INPROCEEDINGS{2005-HuShi,
  author = {Bo Hu and C.-J. Richard Shi},
  title = {Fast-Yet-Accurate PVT Simulation by Combined Direct and Iterative
	Methods},
  booktitle = {Proc. International Conference on Computer-Aided Design (ICCAD)},
  year = {2005},
  pages = { 495 - 501},
  file = {:./files/2005-HuShi.pdf:PDF},
  keywords = { Krylov subspace based iterative method; LU-factorization based direct
	method; PVT simulation; RF circuit design; analog circuit; circuit
	simulation; deep-submicron integrated circuit; digital library cell;
	process-voltage-temperature condition; circuit simulation; integrated
	circuit design; iterative methods;},
  timestamp = {2006.09.27}
}

@INPROCEEDINGS{2016-HuAlthoff.etal,
  author = {Hu, Wei and Althoff, Alric and Ardeshiricham, Armaiti and Kastner,
	Ryan},
  title = {Towards Property Driven Hardware Security},
  booktitle = {Microprocessor and SOC Test and Verification (MTV), 2016 17th International
	Workshop on},
  year = {2016},
  pages = {51--56},
  organization = {IEEE},
  owner = {fadiheh},
  timestamp = {2018.07.12}
}

@INPROCEEDINGS{2017-HuArdeshiricham.etal,
  author = {Hu, Wei and Ardeshiricham, Armaiti and Kastner, Ryan},
  title = {Identifying and Measuring Security Critical Path for Uncovering Circuit
	Vulnerabilities},
  booktitle = {International Workshop on Microprocessor and SOC Test and Verification
	(MTV)},
  year = {2017},
  organization = {IEEE},
  owner = {fadiheh},
  timestamp = {2018.07.12}
}

@ARTICLE{2019-HuangZhang.etal,
  author = {Huang, Bo-Yuan and Zhang, Hongce and Subramanyan, Pramod and Vizel,
	Yakir and Gupta, Aarti and Malik, Sharad},
  title = {Instruction-Level Abstraction ({ILA}): A Uniform Specification for
	System-on-Chip ({SoC}) Verification},
  journal = {ACM Trans. Des. Autom. Electron. Syst},
  year = {2019},
  volume = {24},
  pages = {10:1--10:24},
  number = {1},
  month = jan,
  articleno = {10},
  file = {2019-HuangZhang.etal.pdf:files/2019-HuangZhang.etal.pdf:PDF}
}

@ARTICLE{2001-HuangCheng,
  author = {C.-Y. Huang and K. T. Cheng},
  title = {Using Word-Level {ATPG} and Modular Arithmetic Constraint-Solving
	Techniques for Assertion Property Checking},
  journal = {{IEEE} Transactions on Computer-Aided Design},
  year = {2001},
  volume = {20},
  pages = {381 -391},
  number = {3},
  month = {March},
  file = {:./files/2001-HuangCheng.pdf:PDF},
  keywords = {ATPG search space;arithmetic constraint solver;assertion property
	checking;datapath signals;decision-making process;implication translation
	techniques;industrial designs;industrial front-end hardware description
	language;modular arithmetic constraint-solving techniques;modular
	number system;property-to-constraint converter;register-transfer
	level design verification;target assertion property;word-level ATPG;automatic
	test pattern generation;constraint handling;formal verification;hardware
	description languages;high level synthesis;integrated circuit testing;logic
	testing;}
}

@INPROCEEDINGS{1996a-HuangCheng.etal,
  author = {S.Y. Huang and K.T. Cheng and K.C. Chen and Uwe Glaeser},
  title = {On Verifying the Correctness of Retimed Circuits},
  booktitle = {Proc. Great Lakes Symposium on VLSI},
  year = {1996},
  pages = {277 -280},
  file = {huang96verifying.pdf:huang96verifying.pdf:PDF},
  keywords = {ISCAS89 benchmark circuits;clock cycle time;correctness verification;flip-flops;retimed
	circuits;sequential ATPG techniques;sequential circuit;three-valued
	equivalence;verification framework;automatic testing;clocks;flip-flops;integrated
	circuit testing;logic testing;sequential circuits;}
}

@INPROCEEDINGS{1996-HuangCheng.etal,
  author = {S.Y. Huang and K.T. Cheng and K.C. Chen and Uwe Glaeser},
  title = {An {ATPG}-Based Framework for Verifying Sequential Equivalence},
  booktitle = {Proc. International Test Conference (ITC)},
  year = {1996},
  pages = {865 -874},
  file = {:./files/1996-HuangCheng.etal.pdf:PDF},
  keywords = {ATPG;backward justification;equivalence checking;equivalent hip-hops;flip-flops;memory
	explosion;retiming;sequential ATPG programs;sequential circuits;sequential
	equivalence;sequential optimization;sequential redundancy;sequential
	redundancy removal;structural similarity;test pattern generation;automatic
	testing;flip-flops;logic testing;optimisation;redundancy;sequential
	circuits;synchronisation;}
}

@ARTICLE{2001-HuangCheng.etal,
  author = {Huang, Shi-Yu and Cheng, Kwang-Ting and Chen, Kuang-Chien},
  title = {Verifying sequential equivalence using {ATPG} techniques},
  journal = {{ACM} Trans. Des. Autom. Electron. Syst.},
  year = {2001},
  volume = {6},
  pages = {244--275},
  number = {2},
  month = apr,
  acmid = {376022},
  address = {New York, NY, USA},
  file = {:./files/2001-HuangCheng.etal.pdf:PDF},
  issn = {1084-4309},
  issue_date = {April 2001},
  numpages = {32},
  publisher = {ACM}
}

@INPROCEEDINGS{2008-Hurst,
  author = {A. P. Hurst},
  title = {Automatic synthesis of clock gating logic with controlled netlist
	perturbation},
  booktitle = {Design Automation Conference, 2008. DAC 2008. 45th ACM/IEEE},
  year = {2008},
  pages = {654-657},
  month = {June},
  issn = {0738-100X},
  keywords = {clocks;logic design;logic gates;perturbation theory;automatic synthesis;clock
	gating logic;dynamic clock power;netlist perturbation;registers;Automatic
	control;Automatic logic units;Circuits;Clocks;Cost function;Energy
	consumption;Network synthesis;Registers;Signal synthesis;Switches;Clock
	Gating;Dynamic Power;Logic Optimization;Low Power}
}

@BOOK{2004-HuthRyan,
  title = {Logic in Computer Science - Modelling and Reasoning about Systems},
  publisher = {Cambridge University Press},
  year = {2004},
  author = {Michael Huth and Mark Ryan},
  owner = {bschmidt},
  timestamp = {2014.04.08}
}

@MISC{0000-BeerDavid.etal,
  author = {I.Beer and Shoham B.David and D.Geist and Raanan Gewirtzmann and
	M.Yoeli},
  title = {Formal Verification Of Reactive System},
  file = {0000-BeerDavid.etal.pdf:files/0000-BeerDavid.etal.pdf:PDF},
  owner = {stoffel},
  timestamp = {2006.09.22}
}

@MISC{1979-IBM,
  author = {{IBM}},
  title = {Mathematical Programming System Extended/370 ({MPSX}/370) Program
	Reference Manual},
  year = {1979},
  note = {SH19-1095-3, 4th Ed.},
  address = {White Plains, N.Y.},
  organization = {IBM Corp.},
  owner = {stoffel},
  timestamp = {2016.05.11}
}

@MISC{0000-Sixthsense,
  author = {{IBM }},
  title = {SixthSense: A Tool for Sequential Equivalence Checking and (Semi-)Formal
	Verification},
  owner = {wedler},
  timestamp = {2009.07.20},
  url = {http://domino.research.ibm.com/comm/research_projects.nsf/pages/sixthsense.index.html}
}

@MISC{1999-IBM,
  author = {{IBM Corporation}},
  title = {{CoreConnect Bus Architecture}},
  howpublished = {http://www.ibm.com},
  year = {1999},
  owner = {villarraga},
  publisher = {{IBM Microelectronics Division}},
  timestamp = {2016.07.18}
}

@ARTICLE{1986-IEEE,
  author = {IEEE},
  title = {{IEEE} Standard for Logic Circuit Diagrams. Corrected Edition},
  journal = {{ANSI}/{IEEE} Std 991-1986},
  year = {1986},
  file = {:./files/1986-IEEE.pdf:PDF},
  keywords = {ANSI/IEEE Std 91-1984;ANSI/IEEE Std 991-1986;circuit diagram;logic
	circuit;logic function;product documentation;representation;symbols;logic
	circuits;standards;},
  timestamp = {2010.11.27}
}

@BOOK{2007-IenneLeupers,
  title = {Customizable Embedded Processors},
  publisher = {Morgan Kaufmann Publishers},
  year = {2007},
  author = {P. Ienne and R. Leupers},
  owner = {brehm},
  timestamp = {2007.03.28}
}

@MISC{2001-CPLEX,
  author = {{ILOG CPLEX}},
  title = {Reference Manual},
  year = {2001},
  address = {889 Alder Avenue, Suite 200, Incline Village, NV 89451, USA},
  file = {:./files/2001-CPLEX.pdf:PDF},
  organization = {ILOG CPLEX Division},
  owner = {stoffel},
  timestamp = {2016.05.11},
  url = {http://www.ilog.com/products/cplex}
}

@INBOOK{2008-RiedenPaul,
  pages = {321--326},
  title = {Beweisen als Ingenieurwissenschaft: Verbundprojekt Verisoft (2003--2007)},
  publisher = {Springer},
  year = {2008},
  author = {In der Rieden, T. and Paul, W. J.},
  booktitle = {Informatikforschung in Deutschland},
  ee = {http://www.springerlink.de/content/978-3-540-76549-3/#section=143513&page=1&locus=0},
  owner = {joakim},
  timestamp = {2016.03.18}
}

@MISC{2010-Infineon,
  author = {{Infineon Technologies AG}},
  title = {{TriCore} 2 Architectural Manual, Doc v1.0},
  owner = {stoffel},
  timestamp = {2010.06.15},
  url = {http://www.infineon.com/tricore}
}

@MISC{2008-Infineon,
  author = {{Infineon Technologies AG}},
  title = {{TriCore} TC1797 User's Manual, Doc v1.0},
  year = {2008},
  owner = {bschmidt},
  timestamp = {2010.06.15},
  url = {http://www.infineon.com/tricore}
}

@MISC{web-systemc,
  author = {Accellera Systems Initiative}
}

@MISC{web_intel_bug,
  author = {{Intel Pentium FDIV bug}},
  owner = {pavlenko},
  timestamp = {2011.01.06},
  url = {http://www.cs.earlham.edu/~dusko/cs63/fdiv.html}
}

@INPROCEEDINGS{1991-IshiuraSawada.etal,
  author = {N. Ishiura and H. Sawada and S. Yajima},
  title = {Minimization of Binary Decision Diagrams Based on Exchanges of Variables},
  booktitle = {Proc. International Conference on Computer-Aided Design (ICCAD)},
  year = {1991},
  pages = {472 -475},
  file = {:./files/1991-IshiuraSawada.etal.pdf:PDF},
  keywords = { binary decision diagrams minimisation; exchanges of variables; greedy
	method; intermediate functions; pruning; simulated annealing; logic
	CAD; logic testing; simulated annealing;}
}

@ARTICLE{2004-IvancicYang.etal,
  author = {Franjo Ivancic and Zijiang Yang and Malay K. Ganai and Aarti Gupta
	and Pranav Ashar},
  title = {Efficient {SAT}-based bounded model checking for software verification},
  journal = {Theoretical Computer Science },
  year = {2004},
  volume = {404},
  pages = {256--274},
  number = {3},
  note = {International Symposium on Leveraging Applications of Formal Methods
	(ISoLA 2004) },
  file = {:import/var/jabref/files/2004-IvancicYang.pdf:PDF},
  issn = {0304-3975},
  keywords = {Software verification},
  owner = {stoffel},
  timestamp = {2014.07.31}
}

@INPROCEEDINGS{2000-IversenKristoffersen.etal,
  author = {Torsten K. Iversen and Kare J. Kristoffersen and Kim G. Larsen and
	Morten Laursen and Rune G. Madsen and Steffen K. Mortensen and Paul
	Pettersson and Chris B. Thomasen},
  title = {Model-Checking Real-Time Control Programs},
  booktitle = {Proc. 12th Euromicro Conference on Real-Time Systems ({ECRTS})},
  year = {2000},
  pages = {147 -155},
  file = {:./files/2000-IversenKristoffersen.etal.pdf:PDF},
  keywords = {LEGO MINDSTORMS systems verification;LEGO RCX bricks;UPPAAL;automatic
	verification;concurrent tasks;control programs;fixed scheduling algorithm;model
	checking;real time control programs;real time system;timed automata
	model;verification tool;automata theory;control engineering computing;multiprogramming;program
	verification;real-time systems;scheduling;},
  timestamp = {2006.09.22}
}

@INPROCEEDINGS{1996IyerLong.etal,
  author = {Iyer, Mahesh A. and Long, David E. and Abramovici, Miron},
  title = {Identifying Sequential Redundancies Without Search},
  booktitle = {Proceedings of the 33rd Annual Design Automation Conference},
  year = {1996},
  series = {DAC '96},
  pages = {457--462},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {240605},
  isbn = {0-89791-779-0},
  location = {Las Vegas, Nevada, USA},
  numpages = {6},
  owner = {udupi},
  timestamp = {2015.05.05}
}

@ARTICLE{1992-ArlatCostes.etal,
  author = {J.Arlat and A.Costes and Y.Crouset and J.Laprie and D.Powell},
  title = {Fault Injection and Dependability Evaluation of Fault-Tolerant Systems},
  journal = {{IEEE} Transactions on Computers},
  year = {1992},
  file = {:./files/1992-ArlatCostes.etal.pdf:PDF},
  timestamp = {2006.09.14}
}

@ARTICLE{1994-JaffarMaher,
  author = {J.Jaffar and M. J. Maher},
  title = {Constraint Logic Programming: A survey},
  journal = {The Journal of Logic Programming},
  year = {1994},
  volume = {19},
  pages = {503-582},
  file = {:./files/1994-JaffarMaher.pdf:PDF}
}

@INBOOK{2012-JaervisaloHeule.etal,
  chapter = {Inprocessing Rules},
  pages = {355--370},
  title = {Automated Reasoning: 6th International Joint Conference, IJCAR 2012,
	Manchester, UK, June 26-29, 2012. Proceedings},
  publisher = {Springer Berlin Heidelberg},
  year = {2012},
  editor = {Gramlich, Bernhard and Miller, Dale and Sattler, Uli},
  author = {J{\"a}rvisalo, Matti and Heule, Marijn J. H. and Biere, Armin},
  address = {Berlin, Heidelberg},
  isbn = {978-3-642-31365-3},
  owner = {villarraga},
  timestamp = {2016.07.27}
}

@ARTICLE{2012-JaervisaloLeBerre.etal,
  author = {J{\"a}rvisalo, Matti and Le Berre, Daniel and Roussel, Olivier and
	Simon, Laurent},
  title = {The International SAT Solver Competitions},
  journal = {Artificial Intelligence Magazine},
  year = {2012},
  volume = {33},
  number = {1},
  owner = {villarraga},
  timestamp = {2016.07.27}
}

@PHDTHESIS{2002-Jacobi,
  author = {Christian Jacobi},
  title = {Formal Verification of a Fully {IEEE} Compliant Floating Point Unit},
  school = {Universit\"{a}t des Saarlandes},
  year = {2002},
  file = {:./files/2002-Jacobi.pdf:PDF},
  timestamp = {2006.10.04}
}

@INPROCEEDINGS{1987-JaffarLassez,
  author = {Joxan Jaffar and Jean-Louis Lassez},
  title = {Constraint Logic Programming},
  booktitle = {Proc. ACM SIGPLAN-SIGACT Symposium on Principles of Programming Languages
	(POPL)},
  year = {1987},
  pages = {111--119},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {41635},
  file = {:./files/1987-JaffarLassez.pdf:PDF},
  isbn = {0-89791-215-2},
  location = {Munich, West Germany},
  numpages = {9}
}

@INPROCEEDINGS{2005-JainKroening.etal,
  author = {Himanshu Jain and Daniel Kroening and Natasha Sharygina and Edmund
	Clarke},
  title = {Word level predicate abstraction and refinement for verifying {RTL}
	{V}erilog},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {2005},
  pages = {445--450},
  address = {New York, NY, USA},
  publisher = {ACM Press},
  file = {:./files/2005-JainKroening.etal.pdf:PDF},
  isbn = {1-59593-058-2},
  location = {San Diego, California, USA},
  owner = {nguyen},
  timestamp = {2007.04.12}
}

@ARTICLE{2008-JainKroening.etal,
  author = {Himanshu Jain and Daniel Kroening and Natasha Sharygina and Edmund
	M. Clarke},
  title = {Word-Level Predicate-Abstraction and Refinement Techniques for Verifying
	{RTL} {V}erilog},
  journal = {{IEEE} Transactions on Computer-Aided Design},
  year = {2008},
  volume = {27},
  pages = {366-379},
  number = {2},
  bibsource = {DBLP, http://dblp.uni-trier.de},
  file = {:./files/2008-JainKroening.etal.pdf:PDF}
}

@INPROCEEDINGS{1995-JainMukherjee.etal,
  author = {J. Jain and R. Mukherjee and M. Fujita},
  title = {Advanced Verification Techniques Based on Learning},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {1995},
  pages = {420 - 426},
  file = {:./files/1995-JainMukherjee.etal.pdf:PDF}
}

@ARTICLE{2001-JainGrossmann,
  author = {Vipul Jain and Ignacio E. Grossmann},
  title = {Algorithms for Hybrid {MILP/CP} Models for a Class of Optimization
	Problems},
  journal = {Informs Journal on Computing},
  year = {2001},
  volume = {13},
  pages = {258-276},
  number = {4},
  file = {:./files/2001-JainGrossmann.pdf:PDF}
}

@INPROCEEDINGS{2002-JancarKucera.etal,
  author = {Petr Jancar and Antonin Kucera and Faron Moller and Zdenek Sawa},
  title = {Equivalence-Checking with One-Counter Automata},
  booktitle = {Proc. International Conference on Foundations of Software Science
	and Computation Structures},
  year = {2002},
  series = {FoSSaCS '02},
  pages = {172--186},
  address = {London, UK, UK},
  publisher = {Springer-Verlag},
  acmid = {704842},
  file = {:./files/2002-JancarKucera.etal.pdf:PDF},
  isbn = {3-540-43366-X},
  numpages = {15},
  timestamp = {2006.09.13}
}

@INPROCEEDINGS{2000-JangMoon.etal,
  author = {J. Jang and In-Ho Moon and G. Hachtel},
  title = {Iterative Abstraction Based {CTL} Model Checking},
  booktitle = {Proc. International Conference on Design, Automation and Test in
	Europe ({DATE})},
  year = {2000},
  pages = {502 -507},
  file = {:./files/2000-JangMoon.etal.pdf:PDF},
  keywords = {BDD nodes;BDD variables;automatic approximation;automatic refinement;iterative
	abstraction-based CTL model checking;lower bounds;operational graphs;upper
	bounds;approximation theory;binary decision diagrams;circuit analysis
	computing;graph theory;iterative methods;},
  timestamp = {2006.09.12}
}

@MISC{1997-GanaiJas.etal,
  author = {Malay K.Ganai Abhijit Jas and Alper Sen and Anand ramachandran and
	Cagdas Akturan and Chia bin Liu and Debaleena Das and I-Min Liu and
	Jayanta Bhadra and Justin R.Denison And Kaustubh Das and Padmini
	Gopalakrishnan and Parminder S.Chhabra and Praveen K.Jaini and Adnan
	Aziz},
  title = {Examples Of Hardware Verificatoin Using Vis},
  year = {1997},
  file = {:./files/1997-GanaiJas.etal.pdf:PDF},
  owner = {stoffel},
  timestamp = {2006.09.21}
}

@MISC{0000-Jasper,
  author = {Jasper Design Automation, Inc.},
  owner = {stoffel},
  timestamp = {2016.05.10},
  url = {http://www.jasper-da.com/}
}

@INPROCEEDINGS{2012-JayasingheRagel.etal,
  author = {Jayasinghe, Darshana and Ragel, Roshan and Elkaduwe, Dhammika},
  title = {Constant time encryption as a countermeasure against remote cache
	timing attacks},
  booktitle = {IEEE 6th International Conference on Information and Automation for
	Sustainability (ICIAfS)},
  year = {2012},
  pages = {129--134},
  organization = {IEEE},
  owner = {fadiheh},
  timestamp = {2018.07.12}
}

@INPROCEEDINGS{1994-JennArlat.etal,
  author = {E. Jenn and J. Arlat and M. Rimen and J. Ohlsson and J. Karlsson},
  title = {Fault Injection into VHDL Models: The MEFISTO Tool},
  booktitle = {Proc. 24th International Symposium on Fault-Tolerant Computing},
  year = {1994},
  pages = {66 - 75},
  month = {June},
  file = {:files/1994-JennArlat.etal.pdf:PDF},
  owner = {bartsch},
  timestamp = {2014.07.30}
}

@INPROCEEDINGS{1991-JeongPlessier.etal,
  author = {S.-W. Jeong and B. Plessier and G. D. Hachtel and F. Somenzi},
  title = {Variable Ordering and Selection of {FSM} Traversal},
  booktitle = {Computer-Aided Design, 1991. ICCAD-91. Digest of Technical Papers.,
	1991 IEEE International Conference on},
  year = {1991},
  pages = {476 -479},
  address = {MCNC, Research Triangle Park, NC},
  month = {May},
  file = {:./files/1991-JeongPlessier.etal.pdf:PDF},
  keywords = { FSM traversal; algebraic structure; binary decision diagram; complexity;
	finite state machines; heuristic ordering methods; image computation;
	implicit enumeration; reachable states; selection heuristic; variable
	ordering; verification; finite automata; logic CAD; logic testing;}
}

@ARTICLE{2005-JerrayaWolf,
  author = {A. A. Jerraya and W. Wolf},
  title = {Hardware/software interface codesign for embedded systems},
  journal = {Computer},
  year = {2005},
  volume = {38},
  pages = {63-69},
  number = {2},
  month = {Feb},
  doi = {10.1109/MC.2005.61},
  issn = {0018-9162},
  keywords = {hardware-software codesign;embedded systems;system-on-chip;middleware;multiprocessing
	systems;software reusability;software quality;parallel programming;embedded
	systems;HW/SW interface codesign;heterogeneous multiprocessors;system-on-chip;middleware;software
	reusability;software quality;parallel programming;Hardware;Embedded
	software;Embedded system;Video compression;Costs;Application software;Cameras;Central
	Processing Unit;Design engineering;Software design}
}

@INPROCEEDINGS{2009-JhaLimaye.etal,
  author = {Jha, Susmit and Limaye, Rhishikesh and Seshia, Sanjit},
  title = {Beaver: Engineering an Efficient {SMT} Solver for Bit-Vector Arithmetic},
  booktitle = {Proceedings of the 21st International Conference on Computer Aided
	Verification},
  year = {2009},
  series = {CAV '09},
  pages = {668--674},
  file = {:./files/2009-JhaLimaye.etal.pdf:PDF},
  owner = {pavlenko},
  timestamp = {2010.07.26}
}

@ARTICLE{2009-JhalaMajumdar,
  author = {Jhala, Ranjit and Majumdar, Rupak},
  title = {Software model checking},
  journal = {ACM Comput. Surv.},
  year = {2009},
  volume = {41},
  pages = {21:1--21:54},
  month = {October},
  acmid = {1592438},
  address = {New York, NY, USA},
  articleno = {21},
  file = {2009-JhalaMajumdar.pdf:files/2009-JhalaMajumdar.pdf:PDF},
  issn = {0360-0300},
  issue = {4},
  keywords = {Software model checking, abstraction, counterexample-guided refinement,
	enumerative and symbolic model checking, liveness, safety},
  numpages = {54},
  owner = {villarraga},
  publisher = {ACM},
  timestamp = {2012.08.27}
}

@INPROCEEDINGS{2001-JhalaMcMillan,
  author = {Ranjit Jhala and Kenneth L. McMillan},
  title = {Microarchitecture Verification by Compositional Model Checking},
  booktitle = {Proc. International Conference on Computer Aided Verification ({CAV})},
  year = {2001},
  pages = {396--410},
  address = {London, UK, UK},
  publisher = {Springer-Verlag},
  acmid = {734122},
  file = {:./files/2001-JhalaMcMillan.pdf:PDF},
  isbn = {3-540-42345-1},
  numpages = {15},
  timestamp = {2006.09.13}
}

@ARTICLE{2006-JiangBrayton,
  author = {J.-H. R. Jiang and R. K. Brayton},
  title = {Retiming and Resynthesis: A Complexity Perspective},
  journal = {IEEE Transactions on Computer-Aided Design},
  year = {2006},
  volume = {25},
  pages = {2674-2686},
  number = {12},
  month = {December},
  file = {:./files/2006-JiangBrayton.pdf:PDF},
  owner = {wedler},
  timestamp = {2006.12.21}
}

@INPROCEEDINGS{2005-JiangFu.etal,
  author = {Rong Jiang and Wenyin Fu and Janet Meiling Wang and Vince Lin and
	Charlie Chung-Ping Chen},
  title = {Efficient Statistical Capacitance Variability Modeling with Orthogonal
	Principle Factor Analysis},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2005},
  pages = { 683 - 690},
  file = {:./files/2005-JiangFu.etal.pdf:PDF},
  keywords = { Monte Carlo simulation; VLSI design; closed form capacitance model;
	conductor surface fluctuation; integrated circuit process technology;
	interconnect geometry; layout tool; orthogonal principle factor analysis;
	parasitic capacitance; statistical capacitance variability modeling;
	statistical model order reduction; timing analysis; wafer fabricated
	circuit; Monte Carlo methods; VLSI; capacitance; integrated circuit
	design; integrated circuit interconnections; integrated circuit modelling;
	statistical analysis; variational techniques;},
  timestamp = {2006.09.27}
}

@UNPUBLISHED{2005-Jin,
  author = {HoonSang Jin},
  title = {Efficient Algorithm for Finding All Satisfying Assignments},
  year = {2005},
  file = {:./files/2005-Jin.pdf:PDF},
  owner = {nguyen},
  timestamp = {2007.02.02}
}

@INBOOK{2005-JinHan.etal,
  chapter = {Efficient Conflict Analysis for Finding All Satisfying Assignments
	of a {Boolean} Circuit},
  pages = {287-300},
  title = {Tools and Algorithms for the Construction and Analysis of Systems},
  publisher = {Springer Berlin / Heidelberg},
  year = {2005},
  author = {HoonSang Jin and HyoJung Han and Fabio Somenzi},
  volume = {3440/2005},
  series = {Lecture Notes in Computer Science},
  file = {:./files/2005-JinHan.etal.pdf:PDF},
  timestamp = {2006.09.19}
}

@INPROCEEDINGS{2005-JinSomenzi,
  author = {HoonSang Jin and Fabio Somenzi},
  title = {Prime Clauses for Fast Enumeration of Satisfying Assignments to Boolean
	Circuits},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {2005},
  pages = { 750 - 753},
  file = {:./files/2005-JinSomenzi.pdf:PDF},
  keywords = { {Boolean} circuits; SAT-based unbounded model checking; blocking
	clauses; clause-recording propositional satisfiability solver; conflict
	clauses; prime clauses; satisfiable points; satisfying assignments;
	unsatisfiable points; {Boolean} functions; logic design;},
  owner = {nguyen},
  timestamp = {2007.02.02}
}

@PHDTHESIS{2002-Johannsen,
  author = {Peer Johannsen},
  title = {Speeding Up Hardware Verif ication by Automated Datapath Scaling},
  year = {2002},
  file = {:./files/2002-Johannsen.pdf:PDF},
  timestamp = {2006.09.12}
}

@INPROCEEDINGS{2001-Johannsen,
  author = {P. Johannsen},
  title = {{BOOSTER}: Speeding Up {RTL} Property Checking of Digital Designs
	by Word-Level Abstraction},
  booktitle = {Proc. International Conference Computer Aided Verification ({CAV})},
  year = {2001},
  pages = {373-377},
  month = {July},
  file = {:./files/2001-Johannsen.pdf:PDF}
}

@INPROCEEDINGS{2001-JohannsenDrechsler,
  author = {P. Johannsen and R. Drechsler},
  title = {Formal Verification on the {RT} Level Computing One-To-One Design
	Abstractions by Signal Width Reduction},
  booktitle = {Proc. {IFIP} International Conference on Very Large Scale Integration
	({IFIP} {VLSI-SOC} 2001)},
  year = {2001},
  pages = {127--132},
  address = {Montpellier, France},
  file = {:./files/2001-JohannsenDrechsler.pdf:PDF}
}

@INPROCEEDINGS{2001-JohnsenOwe.etal,
  author = {Johnsen, E.B. and Owe, O. and Munthe-Kaas, E. and Vain, J.},
  title = {Incremental Fault Tolerant Design In An Object-Oriented Setting},
  booktitle = {Quality Software, 2001. Proceedings.Second Asia-Pacific Conference
	on},
  year = {2001},
  pages = {223 -230},
  file = {:./files/2001-JohnsenOwe.etal.pdf:PDF},
  keywords = {communication traces;dependability;design process;distributed systems;first-order
	predicates;formal methods;incremental design;incremental fault-tolerant
	design;intolerant system specification;liveness;object orientation;object-oriented
	system specifications;object-oriented systems;refinement process;refinement
	step;safety;specification language;system development;trace semantics;distributed
	programming;object-oriented programming;software fault tolerance;}
}

@INPROCEEDINGS{1995-JonesDill.etal,
  author = {R. B. {Jones} and D. L. {Dill} and J. R. {Burch}},
  title = {{Efficient Validity Checking for Processor Verification}},
  booktitle = {Proc. of IEEE/ACM Intl. Conference on Computer-aided
	Design (ICCAD)},
  year = {1995},
  pages = {2--6},
  acmid = {224849},
  isbn = {0-8186-7213-7},
  keywords = {decision procedure, formal verification, microprocessor architecture,
	uninterpreted functions, validation},
  numpages = {5},
  owner = {fadiheh},
  timestamp = {2019.09.03}
}

@PHDTHESIS{1997-Jonsson,
  author = {Ari Kristinn Jonsson},
  title = {Procedural Reasoning In Constraint Satisfaction},
  school = {Dept. of Computer Science, Stanford University},
  year = {1997},
  file = {:./files/1997-Jonsson.pdf:PDF},
  timestamp = {2006.09.21}
}

@TECHREPORT{2004-JoswigPfetsch,
  author = {Michael Joswig and Marc E. Pfetsch},
  title = {Computing Optimal Morse Matchings},
  institution = {Zuse Institute Berlin},
  year = {2004},
  number = {04-37},
  file = {:./files/2004-JoswigPfetsch.pdf:PDF},
  url = {http://www.zib.de/Publications/abstracts/ZR-04-37/}
}

@INPROCEEDINGS{2006-JussilaSinz.etal,
  author = {Toni Jussila and Carsten Sinz and Armin Biere},
  title = {Extended resolution proofs for symbolic {SAT} solving with quantification},
  booktitle = {Proc. 9th Intl. Conf. on Theory and Applications of Satisfiability
	Testing ({SAT}'06)},
  year = {2006},
  pages = {54--60},
  publisher = {Springer},
  file = {:./files/2006-JussilaSinz.etal.pdf:PDF},
  owner = {pavlenko},
  timestamp = {2011.03.04}
}

@INPROCEEDINGS{1999-FerdinandKaestner.etal,
  author = {K.Ferdinand and D.Kaestner and M.Langenbach and F.Martin and M.Schmiidt
	and j.Schneider and H.Theiling and R.Wilhelm},
  title = {Run-Time Guarantees for Real-Time Systems - The {USES} Approach},
  booktitle = {Proceedings of Informatik'99-Arbeitstagung GI Jahrestagung},
  year = {1999},
  file = {:./files/1999-FerdinandKaestner.etal.pdf:PDF},
  timestamp = {2006.09.22}
}

@PHDTHESIS{2002-Shimizu,
  author = {K.Shimizu},
  title = {Protocol Specification Using Monitor Module},
  year = {2002},
  file = {:./files/2002-Shimizu.pdf:PDF},
  timestamp = {2006.09.19}
}

@INPROCEEDINGS{2007-KoelblBurch.etal,
  author = {Alfred K{\"{o}}lbl and Jerry R. Burch and Carl Pixley},
  title = {Memory Modeling in {ESL-RTL} Equivalence Checking},
  booktitle = {Proc. Design Automation Conference ({DAC})},
  year = {2007},
  pages = {205--209},
  address = {San Diego, CA, USA},
  month = {June},
  owner = {stoffel},
  timestamp = {2016.05.10}
}

@INPROCEEDINGS{2009-KoelblJacoby.etal,
  author = {K{\"o}lbl, A. and Jacoby, R. and Jain, H. and Pixley, C.},
  title = {Solver technology for system-level to {RTL} equivalence checking},
  booktitle = {Proc. Design, Automation Test in Europe ({DATE})},
  year = {2009},
  pages = {196-201},
  month = {April},
  file = {:./files/2009-KoelblJacoby.etal.pdf:PDF}
}

@ARTICLE{2005-KoelblPixley,
  author = {Alfred K{\"o}lbl and Carl Pixley},
  title = {Constructing Efficient Formal Models from High-Level Descriptions
	Using Symbolic Simulation},
  journal = {International Journal of Parallel Programming},
  year = {2005},
  volume = {33},
  pages = {645--666},
  number = {6},
  month = {dec},
  acmid = {1146110},
  address = {Norwell, MA, USA},
  file = {:./files/2005-KoelblPixley.pdf:PDF},
  issn = {0885-7458},
  issue_date = {December 2005},
  keywords = {data-flow-graph, high-level model, symbolic simulation},
  numpages = {22},
  publisher = {Kluwer Academic Publishers},
  timestamp = {2006.10.04}
}

@INPROCEEDINGS{2010-KuehneBeyer.etal,
  author = {U. {K\"{u}hne} and S. {Beyer} and J. {Bormann} and J. {Barstow}},
  title = {{Automated formal verification of processors based on architectural
	models}},
  booktitle = {Proc. of Conference on FMCAD},
  year = {2010},
  pages = {129--136},
  acmid = {1998521},
  file = {2010-KuehneBeyer.etal.pdf:files/2010-KuehneBeyer.etal.pdf:PDF},
  numpages = {8},
  owner = {villarraga},
  timestamp = {2012.09.12}
}

@INPROCEEDINGS{2002-KaestnerWilhelm,
  author = {Daniel Kaestner and Stephan Wilhelm},
  title = {Generic Control Flow Reconstruction from Assembly Code},
  booktitle = {Proc. Joint Conference on Languages, compilers and tools for embedded
	systems: software and compilers for embedded systems},
  year = {2002},
  pages = {46 - 55},
  file = {:./files/2002-KaestnerWilhelm.pdf:PDF},
  timestamp = {2006.09.22}
}

@MISC{1996-Kahan,
  author = {W. Kahan},
  title = {{IEEE} Standard 754 for Binary Floating-Point Arithmetic},
  howpublished = {Lecture Notes},
  month = {May},
  year = {1996},
  file = {:./files/1996-Kahan.pdf:PDF},
  owner = {loitz},
  timestamp = {2007.01.08}
}

@INPROCEEDINGS{2009-KaivolaGhughal.etal,
  author = {Kaivola, Roope and Ghughal, Rajnish and Narasimhan, Naren and Telfer,
	Amber and Whittemore, Jesse and Pandav, Sudhindra and Slobodov\'{a},
	Anna and Taylor, Christopher and Frolov, Vladimir and Reeber, Erik
	and Naik, Armaghan},
  title = {Replacing Testing with Formal Verification in Intel CoreTM I7 Processor
	Execution Engine Validation},
  booktitle = {Proceedings of the 21st International Conference on Computer Aided
	Verification},
  year = {2009},
  series = {CAV '09},
  pages = {414--429},
  address = {Berlin, Heidelberg},
  publisher = {Springer-Verlag},
  acmid = {1575095},
  isbn = {978-3-642-02657-7},
  location = {Grenoble, France},
  numpages = {16},
  owner = {villarraga},
  timestamp = {2016.04.27}
}

@BOOK{1986-Kalmanson,
  title = {Discrete Mathematics and its Applications},
  publisher = {Addison-Wesley},
  year = {1986},
  author = {K. Kalmanson}
}

@ARTICLE{2006-KangGaudiot,
  author = {J.-Y. Kang and J.-L. Gaudiot},
  title = {A Simple High-Speed Multiplier Design},
  journal = {{IEEE} Transactions on Computers},
  year = {2006},
  volume = {C-55},
  pages = {1253-1258},
  number = {10},
  month = {October},
  file = {:./files/2006-KangGaudiot.pdf:PDF}
}

@ARTICLE{2007-KannoMizuno.etal,
  author = {Y. Kanno and H. Mizuno and Y. Yasu and K. Hirose and Y. Shimazaki
	and T. Hoshi and Y. Miyairi and T. Ishii and T. Yamada and T. Irita
	and T. Hattori and K. Yanagisawa and N. Irie},
  title = {Hierarchical Power Distribution With Power Tree in Dozens of Power
	Domains for 90-nm Low-Power Multi-CPU SoCs},
  journal = {IEEE Journal of Solid-State Circuits},
  year = {2007},
  volume = {42},
  pages = {74-83},
  issn = {0018-9200},
  owner = {udupi},
  timestamp = {2018.08.31}
}

@ARTICLE{1999-KapadiaBenini.etal,
  author = {H. Kapadia and L. Benini and G. De Micheli},
  title = {Reducing switching activity on datapath buses with control-signal
	gating},
  journal = {{IEEE} J. Solid-State Circuits},
  year = {1999},
  volume = {34},
  pages = {405--414},
  number = {3},
  month = {Mar}
}

@ARTICLE{1996-KarriHogstedt.etal,
  author = {Karri, R. and Hogstedt, K. and Orailoglu, A.},
  title = {Computer Aided Design Of Fault Tolerant {VLSI} Systems},
  journal = {Design Test of Computers, {IEEE}},
  year = {1996},
  volume = {13},
  pages = {88 -96},
  number = {3},
  month = {fall},
  file = {:./files/1996-KarriHogstedt.etal.pdf:PDF},
  issn = {0740-7475},
  keywords = {CAD framework;automated synthesis of ICs;computer-aided design;enhanced
	reliability;fault-tolerant VLSI;fault-tolerant VLSI circuit;self-recovery;fault
	tolerant computing;logic CAD;very high speed integrated circuits;}
}

@INPROCEEDINGS{2014-ScheiblerBecker.etal,
  author = {Karsten Scheibler, Bernd Becker},
  title = {Implication Graph Compression inside the SMT Solver iSAT3},
  booktitle = {17. {GI/ITG/GMM} Workshop Methoden und Beschreibungssprachen zur
	Modellierung und Verifikation von Schaltungen und Systemen ({MBMV})},
  year = {2014},
  pages = {25-36},
  owner = {bschmidt},
  timestamp = {2014.01.20}
}

@INPROCEEDINGS{2005-KaruriKraemer.etal,
  author = {Kingshuk Karuri and Mohammad Abdullah Al Faruque and Stefan Kraemer
	and Rainer Leupers and Gerd Ascheid and Heinrich Meyr},
  title = {Fine-Grained Application Source Code Profiling for {ASIP} Design},
  booktitle = {Proc. Annual Conference on Design Automation},
  year = {2005},
  pages = { 329 - 334},
  file = {:./files/2005-KaruriKraemer.etal.pdf:PDF},
  keywords = { ASIP design; application source code profiling; application specific
	instruction set processor; architecture description languages; code
	instrumentation technology; instruction set architecture; instruction-level
	profilers; iterative architecture exploration; microprofiling approach;
	pre-architecture exploration tools; retargetable software development
	tools; source-level profilers; application specific integrated circuits;
	hardware description languages; hardware-software codesign; instruction
	sets; integrated circuit design; microprocessor chips;},
  owner = {loitz},
  review = {Paper on Profiling Source Code for timing analysis for ASIP Deisign.
	ASIP Design for RealTime.},
  timestamp = {2007.01.08}
}

@INPROCEEDINGS{2006-KaruriLeupers.etal,
  author = {Kingshuk Karuri and Rainer Leupers and Gerd Ascheid and Heinrich
	Meyr and Monu Kedia},
  title = {Design and Implementation of a Modular and Portable IEEE 754 Compliant
	Floating-Point Unit},
  booktitle = {Proc. International Conference on Design, Automation and Test in
	Europe ({DATE})},
  year = {2006},
  volume = {2},
  pages = {1 -6},
  file = {:./files/2006-KaruriLeupers.etal.pdf:PDF},
  owner = {loitz},
  timestamp = {2007.01.08}
}

@INPROCEEDINGS{2011-KatebiSakallah.etal,
  author = {Katebi, Hadi and Sakallah, Karem A. and Marques-Silva, Joao P.},
  title = {Empirical Study of the Anatomy of Modern Sat Solvers},
  booktitle = {Proceedings of the 14th International Conference on Theory and Application
	of Satisfiability Testing},
  year = {2011},
  series = {SAT'11},
  pages = {343--356},
  address = {Berlin, Heidelberg},
  publisher = {Springer-Verlag},
  acmid = {2023510},
  isbn = {978-3-642-21580-3},
  location = {Ann Arbor, MI},
  numpages = {14}
}

@BOOK{1994-Katz,
  title = {Contemporary Logic Design},
  publisher = {Benjamin/Cummings},
  year = {1994},
  author = {R. Katz}
}

@INPROCEEDINGS{1999-KatzSagi.etal,
  author = {Katz, Sagi and Grumberg, Orna and Geist, Daniel},
  title = {"Have I written enough Properties?" - A Method of Comparison between
	Specification and Implementation},
  booktitle = {Proc. Advanced Research Working Conference on Correct Hardware Design
	and Verification Methods ({CHARME})},
  year = {1999},
  pages = {280--297},
  address = {London, UK},
  publisher = {Springer-Verlag},
  file = {:./files/1999-KatzSagi.etal.pdf:PDF},
  isbn = {3-540-66559-5},
  owner = {Wedler}
}

@INPROCEEDINGS{1998-KaufmannMartin.etal,
  author = {M. Kaufmann and A. Martin and C. Pixly},
  title = {Design Constraints In Symbolic Model Checking},
  booktitle = {Proc. International Conference on Computer Aided Verification ({CAV})},
  year = {1998},
  pages = {477--487},
  address = {London, UK, UK},
  publisher = {Springer-Verlag},
  acmid = {733768},
  file = {:./files/1998-KaufmannMartin.etal.pdf:PDF},
  isbn = {3-540-64608-6},
  numpages = {11},
  timestamp = {2006.09.19}
}

@INPROCEEDINGS{2013-KaushikPatel,
  author = {A. Kaushik and H. D. Patel},
  title = {{SystemC}-{Clang}: An open-source framework for analyzing mixed-abstraction
	{SystemC} models},
  booktitle = {Forum on Specification \& Design Languages ({FDL})},
  year = {2013},
  pages = {1-8},
  month = {Sept},
  file = {:files/2013-KaushikPatel.pdf:PDF},
  issn = {1636-9874},
  keywords = {Analytical models;Computational modeling;Data mining;Open source software;Payloads;Ports
	(Computers);Sockets;Design automation;Design methodology;Open source
	software}
}

@INPROCEEDINGS{1992-KebschullSchubert.etal,
  author = {U. Kebschull and E. Schubert and W. Rostenstiel},
  title = {Multi-Level Logic Based on Functional Decision Diagrams},
  booktitle = {Proc. European Design Automation Conference (EDAC)},
  year = {1992},
  pages = {43 -47},
  file = {:./files/1992-KebschullSchubert.etal.pdf:PDF},
  keywords = { Berkley Logic Interchange Format; {Boolean} function representation;
	Reed-Muller Expansion; Reed-Muller Transformation; data structure;
	functional decision diagrams; multilevel logic; {Boolean} functions;
	data structures; logic CAD; many-valued logics;}
}

@ARTICLE{2003-KeimDrechsler.etal,
  author = {Martin Keim and Rolf Drechsler and Bernd Becker and Michael Martin
	and Paul Molitor},
  title = {Polynomial Formal Verification of Multipliers},
  journal = {Formal Methods in System Design},
  year = {2003},
  volume = {22},
  pages = {39-58},
  number = {1},
  bibsource = {DBLP, http://dblp.uni-trier.de},
  file = {:./files/2003-KeimDrechsler.etal.pdf},
  owner = {pavlenko},
  timestamp = {2011.06.03}
}

@BOOK{1976-KemenySnell,
  title = {Finite Markov Chains},
  publisher = {Springer-Verlag},
  year = {1976},
  author = {John G. Kemeny and J. Laurie Snell},
  address = {New York},
  file = {:./files/1976-KemenySnell.pdf:PDF}
}

@MISC{2004-Kenney,
  author = {Jim Kenney},
  title = {Optimizing the Design and Verification of Embedded Systems},
  year = {2004},
  file = {:./files/2004-Kenney.pdf:PDF},
  owner = {stoffel},
  timestamp = {2006.09.27}
}

@ARTICLE{2005-KenneySchulte,
  author = {Robert D. Kenney and Michael J. Schulte},
  title = {High-Speed Multioperand Decimal Adders},
  journal = {IEEE Transaction on Computers},
  year = {2005},
  volume = {54},
  pages = {953-963},
  file = {:./files/2005-KenneySchulte.pdf:PDF},
  timestamp = {2006.10.04}
}

@BOOK{2012-Kesel,
  title = {Modellierung von digitalen Systemen mit SystemC: Von der RTL- zur
	Transaction-Level-Modellierung},
  publisher = {De Gruyter},
  year = {2012},
  author = {Kesel, F.},
  isbn = {9783486718959}
}

@INPROCEEDINGS{2007-KillianAnderson.etal,
  author = {Killian, Charles and Anderson, James W. and Jhala, Ranjit and Vahdat,
	Amin},
  title = {Life, death, and the critical transition: finding liveness bugs in
	systems code},
  booktitle = {Proceedings of the 4th {USENIX} {C}onference on {N}etworked {S}ystems
	{D}esign \& {I}mplementation},
  year = {2007},
  series = {NSDI'07},
  pages = {18--18},
  address = {Berkeley, CA, USA},
  publisher = {USENIX Association},
  acmid = {1973448},
  file = {2007-KillianAnderson.etal.pdf:files/2007-KillianAnderson.etal.pdf:PDF},
  location = {Cambridge, MA},
  numpages = {1},
  owner = {villarraga},
  timestamp = {2012.08.27}
}

@INPROCEEDINGS{2005-KimHa,
  author = {Dohyung Kim and Soonhoi Ha},
  title = {Static Analysis and Automatic Code Syntesis of flexible {FSM} Model},
  booktitle = {Design Automation Conference, 2005. Proceedings of the {ASP-DAC}
	2005. Asia and South Pacific},
  year = {2005},
  volume = {1},
  pages = { 161 - 165},
  month = {jan.},
  file = {:./files/2005-KimHa.pdf:PDF},
  keywords = { automatic code synthesis; codesign environment; complex control modules;
	finite state machine; flexible FSM model; formal property; software-hardware
	synthesis; state variable; static analysis; static analyzability;
	concurrency control; finite state machines; hardware-software codesign;
	program diagnostics;}
}

@ARTICLE{1976-King,
  author = {King, James C.},
  title = {Symbolic execution and program testing},
  journal = {Commun. ACM},
  year = {1976},
  volume = {19},
  pages = {385--394},
  number = {7},
  month = jul,
  address = {New York, NY, USA},
  file = {:files/1976-King.pdf:PDF},
  issn = {0001-0782},
  issue_date = {July 1976},
  keywords = {program debugging, program proving, program testing, program verification,
	symbolic execution, symbolic interpretation},
  numpages = {10},
  publisher = {ACM},
  timestamp = {2013.11.12}
}

@MISC{2003-KirnerPuschner,
  author = {Raimund Kirner and Peter Puschner},
  title = {A Simple and Effective Fully Automatic Worst-Case Execution Time
	Analysis for Model-Based Application Development},
  year = {2003},
  file = {:./files/2003-KirnerPuschner.pdf:PDF},
  institution = {Technische Universit�t Wien},
  owner = {stoffel},
  timestamp = {2016.05.10}
}

@INPROCEEDINGS{2003-Klein,
  author = {Russell Klein},
  title = {Hardware/Software Co-Verification},
  booktitle = {Embedded Systems Conference 2003},
  year = {2003},
  file = {:./files/2003-Klein.pdf:PDF},
  timestamp = {2006.09.27}
}

@INPROCEEDINGS{1996-Klein,
  author = {Russel Klein},
  title = {Miami A Hardware Software Cosimulation Environment},
  booktitle = {Proc. {IEEE} on Rapid System Prototyping},
  year = {1996},
  pages = {173 -177},
  file = {:./files/1996-Klein.pdf:PDF},
  keywords = {Miami;design complexity;dynamic partitioning;event driven hardware
	simulator;hardware software co-simulation;system validation;discrete
	event simulation;logic CAD;programming environments;software prototyping;},
  timestamp = {2006.09.27}
}

@INPROCEEDINGS{1997-Knorz,
  author = {Hans Knorz},
  title = {A Fast and Great Algorithm for Waiting},
  booktitle = {Proc. International Conference on Waiting Queues},
  year = {1997},
  pages = {123-127},
  month = {November}
}

@PHDTHESIS{2004a-Koch,
  author = {Thorsten Koch},
  title = {Rapid Mathematical Prototyping},
  school = {Technische Universit{\"a}t Berlin},
  year = {2004},
  type = {Dissertation}
}

@ARTICLE{2004-Koch,
  author = {Thorsten Koch},
  title = {The Final {NETLIB-LP} Results},
  journal = {Operations Research Letters},
  year = {2004},
  volume = {32},
  pages = {138-142},
  file = {:./files/2004-Koch.pdf:PDF},
  issue = {2},
  language = {English},
  publisher = {Elsevier / North-Holland}
}

@TECHREPORT{2001-Koch,
  author = {Thorsten Koch},
  title = {Zimpl User Guide},
  institution = {Zuse Institute Berlin},
  year = {2001},
  number = {01-20},
  file = {:./files/2001-Koch.pdf:PDF},
  url = {http://www.zib.de/koch/zimpl}
}

@ARTICLE{1998-KochMartin,
  author = {Thorsten Koch and Alexander Martin},
  title = {Solving {Steiner} Tree Problems in Graphs to Optimality},
  journal = {Networks},
  year = {1998},
  volume = {32},
  pages = {207-232},
  note = {ZIB-Report SC 96-42},
  file = {:./files/1998-KochMartin.pdf:PDF},
  language = {English}
}

@ARTICLE{2018-KocherGenkin.etal,
  author = {Kocher, Paul and Genkin, Daniel and Gruss, Daniel and Haas, Werner
	and Hamburg, Mike and Lipp, Moritz and Mangard, Stefan and Prescher,
	Thomas and Schwarz, Michael and Yarom, Yuval},
  title = {Spectre attacks: Exploiting speculative execution},
  journal = {arXiv preprint arXiv:1801.01203},
  year = {2018},
  owner = {fadiheh},
  timestamp = {2018.07.12}
}

@INPROCEEDINGS{2014-KoestersGoryachev,
  author = {Johannes Koesters and Alex Goryachev},
  title = {Verification of Non-Mainline Functions in Today's Processor Chips},
  booktitle = {Proceedings International Design Automation Conference ({DAC})},
  year = {2014},
  series = {DAC'14},
  pages = {1:1--1:3},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {2596693},
  articleno = {1},
  file = {:files/2014-KoestersGoryachev.pdf:PDF},
  isbn = {978-1-4503-2730-5},
  location = {San Francisco, CA, USA},
  numpages = {3}
}

@BOOK{1978-Kohavi,
  title = {Switching and Finite Automata Theory},
  publisher = {McGraw-Hill},
  year = {1978},
  author = {Z. Kohavi},
  file = {:./files/1978-Kohavi.pdf:PDF}
}

@MASTERSTHESIS{2011-EmileKommegne,
  author = {Emile Kommegne},
  title = {Effiziente Generierung des Exekution Graphs},
  school = {TU Kaiserslautern},
  year = {2011},
  type = {{Studienarbeit}},
  file = {:files/2011-EmileKommegne.pdf:PDF},
  owner = {bschmidt},
  timestamp = {2013.12.20}
}

@INPROCEEDINGS{2008-KongAciicmez.etal,
  author = {Kong, Jingfei and Aciicmez, Onur and Seifert, Jean-Pierre and Zhou,
	Huiyang},
  title = {Deconstructing new cache designs for thwarting software cache-based
	side channel attacks},
  booktitle = {Proceedings of the 2nd ACM workshop on Computer security architectures},
  year = {2008},
  pages = {25--34},
  organization = {ACM},
  owner = {fadiheh},
  timestamp = {2018.07.12}
}

@INPROCEEDINGS{2014-KooliNatale,
  author = {M. Kooli and G. Di Natale},
  title = {A survey on simulation-based fault injection tools for complex systems},
  booktitle = {9th IEEE International Conference on Design Technology of Integrated
	Systems in Nanoscale Era (DTIS)},
  year = {2014},
  pages = {1-6},
  month = {May},
  file = {2014-KooliNatale.pdf:files/2014-KooliNatale.pdf:PDF},
  owner = {bartsch},
  timestamp = {2016.11.28}
}

@INPROCEEDINGS{2002-KopfermanVardi,
  author = {O. Kopferman and M.Y. Vardi},
  title = {On Bound Specification},
  year = {2002},
  file = {:./files/2002-KopfermanVardi.pdf:PDF},
  timestamp = {2006.09.21}
}

@BOOK{1998-Koren,
  title = {Computer Arithmetic Algorithms},
  publisher = {Brooside Court Publishers},
  year = {1998},
  author = {I. Koren}
}

@INPROCEEDINGS{2005-KouroussisFerzli.etal,
  author = {Dionysios Kouroussis and Imad A. Ferzli and Farid N. Najm},
  title = {Incremental Partitioning-Based Vectorless Power Grid Verification},
  booktitle = {Proc. International Conference on Computer-Aided Design (ICCAD)},
  year = {2005},
  pages = { 358 - 364},
  file = {:./files/2005-KouroussisFerzli.etal.pdf:PDF},
  keywords = { abstracted current constraints; black box macromodels; design verification;
	incremental design analysis; incremental partitioning; linear program;
	local power grid sections; vectorless power grid verification; worst-case
	voltage drop; electric potential; integrated circuit design; integrated
	circuit modelling; power supply circuits;},
  timestamp = {2006.09.27}
}

@INPROCEEDINGS{2008-KrautzJacobi.etal,
  author = {U. Krautz and C. Jacobi and K. Weber and M. Pflanz and W. Kunz and
	M. Wedler},
  title = {Verifying full-custom multipliers by {Boolean} equivalence checking
	and an arithmetic bit level proof},
  booktitle = {{ASP-DAC} '08: Proceedings of the 2008 conference on Asia and South
	Pacific design automation},
  year = {2008},
  pages = {398--403},
  address = {Los Alamitos, CA, USA},
  publisher = {IEEE Computer Society Press},
  file = {:./files/2008-KrautzJacobi.etal.pdf:PDF},
  isbn = {978-1-4244-1922-7},
  location = {Seoul, Korea}
}

@MISC{web-mkjpeg,
  author = {Krepa,Michal},
  title = {{EV}\_{JPEG}\_{ENC} {IP} Core},
  howpublished = {http://opencores.org/project,mkjpeg},
  key = {mkjpeg},
  owner = {fehmel},
  timestamp = {2017.04.23}
}

@ARTICLE{1963-Kripke,
  author = {Kripke, Saul A.},
  title = {Semantical Analysis of Modal Logic {I} Normal Modal Propositional
	Calculi},
  journal = {Mathematical Logic Quarterly},
  year = {1963},
  volume = {9},
  pages = {67--96},
  number = {5-6},
  issn = {1521-3870},
  owner = {villarraga},
  publisher = {WILEY-VCH Verlag Berlin GmbH},
  timestamp = {2016.07.13}
}

@ARTICLE{1959-Kripke,
  author = {Saul A. Kripke},
  title = {A Completeness Theorem in Modal Logic},
  journal = {The Journal of Symbolic Logic},
  year = {1959},
  volume = {24},
  pages = {1-14},
  number = {1},
  issn = {00224812},
  owner = {villarraga},
  publisher = {Association for Symbolic Logic},
  timestamp = {2016.06.29},
  url = {http://www.jstor.org/stable/2964568}
}

@PHDTHESIS{2001-Kroening,
  author = {Kroening, Daniel},
  title = {Formal Verification of Pipelined Microprocessors},
  school = {Saarland University},
  year = {2001},
  file = {:./files/2001-Kroening.pdf:PDF},
  owner = {wedler},
  timestamp = {2007.08.31},
  url = {http://www-wjp.cs.uni-sb.de/publikationen/Kr01.pdf}
}

@INPROCEEDINGS{2004-KroeningGroce.etal,
  author = {Daniel Kroening and Alex Groce and Edmund Clarke},
  title = {Counterexample-Guided Abstraction Refinement via Program Execution},
  booktitle = {Proc. International Conference on Formal Engineering Methods ({ICFEM})},
  year = {2004},
  number = {3308},
  series = {Lecture Notes in Computer Science},
  pages = {224--238},
  publisher = {Springer},
  file = {:./files/2004-KroeningGroce.etal.pdf:PDF},
  owner = {stoffel},
  timestamp = {2011.11.21}
}

@INPROCEEDINGS{2007-KroeningSeshia,
  author = {D. Kroening and S. A. Seshia},
  title = {Formal Verification at Higher Levels of Abstraction},
  booktitle = {Proc. International Conference on Computer-Aided Design (ICCAD)},
  year = {2007},
  owner = {wedler},
  timestamp = {2007.11.14},
  url = {http://eis.eit.uni-kl.de/local/dl/iccad25/PAPERS/2007/PDFFILES/08B_1.PDF}
}

@ARTICLE{2005-KroeningSharygina,
  author = {Daniel Kroening and Natasha Sharygina},
  title = {Formal Verification of {SystemC} by Automatic Hardware/Software Partitioning},
  journal = {Formal Methods and Models for Co-Design},
  year = {2005},
  pages = { 101 - 110},
  file = {:./files/2005-KroeningSharygina.pdf:PDF},
  keywords = { SystemC program; automatic hardware partitioning; automatic software
	partitioning; formal verification; general-purpose programming languages;
	monolithic approach; system-level languages; formal specification;
	formal verification; hardware description languages; hardware-software
	codesign; logic partitioning;},
  timestamp = {2006.09.27}
}

@BOOK{2008-KroeningOfer,
  title = {Decision Procedures: An Algorithmic Point of View},
  publisher = {Springer Publishing Company, Incorporated},
  year = {2008},
  author = {Kroening, Daniel and Strichman, Ofer},
  edition = {1},
  isbn = {3540741046, 9783540741046},
  owner = {pavlenko},
  timestamp = {2010.11.29}
}

@INPROCEEDINGS{2007-Kropf,
  author = {Kropf, Thomas},
  title = {Software Bugs Seen from an Industrial Perspective or Can Formal Methods
	Help on Automotive Software Development?},
  booktitle = {Proceedings of the 19th International Conference on Computer Aided
	Verification},
  year = {2007},
  series = {CAV'07},
  pages = {3--3},
  address = {Berlin, Heidelberg},
  publisher = {Springer-Verlag},
  acmid = {1770355},
  file = {2007-Kropf.pdf:files/2007-Kropf.pdf:PDF},
  isbn = {978-3-540-73367-6},
  location = {Berlin, Germany},
  numpages = {1},
  owner = {villarraga},
  timestamp = {2016.06.17}
}

@INPROCEEDINGS{1991-KropfWunderlich,
  author = {T. Kropf and H. Wunderlich},
  title = {A Common Approach to Test Generation and Hardware Verification Based
	on Temporal Logic},
  booktitle = {Proc. International Test Conference ({ITC})},
  year = {1991},
  pages = {57-66},
  file = {:./files/1991-KropfWunderlich.pdf:PDF}
}

@INPROCEEDINGS{2002-KuboFujita,
  author = {Kubo, M. and Fujita, M.},
  title = {Debug methodology for arithmetic circuits on {FPGAs}},
  year = {2002},
  pages = { 236 - 242},
  month = {dec.},
  file = {:./files/2002-KuboFujita.pdf:PDF},
  journal = {Field-Programmable Technology, 2002. ({FPT}). Proceedings. 2002 {IEEE}
	International Conference on},
  owner = {pavlenko},
  timestamp = {2010.10.15}
}

@INPROCEEDINGS{2001-KuehlmannBaumgartner,
  author = {A. Kuehlmann and J. Baumgartner},
  title = {Transformation-Based Verification Using Generalized Retiming.},
  booktitle = {Proc. International Conference Computer Aided Verification ({CAV})},
  year = {2001},
  pages = {104-117},
  month = {July},
  file = {:./files/2001-KuehlmannBaumgartner.pdf:PDF}
}

@INPROCEEDINGS{2001-KuehlmannGanai.etal,
  author = {Andreas Kuehlmann and Malay K. Ganai and Viresh Paruthi},
  title = {Circuit-based {Boolean} Reasoning},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {2001},
  pages = {232--237},
  address = {New York, NY, USA},
  publisher = {ACM},
  file = {:./files/2001-KuehlmannGanai.etal.pdf:PDF},
  isbn = {1-58113-297-2},
  location = {Las Vegas, Nevada, United States}
}

@INPROCEEDINGS{1997-KuehlmannKrohm,
  author = {Andreas Kuehlmann and Florian Krohm},
  title = {Equivalence Checking Using Cuts and Heaps},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {1997},
  pages = {263-268},
  month = {November},
  file = {:./files/1997-KuehlmannKrohm.pdf:PDF}
}

@INPROCEEDINGS{1994-KungSuchak.etal,
  author = {D. Kung and N. Suchak and J. Gao and P. Hsia and Y. Toyoshima and
	C. Chen},
  title = {On object state testing},
  booktitle = {roceedings Eighteenth Annual International Computer Software and
	Applications Conference (COMPSAC 94)},
  year = {1994},
  owner = {fehmel},
  timestamp = {2019.05.27}
}

@MISC{DFG-1051,
  author = {Wolfgang Kunz},
  title = {Formale Verifikation Firmware-basierter System-on-Chip-Module},
  howpublished = {Projekt der Deutschen Forschungsgemeinschaft, F\"{o}rderkennzeichen
	KU 1051/8-1},
  owner = {stoffel},
  timestamp = {2014.07.31}
}

@INPROCEEDINGS{1993-Kunz,
  author = {W. Kunz},
  title = {{HANNIBAL}: An Efficient Tool for Logic Verification Based on Recursive
	Learning},
  booktitle = {Proc. International Conference on Computer-Aided Design (ICCAD)},
  year = {1993},
  pages = {538-543},
  month = {November},
  file = {:./files/1993-Kunz.pdf:PDF},
  keywords = { HANNIBAL; Sparc Workstation ELC; c6288; c6288nr; combinational circuits;
	expert systems; internal equivalencies; logic verification; multiplier;
	recursive learning; redundancy-free version; verification tools;
	learning (artificial intelligence);}
}

@INPROCEEDINGS{1994-KunzMenon,
  author = {W. Kunz and Prem Menon},
  title = {Multi-Level Logic Optimization by Implication Analysis},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {1994},
  series = {San Jose},
  pages = {6-13},
  month = {November},
  file = {:./files/1994-KunzMenon.pdf:PDF}
}

@PERIODICAL{2008-KunzNguyen,
  title = {Control Flow Analysis for hardware/software verification framework},
  year = {2008},
  series = {Verisoft-{XT} Milestone},
  author = {Wolfgang Kunz and Minh D. Nguyen},
  owner = {stoffel},
  timestamp = {2010.10.29}
}

@ARTICLE{1994-KunzPradhan,
  author = {W. Kunz and D. Pradhan},
  title = {Recursive Learning: A New Implication Technique for Efficient Solutions
	to {CAD} Problems: Test, Verification and Optimization},
  journal = {{IEEE} Transactions on Computer-Aided Design},
  year = {1994},
  volume = {13},
  pages = {1143-1158},
  month = {September},
  file = {:./files/1994-KunzPradhan.pdf:PDF}
}

@BOOK{1997-KunzStoffel,
  title = {Reasoning in {Boolean} Networks - Logic Synthesis and Verification
	Using Testing Techniques},
  publisher = {Kluwer Academic Publishers},
  year = {1997},
  author = {W. Kunz and D. Stoffel},
  address = {Boston}
}

@ARTICLE{1997-KunzStoffel.etal,
  author = {W. Kunz and D. Stoffel and Prem Menon},
  title = {Multi-Level Logic Optimization and Equivalence Checking by Implication
	Analysis},
  journal = {{IEEE} Transactions on Computer-Aided Design},
  year = {1997},
  volume = {16},
  pages = {266-281},
  number = {3},
  month = {March},
  file = {:./files/1997-KunzStoffel.etal.pdf:PDF}
}

@INPROCEEDINGS{2008-MinKuoWeng.etal,
  author = {Yu-Min Kuo and Shih-Hung Weng and Shih-Chieh Chang},
  title = {A novel sequential circuit optimization with clock gating logic},
  booktitle = {2008 IEEE/ACM International Conference on Computer-Aided Design},
  year = {2008},
  pages = {230-233},
  month = {Nov},
  issn = {1092-3152},
  keywords = {flip-flops;optimisation;sequential circuits;clock gating logic;flip-flop;iterative
	optimization;next-state function;sequential circuit optimization;timing;Character
	generation;Clocks;Counting circuits;Energy consumption;Flip-flops;Inverters;Latches;Pulse
	circuits;Sequential circuits;Timing}
}

@ARTICLE{2011-KupferschmidLewis.etal,
  author = {Kupferschmid, Stefan and Lewis, Matthew and Schubert, Tobias and
	Becker, Bernd},
  title = {Incremental preprocessing methods for use in BMC},
  journal = {Formal Methods in System Design},
  year = {2011},
  volume = {39},
  pages = {185 - 204},
  number = {2},
  file = {:files/2011-KupferschmidLewis.etal.pdf:PDF},
  owner = {bartsch},
  timestamp = {2014.08.21},
  url = {http://link.springer.com/article/10.1007%2Fs10703-011-0122-4}
}

@INPROCEEDINGS{1997-KurshanLevin.etal,
  author = {R. Kurshan and V. Levin and M. Minea and D. Peled and H. Yeniguen},
  title = {Verifying Hardware in its Software Context},
  booktitle = {Proc. IEEE/ACM International Conference on Computer-Aided Design},
  year = {1997},
  pages = {742 -749},
  file = {:./files/1997-KurshanLevin.etal.pdf:PDF},
  keywords = {asynchronous abstraction;computational complexity;correct behaviour;hardware
	verification;hardware/software co-design;interface verification problem;localization
	reduction;partial order reduction;purely synchronous models;reduced
	transformed model;software context;software interface;software model;symbolic
	model checking;synchronous RTL model;synchronous transformation;transition
	relation;verification algorithm;computational complexity;formal verification;hardware
	description languages;high level synthesis;program verification;},
  timestamp = {2006.09.27}
}

@ARTICLE{1991-KurshanMcMillan,
  author = {R.P. Kurshan and K.L. McMillan},
  title = {Analysis of Digital Circuits Through Symbolic Reduction},
  journal = {IEEE Transactions on Computer-Aided Design},
  year = {1991},
  volume = {10},
  pages = {1356 -1371},
  number = {11},
  month = {October},
  file = {:./files/1991-KurshanMcMillan.pdf:PDF},
  keywords = { omega;-automata;analog circuit-level model;behavior preserving;digital
	circuits;finite-state models;homomorphic transformations;model extraction;semi-algorithmic
	method;symbolic reduction;verification;circuit analysis computing;digital
	circuits;}
}

@BOOK{1994-Kurshan,
  title = {Computer-Aided Verification of Coordinating Processes -- The Automata-Theoretic
	Approach},
  publisher = {Princeton University Press},
  year = {1994},
  author = {R. P. Kurshan},
  address = {Princeton, New Jersey}
}

@ARTICLE{2002-KurshanLevin.etal,
  author = {Robert P. Kurshan and Vladimir Levin and Marius Minea and Doron Peled
	and Husnu Yenigun},
  title = {Combining Software and Hardware Verification Techniques},
  journal = {Formal Methods in System Design},
  year = {2002},
  volume = {21},
  pages = {251 - 280},
  file = {:./files/2002-KurshanLevin.etal.pdf:PDF},
  timestamp = {2006.09.27}
}

@INPROCEEDINGS{1995-LaiSastry,
  author = {Yung-Te Lai and Sarama Sastry},
  title = {Edge-Valued Binary Decision Diagrams for Multi-Level Hierarchical
	Verification},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {1995},
  pages = {254-260},
  file = {:./files/1995-LaiSastry.pdf:PDF}
}

@INPROCEEDINGS{2000-LajoloRebaudengo.etal,
  author = {M. Lajolo and M. Rebaudengo and M. Sonza Reorda and M. Violante and
	L. Lavagno},
  title = {Evaluating System Dependability in a Co-Design Framework},
  booktitle = {Proc. International Conference on Design, Automation and Test in
	Europe ({DATE})},
  year = {2000},
  pages = {586 -590},
  file = {:./files/2000-LajoloRebaudengo.etal.pdf:PDF},
  keywords = {co-design framework;codesign tool;embedded microprocessor-based systems;fault
	injection techniques;safety critical applications;system dependability
	evaluation;embedded systems;fault simulation;fault tolerant computing;hardware-software
	codesign;safety-critical software;},
  timestamp = {2006.09.14}
}

@INPROCEEDINGS{2009-LangerHeinkel,
  author = {Jan Langer and Ulrich Heinkel},
  title = {High Level Synthesis Using Operation Properties},
  booktitle = {Proc. of Forum on Specification Design Languages ({FDL} 2009)},
  year = {2009},
  pages = {1-6},
  month = {Sep.},
  file = {:./files/2009-LangerHeinkel.pdf:PDF},
  owner = {stoffel},
  timestamp = {2012.03.26}
}

@INPROCEEDINGS{2015-LanikLegriel.etal,
  author = {J. Lanik and J. Legriel and E. Piriou and E. Viaud and F. Rahim and
	O. Maler and S. Rahim},
  title = {Reducing power with activity trigger analysis},
  booktitle = {2015 ACM/IEEE International Conference on Formal Methods and Models
	for Codesign (MEMOCODE)},
  year = {2015},
  owner = {udupi},
  timestamp = {2018.08.02}
}

@INPROCEEDINGS{1990-Larrabee,
  author = {Tracy Larrabee},
  title = {Efficient Generation of Test Patterns Using {Boolean} Satisfiability},
  booktitle = {IEEE Trans. on CAD},
  year = {1990},
  pages = {795--801},
  file = {:./files/1990-Larrabee.pdf:PDF}
}

@INPROCEEDINGS{2007-LarssonHaehnle,
  author = {Daniel Larsson and Reiner Haehnle},
  title = {Symbolic Fault Injection},
  booktitle = {Proc. 4th International Verification Workshop (Verify) in connection
	with CADE-21},
  year = {2007},
  volume = {259},
  pages = {85 - 103},
  file = {2007-LarssonHaehnle.pdf:files/2007-LarssonHaehnle.pdf:PDF},
  owner = {bartsch},
  timestamp = {2015.08.03}
}

@ARTICLE{1964-Lawler,
  author = {Eugene L. Lawler},
  title = {An Approach to Multilevel {Boolean} Minimization},
  journal = {Journal of The Association for Computing Machinery},
  year = {1964},
  volume = {11},
  pages = {283-295},
  number = {3},
  month = {July},
  file = {:./files/1964-Lawler.pdf:PDF}
}

@INPROCEEDINGS{2013-HoangGrosse.etal,
  author = {Hoang M. Le and Daniel Gro{\ss}e and Vladimir Herdt and Rolf Drechsler},
  title = {Verifying {SystemC} using an intermediate verification language and
	symbolic simulation},
  booktitle = {Proc. Intl. Design Automation Conference ({DAC})},
  year = {2013},
  pages = {116:1--116:6},
  owner = {stoffel},
  timestamp = {2016.05.10}
}

@ARTICLE{1959-Lee,
  author = {C. Lee},
  title = {Representation of Switching Circuits by Binary-Decision Programs},
  journal = {Bell Systems Technical Journal},
  year = {1959},
  volume = {38},
  pages = {985-999},
  month = {July},
  file = {:./files/1959-Lee.pdf:PDF}
}

@ARTICLE{2001-Lee,
  author = {Edward A. Lee},
  title = {Embedded Software},
  journal = {Academic Press London 2002},
  year = {2001},
  volume = {56},
  file = {:./files/2001-Lee.pdf:PDF},
  timestamp = {2006.10.04}
}

@INPROCEEDINGS{1991-LeeHa,
  author = {H. K. Lee and D. S. Ha},
  title = {An Efficient Forward Fault Simulation Algorithm Based on the Parallel
	Pattern Single Fault Propagation},
  booktitle = {Proc. International Test Conference ({ITC})},
  year = {1991},
  pages = {946-955},
  month = {October},
  file = {:./files/1991-LeeHa.pdf:PDF}
}

@INPROCEEDINGS{2004-LeeHsiung,
  author = {Te-Chang Lee and Pao-Ann Hsiung},
  title = {Mutation Coverage Estimation for Model Checking},
  booktitle = {Automated Technology for Verification and Analysis ({ATVA})},
  year = {2004},
  editor = {Wang, Farn},
  volume = {3299},
  series = {Lecture Notes in Computer Science},
  pages = {354-368},
  publisher = {Springer Berlin / Heidelberg},
  note = {10.1007/978-3-540-30476-0\_29},
  file = {:./files/2004-LeeHsiung.pdf:PDF},
  isbn = {978-3-540-23610-8},
  keyword = {Computer Science},
  owner = {W},
  timestamp = {2010.01.11}
}

@INPROCEEDINGS{2008-LeinweberBhunia,
  author = {L. Leinweber and S. Bhunia},
  title = {Fine-Grained Supply Gating Through Hypergraph Partitioning and {Shannon}
	Decomposition for Active Power Reduction},
  booktitle = {2008 Design, Automation and Test in Europe},
  year = {2008},
  issn = {1530-1591},
  keywords = {logic CAD;logic circuits;low-power electronics;ISCAS-85 benchmarks;Shannon
	decomposition;fine-grained supply gating;hypergraph partitioning;leakage
	power;logic CAD;logic circuits;size 32 nm;standby power reduction;sub-65nm
	technology regime;Batteries;Circuit simulation;Circuit synthesis;Design
	automation;Design methodology;Energy consumption;Energy efficiency;Logic
	circuits;Logic design;Predictive models;Active Power;Hypergraph Partitioning;Low
	Power Design;Supply Gating},
  owner = {udupi},
  timestamp = {2017.08.15}
}

@TECHREPORT{1996-Leipert,
  author = {Sebastian Leipert},
  title = {The Tree Interface - Version 1.0 User Manual},
  institution = {Institut f{\"u}r Informatik, Universit{\"a}t zu K{\"o}ln},
  year = {1996},
  number = {96.242},
  file = {:./files/1996-Leipert.pdf:PDF},
  url = {http://www.informatik.uni-koeln.de/ls_juenger/research/vbctool}
}

@ARTICLE{1991-LeisersonSaxe,
  author = {C.E. Leiserson and J.B. Saxe},
  title = {Retiming Synchronous Circuitry},
  journal = {Algorithmica},
  year = {1991},
  volume = {6},
  pages = {5-35},
  file = {:./files/1991-LeisersonSaxe.pdf:PDF}
}

@ARTICLE{2002-LetchfordLodi,
  author = {Adam N. Letchford and Andrea Lodi},
  title = {Strengthening Chvatal-Gomory Cuts and Gomory Fractional Cuts},
  journal = {Operations Research Letters},
  year = {2002},
  volume = {30},
  pages = {74-82},
  number = {2},
  file = {:./files/2002-LetchfordLodi.pdf:PDF}
}

@INPROCEEDINGS{2004a-LevenMehler.etal,
  author = {Peter Leven and Tilman Mehler and Stefan Edelkamp},
  title = {Directed Error Detection in C++ with the Assembly-Level Model Checker
	{StEAM}},
  booktitle = {In Spin Workshop},
  year = {2004},
  volume = {Volume 2989/2004},
  series = {Lecture Notes in Computer Science},
  pages = {39--56},
  abstract = {Most approaches for model checking software are based on the generation
	of abstract models from source code, which may greatly reduce the
	search space, but may also introduce errors that are not present
	in the actual program. In this paper, we propose a new model checker
	for the verification of native c++-programs. To allow platform independent
	model checking of the object code for concurrent programs, we have
	extended an existing virtual machine for c++ to include multi-threading
	and different exploration algorithms on a dynamic state description.
	The error reporting capabilities and the lengths of counter-examples
	are improved by using heuristic estimator functions and state space
	compaction techniques that additionally reduce the exploration efforts.
	The evaluation of four scalable simple example problems shows that
	our system StEAM1 can successfully enhance the detection of deadlocks
	and assertion violations.},
  file = {:./files/2004a-LevenMehler.etal.pdf:PDF},
  owner = {nguyen},
  timestamp = {2006.08.29}
}

@INPROCEEDINGS{2003-LiWang.etal,
  author = {Bing Li and Chao Wang and Fabio Somenzi},
  title = {A Satisfiability Based Approach to Abstraction Refinement in Model
	Checking},
  booktitle = {In Workshop on {BMC}},
  year = {2003},
  file = {:./files/2003-LiWang.etal.pdf:PDF},
  timestamp = {2006.09.12}
}

@INPROCEEDINGS{2011-LiXie.etal,
  author = {J. {Li} and F. {Xie} and T. {Ball} and V. {Levin} and C. {McGarvey}},
  title = {Formalizing hardware/software interface specifications},
  booktitle = {2011 26th IEEE/ACM International Conference on Automated Software
	Engineering (ASE 2011)},
  year = {2011},
  pages = {143-152},
  month = {Nov},
  owner = {fehmel},
  timestamp = {2019.05.27}
}

@INPROCEEDINGS{2009-LiRamachandran.etal,
  author = {M. L. Li and P. Ramachandran and U. R. Karpuzcu and S. K. S. Hari
	and S. V. Adve},
  title = {Accurate microarchitecture-level fault modeling for studying hardware
	faults},
  booktitle = {IEEE 15th International Symposium on High Performance Computer Architecture},
  year = {2009},
  pages = {105-116},
  month = {Feb},
  file = {2009-LiRamachandran.etal.pdf:files/2009-LiRamachandran.etal.pdf:PDF},
  issn = {1530-0897},
  owner = {bartsch},
  timestamp = {2016.11.30}
}

@INPROCEEDINGS{2008-LiRamachandran.etal,
  author = {Man-Lap Li and Pradeep Ramachandran and Swarup Kumar Sahoo and Sarita
	V. Adve and Vikram S. Adve and Yuanyuan Zhou},
  title = {Understanding the Propagation of Hard Errors to Software and Implications
	for Resilient System Design},
  booktitle = {Proceedings of the 13th International Conference on Architectural
	Support for Programming Languages and Operating Systems},
  year = {2008},
  series = {ASPLOS XIII},
  pages = {265 - 276},
  file = {2008-LiRamachandran.etal.pdf:files/2008-LiRamachandran.etal.pdf:PDF},
  isbn = {978-1-59593-958-6},
  numpages = {12},
  owner = {bartsch},
  timestamp = {2015.08.03}
}

@ARTICLE{2014-LiKashyap.etal,
  author = {Li, Xun and Kashyap, Vineeth and Oberg, Jason K and Tiwari, Mohit
	and Rajarathinam, Vasanth Ram and Kastner, Ryan and Sherwood, Timothy
	and Hardekopf, Ben and Chong, Frederic T},
  title = {Sapper: A language for hardware-level security policy enforcement},
  journal = {ACM SIGARCH Computer Architecture News},
  year = {2014},
  volume = {42},
  pages = {97--112},
  number = {1},
  owner = {fadiheh},
  publisher = {ACM},
  timestamp = {2018.07.13}
}

@ARTICLE{2005-LiMitra.etal,
  author = {Li, Xianfeng and Mitra, Tulika and Roychoudhury, Abhik},
  title = {Modeling control speculation for timing analysis},
  journal = {Real-Time Syst.},
  year = {2005},
  volume = {29},
  pages = {27--58},
  number = {1},
  month = {jan},
  acmid = {1035389},
  address = {Norwell, MA, USA},
  file = {:./files/2005-LiMitra.etal.pdf:PDF},
  issn = {0922-6443},
  issue_date = {January 2005},
  keywords = {branch prediction, instruction cache, micro-architectural modeling,
	schedulability analysis, worst case execution time},
  numpages = {32},
  publisher = {Kluwer Academic Publishers}
}

@INPROCEEDINGS{2003-LiMitra,
  author = {Xianfeng Li and T. Mitra and A. Roychoudhury},
  title = {Accurate timing analysis by modeling caches, speculation and their
	interaction},
  booktitle = {Proceedings 2003. Design Automation Conference (IEEE Cat. No.03CH37451)},
  year = {2003},
  pages = {466-471},
  month = {June},
  abstract = {Schedulability analysis of real-time embedded systems requires worst
	case timing guarantees of embedded software performance. This involves
	not only language level program analysis, but also modeling the effects
	of complex micro-architectural features in modern processors. Speculative
	execution and caching are very common in current processors. Hence
	one needs to model the effects of these features on the Worst Case
	Execution (WCET) of a program. Even though the individual effects
	of these features have been studied recently, their combined effects
	have not been investigated. We do so in this paper. This is a non-trivial
	task because speculative execution can indirectly affect cache performance
	(e.g., speculatively executed blocks can cause additional cache misses).
	Our technique starts from the control flow graph of the embedded
	program, and uses integer linear programming to estimate the program's
	WCET. The accuracy of our modeling is illustrated by tight estimates
	obtained on realistic benchmarks.},
  file = {2003-LiMitra.pdf:files/2003-LiMitra.pdf:PDF},
  keywords = {cache storage;computational complexity;embedded systems;flow graphs;integer
	programming;linear programming;performance evaluation;timing;accurate
	timing analysis;branch prediction;cache performance;control flow
	graph;integer linear programming;language level program analysis;microarchitectural
	features;real-time embedded system;realistic benchmark;schedulability
	analysis;speculative execution;tight estimate;worst case execution
	time;Embedded computing;Embedded software;Embedded system;Integer
	linear programming;Permission;Pipelines;Predictive models;Prefetching;Scheduling;Timing},
  owner = {schwarz},
  timestamp = {2017.01.09}
}

@ARTICLE{2006-LiRoychoudhury.etal,
  author = {Li, Xianfeng and Roychoudhury, Abhik and Mitra, Tulika},
  title = {Modeling out-of-order processors for {WCET} analysis},
  journal = {Real-Time Systems},
  year = {2006},
  volume = {34},
  pages = {195--227},
  number = {3},
  issn = {1573-1383},
  owner = {villarraga},
  timestamp = {2016.08.10}
}

@INPROCEEDINGS{2004-LiRoychoudhury.etal,
  author = {Xianfeng Li and A. Roychoudhury and T. Mitra},
  title = {Modeling out-of-order processors for software timing analysis},
  booktitle = {25th IEEE International Real-Time Systems Symposium},
  year = {2004},
  pages = {92-103},
  month = {Dec},
  file = {2004-LiRoychoudhury.etal.pdf:files/2004-LiRoychoudhury.etal.pdf:PDF},
  issn = {1052-8725},
  keywords = {integer programming;linear programming;pipeline processing;program
	processors;real-time systems;timing;WCET analysis;data dependencies;integer
	linear programming;microarchitectural features;out-of-order processor
	pipelines;real-time distributed systems;resource contentions;schedulability
	analysis;software timing analysis;timing effects;worst case execution
	time;Delay;Integer linear programming;Microarchitecture;Out of order;Performance
	analysis;Pipelines;Predictive models;Processor scheduling;Real time
	systems;Timing},
  owner = {schwarz},
  timestamp = {2017.01.09}
}

@INPROCEEDINGS{2011-LiTiwari.etal,
  author = {Li, Xun and Tiwari, Mohit and Oberg, Jason K and Kashyap, Vineeth
	and Chong, Frederic T and Sherwood, Timothy and Hardekopf, Ben},
  title = {Caisson: a hardware description language for secure information flow},
  booktitle = {ACM SIGPLAN Notices},
  year = {2011},
  volume = {46},
  number = {6},
  pages = {109--120},
  organization = {ACM},
  owner = {fadiheh},
  timestamp = {2018.07.13}
}

@INPROCEEDINGS{2005-LiWang.etal,
  author = {Xin Li and Jian Wang and Lawrence T. Pileggi and Tun-Shih Chen and
	Wanju Chiang},
  title = {Performance-Centering Optimization for System-Level Analog Design
	Exploration},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2005},
  pages = { 422 - 429},
  file = {:./files/2005-LiWang.etal.pdf:PDF},
  keywords = { analog design exploration; analog design optimization; analog system
	architectures; clock data recovery system; constraint boundary; design
	objective function; independent circuit block design; inscribed ellipsoid;
	performance-centering optimization; system-level design exploration;
	system-level models; analogue integrated circuits; circuit optimisation;
	integrated circuit design; integrated circuit modelling;},
  timestamp = {2006.09.27}
}

@INPROCEEDINGS{1996-LiMalik.etal,
  author = {Li, Y.-T. S. and Malik, S. and Wolfe, A.},
  title = {Cache Modeling for Real-Time Software: Beyond Direct Mapped Instruction
	Caches},
  booktitle = {Real-Time Systems Symposium, 1996., 17th {IEEE}},
  year = {1996},
  pages = {254 -263},
  month = {dec},
  file = {:./files/1996-LiMalik.etal.pdf:PDF},
  issn = {1052-8725},
  keywords = {cache hits;cache misses;cache modeling;cinderella;data caches;design
	tool;direct mapped instruction caches;hardware system;integer-linear-programming;memory
	performance;real-time software;research;set associative instruction
	caches;tight bound;unified caches;worst case execution time;worst
	case timing analysis;cache storage;integer programming;linear programming;real-time
	systems;software performance evaluation;timing;}
}

@BOOK{2002-Liggesmeyer,
  title = {Software Qualit{\"a}t},
  publisher = {Spektrum Akademischer Verlag},
  year = {2002},
  author = {Peter Liggesmeyer},
  comment = {German Book},
  owner = {bschmidt},
  timestamp = {2013.08.07},
  url = {www.liggesmeyer.de}
}

@INPROCEEDINGS{2005-LimLee.etal,
  author = {Hyeonmin Lim and Kyungsoo Lee and Youngjin Cho and Naehyuck Chang},
  title = {Flip-Flop Insertion with Shifted-Phase Clocks for {FPGA} Power Reduction},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2005},
  pages = { 335 - 342},
  file = {:./files/2005-LimLee.etal.pdf:PDF},
  keywords = { FPGA power reduction; NP-complete problem; clock assignment; clock
	frequency; clock phase selection; field programmable gate array;
	flip-flop insertion; full-chip measurements; glitch generation; glitch
	minimization; glitch propagation; look-up table size; phase-shifted
	clock; pipeline structure; propagation model; retiming methods; routing
	paths; shifted-phase clocks; clocks; field programmable gate arrays;
	flip-flops; integrated circuit design; logic design; table lookup;},
  timestamp = {2006.09.27}
}

@INPROCEEDINGS{2005-LinZhou,
  author = {Chuan Lin and Hai Zhou},
  title = {Trade-off between Latch and Flop for Min-Period Sequential Circuit
	Designs with Crosstalk},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2005},
  pages = { 329 - 334},
  file = {:./files/2005-LinZhou.pdf:PDF},
  keywords = { circular time representation; clock period; coupling detection; crosstalk;
	flops; heuristic algorithm; latches; min-period sequential circuit
	designs; optimal configuration; crosstalk; flip-flops; integrated
	circuit design; logic design; sequential circuits;},
  timestamp = {2006.09.27}
}

@INPROCEEDINGS{2015-LinSingh.etal,
  author = {D. Lin and E. Singh and C. Barrett and S. Mitra},
  title = {A structured approach to post-silicon validation and debug using
	symbolic quick error detection},
  booktitle = {Proc. IEEE Intl. Test Conf. (ITC)},
  year = {2015},
  pages = {1-10},
  month = {Oct},
  file = {:files/2015-LinSingh.etal.pdf:PDF}
}

@INPROCEEDINGS{2004-LinYen.etal,
  author = {Hue-Min Lin and Chia-Chih Yen and Che-Hua Shih and Jing-Yang Jou},
  title = {On Compliance Test Of On-Chip Bus For {SOC}},
  booktitle = {Proc. International Conference {ASP} Design Automation},
  year = {2004},
  pages = { 328 - 333},
  file = {:./files/2004-LinYen.etal.pdf:PDF},
  keywords = { AMBA AHB protocol; WISHBONE protocol; compliance test; design error
	detection; monitor-based approach; on-chip bus; system-on chip; finite
	state machines; formal verification; logic testing; protocols; system
	buses; system-on-chip;},
  timestamp = {2006.09.19}
}

@INPROCEEDINGS{2006-LinSrinivasan.etal,
  author = {Lin, I.C. and Srinivasan, S. and Vijaykrishnan, N.},
  title = {Transaction Level Error Susceptibility Model for Bus Based {SoC}
	Architectures},
  booktitle = {Quality Electronic Design, 2006. ISQED '06. 7th International Symposium
	on},
  year = {2006},
  pages = {6 pp. -780},
  month = {march},
  file = {:./files/2006-LinSrinivasan.etal.pdf:PDF},
  keywords = {bus based SoC architectures;single bit error;transaction level error
	susceptibility model;error analysis;system buses;system-on-chip;}
}

@MISC{WWW_LIN2.0,
  author = {{LIN Administration}},
  title = {L{IN} {S}pecification {P}ackage {R}ev. 2.0},
  year = {2003},
  owner = {bschmidt},
  timestamp = {2014.02.21},
  url = {http://www.lin-subbus.org/}
}

@MISC{WWW_LIN,
  author = {{LIN Administration}},
  title = {L{IN} {S}pecification {P}ackage {R}ev. 1.3},
  year = {2002},
  bdsk-url-1 = {http://www.lin-subbus.org/},
  owner = {villarraga},
  timestamp = {2012.08.27},
  url = {http://www.lin-subbus.org/}
}

@MISC{WWW_LIN2.2A,
  author = {{LIN Consortium}},
  title = {L{IN} {S}pecification {P}ackage {R}ev. 2.2A},
  year = {2010},
  owner = {fehmel},
  timestamp = {2016.11.18},
  url = {http://www.lin-subbus.org/}
}

@MISC{2003-LINDO,
  author = {{LINDO}},
  title = {{API} Users Manual},
  year = {2003},
  address = {1415 North Dayton Street, Chicago, Illinois 60622, USA},
  organization = {LINDO Systems, Inc.},
  owner = {stoffel},
  timestamp = {2016.05.11},
  url = {http://www.lindo.com}
}

@TECHREPORT{1996-lions,
  author = {J.L. Lions},
  title = {Ariane 5 Flight 501 Failure, Report by the Inquiry Board},
  year = {1996},
  address = {Paris},
  owner = {bschmidt},
  timestamp = {2014.06.27}
}

@ARTICLE{2018-LippSchwarz.etal,
  author = {Lipp, Moritz and Schwarz, Michael and Gruss, Daniel and Prescher,
	Thomas and Haas, Werner and Mangard, Stefan and Kocher, Paul and
	Genkin, Daniel and Yarom, Yuval and Hamburg, Mike},
  title = {Meltdown},
  journal = {arXiv preprint arXiv:1801.01207},
  year = {2018},
  owner = {fadiheh},
  timestamp = {2018.07.12}
}

@INPROCEEDINGS{2018-LiuYang.etal,
  author = {Liu, Chen and Yang, Zhiliu and Blasingame, Zander and Torres, Gildo
	and Bruska, James},
  title = {Detecting Data Exploits Using Low-level Hardware Information: A Short
	Time Series Approach},
  booktitle = {Proceedings of the First Workshop on Radical and Experiential Security},
  year = {2018},
  pages = {41--47},
  organization = {ACM},
  owner = {fadiheh},
  timestamp = {2018.07.12}
}

@INPROCEEDINGS{2007-LoKhoo.etal,
  author = {Lo, David and Khoo, Siau-Cheng and Liu, Chao},
  title = {Efficient mining of iterative patterns for software specification
	discovery},
  booktitle = {roceedings of the 13th ACM SIGKDD international conference on Knowledge
	discovery and data mining},
  year = {2007},
  owner = {fehmel},
  timestamp = {2019.05.27}
}

@ARTICLE{2005-LoghiMargaria.etal,
  author = {Mirko Loghi and Tiziana Margaria and Graziano Pravadelli and Bernhard
	Steffen},
  title = {Dynamic and Formal Verification of Embedded Systems A Comparative
	Survey},
  journal = {International Journal of Parallel Programming,},
  year = {2005},
  volume = {33},
  pages = {585-611},
  file = {:./files/2005-LoghiMargaria.etal.pdf:PDF},
  timestamp = {2006.10.04}
}

@INPROCEEDINGS{2013-LoiaconoPalena.etal,
  author = {C. Loiacono and M. Palena and P. Pasini and D. Patti and J. Baumgartner},
  title = {Fast Cone-Of-Influence Computation and Estimation in Problems with
	Multiple Properties},
  booktitle = {Proceedings Design Automation and Test In Europe},
  year = {2013},
  pages = {803-806},
  file = {:import/var/jabref/files/2013-LoiaconoPalena.pdf:PDF},
  owner = {stoffel},
  timestamp = {2015.04.02}
}

@INPROCEEDINGS{2008-LoitzWedler.etal,
  author = {S. Loitz and M. Wedler and C. Brehm and T. Vogt and N. Wehn and W.
	Kunz},
  title = {Proving Functional Correctness of Weakly Programmable {IPs} - A Case
	Study with Formal Property Checking},
  booktitle = {Proc. 6th IEEE Symposium on Application Specific Processors ({SASP})},
  year = {2008},
  pages = {48 -54},
  address = {Anaheim, CA, USA},
  month = {June},
  file = {:./files/2008-LoitzWedler.etal.pdf:PDF},
  keywords = {application-specific programs;embedded processors;functional correctness;programmable
	IP blocks;systems-on-chip design;integrated circuit design;microprocessor
	chips;system-on-chip;},
  owner = {wedler},
  timestamp = {2008.06.16}
}

@INCOLLECTION{2012-LoitzWedler.etal,
  author = {Loitz, Sacha and Wedler, Markus and Stoffel, Dominik and Brehm, Christian
	and Kunz, Wolfgang and Wehn, Norbert},
  title = {Formal Hardware/Software Co-verification of Application Specific
	Instruction Set Processors},
  booktitle = {System Specification and Design Languages},
  publisher = {Springer New York},
  year = {2012},
  editor = {Kazmierski, Tom J. J. and Morawiec, Adam},
  volume = {106},
  series = {Lecture Notes in Electrical Engineering},
  pages = {1-20},
  affiliation = {Department of Electrical and Computer Engineering, Technische Universit{\"a}t
	Kaiserslautern, Kaiserslautern, Germany},
  isbn = {978-1-4614-1427-8},
  keyword = {Engineering},
  owner = {villarraga},
  timestamp = {2012.08.27}
}

@INPROCEEDINGS{2010-LoitzWedler.etal,
  author = {Sacha Loitz and Markus Wedler and Dominik Stoffel and Christian Brehm
	and Wolfgang Kunz and Norbert Wehn},
  title = {Complete Verification of Weakly Programmable {IPs} against their
	Operational {ISA} Model},
  booktitle = {Proc. Forum on Specification \& Design Languages},
  year = {2010},
  pages = {1 -8},
  month = {09},
  file = {:./files/2010-LoitzWedler.etal:PDF},
  location = {Southampton, UK},
  owner = {stoffel},
  timestamp = {2010.11.16}
}

@ARTICLE{1998-LokketangenGlover,
  author = {Arne Lokketangen and Fred Glover},
  title = {Solving Zero/One Mixed Integer Programming Problems using Tabu Search},
  journal = {European Journal of Operations Research},
  year = {1998},
  volume = {106},
  pages = {624-658},
  file = {:./files/1998-LokketangenGlover.pdf:PDF}
}

@ARTICLE{2001-LougeeHeimerBarahona.etal,
  author = {Robin Lougee-Heimer and Francisco Barahona and Brenda Dietrich and
	J. P. Fasano and John Forrest and Robert Harder and Laszlo Ladanyi
	and T. Pfender and Theodore Ralphs and Matthew Saltzman and Katya
	Schienberger},
  title = {The {COIN-OR} Initiative: Open-source software accelerates operations
	research progress},
  journal = {ORMS Today},
  year = {2001},
  volume = {28},
  pages = {20-22},
  number = {5},
  month = {October},
  url = {http://www.orms-today.org/orms-10-01/forumfr.html}
}

@INPROCEEDINGS{2018-LowepowerAkella.etal,
  author = {Lowe-Power, Jason and Akella, Venkatesh and Farrens, Matthew K and
	King, Samuel T and Nitta, Christopher J},
  title = {A case for exposing extra-architectural state in the ISA: position
	paper},
  booktitle = {Proceedings of the 7th International Workshop on Hardware and Architectural
	Support for Security and Privacy},
  year = {2018},
  pages = {8},
  organization = {ACM},
  owner = {fadiheh},
  timestamp = {2018.07.12}
}

@INPROCEEDINGS{2019-LudwigSchwarz.etal,
  author = {Tobias Ludwig and Michael Schwarz and Joakim Urdahl and Lucas Deutschmann
	and Salaheddin Hetalani and Dominik Stoffel and Wolfgang Kunz},
  title = {Property-Driven Development of a {RISC-V} {CPU}},
  booktitle = {Proc. Design and Verification Conference United States (DVCON-US)},
  year = {2019},
  owner = {stoffel},
  timestamp = {2019.01.08}
}

@MISC{web-pdd,
  author = {Tobias Ludwig and Joakim Urdahl and Dominik Stoffel and Wolfgang
	Kunz},
  title = {Property-Driven Design Methodology ({PDD}) --- Tool, Manual, Examples},
  howpublished = {GitHub},
  owner = {stoffel},
  timestamp = {2019.01.08},
  url = {https://github.com/ludwig247/PDD}
}

@ARTICLE{2019a-LudwigUrdahl.etal,
  author = {Tobias Ludwig and Joakim Urdahl and Dominik Stoffel and Wolfgang
	Kunz},
  title = {Properties First {--} Correct-By-Construction {RTL} Design in System-Level
	Design Flows},
  journal = {arXiv preprint (Not published yet)},
  year = {2019},
  owner = {stoffel},
  timestamp = {2019.01.25}
}

@PHDTHESIS{2002-Lundqvist,
  author = {Thomas Lundqvist},
  title = {A {WCET} Analysis Method for Pipelined Microprocessors with Cache
	Memories},
  school = {CHALMERS UNIVERSITY OF TECHNOLOGY Goteborg, Sweden},
  year = {2002},
  file = {:./files/2002-Lundqvist.pdf:PDF},
  timestamp = {2006.09.22}
}

@INPROCEEDINGS{2012-LvKalla.etal,
  author = {Jinpeng Lv and Kalla, P. and Enescu, F.},
  title = {Efficient {Gr\"obner} basis reductions for formal verification of
	galois field multipliers},
  booktitle = {Design, Automation Test in Europe Conference Exhibition (DATE), 2012},
  year = {2012},
  pages = {899-904},
  file = {:files/2012-LvKalla.etal.pdf:PDF},
  issn = {1530-1591},
  keywords = {Galois fields;digital arithmetic;formal verification;multiplying circuits;network
	topology;polynomials;process algebra;163-bit circuits;Galois field
	arithmetic;Galois field multiplier;Grobner basis reductions;algebraic
	geometry-based approach;bug detection;circuit topology;computer algebra-based
	approach;formal verification;multiplier circuit modeling;multiplier
	hardware implementation;polynomial system;{Boolean} functions;Computer
	bugs;Data structures;Elliptic curve cryptography;Integrated circuit
	modeling;Logic gates;Polynomials}
}

@ARTICLE{1989-LynchTuttle,
  author = {Nancy A. Lynch and Mark R. Tuttle},
  title = {An introduction to input/output automata},
  journal = {CWI Quarterly},
  year = {1989},
  volume = {2},
  pages = {219--246},
  file = {:./files/1989-LynchTuttle.pdf:PDF}
}

@ARTICLE{1999-ClarkeLong,
  author = {Edmund M.Clarke and David E.Long},
  title = {Model Checking and Abstraction},
  journal = {ACM Transactions on Programming Languages and Systems},
  year = {1999},
  volume = {16},
  pages = {1512 - 1542},
  file = {:./files/1999-ClarkeLong.pdf:PDF},
  timestamp = {2006.09.12}
}

@INPROCEEDINGS{1991-GeoneClaesen.etal,
  author = {M.Geone and L.Claesen and E.Verlind and H.Man and Frank Proesmans},
  title = {Illustration of the {SFG}-Tracing Multi-Level Behavioral Verification
	Methodology by the Correctness Proof of a High to Low Level Synthesis
	Application in {CATHEDRAL-II}},
  booktitle = {Proc. {IEEE} International Conference on Computer Design on {VLSI}
	in Computer \& Processors},
  year = {1991},
  pages = {338 -341},
  file = {:./files/1991-GeoneClaesen.etal.pdf:PDF},
  keywords = {Cathedral-II silicon compiler;SFG-tracing multi-level behavioral verification
	methodology;automatic verification;correctness proof;datapath;design
	for testability;digital synchronous circuit;high to low level synthesis;higher
	level specifications;multi-branch micro coded controller;register
	files;transistor level implementation;transistor switch level;circuit
	layout CAD;logic CAD;logic circuits;logic testing;},
  timestamp = {2006.09.27}
}

@ARTICLE{2001-LiuJoseph,
  author = {Z.Liu M.Joseph},
  title = {Verification Refinement and Scheduling of Real Time Programs},
  journal = {Theoretical Computer Science},
  year = {2001},
  volume = {253},
  pages = {119 - 152},
  file = {:./files/2001-LiuJoseph.pdf:PDF},
  timestamp = {2006.09.14}
}

@INPROCEEDINGS{1996-LiuJoseph,
  author = {Z.Liu M.Joseph},
  title = {Verification of Fault-Tolerance and Real Time},
  booktitle = {Proc. Annual International Symposium on Fault-Tolerant Computing},
  year = {1996},
  pages = {220 -229},
  file = {:./files/1996-LiuJoseph.pdf:PDF},
  keywords = {expressive logic;fault tolerance verification;fault-tolerant system
	verification;functional requirements;real time systems;specification;state
	change;system failure;system failures;transformational method;algebraic
	specification;formal specification;program verification;real-time
	systems;software fault tolerance;},
  timestamp = {2006.09.14}
}

@INPROCEEDINGS{1992-RudnickFuchs.etal,
  author = {M.Rudnick and W. Fuchs and H. Patel},
  title = {Diagnostic Fault Simulation of Sequential Circuits},
  booktitle = {Proc. International Test Conference on Discover the New World of
	Test and Design},
  year = {1992},
  pages = {178},
  file = {:./files/1992-RudnickFuchs.etal.pdf:PDF},
  timestamp = {2006.09.14}
}

@TECHREPORT{1993-Russinoff,
  author = {David M.Russinoff},
  title = {A Formal Langauage For The Specification And Verfication of synchronous
	and Asynchronous},
  institution = {NASA},
  year = {1993},
  file = {:./files/1993-Russinoff.pdf:PDF},
  timestamp = {2006.09.14}
}

@INPROCEEDINGS{2018-GritschnederDittrich.etal,
  author = {D. M{\"u}ller-Gritschneder and M. Dittrich and J. Weinzierl and E.
	Cheng and S. Mitra and U. Schlichtmann},
  title = {{ETISS-ML}: A multi-level instruction set simulator with {RTL}-level
	fault injection support for the evaluation of cross-layer resiliency
	techniques},
  booktitle = {2018 Design, Automation Test in Europe Conference Exhibition (DATE)},
  year = {2018},
  issn = {1558-1101},
  owner = {udupi},
  timestamp = {2018.09.04}
}

@ARTICLE{1988-MahmoodMcCluskey,
  author = {A. Mahmood and E. J. McCluskey},
  title = {Concurrent error detection using watchdog processors-a survey},
  journal = {IEEE Transactions on Computers},
  year = {1988},
  volume = {37},
  pages = {160-174},
  number = {2},
  month = {February},
  file = {1988-MahmoodMcCluskey.pdf:files/1988-MahmoodMcCluskey.pdf:PDF},
  issn = {0018-9340},
  owner = {bartsch},
  timestamp = {2016.09.21}
}

@INPROCEEDINGS{2016-MalikSubramanyan,
  author = {Malik, Sharad and Subramanyan, Pramod},
  title = {Specification and modeling for Systems-on-Chip security verification},
  booktitle = {Design Automation Conference (DAC), 2016 53nd ACM/EDAC/IEEE},
  year = {2016},
  pages = {1--6},
  organization = {IEEE},
  owner = {fadiheh},
  timestamp = {2018.07.12}
}

@INPROCEEDINGS{1988-MalikWang.etal,
  author = {S. Malik and A. Wang and R. Brayton and A. Sangiovanni-Vincentelli},
  title = {Logic Verification using Binary Decision Diagrams in a Logic Synthesis
	Environment},
  booktitle = {Proc. International Conference on Computer-Aided Design (ICCAD)},
  year = {1988},
  pages = {6-9},
  month = {November},
  file = {:./files/1988-MalikWang.etal.pdf:PDF},
  keywords = {{Boolean} functions;MIS;binary decision diagrams;canonical representations;cube
	enumeration;formal logic verification system;functional equivalence;multilevel
	logic synthesis system;variable ordering;{Boolean} functions;logic
	CAD;logic testing;}
}

@INCOLLECTION{2005-Manolios,
  author = {Manolios, Panagiotis},
  title = {Verified Software: Theories, Tools, Experiments},
  booktitle = {The Challenge of Hardware-Software Co-verification},
  publisher = {Springer-Verlag},
  year = {2008},
  editor = {Meyer, Bertrand and Woodcock, Jim},
  pages = {438--447},
  address = {Berlin, Heidelberg},
  acmid = {1417127},
  file = {:./files/2005-Manolios.pdf:PDF},
  isbn = {978-3-540-69147-1},
  numpages = {10}
}

@ARTICLE{2008-ManoliosSudarshan.etal,
  author = {Panagiotis Manolios and Sudarshan K. Srinivasan},
  title = {A Refinement-Based Compositional Reasoning Framework for Pipelined
	Machine Verification},
  journal = {{IEEE} Transactions on {VLSI} Systems},
  year = {2008},
  volume = {16},
  pages = {353-364},
  file = {:./files/2008-ManoliosSudarshan.etal.pdf:PDF},
  owner = {wedler},
  timestamp = {2008.12.16}
}

@INPROCEEDINGS{2005a-ManoliosSrinivasan,
  author = {Panagiotis Manolios and Sudarshan K. Srinivasan},
  title = {Verification of Executable Pipelined Machines with Bit-Level Interfaces},
  booktitle = {Proc. International Conference on Computer-Aided Design (ICCAD)},
  year = {2005},
  pages = { 855 - 862},
  file = {:./files/2005a-ManoliosSrinivasan.pdf:PDF},
  keywords = { ACL2 theorem proving system; UCLID; bit-level interfaces; datapath;
	decision procedures; deductive reasoning; executable pipelined machines;
	instruction set architecture; term level abstraction; bisimulation
	equivalence; circuit CAD; pipeline processing; theorem proving;},
  timestamp = {2006.09.27}
}

@INPROCEEDINGS{2005-ManoliosSrinivasan,
  author = {Panagiotis Manolios and Sudarshan K. Srinivasan},
  title = {A Complete Compositional Reasoning Framework for the Efficient Verification
	of Pipelined Machines},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2005},
  pages = { 863 - 870},
  file = {:./files/2005-ManoliosSrinivasan.pdf:PDF},
  keywords = { composition proof; compositional proof rules; compositional reasoning
	framework; decision procedures; design cycle; instruction set architectures;
	pipelined machine verification; bisimulation equivalence; circuit
	CAD; logic testing; pipeline processing;},
  timestamp = {2006.09.27}
}

@ARTICLE{2005-ManquinhoRoussel,
  author = {V. M. Manquinho and O. Roussel},
  title = {The First Evaluation of Pseudo-{Boolean} Solvers ({PB}'05)},
  journal = {Journal on Satisfiability, {Boolean} Modeling and Computation({JSAT})},
  year = {2005},
  volume = {2},
  pages = {103-143},
  file = {:./files/2005-ManquinhoRoussel.pdf:PDF}
}

@INPROCEEDINGS{1998-MansouriVemuri,
  author = {N. Mansouri and R. Vemuri},
  title = {A Methodology For Automated Verification Of Synthesized {RTL} Design
	And Its Integration With High Level SynthesIs Tool},
  booktitle = {Proc. International Conference on Formal Methods in Computer-Aided
	Design ({FMCAD})},
  year = {1998},
  pages = {204--221},
  file = {:./files/1998-MansouriVemuri.pdf:PDF},
  timestamp = {2006.09.21}
}

@TECHREPORT{1999-MarchandMartin.etal,
  author = {Hugues Marchand and Alexander Martin and Robert Weismantel and Laurence
	A. Wolsey},
  title = {Cutting Planes in Integer and Mixed Integer Programming},
  institution = {Zuse Institute Berlin},
  year = {1999},
  number = {99-44},
  file = {:./files/1999-MarchandMartin.etal.pdf:PDF},
  url = {http://www.zib.de/Publications/abstracts/SC-99-44/}
}

@ARTICLE{2001-MarchandWolsey,
  author = {Hugues Marchand and Laurence A. Wolsey},
  title = {Aggregation and Mixed Integer Rounding to Solve {MIP}s},
  journal = {Operations Research},
  year = {2001},
  volume = {49},
  pages = {363-371},
  number = {3},
  file = {:./files/2001-MarchandWolsey.pdf:PDF}
}

@ARTICLE{1999-MarquesSilvaSakallah,
  author = {P. Marques-Silva and K. A. Sakallah},
  title = {{GRASP}: A Search Algorithm for Propositional Satisfiability},
  journal = {IEEE Transactions on Computers},
  year = {1999},
  volume = {48},
  pages = {506-521},
  number = {5},
  month = {May},
  file = {:./files/1999-MarquesSilvaSakallah.pdf:PDF}
}

@INPROCEEDINGS{2010-MarquetMoy,
  author = {Kevin Marquet and Matthieu Moy},
  title = {{PinaVM}: A {SystemC} Front-end Based on an Executable Intermediate
	Representation},
  booktitle = {Proc. Intl. Conf. on Embedded Software ({EMSOFT})},
  year = {2010},
  pages = {79--88},
  file = {:files/2010-MarquetMoy.pdf:PDF}
}

@BOOKLET{1998-Martin,
  title = {Integer Programs with Block Structure},
  author = {Alexander Martin},
  howpublished = {Habilitations-Schrift},
  address = {Technische Universit{\"a}t Berlin},
  year = {1998},
  file = {:./files/1998-Martin.pdf:PDF},
  url = {http://www.zib.de/Publications/abstracts/SC-99-03/}
}

@INPROCEEDINGS{1998a-MartinWeismantel,
  author = {Alexander Martin and Robert Weismantel},
  title = {The Intersection of Knapsack Polyhedra and Extensions},
  booktitle = {Integer Programming and Combinatorial Optimization},
  year = {1998},
  editor = {Robert E. Bixby and E.A. Boyd and R.Z.R{\'i}os-Mercado},
  series = {Proceedings of the 6th IPCO Conference},
  pages = {243-256},
  file = {:./files/1998a-MartinWeismantel.pdf:PDF},
  url = {http://www.zib.de/Publications/abstracts/SC-97-61/}
}

@TECHREPORT{1998-MartinWeismantel,
  author = {Alexander Martin and Robert Weismantel},
  title = {Conjunctive Cuts for Integer Programs},
  institution = {Zuse Institute Berlin},
  year = {1998},
  number = {98-18},
  file = {:./files/1998-MartinWeismantel.pdf:PDF},
  url = {http://www.zib.de/Publications/abstracts/SC-98-18/}
}

@TECHREPORT{1997-MartinWeismantel,
  author = {Alexander Martin and Robert Weismantel},
  title = {Contributions to General Mixed Integer Knapsack Problems},
  institution = {Zuse Institute Berlin},
  year = {1997},
  number = {97-38},
  file = {:./files/1997-MartinWeismantel.pdf:PDF},
  url = {http://www.zib.de/Publications/abstracts/SC-97-38/}
}

@INPROCEEDINGS{2016-MarxVillarraga.etal,
  author = {Oliver Marx and Carlos Villarraga and Dominik Stoffel and Wolfgang
	Kunz},
  title = {A Computer-Algebraic Approach to Formal Verification of Data-Centric
	Low-Level Software},
  booktitle = {14. ACM-IEEE International Conference on Formal Methods and Models
	for Codesign ({MEMOCODE}) (to appear)},
  year = {2016},
  file = {2016-MarxVillarraga.etal.pdf:files/2016-MarxVillarraga.etal.pdf:PDF},
  owner = {villarraga},
  timestamp = {2016.10.18}
}

@INPROCEEDINGS{2013a-MarxWedler.etal,
  author = {Oliver Marx and Markus Wedler and Alexander Dreyer and Dominik Stoffel
	and Wolfgang Kunz},
  title = {Proof Logging for Computer Algebra based SMT Solving},
  booktitle = {16. {GI/ITG/GMM} Workshop Methoden und Beschreibungssprachen zur
	Modellierung und Verifikation von Schaltungen und Systemen ({MBMV})},
  year = {2013},
  file = {Paper:files/2013a-MarxWedler.etal.pdf:PDF},
  owner = {marx},
  timestamp = {2013.11.11}
}

@INPROCEEDINGS{1996-Matsunaga,
  author = {Y. Matsunaga},
  title = {An Efficient Equivalence Checker for Combinational Circuits},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {1996},
  pages = {629-634},
  month = {June},
  file = {:./files/1996-Matsunaga.pdf:PDF}
}

@INPROCEEDINGS{2000-Maurer,
  author = {Peter M. Maurer},
  title = {Event Driven Simulation Without Loops or Conditionals},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2000},
  pages = {23 -26},
  file = {:./files/2000-Maurer.pdf:PDF},
  keywords = {delay model;event driven simulation;gate simulation;logic model;logic
	simulation;scheduling;subroutine addresses;delays;logic CAD;logic
	simulation;},
  timestamp = {2006.09.21}
}

@BOOK{1986-McCluskey,
  title = {Logic Design Principles},
  publisher = {Prentice-Hall},
  year = {1986},
  author = {E. McCluskey},
  address = {Englewood Cliffs, NJ}
}

@ARTICLE{1956-McCluskey,
  author = {E. McCluskey},
  title = {Minimization of {Boolean} Functions},
  journal = {Bell System Technical Journal},
  year = {1956},
  volume = {35},
  pages = {1417-1444},
  file = {:./files/1956-McCluskey.pdf:PDF}
}

@ARTICLE{2002-McCuneVeroff.etal,
  author = {W. McCune and R. Veroff and B. Fitelson and K. Harris and A. Feist
	and L. Wos},
  title = {Short Single Axioms for {Boolean} Algebra},
  journal = {Journal of Automated Reasoning},
  year = {2002},
  volume = {29},
  pages = {1-16},
  file = {:./files/2002-McCuneVeroff.etal.pdf:PDF}
}

@INPROCEEDINGS{1993-McGeerSanghavi.etal,
  author = {P. McGeer and J. Sanghavi and R. Brayton and A. Sangiovanni-Vincentelli},
  title = {{ESPRESSO-SIGNATURES}: A New Exact Minimizer for Logic Functions},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {1993},
  pages = {618-621},
  file = {:./files/1993-McGeerSanghavi.etal.pdf:PDF}
}

@MISC{1999a-McMillan,
  author = {K.L. McMillan},
  title = {The {SMV} Language},
  year = {1999},
  file = {:./files/1999a-McMillan.pdf:PDF},
  owner = {nguyen},
  timestamp = {2007.02.02}
}

@TECHREPORT{1999b-McMillan,
  author = {K.L. McMillan},
  title = {A Metholodogy for Hardware Verification using Compositional Model
	Checking},
  institution = {Cadence},
  year = {1999},
  file = {:./files/1999b-McMillan.pdf:PDF},
  timestamp = {2006.09.13}
}

@MISC{1999-McMillan,
  author = {K.L. McMillan},
  title = {Getting Started with {SMV}},
  year = {1999},
  file = {:./files/1999-McMillan.pdf:PDF},
  owner = {nguyen},
  timestamp = {2007.02.02}
}

@MISC{2000-McMillan,
  author = {K. L. McMillan},
  title = {Cadence {SMV}},
  owner = {stoffel},
  timestamp = {2016.05.11},
  url = {http://www-cad.eecs.berkeley.edu/~kenmcmil/}
}

@INPROCEEDINGS{2003-McMillan,
  author = {K. L. McMillan},
  title = {Interpolation and {SAT}-based Model Checking},
  booktitle = {Proc. International Conference on Computer Aided Verification ({CAV})},
  year = {2003},
  pages = {1--13},
  file = {:./files/2003-McMillan.pdf:PDF},
  timestamp = {2006.09.19}
}

@INPROCEEDINGS{2002-McMillan,
  author = {K. L. McMillan},
  title = {Applying {SAT} Methods in Unbounded Symbolic Model Checking},
  booktitle = {Proc. International Conference on Computer Aided Verification ({CAV})},
  year = {2002},
  pages = {250--264},
  publisher = {Springer-Verlag},
  file = {:./files/2002-McMillan.pdf:PDF},
  timestamp = {2006.09.19}
}

@INPROCEEDINGS{1997-McMillan,
  author = {McMillan, Kenneth L.},
  title = {A Compositional Rule for Hardware Design Refinement},
  booktitle = {Proceedings of the 9th International Conference on Computer Aided
	Verification},
  year = {1997},
  series = {CAV '97},
  pages = {24--35},
  address = {London, UK, UK},
  publisher = {Springer-Verlag},
  acmid = {733598},
  isbn = {3-540-63166-6},
  numpages = {12},
  owner = {bao},
  timestamp = {2012.11.22}
}

@INPROCEEDINGS{1996-McMillan,
  author = {Kenneth L. McMillan},
  title = {A Conjunctively Decomposed {Boolean} Representation for Symbolic
	Model Checking},
  booktitle = {Proc. International Conference on Computer Aided Verification ({CAV})},
  year = {1996},
  pages = {13--25},
  publisher = {Springer-Verlag},
  file = {:./files/1996-McMillan.pdf:PDF},
  isbn = {3-540-61474-5}
}

@BOOK{1993-McMillan,
  title = {Symbolic Model Checking},
  publisher = {Kluwer Academic Publishers},
  year = {1993},
  author = {K. L. McMillan},
  address = {Boston}
}

@INPROCEEDINGS{2003a-McMillanAmla,
  author = {Kenneth L. McMillan and Nina Amla},
  title = {Automatic Abstraction without Counterexamples.},
  booktitle = {Proc. International Conference on Tools and Algorithms for the Construction
	and Analysis of Systems ({TACAS})},
  year = {2003},
  pages = {2-17},
  bibsource = {DBLP, http://dblp.uni-trier.de},
  file = {:./files/2003a-McMillanAmla.pdf:PDF},
  owner = {nguyen},
  timestamp = {2007.04.12},
  url = {http://link.springer.de/link/service/series/0558/bibs/2619/26190002.htm}
}

@ARTICLE{2003-McMillanAmla,
  author = {K. L. McMillan and Nina Amla},
  title = {Automatic Abtraction without Counterexamples},
  journal = {Cadence Berkeley},
  year = {2003},
  comment = {Lecture Notes in Computer Science},
  file = {:./files/2003-McMillanAmla.pdf:PDF},
  owner = {stoffel},
  timestamp = {2006.09.12}
}

@ARTICLE{McMillanAmla2003,
  author = {K. L. McMillan and Nina Amla},
  title = {Automatic Abtraction without Counter Examples},
  journal = {Cadence Berkeley},
  year = {2003},
  comment = {Lecture Notes in Computer Science},
  file = {:./files/2003-McMillanAmla.pdf:PDF},
  timestamp = {2006.09.12}
}

@INPROCEEDINGS{2000-MeinelStangier,
  author = {Christoph Meinel and Christian Stangier},
  title = {Speeding Up Image Computation by Using {RTL} Information},
  booktitle = {Proc. International Conference on Formal Methods in Computer-Aided
	Design ({FMCAD})},
  year = {2000},
  pages = {443-454},
  file = {:./files/2000-MeinelStangier.pdf:PDF},
  url = {citeseer.ist.psu.edu/meinel00speeding.html}
}

@MISC{web-mentor,
  author = {{Mentor Graphics}},
  howpublished = {https://www.mentor.com/},
  key = {mentor},
  owner = {ludwig},
  timestamp = {2016.05.11}
}

@MANUAL{1996-MentorGraphics,
  title = {Getting Started with Seamless},
  author = {{Mentor Graphics}},
  year = {1996},
  file = {:./files/1996-MentorGraphics.pdf:PDF},
  timestamp = {2006.09.27}
}

@MISC{0000-MercerJones,
  author = {Eric Mercer and Michael Jones},
  title = {A Concurrency Model for Real-time Verification of Embedded Software
	at the Object-Level},
  abstract = {Abstract. We present an asynchronous concurrency model based on networks
	of labeled automata, and we show how object code can be represented
	using this model. A verification tool based on the model is implemented
	using the GNU debugger to provide operational semantics of binary
	executable files. The mapping of object code to networks of labeled
	automata includes a notion of processor time represented as a discrete
	counter. Real-time concurrency errors are preserved in this model
	because discrete time semantics exactly match the host processor?s
	perspective of the world. We mitigate the complexity in state generation
	for the concurrency model by selectively storing states and memory
	contents. We show that these selective storage reduction techniques
	preserve a live variable bisimulation between the complete and reduced
	transition systems. Verification results are given for several simple
	programs and are validated on actual hardware.},
  file = {0000-MercerJones.pdf:files/0000-MercerJones.pdf:PDF},
  owner = {nguyen},
  timestamp = {2006.08.29}
}

@INPROCEEDINGS{2005-MercerJones,
  author = {Eric Mercer and Michael Jones},
  title = {Model Checking Machine Code with the {GNU} Debugger},
  booktitle = {Proc. SPIN Workshop on Model Checking Software},
  year = {2005},
  volume = {Volume LNCS 3639},
  series = {Lecture Notes in Computer Science},
  pages = {251--265},
  publisher = {Springer Verlag},
  abstract = {Abstract. Embedded software verification is an important verification
	problem that requires the ability to reason about the timed semantics
	of concurrent behaviors at a low level of atomicity. The level of
	atomicity is the smallest execution block (such as a machine instruction
	or a C instruction) that cannot be split by an interrupt. Combining
	a cycleaccurate debugger with model checking algorithms provides
	an accurate model of software execution at the machine-code level
	while supporting concurrency and allowing abstractions to manage
	state explosion. We report on the design and implementation of such
	a model checker using the GNU debugger (gdb) with different processor
	backends. A significant feature of the resulting tool is that we
	can adjust the level of atomicity during the model checking run to
	reduce state explosion while focusing on behaviors that are likely
	to generate an error.},
  comment = {In the introduction section, the paper explain why the executable
	code level should be considered but not the C-code level. (C-instructions
	are not automic, the can be interrupted by an interrupt routine,
	which leads to bugs because of interleave events).},
  file = {:./files/2005-MercerJones.pdf:PDF},
  keywords = {Embedded Software Verification, Model Checking, GDB},
  owner = {nguyen},
  timestamp = {2006.08.28}
}

@INPROCEEDINGS{1991-MichelLeveugle.etal,
  author = {T. Michel and R. Leveugle and G. Saucier},
  title = {A new approach to control flow checking without program modification},
  booktitle = {21st International Symposium on Fault-Tolerant Computing},
  year = {1991},
  pages = {334-341},
  month = {June},
  file = {1991-MichelLeveugle.etal.pdf:files/1991-MichelLeveugle.etal.pdf:PDF},
  owner = {bartsch},
  timestamp = {2016.09.21}
}

@BOOK{1994-DeMicheli,
  title = {Synthesis and Optimization of Digital Circuits},
  publisher = {McGraw-Hill},
  year = {1994},
  author = {Giovanni De Micheli},
  key = {DeMi94}
}

@ARTICLE{2014-Miele,
  author = {Antonio Miele},
  title = {A fault-injection methodology for the system-level dependability
	analysis of multiprocessor embedded systems },
  journal = {Microprocessors and Microsystems },
  year = {2014},
  volume = {38},
  pages = {567 - 580},
  number = {6},
  file = {2014-Miele.pdf:files/2014-Miele.pdf:PDF},
  issn = {0141-9331},
  keywords = {Dependability analysis},
  owner = {stoffel},
  timestamp = {2016.08.15}
}

@INCOLLECTION{1990-Milner,
  author = {Milner, Robin},
  title = {Operational and algebraic semantics of concurrent processes},
  booktitle = {Handbook of theoretical computer science (vol. B)},
  publisher = {MIT Press},
  year = {1990},
  editor = {van Leeuwen, Jan},
  pages = {1201--1242},
  address = {Cambridge, MA, USA},
  acmid = {114910},
  isbn = {0-444-88074-7},
  numpages = {42},
  owner = {joakim},
  timestamp = {2013.09.05}
}

@INPROCEEDINGS{1993-Minato,
  author = {Minato, Shin-ichi},
  title = {Zero-suppressed {BDDs} for set manipulation in combinatorial problems},
  booktitle = {{DAC} '93: Proceedings of the 30th international Design Automation
	Conference},
  year = {1993},
  pages = {272--277},
  address = {New York, NY, USA},
  publisher = {ACM},
  file = {:./files/1993-Minato.pdf:PDF},
  isbn = {0-89791-577-1},
  location = {Dallas, Texas, United States},
  owner = {pavlenko},
  timestamp = {2010.08.03}
}

@MISC{2003-Minea,
  author = {Marius Minea},
  title = {Formal Verification: from Challenges to Solutions},
  year = {2003},
  file = {:./files/2003-Minea.pdf:PDF},
  owner = {stoffel},
  timestamp = {2006.09.21}
}

@INPROCEEDINGS{1994-MinerPullela.etal,
  author = {Miner, P.S. and Pullela, S. and Johnson, S.D.},
  title = {Interaction of Formal Design Systems in the Development of a Fault-Tolerant
	Clock Synchronization Circuit1},
  booktitle = {Reliable Distributed Systems, 1994. Proceedings., 13th Symposium
	on},
  year = {1994},
  pages = {128 -137},
  month = {oct},
  file = {:./files/1994-MinerPullela.etal.pdf:PDF},
  keywords = { clock synchronization; fault-tolerant; fault-tolerant clock synchronization
	circuit; formal design systems; gate-level realization; high-level
	specifications; mechanical theorem prover; circuit reliability; formal
	specification; logic design; logic testing;},
  timestamp = {2006.09.14}
}

@ARTICLE{2012-MiorandiSicari.etal,
  author = {Daniele Miorandi and Sabrina Sicari and Francesco De Pellegrini and
	Imrich Chlamtac},
  title = {Internet of things: Vision, applications and research challenges
	},
  journal = {Ad Hoc Networks },
  year = {2012},
  volume = {10},
  pages = {1497 - 1516},
  number = {7},
  abstract = {The term “Internet-of-Things” is used as an umbrella keyword for covering
	various aspects related to the extension of the Internet and the
	Web into the physical realm, by means of the widespread deployment
	of spatially distributed devices with embedded identification, sensing
	and/or actuation capabilities. Internet-of-Things envisions a future
	in which digital and physical entities can be linked, by means of
	appropriate information and communication technologies, to enable
	a whole new class of applications and services. In this article,
	we present a survey of technologies, applications and research challenges
	for Internet-of-Things. },
  issn = {1570-8705},
  keywords = {Internet-of-Things},
  owner = {schwarz},
  timestamp = {2017.01.09},
  url = {http://www.sciencedirect.com/science/article/pii/S1570870512000674}
}

@ARTICLE{2000-MirBalakrishnan.etal,
  author = {Ali Abbas Mir and Subhashini Balakrishnan and Sofiene Tahar},
  title = {Modeling And Verification Of Embedded Systems Using Cadence SMV},
  journal = {Canadian Electrical and Computer Engineering},
  year = {2000},
  file = {:./files/2000-MirBalakrishnan.etal.pdf:PDF},
  timestamp = {2006.09.27}
}

@TECHREPORT{2001-Mishchenko,
  author = {Alan Mishchenko},
  title = {An introduction to zero-suppressed binary decision diagrams},
  institution = {in Proceedings of the 12th Symposium on the Integration of Symbolic
	Computation and Mechanized Reasoning},
  year = {2001},
  file = {:./files/2001-Mishchenko.pdf:PDF},
  owner = {pavlenko},
  timestamp = {2010.08.03}
}

@ARTICLE{2006-MishchenkoBrayton,
  author = {A. Mishchenko and R.K. Brayton},
  title = {A Theory of Nondeterministic Networks},
  journal = {{IEEE} Transactions on Computer-Aided Design},
  year = {2006},
  volume = {25},
  pages = {977-999},
  number = {6},
  month = {June},
  file = {:./files/2006-MishchenkoBrayton.pdf:PDF},
  owner = {wedler},
  timestamp = {2006.09.12}
}

@ARTICLE{2006-MishchenkoZhang.etal,
  author = {Alan Mishchenko and Jin S. Zhang and Subarna Sinha and Jerry R. Burch
	and Robert Brayton and Malgorzata Chrzanowska-Jeske},
  title = {Using Simulation and Satisfiability to Compute Flexibilities in Boolean
	Networks},
  journal = {{IEEE} Transaction on Computer-Aided Design},
  year = {2006},
  volume = {25},
  pages = {743},
  file = {:./files/2006-MishchenkoZhang.etal.pdf:PDF},
  owner = {nguyen},
  timestamp = {2007.02.02}
}

@INPROCEEDINGS{2001-MitraMcCluskey,
  author = {Subhasish Mitra and Edward J. McCluskey},
  title = {Design Diversity For Concurrent Error Detection In Sequential Logic
	Circuits},
  booktitle = {Proc. {IEEE} {VLSI} Test Symposium},
  year = {2001},
  pages = {178 -183},
  file = {:./files/2001-MitraMcCluskey.pdf:PDF},
  keywords = {common-mode failures;comparators;computational complexity;concurrent
	error detection;data integrity analysis;design diversity;diverse
	combinational logic implementation;diverse duplication;flip-flops;multiple
	failures;parity checkers;parity prediction;sequential logic circuits;state
	encoding;VLSI;computational complexity;data integrity;error detection;flip-flops;integrated
	circuit testing;integrated logic circuits;logic design;logic testing;sequential
	circuits;},
  timestamp = {2006.09.14}
}

@INPROCEEDINGS{2000-MitraMcCluskey,
  author = {Subhasish Mitra and Edward J. McCluskey},
  title = {Combinational Logic Synthesis for Diversity In Duplex Systems},
  booktitle = {Proc. International Test Conference},
  year = {2000},
  pages = {179 -188},
  file = {:./files/2000-MitraMcCluskey.pdf:PDF},
  keywords = {combinational logic circuits;combinational logic synthesis;common-mode
	failures;cost function;data integrity;design diversity;diverse duplex
	system;diverse duplex systems;diversity metric;fault tolerance;multilevel
	logic synthesis;synthesis;two level synthesis;combinational circuits;data
	integrity;fault diagnosis;high level synthesis;optimisation;},
  timestamp = {2006.09.14},
  url = {http://crc.stanford.edu}
}

@MISC{2001a-MitraSaxena.etal,
  author = {Subhasish Mitra and Nirmal R. Saxena and Edward J. McCluskey},
  title = {Evaluation And Design Of Dependable Systems With Design Diversity},
  year = {2001},
  file = {:./files/2001a-MitraSaxena.etal.pdf:PDF},
  owner = {stoffel},
  timestamp = {2006.09.14}
}

@INPROCEEDINGS{2001-MitraSaxena.etal,
  author = {Subhasish Mitra and Nirmal R. Saxena and Edward J. McCluskey},
  title = {Techniques For Estimation Of Design Diversity For Combinational Logic
	Circuits},
  booktitle = {Proc. International Conference on Dependable Systems and Networks
	(formerly: FTCS)},
  year = {2001},
  file = {:./files/2001-MitraSaxena.etal.pdf:PDF},
  timestamp = {2006.09.14},
  url = {http://crc.stanford.edu}
}

@INPROCEEDINGS{2000-MitraSaxena.etal,
  author = {Subhasish Mitra and Nirmal R. Saxena and Edward J. McCluskey},
  title = {Fault Escapes In Duplex Systems},
  booktitle = {Proc. {IEEE} {VLSI} Test Symposium ({VTS})},
  year = {2000},
  pages = {453 -458},
  file = {:./files/2000-MitraSaxena.etal.pdf:PDF},
  keywords = {common-mode failures;concurrent error detection;data integrity;duplex
	systems;hardware duplication techniques;non-self-testable faults;test
	point insertion;test points;user-programmable logic elements;built-in
	self test;comparators (circuits);error detection;failure analysis;fault
	diagnosis;logic testing;modules;redundancy;},
  timestamp = {2006.09.14}
}

@INPROCEEDINGS{1999-MitraSaxena.etal,
  author = {Subhasish Mitra and Nirmal R. Saxena and Edward J. McCluskey},
  title = {Design Diversity For Redundant Systems},
  year = {1999},
  file = {:./files/1999-MitraSaxena.etal.pdf:PDF},
  timestamp = {2006.09.14}
}

@ARTICLE{2005-MitraSeifert.etal,
  author = {S. Mitra and N. Seifert and M. Zhang and Q. Shi and K. S. Kim},
  title = {Robust system design with built-in soft-error resilience},
  journal = {Computer},
  year = {2005},
  volume = {38},
  pages = {43-52},
  number = {2},
  month = {February},
  file = {2005-MitraSeifert.etal.pdf:files/2005-MitraSeifert.etal.pdf:PDF},
  issn = {0018-9162},
  owner = {bartsch},
  timestamp = {2016.09.21}
}

@MISC{2003-Mittelmann,
  author = {Hans Mittelmann},
  title = {Decision Tree for Optimization Software: Benchmarks for Optimization
	Software},
  year = {2003},
  owner = {stoffel},
  timestamp = {2016.05.11},
  url = {http://plato.asu.edu/bench.html}
}

@ARTICLE{2019-MoghimiWichelmann.etal,
  author = {Moghimi, Ahmad and Wichelmann, Jan and Eisenbarth, Thomas and Sunar,
	Berk},
  title = {Memjam: A false dependency attack against constant-time crypto implementations},
  journal = {International Journal of Parallel Programming},
  year = {2019},
  volume = {47},
  pages = {538--570},
  number = {4},
  publisher = {Springer}
}

@INPROCEEDINGS{2005-MondalMassoud,
  author = {Mosin Mondal and Yehia Massoud},
  title = {Reducing Pessimism in {RLC} Delay Estimation Using an Accurate Analytical
	Frequency Dependent Model for Inductance},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2005},
  pages = { 691 - 696},
  file = {:./files/2005-MondalMassoud.pdf:PDF},
  keywords = { RLC delay estimation; RLC propagation delay; analytical frequency
	dependent model; chip design; loop self inductance; RLC circuits;
	delay estimation; inductance; integrated circuit design;},
  timestamp = {2006.09.27}
}

@INPROCEEDINGS{2000-MonteiroOliveira,
  author = {Jose C. Monteiro and Arlindo L. Oliveira},
  title = {{FSM} decomposition by direct circuit manipulation applied to low
	power design},
  booktitle = {Proc. Asia and South Pacific Design Automation Conference ({ASPDAC})},
  year = {2000},
  pages = {351--358},
  address = {New York, NY, USA},
  publisher = {ACM Press},
  file = {:./files/2000-MonteiroOliveira.pdf:PDF},
  isbn = {0-7803-5974-7},
  location = {Yokohama, Japan}
}

@INPROCEEDINGS{1999-MoonKukula.etal,
  author = {In-Ho Moon and James Kukula and Tom Shiple and Fabio Somenzi},
  title = {Least Fixpoint Approximations for Reachability Analysis},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {1999},
  pages = {41-44},
  file = {:./files/1999-MoonKukula.etal.pdf:PDF}
}

@INPROCEEDINGS{2000-MoonKukula,
  author = {In-Ho Moon and James H. Kukula and Kavita Ravi and Fabio Somenzi},
  title = {To Split or to Conjoin: the Question in Image Computation},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {2000},
  pages = {23-28},
  file = {:./files/2000-MoonKukula.pdf:PDF}
}

@ARTICLE{1965-Moore,
  author = {Gordon E. Moore},
  title = {Cramming more components onto integrated circuits},
  journal = {Electronics},
  year = {1965},
  volume = {38},
  pages = {114},
  number = {8},
  month = {April},
  file = {:./files/1965-Moore.pdf:PDF},
  owner = {pavlenko},
  timestamp = {2011.01.06}
}

@MISC{2002-MoreTerpstra,
  author = {Shirley More and Dan Terpstra},
  title = {Using Performance Monitoring Hardware for Application Performance
	Analysis},
  howpublished = {International Conference on High Performance Computing In Asia Pacific
	Region (HPC ASIA)},
  month = {12},
  year = {2002},
  note = {Tutorial slides},
  file = {:./files/2002-MoreTerpstra.ppt:PPT},
  owner = {nguyen},
  timestamp = {2007.02.02}
}

@INPROCEEDINGS{2006-MorinAlloryBorrione,
  author = {Katell Morin-Allory and Dominique Borrione},
  title = {Proven correct monitors from {PSL} specifications},
  booktitle = {Proc. International Conference on Design, Automation and Test in
	Europe ({DATE})},
  year = {2006},
  file = {:./files/2006-MorinAlloryBorrione.pdf:PDF},
  isbn = {3-9810801-0-6},
  keywords = {PSL FL operators;PSL specifications;PSL standard;PVS theorem proven;declarative
	specification monitor;design verification;hardware description languages;integrated
	circuit design;logic design;system-on-chip;theorem proving;},
  location = {Munich, Germany},
  owner = {nguyen},
  timestamp = {2007.04.30}
}

@ARTICLE{2000-Mosensoson,
  author = {Guy Mosensoson},
  title = {Practical Approaches to {SoC} Verification},
  journal = {Verisity Design Systems},
  year = {2000},
  file = {:./files/2000-Mosensoson.pdf:PDF},
  timestamp = {2006.09.21}
}

@INPROCEEDINGS{2001-MoskewiczMadigan.etal,
  author = {Matthew W. Moskewicz and Conor F. Madigan and Ying Zhao and Lintao
	Zhang and Sharad Malik},
  title = {Chaff: Engineering an Efficient {SAT} Solver},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {2001},
  pages = { 530 - 535},
  file = {:./files/2001-MoskewiczMadigan.etal.pdf:PDF},
  keywords = { {Boolean} constraint propagation; {Boolean} satisfiability; Chaff;
	SAT benchmarks; SAT solver; artificial intelligence; electronic design
	automation; low overhead decision strategy; {Boolean} functions;
	computational complexity; constraint theory; electronic design automation;
	formal verification;},
  url = {citeseer.ist.psu.edu/moskewicz01chaff.html}
}

@MISC{2000-Moszkowski,
  author = {Ben Moszkowski},
  title = {Executing Temporal Logic Programs},
  year = {2000},
  file = {:./files/2000-Moszkowski.pdf:PDF},
  owner = {stoffel},
  timestamp = {2006.09.13}
}

@INPROCEEDINGS{1998-Moszkowski,
  author = {B.C Moszkowski},
  title = {Compositional Reasoning Using Interval Temporal Logic and Tempura},
  booktitle = {Revised Lectures from the International Symposium on Compositionality:
	The Significant Difference},
  year = {1998},
  series = {COMPOS'97},
  pages = {439--464},
  address = {London, UK, UK},
  publisher = {Springer-Verlag},
  acmid = {701954},
  file = {:./files/1998-Moszkowski.pdf:PDF},
  isbn = {3-540-65493-3},
  numpages = {26},
  timestamp = {2006.09.13}
}

@INPROCEEDINGS{2008-MouraBjorner,
  author = {Leonardo De Moura and Nikolaj Bj{\o}rner},
  title = {Z3: An Efficient {SMT} Solver},
  booktitle = {Conference on Tools and Algorithms for the Construction and Analysis
	of Systems (TACAS)},
  year = {2008},
  pages = {337--340},
  address = {Berlin, Heidelberg},
  publisher = {Springer-Verlag},
  acmid = {1792766},
  file = {:./files/2008-MouraBjorner.pdf:PDF},
  isbn = {3-540-78799-2, 978-3-540-78799-0},
  location = {Budapest, Hungary},
  numpages = {4},
  owner = {pavlenko},
  timestamp = {2010.07.26}
}

@INPROCEEDINGS{2007-MouraBjoerner,
  author = {Leonardo Mendon\c{c}a de Moura and Nikolaj Bjoerner},
  title = {Efficient E-Matching for {SMT} Solvers},
  booktitle = {CADE},
  year = {2007},
  editor = {Frank Pfenning},
  volume = {4603},
  series = {Lecture Notes in Computer Science},
  pages = {183-198},
  publisher = {Springer},
  date = {2007-09-05},
  description = {dblp},
  file = {:./files/2007-MouraBjoerner.pdf:PDF},
  isbn = {978-3-540-73594-6},
  keywords = {dblp}
}

@PHDTHESIS{2005-Moy,
  author = {Matthieu Moy},
  title = {Techniques and Tools for the Verification of Systems-on-a-Chip at
	the Transaction Level},
  school = {INPG, Grenoble, France},
  year = {2005},
  month = {December},
  file = {these-en.pdf:these-en.pdf:PDF},
  owner = {nguyen},
  timestamp = {2007.07.10},
  url = {http://www-verimag.imag.fr/~moy/phd/}
}

@INPROCEEDINGS{2000-MunchWurth.etal,
  author = {M. Muench and B. Wurth and R. Mehra and J. Sproch and N. Wehn},
  title = {Automating {RT}-level Operand Isolation to Minimize Power Consumption
	in Datapaths},
  booktitle = {Proc. Conf. on Design, Automation and Test in Europe (DATE)},
  year = {2000},
  pages = {624--633},
  numpages = {10},
  owner = {udupi},
  timestamp = {2015.05.05}
}

@INPROCEEDINGS{2017-mukherjee.etal,
  author = {Mukherjee, Rajdeep and Purandare, Mitra and Polig, Raphael and Kroening,
	Daniel},
  title = {Formal techniques for effective co-verification of hardware/software
	co-designs},
  booktitle = {Proceedings of the 54th Annual Design Automation Conference 2017},
  year = {2017},
  pages = {35},
  organization = {ACM},
  owner = {schwarz},
  timestamp = {2018.11.23}
}

@INPROCEEDINGS{2003-MukherjeeWeaver.etal,
  author = {S. S. Mukherjee and C. Weaver and J. Emer and S. K. Reinhardt and
	T. Austin},
  title = {A systematic methodology to compute the architectural vulnerability
	factors for a high-performance microprocessor},
  booktitle = {Microarchitecture, 2003. MICRO-36. Proceedings. 36th Annual IEEE/ACM
	International Symposium on},
  year = {2003},
  pages = {29-40},
  month = {Dec},
  file = {2003-MukherjeeWeaver.etal.pdf:files/2003-MukherjeeWeaver.etal.pdf:PDF},
  owner = {villarraga},
  timestamp = {2016.08.18}
}

@ARTICLE{1989-MurogaKambayashi.etal,
  author = {Muroga, S. and Kambayashi, Y. and Lai, H.C. and Culliney, J.N.},
  title = {The Transduction Method - Design of Logic Networks Based on Permissible
	Functions},
  journal = {Computers, IEEE Transactions on},
  year = {1989},
  volume = {38},
  pages = {1404 -1424},
  number = {10},
  month = {oct},
  file = {:./files/1989-MurogaKambayashi.etal.pdf:PDF},
  issn = {0018-9340},
  keywords = {heuristic procedure;logic networks;permissible functions;transduction
	method;logic circuits;logic design;}
}

@INPROCEEDINGS{2018-MushtaqAkram.etal,
  author = {Mushtaq, Maria and Akram, Ayaz and Bhatti, Muhammad Khurram and Chaudhry,
	Maham and Lapotre, Vianney and Gogniat, Guy},
  title = {{NIGHTs-WATCH}: a cache-based side-channel intrusion detector using
	hardware performance counters},
  booktitle = {Proceedings of the 7th International Workshop on Hardware and Architectural
	Support for Security and Privacy},
  year = {2018},
  pages = {1},
  organization = {ACM},
  owner = {fadiheh},
  timestamp = {2018.07.12}
}

@INPROCEEDINGS{2007-MusuvathiMadanlal.etal,
  author = {Musuvathi, Madanlal and Qadeer, Shaz},
  title = {Iterative context bounding for systematic testing of multithreaded
	programs},
  booktitle = {Proceedings of the 2007 {ACM} {SIGPLAN} {C}onference on {P}rogramming
	{L}anguage {D}esign and {I}mplementation},
  year = {2007},
  series = {PLDI '07},
  pages = {446--455},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {1250785},
  file = {2007-MusuvathiMadanlal.etal.pdf:files/2007-MusuvathiMadanlal.etal.pdf:PDF},
  isbn = {978-1-59593-633-2},
  keywords = {concurrency, context-bounding, model checking, multithreading, partial-order
	reduction, shared-memory programs, software testing},
  location = {San Diego, California, USA},
  numpages = {10},
  owner = {villarraga},
  timestamp = {2012.08.27}
}

@ARTICLE{1976-Muth,
  author = {P. Muth},
  title = {A Nine-Valued Logic Model for Test Generation},
  journal = {{IEEE} Transactions on Computers},
  year = {1976},
  volume = {C-25},
  pages = {630-636},
  number = {6},
  month = {June},
  file = {:./files/1976-Muth.pdf:PDF}
}

@INPROCEEDINGS{2008-MyreenGordon.etal,
  author = {Myreen, M.O. and Gordon, M. and Slind, K.},
  title = {Machine-Code Verification for Multiple Architectures - An Application
	of Decompilation into Logic},
  booktitle = {Formal Methods in Computer-Aided Design, 2008. {FMCAD} '08},
  year = {2008},
  pages = {1 -8},
  month = {nov.},
  file = {:./files/2008-MyreenGordon.etal.pdf:PDF},
  keywords = {commercial processors;formal specifications;logic;machine languages;machine-code
	verification;multiple architectures;formal logic;formal specification;program
	compilers;program verification;software architecture;}
}

@INPROCEEDINGS{1999-AmlaEmerson.etal,
  author = {N.Amla and Allen E.Emerson and Kedar S.Namjoshi},
  title = {Efficient Decompositional Model-Checking for Regular Timing Diagrams},
  booktitle = {Proc. {IFIP} WG 10.5 Advanced Research Working Conference on Correct
	Hardware Design and Verification Methods},
  year = {1999},
  pages = {67--81},
  file = {:./files/1999-AmlaEmerson.etal.pdf:PDF},
  timestamp = {2006.09.19}
}

@ARTICLE{2008Nagappan.etal,
  author = {Nagappan, Nachiappan and Maximilien, E. Michael and Bhat, Thirumalesh
	and Williams, Laurie},
  title = {Realizing quality improvement through test driven development: results
	and experiences of four industrial teams},
  journal = {Empirical Software Engineering},
  year = {2008},
  volume = {13},
  pages = {289--302},
  number = {3},
  month = {Jun},
  day = {01}
}

@PHDTHESIS{1975-Nagel,
  author = {Nagel, Laurence W.},
  title = {SPICE2: A Computer Program to Simulate Semiconductor Circuits},
  school = {EECS Department, University of California, Berkeley},
  year = {1975},
  number = {UCB/ERL M520},
  owner = {stoffel},
  timestamp = {2016.05.10}
}

@MISC{2011-NangateSi2,
  author = {{NANGATE} and {Si2}},
  title = {NanGate Open Cell Library},
  month = {8},
  year = {2011},
  organization = {Silicon Integration Initiative ({Si2})},
  owner = {stoffel},
  timestamp = {2016.04.25},
  url = {http://projects.si2.org/openeda.si2.org/projects/nangatelib}
}

@INPROCEEDINGS{1997-NarayanIsles.etal,
  author = {Amit Narayan and Adrian J. Isles and Jawahar Jain and Robert K. Brayton
	and Alberto L. Sangiovanni-Vincentelli},
  title = {Reachability Analysis Using Partitioned-{ROBDDs}},
  booktitle = {Proc. International Conference on Computer-Aided Design},
  year = {1997},
  pages = {388--393},
  publisher = {IEEE Computer Society},
  file = {:./files/1997-NarayanIsles.etal.pdf:PDF},
  isbn = {0-8186-8200-0},
  location = {San Jose, California, United States}
}

@TECHREPORT{2001-NediakEckstein,
  author = {Mikhail Nediak and Jonathan Eckstein},
  title = {Pivot, Cut, and Dive: A Heuristic for 0-1 Mixed Integer Programming},
  institution = {Rutgers University},
  year = {2001},
  number = {RRR 53-2001},
  file = {:./files/2001-NediakEckstein.pdf:PDF}
}

@MISC{2004-NemhauserSavelsbergh,
  author = {George L. Nemhauser and Martin W.P. Savelsbergh},
  title = {{MINTO} 3.1},
  year = {2004},
  owner = {stoffel},
  timestamp = {2016.05.11},
  url = {http://coral.ie.lehigh.edu/~minto}
}

@ARTICLE{1994-NemhauserSavelsbergh.etal,
  author = {George L. Nemhauser and Martin W.P. Savelsbergh and Gabriele C. Sigismondi},
  title = {{MINTO} a Mixed Integer Optimizer},
  journal = {Operations Research Letters},
  year = {1994},
  volume = {15},
  pages = {47-58},
  file = {:./files/1994-NemhauserSavelsbergh.etal.pdf:PDF}
}

@BOOK{1988-NemhauserWolsey,
  title = {Integer and Combinatorial Optimization},
  publisher = {John Wiley \& Sons},
  year = {1988},
  author = {George L. Nemhauser and Laurence A. Wolsey}
}

@INPROCEEDINGS{2003-NeumannStoffel.etal,
  author = {I. Neumann and D. Stoffel and M. Berkelaar and W. Kunz},
  title = {Layout Driven Synthesis of Data Path Circuits using Arithmetic Reasoning},
  booktitle = {Proc. International Workshop on Logic and Synthesis},
  year = {2003},
  pages = {1-6},
  address = {Laguna Beach, California, USA},
  month = {May},
  file = {:./files/2003-NeumannStoffel.etal.pdf:PDF}
}

@INPROCEEDINGS{2009-NguyenThalmaier.etal,
  author = {M.D. Nguyen and M. Thalmaier and M.Wedler and D. Stoffel and W. Kunz},
  title = {A Re-Use Methodology for Formal {SoC} Protocol Compliance},
  booktitle = {Proc. Forum on Specification \& Design Languages({FDL})},
  year = {2009},
  pages = {1 -6},
  address = {Sophia Antipolis, France},
  month = {September},
  file = {:./files/2009-NguyenThalmaier.etal.pdf:PDF},
  keywords = {SAT-based property checking;bounded circuit model;bus protocols;computational
	complexity;formal SoC protocol compliance verification;formal verification
	algorithms;generic recorder finite state transition system;interval
	property checking;re-use methodology;reachability analysis;computational
	complexity;conformance testing;formal verification;protocols;reachability
	analysis;recorders;system-on-chip;},
  owner = {wedler}
}

@MISC{2008-Nguyen,
  author = {Minh D. Nguyen},
  title = {Public Benchmarks for evaluation of the {TBT} algorithm},
  owner = {nguyen},
  timestamp = {2008.04.20},
  url = {http://eis.eit.uni-kl.de/~nguyen/}
}

@INPROCEEDINGS{2005a-NguyenStoffel.etal,
  author = {M. D. Nguyen and D. Stoffel and W. Kunz},
  title = {Enhancing {BMC}-based Protocol Verification Using Transition-By-Transition
	{FSM} Traversal},
  booktitle = {Beitraege der 35. Jahrestagung der Gesellschaft fuer Informatik e.V.
	(GI)},
  year = {2005},
  volume = {67},
  pages = {303-307},
  address = {Bonn, Germany},
  month = {September},
  file = {:./files/2005a-NguyenStoffel.etal.pdf:PDF}
}

@INPROCEEDINGS{2005-NguyenStoffel.etal,
  author = {M. D. Nguyen and D. Stoffel and M. Wedler and W. Kunz},
  title = {Transition-by-Transition {FSM} Traversal for Reachability Analysis
	in Bounded Model Checking},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2005},
  pages = { 1068 - 1075},
  address = {San Jose, USA},
  month = {November},
  file = {:./files/2005-NguyenStoffel.etal.pdf:PDF},
  keywords = { FSM; RTL description; bounded model checking; design code inspection;
	reachability analysis; reachability constraints; state space; verification
	flows; finite state machines; formal verification; sequential circuits;
	state-space methods;}
}

@ARTICLE{2008-NguyenThalmaier.etal,
  author = {Minh D. Nguyen and Max Thalmaier and Markus Wedler and J{\"o}rg Bormann
	and Dominik Stoffel and Wolfgang Kunz},
  title = {Unbounded Protocol Compliance Verification using Interval Property
	Checking with Invariants},
  journal = {{IEEE} Transactions on Computer-Aided Design},
  year = {2008},
  volume = {27},
  pages = {2068-2082},
  number = {11},
  month = {November},
  file = {:./files/2008-NguyenThalmaier.etal.pdf:PDF},
  owner = {nguyen},
  timestamp = {2008.08.26}
}

@INBOOK{2010-NguyenThalmaier.etal,
  chapter = {A Re-Use Methodology for Formal SoC Protocol Compliance Verification},
  pages = {197-212},
  title = {Advances in Design Methods from Modeling Languages for Embedded Systems
	and Soc's},
  publisher = {Springer},
  year = {2010},
  editor = {D. Borrione},
  author = {M. D. Nguyen and M. Thalmaier and M. Wedler and D. Stoffel and W.
	Kunz and J. Bormann},
  file = {:./files/2010-NguyenThalmaier.etal.pdf:PDF},
  owner = {W},
  timestamp = {2010.09.30}
}

@INPROCEEDINGS{2011-NguyenWedler.etal,
  author = {Nguyen, Minh D. and Wedler, Markus and Stoffel, Dominik and Kunz,
	Wolfgang},
  title = {Formal {H}ardware/{S}oftware {C}o-{V}erification by {I}nterval {P}roperty
	{C}hecking with {A}bstraction},
  booktitle = {Proceedings of the 48th {D}esign {A}utomation {C}onference},
  year = {2011},
  series = {DAC '11},
  pages = {510--515},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {2024843},
  file = {2011-NguyenWedler.etal.pdf:files/2011-NguyenWedler.etal.pdf:PDF},
  isbn = {978-1-4503-0636-2},
  keywords = {abstraction, embedded system, formal verification, hardware/software},
  location = {San Diego, California},
  numpages = {6},
  owner = {villarraga},
  timestamp = {2012.08.27}
}

@INPROCEEDINGS{2005-NicolescuPaviot.etal,
  author = {G. Nicolescu and Y. Paviot and S. Yoo and A.A. Jerraya},
  title = {Design And Formal Verification Of Networks On Chip},
  year = {2005},
  file = {:./files/2005-NicolescuPaviot.etal.pdf:PDF},
  timestamp = {2006.09.21}
}

@INPROCEEDINGS{2006-NiemannHaubelt,
  author = {Bernhard Niemann and Christian Haubelt},
  title = {Assertion-Based Verification of Transaction Level Models},
  booktitle = {{GIITGGMM}-Workshop 2006 - Methoden und Beschreibungssprachen zur
	Modellierung und Verifikation von Schaltungen und Systemen},
  year = {2006},
  pages = {232--236},
  address = {Dresden, Germany},
  month = {feb},
  date = {February 20--22},
  file = {:./files/2006-NiemannHaubelt.pdf:PDF},
  owner = {nguyen},
  timestamp = {2007.07.10}
}

@INPROCEEDINGS{2005-NieuwenhuisOliveras,
  author = {Robert Nieuwenhuis and Albert Oliveras},
  title = {Decision Procedures for {SAT}, {SAT Modulo Theories} and Beyond.
	{The BarcelogicTools}},
  booktitle = {LPAR'05, LNCS 3835},
  year = {2005},
  pages = {23--46},
  publisher = {Springer},
  file = {:./files/2005-NieuwenhuisOliveras.pdf:PDF},
  owner = {pavlenko},
  timestamp = {2010.07.26}
}

@INPROCEEDINGS{2005-NieuwoudtMassoud,
  author = {Arthur Nieuwoudt and Yehia Massoud},
  title = {Robust Automated Synthesis Methodology for Integrated Spiral Inductors
	with Variability},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2005},
  pages = { 502 - 507},
  file = {:./files/2005-NieuwoudtMassoud.pdf:PDF},
  keywords = { Pareto surface; integrated spiral inductor; multiobjective optimization;
	process variation; robust automated synthesis; surrogate function;
	Pareto analysis; inductors; semiconductor device models;},
  timestamp = {2006.09.27}
}

@ARTICLE{2001-NightingaleGoodenough,
  author = {Andy Nightingale and John Goodenough},
  title = {Testing for {AMBATM} Compliance},
  journal = {Annual {IEEE} International},
  year = {2001},
  pages = {301 -305},
  file = {:./files/2001-NightingaleGoodenough.pdf:PDF},
  timestamp = {2006.09.19}
}

@BOOK{2009-Manfred_Nitzsche,
  title = {Graphen fuer Einsteiger},
  publisher = {Vieweg+Teubner},
  year = {2009},
  author = {Manfred Nitzsche},
  edition = {3.Auflage},
  owner = {bschmidt},
  timestamp = {2014.03.21}
}

@MISC{0000-Debussy,
  author = {{Novas Software}},
  title = {Debussy\textregistered n{W}ave\texttrademark},
  owner = {nguyen},
  timestamp = {2008.04.20},
  url = {http://www.novas.com/Solutions/Debussy/}
}

@INPROCEEDINGS{2014-NyewOnder.etal,
  author = {Nyew, Hui Meen and Onder, Nilufer and Onder, Soner and Wang, Zhenlin},
  title = {Verifying Micro-architecture Simulators Using Event Traces},
  booktitle = {Proceedings of the 28th ACM International Conference on Supercomputing},
  year = {2014},
  series = {ICS '14},
  pages = {323--332},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {2597680},
  file = {2014-NyewOnder.etal.pdf:files/2014-NyewOnder.etal.pdf:PDF},
  isbn = {978-1-4503-2642-1},
  keywords = {architecture simulator, first order logic, verification},
  location = {Munich, Germany},
  numpages = {10},
  owner = {schwarz},
  timestamp = {2017.01.19}
}

@ARTICLE{2014-ObergMeiklejohn.etal,
  author = {Oberg, Jason and Meiklejohn, Sarah and Sherwood, Timothy and Kastner,
	Ryan},
  title = {Leveraging gate-level properties to identify hardware timing channels},
  journal = {IEEE Transactions on Computer-Aided Design of Integrated Circuits
	and Systems},
  year = {2014},
  volume = {33},
  pages = {1288--1301},
  number = {9},
  owner = {fadiheh},
  publisher = {IEEE},
  timestamp = {2018.07.12}
}

@INPROCEEDINGS{2007-OberkoenigSchikel.etal,
  author = {M. Oberk"onig and M. Schickel and H. Eveking},
  title = {A Quantitative Completeness Analysis for Property-Sets},
  booktitle = {Proc. International Conference on Formal Methods in Computer-AidedDesign
	({FMCAD})},
  year = {2007},
  pages = {158 -161},
  month = {nov.},
  file = {:./files/2007-OberkoenigSchikel.etal.pdf:PDF}
}

@BOOK{1999-Oeberg,
  title = {A Grammar-Based Method for Specification and Hardware Synthesis},
  year = {1999},
  author = {Johnny Oeberg},
  file = {:./files/1999-Oeberg.pdf:PDF},
  timestamp = {2006.09.19}
}

@INPROCEEDINGS{2014-OetjensBannow.etal,
  author = {J. H. Oetjens and N. Bannow and M. Becker and O. Bringmann and A.
	Burger and M. Chaari and S. Chakraborty and R. Drechsler and W. Ecker
	and K. Grüttner and T. Kruse and C. Kuznik and H. M. Le and A. Mauderer
	and W. Müller and D. Müller-Gritschneder and F. Poppen and H. Post
	and S. Reiter and W. Rosenstiel and S. Roth and U. Schlichtmann and
	A. von Schwerin and B. A. Tabacaru and A. Viehl},
  title = {Safety evaluation of automotive electronics using Virtual Prototypes:
	State of the art and research challenges},
  booktitle = {2014 51st ACM/EDAC/IEEE Design Automation Conference (DAC)},
  year = {2014},
  issn = {0738-100X},
  owner = {udupi},
  timestamp = {2018.07.24}
}

@ARTICLE{2002-OhShirvani1.etal,
  author = {N. Oh and P. P. Shirvani and E. J. McCluskey},
  title = {Error detection by duplicated instructions in super-scalar processors},
  journal = {IEEE Transactions on Reliability},
  year = {2002},
  volume = {51},
  pages = {63-75},
  number = {1},
  month = {March},
  file = {2002-OhShirvani1.etal.pdf:files/2002-OhShirvani1.etal.pdf:PDF},
  issn = {0018-9529},
  owner = {bartsch},
  timestamp = {2016.09.21}
}

@ARTICLE{2002-OhShirvani2.etal,
  author = {N. Oh and P. P. Shirvani and E. J. McCluskey},
  title = {Control-flow checking by software signatures},
  journal = {IEEE Transactions on Reliability},
  year = {2002},
  volume = {51},
  pages = {111-122},
  number = {1},
  month = {March},
  file = {2002-OhShirvani2.etal.pdf:files/2002-OhShirvani2.etal.pdf:PDF},
  issn = {0018-9529},
  owner = {bartsch},
  timestamp = {2016.09.21}
}

@PHDTHESIS{0000-Oikonomakos,
  author = {Petros Oikonomakos},
  title = {Transfer Thesis},
  school = {Electronic Systems Design Group, Department of Electronics and Computer
	Science, University of Southampton},
  file = {0000-Oikonomakos.pdf:files/0000-Oikonomakos.pdf:PDF},
  timestamp = {2006.09.14}
}

@INPROCEEDINGS{2002-OliveiraHu,
  author = {Marcio T. Oliveira and Alan J. Hu},
  title = {High-Level Specification and Automatic Generation of IP Interface
	Monitors},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {2002},
  pages = { 129 - 134},
  file = {:./files/2002-OliveiraHu.pdf:PDF},
  keywords = { AMBA AHB protocol; IP interface monitor circuit; Sonics OCP protocol;
	VHDL; Verilog; automatic generation; functional verification; high-level
	specification; system-on-chip; translation algorithm; formal specification;
	formal verification; hardware description languages; high level synthesis;
	industrial property; protocols; system-on-chip;},
  timestamp = {2006.09.19}
}

@ARTICLE{2010-OmanaRossi.etal,
  author = {M. Omana and D. Rossi and C. Metra},
  title = {High-Performance Robust Latches},
  journal = {IEEE Transactions on Computers},
  year = {2010},
  volume = {59},
  pages = {1455-1465},
  number = {11},
  month = {November},
  file = {2010-OmanaRossi.etal.pdf:files/2010-OmanaRossi.etal.pdf:PDF},
  issn = {0018-9340},
  owner = {bartsch},
  timestamp = {2016.09.21}
}

@MISC{web-onespin,
  author = {{Onespin Solutions GmbH}},
  title = {{OneSpin 360 DV-Verify}},
  howpublished = {https://www.onespin.com/products/360-dv-verify/},
  key = {onespin},
  owner = {stoffel},
  timestamp = {2016.05.11}
}

@MISC{web_opencores,
  author = {opencores.org},
  howpublished = {\url{www.opencores.org}},
  owner = {Binghao},
  timestamp = {2012.10.24},
  url = {www.opencores.org}
}

@MISC{2004-DashOptimization,
  author = {Dash Optimization},
  title = {{XPress-MP}},
  organization = {Dash Optimization},
  owner = {stoffel},
  timestamp = {2016.05.11},
  url = {http://www.dashoptimization.com}
}

@INPROCEEDINGS{2001-OschSmolka,
  author = {Michiel van Osch and Scott A. Smolka},
  title = {Finite-State Analysis of the {CAN} Bus Protocol},
  booktitle = {Proc. {IEEE} International Symposium on High-Assurance Systems Engineering:
	Special Topic: Impact of Networking},
  year = {2001},
  pages = {42 -52},
  file = {:./files/2001-OschSmolka.pdf:PDF},
  keywords = {CAN bus protocol;ISO 11898 international standard;ISO standard;controller
	area network;data link layer;data link layers;embedded systems;finite-state
	analysis;formal specification;high-speed serial bus system;ISO standards;controller
	area networks;embedded systems;finite state machines;formal specification;protocols;system
	buses;},
  timestamp = {2006.09.21}
}

@INPROCEEDINGS{1977-CousotCousot,
  author = {P.Cousot and R.Cousot},
  title = {Abstract Interpretation: A Unified Lattice Model For Static Analysis
	Of Programs By Construction Or Approximation Of Fix Point},
  booktitle = {4th {ACM} Symposium on Principles of Programming Languages},
  year = {1977},
  pages = {238-252},
  file = {:./files/1977-CousotCousot.pdf:PDF},
  timestamp = {2006.09.22}
}

@ARTICLE{2010-PasareanuVisser,
  author = {P\u{a}s\u{a}reanu, Corina S. and Visser, Willem},
  title = {A survey of new trends in symbolic execution for software testing
	and analysis},
  journal = {Int. J. Softw. Tools Technol. Transf.},
  year = {2009},
  volume = {11},
  pages = {339--353},
  number = {4},
  month = oct,
  acmid = {1667869},
  address = {Berlin, Heidelberg},
  file = {2010-PasareanuVisser.pdf:files/2010-PasareanuVisser.pdf:PDF},
  issn = {1433-2779},
  issue_date = {October 2009},
  numpages = {15},
  owner = {villarraga},
  publisher = {Springer-Verlag},
  timestamp = {2012.07.18}
}

@INPROCEEDINGS{2005-PachecoErnst,
  author = {Pacheco, Carlos and Ernst, Michael D.},
  title = {Eclat: Automatic Generation and Classification of Test Inputs},
  booktitle = {Proceedings of the 19th European Conference on Object-Oriented Programming},
  year = {2005},
  series = {ECOOP'05},
  pages = {504--527},
  address = {Berlin, Heidelberg},
  publisher = {Springer-Verlag},
  acmid = {2144921},
  isbn = {3-540-27992-X, 978-3-540-27992-1},
  location = {Glasgow, UK},
  numpages = {24},
  owner = {villarraga},
  timestamp = {2016.08.01}
}

@INPROCEEDINGS{2001-Panda,
  author = {P. R. {Panda}},
  title = {SystemC - a modeling platform supporting multiple design abstractions},
  booktitle = {International Symposium on System Synthesis (IEEE Cat. No.01EX526)},
  year = {2001},
  pages = {75-80},
  month = {Sep.},
  doi = {10.1145/500001.500018 },
  keywords = {hardware description languages;C++ language;software libraries;industrial
	property;hardware-software codesign;SystemC;C++ based modeling platform;design
	abstractions;register-transfer level;class library;simulation kernel;C/C++
	design methodology;C++ libraries;Open SystemC Initiative;embedded
	software developers;design automation tool vendors;common design
	environment;hardware-software co-design;IP exchange;modeling abstraction;design
	specification language;system-level design;Embedded software;Hardware
	design languages;Software libraries;Standardization;Design methodology;Integrated
	circuit synthesis;Kernel;System testing;System-level design;Design
	automation},
  owner = {fehmel},
  timestamp = {2019.05.29}
}

@INPROCEEDINGS{2005-PantBlaauw,
  author = {Sanjay Pant and David Blaauw},
  title = {Static Timing Analysis Considering Power Supply Variations},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2005},
  pages = { 365 - 371},
  file = {:./files/2005-PantBlaauw.pdf:PDF},
  keywords = { circuit delay maximization problem; critical paths; deep submicron
	technologies; nonlinear optimization problem; power supply integrity
	verification; power supply noise; power supply variations; static
	timing analysis; worst-case circuit delay; worst-case drop; circuit
	optimisation; delays; integrated circuit design; power supply circuits;
	timing circuits;},
  timestamp = {2006.09.27}
}

@INPROCEEDINGS{1998-PardoHachtel,
  author = {Abelardo Pardo and Gary D. Hachtel},
  title = {Incremental {CTL} Model Checking Using {BDD} Subsetting},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {1998},
  pages = {457 -462},
  file = {:./files/1998-PardoHachtel.pdf:PDF},
  keywords = {BDD-subsetting;conservative verification;model checking;symbolic CTL
	model checking;formal verification;high level synthesis;},
  owner = {thalmaier},
  timestamp = {2006.11.24}
}

@INPROCEEDINGS{1997-PardoHachtel,
  author = {Abelardo Pardo and Gary D. Hachtel},
  title = {Automatic Abstraction Techniques for Propositional $\mu$-calculus
	Model Checking},
  booktitle = {Proc. International Conference on Computer Aided Verification (CAV)},
  year = {1997},
  pages = {12--23},
  file = {:./files/1997-PardoHachtel.pdf:PDF},
  owner = {thalmaier},
  timestamp = {2006.11.24}
}

@BOOK{2000-Parhami,
  title = {Computer Arithmetic Algorithms and Hardware Design},
  publisher = {Oxford University Press},
  year = {2000},
  author = {P. Parhami}
}

@INPROCEEDINGS{1990-ParkShaw,
  author = {Chang Yun Park and Alan C. Shaw},
  title = {Experiment With a Program Timing Tool Based On Source Level Timing
	Schema},
  booktitle = {Proc. Conference on Real-Time Systems Symposium},
  year = {1990},
  file = {:./files/1990-ParkShaw.pdf:PDF},
  keywords = {C;atomic elements;compiler;expressions;formal timing schema;granularity;procedures;program
	timing tool;programs;source-level timing schema;statements;target
	architecture;timing semantics;program verification;},
  timestamp = {2006.09.22}
}

@INPROCEEDINGS{1981-Park,
  author = {Park, David},
  title = {Concurrency and Automata on Infinite Sequences},
  booktitle = {Proceedings of the 5th GI-Conference on Theoretical Computer Science},
  year = {1981},
  pages = {167--183},
  address = {London, UK, UK},
  publisher = {Springer-Verlag},
  isbn = {3-540-10576-X},
  numpages = {17},
  owner = {joakim},
  timestamp = {2014.08.05}
}

@INPROCEEDINGS{2005-ParthasarathyIyer.etal,
  author = {G. Parthasarathy and M. K. Iyer and K.T. Cheng and F. Brewer},
  title = {{RTL} {SAT} Simplification by {Boolean} and Interval Arithmetic Reasoning},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2005},
  pages = { 297 - 302},
  file = {:./files/2005-ParthasarathyIyer.etal.pdf:PDF},
  keywords = { {Boolean} reasoning; RTL SAT simplification; interval arithmetic
	reasoning; interval-arithmetic operations; register-transfer level;
	structural hashing; {Boolean} functions; computability; digital arithmetic;
	logic design;},
  timestamp = {2006.09.27}
}

@INPROCEEDINGS{2004-ParthasarathyIyer,
  author = {G. Parthasarathy and M. K. Iyer and K.-T. Cheng and Li.C. Wang},
  title = {An Efficient Finite-domain Constraint Solver for {RTL} Circuits},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {2004},
  series = {DAC '04},
  pages = {212--217},
  address = {New York, NY, USA},
  month = {June},
  publisher = {ACM},
  acmid = {996628},
  file = {:./files/2004-ParthasarathyIyer.pdf:PDF},
  isbn = {1-58113-828-8},
  keywords = {bit-vector arithmetic, boolean satisfiability, circuits, constraints,
	decision procedures, design verification, integer linear programming},
  location = {San Diego, CA, USA},
  numpages = {6}
}

@ARTICLE{2005-PaschalisGizopoulos,
  author = {A. Paschalis and D. Gizopoulos},
  title = {Effective software-based self-test strategies for on-line periodic
	testing of embedded processors},
  journal = {IEEE Transactions on Computer-Aided Design of Integrated Circuits
	and Systems},
  year = {2005},
  volume = {24},
  pages = {88-99},
  number = {1},
  month = {January},
  file = {2005-PaschalisGizopoulos.pdf:files/2005-PaschalisGizopoulos.pdf:PDF},
  issn = {0278-0070},
  owner = {bartsch},
  timestamp = {2016.09.21}
}

@INPROCEEDINGS{1998-PasseroneRowson.etal,
  author = {R. Passerone and James A. Rowson and Alberto S. Vincentelli},
  title = {Automatic Synthesis of Interfaces between Incompatible Protocols},
  booktitle = {Pro. International Design Automation Conference (DAC)},
  year = {1998},
  pages = {8 -13},
  month = {june},
  file = {:./files/1998-PasseroneRowson.etal.pdf:PDF},
  keywords = {IP blocks;Verilog implementation;interface machine;protocols;reusable
	Intellectual Property;computer interfaces;formal specification;protocols;},
  timestamp = {2006.09.19}
}

@ARTICLE{2013-PattabiramanNakka.etal,
  author = {K. Pattabiraman and N.M. Nakka and Z.T. Kalbarczyk and R.K. Iyer},
  title = {SymPLFIED: Symbolic Program-Level Fault Injection and Error Detection
	Framework},
  journal = {IEEE Transactions on Computers},
  year = {2013},
  volume = {62},
  pages = {2292 - 2307},
  number = {11},
  month = {Nov},
  file = {2013-PattabiramanNakka.etal.pdf:files/2013-PattabiramanNakka.etal.pdf:PDF},
  owner = {bartsch},
  timestamp = {2015.09.09}
}

@BOOK{2013-PattersonHennessy,
  title = {Computer Organization and Design, Fifth Edition: The Hardware/Software
	Interface},
  publisher = {Morgan Kaufmann Publishers Inc.},
  year = {2013},
  author = {Patterson, David A. and Hennessy, John L.},
  address = {San Francisco, CA, USA},
  edition = {5th},
  isbn = {0124077269, 9780124077263},
  owner = {stoffel},
  timestamp = {2018.08.07}
}

@INPROCEEDINGS{2011a-PavlenkoWedler.etal,
  author = {Evgeny Pavlenko and Markus Wedler and Alexander Dreyer and Frank
	Seelisch},
  title = {{STABLE}: Combining Satisfiability, {Boolean} Reasoning and Computer
	Algebra for System-on-Chip Verification},
  booktitle = {Young Researcher Symposium},
  year = {2011},
  address = {ITWM Kaiserslautern, Germany},
  owner = {pavlenko},
  timestamp = {2011.01.21}
}

@INPROCEEDINGS{2007-PavlenkoWedler.etal,
  author = {E. Pavlenko and M. Wedler and D. Stoffel and W. Kunz},
  title = {Arithmetic Constrains in {SAT}-based Property Checking},
  booktitle = {10. {GI/ITG/GMM} Workshop Methoden und Beschreibungssprachen zur
	Modellierung und Verifikation von Schaltungen und Systemen ({MBMV})},
  year = {2007},
  owner = {pavlenko},
  timestamp = {2010.10.08}
}

@INPROCEEDINGS{2011-PavlenkoWedler.etal,
  author = {Evgeny Pavlenko and Markus Wedler and Dominik Stoffel and Wolfgang
	Kunz and Frank Seelisch and Gert-Martin Greuel and Alexander Dreyer},
  title = {{STABLE}: A new {QF-BV SMT} Solver for hard Verification Problems
	combining {Boolean} Reasoning with Computer Algebra},
  booktitle = {Proc. International Conference on Design, Automation and Test in
	Europe (DATE)},
  year = {2011},
  pages = {1 -6},
  file = {:./files/2011-PavlenkoWedler.etal.pdf:PDF},
  keywords = {{Boolean} reasoning;SMT-based property checking flow;SoC;arithmetic
	bit-level information;arithmetic problems;bit-blasting;computer algebra;computer-algebra-based
	engine;fixed-sized bit vectors;hard verification problems;industrial
	data path modules;quantifier-free logic;system-on-chip designs;Boolean
	algebra;formal verification;system-on-chip;},
  owner = {pavlenko},
  timestamp = {2010.11.22}
}

@INBOOK{2009-PavlenkoWedler.etal,
  chapter = {17},
  pages = {257-272},
  title = {A New Verification Technique for Custom-Designed Components at the
	Arithmetic Bit Level},
  publisher = {Springer Netherlands},
  year = {2009},
  editor = {Martin Radetzki},
  author = {E. Pavlenko and M. Wedler and D. Stoffel and W. Kunz and O. Wienand
	and E. Karibaev},
  volume = {Languages for Embedded Systems and their Applications},
  series = {Lecture Notes in Electrical Engineering},
  file = {:./files/2009-PavlenkoWedler.etal.pdf:PDF},
  owner = {W},
  timestamp = {2010.02.12},
  url = {http://www.springerlink.com/content/h34173r4739p4041/}
}

@INPROCEEDINGS{2008a-PavlenkoWedler.etal,
  author = {E. Pavlenko and M. Wedler and D. Stoffel and W. Kunz and O. Wienand
	and E. Karibaev},
  title = {Modeling of Custom-Designed Arithmetic Components for {ABL} Normalization},
  booktitle = {{GI/ITG/GMM} Workshop Methoden und Beschreibungssprachen zur Modellierung
	und Verifikation von Schaltungen und Systemen ({MBMV})},
  year = {2008},
  pages = {124 -129},
  file = {:./files/2008a-PavlenkoWedler.etal.pdf:PDF},
  keywords = {ABL normalization;{Boolean} logic;Reed-Muller expression;arithmetic
	bit-level normalization;arithmetic component;datapath design;formal
	property checking;logic block;register-transfer level;{Boolean} functions;digital
	arithmetic;logic design;logic testing;},
  owner = {wedler},
  timestamp = {2008.02.18}
}

@INPROCEEDINGS{2008-PavlenkoWedler.etal,
  author = {E. Pavlenko and M. Wedler and D. Stoffel and O. Wienand and E. Karibaev
	and W. Kunz:},
  title = {Modeling of Custom-Designed Arithmetic Components in {ABL} Normalization},
  booktitle = {Proc. Forum on Specification \& Design Languages(FDL)},
  year = {2008},
  pages = {124 -129},
  address = {Stuttgart, Germany},
  month = {September},
  file = {:./files/2008-PavlenkoWedler.etal.pdf:PDF},
  keywords = {ABL normalization;{Boolean} logic;Reed-Muller expression;arithmetic
	bit-level normalization;arithmetic component;datapath design;formal
	property checking;logic block;register-transfer level;{Boolean} functions;digital
	arithmetic;logic design;logic testing;},
  owner = {wedler},
  timestamp = {2008.06.16}
}

@INPROCEEDINGS{2005-Percival,
  author = {Percival, Colin},
  title = {Cache missing for fun and profit},
  booktitle = {BSDCan},
  year = {2005},
  owner = {fadiheh},
  timestamp = {2018.07.12},
  url = {http://www.daemonology.net/papers/htt.pdf}
}

@INPROCEEDINGS{2010-PerezAzkarate-Askasua.etal,
  author = {J. Perez and M. Azkarate-Askasua and A. Perez},
  title = {Codesign and Simulated Fault Injection of Safety-Critical Embedded
	Systems Using SystemC},
  booktitle = {European Dependable Computing Conference},
  year = {2010},
  pages = {221-229},
  month = {April},
  file = {2010-PerezAzkarate-Askasua.etal.pdf:files/2010-PerezAzkarate-Askasua.etal.pdf:PDF},
  owner = {bartsch},
  timestamp = {2016.11.28}
}

@ARTICLE{2015-PesslGruss.etal,
  author = {Pessl, Peter and Gruss, Daniel and Maurice, Cl{\'e}mentine and Mangard,
	Stefan},
  title = {Reverse engineering intel {DRAM} addressing and exploitation},
  journal = {ArXiv e-prints},
  year = {2015},
  owner = {fadiheh},
  timestamp = {2018.07.12}
}

@INPROCEEDINGS{2016-PesslGruss.etal,
  author = {Pessl, Peter and Gruss, Daniel and Maurice, Cl{\'e}mentine and Schwarz,
	Michael and Mangard, Stefan},
  title = {{DRAMA}: Exploiting {DRAM} Addressing for Cross-CPU Attacks},
  booktitle = {25th {USENIX} Security Symposium ({USENIX} Security 16)},
  year = {2016},
  pages = {565--581}
}

@INPROCEEDINGS{2016-PetersonBringmann,
  author = {D. Peterson and O. Bringmann},
  title = {{SMoSi}: A framework for the derivation of sleep mode traces from
	{RTL} simulations},
  booktitle = {2016 21st Asia and South Pacific Design Automation Conference (ASP-DAC)},
  year = {2016},
  file = {:/import/var/jabref/files/2016-PetersonBringmann.pdf:PDF},
  owner = {udupi},
  timestamp = {2017.03.28}
}

@INPROCEEDINGS{2013-PetersonBringmann.etal,
  author = {D. Peterson and O. Bringmann and T. Schweizer and W. Rosenstiel},
  title = {{StML}: Bridging the gap between FPGA design and HDL circuit description},
  booktitle = {International Conference on Field-Programmable Technology (FPT)},
  year = {2013},
  pages = {278-285},
  month = {December},
  file = {2013-PetersonBringmann.etal.pdf:files/2013-PetersonBringmann.etal.pdf:PDF},
  owner = {bartsch},
  timestamp = {2016.09.22}
}

@INPROCEEDINGS{2005-PeterssonErmedahl.etal,
  author = {Samuel Petersson and Andreas Ermedahl and Anders Pettersson and Daniel
	Sundmark and Niklas Holsti},
  title = {Using a {WCET} Analysis Tool in Real-Time Systems Education},
  year = {2005},
  file = {:./files/2005-PeterssonErmedahl.etal.pdf:PDF},
  timestamp = {2006.09.22}
}

@ARTICLE{2003-PeymandoustDeMicheli,
  author = {A. Peymandoust and G. De Micheli},
  title = {Application of Symbolic Computer Algebra in High-level data-flow
	Synthesis},
  journal = {{IEEE} Transactions on Computer-Aided Design},
  year = {2003},
  volume = {22},
  pages = {1154-1165},
  number = {9},
  month = {September},
  file = {:./files/2003-PeymandoustDeMicheli.pdf:PDF},
  owner = {wedler},
  timestamp = {2006.09.11}
}

@MASTERSTHESIS{2001-Pfender,
  author = {T. Pfender},
  title = {Anwengung von Neuronalen Netzen zur Beschleunigung von Branch\&Bound-Verfahren
	der Kombinatorischen Optimierung},
  school = {Techn. University Berlin, Dept.of Computer Science},
  year = {2001},
  language = {German}
}

@MASTERSTHESIS{2000-Pfender,
  author = {T. Pfender},
  title = {Arboreszenz-Fluesse in Graphen: polyedrische Uentersuchungen},
  school = {Techn. Ueniversity Berlin, Dept. of Mathematics},
  year = {2000},
  language = {German}
}

@PHDTHESIS{2002-Pfetsch,
  author = {Marc E. Pfetsch},
  title = {The Maximum Feasible Subsystem Problem and Vertex-Facet Incidences
	of Polyhedra},
  school = {Technische Universit{\"a}t Berlin},
  year = {2002},
  type = {Dissertation},
  file = {:./files/2002-Pfetsch.pdf:PDF}
}

@ARTICLE{2001-PflanzVierhaus,
  author = {M. Pflanz and H. T. Vierhaus},
  title = {Online check and recovery techniques for dependable embedded processors},
  journal = {IEEE Micro},
  year = {2001},
  volume = {21},
  pages = {24-40},
  number = {5},
  month = {September},
  file = {2001-PflanzVierhaus.pdf:files/2001-PflanzVierhaus.pdf:PDF},
  issn = {0272-1732},
  owner = {bartsch},
  timestamp = {2016.09.21}
}

@ARTICLE{2003-PflanzWalther.etal,
  author = {M. Pflanz and K. Walther and C. Galke and H.T. Vierhaus},
  title = {On-Line Techniques for Error Detection and Correction in Processor
	Registers with Cross-Parity Check},
  journal = {Journal of Electronic Testing},
  year = {2003},
  volume = {19},
  pages = {501--510},
  number = {5},
  file = {2003-PflanzWalther.etal.pdf:files/2003-PflanzWalther.etal.pdf:PDF},
  issn = {1573-0727},
  owner = {bartsch},
  timestamp = {2016.09.21}
}

@INPROCEEDINGS{1996-Piestrak,
  author = {Stanislaw J. Piestrak},
  title = {Limitations of Design Methods of Self-Checking Synchronous Sequential
	Machines},
  booktitle = {Proc. International Conference on Design and Test of Computers},
  year = {1996},
  file = {:./files/1996-Piestrak.pdf:PDF},
  timestamp = {2006.09.14}
}

@INPROCEEDINGS{1996-PihlAas,
  author = {Johnny Pihl and Einar Aas},
  title = {A Multiplier and a Squarer Generator for High Performance DSP Applications},
  booktitle = {Proc. 39th Midwest Symposium on Circuits and Systems},
  year = {1996},
  pages = {109 -112},
  month = {August},
  file = {:./files/1996-PihlAas.pdf:PDF},
  keywords = {0.8 micron;Booth encoding;CMOS process;VLSI;area reduction;binary
	tree vector merging addition;bit-parallel DSP applications;delay
	reduction;high performance DSP applications;multiplier;optimized
	Wallace trees;partial product reduction scheme;pattern recognition;power
	reduction;squarer generator;weighted square sums;CMOS digital integrated
	circuits;VLSI;delays;digital arithmetic;digital signal processing
	chips;multiplying circuits;trees (mathematics);}
}

@INPROCEEDINGS{2015-PiperWinter.etal,
  author = {T. Piper and S. Winter and N. Suri and T. E. Fuhrman},
  title = {On the Effective Use of Fault Injection for the Assessment of {AUTOSAR}
	Safety Mechanisms},
  booktitle = {11th European Dependable Computing Conference (EDCC)},
  year = {2015},
  pages = {85-96},
  month = {Sept},
  file = {2015-PiperWinter.etal.pdf:files/2015-PiperWinter.etal.pdf:PDF},
  owner = {bartsch},
  timestamp = {2016.11.28}
}

@ARTICLE{1992-Pixley,
  author = {C. Pixley},
  title = {A Theory and Implementation of Sequential Hardware Equivalence},
  journal = {{IEEE} Transactions on Computer-Aided Design},
  year = {1992},
  volume = {11},
  pages = {1469-1478},
  number = {12},
  month = {December},
  file = {:./files/1992-Pixley.pdf:PDF}
}

@INPROCEEDINGS{1994-PixleySinghal.etal,
  author = {C. Pixley and V. Singhal and A. Aziz and R. K. Brayton},
  title = {Multi-level Synthesis for Safe-Replaceability},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {1994},
  pages = {442-449},
  file = {:./files/1994-PixleySinghal.etal.pdf:PDF}
}

@TECHREPORT{2002-PlosilaSeceleanu,
  author = {Juha Plosila and Tiberiu Seceleanu},
  title = {Formal Specification of an Asynchronous on-chip Bus},
  institution = {Turku Centre for Computer Science},
  year = {2002},
  file = {:./files/2002-PlosilaSeceleanu.pdf:PDF},
  timestamp = {2006.09.19}
}

@INPROCEEDINGS{1977-Pnueli,
  author = {Pnueli, Amir},
  title = {The temporal logic of programs},
  booktitle = {Foundations of Computer Science, 1977., 18th Annual Symposium on
	Foundations of Computer Science},
  year = {1977},
  pages = {46 -57},
  month = {31 1977-nov. 2},
  file = {1977-Pnueli.pdf:files/1977-Pnueli.pdf:PDF},
  issn = {0272-5428},
  owner = {villarraga},
  timestamp = {2012.08.30}
}

@INPROCEEDINGS{1998-PnueliSiegel.etal,
  author = {Pnueli, Amir and Siegel, Michael and Singerman, Eli},
  title = {Translation Validation},
  booktitle = {Proceedings of the 4th International Conference on Tools and Algorithms
	for Construction and Analysis of Systems},
  year = {1998},
  series = {TACAS '98},
  pages = {151--166},
  address = {London, UK, UK},
  publisher = {Springer-Verlag},
  acmid = {691453},
  isbn = {3-540-64356-7},
  numpages = {16},
  owner = {villarraga},
  timestamp = {2012.12.03}
}

@INPROCEEDINGS{2005-PodelskiRybalchenko,
  author = {Andreas Podelski and Andrey Rybalchenko},
  title = {Transition Predicate Abstraction and Fair Termination},
  booktitle = {Proc. of {ACM} Symposium on Principles of Programming Languages ({POPL})},
  year = {2005},
  pages = {132--144},
  publisher = {ACM},
  file = {:./files/2005-PodelskiRybalchenko.pdf:PDF},
  owner = {stoffel},
  timestamp = {2010.10.28}
}

@ARTICLE{1996-PomeranzReddy,
  author = {I. Pomeranz and S.M. Reddy},
  title = {On Removing Redundancies from Synchronous Sequential Circuits with
	Synchronizing Sequences},
  journal = {{IEEE} Transactions on Computers},
  year = {1996},
  volume = {45},
  pages = {20-32},
  number = {1},
  month = {January},
  file = {:./files/1996-PomeranzReddy.pdf:PDF}
}

@ARTICLE{2006-PomeranzReddy,
  author = {I. Pomeranz and S. M. Reddy},
  title = {Generation of Functional Broadside Tests for Transition Faults},
  journal = {{IEEE} Transactions on Computer-Aided Design},
  year = {2006},
  volume = {25},
  pages = {2207-2219},
  number = {10},
  month = {October},
  file = {:./files/2006-PomeranzReddy.pdf:PDF},
  owner = {wedler},
  timestamp = {2006.12.15}
}

@ARTICLE{2012-Portela-GarciaLindoso.etal,
  author = {M. Portela-Garcia and A. Lindoso and L. Entrena and M. Garcia-Valderas
	and C. Lopez-Ongil and N. Marroni and B. Pianta and L. Bolzani Poehls
	and F. Vargas},
  title = {Evaluating the Effectiveness of a Software-Based Technique Under
	{SEEs} Using {FPGA}-Based Fault Injection Approach},
  journal = {Journal of Electronic Testing},
  year = {2012},
  volume = {28},
  pages = {777-789},
  number = {6},
  file = {2012-Portela-GarciaLindoso.etal.pdf:files/2012-Portela-GarciaLindoso.etal.pdf:PDF},
  issn = {1573-0727},
  owner = {bartsch},
  timestamp = {2016.11.28}
}

@ARTICLE{2005-PrasadBiere.etal,
  author = {Mukul R Prasad and Armin Biere and Aarti Gupta},
  title = {A Survey of Recent Advances in {SAT}-based Formal Verification},
  journal = {International Journal on Software Tools for Technology},
  year = {2005},
  volume = {7},
  pages = {156--173},
  number = {2},
  month = {apr},
  day = {30},
  file = {:./files/2005-PrasadBiere.etal.pdf:PDF},
  keywords = {sat},
  timestamp = {2006.09.19}
}

@MISC{web_precosat,
  author = {{PrecoSAT 236}},
  owner = {pavlenko},
  timestamp = {2010.02.15},
  url = {http://fmv.jku.at/precosat/}
}

@ARTICLE{1995-Price,
  author = {Price, D.},
  title = {Pentium FDIV Flaw-lessons Learned},
  journal = {IEEE Micro},
  year = {1995},
  volume = {15},
  pages = {86--88},
  number = {2},
  month = apr,
  address = {Los Alamitos, CA, USA},
  issn = {0272-1732},
  issue_date = {April 1995},
  owner = {stoffel},
  publisher = {IEEE Computer Society Press},
  timestamp = {2016.05.10}
}

@TECHREPORT{1994-Puget,
  author = {Jean-Francois Puget},
  title = {A {C++} implementation of {CLP}},
  institution = {ILOG S.A.},
  year = {1994},
  number = {94-01},
  address = {Gentilly, France},
  file = {:./files/1994-Puget.pdf:PDF}
}

@INPROCEEDINGS{1991-Pugh,
  author = {William Pugh},
  title = {The Omega Test: a Fast and Practical Integer Programming Algorithm
	for Dependence Analysis},
  booktitle = {Proc. {ACM/IEEE} International Conference on Supercomputing},
  year = {1991},
  pages = {4 -13},
  file = {:./files/1991-Pugh.pdf:PDF},
  timestamp = {2006.10.04}
}

@ARTICLE{1999-PuschnerBurns,
  author = {Peter Puschner and Alan Burns},
  title = {A Review of Worst-Case Execution-Time Analysis},
  journal = {Real-Time Systems},
  year = {1999},
  pages = {115--128},
  number = {2},
  file = {:./files/1999-PuschnerBurns.pdf:PDF},
  issn = {09226443},
  timestamp = {2006.09.22}
}

@PHDTHESIS{2004-Qin,
  author = {Wei Qin},
  title = {Modeling and Description of Embedded Processors for the Development
	of Software Tools},
  year = {2004},
  file = {:./files/2004-Qin.pdf:PDF},
  timestamp = {2006.10.04}
}

@INPROCEEDINGS{2003-QinMalik,
  author = {Wei Qin and Sharad Malik},
  title = {Flexible and Formal Modeling of Microprocessors with Application
	to Retargetable Simulation},
  booktitle = {Proc. International Conference on Design, Automation and Test in
	Europe ({DATE})},
  year = {2003},
  pages = { 556 - 561},
  month = {March},
  file = {:./files/2003-QinMalik.pdf:PDF},
  keywords = { PowerPC-750 superscalar processor; StrongARM core; application-specific
	processors; complex processor behaviors; declarative model; disciplined
	hardware units interaction; formal modeling; hardware layer; interacting
	layers; microarchitecture simulators; microprocessors; operation
	layer; operation semantics; operation state machine computation model;
	retargetable modeling framework; retargetable simulation; timing;
	VLSI; circuit simulation; integrated circuit modelling; microprocessor
	chips; processor scheduling; timing;},
  owner = {nguyen},
  timestamp = {2007.02.02},
  url = {http://www.gigascale.org/pubs/352.html}
}

@MISC{1996-QuerCabodi.etal,
  author = {Stefano Quer and Gianpiero Cabodi and Paolo Camurati},
  title = {Decomposed Symbolic Forward Traversals of Large Finite State Machines},
  year = {1996},
  booktitle = {Proc. European Design Automation Conference ({EDAC})},
  file = {:./files/1996-QuerCabodi.etal.pdf:PDF},
  isbn = {0-8186-7573-X},
  location = {Geneva, Switzerland},
  owner = {stoffel},
  pages = {170--175},
  publisher = {IEEE Computer Society Press},
  timestamp = {2016.05.11}
}

@INPROCEEDINGS{1996a-QuerCabodi.etal,
  author = {S. Quer and G. Cabodi and P. Camurati and L. Lavagno and E. Sentovich
	and R. K. Brayton},
  title = {Incremental Re-Encoding for Symbolic Traversal of Product Machines},
  booktitle = {Proc. European Design Automation Conference (EDAC)},
  year = {1996},
  pages = {158 -163},
  file = {:./files/1996a-QuerCabodi.etal.pdf:PDF},
  keywords = {backward traversal;combinational verification;finite state machines;forward
	traversal;incremental re-encoding;product machines;reachable states;state
	minimization;state space exploration;symbolic traversal;finite state
	machines;minimisation of switching nets;state assignment;}
}

@ARTICLE{1952-Quine,
  author = {W. Quine},
  title = {The Problem of Simplifying Truth Functions},
  journal = {American Mathematical Monthly},
  year = {1952},
  volume = {59},
  pages = {521-531},
  number = {8},
  copyright = {Copyright � 1952 Mathematical Association of America},
  file = {:./files/1952-Quine.pdf:PDF},
  issn = {00029890},
  language = {English},
  publisher = {Mathematical Association of America},
  url = {http://www.jstor.org/stable/2308219}
}

@ARTICLE{2005-ArmoniFix.etal,
  author = {R.Armoni and L.Fix and R.Fraer},
  title = {{SAT}-Based Induction For Temporal Safty Properties},
  journal = {Electronic Notes in Theoretical Computer Science},
  year = {2005},
  volume = {119},
  pages = {3--16},
  number = {2},
  month = {mar},
  acmid = {1705774},
  address = {Amsterdam, The Netherlands, The Netherlands},
  file = {:./files/2005-ArmoniFix.etal.pdf:PDF},
  issn = {1571-0661},
  issue_date = {March, 2005},
  keywords = {SAT, induction, safety, windowed induction},
  numpages = {14},
  publisher = {Elsevier Science Publishers B. V.},
  timestamp = {2006.09.19}
}

@INPROCEEDINGS{1999-GoswamiSrinivasan.etal,
  author = {R.Goswami and V.Srinivasan and M.Balakrishnan},
  title = {{MPEG}-2 Video Data Simulator: A Case Study In Constrained {HW}-{SW}
	Design},
  booktitle = {Proc. International Conference on {VLSI} Design},
  year = {1999},
  pages = {128 -131},
  month = {jan},
  file = {:./files/1999-GoswamiSrinivasan.etal.pdf:PDF},
  keywords = {C-language simulation;I I I picture sequence;MPEG-2 video;behavioral
	simulation;color-bars data;constrained HW-SW codesign;constrained
	design space;firmware implementation;hierarchical FSM model;implementation
	options;moving picture sequence;video data simulator;C language;data
	compression;digital simulation;finite state machines;firmware;hardware-software
	codesign;signal generators;telecommunication standards;video coding;},
  timestamp = {2006.09.21}
}

@INPROCEEDINGS{1994-KarriHogstedt.etal,
  author = {R.Karri and K.Hogstedt and A.Orailogln},
  title = {Rapid Prototyping Of Fault Tolerant {VLSI} Systems},
  booktitle = {Proc. International Symposium on High-level Synthesis},
  year = {1994},
  pages = {126 -131},
  file = {:./files/1994-KarriHogstedt.etal.pdf:PDF},
  keywords = {16-point FIR filter;algorithmic description;area-efficient fault-tolerant
	VLSI ICs;chip area;environment induced transient faults;fault tolerant
	VLSI systems;fault tolerant implementations;fault-tolerance constraints;fault-tolerant
	designs;rapid prototyping;uninterrupted operation;VLSI;circuit CAD;circuit
	analysis computing;digital filters;},
  timestamp = {2006.09.14}
}

@ARTICLE{1999-KurshanMeritt.etal,
  author = {R.Kurshan and M.Meritt and A.Orda and S.R.Sachs},
  title = {Modelling Asynchrony with a Synchronous Model},
  journal = {Formal Methods in System Design},
  year = {1999},
  volume = {15},
  pages = {175 - 199},
  file = {Modelling asynchrony with a synchronous model.pdf:Modelling asynchrony with a synchronous model.pdf:PDF},
  timestamp = {2006.09.27}
}

@INPROCEEDINGS{2003-TzorefMatusevich.etal,
  author = {R.Tzoref and M.Matusevich and E.Berger I.Beer},
  title = {An Optimized Symbolic Bounded Model Checking Engine},
  year = {2003},
  comment = {Lecture Notes in Computer Science},
  file = {:./files/2003-TzorefMatusevich.etal.pdf:PDF},
  timestamp = {2006.09.19}
}

@INPROCEEDINGS{2005-RabinovitzGrumberg,
  author = {Ishai Rabinovitz and Orna Grumberg},
  title = {Bounded Model Checking Of Concurrent Programs},
  booktitle = {Proceedings of the 17th international conference on Computer Aided
	Verification},
  year = {2005},
  series = {CAV'05},
  pages = {82--97},
  address = {Berlin, Heidelberg},
  publisher = {Springer-Verlag},
  acmid = {2153243},
  file = {BoundedModelCheckingOfConcurrentPrograms.pdf:BoundedModelCheckingOfConcurrentPrograms.pdf:PDF},
  isbn = {3-540-27231-3, 978-3-540-27231-1},
  location = {Edinburgh, Scotland, UK},
  numpages = {16},
  timestamp = {2006.09.22}
}

@INPROCEEDINGS{2016-RajendranDhandayuthapany.etal,
  author = {Rajendran, Jeyavijayan and Dhandayuthapany, Arunshankar Muruga and
	Vedula, Vivekananda and Karri, Ramesh},
  title = {Formal security verification of third party intellectual property
	cores for information leakage},
  booktitle = {VLSI Design and 2016 15th International Conference on Embedded Systems
	(VLSID), 2016 29th International Conference on},
  year = {2016},
  pages = {547--552},
  organization = {IEEE},
  owner = {fadiheh},
  timestamp = {2018.07.12}
}

@INPROCEEDINGS{1990-RajskiVasudevamurthy,
  author = {J. Rajski and J. Vasudevamurthy},
  title = {Testability Preserving Transformations in Multi-Level Logic Synthesis},
  booktitle = {Proc. International Test Conference (ITC)},
  year = {1990},
  pages = {265 -273},
  file = {:./files/1990-RajskiVasudevamurthy.pdf:PDF},
  keywords = {{Boolean} expressions;algebraic divisors;combinatorial logic;decomposition;double-cube
	divisors;factorization;irredundant multilevel networks;multi-level
	logic synthesis;polynomial;reasoning;single-cube divisors;testability;transformations;two-level
	representation;{Boolean} algebra;logic CAD;logic testing;polynomials;}
}

@TECHREPORT{2004-Ralphs,
  author = {Ted K. Ralphs},
  title = {{SYMPHONY} Version 5.0 User's Manual},
  institution = {Lehigh University Industrial and Systems Engineering},
  year = {2004},
  number = {04T-020},
  url = {http://www.coin-or.org/SYMPHONY/man-5.0/}
}

@MASTERSTHESIS{2013-RakeshRaman,
  author = {Rakesh Raman},
  title = {Construction of Cycle-Accurate Program Netlist for the Formal Verification
	of Firmware Based Designs},
  school = {TU Kaiserslautern},
  year = {2013},
  type = {{Masterarbeit}},
  file = {:files/2013-RakeshRaman.pdf:PDF},
  owner = {villarraga},
  timestamp = {2014.02.05}
}

@MISC{2006-RaniseTinelli,
  author = {Silvio Ranise and Cesare Tinelli},
  title = {The Satisfiability Modulo Theories Library ({SMT}-{LIB})},
  year = {2006},
  owner = {pavlenko},
  timestamp = {2010.06.09},
  url = {http://www.SMT-LIB.org}
}

@ARTICLE{2015-RashidPattabiraman.etal,
  author = {L. Rashid and K. Pattabiraman and S. Gopalakrishnan},
  title = {Characterizing the Impact of Intermittent Hardware Faults on Programs},
  journal = {IEEE Transactions on Reliability},
  year = {2015},
  volume = {64},
  pages = {297-310},
  number = {1},
  month = {March},
  file = {2015-RashidPattabiraman.etal.pdf:files/2015-RashidPattabiraman.etal.pdf:PDF},
  issn = {0018-9529},
  owner = {bartsch},
  timestamp = {2015.08.03}
}

@INPROCEEDINGS{2005-RaudvereSingh.etal,
  author = {Tarvo Raudvere and Ashish Kumar Singh and Ingo Sander and Axel Jantsch},
  title = {System Level Verification of Digital Signal Processing Applications
	Based on the Polynomial Abstraction Technique},
  booktitle = {Proc. International Conference on Computer-Aided Design (ICCAD)},
  year = {2005},
  pages = { 285 - 290},
  file = {:./files/2005-RaudvereSingh.etal.pdf:PDF},
  keywords = { abstract model; data abstraction; data properties; digital signal
	processing; infinite domain; model checking; polynomial abstraction
	technique; sequential circuits; system level verification; integrated
	circuit design; integrated circuit modelling; logic design; polynomials;
	sequential circuits;},
  timestamp = {2006.09.27}
}

@INPROCEEDINGS{1995-RaviSomenzi,
  author = {K. Ravi and F. Somenzi},
  title = {High Density Reachability Analysis},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {1995},
  pages = {154-158},
  file = {:./files/1995-RaviSomenzi.pdf:PDF},
  key = {RaSo95}
}

@INPROCEEDINGS{2009-RayHao.etal,
  author = {Ray, Sandip and Hao, Kecheng and Chen, Yan and Xie, Fei and Yang,
	Jin},
  title = {Formal Verification for High-Assurance Behavioral Synthesis},
  booktitle = {Proc. Intl. Symposium on Automated Technology for Verification and
	Analysis (ATVA)},
  year = {2009},
  pages = {337--351},
  address = {Berlin, Heidelberg},
  publisher = {Springer},
  acmid = {1692405},
  file = {:files/2009-RayHao.etal.pdf:PDF},
  location = {Macao, China},
  numpages = {15},
  owner = {joakim},
  timestamp = {2013.05.07}
}

@INPROCEEDINGS{2004-RayHunt,
  author = {Sandip Ray and Hunt, Jr., Warren A.},
  title = {Deductive Verification of Pipelined Machines Using First-Order Quantification},
  booktitle = {Proc. Intl. Conf. on Computer-Aided Verification (CAV)},
  year = {2004},
  pages = {31-43},
  address = {Boston, MA},
  publisher = {Springer},
  file = {:files/2004-RayHunt.pdf:PDF},
  owner = {joakim},
  timestamp = {2012.12.17}
}

@INPROCEEDINGS{1999-RebaudengoViolante.etal,
  author = {Maurizio Rebaudengo and Matteo Sonza Reorda and Marco Torchiano and
	Massimo Violante},
  title = {Soft-error Detection through Software Fault-Tolerance Techniques},
  booktitle = {Defect and Fault Tolerance in {VLSI} Systems, 1999. {DFT} '99. International
	Symposium on},
  year = {1999},
  pages = {210 -218},
  month = {nov},
  file = {:./files/1999-RebaudengoViolante.etal.pdf:PDF},
  keywords = {code redundancy;data redundancy;fault coverage;high-level language;soft-error
	detection;software fault-tolerance techniques;error detection;high
	level languages;redundancy;software fault tolerance;},
  timestamp = {2006.09.14}
}

@ARTICLE{2004-RebaudengoViolante.etal,
  author = {M. Rebaudengo and M. Sonza Reorda and M. Violante},
  title = {A New Approach to Software-Implemented Fault Tolerance},
  journal = {J. Electron. Test.},
  year = {2004},
  volume = {20},
  pages = {433--437},
  number = {4},
  month = aug,
  acmid = {1016939},
  address = {Norwell, MA, USA},
  file = {:./files/2004-RebaudengoViolante.etal.pdf:PDF},
  issn = {0923-8174},
  issue_date = {August 2004},
  keywords = {fault injection, single event upsets, software-implemented fault tolerance},
  numpages = {5},
  publisher = {Kluwer Academic Publishers},
  timestamp = {2006.09.14}
}

@INPROCEEDINGS{2002-RedaDrechsler.etal,
  author = {Sherief Reda and Rolf Drechsler and Alex Orailoglu},
  title = {On Relation between {SAT} and {BDD}s for Equivalence Checking},
  booktitle = {Proc. International Symposium on Quality of Electronic Design ({ISQED})},
  year = {2002},
  pages = { 394 - 399},
  file = {:./files/2002-RedaDrechsler.etal.pdf:PDF},
  keywords = { BDD paths; BDD variable ordering; {Boolean} formulas; {Boolean} operations;
	{Boolean} satisfiability problem; DP procedure; Davis-Putnam procedure;
	SAT solvers; backtracks; binary decision diagrams; equivalence checking;
	verification tools; {Boolean} algebra; backtracking; binary decision
	diagrams; circuit CAD; computability; equivalent circuits; integrated
	circuit design; logic CAD; logic design;},
  timestamp = {2006.09.13}
}

@INPROCEEDINGS{1995-ReddyKunz.etal,
  author = {S. Reddy and W. Kunz and D. Pradhan},
  title = {A Novel Verification Framework Combining Structural and {OBDD} Methods
	in a Synthesis Environment},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {1995},
  pages = {414-419},
  month = {June},
  file = {:./files/1995-ReddyKunz.etal.pdf:PDF}
}

@INPROCEEDINGS{2016-ReidChen.etal,
  author = {A. Reid and R. Chen and A. Deligiannis and D. Gilday and D. Hoyes
	and W. Keen and A. Pathirane and O. Shepherd and P. Vrabel and A.
	Zaidi},
  title = {End-to-End Verification of {ARM} \textsuperscript{\textregistered}
	Processors with {ISA-F}ormal},
  booktitle = {Proceedings of 28th Intl. Conf. on CAV},
  year = {2016},
}

@INBOOK{2016-ReinekeWilhelm,
  pages = {74--87},
  title = {Static Timing Analysis -- What is Special?},
  publisher = {Springer International Publishing},
  year = {2016},
  editor = {Probst, Christian W. and Hankin, Chris and Hansen, Ren{\'e} Rydhof},
  author = {Reineke, Jan and Wilhelm, Reinhard},
  address = {Cham},
  booktitle = {Semantics, Logics, and Calculi: Essays Dedicated to Hanne Riis Nielson
	and Flemming Nielson on the Occasion of Their 60th Birthdays},
  file = {2016-ReinekeWilhelm.pdf:files/2016-ReinekeWilhelm.pdf:PDF},
  isbn = {978-3-319-27810-0},
  owner = {schwarz},
  timestamp = {2017.01.09}
}

@MISC{1995-Reinelt,
  author = {Gerd Reinelt},
  title = {{TSPLIB} 95},
  year = {1995},
  note = {Institut fuer Angewandte Mathematik, Universitaet Heidelberg},
  file = {:./files/1995-Reinelt.pdf:PDF},
  owner = {stoffel},
  timestamp = {2016.05.11},
  url = {http://www.iwr.uni-heidelberg.de/groups/comopt/software/TSPLIB95}
}

@MISC{2005-Renesas,
  author = {{Renesas Electronics Corporation TYO}},
  title = {{SH-1/SH-2/SH-DSP} Software Manual, Rev. 5.0},
  howpublished = {http://www.renesas.com/},
  year = {2005},
  file = {2005-Renesas.pdf:files/2005-Renesas.pdf:PDF},
  owner = {villarraga},
  timestamp = {2010.06.15}
}

@INPROCEEDINGS{1998-Rennels,
  author = {David A. Rennels},
  title = {Fault-Tolerant Computing},
  booktitle = {Encyclopedia of Computer Science},
  year = {1998},
  pages = {698--702},
  address = {Chichester, UK},
  publisher = {John Wiley and Sons Ltd.},
  acmid = {1074394},
  file = {:./files/1998-Rennels.pdf:PDF},
  isbn = {0-470-86412-5},
  numpages = {5},
  timestamp = {2006.09.14}
}

@INPROCEEDINGS{2012-renzelmann.etal,
  author = {Renzelmann, Matthew J and Kadav, Asim and Swift, Michael M},
  title = {SymDrive: Testing Drivers without Devices.},
  booktitle = {Proceedings of the 10th USENIX Symposium on Operating Systems Design
	and Implementation},
  year = {2012},
  volume = {1},
  number = {4},
  series = {OSID'12},
  pages = {279 - 292},
  address = {Hollywood, CA, USA},
  month = {October}
}

@INPROCEEDINGS{2010-RepsLim.etal,
  author = {Reps, Thomas and Lim, Junghee and Thakur, Aditya and Balakrishnan,
	Gogul and Lal, Akash},
  title = {There's plenty of room at the bottom: analyzing and verifying machine
	code},
  booktitle = {Proceedings of the 22nd international conference on Computer Aided
	Verification},
  year = {2010},
  series = {CAV'10},
  pages = {41--56},
  address = {Berlin, Heidelberg},
  publisher = {Springer-Verlag},
  acmid = {2144318},
  file = {2010-RepsLim.etal.pdf:files/2010-RepsLim.etal.pdf:PDF},
  isbn = {3-642-14294-X, 978-3-642-14294-9},
  location = {Edinburgh, UK},
  numpages = {16},
  owner = {villarraga},
  timestamp = {2012.09.12}
}

@INPROCEEDINGS{2003-ReshadiMishra.etal,
  author = {Mehrdad Reshadi and Prabhat Mishra and Nikil Dutt},
  title = {Instruction Set Compiled Simulation A Technique for Fast and Flexible
	Instruction Set Simulation},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {2003},
  pages = { 758 - 763},
  file = {:./files/2003-ReshadiMishra.etal.pdf:PDF},
  keywords = { IS-CS technique; compile time; compiled simulator; decoding process;
	fast instruction accurate simulation; instruction abstraction technique;
	instruction set architecture; instruction set compiled simulation;
	instruction set simulation; interpretive simulator; optimized decoded
	instruction; programmable architecture; simulation performance; time-to-market
	pressure; compiler generators; digital simulation; instruction sets;
	parallel architectures; performance evaluation;},
  timestamp = {2006.09.27}
}

@BOOK{1983-Rich,
  title = {Artificial Intelligence},
  publisher = {McGraw-Hill},
  year = {1983},
  author = {E. Rich},
  file = {:./files/1983-Rich.pdf:PDF}
}

@ARTICLE{2016-RiefertCantoro.etal,
  author = {A. Riefert and R. Cantoro and M. Sauer and M. Sonza Reorda and B.
	Becker},
  title = {A Flexible Framework for the Automatic Generation of SBST Programs},
  journal = {IEEE Transactions on Very Large Scale Integration (VLSI) Systems},
  year = {2016},
  volume = {24},
  pages = {3055-3066},
  number = {10},
  month = {Oct},
  issn = {1063-8210},
  owner = {bartsch},
  timestamp = {2016.12.02}
}

@INPROCEEDINGS{2014-RiefertCiganda.etal,
  author = {Riefert, Andreas and Ciganda, Lyl and Sauer, Matthias and Bernardi,
	Paolo and Reorda, Matteo Sonza and Becker, Bernd},
  title = {An effective approach to automatic functional processor test generation
	for small-delay faults},
  booktitle = {Design, Automation and Test in Europe Conference and Exhibition},
  year = {2014},
  pages = {1 - 6},
  month = {March},
  organization = {IEEE},
  file = {:files/2014-RiefertCiganda.etal.pdf:PDF},
  owner = {bartsch},
  timestamp = {2014.08.21}
}

@INPROCEEDINGS{2013-RiefertMuller.etal,
  author = {Riefert, Andreas and Muller, Jorg and Sauer, Matthias and Burgard,
	Wolfram and Becker, Bernd},
  title = {Identification of critical variables using an FPGA-based fault injection
	framework},
  booktitle = {Proc. 31st VLSI Test Symposium},
  year = {2013},
  pages = {1 - 6},
  month = {May},
  organization = {IEEE},
  file = {:files/2013-RiefertMuller.etal.pdf:PDF},
  owner = {bartsch},
  timestamp = {2014.08.21}
}

@TECHREPORT{1992-RimenOhlsson.etal,
  author = {M. Rimen and J. Ohlsson and J. Karlsson and E. Jenn and J. Arlat},
  title = {Validation-Of-Fault-Tolerance By Fault Injection In {VHDL} Simulation
	Models},
  institution = {Department of Computer Engineering, School of Electrical and Computer
	Engineering, Chalmers University of Technology, G�teborg, Sweden},
  year = {1992},
  file = {:./files/1992-RimenOhlsson.etal.pdf:PDF},
  timestamp = {2006.09.14}
}

@PHDTHESIS{2001-Ritter,
  author = {Gerd Ritter},
  title = {Formal Sequential Equivalence Checking by Simbolic Simulation},
  school = {Darmstadt University of Technology, Germany},
  year = {2001},
  file = {:./files/2001-Ritter.pdf:PDF},
  timestamp = {2006.09.13}
}

@INPROCEEDINGS{2013-RobacheBoland.etal,
  author = {R. Robache and J.-F. Boland and C. Thibeault and Y. Savaria},
  title = {A methodology for system-level fault injection based on gate-level
	faulty behavior},
  booktitle = {New Circuits and Systems Conference (NEWCAS), 2013 IEEE 11th International},
  year = {2013},
  pages = {1 - 4},
  month = {June},
  file = {2013-RobacheBoland.etal.pdf:files/2013-RobacheBoland.etal.pdf:PDF},
  owner = {bartsch},
  timestamp = {2016.01.07}
}

@ARTICLE{1997-RobertsonHoeher.etal,
  author = {P. Robertson and P. Hoeher and E. Villebrun},
  title = {Optimal and Sub-Optimal Maximum a Posteriori Algorithms Suitable
	for Turbo Decoding},
  journal = {European Transactions on Telecommunications ({ETT})},
  year = {1997},
  volume = {8},
  pages = {119--125},
  number = {2},
  month = {March--April},
  file = {:./files/1997-RobertsonHoeher.etal.pdf:PDF},
  optnote = {Almost the same as ICC '95 paper}
}

@INPROCEEDINGS{2016-RodrigueQuintao.etal,
  author = {Rodrigues, Bruno and Quint{\~a}o Pereira, Fernando Magno and Aranha,
	Diego F},
  title = {Sparse representation of implicit flows with applications to side-channel
	detection},
  booktitle = {Proceedings of the 25th International Conference on Compiler Construction},
  year = {2016},
  pages = {110--120},
  organization = {ACM},
  owner = {jmueller},
  timestamp = {2019.08.16}
}

@ARTICLE{2002-RoopSowmya.etal,
  author = {Partha S. Roop and A. Sowmya and S. Ramesh},
  title = {k-time Forced Simulation A Formal Verification Technique for {IP}
	Reuse},
  journal = {{IEEE} Computer Society},
  year = {2002},
  pages = { 50 - 55},
  file = {:./files/2002-RoopSowmya.etal.pdf:PDF},
  keywords = { IP block; IP matching algorithm; bisimulation based algorithms; device
	driver; formal verification; intellectual property matching; k-time
	forced simulation; programmable IP block; bisimulation equivalence;
	circuit simulation; formal verification; hardware description languages;
	hardware-software codesign; industrial property;},
  timestamp = {2006.09.21}
}

@INPROCEEDINGS{0000-RoseSwan.etal,
  author = {Adam Rose and Stuart Swan and John Pierce and Jean-Michel Fernandez},
  title = {Transaction Level Modeling in SystemC},
  file = {0000-RoseSwan.etal.pdf:files/0000-RoseSwan.etal.pdf:PDF},
  timestamp = {2006.09.27}
}

@BOOK{2011-Rosen,
  title = {Discrete Mathematics and Its Applications},
  publisher = {McGraw-Hill Education},
  year = {2011},
  author = {Kenneth H. Rosen}
}

@INPROCEEDINGS{2005-RosenbandArvind,
  author = {Daniel L. Rosenband and Arvind},
  title = {Hardware Synthesis from Guarded Atomic Actions with Performance Specifications},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2005},
  pages = { 784 - 791},
  file = {:./files/2005-RosenbandArvind.pdf:PDF},
  keywords = { Bluespec; guarded atomic actions; hardware synthesis; performance
	specifications; rule composition; rule-based synthesis; scheduling
	specifications; single-issue processor pipeline; superscalar pipeline;
	high level synthesis; pipeline processing; processor scheduling;},
  timestamp = {2006.09.27}
}

@INPROCEEDINGS{2015-rossi.etal,
  author = {Rossi, Davide and Conti, Francesco and Marongiu, Andrea and Pullini,
	Antonio and Loi, Igor and Gautschi, Michael and Tagliavini, Giuseppe
	and Capotondi, Alessandro and Flatresse, Philippe and Benini, Luca},
  title = {PULP: A parallel ultra low power platform for next generation IoT
	applications},
  booktitle = {Hot Chips 27 Symposium (HCS), 2015 IEEE},
  year = {2015},
  pages = {1--39},
  organization = {IEEE}
}

@ARTICLE{1966-Roth,
  author = {J. Paul. Roth},
  title = {Diagnosis of Automata Failures: A Calculus and a Method},
  journal = {{IBM} Journal of Research and Development},
  year = {1966},
  volume = {10},
  pages = {278-291},
  number = {4},
  month = {July},
  file = {:./files/1966-Roth.pdf:PDF}
}

@ARTICLE{1966-RothKarp,
  author = {J. P. Roth and R. M. Karp},
  title = {Minimization over {Boolean} Graphs},
  journal = {{IBM} Journal of Research and Development},
  year = {1966},
  volume = {10},
  pages = {278-291},
  number = {4},
  month = {July},
  file = {:./files/1966-RothKarp.pdf:PDF}
}

@BOOK{2004-Rowen,
  title = {Engineering the Complex {SOC} Fast, Flexible Design with Configurable
	Processors},
  publisher = {Prentice Hall PTR},
  year = {2004},
  author = {C. Rowen}
}

@INPROCEEDINGS{2001-RowenMaydan,
  author = {Chris Rowen and Dror Maydan},
  title = {Automated Processor Generation for System-on-Chip},
  booktitle = {Proc. European Solid-State Circuits Conference},
  year = {2001},
  pages = {464 -469},
  file = {:./files/2001-RowenMaydan.pdf:PDF},
  timestamp = {2006.10.04}
}

@ARTICLE{2003-RoyMukhopadhyay.etal,
  author = {K. Roy and S. Mukhopadhyay and H. Mahmoodi-Meimand},
  title = {Leakage current mechanisms and leakage reduction techniques in deep-submicrometer
	{CMOS} circuits},
  journal = {Proceedings of the IEEE},
  year = {2003},
  volume = {91},
  pages = {305-327},
  file = {:/import/var/jabref/files/2003-RoyMukhopadhyay.etal.pdf:PDF},
  owner = {udupi},
  timestamp = {2017.03.28}
}

@INPROCEEDINGS{2005-RoyDas.etal,
  author = {Suchismita Roy and Sayantan Das and Prasenjit Basu and Pallab Dasgupta
	and P.P. Chakrabarti},
  title = {{SAT} Based Solutions for Consistency Problems in Formal Property
	Specifications for Open Systems},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2005},
  pages = { 885 - 888},
  file = {:./files/2005-RoyDas.etal.pdf:PDF},
  keywords = { SAT based algorithms; assertion-based verification; assume-guarantee
	property; consistency problems; formal language; formal property
	verification; module level validation; open systems; specification
	errors; computability; formal specification; formal verification;
	open systems;},
  timestamp = {2006.09.27}
}

@INPROCEEDINGS{2003-RoychoudhuryMitra.etal,
  author = {Abhik Roychoudhury and Tulika Mitra and S.R. Karri},
  title = {Using formal techniques to Debug the {AMBA} System-on-Chip Bus Protocol},
  booktitle = {Proc. International Conference on Design, Automation and Test in
	Europe},
  year = {2003},
  pages = { 828 - 833},
  file = {:./files/2003-RoychoudhuryMitra.etal.pdf:PDF},
  keywords = { AMBA SoC bus protocol debugging; IP core data transfer; advanced
	micro-controller bus architecture protocol; burst transfers; bus
	starvation; formal specification; formal verification; intellectual
	property cores; model checking; pipelined bus protocols; pipelining;
	split transfers; state space exploration; system-on-chip; formal
	specification; formal verification; industrial property; logic testing;
	pipeline processing; protocols; state-space methods; system buses;
	system-on-chip;},
  timestamp = {2006.09.19}
}

@ARTICLE{2006-RoychoudhuryYang,
  author = {Abhik Roychoudhury and Zijiang Yang},
  title = {Software Verification and Validation},
  journal = {{IEEE} Software},
  year = {2006},
  volume = {6},
  pages = {10 - 17},
  editor = {Abhik Roychoudhury, Zijiang Yang},
  file = {:./files/2006-RoychoudhuryYang.pdf:PDF},
  timestamp = {2006.09.21}
}

@INPROCEEDINGS{1993-Rudell,
  author = {R. Rudell},
  title = {Dynamic Variable Ordering for Ordered Binary Decision Diagrams},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {1993},
  pages = {42-47},
  file = {:./files/1993-Rudell.pdf:PDF}
}

@ARTICLE{1987-RudellSangiovanniVincentelli,
  author = {R. Rudell and A. Sangiovanni-Vincentelli},
  title = {Multiple-valued Minimization for {PLA} Optimization},
  journal = {IEEE Transactions on Computer-Aided Design},
  year = {1987},
  volume = {CAD-6},
  pages = {727-750},
  number = {5},
  month = {September},
  file = {:./files/1987-RudellSangiovanniVincentelli.pdf:PDF}
}

@INPROCEEDINGS{2001-RufHoffmann.etal,
  author = {JuErgen Ruf and Dirk W. Hoffmann and Thomas Kropf and Wolfgang Rosenstiel},
  title = {Simulation-Guided Property Checking Based on Multi-Valued AR-Automata},
  booktitle = {Proc. International Conference on Design, Automation and Test in
	Europe ({DATE})},
  year = {2001},
  pages = {742 -748},
  file = {:./files/2001-RufHoffmann.etal.pdf:PDF},
  keywords = {SystemC language;VHDL code;abstract model;digital design verification;embedded
	hardware/software systems;executable description language;finite
	linear time temporal logic;finite state machines;formal methods;hardware
	verification;multivalued AR-automata;simulation-guided property checking;state
	space reduction;temporal properties;embedded systems;finite state
	machines;formal verification;hardware description languages;hardware-software
	codesign;multivalued logic;temporal logic;},
  timestamp = {2006.09.21}
}

@INPROCEEDINGS{2002-BarnerDavid.etal,
  author = {S.Barner and S. B.David and A.Gringuaze and B.Sterin Y.Wolfsthal},
  title = {An Algorithmic Approach to Design Exploration},
  booktitle = {Proceedings of the International Symposium of Formal Methods Europe
	on Formal Methods - Getting {IT} Right},
  year = {2002},
  series = {FME '02},
  pages = {146--162},
  address = {London, UK, UK},
  publisher = {Springer-Verlag},
  acmid = {730164},
  file = {:./files/2002-BarnerDavid.etal.pdf:PDF},
  isbn = {3-540-43928-5},
  keywords = {hardware debugging, hardware exploration, model checking},
  numpages = {17},
  timestamp = {2006.09.21}
}

@INPROCEEDINGS{2002-CandraGodefroid.etal,
  author = {S.Candra and P.Godefroid and C.Palm},
  title = {Software Model Checking in Practice An Industrial Case Study},
  booktitle = {Proc. the International Conference on Software Engineering},
  year = {2002},
  pages = {431 -441},
  file = {:./files/2002-CandraGodefroid.etal.pdf:PDF},
  keywords = {CDMA call-processing library;CDMA call-processing software;VeriSoft;concurrent
	reactive software;industrial software product;software model checking;wireless
	networks;code division multiple access;program testing;software maintenance;},
  timestamp = {2006.09.22}
}

@MISC{2001-GarlandLynch.etal,
  author = {S.J.Garland and N.A.Lynch and M.Vaziri},
  title = {{IOA} : A Langauge for Specifying Programming and Validating Distributed
	Systems},
  year = {2001},
  file = {:./files/2001-GarlandLynch.etal.pdf:PDF},
  owner = {stoffel},
  timestamp = {2006.09.18}
}

@INPROCEEDINGS{2000-MukhopadhyayPodelski,
  author = {S.Mukhopadhyay and A.Podelski},
  title = {Model Checking for Timed Logic Processes},
  booktitle = {Proceedings of the First International Conference on Computational
	Logic},
  year = {2000},
  pages = {598--612},
  address = {London, UK, UK},
  publisher = {Springer-Verlag},
  acmid = {728429},
  file = {:./files/2000-MukhopadhyayPodelski.pdf:PDF},
  isbn = {3-540-67797-6},
  numpages = {15},
  timestamp = {2006.09.19}
}

@INPROCEEDINGS{1995-OwreRushby.etal,
  author = {S.Owre And J. Rushby And N.Shankar And F.Henke},
  title = {Formal Verfication for Fault-Tolerant Architectures :Prolegomena
	to the Design of {PVS}},
  booktitle = {Software Engineering, IEEE Transactions on},
  year = {1995},
  volume = {21},
  number = {2},
  pages = {107 -125},
  month = {feb},
  file = {:./files/1995-OwreRushby.etal.pdf:PDF},
  keywords = {AAMP5;PVS;collaborative project;collaborative verifications;commercial
	avionics processor;fault-tolerant architecture;fault-tolerant architectures;formal
	specifications;formal verification;life-critical digital flight-control
	applications;reliable computing platform;verification systems;aerospace
	control;computer architecture;fault tolerant computing;formal specification;formal
	verification;reliability;safety-critical software;},
  timestamp = {2006.09.14}
}

@INPROCEEDINGS{2018-SaidQuante.etal,
  author = {W. Said and J. Quante and R. Koschke},
  title = {On State Machine Mining from Embedded Control Software},
  booktitle = {2018 IEEE International Conference on Software Maintenance and Evolution
	(ICSME)},
  year = {2018},
  owner = {fehmel},
  timestamp = {2019.05.27}
}

@MISC{1995-Sakallah,
  author = {Karem A. Sakallah},
  title = {Functional Abstraction and Partial Specification of {Boolean} Function},
  year = {1995},
  file = {:./files/1995-Sakallah.pdf:PDF},
  owner = {stoffel},
  timestamp = {2006.09.12}
}

@TECHREPORT{1988-SaltzmanHillier,
  author = {Robert M. Saltzman and Frederick S. Hillier},
  title = {A Heuristic Ceiling Point Algorithm for General Integer Linear Programming},
  institution = {Department of Operations Research Stanford University},
  year = {1988},
  file = {:./files/1988-SaltzmanHillier.pdf:PDF}
}

@INPROCEEDINGS{1994-Sander,
  author = {Georg Sander},
  title = {Graph Layout Through The Vcg Tool},
  booktitle = {Proc. {DIMACS} International Workshop on Graph Drawing},
  year = {1994},
  file = {:./files/1994-Sander.pdf:PDF},
  timestamp = {2006.09.21}
}

@INPROCEEDINGS{2008-SarbisheiAlizadeh.etal,
  author = {Sarbishei, O. and Alizadeh, B. and Fujita, M.},
  title = {Arithmetic Circuits Verification without Looking for Internal Equivalences},
  year = {2008},
  pages = {7 -16},
  month = {jun.},
  file = {:./files/2008-SarbisheiAlizadeh.etal.pdf:PDF},
  journal = {Formal Methods and Models for Co-Design, 2008. {MEMOCODE} 2008. 6th
	{ACM/IEEE} International Conference on},
  owner = {pavlenko},
  timestamp = {2010.10.04}
}

@ARTICLE{2009-SarbisheiTabandeh.etal,
  author = {O. Sarbishei and M. Tabandeh and B. Alizadeh and M. Fujita},
  title = {A Formal Approach for Debugging Arithmetic Circuits},
  journal = {{IEEE} Transactions on Computer-Aided Design},
  year = {2009},
  volume = {28},
  pages = {742-754},
  number = {05},
  month = {May},
  file = {:./files/2009-SarbisheiTabandeh.etal.pdf:PDF},
  owner = {wedler},
  timestamp = {2009.09.03}
}

@INPROCEEDINGS{2001-SavatonCoussy.etal,
  author = {Guillaume Savaton and Philippe Coussy and Emmanuel Casseau and Eric
	Martin},
  title = {A Methodology for Behavioral Virtual Component Specification Targeting
	{SoC} Design with High-Level Synthesis Tools},
  booktitle = {Proc. Forum on Design Languages ({FDL})},
  year = {2001},
  pages = {3--9},
  file = {:./files/2001-SavatonCoussy.etal.pdf:PDF},
  timestamp = {2006.09.19}
}

@ARTICLE{1994-Savelsbergh,
  author = {Martin W.P. Savelsbergh},
  title = {Preprocessing and Probing Techniques for Mixed Integer Programming
	Problems},
  journal = {{ORSA} Journal on Computing},
  year = {1994},
  volume = {6},
  pages = {445-454},
  file = {:./files/1994-Savelsbergh.pdf:PDF}
}

@INPROCEEDINGS{1991-SavojBrayton.etal,
  author = {H. Savoj and R. K. Brayton and H. Touati},
  title = {Extracting Local Don't-Cares for Network Optimization},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {1991},
  pages = {514-517},
  month = {November},
  file = {:./files/1991-SavojBrayton.etal.pdf:PDF},
  keywords = { {Boolean} network; benchmark circuits; binary decision diagrams;
	image computation techniques; local don't cares extraction; network
	optimization; sequential interactive logic synthesis system; two-level
	minimizer; {Boolean} functions; combinatorial circuits; logic CAD;
	logic testing;}
}

@MISC{0000-Sawada,
  author = {Jun Sawada and Warren A. Hunt and Jr.},
  title = {Decomposing the Verification of Pipelined Microprocessors with Invariant
	Conditions},
  file = {0000-Sawada.pdf:files/0000-Sawada.pdf:PDF},
  owner = {stoffel},
  timestamp = {2016.05.11}
}

@MISC{0000-SayerSonander,
  author = {Carey Sayer and Jeremy Sonander},
  title = {Formal Verification of {AMBA} Bus Systems},
  file = {0000-SayerSonander.pdf:files/0000-SayerSonander.pdf:PDF},
  owner = {stoffel},
  timestamp = {2006.09.21}
}

@INPROCEEDINGS{1997-SchaafJames,
  author = {Schaaf,Jr., James C. and Thompson, Faye Lynn},
  title = {System Concept Development with Virtual Prototyping},
  booktitle = {Proceedings of the 29th Conference on Winter Simulation},
  year = {1997},
  series = {WSC '97},
  pages = {941--947},
  address = {Washington, DC, USA},
  isbn = {0-7803-4278-X},
  location = {Atlanta, Georgia, USA},
  numpages = {7},
  owner = {joakim},
  timestamp = {2016.03.18}
}

@CONFERENCE{2006-SchickelNimbler.etal,
  author = {M. Schickel and V. Nimbler and M. Braun and H. Eveking},
  title = {On Consistency and Completeness of Property Sets: Exploiting the
	Property-Based Design Process},
  booktitle = {Proc. Forum on Design Languages},
  year = {2006},
  file = {:./files/2006-SchickelNimbler.etal.pdf:PDF},
  owner = {stoffel},
  timestamp = {2010.07.28}
}

@ARTICLE{2010-Schlich,
  author = {Schlich, Bastian},
  title = {Model checking of software for microcontrollers},
  journal = {ACM Trans. Embed. Comput. Syst.},
  year = {2010},
  volume = {9},
  pages = {36:1--36:27},
  number = {4},
  month = {March},
  acmid = {1721702},
  address = {New York, NY, USA},
  articleno = {36},
  file = {2010-Schlich.pdf:files/2010-Schlich.pdf:PDF},
  issn = {1539-9087},
  issue_date = {March 2010},
  keywords = {Assembly code, formal verification, microcontroller, model checking,
	static analysis},
  numpages = {27},
  owner = {villarraga},
  publisher = {ACM},
  timestamp = {2012.08.27}
}

@INPROCEEDINGS{2011-SchlichNoll.etal,
  author = {Schlich, Bastian and Noll, Thomas and Brauer, J{\"o}rg and Brutschy,
	Lucas},
  title = {Reduction of interrupt handler executions for model checking embedded
	software},
  booktitle = {Proceedings of the 5th international Haifa verification conference
	on Hardware and software: verification and testing},
  year = {2011},
  series = {HVC'09},
  pages = {5--20},
  address = {Berlin, Heidelberg},
  publisher = {Springer-Verlag},
  acmid = {1965981},
  isbn = {978-3-642-19236-4},
  location = {Haifa, Israel},
  numpages = {16},
  owner = {villarraga},
  timestamp = {2012.10.29}
}

@INPROCEEDINGS{2013-SchmidtVillarraga.etal,
  author = {Bernard Schmidt and Carlos Villarraga and J{\"o}rg Bormann and Dominik
	Stoffel and Markus Wedler and Wolfgang Kunz},
  title = {A Computational Model for {SAT}-Based Verification of Hardware-Dependent
	Low-Level Embedded System Software},
  booktitle = {Proceedings of the 18th Asia and South Pacific Design Automation
	Conference ({ASP-DAC})},
  year = {2013},
  pages = {711-716},
  file = {:files/2013-SchmidtVillarraga.etal.pdf:PDF},
  owner = {bschmidt},
  timestamp = {2013.01.11}
}

@INPROCEEDINGS{2013b-SchmidtVillarraga.etal,
  author = {Bernard Schmidt and Carlos Villarraga and Thomas Fehmel and J{\"o}rg
	Bormann and Dominik Stoffel and Wolfgang Kunz},
  title = {A Hardware-Dependent Model for {SAT}-Based Verification of Interrupt-Driven
	Low-Level Embedded System Software},
  booktitle = {16. {GI/ITG/GMM} Workshop Methoden und Beschreibungssprachen zur
	Modellierung und Verifikation von Schaltungen und Systemen ({MBMV})},
  year = {2013},
  file = {Paper:files/2013b-SchmidtVillarraga.etal.pdf:PDF},
  owner = {bschmidt},
  timestamp = {2013.11.08}
}

@ARTICLE{2013a-SchmidtVillarraga.etal,
  author = {Bernard Schmidt and Carlos Villarraga and Thomas Fehmel and J{\"o}rg
	Bormann and Markus Wedler and Minh Nguyen and Dominik Stoffel and
	Wolfgang Kunz},
  title = {A New Formal Verification Approach for Hardware-dependent Embedded
	System Software},
  journal = {IPSJ Transactions on System LSI Design Methodology (Special Issue
	on ASPDAC-2013)},
  year = {2013},
  volume = {6},
  pages = {135-145},
  file = {2013a-SchmidtVillarraga.etal.pdf:files/2013a-SchmidtVillarraga.etal.pdf:PDF},
  owner = {villarraga},
  timestamp = {2013.09.18}
}

@ARTICLE{2007-SchmidtWehn,
  author = {D. Schmidt and N. Wehn},
  title = {Hardware/Software Tradeoffs for Advanced {3G} Channel Decoding},
  journal = {Customizable Embedded Processors},
  year = {Morgan Kaufmann Publishers 2007},
  pages = {361--379},
  editor = {P. Ienne and R. Leupers},
  owner = {vogt},
  publisher = {Morgan Kaufmann Publishers},
  timestamp = {2006.08.22}
}

@BOOK{2000-Schoening,
  title = {Logik fuer Informatiker, 5. Auflage},
  publisher = {Spektrum Akademischer Verlag},
  year = {2000},
  author = {U. Schoening}
}

@INPROCEEDINGS{2001-SchollChristoph.etal,
  author = {Scholl, Christoph and Becker, Bernd},
  title = {Checking equivalence for partial implementations},
  booktitle = {Proceedings of the 38th annual Design Automation Conference},
  year = {2001},
  series = {DAC '01},
  pages = {238--243},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {378471},
  file = {:./files/2001-SchollChristoph.etal.pdf},
  isbn = {1-58113-297-2},
  location = {Las Vegas, Nevada, United States},
  numpages = {6},
  owner = {pavlenko},
  timestamp = {2011.06.03}
}

@INPROCEEDINGS{1998-SchollBecker.etal,
  author = {C. Scholl and B. Becker and T.M. Weis},
  title = {Word-Level Decision Diagrams, {WLCDs} and Division},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {1998},
  pages = {672-677},
  file = {:./files/1998-SchollBecker.etal.pdf:PDF}
}

@BOOK{1998-Schrijver,
  title = {Theory of linear and integer programming},
  publisher = {John Wiley \& Sons},
  year = {1998},
  author = {Schrijver, Alexander},
  file = {1998-Schrijver.pdf:files/1998-Schrijver.pdf:PDF},
  owner = {schwarz},
  timestamp = {2017.01.11}
}

@ARTICLE{1997-Schubert,
  author = {M. Schubert},
  title = {Mixed Analog-Digital Signal Modeling Using Event-Driven {VHDL}},
  journal = {Brazilian Symposium on Integrated Circuit Design - {SBCCI}},
  year = {1997},
  file = {:./files/1997-Schubert.pdf:PDF}
}

@INPROCEEDINGS{1999-Schulte,
  author = {Christian Schulte},
  title = {Comparing Trailing and Copying for Constraint Programming},
  booktitle = {Proc. International Conference on Logic Programming},
  year = {1999},
  editor = {D. De Schreye},
  pages = {275-289},
  address = {Las Cruces, NM, USA},
  month = {November},
  publisher = {The MIT Press},
  file = {:./files/1999-Schulte.pdf:PDF}
}

@INPROCEEDINGS{1987-SchulzTrischler.etal,
  author = {M. Schulz and E. Trischler and T. Sarfert},
  title = {{SOCRATES}: A Highly Efficient Automatic Test Pattern Generation
	System},
  booktitle = {Computer-Aided Design of Integrated Circuits and Systems, IEEE Transactions
	on},
  year = {1988},
  volume = {7},
  number = {1},
  pages = {126 -137},
  month = {jan},
  keywords = {FAN algorithm;SOCRATES;automatic test pattern generation system;backtrackings;combinational
	benchmark circuits;conflicts;implication;multiple backtrace;redundancies;scan-based
	circuits;sensitization;automatic testing;combinatorial circuits;logic
	testing;}
}

@ARTICLE{2004-SchuppanBiere,
  author = {Viktor Schuppan and Armin Biere},
  title = {Efficient Reduction of Finite State Model Checking to Reachability
	Analysis},
  journal = {International Journal on Software Tools for Technology Transfer (STTT)},
  year = {2004},
  volume = {5},
  pages = {185--204},
  number = {2--3},
  file = {:./files/2004-SchuppanBiere.pdf},
  url = {http://citeseer.ist.psu.edu/schuppan04efficient.html}
}

@INPROCEEDINGS{2010-SchwarzAvgerinos.etal,
  author = {Schwartz, Edward J and Avgerinos, Thanassis and Brumley, David},
  title = {All you ever wanted to know about dynamic taint analysis and forward
	symbolic execution (but might have been afraid to ask)},
  booktitle = {IEEE symposium on Security and privacy (SP)},
  year = {2010},
  pages = {317--331},
  organization = {IEEE},
  owner = {fadiheh},
  timestamp = {2018.11.22}
}

@INPROCEEDINGS{2015-SchwarzChaari.etal,
  author = {Michael Schwarz and Moomen Chaari and Bogdan-Andrei Tabacaru and
	Wolfgang Ecker},
  title = {A Meta-Model-Based Approach for Semantic Fault Modeling on Multiple
	Abstraction Levels},
  booktitle = {Design and Verification Conference and Exhibition Europe},
  year = {2015},
  month = {November},
  file = {2015-SchwarzChaari.etal.pdf:files/2015-SchwarzChaari.etal.pdf:PDF},
  owner = {bartsch},
  timestamp = {2015.09.24}
}

@INPROCEEDINGS{2019-SchwarzStahl.etal,
  author = {Michael Schwarz and Rafael Stahl and Daniel Mueller-Gritschneder
	and Ulf Schlichtmann and Dominik Stoffel and Wolfgang Kunz},
  title = {ACCESS: HW/SW Co-Equivalence Checking for Firmware Optimization},
  booktitle = {Proceedings of the 56th Annual Design Automation Conference 2019},
  year = {2019},
  series = {DAC '19},
  pages = {187:1--187:6},
  address = {New York, NY, USA},
  publisher = {ACM},
  articleno = {187},
  isbn = {978-1-4503-6725-7},
  location = {Las Vegas, NV, USA},
  numpages = {6},
  owner = {schwarz},
  timestamp = {2019.05.07}
}

@INPROCEEDINGS{2019-schwarz-wip.etal,
  author = {Schwarz, Michael and Stoffel, Dominik and Kunz, Wolfgang},
  title = {ACCESS: HW/SW-Co-Equivalence Checking for Firmware Optimization},
  booktitle = {Proceedings of "Methoden und Beschreibungssprachen zur Modellierung
	und Verifikation von Schaltungen und Systemen" (MBMV)},
  year = {2019},
  editor = {Grimm, Christoph and Schneider, Klaus and Zivkovic, Carna},
  volume = {22},
  pages = {4 - 7},
  address = {Kaiserslautern},
  month = {April},
  publisher = {VDE VERLAG GMBH},
  note = {Work-in-Progress-Paper},
  owner = {schwarz},
  timestamp = {2019.08.06}
}

@INPROCEEDINGS{2017-schwarz,
  author = {Schwarz, Michael and Villarraga, Carlos and Stoffel, Dominik and
	Kunz, Wolfgang},
  title = {Cycle-accurate software modeling for RTL verification of embedded
	systems},
  booktitle = {Design and Diagnostics of Electronic Circuits \& Systems (DDECS),
	2017 IEEE 20th International Symposium on},
  year = {2017},
  pages = {103--108},
  organization = {IEEE}
}

@INPROCEEDINGS{2004-SebastianiSingerman.etal,
  author = {Roberto Sebastiani and Eli Singerman and Stefano Tonetta and Moshe
	Y. Vardi},
  title = {{GSTE} Is Partitioned Model Checking.},
  booktitle = {Proc. International Conference on Computer-Aided Verification ({CAV})},
  year = {2004},
  file = {:./files/2004-SebastianiSingerman.etal.pdf:PDF},
  timestamp = {2006.09.21}
}

@ARTICLE{1995-SegerBryant,
  author = {Carl-Johan H. Seger and Randal E. Bryant},
  title = {Formal Verification by Symbolic Evaluation of Partially-Ordered Trajectories},
  journal = {Formal Methods in System Design},
  year = {1995},
  volume = {6},
  pages = {147--189},
  number = {2},
  address = {Hingham, MA, USA},
  file = {:./files/1995-SegerBryant.pdf:PDF},
  issn = {0925-9856},
  publisher = {Kluwer Academic Publishers}
}

@ARTICLE{2005-SenMarinov.etal,
  author = {Sen, Koushik and Marinov, Darko and Agha, Gul},
  title = {{CUTE}: A Concolic Unit Testing Engine for C},
  journal = {SIGSOFT Softw. Eng. Notes},
  year = {2005},
  volume = {30},
  pages = {263--272},
  number = {5},
  month = sep,
  acmid = {1081750},
  address = {New York, NY, USA},
  issn = {0163-5948},
  issue_date = {September 2005},
  keywords = {concolic testing, data structure testing, explicit path model-checking,
	random testing, testing C programs, unit testing},
  numpages = {10},
  owner = {villarraga},
  publisher = {ACM},
  timestamp = {2016.07.19}
}

@ARTICLE{2016-SenMall,
  author = {Sen, Tamal and Mall, Rajib},
  title = {Extracting Finite State Representation of Java Programs},
  journal = {Software and Systems Modeling},
  year = {2016},
  volume = {15},
  pages = {497--511},
  number = {2},
  month = {May},
  owner = {fehmel},
  timestamp = {2019.05.27}
}

@TECHREPORT{1992-SentovichSingh.etal,
  author = {E. Sentovich and K. Singh and L. Lavagno and C. Moon and R. Murgai
	and A. Saldanha and H. Savoj and P. Stephan and R. Brayton and A.
	Sangiovanni-Vincentelli},
  title = {{SIS}: A System for Sequential Circuit Synthesis},
  institution = {Electronics Research Laboratory, University of California at Berlekey},
  year = {1992},
  number = {Memorandum No. UCB/ERL M92/41},
  file = {:./files/1992-SentovichSingh.etal.pdf:PDF}
}

@ARTICLE{2012-SeomunShin.etal,
  author = {J. Seomun and I. Shin and Y. Shin},
  title = {Synthesis of Active-Mode Power-Gating Circuits},
  journal = {IEEE Transactions on Computer-Aided Design of Integrated Circuits
	and Systems},
  year = {2012},
  volume = {31},
  pages = {391-403},
  file = {:/import/var/jabref/files/2012-SeomunShin.pdf:PDF},
  issn = {0278-0070},
  owner = {udupi},
  timestamp = {2017.03.28}
}

@CONFERENCE{2003-SeshiaLahiri.etal,
  author = {Sanjit A. Seshia and Shuvendu K. Lahiri and Randal E. Bryant},
  title = {A Hybrid {SAT}-Based Decision Procedure for Separation Logic with
	Uninterpreted Functions},
  booktitle = {Proc. International Design Automation Conference},
  year = {2003},
  pages = { 425 - 430},
  file = {:./files/2003-SeshiaLahiri.etal.pdf:PDF},
  keywords = { {Boolean} variables; SAT-based decision procedure; atomic subformulas;
	bit-vectors; design verification; first-order logic; formal verification;
	quantifier-free fragment; separation logic; theorem proving; uninterpreted
	functions; distributed decision making; formal verification; integrated
	circuit design; logic design; symbol manipulation; theorem proving;},
  timestamp = {2006.09.19}
}

@INPROCEEDINGS{2007-SeshiaLi.etal,
  author = {S. A. Seshia and W. Li and S. Mitra},
  title = {Verification-Guided Soft Error Resilience},
  booktitle = {Design Automation and Test in Europe},
  year = {2007},
  pages = {1-6},
  month = {April},
  file = {2007-SeshiaLi.etal.pdf:files/2007-SeshiaLi.etal.pdf:PDF},
  issn = {1530-1591},
  owner = {bartsch},
  timestamp = {2016.09.12}
}

@INPROCEEDINGS{2008-ShafikRosinger.etal,
  author = {R. A. Shafik and P. Rosinger and B. M. Al-Hashimi},
  title = {{SystemC}-Based Minimum Intrusive Fault Injection Technique with
	Improved Fault Representation},
  booktitle = {2008 14th IEEE International On-Line Testing Symposium},
  year = {2008},
  issn = {1942-9398},
  owner = {udupi},
  timestamp = {2018.09.04}
}

@INPROCEEDINGS{2005-ShahSrivastava.etal,
  author = {Saumil Shah and Ashish Srivastava and Dushyant Sharma and Dennis
	Sylvester and David Blaauw and Vladimir Zolotov},
  title = {Discrete Vt Assignment and Gate Sizing Using a Self-Snapping Continuous
	Formulation},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2005},
  pages = { 705 - 712},
  file = {:./files/2005-ShahSrivastava.etal.pdf:PDF},
  keywords = { circuit nonlinear optimization; gate sizing; self-snapping continuous
	formulation; snapping heuristic; circuit optimisation; integrated
	circuit design;},
  timestamp = {2006.09.27}
}

@ARTICLE{1938-Shannon,
  author = {C. Shannon},
  title = {A Symbolic Analysis of Relay and Switching Circuits},
  journal = {American Institute of Electrical Engineers, Transactions of the},
  year = {1938},
  volume = {57},
  pages = {713 -723},
  number = {12},
  month = {dec.},
  file = {:./files/1938-Shannon.pdf:PDF}
}

@INPROCEEDINGS{2013-SharmaSloan.etal,
  author = {A. Sharma and J. Sloan and L.F. Wanner and S.H. Elmalaki and M.B.
	Srivastava and P. Gupta},
  title = {Towards analyzing and improving robustness of software applications
	to intermittent and permanent faults in hardware},
  booktitle = {International Conference on Computer Design},
  year = {2013},
  pages = {435 - 438},
  month = {October},
  file = {2013-SharmaSloan.etal.pdf:files/2013-SharmaSloan.etal.pdf:PDF},
  owner = {bartsch},
  timestamp = {2015.09.07}
}

@ARTICLE{1989-Shaw,
  author = {Alan Shaw},
  title = {Reasoning About TimeIn High Level Language Software},
  journal = {{IEEE} Transactions On Software Engineering},
  year = {1989},
  chapter = {16},
  file = {:./files/1989-Shaw.pdf:PDF},
  timestamp = {2006.09.22}
}

@ARTICLE{2010-ShazliTahoori,
  author = {S.Z. Shazli and M.B. Tahoori},
  title = {Using {B}oolean satisfiability for computing soft error rates in
	early design stages},
  journal = {Microelectronics Reliability},
  year = {2010},
  volume = {50},
  pages = {149 - 159},
  number = {1},
  doi = {https://doi.org/10.1016/j.microrel.2009.08.006},
  issn = {0026-2714},
  owner = {udupi},
  timestamp = {2018.09.02}
}

@INPROCEEDINGS{2000-SheeranSingh.etal,
  author = {M. Sheeran and S. Singh and G. Stalmarck},
  title = {Checking Safety Properties Using Induction And A {SAT}-Solver},
  booktitle = {Proc. International Conference on Formal Methods in Computer-Aided
	Design ({FMCAD})},
  year = {2000},
  file = {:./files/2000-SheeranSingh.etal.pdf:PDF},
  timestamp = {2006.09.19}
}

@INPROCEEDINGS{2005-SheiniSakallah,
  author = {H. M. Sheini and K. A. Sakallah},
  title = {Pueblo: A Modern Pseudo-{Boolean} {SAT} Solver},
  booktitle = {Proc. International Conference on Design, Automation and Test in
	Europe (DATE)},
  year = {2005},
  pages = { 684 - 685 Vol. 2},
  address = {Munich, Germany},
  month = {March},
  file = {:./files/2005-SheiniSakallah.pdf:PDF},
  keywords = { {Boolean} constraint propagation; integer programming; learning methods;
	literal watching strategy; logic-based reasoning; overhead minimization;
	pruning power; pseudo-{Boolean} SAT solver; pseudo-{Boolean} constraints;
	satisfiability solver; computability; constraint handling; inference
	mechanisms; integer programming; learning (artificial intelligence);
	minimisation;}
}

@ARTICLE{2007-ShekharPriyank.etal,
  author = {Namrata Shekhar and Priyank Kalla and Florian Enescu},
  title = {Equivalence Verification of Polynomial Datapaths Using Ideal Membership
	Testing},
  journal = {{IEEE} Transactions on Computer-Aided Design},
  year = {2007},
  volume = {26},
  pages = {1320-1330},
  number = {7},
  month = {July},
  file = {:./files/2007-ShekharPriyank.etal.pdf:PDF},
  owner = {wedler},
  timestamp = {2008.03.12}
}

@INPROCEEDINGS{2006-ShekharKalla.etal,
  author = {N. Shekhar and P. Kalla and F. Enescu},
  title = {Equivalence Verification of Arithmetic Datapath with Multiple Word-Length
	Operands},
  booktitle = {Proc. International Conference on Design, Automation and Test in
	Europe (DATE)},
  year = {2006},
  pages = {6 pp.},
  file = {:./files/2006-ShekharKalla.etal.pdf:PDF},
  keywords = {arithmetic computations;arithmetic datapaths;bit-vector arithmetic;commutative
	algebra;digital signal processing;equivalence verification;multiple
	word-length operands;number theory;polynomial function;register-transfer-level;digital
	arithmetic;equivalence classes;polynomials;signal processing;}
}

@INPROCEEDINGS{2005a-ShekharKalla.etal,
  author = {Shekhar, N. and Kalla, P. and Enescu, F. and Gopalakrishnan, S.},
  title = {Exploiting vanishing polynomials for equivalence verification of
	fixed-size arithmetic datapaths},
  booktitle = {Computer Design: VLSI in Computers and Processors, 2005. ICCD 2005.
	Proceedings. 2005 IEEE International Conference on},
  year = {2005},
  pages = {215-220},
  owner = {marx},
  timestamp = {2013.04.08}
}

@INPROCEEDINGS{2005-ShekharKalla.etal,
  author = {Namrata Shekhar and Priyank Kalla and Florian Enescu and Sivaram
	Gopalakrishnan},
  title = {Equivalence Verification Of Polynomial Datapaths With Fixed-Size
	Bit-Vectors Using Finite Ring Algebra},
  booktitle = {Proc. International Conference on Computer-Aided Design (ICCAD)},
  year = {2005},
  pages = { 291 - 296},
  file = {:./files/2005-ShekharKalla.etal.pdf:PDF},
  keywords = { RTL descriptions; canonical form modulo; coefficient matching; datapath-oriented
	designs; equivalence testing; equivalence verification; finite ring
	algebra; fixed-size bit-vectors; multivariate polynomials; polynomial
	algebra; polynomial computations; polynomial datapaths; digital arithmetic;
	equivalence classes; formal verification; integrated circuit design;
	logic design; polynomials;},
  timestamp = {2006.09.27}
}

@ARTICLE{2008-ShekharNamrata.etal,
  author = {Shekhar, Namrata and Kalla, Priyank and Meredith, M. Brandon and
	Enescu, Florian},
  title = {Simulation bounds for equivalence verification of polynomial datapaths
	using finite ring algebra},
  journal = {{IEEE} Trans. Very Large Scale Integr. Syst.},
  year = {2008},
  volume = {16},
  pages = {376--387},
  month = {April},
  file = {:./files/2008-ShekharNamrata.etal.pdf:PDF},
  issn = {1063-8210},
  issue = {4},
  numpages = {12},
  owner = {pavlenko},
  publisher = {IEEE Educational Activities Department},
  timestamp = {2010.11.03}
}

@ARTICLE{1999-ShenAbraham,
  author = {Jian Shen and Jacob A. Abraham},
  title = {An {RTL} Abstraction Technique for Processor MicroarchitectureValidation
	and Test Generation},
  journal = {Journal of Electronic Testing: Theory and Applications},
  year = {2000},
  volume = {16},
  pages = {67--81},
  number = {1-2},
  address = {Norwell, MA, USA},
  file = {:./files/1999-ShenAbraham.pdf:PDF},
  issn = {0923-8174},
  owner = {nguyen},
  publisher = {Kluwer Academic Publishers},
  timestamp = {2006.12.15}
}

@INPROCEEDINGS{2005-ShenQin.etal,
  author = {Shengyu Shen and Ying Qin and SiKun Li},
  title = {A fast counterexample minimization approach with refutation analysis
	and incremental {SAT}},
  booktitle = {Proc. Asia and South Pacific Design Automation Conference (ASPDAC)},
  year = {2005},
  pages = {451--454},
  address = {New York, NY, USA},
  publisher = {ACM},
  file = {:./files/2005-ShenQin.etal.pdf:PDF},
  isbn = {0-7803-8737-6},
  location = {Shanghai, China},
  owner = {nguyen},
  timestamp = {2007.12.14}
}

@INPROCEEDINGS{2002-ShimizuDill,
  author = {Kanna Shimizu and David L. Dill},
  title = {Deriving a Simulation Input Generator and a Coverage Metric From
	a Formal Specification},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {2002},
  pages = { 801 - 806},
  file = {:./files/2002-ShimizuDill.pdf:PDF},
  keywords = { RTL design verification; Stanford FLASH project; correctness checker;
	formal specification; functional coverage metric; functional interface
	specifications; large-scale I/O design; simulation environment; simulation
	input generator; binary decision diagrams; circuit CAD; circuit simulation;
	formal specification; formal verification; logic CAD;},
  timestamp = {2006.09.21}
}

@ARTICLE{2001-ShimizuDill.etal,
  author = {Kanna Shimizu and David L. Dill and Ching-Tsun Chou},
  title = {A Specification Methodology by a Collection of Compact Properties
	as Applied to the {Intel Itanium} Processor Bus Protocol},
  journal = {Lecture Notes in Computer Science},
  year = {2001},
  volume = {2144},
  pages = {340+},
  file = {:./files/2001-ShimizuDill.etal.pdf:PDF}
}

@INPROCEEDINGS{2000-ShimizuDill.etal,
  author = {K. Shimizu and L. Dill and A. J.Hu},
  title = {Monitor-Based Formal Specification of {PCI}},
  booktitle = {Proc. International Conference on Formal Methods in Computer-Aided
	Design ({FMCAD})},
  year = {2000},
  file = {:./files/2000-ShimizuDill.etal.pdf:PDF},
  timestamp = {2006.09.19}
}

@INPROCEEDINGS{2006-ShimizuGupta.etal,
  author = {Kanna Shimizu and Sanja Gupta and Tatsuya Koyama and Takashi Omizo
	and Jamee Abdulhafiz and McConville and Todd Swanson},
  title = {Verification of the Cell Broadband Engine (TM) Processor},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {2006},
  pages = {338 - 343},
  file = {:./files/2006-ShimizuGupta.etal.pdf:PDF},
  owner = {thalmaier},
  timestamp = {2006.11.29}
}

@ARTICLE{2010-ShinYoungsoo.etal,
  author = {Shin, Youngsoo and Seomun, Jun and Choi, Kyu-Myung and Sakurai, Takayasu},
  title = {Power Gating: Circuits, Design Methodologies, and Best Practice for
	Standard-cell {VLSI} Designs},
  journal = {ACM Trans. Des. Autom. Electron. Syst.},
  year = {2010},
  volume = {15},
  pages = {28:1--28:37},
  acmid = {1835421},
  address = {New York, NY, USA},
  articleno = {28},
  issn = {1084-4309},
  issue_date = {September 2010},
  numpages = {37},
  owner = {udupi},
  publisher = {ACM},
  timestamp = {2017.03.28}
}

@INPROCEEDINGS{2002-ShivakumarKistler.etal,
  author = {Premkishore Shivakumar and Michael Kistler and Stephen W. Keckler
	and Doug Burger and Lorenzo Alvisi},
  title = {Modeling the Effect of Technology Trends on the Soft Error Rate of
	Combinational Logic},
  booktitle = {Proc. International Conference on Dependable Systems and Networks},
  year = {2002},
  pages = { 389 - 398},
  file = {:./files/2002-ShivakumarKistler.etal.pdf:PDF},
  keywords = { 50 to 600 nm; CMOS memory circuits; SRAM cells; clock periods; combinational
	logic; computer system design; electrical masking; end-to-end model;
	high-energy neutrons; inverter delays; latching-window masking; logic
	circuits; microarchitectural trends; microprocessor style designs;
	soft error rate; technology scaling; technology trend effect modeling;
	unprotected memory elements; CMOS logic circuits; CMOS memory circuits;
	SRAM chips; combinational circuits; integrated circuit reliability;
	microprocessor chips; neutron effects;},
  timestamp = {2006.09.14}
}

@INPROCEEDINGS{2007-ShohamYahav.etal,
  author = {Shoham, Sharon and Yahav, Eran and Fink, Stephen and Pistoia, Marco},
  title = {Static Specification Mining Using Automata-based Abstractions},
  booktitle = {Proceedings of the 2007 International Symposium on Software Testing
	and Analysis},
  year = {2007},
  series = {ISSTA '07},
  pages = {174--184},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {1273487},
  doi = {10.1145/1273463.1273487},
  isbn = {978-1-59593-734-6},
  keywords = {abstract interpretation, specification mining, static analysis, typestate},
  location = {London, United Kingdom},
  numpages = {11},
  url = {http://doi.acm.org/10.1145/1273463.1273487}
}

@INPROCEEDINGS{2008-Shokrolah-ShiraziMiremadi,
  author = {M. Shokrolah-Shirazi and S. G. Miremadi},
  title = {FPGA-based Fault Injection into Synthesizable Verilog HDL Models},
  booktitle = {Proc. Second International Conference on Secure System Integration
	and Reliability Improvement},
  year = {2008},
  pages = {143 - 149},
  month = {July},
  file = {:files/2008-Shokrolah-ShiraziMiremadi.pdf:PDF},
  owner = {bartsch},
  timestamp = {2014.07.30}
}

@INPROCEEDINGS{2001-ShoumengXingshe,
  author = {Yan Shoumeng and Zhou Xingshe},
  title = {A Simulation Framework For Device Driver Development},
  year = {2001},
  file = {:./files/2001-ShoumengXingshe.pdf:PDF},
  timestamp = {2006.09.21}
}

@INBOOK{2001-Strichman,
  chapter = {Pruning Techniques for the {SAT-Based Bounded Model Checking} Problem},
  pages = {58--70},
  title = {Correct Hardware Design and Verification Methods: 11th IFIP WG 10.5
	Advanced Research Working Conference, CHARME 2001 Livingston, Scotland,
	UK, September 4--7, 2001 Proceedings},
  publisher = {Springer Berlin Heidelberg},
  year = {2001},
  editor = {Margaria, Tiziana and Melham, Tom},
  author = {Shtrichman, Ofer},
  address = {Berlin, Heidelberg},
  booktitle = {Correct Hardware Design and Verification Methods: 11th IFIP WG 10.5
	Advanced Research Working Conference, CHARME 2001 Livingston, Scotland,
	UK, September 4--7, 2001 Proceedings},
  isbn = {978-3-540-44798-6},
  owner = {villarraga},
  timestamp = {2016.07.27}
}

@MISC{2002-Strichman,
  author = {Shtrichman, Ofer},
  title = {Sharing information between instances of a propositional satisfiability
	{(SAT)} problem},
  month = sep # {~5},
  year = {2002},
  note = {US Patent App. 09/990,390}
}

@ARTICLE{2000-Shtrichman,
  author = {Ofer Shtrichman},
  title = {Tuning Sat Checkers For Bounded Model Checking},
  journal = {Lecture Notes In Computer Science},
  year = {2000},
  volume = {1855},
  pages = {480 - 494},
  booktitle = {Proceedings of the 12th International Conference on Computer Aided
	Verification},
  file = {:./files/2000-Shtrichman.pdf:PDF},
  timestamp = {2006.09.19}
}

@OTHER{2014-Siegel,
  author = {Jon M. Siegel},
  month = {june},
  title = {Model Driven Architecture \textsuperscript{\textregistered} (MDA):
	The MDA Guide Rev 2.0 },
  url = {https://www.omg.org/mda/presentations.htm},
  year = {2014}
}

@INPROCEEDINGS{2003-SifakisTripakis.etal,
  author = {J. Sifakis and S. Tripakis and S. Yovine},
  title = {Building models of real-time systems from application software},
  booktitle = {Proc. {IEEE} Special Issue on Modeling and Design of Embedded Software},
  year = {2003},
  pages = {100--111},
  file = {:./files/2003-SifakisTripakis.etal.pdf:PDF},
  owner = {nguyen},
  timestamp = {2006.08.29},
  url = {http://citeseer.ist.psu.edu/sifakis03building.html}
}

@INPROCEEDINGS{1999-SilvaGlass,
  author = {Joao Marques Silva and Thomas Glass},
  title = {Combinational Equivalence Checking using {SAT} and Recursive Learning},
  booktitle = {Proc. International Conference on Design, Automation and Test in
	Europe ({DATE})},
  year = {1999},
  pages = {145 -149},
  file = {:./files/1999-SilvaGlass.pdf:PDF},
  keywords = {{Boolean} satisfiability algorithms;SAT algorithm;combinational circuits;combinational
	equivalence checking;complexity;digital circuits;logic circuits;recursive
	learning;verification;circuit complexity;combinational circuits;computability;learning
	(artificial intelligence);recursive functions;},
  timestamp = {2006.09.13}
}

@INPROCEEDINGS{2005-SinghMani.etal,
  author = {Ashish Kumar Singh and Murari Mani and Michael Orshansky},
  title = {Statistical Technology Mapping for Parametric Yield},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2005},
  pages = { 511 - 518},
  file = {:./files/2005-SinghMani.etal.pdf:PDF},
  keywords = { decision-making; leakage power constraint; library binding; logic
	synthesis; parametric yield; statistical technology mapping; threshold
	voltage; varying transistor channel length; integrated circuit design;
	integrated circuit yield; logic design; statistical analysis; timing;},
  timestamp = {2006.09.27}
}

@ARTICLE{2018-SinghLin.etal,
  author = {Singh, Eshan and Lin, David and Barrett, Clark and Mitra, Subhasish},
  title = {Logic bug detection and localization using symbolic quick error detection},
  journal = {IEEE Transactions on Computer-Aided Design of Integrated Circuits
	and Systems},
  year = {2018},
  owner = {fadiheh},
  publisher = {IEEE},
  timestamp = {2019.08.23}
}

@INPROCEEDINGS{2005-SinghalBozorgzadeh,
  author = {Love Singhal and Elaheh Bozorgzadeh},
  title = {Fast Timing Closure by Interconnect Criticality Driven Delay Relaxation},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2005},
  pages = { 792 - 797},
  file = {:./files/2005-SinghalBozorgzadeh.pdf:PDF},
  keywords = { MediaBench data paths; Xilinx Place; Xilinx VirtexE FPGA devices;
	clock frequency; critical edge minimization; critical edge reduction
	algorithm; deep sub-micron designs; delay relaxation; design flow;
	interconnect criticality; interconnect delay; maximum budgeting;
	retiming; timing closure; total pipelining; transistor sizes; wire
	pipelining; delays; field programmable gate arrays; integrated circuit
	design; integrated circuit interconnections; timing;},
  timestamp = {2006.09.27}
}

@INPROCEEDINGS{2006-SinzBiere,
  author = {Carsten Sinz and Armin Biere},
  title = {Extended resolution proofs for conjoining {BDD}s},
  booktitle = {In: Proc. of the 1st Intl. Computer Science Symp. in Russia (CSR
	2006). LNCS 3967},
  year = {2006},
  pages = {600--611},
  publisher = {Springer},
  file = {:./files/2006-SinzBiere.pdf:PDF},
  owner = {pavlenko},
  timestamp = {2011.03.04}
}

@INPROCEEDINGS{2010-SinzFalke,
  author = {Carsten Sinz and Stephan Falke and Florian Merz},
  title = {A Precise Memory Model for Low-Level Bounded Model Checking},
  booktitle = {Proceedings of the 5th International Workshop on Systems Software
	Verification (SSV '10)\normalfont{, Vancouver, Canada}},
  year = {2010},
  owner = {villarraga},
  timestamp = {2013.05.11}
}

@INCOLLECTION{2012-SinzMerz.etal,
  author = {Sinz, Carsten and Merz, Florian and Falke, Stephan},
  title = {LLBMC: A Bounded Model Checker for LLVM?s Intermediate Representation},
  booktitle = {Tools and Algorithms for the Construction and Analysis of Systems},
  publisher = {Springer Berlin Heidelberg},
  year = {2012},
  editor = {Flanagan, Cormac and K�nig, Barbara},
  volume = {7214},
  series = {Lecture Notes in Computer Science},
  pages = {542-544},
  isbn = {978-3-642-28755-8},
  owner = {villarraga},
  timestamp = {2013.05.11}
}

@INPROCEEDINGS{1998-SmithMicheli,
  author = {James Smith and Giovanni De Micheli},
  title = {Automated Composition of Hardware Components},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {1998},
  pages = {14 -19},
  file = {:./files/1998-SmithMicheli.pdf:PDF},
  keywords = {POLARIS hardware composition;design reuse;hardware subsystems;interfaces;system
	components;computer interfaces;high level synthesis;},
  timestamp = {2006.09.19}
}

@MISC{web_smtcomp_2009,
  author = {{SMT-COMP 2009}},
  year = {2009},
  owner = {stoffel},
  timestamp = {2016.05.10},
  url = {http://www.smtcomp.org/2009/}
}

@MISC{web_smtcomp_2010,
  author = {{SMT-COMP 2010}},
  year = {2010},
  owner = {pavlenko},
  timestamp = {2010.07.27},
  url = {http://www.smtcomp.org/2010/}
}

@MANUAL{0000-Somenzi,
  title = {{CUDD}: {CU} Decision Diagram Package},
  author = {Fabio Somenzi},
  owner = {nguyen},
  timestamp = {2007.05.09},
  url = {http://vlsi.colorado.edu/\url{~}fabio/CUDD/}
}

@INPROCEEDINGS{2000-SomenziBloem,
  author = {Fabio Somenzi and Roderick Bloem},
  title = {Efficient Buchi Automata from {LTL} Formulae},
  booktitle = {Computer Aided Verification},
  year = {2000},
  pages = {248-263},
  file = {:./files/2000-SomenziBloem.pdf:PDF},
  url = {http://citeseer.ist.psu.edu/article/somenzi00efficient.html}
}

@MISC{web_spear,
  author = {Spear},
  owner = {stoffel},
  timestamp = {2008.07.01},
  url = {http://www.domagoj-babic.com}
}

@BOOK{2008-Spear,
  title = {{SystemVerilog} for Verification: A Guide to Learning the Testbench
	Language Features},
  publisher = {Springer},
  year = {2008},
  author = {Chris Spear},
  file = {:./files/2008-Spear.pdf:PDF},
  owner = {wedler},
  timestamp = {2009.09.03}
}

@INPROCEEDINGS{2000-StangierHoltmann.etal,
  author = {Christian Stangier and Ulrich Holtmann and Christoph Meinel},
  title = {Optimizing Partitioning of Transition Relations by Using High-Level
	Information},
  booktitle = {Proceedings of the International Workshop on Logic Synthesis},
  year = {2000},
  file = {:./files/2000-StangierHoltmann.etal.pdf:PDF},
  timestamp = {2006.09.13}
}

@INPROCEEDINGS{1999-Stanion,
  author = {Ted Stanion},
  title = {Implicit Verification of Structurally Dissimilar Arithmetic Circuits},
  booktitle = {Proc. International Conference on Computer Design ({ICCD}-99)},
  year = {1999},
  pages = {46-50},
  month = {October},
  file = {:./files/1999-Stanion.pdf:PDF}
}

@ARTICLE{2018-StecklinaPrescher,
  author = {Stecklina, Julian and Prescher, Thomas},
  title = {{LazyFP}: Leaking {FPU} Register State using Microarchitectural Side-Channels},
  journal = {arXiv preprint arXiv:1806.07480},
  year = {2018},
  owner = {fadiheh},
  timestamp = {2018.08.08}
}

@INPROCEEDINGS{2004-SteinerRushby.etal,
  author = {W. Steiner and J. Rushby and M. Sorea and H. Pfeifer},
  title = {Model checking a fault-tolerant startup algorithm: from design exploration
	to exhaustive fault simulation},
  booktitle = {International Conference on Dependable Systems and Networks},
  year = {2004},
  pages = {189-198},
  month = {June},
  file = {2004-SteinerRushby.etal.pdf:files/2004-SteinerRushby.etal.pdf:PDF},
  owner = {bartsch},
  timestamp = {2015.08.03}
}

@INPROCEEDINGS{2003-SteiningerRahbaran.etal,
  author = {A. Steininger and B. Rahbaran and T. Handl},
  title = {Built-in Fault Injectors - The Logical Continuation of BIST?},
  booktitle = {Proc. Intelligent Solutions in Embedded Systems workshop},
  year = {2003},
  file = {:files/2003-SteiningerRahbaran.etal.pdf:PDF},
  owner = {bartsch},
  timestamp = {2014.07.30}
}

@INPROCEEDINGS{1997-Stewart,
  author = {David B. Stewart},
  title = {An {I/O} Device Driver Model and Framework for Embedded Systems},
  year = {1997},
  file = {:./files/1997-Stewart.pdf:PDF},
  timestamp = {2006.10.04}
}

@ARTICLE{1999-StewartJacob,
  author = {David B. Stewart and Bruce L. Jacob},
  title = {Hardware/Software Co-Design of {I/O} Interfacing Hardware and Real-Time
	Device Drivers for Embedded Systems},
  journal = {{IEEE} Real-Time Applications Symposium},
  year = {1999},
  file = {:./files/1999-StewartJacob.pdf:PDF},
  timestamp = {2006.10.04}
}

@PHDTHESIS{1999-Stoffel,
  author = {D. Stoffel},
  title = {Formal Verification of Sequential Circuits Using Reasoning Techniques},
  school = {Johann Wolfgang Goethe - Universit\"at Frankfurt am Main},
  year = {1999},
  type = {Dissertation},
  file = {:./files/1999-Stoffel.pdf:PDF}
}

@ARTICLE{2004a-StoffelKunz,
  author = {Stoffel, D. and Kunz, W.},
  title = {Equivalence Checking of Arithmetic Circuits on the Arithmetic Bit
	Level},
  journal = {Computer-Aided Design of Integrated Circuits and Systems, IEEE Transactions
	on},
  year = {2004},
  volume = {23},
  pages = {586 - 597},
  number = {5},
  month = {may},
  file = {:./files/2004a-StoffelKunz.pdf:PDF},
  issn = {0278-0070},
  keywords = { {Boolean} mapping algorithm; addition circuit; arithmetic bit level;
	arithmetic circuits; bit-level reverse-engineering; datapath verification;
	equivalence checking; formal hardware verification; gate netlist;
	half adders; multiplier; adders; digital arithmetic; formal verification;
	multiplying circuits; reverse engineering;}
}

@INPROCEEDINGS{2001-StoffelKunz,
  author = {D. Stoffel and W. Kunz},
  title = {Verification of Integer Multipliers on the Arithmetic Bit Level},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2001},
  pages = {183-189},
  address = {San Jose, CA},
  month = {November},
  file = {:./files/2001-StoffelKunz.pdf:PDF}
}

@INPROCEEDINGS{2000-StoffelKunz,
  author = {D. Stoffel and W. Kunz},
  title = {Convergence Behaviour of Structural {FSM} Traversal},
  booktitle = {Proc. of the 3rd Conference on Computer-Aided Technologies in Applied
	Discrete Mathematics (ICADM)},
  year = {2000},
  pages = {176-183},
  address = {Tomsk, Russia},
  file = {:./files/2000-StoffelKunz.pdf:PDF}
}

@INPROCEEDINGS{1997a-StoffelKunz,
  author = {D. Stoffel and W. Kunz},
  title = {{AND/OR} Reasoning Graphs for Determining Prime Implicants in Multi-level
	Combinational Networks},
  booktitle = {Proc. Asia and South Pacific Design Automation Conference ({ASPDAC})},
  year = {1997},
  pages = {529-538},
  month = {January},
  file = {:./files/1997a-StoffelKunz.pdf:PDF}
}

@INPROCEEDINGS{1997-StoffelKunz,
  author = {D. Stoffel and W. Kunz},
  title = {Record \& Play A Structural Fixed Point Iteration for Sequential
	Circuit Verification},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {1997},
  pages = {394-399},
  month = {November},
  file = {:./files/1997-StoffelKunz.pdf:PDF}
}

@INPROCEEDINGS{1996-StoffelKunz,
  author = {D. Stoffel and W. Kunz},
  title = {Logic Equivalence Checking by Optimization Techniques},
  booktitle = {Proc. International Workshop on Computer-Aided Design, Test, and
	Evaluation for Dependability},
  year = {1996},
  pages = {85-90},
  address = {Peking, China},
  month = {July}
}

@ARTICLE{2004-StoffelWedler.etal,
  author = {D. Stoffel and M. Wedler and P. Warkentin and W. Kunz},
  title = {Structural {FSM}-Traversal},
  journal = {{IEEE} Transactions on Computer-Aided Design},
  year = {2004},
  volume = {23},
  pages = {598-619},
  number = {5},
  month = {May},
  file = {:./files/2004-StoffelWedler.etal.pdf:PDF}
}

@MISC{web_stp,
  author = {STP},
  owner = {pavlenko},
  timestamp = {2010.11.03},
  url = {http://sites.google.com/site/stpfastprover/STP-Fast-Prover}
}

@BOOK{2002-Stroud,
  title = {A Designer’s Guide to Built-In Self-Test},
  publisher = {Springer},
  year = {2002},
  author = {Charles E. Stroud},
  owner = {bartsch},
  timestamp = {2016.09.21}
}

@BOOK{2000-Stroustrup,
  title = {Die C++ Programmiersprache},
  publisher = {Addison-Wesley},
  year = {2000},
  author = {Bjarne Stroustrup},
  edition = {4., aktualisierte Auflage, Deutsche Ausgabe der Special Edition},
  owner = {bschmidt},
  timestamp = {2014.07.08}
}

@INPROCEEDINGS{2014-SubramanyanArora,
  author = {Subramanyan, Pramod and Arora, Divya},
  title = {Formal verification of taint-propagation security properties in a
	commercial {SoC} design},
  booktitle = {Design, Automation \& Test in Europe Conference (DATE)},
  year = {2014},
  pages = {313},
  organization = {IEEE},
  owner = {fadiheh},
  timestamp = {2018.07.12}
}

@INPROCEEDINGS{2016-SubramanyanMalik.etal,
  author = {Subramanyan, Pramod and Malik, Sharad and Khattri, Hareesh and Maiti,
	Abhranil and Fung, Jason},
  title = {Verifying information flow properties of firmware using symbolic
	execution},
  booktitle = {Design, Automation \& Test in Europe Conference (DATE)},
  year = {2016},
  pages = {337--342},
  organization = {IEEE},
  owner = {fadiheh},
  timestamp = {2018.07.12}
}

@INPROCEEDINGS{2004-SuhLee.etal,
  author = {Suh, G Edward and Lee, Jae W and Zhang, David and Devadas, Srinivas},
  title = {Secure program execution via dynamic information flow tracking},
  booktitle = {ACM Sigplan Notices},
  year = {2004},
  volume = {39},
  number = {11},
  pages = {85--96},
  organization = {ACM},
  owner = {fadiheh},
  timestamp = {2018.07.12}
}

@MASTERSTHESIS{1999-Sulimma,
  author = {Kolja Sulimma},
  title = {Berechnung von Implikationen in Booleschen Netzen mit {FPGA}s},
  school = {Dept. of Computer Science, University of Frankfurt, Germany},
  year = {1999},
  file = {:./files/1999-Sulimma.pdf:PDF}
}

@INPROCEEDINGS{1999-SulimmaStoffel.etal,
  author = {K. Sulimma and D. Stoffel and W. Kunz},
  title = {Accelerating {Boolean} Implications with {FPGA}s},
  booktitle = {Proc. International Workshop on Field-Programmable Logic and Applications},
  year = {1999},
  editor = {Patrick Lysaght and James Irvine and Reiner Hartenstein},
  volume = {1673},
  series = {Lecture Notes in Computer Science},
  pages = {532-537},
  address = {Glasgow, UK},
  month = {August},
  publisher = {Springer-Verlag},
  file = {:./files/1999-SulimmaStoffel.etal.pdf:PDF}
}

@INPROCEEDINGS{1998-SuriSinha,
  author = {Neeraj Suri and Purnendu Sinha},
  title = {On the use of Formal Techniques for Validation},
  booktitle = {Proc. Annual International Symposium on Fault-Tolerant Computing},
  year = {1998},
  pages = {390 -399},
  file = {:./files/1998-SuriSinha.pdf:PDF},
  keywords = {dependable protocols;fault injection based validation;formal techniques;formal
	verification procedures;graph structures;validation;formal verification;transport
	protocols;},
  timestamp = {2006.09.14}
}

@ARTICLE{2005-Sutter,
  author = {Sutter, Herb},
  title = {{The Free Lunch Is Over: A Fundamental Turn Toward Concurrency in
	Software}},
  journal = {Dr. Dobb's Journal},
  year = {2005},
  volume = {30},
  number = {3},
  citeulike-article-id = {970541},
  keywords = {bibtex-import},
  owner = {stoffel},
  posted-at = {2006-12-01 16:12:35},
  timestamp = {2016.05.10}
}

@INPROCEEDINGS{2006-Swan,
  author = {S. {Swan}},
  title = {SystemC transaction level models and RTL verification},
  booktitle = {2006 43rd ACM/IEEE Design Automation Conference},
  year = {2006},
  pages = {90-92},
  month = {July},
  doi = {10.1145/1146909.1146937},
  issn = {0738-100X},
  keywords = {hardware description languages;hardware-software codesign;integrated
	circuit design;system-on-chip;SystemC;transaction level models;register
	transfer level verification;system-on-chip;Hardware design languages;Integrated
	circuit modeling;System-on-a-chip;Embedded software;Software standards;Permission;Software
	systems;Circuit simulation;Standardization;Wires;Standardization;Languages;Verification;SystemC;Transaction
	Level Model;TLM;RTL Verification;Hardware/Software Co-Design;Hardware/Software
	Co-Verification},
  owner = {fehmel},
  timestamp = {2019.05.29}
}

@MANUAL{2011-PowerCompiler,
  title = {Power Compiler User Guide},
  author = {Synopsys},
  file = {:/import/var/jabref/files/2011-PowerCompiler.pdf:PDF;:files/2011-PowerCompiler.pdf:PDF},
  owner = {udupi},
  timestamp = {2016.04.25}
}

@MISC{2013-Synopsys,
  author = {{Synopsys Inc.}},
  title = {{TetraMAX} {ATPG} User Guide},
  year = {2013},
  owner = {villarraga},
  timestamp = {2016.08.19}
}

@MISC{2010-Synopsys,
  author = {{Synopsys Inc.}},
  title = {{Design Compiler} User Guide},
  year = {2010},
  owner = {villarraga},
  timestamp = {2016.08.19}
}

@MISC{0000-Berkeley,
  author = {Berkeley Logic Synthesis and Verification Group},
  title = {A System for Sequential Synthesis and Verification},
  owner = {thalmaier},
  timestamp = {2010.03.12},
  url = {http://www.eecs.berkeley.edu/~alanmi/abc/}
}

@ARTICLE{2009-SystemVerilog,
  author = {{SystemVerilog Language Working Group}},
  title = {{IEEE} Standard for System Verilog -- Unified Hardware Design, Specification,
	and Verification Language},
  journal = {{IEEE} Std. 1800-2009},
  year = {2009},
  file = {2009-SystemVerilog.pdf:files/2009-SystemVerilog.pdf:PDF},
  keywords = {IEEE standard;SystemVerilog-unified hardware design;Verilog language;hardware
	description language;programming language interface;specification
	language;verification language;hardware description languages;},
  owner = {villarraga},
  timestamp = {2012.08.30},
  url = {http://www.systemverilog.org/}
}

@INPROCEEDINGS{1999-FederHell.etal,
  author = {T.Feder and P.Hell and S.Klein and R.Motwani},
  title = {Complexity Of Graph Partition Proplems},
  booktitle = {Proc. Annual ACM Symposium on Theory of Computing},
  year = {1999},
  pages = {464--472},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {301373},
  file = {:./files/1999-FederHell.etal.pdf:PDF},
  isbn = {1-58113-067-8},
  location = {Atlanta, Georgia, United States},
  numpages = {9},
  timestamp = {2006.09.18}
}

@ARTICLE{2002a-HenzingerJhala.etal,
  author = {T.Henzinger and R.Jhala and R.Majumadar},
  title = {Temporal Safety Proofs For Systems Code},
  journal = {Lecture Notes In Computer Science},
  year = {2002},
  volume = {2404},
  pages = {526 - 538},
  file = {:./files/2002a-HenzingerJhala.etal.pdf:PDF},
  timestamp = {2006.09.21}
}

@INPROCEEDINGS{2006-VogtWehn,
  author = {T.Vogt and N.Wehn},
  title = {A Reconfigurable Application Specific Instruction Set Processor for
	Viterbi and Log-{MAP} Decoding},
  booktitle = {Proc. {IEEE} Workshop on Signal Processing ({SIPS}'06)},
  year = {2006},
  pages = {142--147},
  address = {Banff, Canada},
  month = {October},
  file = {:./files/2006-VogtWehn.pdf:PDF},
  owner = {vogt},
  timestamp = {2006.12.01}
}

@ARTICLE{2014-TabacaruChaari.etal,
  author = {Tabacaru, Bogdan-Andrei and Chaari, Moomen and Ecker, Wolfgang and
	Kruse, Thomas},
  title = {A meta-modeling-based approach for automatic generation of fault-injection
	processes},
  journal = {DVCon Europe},
  year = {2014},
  pages = {1--7},
  file = {2014-TabacaruChaari.etal.pdf:files/2014-TabacaruChaari.etal.pdf:PDF},
  keywords = {fault injection; system-level verification; system-on-chip; SystemC},
  owner = {stoffel},
  timestamp = {2016.08.15}
}

@INPROCEEDINGS{2010-TabakovVardi,
  author = {Tabakov, Deian and Vardi, Moshe Y.},
  title = {Monitoring temporal {SystemC} properties},
  booktitle = {IEEE/ACM Intl. Conf. on Formal Methods and Models for Codesign (MEMOCODE),},
  year = {2010},
  pages = {123 -132},
  month = {July},
  owner = {joakim},
  timestamp = {2012.12.17}
}

@INPROCEEDINGS{2008-TabakovVardi.etal,
  author = {Tabakov, Deian and Vardi, Moshe Y. and Kamhi, Gila and Singerman,
	Eli},
  title = {A temporal language for {SystemC}},
  booktitle = {Proceedings of the 2008 International Conference on Formal Methods
	in Computer-Aided Design},
  year = {2008},
  series = {FMCAD '08},
  pages = {22:1--22:9},
  address = {Piscataway, NJ, USA},
  publisher = {IEEE Press},
  articleno = {22},
  file = {:files/2008-TabakovVardi.etal.pdf:PDF},
  isbn = {978-1-4244-2735-2},
  location = {Portland, Oregon},
  numpages = {9},
  owner = {joakim},
  timestamp = {2012.12.17}
}

@INPROCEEDINGS{1997-TafertshoferGanz.etal,
  author = {P. Tafertshofer and A. Ganz and M. Henftling},
  title = {A {SAT}-Based Implication Engine for Efficient {ATPG}, Equivalence
	Checking, and Optimization of Netlists},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {1997},
  pages = {648-655},
  month = {November},
  file = {:./files/1997-TafertshoferGanz.etal.pdf:PDF}
}

@ARTICLE{2005-TalpinGuernic.etal,
  author = {Jean-Pierre Talpin and Paul Le Guernic and Sandeep Kumar Shukla and
	Rajesh Gupta},
  title = {A Compositional Behavioral Modeling Framework for Embedded System
	Design and Conformance Checking},
  journal = {International Journal of Parallel Programming},
  year = {2005},
  volume = {33},
  file = {:./files/2005-TalpinGuernic.etal.pdf:PDF},
  timestamp = {2006.10.04}
}

@ARTICLE{2001-TasiranKeutzer,
  author = {Serdar Tasiran and Kurt Keutzer},
  title = {Coverage Metrics for Functional Validation of Hardware Designs},
  journal = {{IEEE} Design and Test of Computers},
  year = {2001},
  volume = {18},
  pages = {36 -45},
  number = {4},
  month = {jul/aug},
  file = {:./files/2001-TasiranKeutzer.pdf:PDF},
  keywords = { coverage metrics; functional validation; hardware designs; simulation
	resources; formal verification; logic CAD; logic simulation; logic
	testing;},
  owner = {nguyen},
  timestamp = {2006.12.15}
}

@MISC{2013-ubm,
  author = {UBM Tech},
  title = {2013 Embedded Market Study},
  year = {2013},
  file = {:import/var/jabref/files/2013-ubm.pdf:PDF},
  owner = {bschmidt},
  timestamp = {2014.07.02},
  url = {http://e.ubmelectronics.com/2013EmbeddedStudy/index.html}
}

@ARTICLE{2012-Teich,
  author = {J. Teich},
  title = {Hardware/Software Codesign: The Past, the Present, and Predicting
	the Future},
  journal = {Proceedings of the IEEE},
  year = {2012},
  volume = {100},
  pages = {1411-1430},
  number = {Special Centennial Issue},
  month = {May},
  doi = {10.1109/JPROC.2011.2182009},
  issn = {0018-9219},
  keywords = {electronic design automation;embedded systems;hardware-software codesign;virtual
	prototyping;hardware-software codesign;concurrent design;hardware
	components;software components;complex electronic systems;design
	constraints;time-to-market frame;Hardware design languages;Software
	development;Consumer electronics;System-on-a-chip;Computer architecture;Complexity
	theory;Simulation;Cosimulation;cosynthesis;coverification;design
	space exploration;electronic system level (ESL);hardware/software
	codesign;virtual prototyping}
}

@MISC{web_tensilica,
  author = {Tensilica},
  owner = {stoffel},
  timestamp = {2016.05.11},
  url = {http://www.tensilica.com}
}

@INPROCEEDINGS{2010-ThalmaierNguyen.etal,
  author = {M. Thalmaier and M. Nguyen and M. Wedler and D. Stoffel and J. Bormann
	and W. Kunz},
  title = {Analyzing k-Step Induction to Compute Invariants for {SAT}-Based
	Property Checking},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {2010},
  pages = {176 -181},
  file = {:./files/2010-ThalmaierNguyen.etal.pdf:PDF},
  owner = {W},
  timestamp = {2010.10.01}
}

@CONFERENCE{2007-ThalmaierNguyen.etal,
  author = {Max Thalmaier and Minh D. Nguyen and Markus Wedler and Dominik Stoffel
	and Wolfgang Kunz},
  title = {{Formale Verifikation von {SoC} Protokollimplementierungen}},
  booktitle = {Tagungsband 1.{GMM}/{GI}/{ITG-Fachtagung} Zuverl\"{a}ssigkeit und
	Entwurf},
  year = {2007},
  owner = {nguyen},
  timestamp = {2008.04.20}
}

@INBOOK{1997-TheeuwenSeelen,
  pages = {389--399},
  title = {Power Reduction Through Clock Gating by Symbolic Manipulation},
  publisher = {Springer US},
  year = {1997},
  editor = {Reis, Ricardo and Claesen, Luc},
  author = {Theeuwen, Frans and Seelen, Eric},
  address = {Boston, MA},
  booktitle = {VLSI: Integrated Systems on Silicon: IFIP TC10 WG10.5 International
	Conference on Very Large Scale Integration 26--30 August 1997, Gramado,
	RS, Brazil},
  doi = {10.1007/978-0-387-35311-1_32},
  file = {:/import/var/jabref/files/1997-TheeuwenSeelen.pdf:PDF},
  owner = {udupi},
  timestamp = {2018.04.10},
  url = {https://doi.org/10.1007/978-0-387-35311-1_32}
}

@INPROCEEDINGS{2001-Theiling,
  author = {Henrik Theiling},
  title = {Generating Decision Trees for Decoding Binaries},
  booktitle = {Proc. {ACM} {SIGPLAN} Workshop on Languages, Compilers and Tools
	for Embedded Systems},
  year = {2001},
  pages = {112--120},
  file = {:./files/2001-Theiling.pdf:PDF},
  timestamp = {2006.09.22}
}

@INPROCEEDINGS{2000-Theiling,
  author = {Henrick Theiling},
  title = {Extracting Safe and Precise Control Flow from Binaries},
  booktitle = {Proc. International Conference on Real-Time Systems and Applications
	(RTCSA)},
  year = {2000},
  pages = {23 -30},
  file = {:./files/2000-Theiling.pdf:PDF},
  keywords = {binary executables;block boundaries;bottom-up approach;branch targets;control
	flow graph;entry points;graph approximation;instruction blocks;instruction
	routines;instruction sequence clustering;safe precise control flow
	extraction;safety-critical real-time systems;static program analysis;uncertainties;flow
	graphs;program control structures;program diagnostics;real-time systems;safety-critical
	software;sequences;},
  timestamp = {2006.09.22}
}

@MISC{web_polyspace,
  author = {{{The MathWorks, Inc.} {USA}}},
  title = {{Polyspace - Static Analysis Tools}},
  howpublished = {http://www.mathworks.com/products/polyspace/},
  key = {Polyspace},
  owner = {villarraga},
  timestamp = {2014.04.15},
  url = {http://www.mathworks.com/products/polyspace/}
}

@PHDTHESIS{2004-Thesing,
  author = {Stephan Thesing},
  title = {Safe and Precise {WCET} Determination by Abstract Interpretation
	of Pipeline Models},
  year = {2004},
  file = {:./files/2004-Thesing.pdf:PDF},
  timestamp = {2006.09.22}
}

@MISC{web-sir,
  author = {{The SIR Project}},
  title = {Software-Artifact Infrastructure Repository},
  howpublished = {http://sir.unl.edu},
  note = {Accessed: 2015-09-01},
  owner = {bartsch},
  timestamp = {2015.09.26}
}

@PHDTHESIS{1995-Thienel,
  author = {Stefan Thienel},
  title = {{ABACUS} - A Branch-and-Cut System},
  school = {Institut fuer Informatik, Universitaet zu Koeln},
  year = {1995},
  type = {Dissertation}
}

@ARTICLE{2002-Timpe,
  author = {Christian Timpe},
  title = {Solving Planning and Scheduling Problems with Combined Integer and
	Constraint Programming},
  journal = {{OR} Spectrum},
  year = {2002},
  volume = {24},
  pages = {431-448},
  number = {4},
  month = {November},
  file = {:./files/2002-Timpe.pdf:PDF}
}

@INPROCEEDINGS{2011-TiwariOberg.etal,
  author = {Tiwari, Mohit and Oberg, Jason K and Li, Xun and Valamehr, Jonathan
	and Levin, Timothy and Hardekopf, Ben and Kastner, Ryan and Chong,
	Frederic T and Sherwood, Timothy},
  title = {Crafting a usable microkernel, processor, and I/O system with strict
	and provable information flow security},
  booktitle = {ACM SIGARCH Computer Architecture News},
  year = {2011},
  volume = {39},
  number = {3},
  pages = {189--200},
  organization = {ACM},
  owner = {fadiheh},
  timestamp = {2018.11.28}
}

@INPROCEEDINGS{2009-TiwariWassel.etal,
  author = {Tiwari, Mohit and Wassel, Hassan MG and Mazloom, Bita and Mysore,
	Shashidhar and Chong, Frederic T and Sherwood, Timothy},
  title = {Complete information flow tracking from the gates up},
  booktitle = {ACM Sigplan Notices},
  year = {2009},
  volume = {44},
  number = {3},
  pages = {109--120},
  organization = {ACM},
  owner = {fadiheh},
  timestamp = {2018.07.12}
}

@INPROCEEDINGS{1995-TiwariMalik,
  author = {Tiwari, Vivek and Malik, Sharad and Ashar, Pranav},
  title = {Guarded Evaluation: Pushing Power Management to Logic Synthesis/Design},
  booktitle = {Proceedings of the 1995 International Symposium on Low Power Design},
  year = {1995},
  series = {ISLPED '95},
  pages = {221--226},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {224120},
  isbn = {0-89791-744-8},
  location = {Dana Point, California, USA},
  numpages = {6},
  owner = {udupi},
  timestamp = {2015.11.19}
}

@PHDTHESIS{1999-Torre,
  author = {Salvatore La Torre},
  title = {Advances in Finite Automata and Temporal Logic for System Verification},
  year = {1999},
  file = {:./files/1999-Torre.pdf:PDF},
  timestamp = {2006.09.21}
}

@INPROCEEDINGS{1990-TouatiSavoj.etal,
  author = {Herve J. Touati and Hamid Savoj and Bill Lin and Robert K. Brayton},
  title = {Implicit State Enumeration of Finite State Machines using {BDD}s},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {1990},
  pages = {130-133},
  file = {:./files/1990-TouatiSavoj.etal.pdf:PDF}
}

@INPROCEEDINGS{1997-ToubaMcCluskey,
  author = {Nur A. Touba and Edward J. McCluskey},
  title = {Logic Synthesis of Multilevel Circuits with Concurrent Error Detection},
  booktitle = {Proc. International Conference on Computer-Aided Design},
  year = {1997},
  volume = {16},
  number = {7},
  pages = {783 -789},
  month = {jul},
  file = {:./files/1997-ToubaMcCluskey.pdf:PDF},
  keywords = {Stanford CRCs TOPS synthesis system;concurrent error detection;logic
	synthesis;multilevel circuits;parity-check code;path fault secure;self-checking
	circuit;single stuck-at faults;structure-constrained logic optimization;circuit
	CAD;circuit optimisation;error detection;integrated circuit testing;integrated
	logic circuits;logic CAD;logic testing;multivalued logic circuits;},
  timestamp = {2006.09.14}
}

@ARTICLE{2018-TrippelLustig.etal,
  author = {Trippel, Caroline and Lustig, Daniel and Martonosi, Margaret},
  title = {{MeltdownPrime} and {SpectrePrime}: Automatically-Synthesized Attacks
	Exploiting Invalidation-Based Coherence Protocols},
  journal = {arXiv preprint arXiv:1802.03802},
  year = {2018},
  owner = {fadiheh},
  timestamp = {2018.08.08}
}

@BOOK{1982-Trivedi,
  title = {Probability and Statistics with Reliability, Queuing and Computer
	Science Applications},
  publisher = {Prentice-Hall},
  year = {1982},
  author = {K. S. Trivedi},
  address = {Englewood Cliffs, NJ}
}

@BOOK{2004-Truemper,
  title = {Design of Logic-based Intelligent Systems},
  publisher = {John Wiley \& Sons},
  year = {2004},
  author = {Klaus Truemper},
  address = {Hoboken, New Jersey}
}

@INBOOK{1968-Tseitin,
  chapter = {On the complexity of proof in propositional calculus},
  pages = {234-259},
  title = {Studies in constructive mathematics and mathematical logic. Part~II},
  publisher = {"Nauka", Leningrad. Otdel., Leningrad},
  year = {1968},
  author = {G. S. Tseitin},
  volume = {8},
  owner = {pavlenko},
  timestamp = {2010.07.23}
}

@INPROCEEDINGS{2003-TsunooSaito.etal,
  author = {Tsunoo, Yukiyasu and Saito, Teruo and Suzaki, Tomoyasu and Shigeri,
	Maki and Miyauchi, Hiroshi},
  title = {Cryptanalysis of DES implemented on computers with cache},
  booktitle = {International Workshop on Cryptographic Hardware and Embedded Systems},
  year = {2003},
  pages = {62--76},
  organization = {Springer},
  owner = {fadiheh},
  timestamp = {2018.07.12}
}

@MISC{2005-Tutorial,
  author = {Tutorial},
  title = {The {HOL} System},
  year = {2005},
  file = {:./files/2005-Tutorial.pdf:PDF},
  owner = {stoffel},
  timestamp = {2006.09.21}
}

@MASTERSTHESIS{2011-ShrinidhiUdupi,
  author = {Shrinidhi Udupi},
  title = {Generation of Abstract Cells for Aquarius Architecture via GapFree
	Verification},
  school = {TU Kaiserslautern},
  year = {2011},
  file = {:files/2011-ShrinidhiUdupi.pdf:PDF},
  owner = {bschmidt},
  timestamp = {2013.12.20}
}

@ARTICLE{2019-UdupiUrdahl.etal,
  author = {S. {Udupi} and J. {Urdahl} and D. {Stoffel} and W. {Kunz}},
  title = {Exploiting Hardware Unobservability for Low-Power Design and Safety
	Analysis in Formal Verification-Driven Design Flows},
  journal = {IEEE Transactions on Very Large Scale Integration ({VLSI}) Systems},
  year = {2019},
  volume = {27},
  pages = {1262-1275},
  number = {6},
  month = {June},
  file = {2019-UdupiUrdahl.etal.pdf:files/2019-UdupiUrdahl.etal.pdf:PDF}
}

@INPROCEEDINGS{2017-UdupiUrdahl.etal,
  author = {S. Udupi and J. Urdahl and D. Stoffel and W. Kunz},
  title = {Dynamic Power Optimization Based on Formal Property Checking of Operations},
  booktitle = {Proc. Intl. Conf. on VLSI Design (VLSID)},
  year = {2017},
  file = {:files/2017-UdupiUrdahl.pdf:PDF},
  owner = {udupi},
  timestamp = {2017.04.21}
}

@ARTICLE{2005-UgarteSanchez,
  author = {Inigo Ugarte and Pablo Sanchez},
  title = {Verification of Embedded Systems Based on Interval Analysis},
  journal = {International Journal of Parallel Programming},
  year = {2005},
  volume = {33},
  pages = {697-720},
  note = {10.1007/s10766-005-8909-9},
  file = {:./files/2005-UgarteSanchez.pdf:PDF},
  issue = {6},
  timestamp = {2006.10.04}
}

@ARTICLE{2006-UmansVilla.etal,
  author = {C. Umans and T.Villa and A.L. Sangionvanni-Vincentelli},
  title = {Complexity of Two-Level Logic Minimization},
  journal = {IEEE Transactions on Computer-Aided Design},
  year = {2006},
  volume = {25},
  pages = {1230-1246},
  number = {7},
  month = {July},
  file = {:./files/2006-UmansVilla.etal.pdf},
  owner = {wedler},
  timestamp = {2006.09.13}
}

@MISC{2005-WWW_uDraw,
  author = {{University of Bremen}},
  title = {uDraw(Graph)},
  year = {2005},
  owner = {bschmidt},
  timestamp = {2014.02.27},
  url = {http://www.informatik.uni-bremen.de/uDrawGraph/en/index.html}
}

@MISC{1992-Berkeley,
  author = {{University of California, Berkeley}},
  title = {Berkeley Logic Interchange Format ({BLIF})},
  year = {1992},
  file = {:./files/1992-Berkeley.pdf:PDF},
  owner = {stoffel},
  timestamp = {2006.09.21}
}

@PHDTHESIS{2015-Urdahl,
  author = {Joakim Urdahl},
  title = {{Path Predicate Abstraction for Sound System-Level Modeling of Digital
	Circuits}},
  school = {Technische Universit{\"a}t Kaiserslautern},
  year = {2015},
  month = {December},
  file = {2015-Urdahl.pdf:files/2015-Urdahl.pdf:PDF},
  owner = {joakim},
  timestamp = {2016.09.15}
}

@INPROCEEDINGS{2010-UrdahlStoffel.etal,
  author = {Joakim Urdahl and Dominik Stoffel and J{\"o}rg Bormann and Markus
	Wedler and Wolfgang Kunz},
  title = {Path Predicate Abstraction by Complete Interval Property Checking},
  booktitle = {Proc. International Conference on Formal Methods in Computer-Aided
	Design ({FMCAD})},
  year = {2010},
  pages = {207--215},
  file = {:./files/2010-UrdahlStoffel.etal.pdf:PDF},
  owner = {stoffel},
  timestamp = {2010.11.11}
}

@INPROCEEDINGS{2015-UrdahlStoffel.etal,
  author = {Joakim Urdahl and Dominik Stoffel and Wolfgang Kunz},
  title = {Architectural System Modeling for Correct-by-Construction {RTL} Design},
  booktitle = {Forum on Specification and Design Languages {(FDL)}},
  year = {2015},
  address = {Barcelona, Spain},
  month = {September},
  owner = {joakim},
  timestamp = {2015.10.27}
}

@ARTICLE{2014-UrdahlStoffel.etal,
  author = {Joakim Urdahl and Dominik Stoffel and Wolfgang Kunz},
  title = {Path Predicate Abstraction for Sound System-Level Models of {RT}-Level
	Circuit Designs},
  journal = {IEEE Transactions On Computer-Aided Design of Integrated Circuits
	and Systems (TCAD)},
  year = {2014},
  volume = {33},
  pages = {291--304},
  number = {2},
  month = {Feb.},
  file = {2014-UrdahlStoffel.etal.pdf:files/2014-UrdahlStoffel.etal.pdf:PDF},
  owner = {stoffel},
  timestamp = {2014.02.03}
}

@TECHREPORT{2013a-UrdahlStoffel.etal,
  author = {Joakim Urdahl and Dominik Stoffel and Wolfgang Kunz},
  title = {System- versus {RT}-Level Verification of Systems-on-Chip by Compositional
	Path Predicate Abstraction},
  institution = {Technische Universit{\"a}t Kaiserslautern, Dept. of Electrical and
	Computer Engineering, EDA group},
  year = {2013},
  number = {EDA-2013-01-29},
  month = {Jan},
  file = {:files/2013a-UrdahlStoffel.etal.pdf:PDF},
  owner = {stoffel},
  timestamp = {2013.02.05}
}

@INPROCEEDINGS{2012-UrdahlStoffel.etal,
  author = {Urdahl, Joakim and Stoffel, Dominik and Wedler, Markus and Kunz,
	Wolfgang},
  title = {System verification of concurrent {RTL} modules by compositional
	path predicate abstraction},
  booktitle = {Proc. Design Automation Conference (DAC)},
  year = {2012},
  pages = {334--343},
  file = {:files/2012-UrdahlStoffel.etal.pdf:PDF},
  isbn = {978-1-4503-1199-1},
  keywords = {abstraction, formal system verification},
  location = {San Francisco, California},
  numpages = {10}
}

@INPROCEEDINGS{2016-UrdahlUdupi.etal,
  author = {Joakim Urdahl and Shrinidhi Udupi and Tobias Ludwig and Dominik Stoffel
	and Wolfgang Kunz},
  title = {Properties First? {A} New Design Methodology for Hardware, and its
	Perspectives in Safety Analysis (invited paper)},
  booktitle = {The {IEEE/ACM} International Conference on Computer Aided Design
	{(ICCAD)}},
  year = {2016},
  file = {2016-UrdahlUdupi.etal.pdf:files/2016-UrdahlUdupi.etal.pdf:PDF},
  owner = {joakim},
  timestamp = {2016.09.19}
}

@INPROCEEDINGS{2013-UrdahlUdupi.etal,
  author = {Joakim Urdahl and Shrinidhi Udupi and Dominik Stoffel and Wolfgang
	Kunz},
  title = {Formal System-on-Chip Verfication: An Operation-Based Methodology
	and its Perspectives in Low Power Design},
  booktitle = {Proc. 23th International Workshop on Power and Timing Modeling, Optimization
	and Simulation (PATMOS)},
  year = {2013},
  file = {:files/2013-UrdahlUdupi.etal.pdf:PDF},
  owner = {joakim},
  timestamp = {2013.11.08}
}

@INPROCEEDINGS{2007-UsamiOhkubo,
  author = {K. Usami and N. Ohkubo},
  title = {A Design Approach for Fine-grained Run-Time Power Gating using Locally
	Extracted Sleep Signals},
  booktitle = {2006 International Conference on Computer Design},
  year = {2006},
  issn = {1063-6404},
  owner = {udupi},
  timestamp = {2017.08.15}
}

@INPROCEEDINGS{1996-BoppanaHartanto.etal,
  author = {V.Boppana and I.Hartanto and W.Kent fuchs},
  title = {Fault Diagnosis Using State Information},
  booktitle = {Proc. Annual International Symposium on Fault-Tolerant Computing},
  year = {1996},
  pages = {96 -103},
  file = {:./files/1996-BoppanaHartanto.etal.pdf:PDF},
  keywords = {ISCAS 89 benchmark circuits;diagnostic fault simulation;fault dictionaries;fault
	simulation requirements;large integrated circuits;partial scan circuits;primary
	output information;repeated fault diagnosis;state information based
	diagnosis technique;circuit analysis computing;fault diagnosis;integrated
	circuit testing;},
  timestamp = {2006.09.14}
}

@INPROCEEDINGS{1999-ValeCampos,
  author = {Sergio Vale and Aguiar Campos},
  title = {Symbolic Model Checking in Practice},
  year = {1999},
  file = {:./files/1999-ValeCampos.pdf:PDF},
  timestamp = {2006.09.21}
}

@INPROCEEDINGS{2001-VyatkinHanisch,
  author = {Valeriy Vyatkin, Hans-Michael Hanisch},
  title = {Formal-modeling and Verification in the Software Engineering Framework
	of {IEC61499}: a way to self-verifying systems},
  booktitle = {Proc. {IEEE} Conference on Emerging Technologies in Factory},
  year = {2001},
  volume = {2},
  pages = {113 -118 vol.2},
  month = {oct.},
  file = {:./files/2001-VyatkinHanisch.pdf:PDF},
  keywords = {IEC 61499;VEDA;agile manufacturing systems;distributed architectures;formal
	verification;graphics user interface;model-based simulation;net condition
	event systems;software engineering;software reconfigurations;software
	tools;IEC standards;computer aided production planning;digital simulation;formal
	verification;graphical user interfaces;manufacturing data processing;parallel
	processing;software architecture;software tools;},
  timestamp = {2006.09.22}
}

@ARTICLE{2007-VasudevanViswanath.etal,
  author = {Shobha Vasudevan and Vinod Viswanath and Robert W. Sumners and Jacob
	A.Abraham},
  title = {Automatic Verification of Arithmetic Circuits in {RTL} Using Stepwise
	Refinement of Term Rewriting Systems},
  journal = {IEEE Transactions on Computers},
  year = {2007},
  volume = {56},
  pages = {1401--1414},
  number = {10},
  address = {Washington, DC, USA},
  file = {:./files/2007-VasudevanViswanath.etal.pdf:PDF},
  issn = {0018-9340},
  publisher = {IEEE Computer Society}
}

@INPROCEEDINGS{2004-VivekanandaWhitney.etal,
  author = {Vivekananda M. Vedula and Whitney J. Townsend and Jacob A. Abraham},
  title = {Program Slicing for {ATPG}-based Property Checking},
  booktitle = {Proc. International Conference on {VLSI} Design},
  year = {2004},
  pages = { 591 - 596},
  file = {:./files/2004-VivekanandaWhitney.etal.pdf:PDF},
  keywords = { ATPG based property checking; abstracting designs; automatic test
	pattern generation; bounded model checking; program slicing; satisfiability
	techniques; sequential ATPG techniques; automatic test pattern generation;
	computability; program slicing; program verification; sequential
	circuits;},
  timestamp = {2006.09.21}
}

@ARTICLE{2011-VemuAbraham,
  author = {R. Vemu and J. Abraham},
  title = {CEDA: Control-Flow Error Detection Using Assertions},
  journal = {IEEE Transactions on Computers},
  year = {2011},
  volume = {60},
  pages = {1233-1245},
  number = {9},
  month = {September},
  file = {2011-VemuAbraham.pdf:files/2011-VemuAbraham.pdf:PDF},
  issn = {0018-9340},
  owner = {bartsch},
  timestamp = {2016.09.21}
}

@INPROCEEDINGS{2005-VijayakumarBrewer,
  author = {Aravind Vijayakumar and Forrest Brewer},
  title = {Weighted Control Scheduling},
  booktitle = {Proc. International Conference on Computer-Aided Design (ICCAD)},
  year = {2005},
  pages = { 777 - 783},
  file = {:./files/2005-VijayakumarBrewer.pdf:PDF},
  keywords = { control complexity; control dominated systems; nonBayesian probabilistic
	measure; optimal scheduling; weighted average latency; weighted control
	scheduling; weighted metric; data flow computing; processor scheduling;},
  timestamp = {2006.09.27}
}

@BOOK{2005-VijayaraghavanRamanathan,
  title = {A practical guide for SystemVerilog assertions},
  publisher = {Springer Science \& Business Media},
  year = {2005},
  author = {Vijayaraghavan, Srikanth and Ramanathan, Meyyappan},
  owner = {fadiheh},
  timestamp = {2018.08.02}
}

@PHDTHESIS{2015-Villarraga,
  author = {Carlos Villarraga},
  title = {Equivalence Checking for Hardware-Dependent Software. (tentative
	title)},
  school = {Technische Universit{\"a}t Kaiserslautern},
  year = {2015},
  owner = {bschmidt},
  timestamp = {2014.06.30}
}

@INPROCEEDINGS{2014-VillarragaSchmidt.etal,
  author = {Carlos Villarraga and Bernard Schmidt and Binghao Bao and Rakesh
	Raman and Christian Bartsch and Thomas Fehmel and Dominik Stoffel
	and Wolfgang Kunz},
  title = {Software in a Hardware View: New Models for {HW}-dependent Software
	in {SoC} Verification and Test (Invited Paper)},
  booktitle = {Proc. International Test Conference (ITC'14)},
  year = {2014},
  file = {:files/2014-VillarragaSchmidt.etal.pdf:PDF},
  owner = {stoffel},
  timestamp = {2014.07.31}
}

@INPROCEEDINGS{2013-VillarragaSchmidt.etal,
  author = {Carlos Villarraga and Bernard Schmidt and Christian Bartsch and J{\"o}rg
	Bormann and Dominik Stoffel and Wolfgang Kunz},
  title = {An Equivalence Checker for Hardware-Dependent Software},
  booktitle = {11. ACM-IEEE International Conference on Formal Methods and Models
	for Codesign ({MEMOCODE})},
  year = {2013},
  pages = {119-128},
  file = {2013-VillarragaSchmidt.etal.pdf:files/2013-VillarragaSchmidt.etal.pdf:PDF},
  keywords = {Equivalence Cecker, program netlist, EXG, Hardware-Dependent Software,
	Low-Level Software},
  owner = {bschmidt},
  timestamp = {2013.11.06}
}

@INPROCEEDINGS{2013a-VillarragaSchmidt.etal,
  author = {Carlos Villarraga and Bernard Schmidt and and J{\"o}rg Bormann and
	Dominik Stoffel and Wolfgang Kunz},
  title = {A New {SAT}-Based Approach for Equivalence Checking of Hardware-Dependent
	Low-Level Embedded System Software},
  booktitle = {edaWorkshop 13},
  year = {2013},
  pages = {31-37},
  month = {May},
  publisher = {VDE Verlag GMBH},
  file = {2013a-VillarragaSchmidt.etal.pdf:files/2013a-VillarragaSchmidt.etal.pdf:PDF},
  owner = {villarraga},
  timestamp = {2013.11.11}
}

@INBOOK{2018-VillarragaStoffel.etal,
  chapter = {Software in a Hardware View: New Models for {HW}-dependent Software
	in {SoC} Verification},
  pages = {123 - 153},
  title = {Formal System Verification},
  publisher = {Springer International Publishing},
  year = {2018},
  editor = {Rolf Drechsler},
  author = {Villarraga, Carlos and Stoffel, Dominik and Kunz, Wolfgang},
  owner = {villarraga},
  timestamp = {2016.04.26}
}

@INBOOK{2016-VillarragaStoffel.etal,
  chapter = {Software in a Hardware View: New Models for {HW}-dependent Software
	in {SoC} Verification},
  title = {Formal System Verification},
  publisher = {Springer (to appear)},
  year = {2016},
  editor = {Rolf Drechsler},
  author = {Villarraga, Carlos and Stoffel, Dominik and Kunz, Wolfgang},
  owner = {villarraga},
  timestamp = {2016.04.26}
}

@ARTICLE{2017-VlaovicVreze.etal,
  author = {Vlaovic, Bostjan and Vreže, Aleksander and Brezočnik, Zmago},
  title = {Applying Automated Model Extraction for Simulation and Verification
	of Real-Life SDL Specification with Spin},
  journal = {IEEE Access},
  year = {2017},
  volume = {5},
  pages = {5046-5058},
  owner = {fehmel},
  timestamp = {2019.05.27}
}

@ARTICLE{2008a-VogtWehn,
  author = {Timo Vogt and Norbert Wehn},
  title = {A Reconfigurable {ASIP} for Convolutional and Turbo Decoding in an
	{SDR} Environment.},
  journal = {{IEEE} Trans. {VLSI} Syst.},
  year = {2008},
  volume = {16},
  pages = {1309--1320},
  number = {10},
  biburl = {http://www.bibsonomy.org/bibtex/2b811901cb7bdc5b93899b80e399f83d0/dblp},
  date = {2009-01-31},
  description = {dblp},
  file = {:./files/2008a-VogtWehn.pdf},
  keywords = {dblp}
}

@INPROCEEDINGS{2008-VogtWehn,
  author = {Timo Vogt and Norbert Wehn},
  title = {A Reconfigurable Application Specific Instruction Set Processor for
	Convolutional and Turbo Decoding in a {SDR} Environment},
  booktitle = {Proc. International Conference on Design, Automation and Test in
	Europe ({DATE})},
  year = {2008},
  pages = {38 -43},
  file = {:./files/2008-VogtWehn.pdf:PDF},
  keywords = {ASIP;SDR environment;Viterbi decoding;application-specific instruction-set
	processors;binary convolutional decoding;channel coding;logic synthesis;programmable
	IP core;protocols;software defined radio;turbo decoding;wireless
	communication systems;Viterbi decoding;channel coding;software radio;turbo
	codes;},
  owner = {loitz},
  timestamp = {2008.02.19}
}

@INPROCEEDINGS{2010-OheimbMoedersheim,
  author = {Von Oheimb, David and M{\"o}dersheim, Sebastian},
  title = {{ASLan++}—a formal security specification language for distributed
	spercystems},
  booktitle = {Intl. Symp. on Formal Methods for Components and Objects},
  year = {2010},
  pages = {1--22},
  organization = {Springer},
  owner = {fadiheh},
  timestamp = {2018.11.22}
}

@INPROCEEDINGS{2002-WahlenGlokler.etal,
  author = {Oliver Wahlen and Tilman Glokler and Achim Nohl and Andreas Hoffmann
	and Rainer Leupers and Heinrich Meyr},
  title = {Application Specific Compiler/Architecture Codesign: A Case Study},
  booktitle = {Proc. Joint Conference on Languages, Compilers and Tools for Embedded
	Systems},
  year = {2002},
  series = {LCTES/SCOPES '02},
  pages = {185--193},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {513861},
  file = {:./files/2002-WahlenGlokler.etal.pdf:PDF},
  isbn = {1-58113-527-0},
  keywords = {ASIP, architecture exploration, retargetable compiler},
  location = {Berlin, Germany},
  numpages = {9}
}

@ARTICLE{1964-Wallace,
  author = {C. S. Wallace},
  title = {A Suggestion for a Fast Multiplier},
  journal = {{IEEE} Transactions on Electronic Computers},
  year = {1964},
  volume = {EC-13},
  pages = {14-17},
  month = {February},
  file = {:./files/1964-Wallace.pdf:PDF}
}

@INPROCEEDINGS{2004-WangHachtel.etal,
  author = {Chao Wang and Gary D. Hachtel and Fabio Domenzi},
  title = {Fine-Grain Abstraction and Sequential Don't Cares for Large Scale
	Model Checking},
  booktitle = {Proc. International Conference on Computer Design ({ICCD} 2004)},
  year = {2004},
  pages = { 112 - 118},
  file = {:./files/2004-WangHachtel.etal.pdf:PDF},
  keywords = { {Boolean} direction; SAT based method; combinational logic cones;
	fine grain abstraction refinement; greedy minimization; industrial
	scale designs; large scale model checking; {Boolean} algebra; combinational
	circuits; computability; greedy algorithms; logic design; minimisation;},
  owner = {thalmaier},
  timestamp = {2006.11.24}
}

@ARTICLE{2006-WangLi.etal,
  author = {C. Wang and B. Li and H. Jin and G. Hachtel and F. Somenzi},
  title = {Improving Ariadne's Bundle by following Multiple Threads in Abstraction
	Refinement},
  journal = {{IEEE} Transactions on Computer-Aided Design},
  year = {2006},
  volume = {25},
  pages = {2297 - 2316},
  file = {:./files/2006-WangLi.etal.pdf:PDF},
  owner = {thalmaier},
  timestamp = {2006.12.11}
}

@INPROCEEDINGS{2003-WangLi.etal,
  author = {Chao Wang and Bing Li and HoonSang Jin and Gary D. Hachtel and Fabio
	Somenzi},
  title = {Improving Ariadne's Bundle by Following Multiple Threads in Abstraction
	Refinement},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2003},
  pages = { 408 - 415},
  month = {nov.},
  file = {:./files/2003-WangLi.etal.pdf:PDF},
  keywords = { ACE; Ariadne bundle; SAT based concretization test; SOR; abstract
	counter examples; abstraction efficiency; abstraction refinement
	algorithm; abstraction refinement method; abstraction refinement
	process; formal verification; multiple thread concretization; scalability;
	synchronous onion rings; abstract data types; formal verification;
	multi-threading;},
  timestamp = {2006.09.12}
}

@INPROCEEDINGS{2006-WangYang.etal,
  author = {Chao Wang and Zijiang Yang and Franjo Ivancic and Aarti Gupta},
  title = {Disjunctive Image Computation for Embedded Software Verification},
  booktitle = {Proc. Internatioanl Conference on Design, Automation and Test in
	Europe (DATE)},
  year = {2006},
  pages = {1205--1210},
  address = {3001 Leuven, Belgium, Belgium},
  publisher = {European Design and Automation Association},
  abstract = {Finite state models generated from software programs have unique characteristics
	that are not exploited by existing model checking algorithms. In
	this paper, we propose a novel disjunctive image computation algorithm
	and other simplifications based on these characteristics. Our algorithm
	divides an image computation into a disjunctive set of easier ones
	that can be performed in isolation. Hypergraph partitioning is used
	to minimize the number of live variables in each disjunctive component.
	We use the live variables to simplify transition relations and reachable
	state subsets. Our experiments on a set of real-world C programs
	show that the new algorithm achieves orders-of-magnitude performance
	improvement over the best known conjunctive image computation algorithm.},
  file = {:./files/2006-WangYang.etal.pdf:PDF},
  isbn = {3-9810801-0-6},
  location = {Munich, Germany},
  owner = {nguyen},
  timestamp = {2006.09.08}
}

@INPROCEEDINGS{2001-WangHo.etal,
  author = {Dong Wang and Pei-Hsin Ho and Jiang Long and James Kukula and Yunshan
	Zhu and Tony Ma and Robert Damiano},
  title = {Formal Property Verification by Abstraction Refinement with Formal
	Simulation and Hybrid Engines},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {2001},
  pages = { 35 - 40},
  file = {:./files/2001-WangHo.etal.pdf:PDF},
  keywords = { BDD-ATPG hybrid engine; BDD-based fixpoint engine; RFN; abstraction
	refinement; design violation; formal property verification; multiple
	formal verification engines; real-world designs; sequential ATPG;
	two-phase process; automatic test pattern generation; binary decision
	diagrams; fixed point arithmetic; formal verification; logic testing;
	sequential circuits;},
  timestamp = {2006.09.12}
}

@INPROCEEDINGS{2003-WangMalik.etal,
  author = {Shaojie Wang and Sharad Malik and Reinaldo A. Bergamaschi},
  title = {Modeling and Integration of Peripheral Devices in Embedded Systems},
  booktitle = {Proc. International Conference On Design, Automation And Test In
	Europe ({DATE})},
  year = {2003},
  pages = { 136 - 141},
  file = {:./files/2003-WangMalik.etal.pdf:PDF},
  keywords = { IP-based embedded systems; Linux; USB device driver; automated device
	driver development; communication channels; constraints; declaratively
	described rules; device behavior formal specification models; event
	driven finite state machines; peripheral device integration; peripheral
	device modeling; platform independent virtual environment; software
	reliability; software reusability; synthesis patterns; device drivers;
	embedded systems; finite state machines; formal specification; peripheral
	interfaces; software reliability; software reusability;},
  timestamp = {2006.10.04}
}

@INPROCEEDINGS{2013-WasselGao.etal,
  author = {Wassel, Hassan MG and Gao, Ying and Oberg, Jason K and Huffmire,
	Ted and Kastner, Ryan and Chong, Frederic T and Sherwood, Timothy},
  title = {{SurfNoC}: a low latency and provably non-interfering approach to
	secure networks-on-chip},
  booktitle = {ACM SIGARCH Computer Architecture News},
  year = {2013},
  volume = {41},
  number = {3},
  pages = {583--594},
  organization = {ACM},
  owner = {fadiheh},
  timestamp = {2018.11.28}
}

@INPROCEEDINGS{2007-WatanabeHomma.etal,
  author = {Yuki Watanabe and Naofumi Homma and Takafumi Aoki and Tatsuo Higuchi},
  title = {Application of Symbolic Computer Algebra to Arithmetic Circuit Verification},
  booktitle = {Proc. International Conference on Computer Design ({ICCD})},
  year = {2007},
  pages = {25 - 32},
  month = {October},
  file = {:./files/2007-WatanabeHomma.etal.pdf:PDF},
  keywords = {FIR filter;Grobner Bases;arithmetic circuit verification;circuit description;polynomial
	reduction techniques;symbolic computer algebra;FIR filters;digital
	arithmetic;polynomials;},
  owner = {wedler},
  timestamp = {2007.11.21}
}

@ARTICLE{2016-WatermanLee.etal,
  author = {Waterman, Andrew and Lee, Yunsup and Avizienis, Rimas and Patterson,David
	A and Asanovi{\'c}, Krste},
  title = {The {RISC-V} instruction set manual volume {II}: Privileged architecture
	version~1.9},
  journal = {EECS Department, University of California, Berkeley, Tech. Rep. UCB/EECS-2016-161},
  year = {2016},
  owner = {fadiheh},
  timestamp = {2018.08.08}
}

@TECHREPORT{2014-WatermanLee.etal,
  author = {Waterman, Andrew and Lee, Yunsup and Patterson, David A and Asanovi{\'c},
	Krste},
  title = {The {RISC-V} Instruction Set Manual. Volume 1: User-Level {ISA},
	Version 2.0},
  institution = {California Univ Berkeley Dept of Electrical Engineering and Computer
	Sciences},
  year = {2014},
  owner = {fadiheh},
  timestamp = {2018.07.25}
}

@MISC{2012-Waugh,
  author = {Waugh, R},
  title = {Could a vulnerable computer chip allow hackers to down a boeing 787?‘back
	door’could allow cyber-criminals a way in},
  year = {2012},
  journal = {2016-12-04]. http://www. dailymail. co. uk/sciencetech/article-2152284},
  owner = {fadiheh},
  timestamp = {2018.07.18}
}

@ARTICLE{2001-WeaverAustin,
  author = {Chris Weaver and Todd Austin},
  title = {A Fault Tolerant Approach to Microprocessor Design},
  journal = {Dependable Systems and Networks},
  year = {2001},
  pages = {411 -420},
  file = {:./files/2001-WeaverAustin.pdf:PDF},
  keywords = {0.25 mum;Alpha 21264 processor;Alpha instructions;area overheads;core
	processor design errors;cycle-accurate simulation;energetic particle
	strikes;fault tolerant approach;fully synthesized unpipelined 4-wide
	checker component;high-performance microprocessor model;online checker
	component;operational faults;physical checker design;power demands;processor
	pipeline;prototype checker;reliable microprocessor design;simple
	checker design;simple state machine;supply voltage noise;system performance;timing
	analyses;timing analysis;computer architecture;fault tolerant computing;finite
	state machines;instruction sets;microprocessor chips;performance
	evaluation;},
  timestamp = {2006.09.14}
}

@ARTICLE{2012-WebelPflueger.etal,
  author = {Webel, T. and Pflueger, T. and Ludewig, R. and Lichtenau, C. and
	Niklaus, W. and Schaufler, R.},
  title = {Scalable and Modular Pervasive Logic/Firmware Design},
  journal = {IBM J. Res. Dev.},
  year = {2012},
  volume = {56},
  pages = {54--63},
  number = {1},
  month = jan,
  acmid = {2481727},
  address = {Riverton, NJ, USA},
  issn = {0018-8646},
  issue_date = {January 2012},
  numpages = {10},
  owner = {villarraga},
  publisher = {IBM Corp.},
  timestamp = {2016.06.17}
}

@ARTICLE{2012-WedlerCabrill.etal,
  author = {Wedler, M. and Cabrill, E. and Graham, S. and Patrick, L.},
  title = {Using Formal Verfication for {HW}/{SW} Co-verification of an {FPGA}
	{IP} Core},
  journal = {Xcell Journal (Xilinx, Inc.)},
  year = {2012},
  volume = {0},
  pages = {56-61},
  file = {2012-WedlerCabrill.etal.pdf:files/2012-WedlerCabrill.etal.pdf:PDF},
  owner = {villarraga},
  timestamp = {2012.08.27}
}

@INPROCEEDINGS{2010-WedlerPavlenko.etal,
  author = {Markus Wedler and Evgeny Pavlenko and Alexander Dreyer and Frank
	Seelisch and Dominik Stoffel and Gert-Martin Greuel and Wolfgang
	Kunz},
  title = {Solving Hard Instances in {QF-BV} Combining {Boolean} Reasoning with
	Computer Algebra},
  booktitle = {Algorithms and Applications for Next Generation {SAT} Solvers},
  year = {2010},
  number = {09461},
  series = {Dagstuhl Seminar Proceedings},
  address = {Dagstuhl, Germany},
  publisher = {Schloss Dagstuhl - Leibniz-Zentrum fuer Informatik, Germany},
  annote = {Keywords: SAT modulo Theory, Quantifier Free logic over fixed sized
	bitvectors; Computer Algebra},
  file = {:./files/2010-WedlerPavlenko.etal.pdf:PDF},
  issn = {1862-4405},
  owner = {pavlenko},
  timestamp = {2010.12.13},
  url = {http://drops.dagstuhl.de/opus/volltexte/2010/2509}
}

@ARTICLE{2007-WedlerStoffel.etal,
  author = {M. Wedler and D. Stoffel and R. Brinkmann and W. Kunz},
  title = {A Normalization Method for Arithmetic Data-Path Verification},
  journal = {{IEEE} Transactions on Computer-Aided Design},
  year = {2007},
  volume = {26},
  pages = {1909-1922},
  number = {11},
  month = {November},
  file = {:./files/2007-WedlerStoffel.etal.pdf:PDF},
  owner = {wedler},
  timestamp = {2007.10.25}
}

@INPROCEEDINGS{2005-WedlerStoffel.etal,
  author = {M. Wedler and D. Stoffel and W. Kunz},
  title = {Frontend Model Generation for {SAT}-Based Property Checking},
  booktitle = {Proc. International Conference On {ASIC} ({ASICON})},
  year = {2005 (invited paper)},
  pages = { 1017 - 1022},
  address = {Shanghai, China},
  month = {October},
  comment = {Read it IN},
  file = {:./files/2005-WedlerStoffel.etal.pdf:PDF},
  keywords = { SAT-based property checking; arithmetic datapath verification; state
	machines; verification algorithms; computability; electronic design
	automation; logic testing;},
  owner = {wedler},
  timestamp = {2006.08.29}
}

@INPROCEEDINGS{2005a-WedlerStoffel.etal,
  author = {M. Wedler and D. Stoffel and W. Kunz},
  title = {Normalization at the Arithmetic Bit Level},
  booktitle = {Proc. International Design Automation Conference (DAC-05)},
  year = {2005},
  month = {June},
  file = {dac05.pdf:dac05.pdf:PDF}
}

@INPROCEEDINGS{2004a-WedlerStoffel.etal,
  author = {M. Wedler and D. Stoffel and W. Kunz},
  title = {Arithmetic Reasoning in {DPLL}-based {SAT} Solving},
  booktitle = {Proc. International Conference on Design, Automation and Test in
	Europe ({DATE})},
  year = {2004},
  pages = { 30 - 35 Vol.1},
  address = {Paris, France},
  month = {February},
  file = {:./files/2004a-WedlerStoffel.etal.pdf:PDF},
  keywords = { DPLL; DPLL-based SAT solving; Davis Putnam Longman Loveland; RTL
	property checker; arithmetic bit level description; arithmetic circuit
	parts; arithmetic reasoning; formal verification; computability;
	digital arithmetic; formal verification; problem solving;}
}

@INPROCEEDINGS{2004-WedlerStoffel.etal,
  author = {M. Wedler and D. Stoffel and W. Kunz},
  title = {Exploiting State Encoding for Invariant Generation in Induction-Based
	Property Checking},
  booktitle = {Proc. Asia and South Pacific Design Automation Conference (ASPDAC)},
  year = {2004},
  pages = { 424 - 429},
  address = {Yokohama, Japan},
  month = {January},
  file = {aspdac04.pdf:aspdac04.pdf:PDF},
  keywords = { gate-level circuit representation; induction-based property checking;
	sequential circuit safety property checking; state encoding; finite
	state machines; logic CAD; safety; sequential circuits;}
}

@TECHREPORT{2003a-WedlerStoffel.etal,
  author = {M. Wedler and D. Stoffel and W. Kunz},
  title = {Arithmetik Reasoning in {DPLL}-based {SAT} Solving},
  institution = {Dept. of Electrical and Computer Engineering, Technische Universit{\"a}t
	Kaiserslautern, Germany},
  year = {2003},
  number = {EIS-11-03-1},
  file = {:./files/2003a-WedlerStoffel.etal.pdf:PDF},
  keywords = { DPLL; DPLL-based SAT solving; Davis Putnam Longman Loveland; RTL
	property checker; arithmetic bit level description; arithmetic circuit
	parts; arithmetic reasoning; formal verification; computability;
	digital arithmetic; formal verification; problem solving;},
  pages = { 30 - 35 Vol.1}
}

@INPROCEEDINGS{2003-WedlerStoffel.etal,
  author = {M. Wedler and D. Stoffel and W. Kunz},
  title = {Using {RTL} Statespace Information and State Encoding for Induction
	Based Property Checking},
  booktitle = {Proc. International Conference on Design, Automation and Test in
	Europe ({DATE})},
  year = {2003},
  pages = { 1156 - 1157},
  address = {Munich, Germany},
  month = {March},
  file = {:./files/2003-WedlerStoffel.etal.pdf:PDF},
  keywords = { RTL state space information; circuit gate-level representation; effective
	invariants computation; finite state machine; induction based property
	checking; safety properties checking; sequential circuits; state
	encoding; verification; finite state machines; formal verification;
	invariance; logic design; logic testing; sequential circuits; state-space
	methods;}
}

@INPROCEEDINGS{2002-WedlerStoffel.etal,
  author = {M. Wedler and D. Stoffel and W. Kunz},
  title = {Improving Structural {FSM}-Traversal by Constraint-Satisfying Simulation},
  booktitle = {Proc. {IEEE} Computer Society Annual Symposium on {VLSI}},
  year = {2002},
  pages = {151-158},
  month = {April},
  file = {:./files/2002-WedlerStoffel.etal.pdf:PDF}
}

@INPROCEEDINGS{2000-WefelMolitor,
  author = {Sandro Wefel and Paul Molitor},
  title = {Prove that a faulty multiplier is faulty!?},
  booktitle = {GLSVLSI '00: Proceedings of the 10th Great Lakes symposium on {VLSI}},
  year = {2000},
  pages = {43--46},
  address = {New York, NY, USA},
  publisher = {ACM Press},
  file = {:./files/2000-WefelMolitor.pdf:PDF},
  isbn = {1-58113-251-4},
  location = {Chicago, Illinois, United States},
  owner = {wedler},
  timestamp = {2007.10.24}
}

@BOOK{1987-Wegener,
  title = {The Complexity of {Boolean} Functions},
  year = {1987},
  author = {Ingo Wegener},
  file = {:./files/1987-Wegener.pdf:PDF}
}

@INPROCEEDINGS{0000-WenMizoguchi,
  author = {Wu Wen and Fumio Mizoguchi},
  title = {A Case Study on Model Checking Multi-Agent System Using SMV},
  comment = {year and booktitle are unknown},
  file = {0000-WenMizoguchi.pdf:files/0000-WenMizoguchi.pdf:PDF},
  timestamp = {2006.09.14}
}

@PHDTHESIS{2000-Wessaely,
  author = {Roland Wessaly},
  title = {Dimensioning Survivable Capacitated Networks},
  school = {Technische Universitaet Berlin},
  year = {2000},
  type = {Dissertation},
  file = {:./files/2000-Wessaely.pdf:PDF}
}

@INPROCEEDINGS{2002-WhaleyMartin.etal,
  author = {Whaley, John and Martin, Michael C. and Lam, Monica S.},
  title = {Automatic Extraction of Object-oriented Component Interfaces},
  booktitle = {Proceedings of the 2002 ACM SIGSOFT International Symposium on Software
	Testing and Analysis},
  year = {2002},
  series = {ISSTA '02},
  pages = {218--228},
  address = {New York, NY, USA},
  publisher = {ACM},
  acmid = {566212},
  doi = {10.1145/566172.566212},
  isbn = {1-58113-562-9},
  location = {Roma, Italy},
  numpages = {11},
  url = {http://doi.acm.org/10.1145/566172.566212}
}

@INPROCEEDINGS{2001-WhittemoreKim.etal,
  author = {Jesse Whittemore and Joonyoung Kim and Karem Sakallah},
  title = {{SATIRE}: A New Incremental Satisfiability Engine},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {2001},
  pages = { 542 - 545},
  file = {:./files/2001-WhittemoreKim.etal.pdf:PDF},
  keywords = { ATPG; SATIRE; electronic design automation; incremental satisfiability
	engine; incremental solution; logic design; logic testing; nonCNF
	constraints; optimization problems; verification; {Boolean} functions;
	automatic test pattern generation; circuit optimisation; computability;
	design for testability; electronic design automation; formal verification;
	logic CAD; logic testing;},
  timestamp = {2006.10.04}
}

@MISC{2008-Wienand,
  author = {O. Wienand},
  title = {Standard Bases over Ring and Applications. PhD Thesis},
  howpublished = {To appear in 2011},
  owner = {wedler},
  timestamp = {2008.01.21}
}

@INPROCEEDINGS{2008-WienandWedler.etal,
  author = {Oliver Wienand and Markus Wedler and Dominik Stoffel and Wolfgang
	Kunz and Gert-Martin Greuel},
  title = {An algebraic approach for proving data correctness in arithmetic
	data paths},
  booktitle = {Proc. International Conference Computer Aided Verification ({CAV})},
  year = {2008},
  pages = {473-486},
  address = {Princeton, NJ, USA},
  month = {July},
  file = {:./files/2008-WienandWedler.etal.pdf:PDF},
  owner = {wedler},
  timestamp = {2008.02.18}
}

@ARTICLE{2008-WilhelmEngblom.etal,
  author = {Wilhelm, Reinhard and Engblom, Jakob and Ermedahl, Andreas and Holsti,
	Niklas and Thesing, Stephan and Whalley, David and Bernat, Guillem
	and Ferdinand, Christian and Heckmann, Reinhold and Mitra, Tulika
	and Mueller, Frank and Puaut, Isabelle and Puschner, Peter and Staschulat,
	Jan and Stenstr\"{o}m, Per},
  title = {{The Worst-case Execution-time Problem-Overview of Methods and Survey
	of Tools}},
  journal = {ACM Trans. Embed. Comput. Syst.},
  year = {2008},
  volume = {7},
  pages = {36:1--36:53},
  number = {3},
  month = may,
  acmid = {1347389},
  address = {New York, NY, USA},
  articleno = {36},
  file = {2008-WilhelmEngblom.etal.pdf:files/2008-WilhelmEngblom.etal.pdf:PDF},
  issn = {1539-9087},
  issue_date = {April 2008},
  keywords = {Hard real time, worst-case execution times},
  numpages = {53},
  owner = {villarraga},
  publisher = {ACM},
  timestamp = {2016.06.10}
}

@ARTICLE{2008-WilhelmReinhard.etal,
  author = {Wilhelm, Reinhard and Engblom, Jakob and Ermedahl, Andreas and Holsti,
	Niklas and Thesing, Stephan and Whalley, David and Bernat, Guillem
	and Ferdinand, Christian and Heckmann, Reinhold and Mitra, Tulika
	and Mueller, Frank and Puaut, Isabelle and Puschner, Peter and Staschulat,
	Jan and Stenstr\"{o}m, Per},
  title = {The Worst-case Execution-time Problem --- Overview of Methods and
	Survey of Tools},
  journal = {ACM Trans. Embed. Comput. Syst.},
  year = {2008},
  volume = {7},
  pages = {1--53},
  number = {3},
  month = may,
  acmid = {1347389},
  address = {New York, NY, USA},
  articleno = {36},
  doi = {10.1145/1347375.1347389},
  issn = {1539-9087},
  issue_date = {April 2008},
  keywords = {Hard real time, worst-case execution times},
  numpages = {53},
  publisher = {ACM}
}

@INPROCEEDINGS{2005-Wilhelm,
  author = {Stephan Wilhelm},
  title = {Efficient Analysis of Pipeline Models for {WCET} Computation},
  year = {2005},
  file = {:./files/2005-Wilhelm.pdf:PDF},
  timestamp = {2006.09.22}
}

@MASTERSTHESIS{2009-FabianWilhelms,
  author = {Fabian Wilhelms},
  title = {Entwurf einer XML-Struktur fuer die Implementierung Abstrakter Zellen
	am Beispiel des OpenCore Aquarius},
  school = {TU Kaiserslautern},
  year = {2009},
  type = {{Studienarbeit}},
  file = {:files/2009-FabianWilhelms.pdf:PDF},
  owner = {bschmidt},
  timestamp = {2014.01.30}
}

@INPROCEEDINGS{2000-WilsonDill.etal,
  author = {Wilson, Chris and Dill, David L. and Bryant, Randal E.},
  title = {Symbolic Simulation with Approximate Values},
  booktitle = {Proceedings of the Third International Conference on Formal Methods
	in Computer-Aided Design},
  year = {2000},
  acmid = {683235},
  file = {2000-WilsonDill.etal:2000-WilsonDill.etal.683235:Djvu},
  isbn = {3-540-41219-0},
  numpages = {16},
  owner = {udupi},
  timestamp = {2017.11.28}
}

@ARTICLE{2014-WimerKoren,
  author = {S. Wimer and I. Koren},
  title = {Design Flow for Flip-Flop Grouping in Data-Driven Clock Gating},
  journal = {IEEE Transactions on Very Large Scale Integration (VLSI) Systems},
  year = {2014},
  volume = {22},
  pages = {771-778},
  number = {4},
  month = {April},
  abstract = {Clock gating is a predominant technique used for power saving. It
	is observed that the commonly used synthesis-based gating still leaves
	a large amount of redundant clock pulses. Data-driven gating aims
	to disable these. To reduce the hardware overhead involved, flip-flops
	(FFs) are grouped so that they share a common clock enabling signal.
	The question of what is the group size maximizing the power savings
	is answered in a previous paper. Here we answer the question of which
	FFs should be placed in a group to maximize the power reduction.
	We propose a practical solution based on the toggling activity correlations
	of FFs and their physical position proximity constraints in the layout.
	Our data-driven clock gating is integrated into an Electronic Design
	Automation (EDA) commercial backend design flow, achieving total
	power reduction of 15%-20% for various types of large-scale state-of-the-art
	industrial and academic designs in 40 and 65 manometer process technologies.
	These savings are achieved on top of the sClock gating is a predominant
	technique used for power saving. It is observed that the commonly
	used synthesis-based gating still leaves a large amount of redundant
	clock pulses. Data-driven gating aims to disable these. To reduce
	the hardware overhead involved, flip-flops (FFs) are grouped so that
	they share a common clock enabling signal. The question of what is
	the group size maximizing the power savings is answered in a previous
	paper. Here we answer the question of which FFs should be placed
	in a group to maximize the power reduction. We propose a practical
	solution based on the toggling activity correlations of FFs and their
	physical position proximity constraints in the layout. Our data-driven
	clock gating is integrated into an Electronic Design Automation (EDA)
	commercial backend design flow, achieving total power reduction of
	15%-20% for various types of large-scale state-of-the-art industrial
	and academic designs in 40 and 65 manometer process technol- gies.
	These savings are achieved on top of the savings obtained by clock
	gating synthesis performed by commercial EDA tools, and gating manually
	inserted into the register transfer level design.avings obtained
	by clock gating synthesis performed by commercial EDA tools, and
	gating manually inserted into the register transfer level design.},
  issn = {1063-8210},
  keywords = {electronic design automation;flip-flops;logic design;commercial EDA
	tools;common clock enabling signal;data-driven clock gating;design
	flow;electronic design automation;flip-flop grouping;large-scale
	academic designs;large-scale industrial designs;physical position
	proximity constraints;power saving;predominant technique;redundant
	clock pulses;register transfer level design;synthesis-based gating;Clock
	gating;clock networks;dynamic power reduction}
}

@INPROCEEDINGS{2004-WinkelmannStoffel.etal,
  author = {K. Winkelmann and D. Stoffel and G. Fey and H. Trylus},
  title = {Cost-Efficient Block Verification for a {UMTS} Up-Link Chip-Rate
	Coprocessor},
  booktitle = {Proc. International Conference on Design, Automation and Test in
	Europe ({DATE})},
  year = {2004},
  pages = { 162 - 167 Vol.1},
  address = {Paris, France},
  month = {February},
  file = {:./files/2004-WinkelmannStoffel.etal.pdf:PDF},
  keywords = { ASIC designs; CVE property checker; UMTS; block-level functional
	correctness; cost-efficient block verification; formal property checking;
	functional verification; productivity gains; state space; static
	timing analysis; timing verification; universal mobile telecommunication
	system; up-link chip-rate coprocessor; 3G mobile communication; application
	specific integrated circuits; coprocessors; formal verification;
	integrated circuit testing;}
}

@ARTICLE{1990-Wolsey,
  author = {Laurence A. Wolsey},
  title = {Valid Inequalities for 0-1 Knapsacks and {MIP}s with Generalized
	Upper Bound Constraints},
  journal = {Discrete Applied Mathematics},
  year = {1990},
  volume = {29},
  pages = {251-261},
  file = {:./files/1990-Wolsey.pdf:PDF}
}

@ARTICLE{2006-WuHsiao,
  author = {Q. Wu and M. S. Hsiao},
  title = {A New Simulation-Based Property Checking Algorithm Based on Partitioned
	Alternative Search Space Traversal},
  journal = {IEEE Transactions on Computers},
  year = {2006},
  volume = {55},
  pages = {1325-1334},
  number = {11},
  month = {November},
  file = {:./files/2006-WuHsiao.pdf:PDF},
  owner = {wedler},
  timestamp = {2006.12.19}
}

@BOOK{1991-Winderlich,
  title = {Hochintegrierte Schaltungen: Pruefgerechter Entwurf und Test},
  year = {1991},
  author = {H.-J. Wunderlich},
  address = {Berlin, Heidelberg, New York}
}

@PHDTHESIS{1996-Wunderling,
  author = {Roland Wunderling},
  title = {Paralleler und objektorientierter Simplex-Algorithmus},
  school = {Technische Universit{\"a}t Berlin},
  year = {1996},
  type = {Dissertation},
  file = {:./files/1996-Wunderling.pdf:PDF},
  url = {http://www.zib.de/Publications/abstracts/TR-96-09/}
}

@ARTICLE{1992-ShiAllen,
  author = {X.Shi and P.E.Allen},
  title = {Use of {VHDL} to Model and Simulate Analog-Digital {IC's}},
  journal = {Proceedings of the 35th Midwest Symposium on Circuits and Systems},
  year = {1992},
  volume = {2},
  pages = {908 -911},
  month = {aug},
  file = {:./files/1992-ShiAllen.pdf:PDF},
  keywords = {VHDL;analog-digital ICs;behavioral modeling;event driven simulator;mixed
	analog-digital circuits;oversampling sigma-delta A/D convertor;circuit
	analysis computing;digital simulation;mixed analogue-digital integrated
	circuits;specification languages;}
}

@MISC{2003-XieBrowne.etal,
  author = {Fei Xie and James C. Browne and Robert P. Kurshan and Vladimir Levin},
  title = {Verification Case Studies with ObjectCheck},
  note = {Slides},
  file = {:./files/2003-XieBrowne.etal.pdf:PDF},
  owner = {nguyen},
  timestamp = {2007.02.02}
}

@INPROCEEDINGS{2006-XieMartin.etal,
  author = {Xie, Tao and Martin, Evan and Yuan, Hai},
  title = {Automatic extraction of abstract-object-state machines from unit-test
	executions},
  booktitle = {Proceedings of the 28th international conference on Software engineering},
  year = {2006},
  owner = {fehmel},
  timestamp = {2019.05.27}
}

@ARTICLE{2007-XieAiken,
  author = {Xie, Yichen and Aiken, Alex},
  title = {Saturn: A scalable framework for error detection using {Boolean}
	satisfiability},
  journal = {ACM Trans. Program. Lang. Syst.},
  year = {2007},
  volume = {29},
  number = {3},
  month = may,
  acmid = {1232423},
  address = {New York, NY, USA},
  articleno = {16},
  file = {2007-XieAiken.pdf:files/2007-XieAiken.pdf:PDF},
  issn = {0164-0925},
  issue_date = {May 2007},
  keywords = {{Boolean} satisfiability, Program analysis, error detection},
  owner = {villarraga},
  publisher = {ACM},
  timestamp = {2013.05.11}
}

@INPROCEEDINGS{2003-XieChou,
  author = {Yichen Xie and Andy Chou},
  title = {Path Sensitive Program Analysis using {Boolean} Satisfiability},
  year = {2003},
  file = {:./files/2003-XieChou.pdf:PDF},
  timestamp = {2006.09.19}
}

@MISC{2005-Xilinx,
  author = {{XILINX}},
  title = {Product Selection Matrix},
  year = {2005},
  file = {:./files/2005-Xilinx.pdf:PDF},
  owner = {stoffel},
  timestamp = {2006.09.21}
}

@MISC{2011a-Xilinx,
  author = {{Xilinx, Inc.}},
  title = {LogiCORE IP Soft Error Mitigation Controller v3.1},
  year = {2011},
  file = {2011a-Xilinx.pdf:files/2011a-Xilinx.pdf:PDF},
  owner = {villarraga},
  timestamp = {2016.06.07},
  url = {http://www.xilinx.com/}
}

@MISC{2011-Xilinx,
  author = {{Xilinx, Inc.}},
  title = {{PicoBlaze} 8-bit Embedded Microcontroller User Guide},
  year = {2011},
  file = {2011-Xilinx.pdf:files/2011-Xilinx.pdf:PDF},
  owner = {villarraga},
  timestamp = {2016.06.07},
  url = {http://www.xilinx.com/}
}

@TECHREPORT{2002-Xu,
  author = {Fang Xu},
  title = {Fault Injection--A Dependability Evaluation Technology},
  institution = {University of Virginia},
  year = {2002},
  file = {:./files/2002-Xu.pdf:PDF},
  timestamp = {2006.09.14}
}

@INPROCEEDINGS{1997-LakhnechSiegel,
  author = {Y.Lakhnech and M.Siegel},
  title = {Temporal Logic for Stabilizing Systems},
  booktitle = {Proc. International Conference on Temporal Logic},
  year = {1997},
  file = {:./files/1997-LakhnechSiegel.pdf:PDF},
  timestamp = {2006.09.14}
}

@CONFERENCE{2004-NovikovBrinkmann,
  author = {Yakov Novikov , Raik Brinkmann},
  title = {Foundations of Hierarchical {SAT}-Solving},
  booktitle = {Proc. Intranational Workshop on {Boolean} Problems},
  year = {2004},
  file = {:./files/2004-NovikovBrinkmann.pdf:PDF},
  timestamp = {2006.12.12}
}

@ARTICLE{1998-Yan,
  author = {Yan,T.},
  title = {The Geobucket Data Structure for Polynomials},
  journal = {Journal of Symbolic Computation},
  year = {1998},
  volume = {25},
  pages = {285?294},
  number = {3},
  month = {March},
  owner = {wedler},
  timestamp = {2008.02.18}
}

@INPROCEEDINGS{2005-IvancicYang.etal,
  author = {F.Ivancic Z. Yang and M.K. Ganai and A. Gupta and I. Shlyakhter and
	P. Ashar},
  title = {{FSoft} Software Verification Platform},
  booktitle = {Proc. International Conference Computer Aided Verification ({CAV})},
  year = {2005},
  pages = {301--306},
  publisher = {Springer},
  file = {IvancicYang-FSoftSoftwareVerificationPlatform.pdf:IvancicYang-FSoftSoftwareVerificationPlatform.pdf:PDF},
  timestamp = {2006.09.22}
}

@MISC{2004-YangSeger,
  author = {Jin Yang and Carl-Johan and H. Seger},
  title = {Compositional Specification and Model Checking in {GSTE}},
  year = {2004},
  file = {:./files/2004-YangSeger.pdf:PDF},
  owner = {stoffel},
  pages = {216-228},
  timestamp = {2006.09.21}
}

@INPROCEEDINGS{2002-YangGoel,
  author = {Jin Yang and Amit Goel},
  title = {{GSTE} Through A Case Study},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2002},
  pages = { 534 - 541},
  file = {:./files/2002-YangGoel.pdf:PDF},
  keywords = { FIFO verification; GSTE model checking efficiency/accuracy refinement;
	STE extensions; STE symbolic quaternary models; assertion graphs;
	digital IC verification; generalized symbolic trajectory evaluation;
	quaternary symbolic simulation; circuit CAD; circuit simulation;
	formal verification; integrated circuit design; integrated circuit
	modelling; logic CAD; logic simulation;},
  timestamp = {2006.09.21}
}

@INPROCEEDINGS{2001-YangSeger,
  author = {Jin Yang and Seger, C.-J.H.},
  title = {Introduction To Generalized Symbolic Trajectory Evaluation},
  booktitle = {Computer Design, 2001. {ICCD} 2001. Proceedings. 2001 International
	Conference on},
  year = {2001},
  pages = {360 -365},
  file = {:./files/2001-YangSeger.pdf:PDF},
  keywords = {Symbolic trajectory evaluation;assertion graphs;formal semantics;industrial
	memory verification;lattice-based model checking;symbolic simulation;formal
	verification;logic testing;symbol manipulation;}
}

@ARTICLE{2003-YangSeger,
  author = {Jin Yang and Carl-Johan H. Seger},
  title = {Introduction To Generalized Symbolic Trajectory Evaluation},
  journal = {{IEEE} Transactions on {VLSI} Systems},
  year = {2003},
  volume = {11},
  pages = {345--353},
  number = {3},
  address = {Piscataway, NJ, USA},
  file = {:./files/2003-YangSeger.pdf:PDF},
  issn = {1063-8210},
  publisher = {IEEE Educational Activities Department}
}

@INPROCEEDINGS{2002-YangSeger,
  author = {Jin Yang and Carl-Johan H. Seger},
  title = {Generalized Symbolic Trajectory Evaluation - Abstraction in Action},
  booktitle = {Proc. International Conference on Formal Methods in Computer-Aided
	Design ({FMCAD})},
  year = {2002},
  pages = {70--87},
  address = {London, UK},
  publisher = {Springer-Verlag},
  file = {:./files/2002-YangSeger.pdf:PDF},
  isbn = {3-540-00116-6},
  owner = {nguyen},
  timestamp = {2007.12.13}
}

@INPROCEEDINGS{2005-YangHuang.etal,
  author = {Ya-Ching Yang and Juinn-Dar Huang and Chia-Chih Yen and Che-Hua Shih
	and Jing-Yang Jou},
  title = {Formal Compliance Verification Of Interface Protocols},
  booktitle = {Proc. {IEEE} International Symposium on {VLSI}},
  year = {2005},
  pages = { 12 - 15},
  file = {:./files/2005-YangHuang.etal.pdf:PDF},
  keywords = { SoC; branch-and-bound algorithm; finite state machines; formal compliance
	verification; interface logic; interface protocol compliance verification;
	logic design; specification FSM; system on chip; time complexity;
	computational complexity; finite state machines; formal verification;
	logic design; protocols; system-on-chip; tree searching;},
  owner = {nguyen}
}

@INPROCEEDINGS{2014-YaromFalkner,
  author = {Yarom, Yuval and Falkner, Katrina},
  title = {{FLUSH+ RELOAD:} A High Resolution, Low Noise, {L3} Cache Side-Channel
	Attack.},
  booktitle = {USENIX Security Symposium},
  year = {2014},
  volume = {1},
  pages = {22--25},
  owner = {fadiheh},
  timestamp = {2018.07.12}
}

@ARTICLE{2017-YaromGenkin.etal,
  author = {Yarom, Yuval and Genkin, Daniel and Heninger, Nadia},
  title = {CacheBleed: a timing attack on {OpenSSL} constant-time {RSA}},
  journal = {Journal of Cryptographic Engineering},
  year = {2017},
  volume = {7},
  pages = {99--112},
  number = {2},
  owner = {fadiheh},
  publisher = {Springer},
  timestamp = {2018.07.12}
}

@MISC{web_yices,
  author = {Yices},
  owner = {pavlenko},
  timestamp = {2011.03.08},
  url = {http://yices.csl.sri.com/}
}

@INPROCEEDINGS{1995-YorkThuns.etal,
  author = {Cary York and R .M.Thuns and J.Pattel and D.Beatty},
  title = {An Integrated Environment for {HDL} Verification},
  booktitle = {Proc. International Verilog {HDL} Conference},
  year = {1995},
  pages = {9 -18},
  file = {:./files/1995-YorkThuns.etal.pdf:PDF},
  keywords = { CTL model checking; HDL verification; VHDL; Verilog-HDL; combinational
	equivalence; digital design verification; equivalence checking; formal
	methods; formal verification; formal verification prototype; functional
	verification; higher-level specification; integrated environment;
	model checking; object-oriented design; property checking; sequential
	equivalence; simulation; smart simulator; specification; symbolic
	simulation; top-down design flow; computer architecture; formal specification;
	formal verification; hardware description languages; object-oriented
	programming; software tools; virtual machines;},
  timestamp = {2006.09.21}
}

@MISC{2007-Yoshino,
  author = {Ben Yoshino},
  title = {Make Tutorial},
  note = {Make tutorial slides.},
  file = {:./files/2007-Yoshino.ppt:PPT},
  owner = {nguyen},
  timestamp = {2007.02.02},
  url = {http://www.eng.hawaii.edu/Tutor/Make}
}

@MISC{1993-YoungerWard,
  author = {Eddy Younger and Martin Ward},
  title = {Understanding Concurrent Programs using Program Transformations},
  year = {1993},
  address = {Capri, Italy},
  booktitle = {Proc. {IEEE} Workshop on Program Comprehension},
  file = {:./files/1993-YoungerWard.pdf:PDF},
  keywords = {WSL;concurrent programs;interrupts;inverse engineering;program transformations;real-time
	programs;reverse engineering;sequential program;specification;timing
	constraints;wide spectrum language;parallel programming;real-time
	systems;software maintenance;specification languages;},
  owner = {nguyen},
  pages = {160 -168},
  timestamp = {2016.05.11}
}

@INPROCEEDINGS{2004-YoussefYoo.etal,
  author = {Mohamed-Wassim Youssef and Sungjoo Yoo and Arif Sasongko and Yanick
	Paviot and Ahmed A. Jerraya},
  title = {Debugging {HW/SW} Interface for {MPSoC}: Video Encoder System Design
	Case Study},
  booktitle = {Proc. International Design Automation Conference ({DAC})},
  year = {2004},
  pages = {908 -913},
  file = {:./files/2004-YoussefYoo.etal.pdf:PDF},
  timestamp = {2006.09.27}
}

@INPROCEEDINGS{2019-YuHsiung.etal,
  author = {Yu, Jiyong and Hsiung, Lucas and El Hajj, Mohamad and Fletcher, Christopher
	W},
  title = {Data Oblivious ISA Extensions for Side Channel-Resistant and High
	Performance Computing.},
  booktitle = {The Network and Distributed System Security Symposium (NDSS)},
  year = {2019}
}

@PHDTHESIS{1992-Yu,
  author = {Yuan Yu},
  title = {Automate Proof Object Code For Widely Used Microprocessor},
  school = {The University of Texas at Austin},
  year = {1992},
  file = {:./files/1992-Yu.pdf:PDF},
  timestamp = {2006.09.18}
}

@TECHREPORT{2001-YuJohnson,
  author = {Yangyang Yu and Barry Johnson},
  title = {A Perspective on the State of Research on Fault Injection Techniques},
  year = {2001},
  file = {:./files/2001-YuJohnson.pdf:PDF},
  timestamp = {2006.09.14}
}

@INPROCEEDINGS{2014-YuSubramanyan.etal,
  author = {Yu, Yinlei and Subramanyan, Pramod and Tsiskaridze, Nestan and Malik,
	Sharad},
  title = {All-SAT Using Minimal Blocking Clauses},
  booktitle = {Proceedings of the 2014 27th International Conference on VLSI Design
	and 2014 13th International Conference on Embedded Systems},
  year = {2014},
  series = {VLSID '14},
  pages = {86--91},
  address = {Washington, DC, USA},
  publisher = {IEEE Computer Society},
  acmid = {2586827},
  isbn = {978-1-4799-2513-1},
  keywords = {All-SAT, SAT, SAT solver, verification, reachability},
  numpages = {6},
  owner = {villarraga},
  timestamp = {2016.07.28}
}

@BOOK{2006-YuanPixley.etal,
  title = {Constraint-based verification},
  publisher = {Springer},
  year = {2006},
  author = {J. Yuan and C. Pixley and A. Aziz},
  owner = {Binghao},
  timestamp = {2012.02.20}
}

@ARTICLE{1999-Liu,
  author = {Z.Liu},
  title = {Specification And Verification Of Fault Tolerance Timing And Scheduling},
  journal = {{ACM} Transactions on Programming Languages and Systems},
  year = {1999},
  volume = {21},
  pages = {46 - 89},
  file = {:./files/1999-Liu.pdf:PDF},
  timestamp = {2006.09.14}
}

@INPROCEEDINGS{1996-Liu,
  author = {Z.Liu},
  title = {Formalizing Real Time Scheduling As Program Refinement},
  booktitle = {Proc. International {AMAST} Workshop on Real-Time Systems and Concurrent
	and Distributed Software: Transformation-Based Reactive Systems Development},
  year = {1996},
  file = {:./files/1996-Liu.pdf:PDF},
  timestamp = {2006.09.14}
}

@INPROCEEDINGS{1988-ZabihMcAllester,
  author = {Ramin Zabih and David A. McAllester},
  title = {A Rearrangement Search Strategy for Determining Propositional Satisfiability},
  booktitle = {Proc. National Conference on Artificial Intelligence},
  year = {1988},
  pages = {155-160},
  file = {:./files/1988-ZabihMcAllester.pdf:PDF}
}

@ARTICLE{2013-ZahirEwert.etal,
  author = {R. Zahir and M. Ewert and H. Seshadri},
  title = {The Medfield Smartphone: Intel Architecture in a Handheld Form Factor},
  journal = {IEEE Micro},
  year = {2013},
  volume = {33},
  pages = {38-46},
  number = {6},
  month = {Nov},
  file = {2013-ZahirEwert.etal.pdf:files/2013-ZahirEwert.etal.pdf:PDF},
  issn = {0272-1732},
  keywords = {energy management systems;integrated circuit layout;integrated circuit
	packaging;low-power electronics;microprocessor chips;smart phones;system-on-chip;IA
	processor;Intel Atom Z2480 processor;Intel Hi-K process technology;Intel
	architecture processor;Intel smartphone platform;Medfield smartphone;SoC
	design;board layout;chip packaging;handheld form factor;hardware
	power-management technique;size 32 nm;software architecture;software
	power-management technique;system-on-a-chip design;Androids;Batteries;Humanoid
	robots;Process control;Smart phones;System-on-chip;Android;Atom;Intel;Medfield;SoC;low-power
	design;smartphone;system-on-a-chip},
  owner = {villarraga},
  timestamp = {2016.06.17}
}

@INPROCEEDINGS{2004-ZaninMancini,
  author = {Zanin, Giorgio and Mancini, Luigi Vincenzo},
  title = {Towards a formal model for security policies specification and validation
	in the selinux system},
  booktitle = {Proceedings of the ninth ACM symposium on Access control models and
	technologies},
  year = {2004},
  pages = {136--145},
  organization = {ACM},
  owner = {fadiheh},
  timestamp = {2018.11.22}
}

@INPROCEEDINGS{2005-ZaraketBaumgartner.etal,
  author = {Fadi Zaraket and Jason Baumgartner and Adnan Aziz},
  title = {Scalable Compositional Minimization via Static Analysis},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2005},
  pages = { 1060 - 1067},
  file = {:./files/2005-ZaraketBaumgartner.etal.pdf:PDF},
  keywords = { bisimulation minimization; combinational logic; compositional minimization;
	heuristic algorithm; state transition; static analysis; verification
	tasks; bisimulation equivalence; combinatorial mathematics; computational
	complexity; formal verification; high level synthesis; minimisation;
	redundancy; state-space methods;},
  timestamp = {2006.09.27}
}

@INPROCEEDINGS{2003-ZarandiMiremadi.etal,
  author = {H. R. Zarandi and S. G. Miremadi and A. Ejlali},
  title = {Fault Injection into Verilog Models for Dependability Evaluation
	of Digital Systems},
  booktitle = {Proc. Second International Symposium on Parallel and Distributed
	Computing},
  year = {2003},
  pages = {281 - 287},
  month = {October},
  file = {:files/2003-ZarandiMiremadi.pdf:PDF},
  owner = {bartsch},
  timestamp = {2014.07.30}
}

@INPROCEEDINGS{2005-ZaretskyMittal.etal,
  author = {David C. Zaretsky and Gaurav Mittal and Robert Dick and Prith Banerjee},
  title = {Generation Of Control And Data Flow Graphs From Scheduled And Pipelined
	Assembly Code},
  year = {2005},
  file = {:./files/2005-ZaretskyMittal.etal.pdf:PDF},
  timestamp = {2006.09.21}
}

@INPROCEEDINGS{2000-ZedanCan,
  author = {Hussein Zedan And Antonio Can},
  title = {A Logic-Based Approach for Hardware-Software Co-Design},
  booktitle = {IEE Colloquium Hardware-Software Co-Design},
  year = {2000},
  number = {111},
  pages = {4-4},
  file = {:./files/2000-ZedanCan.pdf:PDF},
  keywords = {logic-based approach; hardware/software co-design; co-simulation;
	simulation process; formal verification; rapid prototyping; formal
	techniques; integrated support; AnaTempura; Interval Temporal Logic;
	safety; liveness; timeliness},
  url = {http://link.aip.org/link/abstract/IEESEM/v2000/i111/p4/s1}
}

@INPROCEEDINGS{1999-ChaohuangSaxena.etal,
  author = {Chaohuang Zeng and Saxena, N. and McCluskey, E.J.},
  title = {Finite State Machine Synthesis With Concurrent Error Detection},
  booktitle = {Test Conference, 1999. Proceedings. International},
  year = {1999},
  pages = {672 -679},
  file = {:./files/1999-ChaohuangSaxena.etal.pdf:PDF},
  keywords = {JEDI program;MCNC'89 FSM benchmark circuits;bistable elements;combinational
	circuit;concurrent error detection;design choices;finite state machine
	synthesis;multi-parity-group technique;next-state logic;on-line parity
	checking;output logic;parity prediction circuits;reduction in literal
	counts;self-checking FSM;sequential circuit synthesis;single-parity-group
	technique;state assignment;state diagram;state encoding technique;built-in
	self test;combinational circuits;error detection codes;finite state
	machines;logic CAD;sequential circuits;state assignment;}
}

@INPROCEEDINGS{2001-ZengCiesielski.etal,
  author = {Z. Zeng and M. Ciesielski and B. Rouzeyre},
  title = {Functional Test Generation using Constraint Logic Programming},
  booktitle = {Proc. International Federation for Information Processing, International
	Conference on Very Large Scale Integration ({IFIP} {VLSI-SOC})},
  year = {2001},
  pages = {375--387},
  address = {Montpellier, France},
  file = {:./files/2001-ZengCiesielski.etal.pdf:PDF}
}

@INPROCEEDINGS{2001-ZengKalla.etal,
  author = {Z. Zeng and P. Kalla and M. Ciesielski},
  title = {{LPSAT}: A Unified Approach to {RTL} Satisfiability},
  booktitle = {Proc. International Conference on Design, Automation and Test in
	Europe ({DATE})},
  year = {2001},
  pages = {398 -402},
  address = {Munich, Germany},
  month = {March},
  file = {:./files/2001-ZengKalla.etal.pdf:PDF},
  keywords = {LP-based comprehensive infrastructure;LPSAT;MILP solver;RTL satisfiability;bit-level
	{Boolean} logic;complex RTL designs;constraint propagation;constraints
	modeling;mixed integer linear program;satisfiability problem;unified
	approach;word-level arithmetic operators;{Boolean} functions;computability;constraint
	handling;integer programming;linear programming;logic CAD;logic partitioning;}
}

@INPROCEEDINGS{2005-YapingStrojwas.etal,
  author = {Yaping Zhan and Strojwas, A.J. and Sharma, M. and Newmark, D.},
  booktitle = {Computer-Aided Design, 2005. {ICCAD}-2005. {IEEE/ACM} International
	Conference on},
  year = {2005},
  pages = { 699 - 704},
  month = {nov.},
  file = {:./files/2005-YapingStrojwas.etal.pdf:PDF},
  keywords = { block-based statistical timing tool; circuit performance; nanometer
	IC technology; process variations; statistical critical path analysis;
	statistical nonlinear delay model; timing verification; VLSI; critical
	path analysis; delay estimation; integrated circuit design; integrated
	circuit technology; nanoelectronics; network analysis; statistical
	analysis;}
}

@ARTICLE{2015-ZhangWang.etal,
  author = {Zhang, Danfeng and Wang, Yao and Suh, G Edward and Myers, Andrew
	C},
  title = {A hardware design language for timing-sensitive information-flow
	security},
  journal = {ACM SIGPLAN Notices},
  year = {2015},
  volume = {50},
  pages = {503--516},
  number = {4},
  owner = {fadiheh},
  publisher = {ACM},
  timestamp = {2018.07.13}
}

@ARTICLE{2006-ZhangMishchenko.etal,
  author = {Zhang, J.S. and Chrzanowska-Jeske, M. and Mishchenko, A. and Burch,
	J.R.},
  title = {Linear Cofactor Relationships in {Boolean} Functions},
  journal = {Computer-Aided Design of Integrated Circuits and Systems, {IEEE}
	Transactions on},
  year = {2006},
  volume = {25},
  pages = {1011 -1023},
  number = {6},
  month = {june },
  file = {:./files/2006-ZhangMishchenko.etal.pdf:PDF},
  issn = {0278-0070},
  keywords = {{Boolean} functions;{Boolean} matching;classical symmetries;decision
	diagrams;layout-friendly logic circuits;linear cofactor relationships;logic
	synthesis;single-variable symmetries;support-reducing bound sets;{Boolean}
	functions;logic circuits;logic design;}
}

@INPROCEEDINGS{2001-ZhangMadigan.etal,
  author = {Lintao Zhang and Conor F. Madigan and Matthew W. Moskewicz and Sharad
	Malik},
  title = {Efficient Conflict Driven Learning in {Boolean} Satisfiability Solver},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2001},
  pages = {279-285},
  file = {:./files/2001-ZhangMadigan.etal.pdf:PDF}
}

@INPROCEEDINGS{2002-ZhangMalik,
  author = {Zhang, Lintao and Malik, Sharad},
  title = {The Quest for Efficient Boolean Satisfiability Solvers},
  booktitle = {Proceedings of the 14th International Conference on Computer Aided
	Verification},
  year = {2002},
  series = {CAV '02},
  pages = {17--36},
  address = {London, UK, UK},
  publisher = {Springer-Verlag},
  acmid = {734434},
  isbn = {3-540-43997-8},
  numpages = {20}
}

@INPROCEEDINGS{2005-ZhongWong,
  author = {Yu Zhong and Martin D. F. Wong},
  title = {Fast Algorithms for {IR} Drop Analysis in Large Power Grid},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2005},
  pages = { 351 - 357},
  file = {:./files/2005-ZhongWong.pdf:PDF},
  keywords = { 19.6 hours; 26.47 mins; 5.7 mV; IR drop analysis; fast algorithms;
	iterative algorithms; large power grid; linear system; node-by-node
	traversals; random-walk-based algorithm; row-based algorithm; row-by-row
	traversals; successive over relaxation iterative method; VLSI; electric
	potential; iterative methods; linear systems; power supply circuits;
	random processes;},
  timestamp = {2006.09.27}
}

@ARTICLE{2006-ZhouMohanram,
  author = {Quming Zhou and K. Mohanram},
  title = {Gate sizing to radiation harden combinational logic},
  journal = {IEEE Transactions on Computer-Aided Design of Integrated Circuits
	and Systems},
  year = {2006},
  volume = {25},
  pages = {155-166},
  number = {1},
  month = {January},
  file = {2006-ZhouMohanram.pdf:files/2006-ZhouMohanram.pdf:PDF},
  issn = {0278-0070},
  owner = {bartsch},
  timestamp = {2016.09.21}
}

@INPROCEEDINGS{2005-ZhouYao.etal,
  author = {Shuo Zhou and Bo Yao and Hongyu Chen and Yi Zhu and Mike Hutton and
	Truman Collins and Sridhar Srinivasan,},
  title = {Improving the Efficiency of Static Timing Analysis with False Paths},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2005},
  pages = { 527 - 531},
  file = {:./files/2005-ZhouYao.etal.pdf:PDF},
  keywords = { NP complete; biclique covering; bipartite graph; false path; false
	sub-graphs; static timing analysis; tag minimization; circuit analysis
	computing; circuit optimisation; timing;},
  timestamp = {2006.09.27}
}

@INPROCEEDINGS{1999-ZhuGajski,
  author = {Jianwen Zhu and Daniel D. Gajski},
  title = {A Retargetable, Ultra-fast Instruction Set Simulator},
  booktitle = {Proc. International Conference on Design, Automation and Test in
	Europe ({DATE})},
  year = {1999},
  pages = {298 -302},
  file = {:./files/1999-ZhuGajski.pdf:PDF},
  timestamp = {2006.09.27}
}

@INPROCEEDINGS{2005-Zhu,
  author = {Y. Zhu},
  title = {Applying formal techniques in simulation-based verification},
  booktitle = {Proc. International Conference On {ASIC} ({ASICON})},
  year = {2005},
  volume = {2},
  pages = {1036 -1041},
  address = {Shanghai, China},
  month = {October},
  comment = {Read it IN},
  file = {:./files/2005-Zhu.pdf:PDF},
  keywords = {data independence;debugging overhead;formal verification;functional
	verification;hardware verification;formal verification;integrated
	circuit design;},
  owner = {wedler}
}

@INPROCEEDINGS{2005-ZhuWhite,
  author = {Zhenhai Zhu and Jacob White},
  title = {FastSies: A Fast Stochastic Integral Equation Solver for Modeling
	the Rough Surface Effect},
  booktitle = {Proc. International Conference on Computer-Aided Design ({ICCAD})},
  year = {2005},
  pages = { 675 - 682},
  file = {:./files/2005-ZhuWhite.pdf:PDF},
  keywords = { 3D interconnects; fast stochastic integral equation solver; random
	surface roughness; rough surface effect; sparsification techniques;
	integral equations; integrated circuit interconnections; rough surfaces;
	stochastic processes; surface roughness;},
  timestamp = {2006.09.27}
}

@ARTICLE{2004-ziadeayoubi.etal,
  author = {Haissam Ziade and Rafic Ayoubi and Raoul Velazco},
  title = {A Survey on Fault Injection Techniques},
  journal = {The International Arab Journal of Information Technology},
  year = {2004},
  volume = {1},
  number = {2},
  month = {July},
  file = {:import/var/jabref/files/2004-ziadeayoubi.etal.pdf:PDF},
  owner = {bschmidt},
  timestamp = {2014.07.29}
}

@BOOK{1999-AptMarek.etal,
  title = {The Logic Programming Paradigm A 25-Year Perspective},
  publisher = {Springer},
  year = {1999},
  editor = {K. R. Apt and V. W. Marek and M. Truszczynski and D. S. Warren}
}

@BOOK{2009-BiereHeule.etal,
  title = {Handbook of Satisfiability},
  publisher = {IOS Press},
  year = {2009},
  editor = {Biere, Armin and Heule, Marijn J. H. and van Maaren, Hans and Walsh,
	Toby},
  volume = {185},
  pages = {980},
  series = {Frontiers in Artificial Intelligence and Applications},
  month = {February},
  file = {:./files/2009-BiereHeule.etal.pdf:PDF},
  isbn = {978-1-58603-929-5},
  issn = {0922-6389},
  owner = {pavlenko},
  timestamp = {2010.02.25}
}

@PROCEEDINGS{2010-EsparzaMajumdar,
  title = {Tools and Algorithms for the Construction and Analysis of Systems,
	16th International Conference, TACAS 2010},
  year = {2010},
  editor = {Javier Esparza and Rupak Majumdar},
  volume = {6015},
  series = {Lecture Notes in Computer Science},
  publisher = {Springer},
  bibsource = {DBLP, http://dblp.uni-trier.de},
  isbn = {978-3-642-12001-5},
  owner = {pavlenko},
  timestamp = {2010.07.26}
}

@PROCEEDINGS{1995-FulopGecseg,
  title = {Automata, Languages and Programming, 22nd International Colloquium,
	{ICALP95}, Szeged, Hungary, July 10-14, 1995, Proceedings},
  year = {1995},
  editor = {Zolt{\'a}n F{\"u}l{\"o}p and Ferenc G{\'e}cseg},
  volume = {944},
  series = {Lecture Notes in Computer Science},
  publisher = {Springer},
  bibsource = {DBLP, http://dblp.uni-trier.de},
  booktitle = {ICALP},
  isbn = {3-540-60084-1},
  owner = {pavlenko},
  timestamp = {2011.06.03}
}

@BOOK{2002-HassounSasao,
  title = {Logic Synthesis and Verification},
  publisher = {Kluwer Academic Publishers},
  year = {2002},
  editor = {S. Hassoun and T. Sasao}
}

@BOOK{1994-MayohTyugu.etal,
  title = {Constraint Programming},
  publisher = {Springer},
  year = {1994},
  editor = {B. Mayoh and E. Tyugu and J. Penjam}
}

@MISC{std-systemverilog,
  title = {{IEEE} 1800 -- Standard for {S}ystem{V}erilog--Unified Hardware Design,
	Specification, and Verification Language},
  institution = {{1800 WG} - {S}ystem{V}erilog Language Working Group},
  organization = {IEEE},
  owner = {stoffel},
  timestamp = {2016.05.11}
}

@MISC{web_coware,
  title = {Co-Ware Inc.},
  key = {coware},
  owner = {stoffel},
  timestamp = {2016.05.11},
  url = {http://www.coware.com}
}

@MISC{web_lisa,
  title = {Co-Ware Processor Designer},
  key = {lisa},
  keywords = {Coware Processor Designer},
  owner = {stoffel},
  timestamp = {2016.05.11},
  url = {http://coware.com/products/processordesigner.php}
}

@MISC{web_moores_interview,
  title = {Excerpts from a Conversation with Gordon Moore: Moore's Law},
  file = {Excepts_A_Conversation_with_Gordon_Moore.pdf:/import/var/jabref/Excepts_A_Conversation_with_Gordon_Moore.pdf:PDF},
  owner = {pavlenko},
  timestamp = {2011.02.08},
  url = {ftp://download.intel.com/museum/Moores_Law/Video-transcripts/Excepts_A_Conversation_with_Gordon_Moore.pdf}
}

@MISC{web_res,
  title = {The {{RES}} file format},
  owner = {marx},
  timestamp = {2012.11.09},
  url = {http://users.soe.ucsc.edu/~avg/ProofChecker/ProofChecker-fileformat.txt}
}

@MISC{web_rup,
  title = {The {{RUP}} file format},
  owner = {marx},
  timestamp = {2012.11.09},
  url = {http://www.cse.ucsc.edu/~avg/ProofChecker/fileformat\_rup.txt}
}

@MISC{web-descam,
  title = {{DeSCAM}},
  howpublished = {https://github.com/ludwig247/DeSCAM},
  owner = {stoffel},
  timestamp = {2018.05.04}
}

@MISC{web-dlf-interview-upec,
  title = {Deutschlandfunk-Interview},
  howpublished = {\url{https://ondemand-mp3.dradio.de/file/dradio/2019/05/18/prozessor_check_wie_seitenkanal_angriffe_verhindert_werden_dlf_20190518_1645_284608be.mp3}},
  owner = {stoffel},
  timestamp = {2019.07.29},
  url = {\url{https://ondemand-mp3.dradio.de/file/dradio/2019/05/18/prozessor_check_wie_seitenkanal_angriffe_verhindert_werden_dlf_20190518_1645_284608be.mp3}}
}

@MISC{web-eetimes-upec,
  title = {{EETimes} Article},
  howpublished = {\url{https://www.eetimes.com/author.asp?section_id=36&doc_id=1334783}},
  owner = {stoffel},
  timestamp = {2019.07.29},
  url = {\url{https://www.eetimes.com/author.asp?section_id=36&doc_id=1334783}}
}

@MISC{web-focus-upec,
  title = {{FOCUS} News Magazine, {G}ermany},
  howpublished = {\url{http://www.focus.de/wissen/natur/meltdown-und-spectre-auch-einfache-chips-betroffen_id_10500464.html}},
  owner = {stoffel},
  timestamp = {2019.07.29},
  url = {\url{https://www.focus.de/wissen/natur/meltdown-und-spectre-auch-einfache-chips-betroffen_id_10500464.html}}
}

@MISC{web-scam,
  title = {{SCAM}},
  howpublished = {https://github.com/ludwig247/SCAM},
  owner = {stoffel},
  timestamp = {2018.05.04},
  url = {https://github.com/ludwig247/SCAM}
}

@MISC{web-spp-call-sec,
  title = {{SPP} call},
  howpublished = {\url{https://www.dfg.de/foerderung/info_wissenschaft/2019/info_wissenschaft_19_34/}},
  owner = {stoffel},
  timestamp = {2019.07.29},
  url = {\url{https://www.dfg.de/foerderung/info_wissenschaft/2019/info_wissenschaft_19_34/}}
}

@MISC{web-verdict-co-uk-upec,
  title = {Verdict {UK}},
  howpublished = {\url{https://www.verdict.co.uk/chip-security-upec/}},
  owner = {stoffel},
  timestamp = {2019.07.29},
  url = {\url{https://www.verdict.co.uk/chip-security-upec/}}
}

@MISC{2012-vlsi-vs1053b-datasheet,
  title = {Datasheet VLSI VS1053b MP3 decoder chip},
  year = {2012},
  owner = {bschmidt},
  timestamp = {2014.06.27}
}

@MISC{web-systemc-standard,
  title = {IEEE Standard for Standard SystemC Language Reference Manual},
  month = {Jan},
  year = {2012},
  journal = {IEEE Std 1666-2011 (Revision of IEEE Std 1666-2005)}
}

@ARTICLE{2011-SystemC,
  title = {Standard {SystemC} Language Reference Manual},
  journal = {{IEEE} Std 1666-2011},
  year = {2011},
  owner = {joakim},
  timestamp = {2013.07.25}
}

@MISC{2009a,
  title = {International Technology Roadmap for Semiconductors},
  year = {2009},
  owner = {stoffel},
  timestamp = {2016.05.10}
}

@ARTICLE{2005-PSL,
  title = {{IEEE Standard for {Property Specification Language} (PSL)}},
  journal = {{IEEE} Std 1850-2005},
  year = {2005},
  owner = {joakim},
  timestamp = {2013.01.01},
  url = {http://www.eda.org/ieee-1850/}
}

@MISC{1995-PCI,
  title = {{PCI} Local Bus Specification 2.1},
  howpublished = {http://www.pcisig.com/specifications},
  year = {1995},
  owner = {stoffel},
  timestamp = {2016.05.11},
  url = {http://www.pcisig.com/specifications}
}

@PROCEEDINGS{1994-DBLP,
  title = {Proceedings 1994 {IEEE} International Conference on Computer Design:
	{VLSI} in Computer {\&} Processors, {ICCD} '94, Cambridge, {MA},
	{USA}, October 10-12, 1994},
  year = {1994},
  publisher = {IEEE Computer Society},
  bibsource = {DBLP, http://dblp.uni-trier.de},
  isbn = {0-8186-6565-3},
  owner = {pavlenko},
  timestamp = {2011.06.03},
  url = {http://www.dblp.org/db/conf/iccd/iccd1994.html}
}

@MISC{TCL_TK_WWW,
  title = {{T}ool {c}ommand {l}anguage},
  year = {1988},
  owner = {bschmidt},
  timestamp = {2014.02.21},
  url = {http://www.tcl.tk}
}

@comment{jabref-meta: databaseType:biblatex;}

@comment{jabref-meta: selector_Booktitle:Proc. 6. International Confer
ence On ASIC (ASICON 2005) ;}

@article{UART,
author = {Ali, Md. Liakot and Sidek, Roslina and Aris, Ishak and Mohd Ali, Mohd and Suparjo, Bambang},
year = {2004},
month = {06},
pages = {257-268},
title = {Design of a micro-UART for SoC application},
volume = {30},
journal = {Computers & Electrical Engineering},
doi = {10.1016/j.compeleceng.2003.01.002}
}

@INPROCEEDINGS{1594726,
  author={Man-Yun Su and Che-Hua Shih and Juinn-Dar Huang and Jing-Yang Jou},
  booktitle={Asia and South Pacific Conference on Design Automation, 2006.}, 
  title={FSM-based transaction-level functional coverage for interface compliance verification}, 
  year={2006},
  volume={},
  number={},
  pages={6 pp.-},
  doi={10.1109/ASPDAC.2006.1594726}}
  
  
  
  
@ARTICLE{baraza-etal1,
  author={Baraza, Juan-Carlos and Gracia, JoaquÍn and Blanc, Sara and Gil, Daniel and Gil, Pedro-J.},
  journal={IEEE Transactions on Very Large Scale Integration (VLSI) Systems}, 
  title={Enhancement of Fault Injection Techniques Based on the Modification of VHDL Code}, 
  year={2008},
  volume={16},
  number={6},
  pages={693-706},
  doi={10.1109/TVLSI.2008.2000254}}

@INPROCEEDINGS{baraza-etal2,
  author={Baraza, J.C. and Gracia, J. and Gil, D. and Gil, P.J.},
  booktitle={Tenth IEEE International High-Level Design Validation and Test Workshop, 2005.}, 
  title={Improvement of fault injection techniques based on VHDL code modification}, 
  year={2005},
  volume={},
  number={},
  pages={19-26},
  doi={10.1109/HLDVT.2005.1568808}}

@INPROCEEDINGS{mefisto,
  author={Jenn, E. and Arlat, J. and Rimen, M. and Ohlsson, J. and Karlsson, J.},
  booktitle={Proceedings of IEEE 24th International Symposium on Fault- Tolerant Computing}, 
  title={Fault injection into VHDL models: the MEFISTO tool}, 
  year={1994},
  volume={},
  number={},
  pages={66-75},
  doi={10.1109/FTCS.1994.315656}}

@ARTICLE{syfi,
  author={Lee, Dongwoo and Na, Jongwhoa},
  journal={IEEE Design   Test of Computers}, 
  title={A Novel Simulation Fault Injection Method for Dependability Analysis}, 
  year={2009},
  volume={26},
  number={6},
  pages={50-61},
  doi={10.1109/MDT.2009.135}}

@INPROCEEDINGS{gemfi,
  author={Parasyris, Konstantinos and Tziantzoulis, Georgios and Antonopoulos, Christos D. and Bellas, Nikolaos},
  booktitle={2014 44th Annual IEEE/IFIP International Conference on Dependable Systems and Networks}, 
  title={GemFI: A Fault Injection Tool for Studying the Behavior of Applications on Unreliable Substrates}, 
  year={2014},
  volume={},
  number={},
  pages={622-629},
  doi={10.1109/DSN.2014.96}}

@INPROCEEDINGS{genfi,
  author={Kaliorakis, Manolis and Tselonis, Sotiris and Chatzidimitriou, Athanasios and Foutris, Nikos and Gizopoulos, Dimitris},
  booktitle={2015 IEEE International Symposium on Workload Characterization}, 
  title={Differential Fault Injection on Microarchitectural Simulators}, 
  year={2015},
  volume={},
  number={},
  pages={172-182},
  doi={10.1109/IISWC.2015.28}}



@INPROCEEDINGS{bagbaba,
  author={Bagbaba, Ahmet Cagri and Jenihhin, Maksim and Ubar, Raimund and Sauer, Christian},
  booktitle={2020 IEEE 26th International Symposium on On-Line Testing and Robust System Design (IOLTS)}, 
  title={Representing Gate-Level SET Faults by Multiple SEU Faults at RTL}, 
  year={2020},
  volume={},
  number={},
  pages={1-6},
  doi={10.1109/IOLTS50870.2020.9159715}}

@ARTICLE{Thaker,
  author={Thaker, P.A. and Agrawal, V.D. and Zaghloul, M.E.},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems}, 
  title={A test evaluation technique for VLSI circuits using register-transfer level fault modeling}, 
  year={2003},
  volume={22},
  number={8},
  pages={1104-1113},
  doi={10.1109/TCAD.2003.814958}}

@INPROCEEDINGS{Corno,
  author={Corno, F. and Cumani, G. and Sonza Reorda, M. and Squillero, G.},
  booktitle={Proceedings IEEE International High-Level Design Validation and Test Workshop (Cat. No.PR00786)}, 
  title={An RT-level fault model with high gate level correlation}, 
  year={2000},
  volume={},
  number={},
  pages={3-8},
  doi={10.1109/HLDVT.2000.889551}}

@INPROCEEDINGS{Hayne,
  author={Hayne, R.J. and Johnson, B.W.},
  booktitle={Proceedings 17th IEEE VLSI Test Symposium (Cat. No.PR00146)}, 
  title={Behavioral fault modeling in a VHDL synthesis environment}, 
  year={1999},
  volume={},
  number={},
  pages={333-340},
  doi={10.1109/VTEST.1999.766684}}

@Misc{Yosys,
	author =   {Yosys},
	title =    {{Yosys}},
	howpublished = {\url{http://www.clifford.at/yosys/}},
	url = {\url{http://www.clifford.at/yosys/}},
	timestamp = {[Online: Accessed 27.May.2021]}
	}

@Misc{Verilator,
	author =   {{Verilator}},
	title =    {{Verilator}},
	note = {\url{https://www.veripool.org/verilator/}},
	note = "[Online: Accessed 27.May.2021]",}

@Misc{ISE,
	author =   {{Xilinx}},
	title =    {{ISE Design Suite}},
	note = {\url{https://www.xilinx.com/products/design-tools/ise-design-suite.html}},
	note = "[Online: Accessed 27.May.2021]",}

@Misc{Xcelium,
	author =   {{Cadence Design Systems}},
	title =    {{Xcelium Logic Simulation}},
	note = {\url{https://www.cadence.com/ko_KR/home/tools/system-design-and-verification/simulation-and-testbench-verification/xcelium-simulator.html}},
	note = "[Online: Accessed 27.May.2021]",}
	
@MISC{ISO26262,
  title =    {{Road vehicles — Functional safety — Part 11: Guidelines on application of ISO 26262 to semiconductors}},
  howpublished = {\url{https://www.iso.org/obp/ui/#iso:std:iso:26262:-11:ed-1:v1:en}},
  owner = {stoffel},
  timestamp = {Online: Accessed 07.June.2021},
  url = {\url{https://www.iso.org/obp/ui/#iso:std:iso:26262:-11:ed-1:v1:en}}
}

@ARTICLE{MOZART,
  author={Gai, S. and Montessoro, P.L. and Somenzi, F.},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems}, 
  title={MOZART: a concurrent multilevel simulator}, 
  year={1988},
  volume={7},
  number={9},
  pages={1005-1016},
  doi={10.1109/43.7799}}

@INPROCEEDINGS{Lentz,
  author={Lentz, K.P. and Homer, J.B.},
  booktitle={Proceedings 33rd Annual Simulation Symposium (SS 2000)}, 
  title={Handling behavioral components in multi-level concurrent fault simulation}, 
  year={2000},
  volume={},
  number={},
  pages={149-156},
  doi={10.1109/SIMSYM.2000.844911}}

@INPROCEEDINGS{Kochte,
  author={Kochte, Michael A. and Zoellin, Christian G. and Baranowski, Rafal and Imhof, Michael E. and Wunderlich, Hans-Joachim and Hatami, Nadereh and Carlo, Stefano Di and Prinetto, Paolo},
  booktitle={2010 19th IEEE Asian Test Symposium}, 
  title={Efficient Simulation of Structural Faults for the Reliability Evaluation at System-Level}, 
  year={2010},
  volume={},
  number={},
  pages={3-8},
  doi={10.1109/ATS.2010.10}}

@Misc{Tabacaru,
author = {Tabacaru, Bogdan-Andrei},
year = {2019},
month = {12},
pages = {},
howpublished= "\url{https://mediatum.ub.tum.de/doc/1471529/1471529.pdf}",
title = {{On Fault-Effect Analysis at the Virtual-Prototype Abstraction Level}},
note 		 = "[Online: Accessed on 20.May.2020]"
}

@INPROCEEDINGS{Oetjens,
  author={Oetjens, J.-H. and Bannow, N. and Becker, M. and Bringmann, O. and Burger, A. and Chaari, M. and Chakraborty, S. and Drechsler, R. and Ecker, W. and Grüttner, K. and Kruse, Th. and Kuznik, C. and Le, H. M. and Mauderer, A. and Müller, W. and Müller-Gritschneder, D. and Poppen, F. and Post, H. and Reiter, S. and Rosenstiel, W. and Roth, S. and Schlichtmann, U. and von Schwerin, A. and Tabacaru, B.-A. and Viehl, A.},
  booktitle={2014 51st ACM/EDAC/IEEE Design Automation Conference (DAC)}, 
  title={Safety evaluation of automotive electronics using Virtual Prototypes: State of the art and research challenges}, 
  year={2014},
  volume={},
  number={},
  pages={1-6},
  doi={10.1145/2593069.2602976}}
  
@INPROCEEDINGS{Espinosa,
  author={Espinosa, Jaime and Hernandez, Carles and Abella, Jaume and de Andres, David and Ruiz, Juan Carlos},
  booktitle={2015 52nd ACM/EDAC/IEEE Design Automation Conference (DAC)}, 
  title={Analysis and RTL correlation of instruction set simulators for automotive microcontroller robustness verification}, 
  year={2015},
  volume={},
  number={},
  pages={1-6},
  doi={10.1145/2744769.2744798}}

@ARTICLE{Hwang,
  author={Shih-Arn Hwang and Jin-Hua Hong and Cheng-Wen Wu},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems}, 
  title={Sequential circuit fault simulation using logic emulation}, 
  year={1998},
  volume={17},
  number={8},
  pages={724-736},
  doi={10.1109/43.712103}}
  
  
  @INPROCEEDINGS{permanent_fault,
  author={Henkel, Jörg and Bauer, Lars and Dutt, Nikil and Gupta, Puneet and Nassif, Sani and Shafique, Muhammad and Tahoori, Mehdi and Wehn, Norbert},
  booktitle={2013 50th ACM/EDAC/IEEE Design Automation Conference (DAC)}, 
  title={Reliable on-chip systems in the nano-era: Lessons learnt and future trends}, 
  year={2013},
  volume={},
  number={},
  pages={1-10},
  doi={10.1145/2463209.2488857}}
  
  
@inproceedings{transient_fault,
author = {Herkersdorf, Andreas and Engel, Michael and Glaß, Michael and Henkel, Jörg and Kleeberger, Veit and Kochte, Michael and Kühn, Johannes and Nassif, Sani and Rauchfuss, Holm and Rosenstiel, Wolfgang and Schlichtmann, Ulf and Shafique, Muhammad and Tahoori, Mehdi and Teich, Jürgen and Wehn, Norbert and Weis, Christian and Wunderlich, Hans-Joachim},
year = {2013},
month = {03},
pages = {},
title = {Cross-Layer Dependability Modeling and Abstraction in System on Chip}
}

@INPROCEEDINGS{arlat,
  author={Arlat, J. and Crouzet, Y. and Laprie, J.-C.},
  booktitle={[1989] The Nineteenth International Symposium on Fault-Tolerant Computing. Digest of Papers}, 
  title={Fault injection for dependability validation of fault-tolerant computing systems}, 
  year={1989},
  volume={},
  number={},
  pages={348-355},
  doi={10.1109/FTCS.1989.105591}}
 
@article{ziade,
author = {Ziade, Haissam and Ayoubi, Rafic and Velazco, R.},
year = {2004},
month = {01},
pages = {171-186},
title = {A Survey on Fault Injection Techniques},
volume = {1},
journal = {Int. Arab J. Inf. Technol.}
}


@INPROCEEDINGS{kaja,
  author={Kaja, Endri and Gerlin, Nicolas and Vaddeboina, Mounika and Rivas, Luis and Prebeck, Sebastian and Han, Zhao and Devarajegowda, Keerthikumara and Ecker, Wolfgang},
  booktitle={2021 IEEE International Symposium on Defect and Fault Tolerance in VLSI and Nanotechnology Systems (DFT)}, 
  title={Towards Fault Simulation at Mixed Register-Transfer/Gate-Level Models}, 
  year={2021},
  volume={},
  number={},
  pages={1-6},
  doi={10.1109/DFT52944.2021.9568310}}

@ARTICLE{Breuer,
  author={Breuer, M.A.},
  journal={IEEE Transactions on Computers}, 
  title={The Effects of Races, Delays, and Delay Faults on Test Generation}, 
  year={1974},
  volume={C-23},
  number={10},
  pages={1078-1092},
  doi={10.1109/T-C.1974.223808}}
  
@INPROCEEDINGS{Luong,
  author={Luong, G.M. and Walker, D.M.H.},
  booktitle={Proceedings International Test Conference 1996. Test and Design Validity}, 
  title={Test generation for global delay faults}, 
  year={1996},
  volume={},
  number={},
  pages={433-442},
  doi={10.1109/TEST.1996.557048}}

@ARTICLE{Malaiya,
  author={Malaiya, Yashwant K. and Narayanaswamy, Ramesh},
  journal={IEEE Design   Test of Computers}, 
  title={Modeling and Testing for Timing Faults in Synchronous Sequential Circuits}, 
  year={1984},
  volume={1},
  number={4},
  pages={62-74},
  doi={10.1109/MDT.1984.5005692}}

@ARTICLE{Baumann,
  author={Baumann, R.C.},
  journal={IEEE Transactions on Device and Materials Reliability}, 
  title={Radiation-induced soft errors in advanced semiconductor technologies}, 
  year={2005},
  volume={5},
  number={3},
  pages={305-316},
  doi={10.1109/TDMR.2005.853449}}
  
@inbook{Ecker_MM,
author = {Ecker, Wolfgang and Schreiner, Johannes},
year = {2016},
month = {01},
pages = {1-41},
title = {Metamodeling and Code Generation in the Springer Science+Business Media Dordrecht},
doi = {10.1007/978-94-017-7358-4_32-1}
}

@INPROCEEDINGS{SFI,
  author={Leveugle, R. and Calvez, A. and Maistri, P. and Vanhauwaert, P.},
  booktitle={2009 Design, Automation   Test in Europe Conference   Exhibition}, 
  title={Statistical fault injection: Quantified error and confidence}, 
  year={2009},
  volume={},
  number={},
  pages={502-506},
  doi={10.1109/DATE.2009.5090716}}

@INPROCEEDINGS{Pravadelli,
  author={Ferraretto, Davide and Pravadelli, Graziano},
  booktitle={2015 16th Latin-American Test Symposium (LATS)}, 
  title={Efficient fault injection in QEMU}, 
  year={2015},
  volume={},
  number={},
  pages={1-6},
  doi={10.1109/LATW.2015.7102401}}


@INPROCEEDINGS{Kammler,
  author={Kammler, David and Guan, Junqing and Ascheid, Gerd and Leupers, Rainer and Meyr, Heinrich},
  booktitle={2009 Third IEEE International Conference on Secure Software Integration and Reliability Improvement}, 
  title={A Fast and Flexible Platform for Fault Injection and Evaluation in Verilog-Based Simulations}, 
  year={2009},
  volume={},
  number={},
  pages={309-314},
  doi={10.1109/SSIRI.2009.38}}
  

@INPROCEEDINGS{Rosa,
  author={Rosa, Felipe and Kastensmidt, Fernanda and Reis, Ricardo and Ost, Luciano},
  booktitle={2015 IEEE International Symposium on Defect and Fault Tolerance in VLSI and Nanotechnology Systems (DFTS)}, 
  title={A fast and scalable fault injection framework to evaluate multi/many-core soft error reliability}, 
  year={2015},
  volume={},
  number={},
  pages={211-214},
  doi={10.1109/DFT.2015.7315164}}

@ARTICLE{Magnusson,
  author={Magnusson, P.S. and Christensson, M. and Eskilson, J. and Forsgren, D. and Hallberg, G. and Hogberg, J. and Larsson, F. and Moestedt, A. and Werner, B.},
  journal={Computer}, 
  title={Simics: A full system simulation platform}, 
  year={2002},
  volume={35},
  number={2},
  pages={50-58},
  doi={10.1109/2.982916}}

@INPROCEEDINGS{Zarandi,
  author={Zarandi, H.R. and Miremadi, S.G. and Ejlali, A.},
  booktitle={Proceedings 18th IEEE Symposium on Defect and Fault Tolerance in VLSI Systems}, 
  title={Dependability analysis using a fault injection tool based on synthesizability of HDL models}, 
  year={2003},
  volume={},
  number={},
  pages={485-492},
  doi={10.1109/DFTVS.2003.1250147}}
